Revisiting Weight Averaging for Model Merging

Model merging aims to build a multi-task learner by combining the parameters of individually fine-tuned models without additional training. While a straightforward approach is to average model parameters across tasks, this often results in suboptimal performance due to interference among parameters across tasks. In this paper, we present intriguing results that weight averaging implicitly induces task vectors centered around the weight averaging itself and that applying a low-rank approximation to these centered task vectors significantly improves merging performance. Our analysis shows that centering the task vectors effectively reduces task interference and most of task-specific knowledge is concentrated in the top singular vectors. Our method demonstrates robust and scalable performance on vision benchmarks across varying numbers of tasks and model sizes. Furthermore, we observe that our approach is applicable to natural language processing tasks with competitive performance.

==> sec/backups/2024_research_bib <==
@online{01000000JobRay,
  title = {01000000 | {{Job}} | {{Ray Dashboard}}},
  url = {http://localhost:8265/#/jobs/01000000},
  urldate = {2024-03-18},
  keywords = {notion}
}

@misc{08_gnnPdf,
  title = {08\_gnn.Pdf},
  file = {Y:\paper\textbook\2022 AI exp lab\08_gnn.pdf}
}

@misc{09_meta_learningPdf,
  title = {09\_meta\_learning.Pdf},
  file = {Y:\paper\textbook\2022 AI exp lab\09_meta_learning.pdf}
}

@misc{10_gan_ansPdf,
  title = {10\_gan\_ans.Pdf},
  file = {C:\Users\chsey\Zotero\storage\ZZ39QBTT\10_gan_ans.pdf}
}

@online{150504597UNet,
  title = {[1505.04597] {{U-Net}}: {{Convolutional Networks}} for {{Biomedical Image Segmentation}}},
  url = {https://arxiv.org/abs/1505.04597},
  urldate = {2022-12-09},
  file = {C:\Users\chsey\Zotero\storage\ZN2D29FT\1505.html}
}

@online{210303231DONeRF,
  title = {[2103.03231] {{DONeRF}}: {{Towards Real-Time Rendering}} of {{Compact Neural Radiance Fields}} Using {{Depth Oracle Networks}}},
  url = {https://arxiv.org/abs/2103.03231},
  urldate = {2023-01-25},
  file = {C:\Users\chsey\Zotero\storage\3Q6J4HIF\2103.html}
}

@online{230601708TIESMergingResolving,
  title = {[2306.01708] {{TIES-Merging}}: {{Resolving Interference When Merging Models}}},
  url = {https://arxiv.org/abs/2306.01708},
  urldate = {2024-10-26},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\ZKHJA5WF\2306.html}
}

@online{abbasSharpMAMLSharpnessAwareModelAgnostic2022,
  title = {Sharp-{{MAML}}: {{Sharpness-Aware Model-Agnostic Meta Learning}}},
  shorttitle = {Sharp-{{MAML}}},
  author = {Abbas, Momin and Xiao, Quan and Chen, Lisha and Chen, Pin-Yu and Chen, Tianyi},
  date = {2022-08-14},
  eprint = {2206.03996},
  eprinttype = {arXiv},
  eprintclass = {cs, eess, math, stat},
  doi = {10.48550/arXiv.2206.03996},
  url = {http://arxiv.org/abs/2206.03996},
  urldate = {2023-07-05},
  abstract = {Model-agnostic meta learning (MAML) is currently one of the dominating approaches for few-shot meta-learning. Albeit its effectiveness, the optimization of MAML can be challenging due to the innate bilevel problem structure. Specifically, the loss landscape of MAML is much more complex with possibly more saddle points and local minimizers than its empirical risk minimization counterpart. To address this challenge, we leverage the recently invented sharpness-aware minimization and develop a sharpness-aware MAML approach that we term Sharp-MAML. We empirically demonstrate that Sharp-MAML and its computation-efficient variant can outperform the plain-vanilla MAML baseline (e.g., \$+3\textbackslash\%\$ accuracy on Mini-Imagenet). We complement the empirical study with the convergence rate analysis and the generalization bound of Sharp-MAML. To the best of our knowledge, this is the first empirical and theoretical study on sharpness-aware minimization in the context of bilevel learning. The code is available at https://github.com/mominabbass/Sharp-MAML.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Electrical Engineering and Systems Science - Systems and Control,Mathematics - Optimization and Control,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Abbas et al_2022_Sharp-MAML.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AH9GZYU5\\2206.html}
}

@article{abdiPanoramicDentalXrays2020,
  title = {Panoramic {{Dental X-rays With Segmented Mandibles}}},
  author = {Abdi, Amir and Kasaei, Shohreh},
  date = {2020-07-02},
  volume = {2},
  publisher = {Mendeley Data},
  doi = {10.17632/hxt48yk462.2},
  url = {https://data.mendeley.com/datasets/hxt48yk462/2},
  urldate = {2022-07-09},
  abstract = {This dataset consists of anonymized and deidentified panoramic dental X-rays of 116 patients, taken at Noor Medical Imaging Center, Qom, Iran. The subjects cover a wide range of dental conditions from healthy, to partial and complete edentulous cases. The mandibles of all cases are manually segmented by two dentists. This dataset is used as the basis for the article by Abdi et al [1]. [1] A. H. Abdi, S. Kasaei, and M. Mehdizadeh, “Automatic segmentation of mandible in panoramic x-ray,” J. Med. Imaging, vol. 2, no. 4, p. 44003, 2015.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\SVDN2RM9\2.html}
}

@online{achilleTask2VecTaskEmbedding2019,
  title = {{{Task2Vec}}: {{Task Embedding}} for {{Meta-Learning}}},
  shorttitle = {{{Task2Vec}}},
  author = {Achille, Alessandro and Lam, Michael and Tewari, Rahul and Ravichandran, Avinash and Maji, Subhransu and Fowlkes, Charless and Soatto, Stefano and Perona, Pietro},
  date = {2019-02-10},
  eprint = {1902.03545},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1902.03545},
  url = {http://arxiv.org/abs/1902.03545},
  urldate = {2023-11-21},
  abstract = {We introduce a method to provide vectorial representations of visual classification tasks which can be used to reason about the nature of those tasks and their relations. Given a dataset with ground-truth labels and a loss function defined over those labels, we process images through a "probe network" and compute an embedding based on estimates of the Fisher information matrix associated with the probe network parameters. This provides a fixed-dimensional embedding of the task that is independent of details such as the number of classes and does not require any understanding of the class label semantics. We demonstrate that this embedding is capable of predicting task similarities that match our intuition about semantic and taxonomic relations between different visual tasks (e.g., tasks based on classifying different types of plants are similar) We also demonstrate the practical value of this framework for the meta-task of selecting a pre-trained feature extractor for a new task. We present a simple meta-learning framework for learning a metric on embeddings that is capable of predicting which feature extractors will perform well. Selecting a feature extractor with task embedding obtains a performance close to the best available feature extractor, while costing substantially less than exhaustively training and evaluating on all available feature extractors.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Achille et al_2019_Task2Vec.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UILDECXE\\1902.html}
}

@article{adilovaLAYERWISELINEARMODE2024,
  title = {{{LAYER-WISE LINEAR MODE CONNECTIVITY}}},
  author = {Adilova, Linara and Andriushchenko, Maksym and Kamp, Michael and Fischer, Asja and Jaggi, Martin},
  date = {2024},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\PMZDH5Z5\Adilova 등 - 2024 - LAYER-WISE LINEAR MODE CONNECTIVITY.pdf}
}

@online{aghajanyanBetterFineTuningReducing2020,
  title = {Better {{Fine-Tuning}} by {{Reducing Representational Collapse}}},
  author = {Aghajanyan, Armen and Shrivastava, Akshat and Gupta, Anchit and Goyal, Naman and Zettlemoyer, Luke and Gupta, Sonal},
  date = {2020-08-05},
  eprint = {2008.03156},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2008.03156},
  urldate = {2024-04-17},
  abstract = {Although widely adopted, existing approaches for fine-tuning pre-trained language models have been shown to be unstable across hyper-parameter settings, motivating recent work on trust region methods. In this paper, we present a simplified and efficient method rooted in trust region theory that replaces previously used adversarial objectives with parametric noise (sampling from either a normal or uniform distribution), thereby discouraging representation change during fine-tuning when possible without hurting performance. We also introduce a new analysis to motivate the use of trust region methods more generally, by studying representational collapse; the degradation of generalizable representations from pre-trained models as they are fine-tuned for a specific end task. Extensive experiments show that our fine-tuning method matches or exceeds the performance of previous trust region methods on a range of understanding and generation tasks (including DailyMail/CNN, Gigaword, Reddit TIFU, and the GLUE benchmark), while also being much faster. We also show that it is less prone to representation collapse; the pre-trained models maintain more generalizable representations every time they are fine-tuned.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Aghajanyan et al_2020_Better Fine-Tuning by Reducing Representational Collapse.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HJVT6IW9\\2008.html}
}

@online{aghajanyanBetterFineTuningReducing2020a,
  title = {Better {{Fine-Tuning}} by {{Reducing Representational Collapse}}},
  author = {Aghajanyan, Armen and Shrivastava, Akshat and Gupta, Anchit and Goyal, Naman and Zettlemoyer, Luke and Gupta, Sonal},
  date = {2020-08-05},
  eprint = {2008.03156},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2008.03156},
  url = {http://arxiv.org/abs/2008.03156},
  urldate = {2024-04-17},
  abstract = {Although widely adopted, existing approaches for fine-tuning pre-trained language models have been shown to be unstable across hyper-parameter settings, motivating recent work on trust region methods. In this paper, we present a simplified and efficient method rooted in trust region theory that replaces previously used adversarial objectives with parametric noise (sampling from either a normal or uniform distribution), thereby discouraging representation change during fine-tuning when possible without hurting performance. We also introduce a new analysis to motivate the use of trust region methods more generally, by studying representational collapse; the degradation of generalizable representations from pre-trained models as they are fine-tuned for a specific end task. Extensive experiments show that our fine-tuning method matches or exceeds the performance of previous trust region methods on a range of understanding and generation tasks (including DailyMail/CNN, Gigaword, Reddit TIFU, and the GLUE benchmark), while also being much faster. We also show that it is less prone to representation collapse; the pre-trained models maintain more generalizable representations every time they are fine-tuned.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Aghajanyan et al_2020_Better Fine-Tuning by Reducing Representational Collapse2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LJDFNZY4\\2008.html}
}

@online{aghajanyanIntrinsicDimensionalityExplains2020,
  title = {Intrinsic {{Dimensionality Explains}} the {{Effectiveness}} of {{Language Model Fine-Tuning}}},
  author = {Aghajanyan, Armen and Zettlemoyer, Luke and Gupta, Sonal},
  date = {2020-12-22},
  eprint = {2012.13255},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2012.13255},
  urldate = {2024-04-17},
  abstract = {Although pretrained language models can be fine-tuned to produce state-of-the-art results for a very wide range of language understanding tasks, the dynamics of this process are not well understood, especially in the low data regime. Why can we use relatively vanilla gradient descent algorithms (e.g., without strong regularization) to tune a model with hundreds of millions of parameters on datasets with only hundreds or thousands of labeled examples? In this paper, we argue that analyzing fine-tuning through the lens of intrinsic dimension provides us with empirical and theoretical intuitions to explain this remarkable phenomenon. We empirically show that common pre-trained models have a very low intrinsic dimension; in other words, there exists a low dimension reparameterization that is as effective for fine-tuning as the full parameter space. For example, by optimizing only 200 trainable parameters randomly projected back into the full space, we can tune a RoBERTa model to achieve 90\textbackslash\% of the full parameter performance levels on MRPC. Furthermore, we empirically show that pre-training implicitly minimizes intrinsic dimension and, perhaps surprisingly, larger models tend to have lower intrinsic dimension after a fixed number of pre-training updates, at least in part explaining their extreme effectiveness. Lastly, we connect intrinsic dimensionality with low dimensional task representations and compression based generalization bounds to provide intrinsic-dimension-based generalization bounds that are independent of the full parameter count.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Aghajanyan et al_2020_Intrinsic Dimensionality Explains the Effectiveness of Language Model.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EI9WAHKG\\2012.html}
}

@inproceedings{aghajanyanIntrinsicDimensionalityExplains2021,
  title = {Intrinsic {{Dimensionality Explains}} the {{Effectiveness}} of {{Language Model Fine-Tuning}}},
  booktitle = {Proceedings of the 59th {{Annual Meeting}} of the {{Association}} for {{Computational Linguistics}} and the 11th {{International Joint Conference}} on {{Natural Language Processing}} ({{Volume}} 1: {{Long Papers}})},
  author = {Aghajanyan, Armen and Gupta, Sonal and Zettlemoyer, Luke},
  editor = {Zong, Chengqing and Xia, Fei and Li, Wenjie and Navigli, Roberto},
  date = {2021-08},
  pages = {7319--7328},
  publisher = {Association for Computational Linguistics},
  location = {Online},
  doi = {10.18653/v1/2021.acl-long.568},
  url = {https://aclanthology.org/2021.acl-long.568},
  urldate = {2024-03-18},
  abstract = {Although pretrained language models can be fine-tuned to produce state-of-the-art results for a very wide range of language understanding tasks, the dynamics of this process are not well understood, especially in the low data regime. Why can we use relatively vanilla gradient descent algorithms (e.g., without strong regularization) to tune a model with hundreds of millions of parameters on datasets with only hundreds or thousands of labeled examples? In this paper, we argue that analyzing fine-tuning through the lens of intrinsic dimension provides us with empirical and theoretical intuitions to explain this remarkable phenomenon. We empirically show that common pre-trained models have a very low intrinsic dimension; in other words, there exists a low dimension reparameterization that is as effective for fine-tuning as the full parameter space. For example, by optimizing only 200 trainable parameters randomly projected back into the full space, we can tune a RoBERTa model to achieve 90\% of the full parameter performance levels on MRPC. Furthermore, we empirically show that pre-training implicitly minimizes intrinsic dimension and, perhaps surprisingly, larger models tend to have lower intrinsic dimension after a fixed number of pre-training updates, at least in part explaining their extreme effectiveness. Lastly, we connect intrinsic dimensionality with low dimensional task representations and compression based generalization bounds to provide intrinsic-dimension-based generalization bounds that are independent of the full parameter count.},
  eventtitle = {{{ACL-IJCNLP}} 2021},
  keywords = {notion},
  file = {Y:\paper\2024_research\Aghajanyan et al_2021_Intrinsic Dimensionality Explains the Effectiveness of Language Model.pdf}
}

@online{aghajanyanScalingLawsGenerative2023,
  title = {Scaling {{Laws}} for {{Generative Mixed-Modal Language Models}}},
  author = {Aghajanyan, Armen and Yu, Lili and Conneau, Alexis and Hsu, Wei-Ning and Hambardzumyan, Karen and Zhang, Susan and Roller, Stephen and Goyal, Naman and Levy, Omer and Zettlemoyer, Luke},
  date = {2023-01-09},
  eprint = {2301.03728},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2301.03728},
  urldate = {2024-05-19},
  abstract = {Generative language models define distributions over sequences of tokens that can represent essentially any combination of data modalities (e.g., any permutation of image tokens from VQ-VAEs, speech tokens from HuBERT, BPE tokens for language or code, and so on). To better understand the scaling properties of such mixed-modal models, we conducted over 250 experiments using seven different modalities and model sizes ranging from 8 million to 30 billion, trained on 5-100 billion tokens. We report new mixed-modal scaling laws that unify the contributions of individual modalities and the interactions between them. Specifically, we explicitly model the optimal synergy and competition due to data and model size as an additive term to previous uni-modal scaling laws. We also find four empirical phenomena observed during the training, such as emergent coordinate-ascent style training that naturally alternates between modalities, guidelines for selecting critical hyper-parameters, and connections between mixed-modal competition and training stability. Finally, we test our scaling law by training a 30B speechtext model, which significantly outperforms the corresponding unimodal models. Overall, our research provides valuable insights into the design and training of mixed-modal generative models, an important new class of unified models that have unique distributional properties.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\9IND2KZF\Aghajanyan 등 - 2023 - Scaling Laws for Generative Mixed-Modal Language M.pdf}
}

@online{agrawalVQAVisualQuestion2016,
  title = {{{VQA}}: {{Visual Question Answering}}},
  shorttitle = {{{VQA}}},
  author = {Agrawal, Aishwarya and Lu, Jiasen and Antol, Stanislaw and Mitchell, Margaret and Zitnick, C. Lawrence and Batra, Dhruv and Parikh, Devi},
  date = {2016-10-26},
  eprint = {1505.00468},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1505.00468},
  url = {http://arxiv.org/abs/1505.00468},
  urldate = {2023-08-05},
  abstract = {We propose the task of free-form and open-ended Visual Question Answering (VQA). Given an image and a natural language question about the image, the task is to provide an accurate natural language answer. Mirroring real-world scenarios, such as helping the visually impaired, both the questions and answers are open-ended. Visual questions selectively target different areas of an image, including background details and underlying context. As a result, a system that succeeds at VQA typically needs a more detailed understanding of the image and complex reasoning than a system producing generic image captions. Moreover, VQA is amenable to automatic evaluation, since many open-ended answers contain only a few words or a closed set of answers that can be provided in a multiple-choice format. We provide a dataset containing \textasciitilde 0.25M images, \textasciitilde 0.76M questions, and \textasciitilde 10M answers (www.visualqa.org), and discuss the information it provides. Numerous baselines and methods for VQA are provided and compared with human performance. Our VQA demo is available on CloudCV (http://cloudcv.org/vqa).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\vision and language\\Agrawal et al_2016_VQA.pdf;C\:\\Users\\chsey\\Zotero\\storage\\68D33F3P\\1505.html}
}

@online{ahnLinearAttentionMaybe2024,
  title = {Linear Attention Is (Maybe) All You Need (to Understand Transformer Optimization)},
  author = {Ahn, Kwangjun and Cheng, Xiang and Song, Minhak and Yun, Chulhee and Jadbabaie, Ali and Sra, Suvrit},
  date = {2024-03-13},
  eprint = {2310.01082},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/2310.01082},
  urldate = {2024-06-01},
  abstract = {Transformer training is notoriously difficult, requiring a careful design of optimizers and use of various heuristics. We make progress towards understanding the subtleties of training Transformers by carefully studying a simple yet canonical linearized shallow Transformer model. Specifically, we train linear Transformers to solve regression tasks, inspired by J. von Oswald et al. (ICML 2023), and K. Ahn et al. (NeurIPS 2023). Most importantly, we observe that our proposed linearized models can reproduce several prominent aspects of Transformer training dynamics. Consequently, the results obtained in this paper suggest that a simple linearized Transformer model could actually be a valuable, realistic abstraction for understanding Transformer optimization.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Mathematics - Optimization and Control,notion},
  file = {C:\Users\chsey\Zotero\storage\V9N2ESQ7\2310.pdf}
}

@online{ainsworthGitReBasinMerging2023,
  title = {Git {{Re-Basin}}: {{Merging Models}} modulo {{Permutation Symmetries}}},
  shorttitle = {Git {{Re-Basin}}},
  author = {Ainsworth, Samuel K. and Hayase, Jonathan and Srinivasa, Siddhartha},
  date = {2023-03-01},
  eprint = {2209.04836},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2209.04836},
  url = {http://arxiv.org/abs/2209.04836},
  urldate = {2024-09-12},
  abstract = {The success of deep learning is due in large part to our ability to solve certain massive non-convex optimization problems with relative ease. Though non-convex optimization is NP-hard, simple algorithms -- often variants of stochastic gradient descent -- exhibit surprising effectiveness in fitting large neural networks in practice. We argue that neural network loss landscapes often contain (nearly) a single basin after accounting for all possible permutation symmetries of hidden units a la Entezari et al. 2021. We introduce three algorithms to permute the units of one model to bring them into alignment with a reference model in order to merge the two models in weight space. This transformation produces a functionally equivalent set of weights that lie in an approximately convex basin near the reference model. Experimentally, we demonstrate the single basin phenomenon across a variety of model architectures and datasets, including the first (to our knowledge) demonstration of zero-barrier linear mode connectivity between independently trained ResNet models on CIFAR-10. Additionally, we identify intriguing phenomena relating model width and training time to mode connectivity. Finally, we discuss shortcomings of the linear mode connectivity hypothesis, including a counterexample to the single basin theory.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Ainsworth et al_2023_Git Re-Basin.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3PZKUQN5\\2209.html}
}

@online{akbariVATTTransformersMultimodal2021,
  title = {{{VATT}}: {{Transformers}} for {{Multimodal Self-Supervised Learning}} from {{Raw Video}}, {{Audio}} and {{Text}}},
  shorttitle = {{{VATT}}},
  author = {Akbari, Hassan and Yuan, Liangzhe and Qian, Rui and Chuang, Wei-Hong and Chang, Shih-Fu and Cui, Yin and Gong, Boqing},
  date = {2021-12-06},
  eprint = {2104.11178},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2104.11178},
  urldate = {2024-01-23},
  abstract = {We present a framework for learning multimodal representations from unlabeled data using convolution-free Transformer architectures. Specifically, our Video-Audio-Text Transformer (VATT) takes raw signals as inputs and extracts multimodal representations that are rich enough to benefit a variety of downstream tasks. We train VATT end-to-end from scratch using multimodal contrastive losses and evaluate its performance by the downstream tasks of video action recognition, audio event classification, image classification, and text-to-video retrieval. Furthermore, we study a modality-agnostic, single-backbone Transformer by sharing weights among the three modalities. We show that the convolution-free VATT outperforms state-of-the-art ConvNet-based architectures in the downstream tasks. Especially, VATT's vision Transformer achieves the top-1 accuracy of 82.1\% on Kinetics-400, 83.6\% on Kinetics-600, 72.7\% on Kinetics-700, and 41.1\% on Moments in Time, new records while avoiding supervised pre-training. Transferring to image classification leads to 78.7\% top-1 accuracy on ImageNet compared to 64.7\% by training the same Transformer from scratch, showing the generalizability of our model despite the domain gap between videos and images. VATT's audio Transformer also sets a new record on waveform-based audio event recognition by achieving the mAP of 39.4\% on AudioSet without any supervised pre-training. VATT's source code is publicly available.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_prompt\\Akbari et al_2021_VATT.pdf;Y\:\\research\\research_paper\\vatt-transformers-for-multimodal-self-supervised-learning-from-raw-video,-audio-and-text - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\583ZBBXE\\2104.html}
}

@online{akibaOptunaNextgenerationHyperparameter2019,
  title = {Optuna: {{A Next-generation Hyperparameter Optimization Framework}}},
  shorttitle = {Optuna},
  author = {Akiba, Takuya and Sano, Shotaro and Yanase, Toshihiko and Ohta, Takeru and Koyama, Masanori},
  date = {2019-07-25},
  eprint = {1907.10902},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1907.10902},
  urldate = {2022-09-30},
  abstract = {The purpose of this study is to introduce new design-criteria for next-generation hyperparameter optimization software. The criteria we propose include (1) define-by-run API that allows users to construct the parameter search space dynamically, (2) efficient implementation of both searching and pruning strategies, and (3) easy-to-setup, versatile architecture that can be deployed for various purposes, ranging from scalable distributed computing to light-weight experiment conducted via interactive interface. In order to prove our point, we will introduce Optuna, an optimization software which is a culmination of our effort in the development of a next generation optimization software. As an optimization software designed with define-by-run principle, Optuna is particularly the first of its kind. We will present the design-techniques that became necessary in the development of the software that meets the above criteria, and demonstrate the power of our new design through experimental results and real world applications. Our software is available under the MIT license (https://github.com/pfnet/optuna/).},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Akiba et al_2019_Optuna.pdf;C\:\\Users\\chsey\\Zotero\\storage\\W5WDPHIT\\1907.html}
}

@article{alamCrisisMMDMultimodalTwitter2018,
  title = {{{CrisisMMD}}: {{Multimodal Twitter Datasets}} from {{Natural Disasters}}},
  shorttitle = {{{CrisisMMD}}},
  author = {Alam, Firoj and Ofli, Ferda and Imran, Muhammad},
  date = {2018-06-15},
  journaltitle = {Proceedings of the International AAAI Conference on Web and Social Media},
  volume = {12},
  number = {1},
  issn = {2334-0770},
  doi = {10.1609/icwsm.v12i1.14983},
  url = {https://ojs.aaai.org/index.php/ICWSM/article/view/14983},
  urldate = {2023-05-25},
  abstract = {During natural and man-made disasters, people use social media platforms such as Twitter to post textual and multimedia content to report updates about injured or dead people, infrastructure damage, missing or found people, among other information types. Studies have revealed that this online information, if processed timely and effectively, is extremely useful for humanitarian organizations to gain situational awareness and plan relief operations. In addition to the analysis of textual content, recent studies have shown that imagery content on social media can boost disaster response significantly. Despite extensive research that mainly focuses on textual content to extract useful information, limited work has focused on the use of imagery content or the combination of both content types. One of the reasons is the lack of labeled imagery data in this domain. Therefore, in this paper, we aim to tackle this limitation by releasing a large multi-modal dataset from natural disasters collected from Twitter. We provide three types of annotations, which are useful to address a number of crisis response and management tasks for different humanitarian organizations.},
  issue = {1},
  langid = {english},
  keywords = {Natural disasters},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Alam et al_2018_CrisisMMD.pdf}
}

@article{alamMEDICMultitaskLearning2023,
  title = {{{MEDIC}}: A Multi-Task Learning Dataset for Disaster Image Classification},
  shorttitle = {{{MEDIC}}},
  author = {Alam, Firoj and Alam, Tanvirul and Hasan, Md. Arid and Hasnat, Abul and Imran, Muhammad and Ofli, Ferda},
  date = {2023-01-01},
  journaltitle = {Neural Computing and Applications},
  shortjournal = {Neural Comput \& Applic},
  volume = {35},
  number = {3},
  pages = {2609--2632},
  issn = {1433-3058},
  doi = {10.1007/s00521-022-07717-0},
  url = {https://doi.org/10.1007/s00521-022-07717-0},
  urldate = {2023-05-25},
  abstract = {Recent research in disaster informatics demonstrates a practical and important use case of artificial intelligence to save human lives and suffering during natural disasters based on social media contents (text and images). While notable progress has been made using texts, research on exploiting the images remains relatively under-explored. To advance image-based approaches, we propose MEDIC (https://crisisnlp.qcri.org/medic/index.html), which is the largest social media image classification dataset for humanitarian response consisting of 71,198 images to address four different tasks in a multi-task learning setup. This is the first dataset of its kind: social media images, disaster response, and multi-task learning research. An important property of this dataset is its high potential to facilitate research on multi-task learning, which recently receives much interest from the machine learning community and has shown remarkable results in terms of memory, inference speed, performance, and generalization capability. Therefore, the proposed dataset is an important resource for advancing image-based disaster management and multi-task machine learning research. We experiment with different deep learning architectures and report promising results, which are above the majority baselines for all tasks. Along with the dataset, we also release all relevant scripts (https://github.com/firojalam/medic).},
  langid = {english},
  keywords = {Crisis informatics,Dataset,Deep learning,Image classification,Multi-task learning,Natural disasters,Social media images},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Alam et al_2023_MEDIC.pdf}
}

@online{alayracFlamingoVisualLanguage2022,
  title = {Flamingo: A {{Visual Language Model}} for {{Few-Shot Learning}}},
  shorttitle = {Flamingo},
  author = {Alayrac, Jean-Baptiste and Donahue, Jeff and Luc, Pauline and Miech, Antoine and Barr, Iain and Hasson, Yana and Lenc, Karel and Mensch, Arthur and Millican, Katie and Reynolds, Malcolm and Ring, Roman and Rutherford, Eliza and Cabi, Serkan and Han, Tengda and Gong, Zhitao and Samangooei, Sina and Monteiro, Marianne and Menick, Jacob and Borgeaud, Sebastian and Brock, Andrew and Nematzadeh, Aida and Sharifzadeh, Sahand and Binkowski, Mikolaj and Barreira, Ricardo and Vinyals, Oriol and Zisserman, Andrew and Simonyan, Karen},
  date = {2022-11-15},
  eprint = {2204.14198},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2204.14198},
  urldate = {2024-04-23},
  abstract = {Building models that can be rapidly adapted to novel tasks using only a handful of annotated examples is an open challenge for multimodal machine learning research. We introduce Flamingo, a family of Visual Language Models (VLM) with this ability. We propose key architectural innovations to: (i) bridge powerful pretrained vision-only and language-only models, (ii) handle sequences of arbitrarily interleaved visual and textual data, and (iii) seamlessly ingest images or videos as inputs. Thanks to their flexibility, Flamingo models can be trained on large-scale multimodal web corpora containing arbitrarily interleaved text and images, which is key to endow them with in-context few-shot learning capabilities. We perform a thorough evaluation of our models, exploring and measuring their ability to rapidly adapt to a variety of image and video tasks. These include open-ended tasks such as visual question-answering, where the model is prompted with a question which it has to answer; captioning tasks, which evaluate the ability to describe a scene or an event; and close-ended tasks such as multiple-choice visual question-answering. For tasks lying anywhere on this spectrum, a single Flamingo model can achieve a new state of the art with few-shot learning, simply by prompting the model with task-specific examples. On numerous benchmarks, Flamingo outperforms models fine-tuned on thousands of times more task-specific data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Alayrac et al_2022_Flamingo.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y3NR2R8T\\2204.html}
}

@online{aldahdoohRevealVisionTransformers2021,
  title = {Reveal of {{Vision Transformers Robustness}} against {{Adversarial Attacks}}},
  author = {Aldahdooh, Ahmed and Hamidouche, Wassim and Deforges, Olivier},
  date = {2021-09-20},
  eprint = {2106.03734},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.03734},
  urldate = {2024-02-26},
  abstract = {The major part of the vanilla vision transformer (ViT) is the attention block that brings the power of mimicking the global context of the input image. For better performance, ViT needs large-scale training data. To overcome this data hunger limitation, many ViT-based networks, or hybrid-ViT, have been proposed to include local context during the training. The robustness of ViTs and its variants against adversarial attacks has not been widely investigated in the literature like CNNs. This work studies the robustness of ViT variants 1) against different Lp-based adversarial attacks in comparison with CNNs, 2) under adversarial examples (AEs) after applying preprocessing defense methods and 3) under the adaptive attacks using expectation over transformation (EOT) framework. To that end, we run a set of experiments on 1000 images from ImageNet-1k and then provide an analysis that reveals that vanilla ViT or hybrid-ViT are more robust than CNNs. For instance, we found that 1) Vanilla ViTs or hybrid-ViTs are more robust than CNNs under Lp-based attacks and under adaptive attacks. 2) Unlike hybrid-ViTs, Vanilla ViTs are not responding to preprocessing defenses that mainly reduce the high frequency components. Furthermore, feature maps, attention maps, and Grad-CAM visualization jointly with image quality measures, and perturbations' energy spectrum are provided for an insight understanding of attention-based models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition}
}

@inproceedings{alexeWhatObject2010,
  title = {What Is an Object?},
  author = {Alexe, Bogdan and Deselaers, Thomas and Ferrari, Vittorio},
  date = {2010-06-01},
  pages = {73--80},
  publisher = {IEEE Computer Society},
  doi = {10.1109/CVPR.2010.5540226},
  url = {https://www.computer.org/csdl/proceedings-article/cvpr/2010/05540226/12OmNvSbBDs},
  urldate = {2023-11-18},
  abstract = {We present a generic objectness measure, quantifying how likely it is for an image window to contain an object of any class. We explicitly train it to distinguish objects with a well-defined boundary in space, such as cows and telephones, from amorphous background elements, such as grass and road. The measure combines in a Bayesian framework several image cues measuring characteristics of objects, such as appearing different from their surroundings and having a closed boundary. This includes an innovative cue measuring the closed boundary characteristic. In experiments on the challenging PASCAL VOC 07 dataset, we show this new cue to outperform a state-of-the-art saliency measure [17], and the combined measure to perform better than any cue alone. Finally, we show how to sample windows from an image according to their objectness distribution and give an algorithm to employ them as location priors for modern class-specific object detectors. In experiments on PASCAL VOC 07 we show this greatly reduces the number of windows evaluated by class-specific object detectors.},
  eventtitle = {2010 {{IEEE Computer Society Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  isbn = {978-1-4244-6984-0},
  langid = {english}
}

@online{aljundiMemoryAwareSynapses2018,
  title = {Memory {{Aware Synapses}}: {{Learning}} What (Not) to Forget},
  shorttitle = {Memory {{Aware Synapses}}},
  author = {Aljundi, Rahaf and Babiloni, Francesca and Elhoseiny, Mohamed and Rohrbach, Marcus and Tuytelaars, Tinne},
  date = {2018-10-05},
  eprint = {1711.09601},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1711.09601},
  urldate = {2023-12-24},
  abstract = {Humans can learn in a continuous manner. Old rarely utilized knowledge can be overwritten by new incoming information while important, frequently used knowledge is prevented from being erased. In artificial learning systems, lifelong learning so far has focused mainly on accumulating knowledge over tasks and overcoming catastrophic forgetting. In this paper, we argue that, given the limited model capacity and the unlimited new information to be learned, knowledge has to be preserved or erased selectively. Inspired by neuroplasticity, we propose a novel approach for lifelong learning, coined Memory Aware Synapses (MAS). It computes the importance of the parameters of a neural network in an unsupervised and online manner. Given a new sample which is fed to the network, MAS accumulates an importance measure for each parameter of the network, based on how sensitive the predicted output function is to a change in this parameter. When learning a new task, changes to important parameters can then be penalized, effectively preventing important knowledge related to previous tasks from being overwritten. Further, we show an interesting connection between a local version of our method and Hebb's rule,which is a model for the learning process in the brain. We test our method on a sequence of object recognition tasks and on the challenging problem of learning an embedding for predicting \${$<\$$}subject, predicate, object\${$>\$$} triplets. We show state-of-the-art performance and, for the first time, the ability to adapt the importance of the parameters based on unlabeled data towards what the network needs (not) to forget, which may vary depending on test conditions.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\incremental_learning\\Aljundi et al_2018_Memory Aware Synapses.pdf;C\:\\Users\\chsey\\Zotero\\storage\\T26PJNZV\\1711.html}
}

@online{AmericaStockMarket2017,
  title = {America's Stock Market Was Dominated by One Industry in 1900},
  date = {2017-02-24},
  url = {http://finance.yahoo.com/news/americas-stock-market-was-dominated-by-one-industry-in-1900-134439952.html},
  urldate = {2023-12-17},
  abstract = {An engineer oils a locomotive of the Michigan Central Railroad, ca.  Americans have been trading stocks for over 200 years, but the~composition of the stock market has shifted as innovation creates new industries and~renders others irrelevant.  Credit Suisse’s recent “Global Investment Returns Yearbook 2017” provides an interesting snapshot of just how much the US market has transformed since 1900.},
  langid = {american},
  organization = {Yahoo Finance}
}

@online{AnalysisModelingClient,
  title = {Analysis and Modeling of Client Order Flow in Limit Order Markets},
  url = {https://www.tandfonline.com/doi/epdf/10.1080/14697688.2022.2150282?needAccess=true},
  urldate = {2024-09-11},
  file = {C:\Users\chsey\Zotero\storage\TPQF35H9\14697688.2022.html}
}

@article{andrewesWatchmakingGeorgeDaniels1983,
  title = {Watchmaking by {{George Daniels}} (Review)},
  author = {Andrewes, William},
  date = {1983},
  journaltitle = {Technology and Culture},
  volume = {24},
  number = {3},
  pages = {545--546},
  publisher = {Johns Hopkins University Press},
  issn = {1097-3729},
  url = {https://muse.jhu.edu/pub/1/article/891424},
  urldate = {2023-12-26},
  abstract = {TECHNOLOGY AND CULTURE Hook Reviews 545 meaning in part defined through instruments. For example, “It was among the physician’s duties to assist in setting up health related job standards” (p. 211). At its most positive, health often meant no more than the capacity to work. This capacity was defined biologically by the new pathology, which itself was created, not merely discovered, by the use of instruments such as the microscope and the sphyg­ momanometer. But how did these changes occur? Certain obvious models come to mind. Was it, as customary account might have it, the result of the gradual evolution of a new medical profession which learned more about nature by using new instruments? Or was it, to caricature slightly another view, part of the emergence of the bourgeois hegemony in which a new ideology redefined life, death, and disease? Well, nothing so simple, no doubt; but there are important questions here about power, control, and definitions of reality. Davis has not really tackled them, but she has shown historians of medicine an important area where they should be confronted. G H R1S 1OPHER LAWREN CE* Watchmaking. By George Daniels. Totowa, N.J.: Sotheby Publications, 1981. Pp. xv+416; illustrations, index. \$65.00. The techniques of watchmaking, developed over the past 450 years, have not only provided a significant contribution to the history of technology but have also produced instruments which greatly in­ fluenced the growth of civilization. In the past, these varied and de­ manding techniques created a number of distinctive and separate trades which, over the last century, have slowly been destroyed by the introduction of mass production techniques and the advent of quartz crystal. Today, a watchmaker can no longer rely upon the assistance of different trades in the production of his work and must be pre­ pared to master all the techniques himself. Although there are still several schools which teach the basic theory and practice of this trade, there is no substitute for learning from the experience of a great master. George Daniels, the most celebrated watchmaker in the world, decided to publish a detailed account of his methods and tech­ niques for the many students who are seeking such advice and assis­ tance. This valuable publication is the result. Daniels is one of the few people professionally engaged in designing and making watches by hand; happily, he has a natural writing ability and is the author of several other major works on horology. *Dr. Lawrence is historian to the Wellcome Institute for the History of Medicine, the Science Museum, London. He has published papers on concepts of disease and on the history of cardiovascular technology. He is currently working on a history of car­ diology since 1880, especially as it relates to technology. 546 Book Reviews TECHNOLOGY AND CULTURE Daniels begins with a brief summary of the history of watchmaking and describes some of the events w'hich have influenced his career. He explains the basic philosophy and approach every aspiring watch­ maker should adopt in order to achieve success. The book is divided into thirteen chapters, each concerned w'ith a different stage or skill involved in the production of a watch. In addition to the descriptions of the techniques and methods involved, there is an interesting sec­ tion on the details which should be considered in the design of the workshop. The author notes the main tools and equipment which should be acquired but emphasizes that, if a watchmaker cannot do the work without machinery, then he will not improve with its aid. He explains how to make the essential hand tools and describes the man­ ner in which they should be used. Many traditional methods are discussed, some of w hich also relate to other crafts. All the techniques involved are listed in the index. This book is a useful reference for craftsmen and historians of horology as well as watchmakers. The text is clearly illustrated with excellent line drawings (produced by David Penney) of each stage of manufacture, and the finished components are shown in fine color photographs. The book is pro­ duced in a useful format and has been carefully designed to provide a clear presentation of the...}
}

@inproceedings{antolVQAVisualQuestion2015,
  title = {{{VQA}}: {{Visual Question Answering}}},
  shorttitle = {{{VQA}}},
  author = {Antol, Stanislaw and Agrawal, Aishwarya and Lu, Jiasen and Mitchell, Margaret and Batra, Dhruv and Zitnick, C. Lawrence and Parikh, Devi},
  date = {2015},
  pages = {2425--2433},
  url = {https://openaccess.thecvf.com/content_iccv_2015/html/Antol_VQA_Visual_Question_ICCV_2015_paper.html},
  urldate = {2023-05-28},
  eventtitle = {Proceedings of the {{IEEE International Conference}} on {{Computer Vision}}},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Antol et al_2015_VQA.pdf}
}

@online{antoniouHowTrainYour2019,
  title = {How to Train Your {{MAML}}},
  author = {Antoniou, Antreas and Edwards, Harrison and Storkey, Amos},
  date = {2019-03-05},
  eprint = {1810.09502},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1810.09502},
  url = {http://arxiv.org/abs/1810.09502},
  urldate = {2022-12-20},
  abstract = {The field of few-shot learning has recently seen substantial advancements. Most of these advancements came from casting few-shot learning as a meta-learning problem. Model Agnostic Meta Learning or MAML is currently one of the best approaches for few-shot learning via meta-learning. MAML is simple, elegant and very powerful, however, it has a variety of issues, such as being very sensitive to neural network architectures, often leading to instability during training, requiring arduous hyperparameter searches to stabilize training and achieve high generalization and being very computationally expensive at both training and inference times. In this paper, we propose various modifications to MAML that not only stabilize the system, but also substantially improve the generalization performance, convergence speed and computational overhead of MAML, which we call MAML++.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Antoniou et al_2019_How to train your MAML.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V7HDEGU2\\1810.html}
}

@article{arbelaezContourDetectionHierarchical2011,
  title = {Contour {{Detection}} and {{Hierarchical Image Segmentation}}},
  author = {Arbeláez, Pablo and Maire, Michael and Fowlkes, Charless and Malik, Jitendra},
  date = {2011-05},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {33},
  number = {5},
  pages = {898--916},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2010.161},
  url = {https://ieeexplore.ieee.org/document/5557884},
  urldate = {2023-11-18},
  abstract = {This paper investigates two fundamental problems in computer vision: contour detection and image segmentation. We present state-of-the-art algorithms for both of these tasks. Our contour detector combines multiple local cues into a globalization framework based on spectral clustering. Our segmentation algorithm consists of generic machinery for transforming the output of any contour detector into a hierarchical region tree. In this manner, we reduce the problem of image segmentation to that of contour detection. Extensive experimental evaluation demonstrates that both our contour detection and segmentation methods significantly outperform competing algorithms. The automatically generated hierarchical segmentations can be interactively refined by user-specified annotations. Computation at multiple image resolutions provides a means of coupling our system to recognition applications.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  file = {Y\:\\paper\\2023 graduation\\Arbeláez et al_2011_Contour Detection and Hierarchical Image Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HRG66P2X\\5557884.html}
}

@online{asadiDoesCombiningParameterefficient2024,
  title = {Does {{Combining Parameter-efficient Modules Improve Few-shot Transfer Accuracy}}?},
  author = {Asadi, Nader and Beitollahi, Mahdi and Khalil, Yasser and Li, Yinchuan and Zhang, Guojun and Chen, Xi},
  date = {2024-02-23},
  eprint = {2402.15414},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2402.15414},
  urldate = {2024-09-13},
  abstract = {Parameter-efficient fine-tuning stands as the standard for efficiently fine-tuning large language and vision models on downstream tasks. Specifically, the efficiency of low-rank adaptation has facilitated the creation and sharing of hundreds of custom LoRA modules, each trained on distinct data from various downstream tasks. In this paper, we explore the composability of LoRA modules, examining if combining these pre-trained modules enhances generalization to unseen downstream tasks. Our investigation involves evaluating two approaches: (a) uniform composition, involving averaging upstream LoRA modules with equal weights, and (b) learned composition, where we learn the weights for each upstream module and perform weighted averaging. Our experimental results on both vision and language models reveal that in few-shot settings, where only a limited number of samples are available for the downstream task, both uniform and learned composition methods result in better transfer accuracy; outperforming full fine-tuning and training a LoRA from scratch. Moreover, in full-shot settings, learned composition performs comparably to regular LoRA training with significantly fewer number of trainable parameters. Our research unveils the potential of uniform composition for enhancing transferability in low-shot settings, without introducing additional learnable parameters.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Asadi et al_2024_Does Combining Parameter-efficient Modules Improve Few-shot Transfer Accuracy.pdf}
}

@article{ashktorabTweedrMiningTwitter2014,
  title = {Tweedr: {{Mining Twitter}} to {{Inform}}},
  author = {Ashktorab, Zahra and Brown, Christopher and Nandi, Manojit and Culotta, Aron},
  date = {2014},
  series = {{{ISCRAM}}},
  abstract = {In this paper, we introduce Tweedr, a Twitter-mining tool that extracts actionable information for disaster relief workers during natural disasters. The Tweedr pipeline consists of three main parts: classification, clustering and extraction. In the classification phase, we use a variety of classification methods (sLDA, SVM, and logistic regression) to identify tweets reporting damage or casualties. In the clustering phase, we use filters to merge tweets that are similar to one another; and finally, in the extraction phase, we extract tokens and phrases that report specific information about different classes of infrastructure damage, damage types, and casualties. We empirically validate our approach with tweets collected from 12 different crises in the United States since 2006.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\X7PEI3EF\Ashktorab 등 - 2014 - Tweedr Mining Twitter to Inform.pdf}
}

@inreference{AstronWristwatch2023,
  title = {Astron (Wristwatch)},
  booktitle = {Wikipedia},
  date = {2023-09-13T17:38:09Z},
  url = {https://en.wikipedia.org/w/index.php?title=Astron_(wristwatch)&oldid=1175241460},
  urldate = {2023-12-26},
  abstract = {The Astron wristwatch, formally known as the Seiko Quartz-Astron 35SQ, was the world's first "quartz clock" wristwatch. It is now registered on the List of IEEE Milestones as a key advance in electrical engineering.},
  langid = {english},
  annotation = {Page Version ID: 1175241460}
}

@online{attalHyperReelHighFidelity6DoF2023,
  title = {{{HyperReel}}: {{High-Fidelity}} 6-{{DoF Video}} with {{Ray-Conditioned Sampling}}},
  shorttitle = {{{HyperReel}}},
  author = {Attal, Benjamin and Huang, Jia-Bin and Richardt, Christian and Zollhoefer, Michael and Kopf, Johannes and O'Toole, Matthew and Kim, Changil},
  date = {2023-01-05},
  eprint = {2301.02238},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2301.02238},
  urldate = {2023-01-24},
  abstract = {Volumetric scene representations enable photorealistic view synthesis for static scenes and form the basis of several existing 6-DoF video techniques. However, the volume rendering procedures that drive these representations necessitate careful trade-offs in terms of quality, rendering speed, and memory efficiency. In particular, existing methods fail to simultaneously achieve real-time performance, small memory footprint, and high-quality rendering for challenging real-world scenes. To address these issues, we present HyperReel -- a novel 6-DoF video representation. The two core components of HyperReel are: (1) a ray-conditioned sample prediction network that enables high-fidelity, high frame rate rendering at high resolutions and (2) a compact and memory efficient dynamic volume representation. Our 6-DoF video pipeline achieves the best performance compared to prior and contemporary approaches in terms of visual quality with small memory requirements, while also rendering at up to 18 frames-per-second at megapixel resolution without any custom CUDA code.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Attal et al_2023_HyperReel.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FBC39NAF\\2301.html}
}

@online{attalLearningNeuralLight2022,
  title = {Learning {{Neural Light Fields}} with {{Ray-Space Embedding Networks}}},
  author = {Attal, Benjamin and Huang, Jia-Bin and Zollhoefer, Michael and Kopf, Johannes and Kim, Changil},
  date = {2022-05-10},
  eprint = {2112.01523},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.01523},
  urldate = {2023-04-08},
  abstract = {Neural radiance fields (NeRFs) produce state-of-the-art view synthesis results. However, they are slow to render, requiring hundreds of network evaluations per pixel to approximate a volume rendering integral. Baking NeRFs into explicit data structures enables efficient rendering, but results in a large increase in memory footprint and, in many cases, a quality reduction. In this paper, we propose a novel neural light field representation that, in contrast, is compact and directly predicts integrated radiance along rays. Our method supports rendering with a single network evaluation per pixel for small baseline light field datasets and can also be applied to larger baselines with only a few evaluations per pixel. At the core of our approach is a ray-space embedding network that maps the 4D ray-space manifold into an intermediate, interpolable latent space. Our method achieves state-of-the-art quality on dense forward-facing datasets such as the Stanford Light Field dataset. In addition, for forward-facing scenes with sparser inputs we achieve results that are competitive with NeRF-based approaches in terms of quality while providing a better speed/quality/memory trade-off with far fewer network evaluations.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\my_research\\Attal et al_2022_Learning Neural Light Fields with Ray-Space Embedding Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6XL57UBQ\\2112.html}
}

@inproceedings{attalToRFTimeofFlightRadiance2021,
  title = {{{TöRF}}: {{Time-of-Flight Radiance Fields}} for {{Dynamic Scene View Synthesis}}},
  shorttitle = {{{TöRF}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Attal, Benjamin and Laidlaw, Eliot and Gokaslan, Aaron and Kim, Changil and Richardt, Christian and Tompkin, James and O' Toole, Matthew},
  date = {2021},
  volume = {34},
  pages = {26289--26301},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2021/hash/dd03de08bfdff4d8ab01117276564cc7-Abstract.html},
  urldate = {2023-01-21},
  abstract = {Neural networks can represent and accurately reconstruct radiance fields for static 3D scenes (e.g., NeRF). Several works extend these to dynamic scenes captured with monocular video, with promising performance. However, the monocular setting is known to be an under-constrained problem, and so methods rely on data-driven priors for reconstructing dynamic content. We replace these priors with measurements from a time-of-flight (ToF) camera, and introduce a neural representation based on an image formation model for continuous-wave ToF cameras. Instead of working with processed depth maps, we model the raw ToF sensor measurements to improve reconstruction quality and avoid issues with low reflectance regions, multi-path interference, and a sensor's limited unambiguous depth range. We show that this approach improves robustness of dynamic scene reconstruction to erroneous calibration and large motions, and discuss the benefits and limitations of integrating RGB+ToF sensors now available on modern smartphones.},
  file = {Y:\paper\2022 winter intern\Attal et al_2021_TöRF.pdf}
}

@online{AutomaticClassificationCOVID19,
  title = {Automatic Classification between {{COVID-19}} Pneumonia, Non-{{COVID-19}} Pneumonia, and the Healthy on Chest {{X-ray}} Image: Combination of Data Augmentation Methods | {{Scientific Reports}}},
  url = {https://www.nature.com/articles/s41598-020-74539-2},
  urldate = {2022-07-27},
  file = {C:\Users\chsey\Zotero\storage\JBB2M3UG\s41598-020-74539-2.html}
}

@online{aytarSoundNetLearningSound2016,
  title = {{{SoundNet}}: {{Learning Sound Representations}} from {{Unlabeled Video}}},
  shorttitle = {{{SoundNet}}},
  author = {Aytar, Yusuf and Vondrick, Carl and Torralba, Antonio},
  date = {2016-10-27},
  eprint = {1610.09001},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1610.09001},
  urldate = {2024-07-26},
  abstract = {We learn rich natural sound representations by capitalizing on large amounts of unlabeled sound data collected in the wild. We leverage the natural synchronization between vision and sound to learn an acoustic representation using two-million unlabeled videos. Unlabeled video has the advantage that it can be economically acquired at massive scales, yet contains useful signals about natural sound. We propose a student-teacher training procedure which transfers discriminative visual knowledge from well established visual recognition models into the sound modality using unlabeled video as a bridge. Our sound representation yields significant performance improvements over the state-of-the-art results on standard benchmarks for acoustic scene/object classification. Visualizations suggest some high-level semantics automatically emerge in the sound network, even though it is trained without ground truth labels.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Sound,notion},
  file = {C:\Users\chsey\Zotero\storage\9D8KBGWK\Aytar 등 - 2016 - SoundNet Learning Sound Representations from Unla.pdf}
}

@online{azorinItMatchBenchmark2023,
  title = {"{{It}}'s a {{Match}}!" -- {{A Benchmark}} of {{Task Affinity Scores}} for {{Joint Learning}}},
  author = {Azorin, Raphael and Gallo, Massimo and Finamore, Alessandro and Rossi, Dario and Michiardi, Pietro},
  date = {2023-01-07},
  eprint = {2301.02873},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2301.02873},
  urldate = {2023-11-14},
  abstract = {While the promises of Multi-Task Learning (MTL) are attractive, characterizing the conditions of its success is still an open problem in Deep Learning. Some tasks may benefit from being learned together while others may be detrimental to one another. From a task perspective, grouping cooperative tasks while separating competing tasks is paramount to reap the benefits of MTL, i.e., reducing training and inference costs. Therefore, estimating task affinity for joint learning is a key endeavor. Recent work suggests that the training conditions themselves have a significant impact on the outcomes of MTL. Yet, the literature is lacking of a benchmark to assess the effectiveness of tasks affinity estimation techniques and their relation with actual MTL performance. In this paper, we take a first step in recovering this gap by (i) defining a set of affinity scores by both revisiting contributions from previous literature as well presenting new ones and (ii) benchmarking them on the Taskonomy dataset. Our empirical campaign reveals how, even in a small-scale scenario, task affinity scoring does not correlate well with actual MTL performance. Yet, some metrics can be more indicative than others.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,I.2.6},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Azorin et al_2023_It's a Match.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XIUXJZFJ\\2301.html}
}

@online{bachmannMultiMAEMultimodalMultitask2022,
  title = {{{MultiMAE}}: {{Multi-modal Multi-task Masked Autoencoders}}},
  shorttitle = {{{MultiMAE}}},
  author = {Bachmann, Roman and Mizrahi, David and Atanov, Andrei and Zamir, Amir},
  date = {2022-04-04},
  eprint = {2204.01678},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2204.01678},
  url = {http://arxiv.org/abs/2204.01678},
  urldate = {2024-05-07},
  abstract = {We propose a pre-training strategy called Multi-modal Multi-task Masked Autoencoders (MultiMAE). It differs from standard Masked Autoencoding in two key aspects: I) it can optionally accept additional modalities of information in the input besides the RGB image (hence "multi-modal"), and II) its training objective accordingly includes predicting multiple outputs besides the RGB image (hence "multi-task"). We make use of masking (across image patches and input modalities) to make training MultiMAE tractable as well as to ensure cross-modality predictive coding is indeed learned by the network. We show this pre-training strategy leads to a flexible, simple, and efficient framework with improved transfer results to downstream tasks. In particular, the same exact pre-trained network can be flexibly used when additional information besides RGB images is available or when no information other than RGB is available - in all configurations yielding competitive to or significantly better results than the baselines. To avoid needing training datasets with multiple modalities and tasks, we train MultiMAE entirely using pseudo labeling, which makes the framework widely applicable to any RGB dataset. The experiments are performed on multiple transfer tasks (image classification, semantic segmentation, depth estimation) and datasets (ImageNet, ADE20K, Taskonomy, Hypersim, NYUv2). The results show an intriguingly impressive capability by the model in cross-modal/task predictive coding and transfer.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Bachmann et al_2022_MultiMAE.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JSQGNP3J\\2204.html}
}

@incollection{bachmannMultiMAEMultimodalMultitask2022a,
  title = {{{MultiMAE}}: {{Multi-modal Multi-task Masked Autoencoders}}},
  shorttitle = {{{MultiMAE}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2022},
  author = {Bachmann, Roman and Mizrahi, David and Atanov, Andrei and Zamir, Amir},
  editor = {Avidan, Shai and Brostow, Gabriel and Cissé, Moustapha and Farinella, Giovanni Maria and Hassner, Tal},
  date = {2022},
  volume = {13697},
  pages = {348--367},
  publisher = {Springer Nature Switzerland},
  location = {Cham},
  doi = {10.1007/978-3-031-19836-6_20},
  url = {https://link.springer.com/10.1007/978-3-031-19836-6_20},
  urldate = {2024-05-07},
  abstract = {We propose a pre-training strategy called Multi-modal Multi-task Masked Autoencoders (MultiMAE). It differs from standard Masked Autoencoding in two key aspects: I) it can optionally accept additional modalities of information in the input besides the RGB image (hence “multimodal”), and II) its training objective accordingly includes predicting multiple outputs besides the RGB image (hence “multi-task”).},
  isbn = {978-3-031-19835-9 978-3-031-19836-6},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Bachmann et al_2022_MultiMAE2.pdf}
}

@online{BackendAI,
  title = {Backend.{{AI}}},
  url = {http://172.25.161.250:10080/},
  urldate = {2022-11-23},
  file = {C:\Users\chsey\Zotero\storage\6A99UJAS\172.25.161.250.html}
}

@online{BackendAIa,
  title = {Backend.{{AI}}},
  url = {http://172.25.161.250:10080/summary},
  urldate = {2022-11-23},
  file = {C:\Users\chsey\Zotero\storage\EPCNRVAE\summary.html}
}

@online{BackendAIb,
  title = {Backend.{{AI}}},
  url = {http://172.25.161.250:10080/summary},
  urldate = {2022-11-23},
  file = {C:\Users\chsey\Zotero\storage\XRPBEIS7\summary.html}
}

@online{bagherinezhadAreElephantsBigger2016,
  title = {Are {{Elephants Bigger}} than {{Butterflies}}? {{Reasoning}} about {{Sizes}} of {{Objects}}},
  shorttitle = {Are {{Elephants Bigger}} than {{Butterflies}}?},
  author = {Bagherinezhad, Hessam and Hajishirzi, Hannaneh and Choi, Yejin and Farhadi, Ali},
  date = {2016-02-01},
  eprint = {1602.00753},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1602.00753},
  url = {http://arxiv.org/abs/1602.00753},
  urldate = {2023-08-05},
  abstract = {Human vision greatly benefits from the information about sizes of objects. The role of size in several visual reasoning tasks has been thoroughly explored in human perception and cognition. However, the impact of the information about sizes of objects is yet to be determined in AI. We postulate that this is mainly attributed to the lack of a comprehensive repository of size information. In this paper, we introduce a method to automatically infer object sizes, leveraging visual and textual information from web. By maximizing the joint likelihood of textual and visual observations, our method learns reliable relative size estimates, with no explicit human supervision. We introduce the relative size dataset and show that our method outperforms competitive textual and visual baselines in reasoning about size comparisons.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\visual common sense reasoning\\Bagherinezhad et al_2016_Are Elephants Bigger than Butterflies.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V58DSLW8\\1602.html}
}

@online{bahngExploringVisualPrompts2022,
  title = {Exploring {{Visual Prompts}} for {{Adapting Large-Scale Models}}},
  author = {Bahng, Hyojin and Jahanian, Ali and Sankaranarayanan, Swami and Isola, Phillip},
  date = {2022-06-03},
  eprint = {2203.17274},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2203.17274},
  urldate = {2023-08-21},
  abstract = {We investigate the efficacy of visual prompting to adapt large-scale models in vision. Following the recent approach from prompt tuning and adversarial reprogramming, we learn a single image perturbation such that a frozen model prompted with this perturbation performs a new task. Through comprehensive experiments, we demonstrate that visual prompting is particularly effective for CLIP and robust to distribution shift, achieving performance competitive with standard linear probes. We further analyze properties of the downstream dataset, prompt design, and output transformation in regard to adaptation performance. The surprising effectiveness of visual prompting provides a new perspective on adapting pre-trained models in vision. Code is available at http://hjbahng.github.io/visual\_prompting .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Bahng et al_2022_Exploring Visual Prompts for Adapting Large-Scale Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\K9NVVS7N\\2203.html}
}

@online{baLayerNormalization2016,
  title = {Layer {{Normalization}}},
  author = {Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E.},
  date = {2016-07-21},
  eprint = {1607.06450},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1607.06450},
  url = {http://arxiv.org/abs/1607.06450},
  urldate = {2024-02-08},
  abstract = {Training state-of-the-art, deep neural networks is computationally expensive. One way to reduce the training time is to normalize the activities of the neurons. A recently introduced technique called batch normalization uses the distribution of the summed input to a neuron over a mini-batch of training cases to compute a mean and variance which are then used to normalize the summed input to that neuron on each training case. This significantly reduces the training time in feed-forward neural networks. However, the effect of batch normalization is dependent on the mini-batch size and it is not obvious how to apply it to recurrent neural networks. In this paper, we transpose batch normalization into layer normalization by computing the mean and variance used for normalization from all of the summed inputs to the neurons in a layer on a single training case. Like batch normalization, we also give each neuron its own adaptive bias and gain which are applied after the normalization but before the non-linearity. Unlike batch normalization, layer normalization performs exactly the same computation at training and test times. It is also straightforward to apply to recurrent neural networks by computing the normalization statistics separately at each time step. Layer normalization is very effective at stabilizing the hidden state dynamics in recurrent networks. Empirically, we show that layer normalization can substantially reduce the training time compared with previously published techniques.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Ba et al_2016_Layer Normalization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SA6XDZW4\\1607.html}
}

@online{baLayerNormalization2016a,
  title = {Layer {{Normalization}}},
  author = {Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E.},
  date = {2016-07-21},
  eprint = {1607.06450},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1607.06450},
  urldate = {2023-07-28},
  abstract = {Training state-of-the-art, deep neural networks is computationally expensive. One way to reduce the training time is to normalize the activities of the neurons. A recently introduced technique called batch normalization uses the distribution of the summed input to a neuron over a mini-batch of training cases to compute a mean and variance which are then used to normalize the summed input to that neuron on each training case. This significantly reduces the training time in feed-forward neural networks. However, the effect of batch normalization is dependent on the mini-batch size and it is not obvious how to apply it to recurrent neural networks. In this paper, we transpose batch normalization into layer normalization by computing the mean and variance used for normalization from all of the summed inputs to the neurons in a layer on a single training case. Like batch normalization, we also give each neuron its own adaptive bias and gain which are applied after the normalization but before the non-linearity. Unlike batch normalization, layer normalization performs exactly the same computation at training and test times. It is also straightforward to apply to recurrent neural networks by computing the normalization statistics separately at each time step. Layer normalization is very effective at stabilizing the hidden state dynamics in recurrent networks. Empirically, we show that layer normalization can substantially reduce the training time compared with previously published techniques.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Ba et al_2016_Layer Normalization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DGQXQZ8J\\1607.html}
}

@online{balazevicIncontextSceneUnderstanding2023,
  title = {Towards {{In-context Scene Understanding}}},
  author = {Balažević, Ivana and Steiner, David and Parthasarathy, Nikhil and Arandjelović, Relja and Hénaff, Olivier J.},
  date = {2023-06-02},
  eprint = {2306.01667},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2306.01667},
  urldate = {2023-08-22},
  abstract = {In-context learning\$\textbackslash unicode\{x2013\}\$the ability to configure a model's behavior with different prompts\$\textbackslash unicode\{x2013\}\$has revolutionized the field of natural language processing, alleviating the need for task-specific models and paving the way for generalist models capable of assisting with any query. Computer vision, in contrast, has largely stayed in the former regime: specialized decoders and finetuning protocols are generally required to perform dense tasks such as semantic segmentation and depth estimation. In this work we explore a simple mechanism for in-context learning of such scene understanding tasks: nearest neighbor retrieval from a prompt of annotated features. We propose a new pretraining protocol\$\textbackslash unicode\{x2013\}\$leveraging attention within and across images\$\textbackslash unicode\{x2013\}\$which yields representations particularly useful in this regime. The resulting Hummingbird model, suitably prompted, performs various scene understanding tasks without modification while approaching the performance of specialists that have been finetuned for each task. Moreover, Hummingbird can be configured to perform new tasks much more efficiently than finetuned models, raising the possibility of scene understanding in the interactive assistant regime.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Balažević et al_2023_Towards In-context Scene Understanding.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8QFPGTMU\\2306.html}
}

@online{baoBEiTBERTPreTraining2022,
  title = {{{BEiT}}: {{BERT Pre-Training}} of {{Image Transformers}}},
  shorttitle = {{{BEiT}}},
  author = {Bao, Hangbo and Dong, Li and Piao, Songhao and Wei, Furu},
  date = {2022-09-03},
  eprint = {2106.08254},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2106.08254},
  url = {http://arxiv.org/abs/2106.08254},
  urldate = {2024-02-08},
  abstract = {We introduce a self-supervised vision representation model BEiT, which stands for Bidirectional Encoder representation from Image Transformers. Following BERT developed in the natural language processing area, we propose a masked image modeling task to pretrain vision Transformers. Specifically, each image has two views in our pre-training, i.e, image patches (such as 16x16 pixels), and visual tokens (i.e., discrete tokens). We first "tokenize" the original image into visual tokens. Then we randomly mask some image patches and fed them into the backbone Transformer. The pre-training objective is to recover the original visual tokens based on the corrupted image patches. After pre-training BEiT, we directly fine-tune the model parameters on downstream tasks by appending task layers upon the pretrained encoder. Experimental results on image classification and semantic segmentation show that our model achieves competitive results with previous pre-training methods. For example, base-size BEiT achieves 83.2\% top-1 accuracy on ImageNet-1K, significantly outperforming from-scratch DeiT training (81.8\%) with the same setup. Moreover, large-size BEiT obtains 86.3\% only using ImageNet-1K, even outperforming ViT-L with supervised pre-training on ImageNet-22K (85.2\%). The code and pretrained models are available at https://aka.ms/beit.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Bao et al_2022_BEiT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AF5N4BN6\\2106.html}
}

@online{baoBEiTBERTPreTraining2022a,
  title = {{{BEiT}}: {{BERT Pre-Training}} of {{Image Transformers}}},
  shorttitle = {{{BEiT}}},
  author = {Bao, Hangbo and Dong, Li and Piao, Songhao and Wei, Furu},
  date = {2022-09-03},
  eprint = {2106.08254},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.08254},
  urldate = {2023-07-03},
  abstract = {We introduce a self-supervised vision representation model BEiT, which stands for Bidirectional Encoder representation from Image Transformers. Following BERT developed in the natural language processing area, we propose a masked image modeling task to pretrain vision Transformers. Specifically, each image has two views in our pre-training, i.e, image patches (such as 16x16 pixels), and visual tokens (i.e., discrete tokens). We first "tokenize" the original image into visual tokens. Then we randomly mask some image patches and fed them into the backbone Transformer. The pre-training objective is to recover the original visual tokens based on the corrupted image patches. After pre-training BEiT, we directly fine-tune the model parameters on downstream tasks by appending task layers upon the pretrained encoder. Experimental results on image classification and semantic segmentation show that our model achieves competitive results with previous pre-training methods. For example, base-size BEiT achieves 83.2\% top-1 accuracy on ImageNet-1K, significantly outperforming from-scratch DeiT training (81.8\%) with the same setup. Moreover, large-size BEiT obtains 86.3\% only using ImageNet-1K, even outperforming ViT-L with supervised pre-training on ImageNet-22K (85.2\%). The code and pretrained models are available at https://aka.ms/beit.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Bao et al_2022_BEiT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3QC5PASQ\\2106.html}
}

@online{baoS2sftFineTuningPretrained2021,
  title = {S2s-Ft: {{Fine-Tuning Pretrained Transformer Encoders}} for {{Sequence-to-Sequence Learning}}},
  shorttitle = {S2s-Ft},
  author = {Bao, Hangbo and Dong, Li and Wang, Wenhui and Yang, Nan and Wei, Furu},
  date = {2021-10-26},
  eprint = {2110.13640},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2110.13640},
  urldate = {2024-08-22},
  abstract = {Pretrained bidirectional Transformers, such as BERT (Devlin et al., 2019), have achieved significant improvements in a wide variety of language understanding tasks, while it is not straightforward to directly apply them for natural language generation. In this paper, we present a sequence-to-sequence fine-tuning toolkit s2s-ft, which adopts pretrained Transformers for conditional generation tasks. Inspired by UniLM (Dong et al., 2019; Bao et al., 2020), we implement three sequenceto-sequence fine-tuning algorithms, namely, causal fine-tuning, masked fine-tuning, and pseudo-masked fine-tuning. By leveraging the existing pretrained bidirectional Transformers, experimental results show that s2s-ft achieves strong performance on several benchmarks of abstractive summarization, and question generation. Moreover, we demonstrate that the package s2s-ft supports both monolingual and multilingual NLG tasks. The s2s-ft toolkit is available at https://github.com/microsoft/ unilm/tree/master/s2s-ft.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {C:\Users\chsey\Zotero\storage\7Z9YKDT2\2110.pdf}
}

@online{baoVLBEiTGenerativeVisionLanguage2022,
  title = {{{VL-BEiT}}: {{Generative Vision-Language Pretraining}}},
  shorttitle = {{{VL-BEiT}}},
  author = {Bao, Hangbo and Wang, Wenhui and Dong, Li and Wei, Furu},
  date = {2022-09-03},
  eprint = {2206.01127},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.01127},
  urldate = {2024-05-02},
  abstract = {We introduce a vision-language foundation model called VL-BEIT, which is a bidirectional multimodal Transformer learned by generative pretraining. Our minimalist solution conducts masked prediction on both monomodal and multimodal data with a shared Transformer. Specifically, we perform masked vision-language modeling on image-text pairs, masked language modeling on texts, and masked image modeling on images. VL-BEIT is learned from scratch with one unified pretraining task, one shared backbone, and one-stage training. Our method is conceptually simple and empirically effective. Experimental results show that VL-BEIT obtains strong results on various vision-language benchmarks, such as visual question answering, visual reasoning, and image-text retrieval. Moreover, our method learns transferable visual features, achieving competitive performance on image classification, and semantic segmentation.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y:\paper\2024_research\Bao et al_2022_VL-BEiT.pdf}
}

@online{baoVLMoUnifiedVisionLanguage2022,
  title = {{{VLMo}}: {{Unified Vision-Language Pre-Training}} with {{Mixture-of-Modality-Experts}}},
  shorttitle = {{{VLMo}}},
  author = {Bao, Hangbo and Wang, Wenhui and Dong, Li and Liu, Qiang and Mohammed, Owais Khan and Aggarwal, Kriti and Som, Subhojit and Wei, Furu},
  date = {2022-05-27},
  eprint = {2111.02358},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.02358},
  urldate = {2024-02-06},
  abstract = {We present a unified Vision-Language pretrained Model (VLMo) that jointly learns a dual encoder and a fusion encoder with a modular Transformer network. Specifically, we introduce Mixture-of-Modality-Experts (MoME) Transformer, where each block contains a pool of modality-specific experts and a shared self-attention layer. Because of the modeling flexibility of MoME, pretrained VLMo can be fine-tuned as a fusion encoder for vision-language classification tasks, or used as a dual encoder for efficient image-text retrieval. Moreover, we propose a stagewise pre-training strategy, which effectively leverages large-scale image-only and text-only data besides image-text pairs. Experimental results show that VLMo achieves state-of-the-art results on various vision-language tasks, including VQA, NLVR2 and image-text retrieval. The code and pretrained models are available at https://aka.ms/vlmo.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Bao et al_2022_VLMo.pdf;C\:\\Users\\chsey\\Zotero\\storage\\W53BLCTQ\\2111.html}
}

@online{barriosMultilayerLearnableAttention2024,
  title = {Multi-Layer {{Learnable Attention Mask}} for {{Multimodal Tasks}}},
  author = {Barrios, Wayner and Jin, SouYoung},
  date = {2024-06-04},
  eprint = {2406.02761},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2406.02761},
  urldate = {2024-06-30},
  abstract = {While the Self-Attention mechanism in the Transformer model has proven to be effective in many domains, we observe that it is less effective in more diverse settings (e.g. multimodality) due to the varying granularity of each token and the high computational demands of lengthy sequences. To address the challenges, we introduce the Learnable Attention Mask (LAM), strategically designed to globally regulate attention maps and prioritize critical tokens within the sequence. Leveraging the Self-Attention module in a BERT-like transformer network, our approach adeptly captures associations between tokens. The extension of the LAM to a multi-layer version accommodates the varied information aspects embedded at each layer of the Transformer network. Comprehensive experimental validation on various datasets, such as MADv2, QVHighlights, ImageNet 1K, and MSRVTT, demonstrates the efficacy of the LAM, exemplifying its ability to enhance model performance while mitigating redundant computations. This pioneering approach presents a significant advancement in enhancing the understanding of complex scenarios, such as in movie understanding.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {C:\Users\chsey\Zotero\storage\IRMDZQ96\Barrios 그리고 Jin - 2024 - Multi-layer Learnable Attention Mask for Multimoda.pdf}
}

@online{barronMipNeRFMultiscaleRepresentation2021,
  title = {Mip-{{NeRF}}: {{A Multiscale Representation}} for {{Anti-Aliasing Neural Radiance Fields}}},
  shorttitle = {Mip-{{NeRF}}},
  author = {Barron, Jonathan T. and Mildenhall, Ben and Tancik, Matthew and Hedman, Peter and Martin-Brualla, Ricardo and Srinivasan, Pratul P.},
  date = {2021-08-13},
  eprint = {2103.13415},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.13415},
  urldate = {2023-01-18},
  abstract = {The rendering procedure used by neural radiance fields (NeRF) samples a scene with a single ray per pixel and may therefore produce renderings that are excessively blurred or aliased when training or testing images observe scene content at different resolutions. The straightforward solution of supersampling by rendering with multiple rays per pixel is impractical for NeRF, because rendering each ray requires querying a multilayer perceptron hundreds of times. Our solution, which we call "mip-NeRF" (a la "mipmap"), extends NeRF to represent the scene at a continuously-valued scale. By efficiently rendering anti-aliased conical frustums instead of rays, mip-NeRF reduces objectionable aliasing artifacts and significantly improves NeRF's ability to represent fine details, while also being 7\% faster than NeRF and half the size. Compared to NeRF, mip-NeRF reduces average error rates by 17\% on the dataset presented with NeRF and by 60\% on a challenging multiscale variant of that dataset that we present. Mip-NeRF is also able to match the accuracy of a brute-force supersampled NeRF on our multiscale dataset while being 22x faster.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Barron et al_2021_Mip-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VHHHKGKX\\2103.html}
}

@inproceedings{bartoli3DLineMotion2001,
  title = {The {{3D}} Line Motion Matrix and Alignment of Line Reconstructions},
  booktitle = {Proceedings of the 2001 {{IEEE Computer Society Conference}} on {{Computer Vision}} and {{Pattern Recognition}}. {{CVPR}} 2001},
  author = {Bartoli, A. and Sturm, P.},
  date = {2001-02},
  volume = {1},
  pages = {I-I},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2001.990488},
  abstract = {We study the problem of aligning two 3D line reconstructions expressed in Plucker line coordinates. We introduce the 6/spl times/6 3D line motion matrix that acts on Plucker coordinates in projective, affine or Euclidean space. We characterize its algebraic properties and its relation to the usual 4/spl times/4 point motion matrix, and propose various methods for estimating 3D motion from line correspondences, based on image-related and 3D cost functions. We assess the quality of the different estimation methods using simulated data and real images.},
  eventtitle = {Proceedings of the 2001 {{IEEE Computer Society Conference}} on {{Computer Vision}} and {{Pattern Recognition}}. {{CVPR}} 2001},
  keywords = {Cameras,Computational modeling,Computer vision,Cost function,Image reconstruction,Image segmentation,Motion detection,Motion estimation,Tracking,Visual servoing},
  file = {Y\:\\paper\\2022 winter intern\\geommetric\\Bartoli_Sturm_2001_The 3D line motion matrix and alignment of line reconstructions.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6XP2XMK7\\990488.html}
}

@article{bartoliStructurefrommotionUsingLines2005,
  title = {Structure-from-Motion Using Lines: {{Representation}}, Triangulation, and Bundle Adjustment},
  shorttitle = {Structure-from-Motion Using Lines},
  author = {Bartoli, Adrien and Sturm, Peter},
  date = {2005-12-01},
  journaltitle = {Computer Vision and Image Understanding},
  shortjournal = {Computer Vision and Image Understanding},
  volume = {100},
  number = {3},
  pages = {416--441},
  issn = {1077-3142},
  doi = {10.1016/j.cviu.2005.06.001},
  url = {https://www.sciencedirect.com/science/article/pii/S1077314205000846},
  urldate = {2023-01-26},
  abstract = {We address the problem of camera motion and 3D structure reconstruction from line correspondences across multiple views, from initialization to final bundle adjustment. One of the main difficulties when dealing with line features is their algebraic representation. First, we consider the triangulation problem. Based on Plücker coordinates to represent the 3D lines, we propose a maximum likelihood algorithm, relying on linearizing the Plücker constraint and on a Plücker correction procedure, computing the closest Plücker coordinates to a given 6-vector. Second, we consider the bundle adjustment problem, which is essentially a nonlinear optimization process on camera motion and 3D line parameters. Previous overparameterizations of 3D lines induce gauge freedoms and/or internal consistency constraints. We propose the orthonormal representation, which allows handy nonlinear optimization of 3D lines using the minimum four parameters with an unconstrained optimization engine. We compare our algorithms to existing ones on simulated and real data. Results show that our triangulation algorithm outperforms standard linear and bias-corrected quasi-linear algorithms, and that bundle adjustment using our orthonormal representation yields results similar to the standard maximum likelihood trifocal tensor algorithm, while being usable for any number of views.},
  langid = {english},
  keywords = {Bundle adjustment,Lines,Representation,Structure-from-motion,Triangulation},
  file = {Y\:\\paper\\2022 winter intern\\gemmetric\\Bartoli_Sturm_2005_Structure-from-motion using lines.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HYSG3QLW\\S1077314205000846.html}
}

@online{barVisualPromptingImage2022,
  title = {Visual {{Prompting}} via {{Image Inpainting}}},
  author = {Bar, Amir and Gandelsman, Yossi and Darrell, Trevor and Globerson, Amir and Efros, Alexei A.},
  date = {2022-09-01},
  eprint = {2209.00647},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2209.00647},
  url = {http://arxiv.org/abs/2209.00647},
  urldate = {2023-06-29},
  abstract = {How does one adapt a pre-trained visual model to novel downstream tasks without task-specific finetuning or any model modification? Inspired by prompting in NLP, this paper investigates visual prompting: given input-output image example(s) of a new task at test time and a new input image, the goal is to automatically produce the output image, consistent with the given examples. We show that posing this problem as simple image inpainting - literally just filling in a hole in a concatenated visual prompt image - turns out to be surprisingly effective, provided that the inpainting algorithm has been trained on the right data. We train masked auto-encoders on a new dataset that we curated - 88k unlabeled figures from academic papers sources on Arxiv. We apply visual prompting to these pretrained models and demonstrate results on various downstream image-to-image tasks, including foreground segmentation, single object detection, colorization, edge detection, etc.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Bar et al_2022_Visual Prompting via Image Inpainting.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KMGARACQ\\2209.html}
}

@online{bauRewritingDeepGenerative2020,
  title = {Rewriting a {{Deep Generative Model}}},
  author = {Bau, David and Liu, Steven and Wang, Tongzhou and Zhu, Jun-Yan and Torralba, Antonio},
  date = {2020-07-30},
  eprint = {2007.15646},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2007.15646},
  urldate = {2024-09-22},
  abstract = {A deep generative model such as a GAN learns to model a rich set of semantic and physical rules about the target distribution, but up to now, it has been obscure how such rules are encoded in the network, or how a rule could be changed. In this paper, we introduce a new problem setting: manipulation of specific rules encoded by a deep generative model. To address the problem, we propose a formulation in which the desired rule is changed by manipulating a layer of a deep network as a linear associative memory. We derive an algorithm for modifying one entry of the associative memory, and we demonstrate that several interesting structural rules can be located and modified within the layers of state-ofthe-art generative models. We present a user interface to enable users to interactively change the rules of a generative model to achieve desired effects, and we show several proof-of-concept applications. Finally, results on multiple datasets demonstrate the advantage of our method against standard fine-tuning methods and edit transfer algorithms.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning,I.2.10,I.2.6,I.3.3,notion},
  file = {C:\Users\chsey\Zotero\storage\CD4249V3\Bau 등 - 2020 - Rewriting a Deep Generative Model.pdf}
}

@online{bemanaEikonalFieldsRefractive2022,
  title = {Eikonal {{Fields}} for {{Refractive Novel-View Synthesis}}},
  author = {Bemana, Mojtaba and Myszkowski, Karol and Frisvad, Jeppe Revall and Seidel, Hans-Peter and Ritschel, Tobias},
  date = {2022-06-15},
  eprint = {2202.00948},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2202.00948},
  url = {http://arxiv.org/abs/2202.00948},
  urldate = {2023-01-25},
  abstract = {We tackle the problem of generating novel-view images from collections of 2D images showing refractive and reflective objects. Current solutions assume opaque or transparent light transport along straight paths following the emission-absorption model. Instead, we optimize for a field of 3D-varying Index of Refraction (IoR) and trace light through it that bends toward the spatial gradients of said IoR according to the laws of eikonal light transport.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,nerf refractive,연구 - 대상},
  file = {Y\:\\paper\\2022 winter intern\\Bemana et al_2022_Eikonal Fields for Refractive Novel-View Synthesis.pdf;C\:\\Users\\chsey\\Zotero\\storage\\W39KE6YZ\\2202.html}
}

@online{bengioEstimatingPropagatingGradients2013,
  title = {Estimating or {{Propagating Gradients Through Stochastic Neurons}} for {{Conditional Computation}}},
  author = {Bengio, Yoshua and Léonard, Nicholas and Courville, Aaron},
  date = {2013-08-15},
  eprint = {1308.3432},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.1308.3432},
  url = {http://arxiv.org/abs/1308.3432},
  urldate = {2024-11-07},
  abstract = {Stochastic neurons and hard non-linearities can be useful for a number of reasons in deep learning models, but in many cases they pose a challenging problem: how to estimate the gradient of a loss function with respect to the input of such stochastic or non-smooth neurons? I.e., can we "back-propagate" through these stochastic neurons? We examine this question, existing approaches, and compare four families of solutions, applicable in different settings. One of them is the minimum variance unbiased gradient estimator for stochatic binary neurons (a special case of the REINFORCE algorithm). A second approach, introduced here, decomposes the operation of a binary stochastic neuron into a stochastic binary part and a smooth differentiable part, which approximates the expected effect of the pure stochatic binary neuron to first order. A third approach involves the injection of additive or multiplicative noise in a computational graph that is otherwise differentiable. A fourth approach heuristically copies the gradient with respect to the stochastic output directly as an estimator of the gradient with respect to the sigmoid argument (we call this the straight-through estimator). To explore a context where these estimators are useful, we consider a small-scale version of \{\textbackslash em conditional computation\}, where sparse stochastic units form a distributed representation of gaters that can turn off in combinatorially many ways large chunks of the computation performed in the rest of the neural network. In this case, it is important that the gating units produce an actual 0 most of the time. The resulting sparsity can be potentially be exploited to greatly reduce the computational cost of large deep networks for which conditional computation would be useful.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Bengio et al_2013_Estimating or Propagating Gradients Through Stochastic Neurons for Conditional.pdf;C\:\\Users\\chsey\\Zotero\\storage\\73AL5I3I\\1308.html}
}

@online{bhattacharjeeMulTEndtoEndMultitask2022,
  title = {{{MulT}}: {{An End-to-End Multitask Learning Transformer}}},
  shorttitle = {{{MulT}}},
  author = {Bhattacharjee, Deblina and Zhang, Tong and Süsstrunk, Sabine and Salzmann, Mathieu},
  date = {2022-05-17},
  eprint = {2205.08303},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.08303},
  urldate = {2023-11-07},
  abstract = {We propose an end-to-end Multitask Learning Transformer framework, named MulT, to simultaneously learn multiple high-level vision tasks, including depth estimation, semantic segmentation, reshading, surface normal estimation, 2D keypoint detection, and edge detection. Based on the Swin transformer model, our framework encodes the input image into a shared representation and makes predictions for each vision task using task-specific transformer-based decoder heads. At the heart of our approach is a shared attention mechanism modeling the dependencies across the tasks. We evaluate our model on several multitask benchmarks, showing that our MulT framework outperforms both the state-of-the art multitask convolutional neural network models and all the respective single task transformer models. Our experiments further highlight the benefits of sharing attention across all the tasks, and demonstrate that our MulT model is robust and generalizes well to new domains. Our project website is at https://ivrl.github.io/MulT/.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Bhattacharjee et al_2022_MulT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QUWPGW2N\\2205.html}
}

@online{bhattacharjeeVisionTransformerAdapters2023,
  title = {Vision {{Transformer Adapters}} for {{Generalizable Multitask Learning}}},
  author = {Bhattacharjee, Deblina and Süsstrunk, Sabine and Salzmann, Mathieu},
  date = {2023-08-23},
  eprint = {2308.12372},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2308.12372},
  url = {http://arxiv.org/abs/2308.12372},
  urldate = {2023-10-15},
  abstract = {We introduce the first multitasking vision transformer adapters that learn generalizable task affinities which can be applied to novel tasks and domains. Integrated into an off-the-shelf vision transformer backbone, our adapters can simultaneously solve multiple dense vision tasks in a parameter-efficient manner, unlike existing multitasking transformers that are parametrically expensive. In contrast to concurrent methods, we do not require retraining or fine-tuning whenever a new task or domain is added. We introduce a task-adapted attention mechanism within our adapter framework that combines gradient-based task similarities with attention-based ones. The learned task affinities generalize to the following settings: zero-shot task transfer, unsupervised domain adaptation, and generalization without fine-tuning to novel domains. We demonstrate that our approach outperforms not only the existing convolutional neural network-based multitasking methods but also the vision transformer-based ones. Our project page is at \textbackslash url\{https://ivrl.github.io/VTAGML\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_few_shot\\Bhattacharjee et al_2023_Vision Transformer Adapters for Generalizable Multitask Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AE6DGPF8\\2308.html}
}

@online{bhatZoeDepthZeroshotTransfer2023,
  title = {{{ZoeDepth}}: {{Zero-shot Transfer}} by {{Combining Relative}} and {{Metric Depth}}},
  shorttitle = {{{ZoeDepth}}},
  author = {Bhat, Shariq Farooq and Birkl, Reiner and Wofk, Diana and Wonka, Peter and Müller, Matthias},
  date = {2023-02-23},
  eprint = {2302.12288},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2302.12288},
  url = {http://arxiv.org/abs/2302.12288},
  urldate = {2023-10-31},
  abstract = {This paper tackles the problem of depth estimation from a single image. Existing work either focuses on generalization performance disregarding metric scale, i.e. relative depth estimation, or state-of-the-art results on specific datasets, i.e. metric depth estimation. We propose the first approach that combines both worlds, leading to a model with excellent generalization performance while maintaining metric scale. Our flagship model, ZoeD-M12-NK, is pre-trained on 12 datasets using relative depth and fine-tuned on two datasets using metric depth. We use a lightweight head with a novel bin adjustment design called metric bins module for each domain. During inference, each input image is automatically routed to the appropriate head using a latent classifier. Our framework admits multiple configurations depending on the datasets used for relative depth pre-training and metric fine-tuning. Without pre-training, we can already significantly improve the state of the art (SOTA) on the NYU Depth v2 indoor dataset. Pre-training on twelve datasets and fine-tuning on the NYU Depth v2 indoor dataset, we can further improve SOTA for a total of 21\% in terms of relative absolute error (REL). Finally, ZoeD-M12-NK is the first model that can jointly train on multiple datasets (NYU Depth v2 and KITTI) without a significant drop in performance and achieve unprecedented zero-shot generalization performance to eight unseen datasets from both indoor and outdoor domains. The code and pre-trained models are publicly available at https://github.com/isl-org/ZoeDepth .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Bhat et al_2023_ZoeDepth.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V4L2MIQS\\2302.html}
}

@article{bjorckAutomaticDetectionCompression2019,
  title = {Automatic {{Detection}} and {{Compression}} for {{Passive Acoustic Monitoring}} of the {{African Forest Elephant}}},
  author = {Bjorck, Johan and Rappazzo, Brendan H. and Chen, Di and Bernstein, Richard and Wrege, Peter H. and Gomes, Carla P.},
  date = {2019-07-17},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {33},
  number = {01},
  pages = {476--484},
  issn = {2374-3468},
  doi = {10.1609/aaai.v33i01.3301476},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/3820},
  urldate = {2023-05-24},
  abstract = {In this work, we consider applying machine learning to the analysis and compression of audio signals in the context of monitoring elephants in sub-Saharan Africa. Earth’s biodiversity is increasingly under threat by sources of anthropogenic change (e.g. resource extraction, land use change, and climate change) and surveying animal populations is critical for developing conservation strategies. However, manually monitoring tropical forests or deep oceans is intractable. For species that communicate acoustically, researchers have argued for placing audio recorders in the habitats as a costeffective and non-invasive method, a strategy known as passive acoustic monitoring (PAM). In collaboration with conservation efforts, we construct a large labeled dataset of passive acoustic recordings of the African Forest Elephant via crowdsourcing, compromising thousands of hours of recordings in the wild. Using state-of-the-art techniques in artificial intelligence we improve upon previously proposed methods for passive acoustic monitoring for classification and segmentation. In real-time detection of elephant calls, network bandwidth quickly becomes a bottleneck and efficient ways to compress the data are needed. Most audio compression schemes are aimed at human listeners and are unsuitable for low-frequency elephant calls. To remedy this, we provide a novel end-to-end differentiable method for compression of audio signals that can be adapted to acoustic monitoring of any species and dramatically improves over naive coding strategies. \&nbsp;},
  issue = {01},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Bjorck et al_2019_Automatic Detection and Compression for Passive Acoustic Monitoring of the.pdf}
}

@inproceedings{bjorckUnderstandingBatchNormalization2018,
  title = {Understanding {{Batch Normalization}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Bjorck, Nils and Gomes, Carla P and Selman, Bart and Weinberger, Kilian Q},
  date = {2018},
  volume = {31},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2018/hash/36072923bfc3cf47745d704feb489480-Abstract.html},
  urldate = {2022-07-09},
  abstract = {Batch normalization (BN) is a technique to normalize activations in intermediate layers of deep neural networks. Its tendency to improve accuracy and speed up training have established BN as a favorite technique in deep learning. Yet, despite its enormous success, there remains little consensus on the exact reason and mechanism behind these improvements. In this paper we take a step towards a better understanding of BN, following an empirical approach. We conduct several experiments, and show that BN primarily enables training with larger learning rates, which is the cause for faster convergence and better generalization. For networks without BN we demonstrate how large gradient updates can result in diverging loss and activations growing uncontrollably with network depth, which limits possible learning rates. BN avoids this problem by constantly correcting activations to be zero-mean and of unit standard deviation, which enables larger gradient steps, yields faster convergence and may help bypass sharp local minima. We further show various ways in which gradients and activations of deep unnormalized networks are ill-behaved. We contrast our results against recent findings in random matrix theory, shedding new light on classical initialization schemes and their consequences.},
  file = {Y:\paper\Computer Vision\temporary\Bjorck et al_2018_Understanding Batch Normalization.pdf}
}

@article{bollesEpipolarplaneImageAnalysis1987,
  title = {Epipolar-Plane Image Analysis: {{An}} Approach to Determining Structure from Motion},
  shorttitle = {Epipolar-Plane Image Analysis},
  author = {Bolles, Robert C. and Baker, H. Harlyn and Marimont, David H.},
  date = {1987},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vision},
  volume = {1},
  number = {1},
  pages = {7--55},
  issn = {0920-5691, 1573-1405},
  doi = {10.1007/BF00128525},
  url = {http://link.springer.com/10.1007/BF00128525},
  urldate = {2023-02-12},
  abstract = {We present a technique for building a three-dimensional description of a static scene from a dense sequence of images. These images are taken in such rapid succession that they form a solid block of data in which the temporal continuity from image to image is approximately equal to the spatial continuity in an individual image. The technique utilizes knowledge of the camera motion to form and analyze slices of this solid. These slices directly encode not only the three-dimensional positions of objects, but also such spatiotemporal events as the occlusion of one object by another. For straight-line camera motions, these slices have a simple linear structure that makes them easier to analyze. The analysis computes the threedimensional positions of object features, marks occlusion boundaries on the objects, and builds a threedimensional map of "free space." In our article, we first describe the application of this technique to a simple camera motion, and then show how projective duality is used to extend the analysis to a wider class of camera motions and object types that include curved and moving objects.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\D3HWJ68R\Bolles 등 - 1987 - Epipolar-plane image analysis An approach to dete.pdf}
}

@online{bommasaniOpportunitiesRisksFoundation2022,
  title = {On the {{Opportunities}} and {{Risks}} of {{Foundation Models}}},
  author = {Bommasani, Rishi and Hudson, Drew A. and Adeli, Ehsan and Altman, Russ and Arora, Simran and family=Arx, given=Sydney, prefix=von, useprefix=true and Bernstein, Michael S. and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and Brynjolfsson, Erik and Buch, Shyamal and Card, Dallas and Castellon, Rodrigo and Chatterji, Niladri and Chen, Annie and Creel, Kathleen and Davis, Jared Quincy and Demszky, Dora and Donahue, Chris and Doumbouya, Moussa and Durmus, Esin and Ermon, Stefano and Etchemendy, John and Ethayarajh, Kawin and Fei-Fei, Li and Finn, Chelsea and Gale, Trevor and Gillespie, Lauren and Goel, Karan and Goodman, Noah and Grossman, Shelby and Guha, Neel and Hashimoto, Tatsunori and Henderson, Peter and Hewitt, John and Ho, Daniel E. and Hong, Jenny and Hsu, Kyle and Huang, Jing and Icard, Thomas and Jain, Saahil and Jurafsky, Dan and Kalluri, Pratyusha and Karamcheti, Siddharth and Keeling, Geoff and Khani, Fereshte and Khattab, Omar and Koh, Pang Wei and Krass, Mark and Krishna, Ranjay and Kuditipudi, Rohith and Kumar, Ananya and Ladhak, Faisal and Lee, Mina and Lee, Tony and Leskovec, Jure and Levent, Isabelle and Li, Xiang Lisa and Li, Xuechen and Ma, Tengyu and Malik, Ali and Manning, Christopher D. and Mirchandani, Suvir and Mitchell, Eric and Munyikwa, Zanele and Nair, Suraj and Narayan, Avanika and Narayanan, Deepak and Newman, Ben and Nie, Allen and Niebles, Juan Carlos and Nilforoshan, Hamed and Nyarko, Julian and Ogut, Giray and Orr, Laurel and Papadimitriou, Isabel and Park, Joon Sung and Piech, Chris and Portelance, Eva and Potts, Christopher and Raghunathan, Aditi and Reich, Rob and Ren, Hongyu and Rong, Frieda and Roohani, Yusuf and Ruiz, Camilo and Ryan, Jack and Ré, Christopher and Sadigh, Dorsa and Sagawa, Shiori and Santhanam, Keshav and Shih, Andy and Srinivasan, Krishnan and Tamkin, Alex and Taori, Rohan and Thomas, Armin W. and Tramèr, Florian and Wang, Rose E. and Wang, William and Wu, Bohan and Wu, Jiajun and Wu, Yuhuai and Xie, Sang Michael and Yasunaga, Michihiro and You, Jiaxuan and Zaharia, Matei and Zhang, Michael and Zhang, Tianyi and Zhang, Xikun and Zhang, Yuhui and Zheng, Lucia and Zhou, Kaitlyn and Liang, Percy},
  date = {2022-07-12},
  eprint = {2108.07258},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2108.07258},
  urldate = {2023-11-17},
  abstract = {AI is undergoing a paradigm shift with the rise of models (e.g., BERT, DALL-E, GPT-3) that are trained on broad data at scale and are adaptable to a wide range of downstream tasks. We call these models foundation models to underscore their critically central yet incomplete character. This report provides a thorough account of the opportunities and risks of foundation models, ranging from their capabilities (e.g., language, vision, robotics, reasoning, human interaction) and technical principles(e.g., model architectures, training procedures, data, systems, security, evaluation, theory) to their applications (e.g., law, healthcare, education) and societal impact (e.g., inequity, misuse, economic and environmental impact, legal and ethical considerations). Though foundation models are based on standard deep learning and transfer learning, their scale results in new emergent capabilities,and their effectiveness across so many tasks incentivizes homogenization. Homogenization provides powerful leverage but demands caution, as the defects of the foundation model are inherited by all the adapted models downstream. Despite the impending widespread deployment of foundation models, we currently lack a clear understanding of how they work, when they fail, and what they are even capable of due to their emergent properties. To tackle these questions, we believe much of the critical research on foundation models will require deep interdisciplinary collaboration commensurate with their fundamentally sociotechnical nature.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computers and Society,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\Bommasani et al_2022_On the Opportunities and Risks of Foundation Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NA6AJ9KW\\2108.html}
}

@online{BrainTumorClassification,
  title = {Brain Tumor Classification Using Deep {{CNN}} Features via Transfer Learning | {{Elsevier Enhanced Reader}}},
  doi = {10.1016/j.compbiomed.2019.103345},
  url = {https://reader.elsevier.com/reader/sd/pii/S0010482519302148?token=C3C378C7660653F64C0593046BEA68970957E22B81EE58628FD6D38E8D57DC82A97CA7009E7EF7BB5E7277E23F0A70ED&originRegion=us-east-1&originCreation=20220804041719},
  urldate = {2022-08-04},
  langid = {english},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\reproduction\\Brain tumor classification using deep CNN features via transfer learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\C3WPX82C\\S0010482519302148.html}
}

@online{BriefHistoryNavy,
  title = {A {{Brief History}} of {{U}}.{{S}}. {{Navy Fleet Ballistic Missiles}} and {{Submarines}}},
  url = {http://public2.nhhcaws.local/content/history/nhhc/browse-by-topic/wars-conflicts-and-operations/cold-war/strategic-deterrence/fleet-ballistic-missiles-submarines.html},
  urldate = {2023-12-28},
  abstract = {Shortly after World War II, the United States began exploring ways to combine its advances in submarine technology with its rapidly developing missile technology to serve as a deterrent against Soviet aggression. In 1947, the U.S. Navy made the first successful guided-missile launch from a submarine when Cusk (SS-348), a Balao-class submarine, retrofitted with an airtight missile hangar and launch ramp behind its sail, successfully launched a Loon missile. Lacking underwater launch capability, Cusk fired the test missile while surfaced.},
  langid = {american},
  file = {C:\Users\chsey\Zotero\storage\AJQGTIMF\fleet-ballistic-missiles-submarines.html}
}

@online{britannicaSubmarineNuclearPropulsion2023,
  title = {Submarine - {{Nuclear}} Propulsion | {{Britannica}}},
  author = {Britannica},
  date = {2023-12-22},
  url = {https://www.britannica.com/technology/submarine-naval-vessel/Nuclear-propulsion},
  urldate = {2023-12-28},
  abstract = {Submarine - Nuclear propulsion: In 1954, with the commissioning of USS Nautilus, nuclear power became available. Since the nuclear reactor needed no oxygen at all, a single power plant could now suffice for both surface and submerged operation. Moreover, since a very small quantity of nuclear fuel (enriched uranium) provided power over a very long period, a nuclear submarine could operate completely submerged at high speed indefinitely. This change was revolutionary. In the typical prenuclear submarine attack, the submarine approached the target on the surface to avoid draining the battery and submerged only just before coming within sight of the target. The submerged approach},
  langid = {english}
}

@online{brockHighPerformanceLargeScaleImage2021,
  title = {High-{{Performance Large-Scale Image Recognition Without Normalization}}},
  author = {Brock, Andrew and De, Soham and Smith, Samuel L. and Simonyan, Karen},
  date = {2021-02-11},
  eprint = {2102.06171},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2102.06171},
  url = {http://arxiv.org/abs/2102.06171},
  urldate = {2023-06-28},
  abstract = {Batch normalization is a key component of most image classification models, but it has many undesirable properties stemming from its dependence on the batch size and interactions between examples. Although recent work has succeeded in training deep ResNets without normalization layers, these models do not match the test accuracies of the best batch-normalized networks, and are often unstable for large learning rates or strong data augmentations. In this work, we develop an adaptive gradient clipping technique which overcomes these instabilities, and design a significantly improved class of Normalizer-Free ResNets. Our smaller models match the test accuracy of an EfficientNet-B7 on ImageNet while being up to 8.7x faster to train, and our largest models attain a new state-of-the-art top-1 accuracy of 86.5\%. In addition, Normalizer-Free models attain significantly better performance than their batch-normalized counterparts when finetuning on ImageNet after large-scale pre-training on a dataset of 300 million labeled images, with our best models obtaining an accuracy of 89.2\%. Our code is available at https://github.com/deepmind/ deepmind-research/tree/master/nfnets},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\layer\\Brock et al_2021_High-Performance Large-Scale Image Recognition Without Normalization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9GQPGH2M\\2102.html}
}

@online{brockLargeScaleGAN2019,
  title = {Large {{Scale GAN Training}} for {{High Fidelity Natural Image Synthesis}}},
  author = {Brock, Andrew and Donahue, Jeff and Simonyan, Karen},
  date = {2019-02-25},
  eprint = {1809.11096},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1809.11096},
  url = {http://arxiv.org/abs/1809.11096},
  urldate = {2023-08-05},
  abstract = {Despite recent progress in generative image modeling, successfully generating high-resolution, diverse samples from complex datasets such as ImageNet remains an elusive goal. To this end, we train Generative Adversarial Networks at the largest scale yet attempted, and study the instabilities specific to such scale. We find that applying orthogonal regularization to the generator renders it amenable to a simple "truncation trick," allowing fine control over the trade-off between sample fidelity and variety by reducing the variance of the Generator's input. Our modifications lead to models which set the new state of the art in class-conditional image synthesis. When trained on ImageNet at 128x128 resolution, our models (BigGANs) achieve an Inception Score (IS) of 166.5 and Frechet Inception Distance (FID) of 7.4, improving over the previous best IS of 52.52 and FID of 18.6.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\generative model\\Brock et al_2019_Large Scale GAN Training for High Fidelity Natural Image Synthesis.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4MKEBSPG\\1809.html}
}

@online{brownLanguageModelsAre2020,
  title = {Language {{Models}} Are {{Few-Shot Learners}}},
  author = {Brown, Tom B. and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel M. and Wu, Jeffrey and Winter, Clemens and Hesse, Christopher and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
  date = {2020-07-22},
  eprint = {2005.14165},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2005.14165},
  url = {http://arxiv.org/abs/2005.14165},
  urldate = {2023-11-17},
  abstract = {Recent work has demonstrated substantial gains on many NLP tasks and benchmarks by pre-training on a large corpus of text followed by fine-tuning on a specific task. While typically task-agnostic in architecture, this method still requires task-specific fine-tuning datasets of thousands or tens of thousands of examples. By contrast, humans can generally perform a new language task from only a few examples or from simple instructions - something which current NLP systems still largely struggle to do. Here we show that scaling up language models greatly improves task-agnostic, few-shot performance, sometimes even reaching competitiveness with prior state-of-the-art fine-tuning approaches. Specifically, we train GPT-3, an autoregressive language model with 175 billion parameters, 10x more than any previous non-sparse language model, and test its performance in the few-shot setting. For all tasks, GPT-3 is applied without any gradient updates or fine-tuning, with tasks and few-shot demonstrations specified purely via text interaction with the model. GPT-3 achieves strong performance on many NLP datasets, including translation, question-answering, and cloze tasks, as well as several tasks that require on-the-fly reasoning or domain adaptation, such as unscrambling words, using a novel word in a sentence, or performing 3-digit arithmetic. At the same time, we also identify some datasets where GPT-3's few-shot learning still struggles, as well as some datasets where GPT-3 faces methodological issues related to training on large web corpora. Finally, we find that GPT-3 can generate samples of news articles which human evaluators have difficulty distinguishing from articles written by humans. We discuss broader societal impacts of this finding and of GPT-3 in general.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\Brown et al_2020_Language Models are Few-Shot Learners.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WI9MYEDQ\\2005.html}
}

@online{brownLanguageModelsAre2020a,
  title = {Language {{Models}} Are {{Few-Shot Learners}}},
  author = {Brown, Tom B. and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel M. and Wu, Jeffrey and Winter, Clemens and Hesse, Christopher and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
  date = {2020-07-22},
  eprint = {2005.14165},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2005.14165},
  url = {http://arxiv.org/abs/2005.14165},
  urldate = {2023-08-25},
  abstract = {Recent work has demonstrated substantial gains on many NLP tasks and benchmarks by pre-training on a large corpus of text followed by fine-tuning on a specific task. While typically task-agnostic in architecture, this method still requires task-specific fine-tuning datasets of thousands or tens of thousands of examples. By contrast, humans can generally perform a new language task from only a few examples or from simple instructions - something which current NLP systems still largely struggle to do. Here we show that scaling up language models greatly improves task-agnostic, few-shot performance, sometimes even reaching competitiveness with prior state-of-the-art fine-tuning approaches. Specifically, we train GPT-3, an autoregressive language model with 175 billion parameters, 10x more than any previous non-sparse language model, and test its performance in the few-shot setting. For all tasks, GPT-3 is applied without any gradient updates or fine-tuning, with tasks and few-shot demonstrations specified purely via text interaction with the model. GPT-3 achieves strong performance on many NLP datasets, including translation, question-answering, and cloze tasks, as well as several tasks that require on-the-fly reasoning or domain adaptation, such as unscrambling words, using a novel word in a sentence, or performing 3-digit arithmetic. At the same time, we also identify some datasets where GPT-3's few-shot learning still struggles, as well as some datasets where GPT-3 faces methodological issues related to training on large web corpora. Finally, we find that GPT-3 can generate samples of news articles which human evaluators have difficulty distinguishing from articles written by humans. We discuss broader societal impacts of this finding and of GPT-3 in general.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\CJ_paper\\Brown et al_2020_Language Models are Few-Shot Learners.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7YBGT8HD\\2005.html}
}

@online{buehlerDeepBellmanHedging2024,
  title = {Deep {{Bellman Hedging}}},
  author = {Buehler, Hans and Murray, Phillip and Wood, Ben},
  date = {2024-06-25},
  eprint = {2207.00932},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.2207.00932},
  url = {http://arxiv.org/abs/2207.00932},
  urldate = {2024-10-27},
  abstract = {We present an actor-critic-type reinforcement learning algorithm for solving the problem of hedging a portfolio of financial instruments such as securities and over-the-counter derivatives using purely historic data. The key characteristics of our approach are: the ability to hedge with derivatives such as forwards, swaps, futures, options; incorporation of trading frictions such as trading cost and liquidity constraints; applicability for any reasonable portfolio of financial instruments; realistic, continuous state and action spaces; and formal risk-adjusted return objectives. Most importantly, the trained model provides an optimal hedge for arbitrary initial portfolios and market states without the need for re-training. We also prove existence of finite solutions to our Bellman equation, and show the relation to our vanilla Deep Hedging approach},
  pubstate = {prepublished},
  keywords = {Quantitative Finance - Computational Finance,Quantitative Finance - Statistical Finance},
  file = {Y\:\\paper\\2024_lecture\\Buehler et al_2024_Deep Bellman Hedging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\H5G7KW9E\\2207.html}
}

@online{buhlerDeepHedging2018,
  title = {Deep {{Hedging}}},
  author = {Bühler, Hans and Gonon, Lukas and Teichmann, Josef and Wood, Ben},
  date = {2018-02-08},
  eprint = {1802.03042},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.1802.03042},
  url = {http://arxiv.org/abs/1802.03042},
  urldate = {2024-10-26},
  abstract = {We present a framework for hedging a portfolio of derivatives in the presence of market frictions such as transaction costs, market impact, liquidity constraints or risk limits using modern deep reinforcement machine learning methods. We discuss how standard reinforcement learning methods can be applied to non-linear reward structures, i.e. in our case convex risk measures. As a general contribution to the use of deep learning for stochastic processes, we also show that the set of constrained trading strategies used by our algorithm is large enough to \$\textbackslash epsilon\$-approximate any optimal solution. Our algorithm can be implemented efficiently even in high-dimensional situations using modern machine learning tools. Its structure does not depend on specific market dynamics, and generalizes across hedging instruments including the use of liquid derivatives. Its computational performance is largely invariant in the size of the portfolio as it depends mainly on the number of hedging instruments available. We illustrate our approach by showing the effect on hedging under transaction costs in a synthetic market driven by the Heston model, where we outperform the standard "complete market" solution.},
  pubstate = {prepublished},
  keywords = {Mathematics - Numerical Analysis,Mathematics - Optimization and Control,Mathematics - Probability,Quantitative Finance - Computational Finance,Quantitative Finance - Risk Management},
  file = {Y\:\\paper\\2024_lecture\\Bühler et al_2018_Deep Hedging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\336NNPXN\\1802.html}
}

@article{burleyExtendingDisneyBRDF,
  title = {Extending the {{Disney BRDF}} to a {{BSDF}} with {{Integrated Subsurface Scattering}}},
  author = {Burley, Brent and Studios, Walt Disney Animation},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\VT7DSE9I\Burley 그리고 Studios - Extending the Disney BRDF to a BSDF with Integrate.pdf}
}

@article{buslaevAlbumentationsFastFlexible2020,
  title = {Albumentations: {{Fast}} and {{Flexible Image Augmentations}}},
  shorttitle = {Albumentations},
  author = {Buslaev, Alexander and Iglovikov, Vladimir I. and Khvedchenya, Eugene and Parinov, Alex and Druzhinin, Mikhail and Kalinin, Alexandr A.},
  date = {2020-02},
  journaltitle = {Information},
  volume = {11},
  number = {2},
  pages = {125},
  publisher = {Multidisciplinary Digital Publishing Institute},
  issn = {2078-2489},
  doi = {10.3390/info11020125},
  url = {https://www.mdpi.com/2078-2489/11/2/125},
  urldate = {2022-12-09},
  abstract = {Data augmentation is a commonly used technique for increasing both the size and the diversity of labeled training sets by leveraging input transformations that preserve corresponding output labels. In computer vision, image augmentations have become a common implicit regularization technique to combat overfitting in deep learning models and are ubiquitously used to improve performance. While most deep learning frameworks implement basic image transformations, the list is typically limited to some variations of flipping, rotating, scaling, and cropping. Moreover, image processing speed varies in existing image augmentation libraries. We present Albumentations, a fast and flexible open source library for image augmentation with many various image transform operations available that is also an easy-to-use wrapper around other augmentation libraries. We discuss the design principles that drove the implementation of Albumentations and give an overview of the key features and distinct capabilities. Finally, we provide examples of image augmentations for different computer vision tasks and demonstrate that Albumentations is faster than other commonly used image augmentation tools on most image transform operations.},
  issue = {2},
  langid = {english},
  keywords = {computer vision,data augmentation,deep learning},
  file = {Y:\paper\Computer Vision\traditional\PA3\Buslaev et al_2020_Albumentations.pdf}
}

@online{cacciaMultiHeadAdapterRouting2023,
  title = {Multi-{{Head Adapter Routing}} for {{Cross-Task Generalization}}},
  author = {Caccia, Lucas and Ponti, Edoardo and Su, Zhan and Pereira, Matheus and Roux, Nicolas Le and Sordoni, Alessandro},
  date = {2023-11-13},
  eprint = {2211.03831},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2211.03831},
  urldate = {2024-09-17},
  abstract = {Parameter-efficient fine-tuning (PEFT) for cross-task generalization consists in pre-training adapters on a multi-task training set before few-shot adaptation to test tasks. Polytropon [Ponti et al., 2023] (Poly) jointly learns an inventory of adapters and a routing function that selects a (variable-size) subset of adapters for each task during both pre-training and few-shot adaptation. In this paper, we investigate the role that adapter routing plays in its success and design new variants based on our findings. First, we build on the intuition that finer-grained routing provides more expressivity. Hence, we propose MHR (Multi-Head Routing), which combines blocks of parameters from different adapters and outperforms Poly under a comparable parameter budget; by only fine-tuning the routing function and not the adapters (MHR-z), we achieve competitive performance with extreme parameter efficiency. Second, we find that Poly/MHR performance is a result of better multi-task optimization, rather than modular inductive biases that facilitate adapter recombination and local adaptation, as previously hypothesized. In fact, we find that MHR exhibits high gradient alignment between training tasks. We find that routing is most beneficial during multi-task pre-training rather than during few-shot adaptation and propose MHR-µ, which discards routing and fine-tunes the average of the pre-trained adapters on each downstream tasks. This establishes MHR-µ as an effective method for single-adapter fine-tuning. We also show that MHR-µ can be used as an effective zero-shot transfer method by training the average of the pre-trained adapters for a few additional steps on the multi-task training set: this yields gains up to 3\% on absolute accuracy w.r.t. the baselines. Code is available at https://github.com/microsoft/mttl.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,notion},
  file = {C:\Users\chsey\Zotero\storage\DNH7YVCK\Caccia 등 - 2023 - Multi-Head Adapter Routing for Cross-Task Generali.pdf}
}

@article{campbell-kellyProductsServicesSoftware2007,
  title = {From {{Products}} to {{Services}}: {{The Software Industry}} in the {{Internet Era}}},
  shorttitle = {From {{Products}} to {{Services}}},
  author = {Campbell-Kelly, Martin and Garcia-Swartz, Daniel D.},
  date = {2007},
  journaltitle = {The Business History Review},
  volume = {81},
  number = {4},
  eprint = {25097422},
  eprinttype = {jstor},
  pages = {735--764},
  publisher = {{[The President and Fellows of Harvard College, Cambridge University Press]}},
  issn = {0007-6805},
  doi = {10.2307/25097422},
  url = {https://www.jstor.org/stable/25097422},
  urldate = {2023-12-29},
  abstract = {The computer-services and software industry used to be conveniently divided into three main sectors: mass-market software vendors, enterprise software vendors, and computer services. The three sectors were distinct, because personal computers, corporate mainframes, and online computer networks operated in relative isolation. The arrival of the Internet effectively connected everything, facilitating the entry of mass-market vendors into enterprise software and of both mass-market and enterprise software vendors into computer services. As the turbulence of the first decade of the Internet era subsides, a gradual transition from traditional software products to "Web services" is taking place.},
  file = {Y:\paper\management\Campbell-Kelly_Garcia-Swartz_2007_From Products to Services4.pdf}
}

@article{campbell-kellyProductsServicesSoftware2007a,
  title = {From {{Products}} to {{Services}}: {{The Software Industry}} in the {{Internet Era}}},
  shorttitle = {From {{Products}} to {{Services}}},
  author = {Campbell-Kelly, Martin and Garcia-Swartz, Daniel D.},
  date = {2007},
  journaltitle = {The Business History Review},
  volume = {81},
  number = {4},
  eprint = {25097422},
  eprinttype = {jstor},
  pages = {735--764},
  publisher = {{[The President and Fellows of Harvard College, Cambridge University Press]}},
  issn = {0007-6805},
  doi = {10.2307/25097422},
  url = {https://www.jstor.org/stable/25097422},
  urldate = {2023-12-29},
  abstract = {The computer-services and software industry used to be conveniently divided into three main sectors: mass-market software vendors, enterprise software vendors, and computer services. The three sectors were distinct, because personal computers, corporate mainframes, and online computer networks operated in relative isolation. The arrival of the Internet effectively connected everything, facilitating the entry of mass-market vendors into enterprise software and of both mass-market and enterprise software vendors into computer services. As the turbulence of the first decade of the Internet era subsides, a gradual transition from traditional software products to "Web services" is taking place.},
  file = {Y:\paper\management\Campbell-Kelly_Garcia-Swartz_2007_From Products to Services2.pdf}
}

@incollection{carionEndtoEndObjectDetection2020,
  title = {End-to-{{End Object Detection}} with {{Transformers}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  volume = {12346},
  pages = {213--229},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58452-8_13},
  url = {https://link.springer.com/10.1007/978-3-030-58452-8_13},
  urldate = {2023-05-28},
  abstract = {We present a new method that views object detection as a direct set prediction problem. Our approach streamlines the detection pipeline, effectively removing the need for many hand-designed components like a non-maximum suppression procedure or anchor generation that explicitly encode our prior knowledge about the task. The main ingredients of the new framework, called DEtection TRansformer or DETR, are a set-based global loss that forces unique predictions via bipartite matching, and a transformer encoder-decoder architecture. Given a fixed small set of learned object queries, DETR reasons about the relations of the objects and the global image context to directly output the final set of predictions in parallel. The new model is conceptually simple and does not require a specialized library, unlike many other modern detectors. DETR demonstrates accuracy and run-time performance on par with the well-established and highly-optimized Faster RCNN baseline on the challenging COCO object detection dataset. Moreover, DETR can be easily generalized to produce panoptic segmentation in a unified manner. We show that it significantly outperforms competitive baselines. Training code and pretrained models are available at https://github.com/facebookresearch/detr.},
  isbn = {978-3-030-58451-1 978-3-030-58452-8},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Carion et al_2020_End-to-End Object Detection with Transformers.pdf}
}

@online{caronEmergingPropertiesSelfSupervised2021,
  title = {Emerging {{Properties}} in {{Self-Supervised Vision Transformers}}},
  author = {Caron, Mathilde and Touvron, Hugo and Misra, Ishan and Jégou, Hervé and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  date = {2021-05-24},
  eprint = {2104.14294},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2104.14294},
  url = {http://arxiv.org/abs/2104.14294},
  urldate = {2023-08-24},
  abstract = {In this paper, we question if self-supervised learning provides new properties to Vision Transformer (ViT) that stand out compared to convolutional networks (convnets). Beyond the fact that adapting self-supervised methods to this architecture works particularly well, we make the following observations: first, self-supervised ViT features contain explicit information about the semantic segmentation of an image, which does not emerge as clearly with supervised ViTs, nor with convnets. Second, these features are also excellent k-NN classifiers, reaching 78.3\% top-1 on ImageNet with a small ViT. Our study also underlines the importance of momentum encoder, multi-crop training, and the use of small patches with ViTs. We implement our findings into a simple self-supervised method, called DINO, which we interpret as a form of self-distillation with no labels. We show the synergy between DINO and ViTs by achieving 80.1\% top-1 on ImageNet in linear evaluation with ViT-Base.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Caron et al_2021_Emerging Properties in Self-Supervised Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Q2VAR2HR\\2104.html}
}

@online{carreiraQuoVadisAction2018,
  title = {Quo {{Vadis}}, {{Action Recognition}}? {{A New Model}} and the {{Kinetics Dataset}}},
  shorttitle = {Quo {{Vadis}}, {{Action Recognition}}?},
  author = {Carreira, Joao and Zisserman, Andrew},
  date = {2018-02-12},
  eprint = {1705.07750},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1705.07750},
  url = {http://arxiv.org/abs/1705.07750},
  urldate = {2023-08-05},
  abstract = {The paucity of videos in current action classification datasets (UCF-101 and HMDB-51) has made it difficult to identify good video architectures, as most methods obtain similar performance on existing small-scale benchmarks. This paper re-evaluates state-of-the-art architectures in light of the new Kinetics Human Action Video dataset. Kinetics has two orders of magnitude more data, with 400 human action classes and over 400 clips per class, and is collected from realistic, challenging YouTube videos. We provide an analysis on how current architectures fare on the task of action classification on this dataset and how much performance improves on the smaller benchmark datasets after pre-training on Kinetics. We also introduce a new Two-Stream Inflated 3D ConvNet (I3D) that is based on 2D ConvNet inflation: filters and pooling kernels of very deep image classification ConvNets are expanded into 3D, making it possible to learn seamless spatio-temporal feature extractors from video while leveraging successful ImageNet architecture designs and even their parameters. We show that, after pre-training on Kinetics, I3D models considerably improve upon the state-of-the-art in action classification, reaching 80.9\% on HMDB-51 and 98.0\% on UCF-101.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Carreira_Zisserman_2018_Quo Vadis, Action Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6A6TBRCT\\1705.html}
}

@online{CatchMeIf,
  title = {Catch {{Me If You Can}} | {{Proceedings}} of the 22nd {{ACM SIGKDD International Conference}} on {{Knowledge Discovery}} and {{Data Mining}}},
  url = {https://dl.acm.org/doi/10.1145/2939672.2939687},
  urldate = {2023-05-24},
  file = {C:\Users\chsey\Zotero\storage\HUWYRKJH\2939672.html}
}

@online{Ch_bezierPdf,
  title = {Ch\_bezier.Pdf},
  url = {https://www.math.umd.edu/~immortal/MATH431/book/ch_bezier.pdf},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\geommetric\UMD_vision\ch_bezier.pdf}
}

@online{Ch_complexPdf,
  title = {Ch\_complex.Pdf},
  url = {https://www.math.umd.edu/~immortal/MATH431/book/ch_complex.pdf},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\geommetric\UMD_vision\ch_complex.pdf}
}

@online{Ch_gimballockPdf,
  title = {Ch\_gimballock.Pdf},
  url = {https://www.math.umd.edu/~immortal/MATH431/book/ch_gimballock.pdf},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\geommetric\UMD_vision\ch_gimballock.pdf}
}

@online{Ch_quaternionsPdf,
  title = {Ch\_quaternions.Pdf},
  url = {https://www.math.umd.edu/~immortal/MATH431/book/ch_quaternions.pdf},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\geommetric\UMD_vision\ch_quaternions.pdf}
}

@online{chakrabortyDifferentSystemsNaval2021,
  title = {Different {{Systems}} on a {{Naval Submarine}}},
  author = {Chakraborty, Soumya},
  date = {2021-04-17T17:54:44+00:00},
  url = {https://www.marineinsight.com/naval-architecture/different-systems-on-a-naval-submarine/},
  urldate = {2023-12-28},
  abstract = {Though a typical diesel electric submarine would have more than 150 systems in all, lets take a look on the primary systems used on-board a naval submarine.},
  langid = {american},
  organization = {Marine Insight},
  file = {C:\Users\chsey\Zotero\storage\PPKGHWWI\different-systems-on-a-naval-submarine.html}
}

@online{chakrabortyDifferentSystemsNaval2021a,
  title = {Different {{Systems}} on a {{Naval Submarine}}},
  author = {Chakraborty, Soumya},
  date = {2021-04-17T17:54:44+00:00},
  url = {https://www.marineinsight.com/naval-architecture/different-systems-on-a-naval-submarine/},
  urldate = {2023-12-27},
  abstract = {Though a typical diesel electric submarine would have more than 150 systems in all, lets take a look on the primary systems used on-board a naval submarine.},
  langid = {american},
  organization = {Marine Insight}
}

@online{chameleonteamChameleonMixedModalEarlyFusion2024,
  title = {Chameleon: {{Mixed-Modal Early-Fusion Foundation Models}}},
  shorttitle = {Chameleon},
  author = {Chameleon Team},
  date = {2024-05-16},
  eprint = {2405.09818},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2405.09818},
  urldate = {2024-05-24},
  abstract = {We present Chameleon, a family of early-fusion token-based mixed-modal models capable of understanding and generating images and text in any arbitrary sequence. We outline a stable training approach from inception, an alignment recipe, and an architectural parameterization tailored for the early-fusion, token-based, mixed-modal setting. The models are evaluated on a comprehensive range of tasks, including visual question answering, image captioning, text generation, image generation, and long-form mixed modal generation. Chameleon demonstrates broad and general capabilities, including state-of-the-art performance in image captioning tasks, outperforms Llama-2 in text-only tasks while being competitive with models such as Mixtral 8x7B and Gemini-Pro, and performs non-trivial image generation, all in a single model. It also matches or exceeds the performance of much larger models, including Gemini Pro and GPT-4V, according to human judgments on a new long-form mixed-modal generation evaluation, where either the prompt or outputs contain mixed sequences of both images and text. Chameleon marks a significant step forward in a unified modeling of full multimodal documents.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {C:\Users\chsey\Zotero\storage\E9HEJ7VG\Chameleon Team - 2024 - Chameleon Mixed-Modal Early-Fusion Foundation Mod.pdf}
}

@online{chenAdaptFormerAdaptingVision2022,
  title = {{{AdaptFormer}}: {{Adapting Vision Transformers}} for {{Scalable Visual Recognition}}},
  shorttitle = {{{AdaptFormer}}},
  author = {Chen, Shoufa and Ge, Chongjian and Tong, Zhan and Wang, Jiangliu and Song, Yibing and Wang, Jue and Luo, Ping},
  date = {2022-10-14},
  eprint = {2205.13535},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.13535},
  urldate = {2023-11-11},
  abstract = {Pretraining Vision Transformers (ViTs) has achieved great success in visual recognition. A following scenario is to adapt a ViT to various image and video recognition tasks. The adaptation is challenging because of heavy computation and memory storage. Each model needs an independent and complete finetuning process to adapt to different tasks, which limits its transferability to different visual domains. To address this challenge, we propose an effective adaptation approach for Transformer, namely AdaptFormer, which can adapt the pre-trained ViTs into many different image and video tasks efficiently. It possesses several benefits more appealing than prior arts. Firstly, AdaptFormer introduces lightweight modules that only add less than 2\% extra parameters to a ViT, while it is able to increase the ViT's transferability without updating its original pre-trained parameters, significantly outperforming the existing 100\textbackslash\% fully fine-tuned models on action recognition benchmarks. Secondly, it can be plug-and-play in different Transformers and scalable to many visual tasks. Thirdly, extensive experiments on five image and video datasets show that AdaptFormer largely improves ViTs in the target domains. For example, when updating just 1.5\% extra parameters, it achieves about 10\% and 19\% relative improvement compared to the fully fine-tuned models on Something-Something\textasciitilde v2 and HMDB51, respectively. Code is available at https://github.com/ShoufaChen/AdaptFormer.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Chen et al_2022_AdaptFormer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HPVRJF25\\2205.html}
}

@online{chenDecisionTransformerReinforcement2021,
  title = {Decision {{Transformer}}: {{Reinforcement Learning}} via {{Sequence Modeling}}},
  shorttitle = {Decision {{Transformer}}},
  author = {Chen, Lili and Lu, Kevin and Rajeswaran, Aravind and Lee, Kimin and Grover, Aditya and Laskin, Michael and Abbeel, Pieter and Srinivas, Aravind and Mordatch, Igor},
  date = {2021-06-24},
  eprint = {2106.01345},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.01345},
  urldate = {2024-05-07},
  abstract = {We introduce a framework that abstracts Reinforcement Learning (RL) as a sequence modeling problem. This allows us to draw upon the simplicity and scalability of the Transformer architecture, and associated advances in language modeling such as GPT-x and BERT. In particular, we present Decision Transformer, an architecture that casts the problem of RL as conditional sequence modeling. Unlike prior approaches to RL that fit value functions or compute policy gradients, Decision Transformer simply outputs the optimal actions by leveraging a causally masked Transformer. By conditioning an autoregressive model on the desired return (reward), past states, and actions, our Decision Transformer model can generate future actions that achieve the desired return. Despite its simplicity, Decision Transformer matches or exceeds the performance of state-of-the-art model-free offline RL baselines on Atari, OpenAI Gym, and Key-to-Door tasks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Chen et al_2021_Decision Transformer.pdf}
}

@online{chenEATSelfSupervisedPreTraining2024,
  title = {{{EAT}}: {{Self-Supervised Pre-Training}} with {{Efficient Audio Transformer}}},
  shorttitle = {{{EAT}}},
  author = {Chen, Wenxi and Liang, Yuzhe and Ma, Ziyang and Zheng, Zhisheng and Chen, Xie},
  date = {2024-01-07},
  eprint = {2401.03497},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2401.03497},
  urldate = {2024-07-05},
  abstract = {Audio self-supervised learning (SSL) pre-training, which aims to learn good representations from unlabeled audio, has made remarkable progress. However, the extensive computational demands during pre-training pose a significant barrier to the potential application and optimization of audio SSL models. In this paper, inspired by the success of data2vec 2.0 in image modality and Audio-MAE in audio modality, we introduce Efficient Audio Transformer (EAT) to further improve the effectiveness and efficiency in audio SSL. The proposed EAT adopts the bootstrap self-supervised training paradigm to the audio domain. A novel Utterance-Frame Objective (UFO) is designed to enhance the modeling capability of acoustic events. Furthermore, we reveal that the masking strategy is critical in audio SSL pre-training, and superior audio representations can be obtained with large inverse block masks. Experiment results demonstrate that EAT achieves state-of-the-art (SOTA) performance on a range of audio-related tasks, including AudioSet (AS-2M, AS-20K), ESC-50, and SPC-2, along with a significant pre-training speedup up to \textasciitilde 15x compared to existing audio SSL models.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,Computer Science - Sound,Electrical Engineering and Systems Science - Audio and Speech Processing,notion},
  file = {C:\Users\chsey\Zotero\storage\JLWCPB2F\Chen 등 - 2024 - EAT Self-Supervised Pre-Training with Efficient A.pdf}
}

@online{chenEmpiricalStudyTraining2021,
  title = {An {{Empirical Study}} of {{Training Self-Supervised Vision Transformers}}},
  author = {Chen, Xinlei and Xie, Saining and He, Kaiming},
  date = {2021-08-16},
  eprint = {2104.02057},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2104.02057},
  url = {http://arxiv.org/abs/2104.02057},
  urldate = {2023-07-04},
  abstract = {This paper does not describe a novel method. Instead, it studies a straightforward, incremental, yet must-know baseline given the recent progress in computer vision: self-supervised learning for Vision Transformers (ViT). While the training recipes for standard convolutional networks have been highly mature and robust, the recipes for ViT are yet to be built, especially in the self-supervised scenarios where training becomes more challenging. In this work, we go back to basics and investigate the effects of several fundamental components for training self-supervised ViT. We observe that instability is a major issue that degrades accuracy, and it can be hidden by apparently good results. We reveal that these results are indeed partial failure, and they can be improved when training is made more stable. We benchmark ViT results in MoCo v3 and several other self-supervised frameworks, with ablations in various aspects. We discuss the currently positive evidence as well as challenges and open questions. We hope that this work will provide useful data points and experience for future research.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Chen et al_2021_An Empirical Study of Training Self-Supervised Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XZZMT3AD\\2104.html}
}

@article{chenEVEEfficientVisionLanguage2024,
  title = {{{EVE}}: {{Efficient Vision-Language Pre-training}} with {{Masked Prediction}} and {{Modality-Aware MoE}}},
  shorttitle = {{{EVE}}},
  author = {Chen, Junyi and Guo, Longteng and Sun, Jia and Shao, Shuai and Yuan, Zehuan and Lin, Liang and Zhang, Dongyu},
  date = {2024-03-24},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {38},
  number = {2},
  pages = {1110--1119},
  issn = {2374-3468},
  doi = {10.1609/aaai.v38i2.27872},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/27872},
  urldate = {2024-06-07},
  abstract = {Building scalable vision-language models to learn from diverse, multimodal data remains an open challenge. In this paper, we introduce an Efficient Vision-languagE foundation model, namely EVE, which is one unified multimodal Transformer pre-trained solely by one unified pre-training task. Specifically, EVE encodes both vision and language within a shared Transformer network integrated with modality-aware sparse Mixture-of-Experts (MoE) modules, which capture modality-specific information by selectively switching to different experts. To unify pre-training tasks of vision and language, EVE performs masked signal modeling on image-text pairs to reconstruct masked signals, i.e., image pixels and text tokens, given visible signals. This simple yet effective pre-training objective accelerates training by 4x compared to the model pre-trained with Image-Text Contrastive and Image-Text Matching losses. Owing to the combination of the unified architecture and pre-training task, EVE is easy to scale up, enabling better downstream performance with fewer resources and faster training speed. Despite its simplicity, EVE achieves state-of-the-art performance on various vision-language downstream tasks, including visual question answering, visual reasoning, and image-text retrieval.},
  issue = {2},
  langid = {english},
  keywords = {CV: Multi-modal Vision,notion},
  file = {C:\Users\chsey\Zotero\storage\VAIQXS8K\Chen 등 - 2024 - EVE Efficient Vision-Language Pre-training with M.pdf}
}

@online{chenEVEEfficientVisionLanguage2024a,
  title = {{{EVE}}: {{Efficient Vision-Language Pre-training}} with {{Masked Prediction}} and {{Modality-Aware MoE}}},
  shorttitle = {{{EVE}}},
  author = {Chen, Junyi and Guo, Longteng and Sun, Jia and Shao, Shuai and Yuan, Zehuan and Lin, Liang and Zhang, Dongyu},
  date = {2024-03-01},
  eprint = {2308.11971},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2308.11971},
  urldate = {2024-06-17},
  abstract = {Building scalable vision-language models to learn from diverse, multimodal data remains an open challenge. In this paper, we introduce an Efficient Vision-languagE foundation model, namely EVE, which is one unified multimodal Transformer pre-trained solely by one unified pre-training task. Specifically, EVE encodes both vision and language within a shared Transformer network integrated with modality-aware sparse Mixture-of-Experts (MoE) modules, which capture modality-specific information by selectively switching to different experts. To unify pre-training tasks of vision and language, EVE performs masked signal modeling on image-text pairs to reconstruct masked signals, i.e., image pixels and text tokens, given visible signals. This simple yet effective pre-training objective accelerates training by 3.5x compared to the model pre-trained with Image-Text Contrastive and Image-Text Matching losses. Owing to the combination of the unified architecture and pre-training task, EVE is easy to scale up, enabling better downstream performance with fewer resources and faster training speed. Despite its simplicity, EVE achieves state-of-the-art performance on various vision-language downstream tasks, including visual question answering, visual reasoning, and image-text retrieval.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {C:\Users\chsey\Zotero\storage\XFEAQLAH\Chen 등 - 2024 - EVE Efficient Vision-Language Pre-training with M.pdf}
}

@article{chenHarnessingStructuresBig2018,
  title = {Harnessing {{Structures}} in {{Big Data}} via {{Guaranteed Low-Rank Matrix Estimation}}: {{Recent Theory}} and {{Fast Algorithms}} via {{Convex}} and {{Nonconvex Optimization}}},
  shorttitle = {Harnessing {{Structures}} in {{Big Data}} via {{Guaranteed Low-Rank Matrix Estimation}}},
  author = {Chen, Yudong and Chi, Yuejie},
  date = {2018-07},
  journaltitle = {IEEE Signal Processing Magazine},
  volume = {35},
  number = {4},
  pages = {14--31},
  issn = {1558-0792},
  doi = {10.1109/MSP.2018.2821706},
  url = {https://ieeexplore.ieee.org/abstract/document/8399563?casa_token=Y4nPrCkN1ugAAAAA:k1hIgRbTMEAbhKIzOwacrMpgY6aFxpCDhlBdzeJu8Dk4T-HQzTs-UPu-CHfvUjWGDzhVFLp0W40},
  urldate = {2024-04-11},
  abstract = {Low-rank modeling plays a pivotal role in signal processing and machine learning, with applications ranging from collaborative filtering, video surveillance, and medical imaging to dimensionality reduction and adaptive filtering. Many modern high-dimensional data and interactions thereof can be modeled as lying approximately in a low-dimensional subspace or manifold, possibly with additional structures, and its proper exploitations lead to significant cost reduction in sensing, computation, and storage. In recent years, there has been a plethora of progress in understanding how to exploit low-rank structures using computationally efficient procedures in a provable manner, including both convex and nonconvex approaches. On one side, convex relaxations such as nuclear norm minimization often lead to statistically optimal procedures for estimating low-rank matrices, where first-order methods are developed to address the computational challenges; on the other side, there is emerging evidence that properly designed nonconvex procedures, such as projected gradient descent, often provide globally optimal solutions with a much lower computational cost in many problems. This survey article provides a unified overview of these recent advances in low-rank matrix estimation from incomplete measurements. Attention is paid to rigorous characterization of the performance of these algorithms and to problems where the low-rank matrix has additional structural properties that require new algorithmic designs and theoretical analysis.},
  eventtitle = {{{IEEE Signal Processing Magazine}}},
  keywords = {Compressed sensing,Data models,Estimation,notion,Optimization,Signal processing,Signal processing algorithms,Sparse matrices},
  file = {Y\:\\paper\\2024_research\\Chen_Chi_2018_Harnessing Structures in Big Data via Guaranteed Low-Rank Matrix Estimation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SP8SVYSY\\8399563.html}
}

@inproceedings{chenHowInternetAffects2021,
  title = {How the {{Internet Affects}} the {{Development}} of {{Retail Industry}}},
  booktitle = {2020 {{International Conference}} on {{Applications}} and {{Techniques}} in {{Cyber Intelligence}}},
  author = {Chen, Ying},
  editor = {Abawajy, Jemal H. and Choo, Kim-Kwang Raymond and Xu, Zheng and Atiquzzaman, Mohammed},
  date = {2021},
  series = {Advances in {{Intelligent Systems}} and {{Computing}}},
  pages = {960--965},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-53980-1_141},
  abstract = {Over the past decade, the Internet has had an important impact on the retail industry. The purpose of this paper is to study the impact and current situation of Internet on the development of retail industry. This paper mainly uses the method of literature reading and material analysis. It is found that in recent years, with the help of the Internet, e-commerce has attracted a large number of customers with lower prices and richer commodity categories, which has largely encroached on the offline retail market. The new retail model impacts the traditional retail model, making up for the traditional retail industry information asymmetry, subject to spatial constraints and other characteristics. But at the same time, offline real retail industry will not be completely replaced due to its own characteristics. Because online shopping has gradually failed to meet people’s growing demand for personalized, experiential and quality consumption. Therefore, the retail industry needs to make use of the Internet, combine the advantages of online retail and offline retail, carry out precise production and marketing, and provide better services for consumers.},
  isbn = {978-3-030-53980-1},
  langid = {english},
  keywords = {Information technology,Internet,Online retailers,Retail industry}
}

@online{chenMicrosoftCOCOCaptions2015,
  title = {Microsoft {{COCO Captions}}: {{Data Collection}} and {{Evaluation Server}}},
  shorttitle = {Microsoft {{COCO Captions}}},
  author = {Chen, Xinlei and Fang, Hao and Lin, Tsung-Yi and Vedantam, Ramakrishna and Gupta, Saurabh and Dollar, Piotr and Zitnick, C. Lawrence},
  date = {2015-04-03},
  eprint = {1504.00325},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1504.00325},
  urldate = {2023-05-27},
  abstract = {In this paper we describe the Microsoft COCO Caption dataset and evaluation server. When completed, the dataset will contain over one and a half million captions describing over 330,000 images. For the training and validation images, five independent human generated captions will be provided. To ensure consistency in evaluation of automatic caption generation algorithms, an evaluation server is used. The evaluation server receives candidate captions and scores them using several popular metrics, including BLEU, METEOR, ROUGE and CIDEr. Instructions for using the evaluation server are provided.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\image captioning\\Chen et al_2015_Microsoft COCO Captions.pdf;C\:\\Users\\chsey\\Zotero\\storage\\G63CLD3J\\1504.html}
}

@inproceedings{chenNEILExtractingVisual2013,
  title = {{{NEIL}}: {{Extracting Visual Knowledge}} from {{Web Data}}},
  shorttitle = {{{NEIL}}},
  booktitle = {2013 {{IEEE International Conference}} on {{Computer Vision}}},
  author = {Chen, Xinlei and Shrivastava, Abhinav and Gupta, Abhinav},
  date = {2013-02},
  pages = {1409--1416},
  issn = {2380-7504},
  doi = {10.1109/ICCV.2013.178},
  abstract = {We propose NEIL (Never Ending Image Learner), a computer program that runs 24 hours per day and 7 days per week to automatically extract visual knowledge from Internet data. NEIL uses a semi-supervised learning algorithm that jointly discovers common sense relationships (e.g., "Corolla is a kind of/looks similar to Car", "Wheel is a part of Car") and labels instances of the given visual categories. It is an attempt to develop the world's largest visual structured knowledge base with minimum human labeling effort. As of 10th October 2013, NEIL has been continuously running for 2.5 months on 200 core cluster (more than 350K CPU hours) and has an ontology of 1152 object categories, 1034 scene categories and 87 attributes. During this period, NEIL has discovered more than 1700 relationships and has labeled more than 400K visual instances.},
  eventtitle = {2013 {{IEEE International Conference}} on {{Computer Vision}}},
  keywords = {attributes,common sense relationships,Computers,Data mining,Detectors,Knowledge based systems,macro vision,never ending learning,notion,object detection,scene classification,Semantics,semi-supervised learning,Semisupervised learning,visual knowledge base,Visualization},
  file = {Y:\paper\computer_vision_topics_18\lifelong learning\Chen et al_2013_NEIL.pdf}
}

@inproceedings{chenNeuralOrdinaryDifferential2018,
  title = {Neural {{Ordinary Differential Equations}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Chen, Ricky T. Q. and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David K},
  date = {2018},
  volume = {31},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper_files/paper/2018/hash/69386f6bb1dfed68692a24c8686939b9-Abstract.html},
  urldate = {2023-05-30},
  abstract = {We introduce a new family of deep neural network models. Instead of specifying a discrete sequence of hidden layers, we parameterize the derivative of the hidden state using a neural network. The output of the network is computed using a blackbox differential equation solver. These continuous-depth models have constant memory cost, adapt their evaluation strategy to each input, and can explicitly trade numerical precision for speed. We demonstrate these properties in continuous-depth residual networks and continuous-time latent variable models. We also construct continuous normalizing flows, a generative model that can train by maximum likelihood, without partitioning or ordering the data dimensions. For training, we show how to scalably backpropagate through any ODE solver, without access to its internal operations. This allows end-to-end training of ODEs within larger models.},
  file = {Y:\paper\2022 winter intern\Chen et al_2018_Neural Ordinary Differential Equations.pdf}
}

@online{chenPaLIXScalingMultilingual2023,
  title = {{{PaLI-X}}: {{On Scaling}} up a {{Multilingual Vision}} and {{Language Model}}},
  shorttitle = {{{PaLI-X}}},
  author = {Chen, Xi and Djolonga, Josip and Padlewski, Piotr and Mustafa, Basil and Changpinyo, Soravit and Wu, Jialin and Ruiz, Carlos Riquelme and Goodman, Sebastian and Wang, Xiao and Tay, Yi and Shakeri, Siamak and Dehghani, Mostafa and Salz, Daniel and Lucic, Mario and Tschannen, Michael and Nagrani, Arsha and Hu, Hexiang and Joshi, Mandar and Pang, Bo and Montgomery, Ceslee and Pietrzyk, Paulina and Ritter, Marvin and Piergiovanni, A. J. and Minderer, Matthias and Pavetic, Filip and Waters, Austin and Li, Gang and Alabdulmohsin, Ibrahim and Beyer, Lucas and Amelot, Julien and Lee, Kenton and Steiner, Andreas Peter and Li, Yang and Keysers, Daniel and Arnab, Anurag and Xu, Yuanzhong and Rong, Keran and Kolesnikov, Alexander and Seyedhosseini, Mojtaba and Angelova, Anelia and Zhai, Xiaohua and Houlsby, Neil and Soricut, Radu},
  date = {2023-05-29},
  eprint = {2305.18565},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.18565},
  urldate = {2024-06-16},
  abstract = {We present the training recipe and results of scaling up PaLI-X, a multilingual vision and language model, both in terms of size of the components and the breadth of its training task mixture. Our model achieves new levels of performance on a wide-range of varied and complex tasks, including multiple image-based captioning and question-answering tasks, image-based document understanding and few-shot (in-context) learning, as well as object detection, video question answering, and video captioning. PaLI-X advances the state-of-the-art on most vision-and-language benchmarks considered (25+ of them). Finally, we observe emerging capabilities, such as complex counting and multilingual object detection, tasks that are not explicitly in the training mix.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\M9JZNBII\Chen 등 - 2023 - PaLI-X On Scaling up a Multilingual Vision and La.pdf}
}

@online{chenProgressiveDifferentiableArchitecture2019,
  title = {Progressive {{Differentiable Architecture Search}}: {{Bridging}} the {{Depth Gap}} between {{Search}} and {{Evaluation}}},
  shorttitle = {Progressive {{Differentiable Architecture Search}}},
  author = {Chen, Xin and Xie, Lingxi and Wu, Jun and Tian, Qi},
  date = {2019-04-29},
  eprint = {1904.12760},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.12760},
  url = {http://arxiv.org/abs/1904.12760},
  urldate = {2023-08-05},
  abstract = {Recently, differentiable search methods have made major progress in reducing the computational costs of neural architecture search. However, these approaches often report lower accuracy in evaluating the searched architecture or transferring it to another dataset. This is arguably due to the large gap between the architecture depths in search and evaluation scenarios. In this paper, we present an efficient algorithm which allows the depth of searched architectures to grow gradually during the training procedure. This brings two issues, namely, heavier computational overheads and weaker search stability, which we solve using search space approximation and regularization, respectively. With a significantly reduced search time (\textasciitilde 7 hours on a single GPU), our approach achieves state-of-the-art performance on both the proxy dataset (CIFAR10 or CIFAR100) and the target dataset (ImageNet). Code is available at https://github.com/chenxin061/pdarts.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\neural architecture search\\Chen et al_2019_Progressive Differentiable Architecture Search.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SE5Z4X5E\\1904.html}
}

@inproceedings{chenRetrospectMultipromptLearning2023,
  title = {A {{Retrospect}} to {{Multi-prompt Learning}} across {{Vision}} and {{Language}}},
  author = {Chen, Ziliang and Huang, Xin and Guan, Quanlong and Lin, Liang and Luo, Weiqi},
  date = {2023},
  pages = {22190--22201},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Chen_A_Retrospect_to_Multi-prompt_Learning_across_Vision_and_Language_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Chen et al_2023_A Retrospect to Multi-prompt Learning across Vision and Language.pdf}
}

@online{chenSingleImageDepthPerception2017,
  title = {Single-{{Image Depth Perception}} in the {{Wild}}},
  author = {Chen, Weifeng and Fu, Zhao and Yang, Dawei and Deng, Jia},
  date = {2017-01-06},
  eprint = {1604.03901},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1604.03901},
  url = {http://arxiv.org/abs/1604.03901},
  urldate = {2023-08-05},
  abstract = {This paper studies single-image depth perception in the wild, i.e., recovering depth from a single image taken in unconstrained settings. We introduce a new dataset "Depth in the Wild" consisting of images in the wild annotated with relative depth between pairs of random points. We also propose a new algorithm that learns to estimate metric depth using annotations of relative depth. Compared to the state of the art, our algorithm is simpler and performs better. Experiments show that our algorithm, combined with existing RGB-D data and our new relative depth annotations, significantly improves single-image depth perception in the wild.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\2.5d image understanding\\Chen et al_2017_Single-Image Depth Perception in the Wild.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Q8KUPCXW\\1604.html}
}

@online{chenTensoRFTensorialRadiance2022,
  title = {{{TensoRF}}: {{Tensorial Radiance Fields}}},
  shorttitle = {{{TensoRF}}},
  author = {Chen, Anpei and Xu, Zexiang and Geiger, Andreas and Yu, Jingyi and Su, Hao},
  date = {2022-11-29},
  eprint = {2203.09517},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.09517},
  url = {http://arxiv.org/abs/2203.09517},
  urldate = {2023-01-24},
  abstract = {We present TensoRF, a novel approach to model and reconstruct radiance fields. Unlike NeRF that purely uses MLPs, we model the radiance field of a scene as a 4D tensor, which represents a 3D voxel grid with per-voxel multi-channel features. Our central idea is to factorize the 4D scene tensor into multiple compact low-rank tensor components. We demonstrate that applying traditional CP decomposition -- that factorizes tensors into rank-one components with compact vectors -- in our framework leads to improvements over vanilla NeRF. To further boost performance, we introduce a novel vector-matrix (VM) decomposition that relaxes the low-rank constraints for two modes of a tensor and factorizes tensors into compact vector and matrix factors. Beyond superior rendering quality, our models with CP and VM decompositions lead to a significantly lower memory footprint in comparison to previous and concurrent works that directly optimize per-voxel features. Experimentally, we demonstrate that TensoRF with CP decomposition achieves fast reconstruction ({$<$}30 min) with better rendering quality and even a smaller model size ({$<$}4 MB) compared to NeRF. Moreover, TensoRF with VM decomposition further boosts rendering quality and outperforms previous state-of-the-art methods, while reducing the reconstruction time ({$<$}10 min) and retaining a compact model size ({$<$}75 MB).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Chen et al_2022_TensoRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LY6BZC6P\\2203.html}
}

@online{chenTensorMaskFoundationDense2019,
  title = {{{TensorMask}}: {{A Foundation}} for {{Dense Object Segmentation}}},
  shorttitle = {{{TensorMask}}},
  author = {Chen, Xinlei and Girshick, Ross and He, Kaiming and Dollár, Piotr},
  date = {2019-08-27},
  eprint = {1903.12174},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1903.12174},
  url = {http://arxiv.org/abs/1903.12174},
  urldate = {2023-08-05},
  abstract = {Sliding-window object detectors that generate bounding-box object predictions over a dense, regular grid have advanced rapidly and proven popular. In contrast, modern instance segmentation approaches are dominated by methods that first detect object bounding boxes, and then crop and segment these regions, as popularized by Mask R-CNN. In this work, we investigate the paradigm of dense sliding-window instance segmentation, which is surprisingly under-explored. Our core observation is that this task is fundamentally different than other dense prediction tasks such as semantic segmentation or bounding-box object detection, as the output at every spatial location is itself a geometric structure with its own spatial dimensions. To formalize this, we treat dense instance segmentation as a prediction task over 4D tensors and present a general framework called TensorMask that explicitly captures this geometry and enables novel operators on 4D tensors. We demonstrate that the tensor view leads to large gains over baselines that ignore this structure, and leads to results comparable to Mask R-CNN. These promising results suggest that TensorMask can serve as a foundation for novel advances in dense mask prediction and a more complete understanding of the task. Code will be made available.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image segmentation\\Chen et al_2019_TensorMask.pdf;C\:\\Users\\chsey\\Zotero\\storage\\G3XFAK6V\\1903.html}
}

@online{chenUnderstandingImprovingVisual2023,
  title = {Understanding and {{Improving Visual Prompting}}: {{A Label-Mapping Perspective}}},
  shorttitle = {Understanding and {{Improving Visual Prompting}}},
  author = {Chen, Aochuan and Yao, Yuguang and Chen, Pin-Yu and Zhang, Yihua and Liu, Sijia},
  date = {2023-03-24},
  eprint = {2211.11635},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2211.11635},
  url = {http://arxiv.org/abs/2211.11635},
  urldate = {2023-11-06},
  abstract = {We revisit and advance visual prompting (VP), an input prompting technique for vision tasks. VP can reprogram a fixed, pre-trained source model to accomplish downstream tasks in the target domain by simply incorporating universal prompts (in terms of input perturbation patterns) into downstream data points. Yet, it remains elusive why VP stays effective even given a ruleless label mapping (LM) between the source classes and the target classes. Inspired by the above, we ask: How is LM interrelated with VP? And how to exploit such a relationship to improve its accuracy on target tasks? We peer into the influence of LM on VP and provide an affirmative answer that a better 'quality' of LM (assessed by mapping precision and explanation) can consistently improve the effectiveness of VP. This is in contrast to the prior art where the factor of LM was missing. To optimize LM, we propose a new VP framework, termed ILM-VP (iterative label mapping-based visual prompting), which automatically re-maps the source labels to the target labels and progressively improves the target task accuracy of VP. Further, when using a contrastive language-image pretrained (CLIP) model, we propose to integrate an LM process to assist the text prompt selection of CLIP and to improve the target task accuracy. Extensive experiments demonstrate that our proposal significantly outperforms state-of-the-art VP methods. As highlighted below, we show that when reprogramming an ImageNet-pretrained ResNet-18 to 13 target tasks, our method outperforms baselines by a substantial margin, e.g., 7.9\% and 6.7\% accuracy improvements in transfer learning to the target Flowers102 and CIFAR100 datasets. Besides, our proposal on CLIP-based VP provides 13.7\% and 7.1\% accuracy improvements on Flowers102 and DTD respectively. Our code is available at https://github.com/OPTML-Group/ILM-VP.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Chen et al_2023_Understanding and Improving Visual Prompting.pdf;C\:\\Users\\chsey\\Zotero\\storage\\92CRPI4B\\2211.html}
}

@inproceedings{chenViewInterpolationImage1993,
  title = {View Interpolation for Image Synthesis},
  booktitle = {Proceedings of the 20th Annual Conference on {{Computer}} Graphics and Interactive Techniques},
  author = {Chen, Shenchang Eric and Williams, Lance},
  year = {9월 1, 1993},
  series = {{{SIGGRAPH}} '93},
  pages = {279--288},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/166117.166153},
  url = {https://doi.org/10.1145/166117.166153},
  urldate = {2023-02-12},
  isbn = {978-0-89791-601-1},
  keywords = {image morphing,incremental rendering,interpolation,motion blur,motion compensation,real-time display,shadow,virtual holography,virtual reality},
  file = {Y:\paper\2022 winter intern\Chen_Williams_1993_View interpolation for image synthesis.pdf}
}

@online{chenVisionTransformerAdapter2023,
  title = {Vision {{Transformer Adapter}} for {{Dense Predictions}}},
  author = {Chen, Zhe and Duan, Yuchen and Wang, Wenhai and He, Junjun and Lu, Tong and Dai, Jifeng and Qiao, Yu},
  date = {2023-02-13},
  eprint = {2205.08534},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.08534},
  urldate = {2023-07-25},
  abstract = {This work investigates a simple yet powerful dense prediction task adapter for Vision Transformer (ViT). Unlike recently advanced variants that incorporate vision-specific inductive biases into their architectures, the plain ViT suffers inferior performance on dense predictions due to weak prior assumptions. To address this issue, we propose the ViT-Adapter, which allows plain ViT to achieve comparable performance to vision-specific transformers. Specifically, the backbone in our framework is a plain ViT that can learn powerful representations from large-scale multi-modal data. When transferring to downstream tasks, a pre-training-free adapter is used to introduce the image-related inductive biases into the model, making it suitable for these tasks. We verify ViT-Adapter on multiple dense prediction tasks, including object detection, instance segmentation, and semantic segmentation. Notably, without using extra detection data, our ViT-Adapter-L yields state-of-the-art 60.9 box AP and 53.0 mask AP on COCO test-dev. We hope that the ViT-Adapter could serve as an alternative for vision-specific transformers and facilitate future research. The code and models will be released at https://github.com/czczup/ViT-Adapter.},
  pubstate = {prepublished},
  version = {4},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Chen et al_2023_Vision Transformer Adapter for Dense Predictions.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2XLB5FFQ\\2205.html}
}

@online{chenVisionTransformerAdapter2023a,
  title = {Vision {{Transformer Adapter}} for {{Dense Predictions}}},
  author = {Chen, Zhe and Duan, Yuchen and Wang, Wenhai and He, Junjun and Lu, Tong and Dai, Jifeng and Qiao, Yu},
  date = {2023-02-13},
  eprint = {2205.08534},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2205.08534},
  url = {http://arxiv.org/abs/2205.08534},
  urldate = {2023-10-23},
  abstract = {This work investigates a simple yet powerful dense prediction task adapter for Vision Transformer (ViT). Unlike recently advanced variants that incorporate vision-specific inductive biases into their architectures, the plain ViT suffers inferior performance on dense predictions due to weak prior assumptions. To address this issue, we propose the ViT-Adapter, which allows plain ViT to achieve comparable performance to vision-specific transformers. Specifically, the backbone in our framework is a plain ViT that can learn powerful representations from large-scale multi-modal data. When transferring to downstream tasks, a pre-training-free adapter is used to introduce the image-related inductive biases into the model, making it suitable for these tasks. We verify ViT-Adapter on multiple dense prediction tasks, including object detection, instance segmentation, and semantic segmentation. Notably, without using extra detection data, our ViT-Adapter-L yields state-of-the-art 60.9 box AP and 53.0 mask AP on COCO test-dev. We hope that the ViT-Adapter could serve as an alternative for vision-specific transformers and facilitate future research. The code and models will be released at https://github.com/czczup/ViT-Adapter.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Chen et al_2023_Vision Transformer Adapter for Dense Predictions2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JSVYECFH\\2205.html}
}

@online{chenVisualPromptingAdversarial2023,
  title = {Visual {{Prompting}} for {{Adversarial Robustness}}},
  author = {Chen, Aochuan and Lorenz, Peter and Yao, Yuguang and Chen, Pin-Yu and Liu, Sijia},
  date = {2023-04-30},
  eprint = {2210.06284},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2210.06284},
  url = {http://arxiv.org/abs/2210.06284},
  urldate = {2023-11-06},
  abstract = {In this work, we leverage visual prompting (VP) to improve adversarial robustness of a fixed, pre-trained model at testing time. Compared to conventional adversarial defenses, VP allows us to design universal (i.e., data-agnostic) input prompting templates, which have plug-and-play capabilities at testing time to achieve desired model performance without introducing much computation overhead. Although VP has been successfully applied to improving model generalization, it remains elusive whether and how it can be used to defend against adversarial attacks. We investigate this problem and show that the vanilla VP approach is not effective in adversarial defense since a universal input prompt lacks the capacity for robust learning against sample-specific adversarial perturbations. To circumvent it, we propose a new VP method, termed Class-wise Adversarial Visual Prompting (C-AVP), to generate class-wise visual prompts so as to not only leverage the strengths of ensemble prompts but also optimize their interrelations to improve model robustness. Our experiments show that C-AVP outperforms the conventional VP method, with 2.1X standard accuracy gain and 2X robust accuracy gain. Compared to classical test-time defenses, C-AVP also yields a 42X inference time speedup.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Cryptography and Security,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Chen et al_2023_Visual Prompting for Adversarial Robustness.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TWNKAFDS\\2210.html}
}

@article{chenWavLMLargeScaleSelfSupervised2022,
  title = {{{WavLM}}: {{Large-Scale Self-Supervised Pre-Training}} for {{Full Stack Speech Processing}}},
  shorttitle = {{{WavLM}}},
  author = {Chen, Sanyuan and Wang, Chengyi and Chen, Zhengyang and Wu, Yu and Liu, Shujie and Chen, Zhuo and Li, Jinyu and Kanda, Naoyuki and Yoshioka, Takuya and Xiao, Xiong and Wu, Jian and Zhou, Long and Ren, Shuo and Qian, Yanmin and Qian, Yao and Wu, Jian and Zeng, Michael and Yu, Xiangzhan and Wei, Furu},
  date = {2022-10},
  journaltitle = {IEEE Journal of Selected Topics in Signal Processing},
  shortjournal = {IEEE J. Sel. Top. Signal Process.},
  volume = {16},
  number = {6},
  eprint = {2110.13900},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  pages = {1505--1518},
  issn = {1932-4553, 1941-0484},
  doi = {10.1109/JSTSP.2022.3188113},
  url = {http://arxiv.org/abs/2110.13900},
  urldate = {2024-03-17},
  abstract = {Self-supervised learning (SSL) achieves great success in speech recognition, while limited exploration has been attempted for other speech processing tasks. As speech signal contains multi-faceted information including speaker identity, paralinguistics, spoken content, etc., learning universal representations for all speech tasks is challenging. To tackle the problem, we propose a new pre-trained model, WavLM, to solve full-stack downstream speech tasks. WavLM jointly learns masked speech prediction and denoising in pre-training. By this means, WavLM does not only keep the speech content modeling capability by the masked speech prediction, but also improves the potential to non-ASR tasks by the speech denoising. In addition, WavLM employs gated relative position bias for the Transformer structure to better capture the sequence ordering of input speech. We also scale up the training dataset from 60k hours to 94k hours. WavLM Large achieves state-of-the-art performance on the SUPERB benchmark, and brings significant improvements for various speech processing tasks on their representative benchmarks. The code and pre-trained models are available at https://aka.ms/wavlm.},
  keywords = {Computer Science - Computation and Language,Computer Science - Sound,Electrical Engineering and Systems Science - Audio and Speech Processing,notion},
  file = {Y\:\\paper\\2024_research\\Chen et al_2022_WavLM.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KPB57X5Q\\2110.html}
}

@online{chenWeightedTrainingCrossTask2022,
  title = {Weighted {{Training}} for {{Cross-Task Learning}}},
  author = {Chen, Shuxiao and Crammer, Koby and He, Hangfeng and Roth, Dan and Su, Weijie J.},
  date = {2022-03-01},
  eprint = {2105.14095},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2105.14095},
  url = {http://arxiv.org/abs/2105.14095},
  urldate = {2023-10-25},
  abstract = {In this paper, we introduce Target-Aware Weighted Training (TAWT), a weighted training algorithm for cross-task learning based on minimizing a representation-based task distance between the source and target tasks. We show that TAWT is easy to implement, is computationally efficient, requires little hyperparameter tuning, and enjoys non-asymptotic learning-theoretic guarantees. The effectiveness of TAWT is corroborated through extensive experiments with BERT on four sequence tagging tasks in natural language processing (NLP), including part-of-speech (PoS) tagging, chunking, predicate detection, and named entity recognition (NER). As a byproduct, the proposed representation-based task distance allows one to reason in a theoretically principled way about several critical aspects of cross-task learning, such as the choice of the source data and the impact of fine-tuning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Chen et al_2022_Weighted Training for Cross-Task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GEJ4U8JE\\2105.html}
}

@inproceedings{choDistributionAwarePromptTuning2023,
  title = {Distribution-{{Aware Prompt Tuning}} for {{Vision-Language Models}}},
  author = {Cho, Eulrang and Kim, Jooyeon and Kim, Hyunwoo J.},
  date = {2023},
  pages = {22004--22013},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Cho_Distribution-Aware_Prompt_Tuning_for_Vision-Language_Models_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {domain adaptation,notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Cho et al_2023_Distribution-Aware Prompt Tuning for Vision-Language Models.pdf}
}

@online{CiteOpenCVOpencvOpencv,
  title = {{{CiteOpenCV}} · Opencv/Opencv {{Wiki}}},
  url = {https://github.com/opencv/opencv},
  urldate = {2022-11-04},
  abstract = {Open Source Computer Vision Library. Contribute to opencv/opencv development by creating an account on GitHub.},
  langid = {english},
  organization = {GitHub},
  file = {C:\Users\chsey\Zotero\storage\AY9KPZZM\CiteOpenCV.html}
}

@online{clarkWhatDoesBERT2019,
  title = {What {{Does BERT Look At}}? {{An Analysis}} of {{BERT}}'s {{Attention}}},
  shorttitle = {What {{Does BERT Look At}}?},
  author = {Clark, Kevin and Khandelwal, Urvashi and Levy, Omer and Manning, Christopher D.},
  date = {2019-06-10},
  eprint = {1906.04341},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1906.04341},
  url = {http://arxiv.org/abs/1906.04341},
  urldate = {2024-04-17},
  abstract = {Large pre-trained neural networks such as BERT have had great recent success in NLP, motivating a growing body of research investigating what aspects of language they are able to learn from unlabeled data. Most recent analysis has focused on model outputs (e.g., language model surprisal) or internal vector representations (e.g., probing classifiers). Complementary to these works, we propose methods for analyzing the attention mechanisms of pre-trained models and apply them to BERT. BERT's attention heads exhibit patterns such as attending to delimiter tokens, specific positional offsets, or broadly attending over the whole sentence, with heads in the same layer often exhibiting similar behaviors. We further show that certain attention heads correspond well to linguistic notions of syntax and coreference. For example, we find heads that attend to the direct objects of verbs, determiners of nouns, objects of prepositions, and coreferent mentions with remarkably high accuracy. Lastly, we propose an attention-based probing classifier and use it to further demonstrate that substantial syntactic information is captured in BERT's attention.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Clark et al_2019_What Does BERT Look At.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NSZN5BJ6\\1906.html}
}

@online{colasEventNarrativeLargescaleEventcentric2022,
  title = {{{EventNarrative}}: {{A}} Large-Scale {{Event-centric Dataset}} for {{Knowledge Graph-to-Text Generation}}},
  shorttitle = {{{EventNarrative}}},
  author = {Colas, Anthony and Sadeghian, Ali and Wang, Yue and Wang, Daisy Zhe},
  date = {2022-04-13},
  eprint = {2111.00276},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.00276},
  url = {http://arxiv.org/abs/2111.00276},
  urldate = {2023-05-23},
  abstract = {We introduce EventNarrative, a knowledge graph-to-text dataset from publicly available open-world knowledge graphs. Given the recent advances in event-driven Information Extraction (IE), and that prior research on graph-to-text only focused on entity-driven KGs, this paper focuses on event-centric data. However, our data generation system can still be adapted to other other types of KG data. Existing large-scale datasets in the graph-to-text area are non-parallel, meaning there is a large disconnect between the KGs and text. The datasets that have a paired KG and text, are small scale and manually generated or generated without a rich ontology, making the corresponding graphs sparse. Furthermore, these datasets contain many unlinked entities between their KG and text pairs. EventNarrative consists of approximately 230,000 graphs and their corresponding natural language text, 6 times larger than the current largest parallel dataset. It makes use of a rich ontology, all of the KGs entities are linked to the text, and our manual annotations confirm a high data quality. Our aim is two-fold: help break new ground in event-centric research where data is lacking, and to give researchers a well-defined, large-scale dataset in order to better evaluate existing and future knowledge graph-to-text models. We also evaluate two types of baseline on EventNarrative: a graph-to-text specific model and two state-of-the-art language models, which previous work has shown to be adaptable to the knowledge graph-to-text domain.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\Colas et al_2022_EventNarrative.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RVIGZP5U\\2111.html}
}

@book{commissionReportCommitteeWays1977,
  title = {Report to the {{Committee}} on {{Ways}} and {{Means}} on {{Watches}} and {{Parts Therefor}} (Investigation {{No}}. 332-80) {{Under Section}} 332 of the {{Tariff Act}} of 1930},
  author = {Commission, United States International Trade},
  date = {1977},
  eprint = {_DBzHzS07mgC},
  eprinttype = {googlebooks},
  publisher = {U.S. Government Printing Office},
  langid = {english},
  pagetotal = {248},
  file = {Y:\paper\management\Commission_Means_1977_Report to the Committee on Ways and Means on Watches and Parts Therefor.pdf}
}

@article{congDoveNetDeepImage2019,
  title = {{{DoveNet}}: {{Deep Image Harmonization}} via {{Domain Verification}}},
  shorttitle = {{{DoveNet}}},
  author = {Cong, Wenyan and Zhang, Jianfu and Niu, Li and Liu, Liu and Ling, Zhixin and Li, Weiyuan and Zhang, Liqing},
  date = {2019-11-27},
  doi = {10.48550/arXiv.1911.13239},
  url = {https://arxiv.org/abs/1911.13239v3},
  urldate = {2022-12-09},
  abstract = {Image composition is an important operation in image processing, but the inconsistency between foreground and background significantly degrades the quality of composite image. Image harmonization, aiming to make the foreground compatible with the background, is a promising yet challenging task. However, the lack of high-quality publicly available dataset for image harmonization greatly hinders the development of image harmonization techniques. In this work, we contribute an image harmonization dataset iHarmony4 by generating synthesized composite images based on COCO (resp., Adobe5k, Flickr, day2night) dataset, leading to our HCOCO (resp., HAdobe5k, HFlickr, Hday2night) sub-dataset. Moreover, we propose a new deep image harmonization method DoveNet using a novel domain verification discriminator, with the insight that the foreground needs to be translated to the same domain as background. Extensive experiments on our constructed dataset demonstrate the effectiveness of our proposed method. Our dataset and code are available at https://github.com/bcmi/Image\_Harmonization\_Datasets.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA3\Cong et al_2019_DoveNet.pdf}
}

@article{contAnalysisModelingClient2023,
  title = {Analysis and Modeling of Client Order Flow in Limit Order Markets},
  author = {Cont, Rama and Cucuringu, Mihai and Glukhov, Vacslav and Prenzel, Felix},
  date = {2023-02-01},
  journaltitle = {Quantitative Finance},
  volume = {23},
  number = {2},
  pages = {187--205},
  publisher = {Routledge},
  issn = {1469-7688},
  doi = {10.1080/14697688.2022.2150282},
  url = {https://doi.org/10.1080/14697688.2022.2150282},
  urldate = {2024-09-11},
  abstract = {Four distinct clusters of client order flow are identified and their properties analyzed},
  keywords = {notion},
  file = {Y:\paper\2024_lecture\Cont et al_2023_Analysis and modeling of client order flow in limit order markets.pdf}
}

@online{ContourDetectionHierarchical,
  title = {Contour {{Detection}} and {{Hierarchical Image Segmentation}} | {{IEEE Journals}} \& {{Magazine}} | {{IEEE Xplore}}},
  url = {https://ieeexplore.ieee.org/document/5557884},
  urldate = {2023-11-18},
  file = {C:\Users\chsey\Zotero\storage\2C5XXLJ5\5557884.html}
}

@article{cowlsDefinitionBenchmarkDatabase2021,
  title = {A Definition, Benchmark and Database of {{AI}} for Social Good Initiatives},
  author = {Cowls, Josh and Tsamados, Andreas and Taddeo, Mariarosaria and Floridi, Luciano},
  date = {2021-02},
  journaltitle = {Nature Machine Intelligence},
  shortjournal = {Nat Mach Intell},
  volume = {3},
  number = {2},
  pages = {111--115},
  publisher = {Nature Publishing Group},
  issn = {2522-5839},
  doi = {10.1038/s42256-021-00296-0},
  url = {https://www.nature.com/articles/s42256-021-00296-0},
  urldate = {2023-05-24},
  abstract = {Initiatives relying on artificial intelligence (AI) to deliver socially beneficial outcomes—AI for social good (AI4SG)—are on the rise. However, existing attempts to understand and foster AI4SG initiatives have so far been limited by the lack of normative analyses and a shortage of empirical evidence. In this Perspective, we address these limitations by providing a definition of AI4SG and by advocating the use of the United Nations’ Sustainable Development Goals (SDGs) as a benchmark for tracing the scope and spread of AI4SG. We introduce a database of AI4SG projects gathered using this benchmark, and discuss several key insights, including the extent to which different SDGs are being addressed. This analysis makes possible the identification of pressing problems that, if left unaddressed, risk hampering the effectiveness of AI4SG initiatives.},
  issue = {2},
  langid = {english},
  keywords = {Ethics,Science,technology and society},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Cowls et al_2021_A definition, benchmark and database of AI for social good initiatives.pdf}
}

@online{cubukAutoAugmentLearningAugmentation2019,
  title = {{{AutoAugment}}: {{Learning Augmentation Policies}} from {{Data}}},
  shorttitle = {{{AutoAugment}}},
  author = {Cubuk, Ekin D. and Zoph, Barret and Mane, Dandelion and Vasudevan, Vijay and Le, Quoc V.},
  date = {2019-04-11},
  eprint = {1805.09501},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1805.09501},
  url = {http://arxiv.org/abs/1805.09501},
  urldate = {2023-08-05},
  abstract = {Data augmentation is an effective technique for improving the accuracy of modern image classifiers. However, current data augmentation implementations are manually designed. In this paper, we describe a simple procedure called AutoAugment to automatically search for improved data augmentation policies. In our implementation, we have designed a search space where a policy consists of many sub-policies, one of which is randomly chosen for each image in each mini-batch. A sub-policy consists of two operations, each operation being an image processing function such as translation, rotation, or shearing, and the probabilities and magnitudes with which the functions are applied. We use a search algorithm to find the best policy such that the neural network yields the highest validation accuracy on a target dataset. Our method achieves state-of-the-art accuracy on CIFAR-10, CIFAR-100, SVHN, and ImageNet (without additional data). On ImageNet, we attain a Top-1 accuracy of 83.5\% which is 0.4\% better than the previous record of 83.1\%. On CIFAR-10, we achieve an error rate of 1.5\%, which is 0.6\% better than the previous state-of-the-art. Augmentation policies we find are transferable between datasets. The policy learned on ImageNet transfers well to achieve significant improvements on other datasets, such as Oxford Flowers, Caltech-101, Oxford-IIT Pets, FGVC Aircraft, and Stanford Cars.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\image classification\\Cubuk et al_2019_AutoAugment.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V6CH5NSK\\1805.html}
}

@inproceedings{cuiToothNetAutomaticTooth2019,
  title = {{{ToothNet}}: {{Automatic Tooth Instance Segmentation}} and {{Identification From Cone Beam CT Images}}},
  shorttitle = {{{ToothNet}}},
  booktitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Cui, Zhiming and Li, Changjian and Wang, Wenping},
  date = {2019-06},
  pages = {6361--6370},
  issn = {2575-7075},
  doi = {10.1109/CVPR.2019.00653},
  abstract = {This paper proposes a method that uses deep convolutional neural networks to achieve automatic and accurate tooth instance segmentation and identification from CBCT (cone beam CT) images for digital dentistry. The core of our method is a two-stage network. In the first stage, an edge map is extracted from the input CBCT image to enhance image contrast along shape boundaries. Then this edge map and the input images are passed to the second stage. In the second stage, we build our network upon the 3D region proposal network (RPN) with a novel learned-similarity matrix to help efficiently remove redundant proposals, speed up training and save GPU memory. To resolve the ambiguity in the identification task, we encode teeth spatial relationships as an additional feature input in the identification task, which helps to remarkably improve the identification accuracy. Our evaluation, comparison and comprehensive ablation studies demonstrate that our method produces accurate instance segmentation and identification results automatically and outperforms the state-of-the-art approaches. To the best of our knowledge, our method is the first to use neural networks to achieve automatic tooth segmentation and identification from CBCT images.},
  eventtitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  keywords = {Biological and Cell Microscopy,Categorization,Grouping and Shape,Medical,Recognition: Detection,Retrieval,Segmentation},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\reproduction\\Cui et al_2019_ToothNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SX4UMCM7\\8954147.html}
}

@online{curthUturnDoubleDescent2023,
  title = {A {{U-turn}} on {{Double Descent}}: {{Rethinking Parameter Counting}} in {{Statistical Learning}}},
  shorttitle = {A {{U-turn}} on {{Double Descent}}},
  author = {Curth, Alicia and Jeffares, Alan and family=Schaar, given=Mihaela, prefix=van der, useprefix=true},
  date = {2023-10-29},
  eprint = {2310.18988},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2310.18988},
  urldate = {2024-02-26},
  abstract = {Conventional statistical wisdom established a well-understood relationship between model complexity and prediction error, typically presented as a U-shaped curve reflecting a transition between under- and overfitting regimes. However, motivated by the success of overparametrized neural networks, recent influential work has suggested this theory to be generally incomplete, introducing an additional regime that exhibits a second descent in test error as the parameter count p grows past sample size n - a phenomenon dubbed double descent. While most attention has naturally been given to the deep-learning setting, double descent was shown to emerge more generally across non-neural models: known cases include linear regression, trees, and boosting. In this work, we take a closer look at evidence surrounding these more classical statistical machine learning methods and challenge the claim that observed cases of double descent truly extend the limits of a traditional U-shaped complexity-generalization curve therein. We show that once careful consideration is given to what is being plotted on the x-axes of their double descent plots, it becomes apparent that there are implicitly multiple complexity axes along which the parameter count grows. We demonstrate that the second descent appears exactly (and only) when and where the transition between these underlying axes occurs, and that its location is thus not inherently tied to the interpolation threshold p=n. We then gain further insight by adopting a classical nonparametric statistics perspective. We interpret the investigated methods as smoothers and propose a generalized measure for the effective number of parameters they use on unseen examples, using which we find that their apparent double descent curves indeed fold back into more traditional convex shapes - providing a resolution to tensions between double descent and statistical intuition.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning}
}

@online{daiCoAtNetMarryingConvolution2021,
  title = {{{CoAtNet}}: {{Marrying Convolution}} and {{Attention}} for {{All Data Sizes}}},
  shorttitle = {{{CoAtNet}}},
  author = {Dai, Zihang and Liu, Hanxiao and Le, Quoc V. and Tan, Mingxing},
  date = {2021-09-15},
  eprint = {2106.04803},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.04803},
  urldate = {2023-06-28},
  abstract = {Transformers have attracted increasing interests in computer vision, but they still fall behind state-of-the-art convolutional networks. In this work, we show that while Transformers tend to have larger model capacity, their generalization can be worse than convolutional networks due to the lack of the right inductive bias. To effectively combine the strengths from both architectures, we present CoAtNets(pronounced "coat" nets), a family of hybrid models built from two key insights: (1) depthwise Convolution and self-Attention can be naturally unified via simple relative attention; (2) vertically stacking convolution layers and attention layers in a principled way is surprisingly effective in improving generalization, capacity and efficiency. Experiments show that our CoAtNets achieve state-of-the-art performance under different resource constraints across various datasets: Without extra data, CoAtNet achieves 86.0\% ImageNet top-1 accuracy; When pre-trained with 13M images from ImageNet-21K, our CoAtNet achieves 88.56\% top-1 accuracy, matching ViT-huge pre-trained with 300M images from JFT-300M while using 23x less data; Notably, when we further scale up CoAtNet with JFT-3B, it achieves 90.88\% top-1 accuracy on ImageNet, establishing a new state-of-the-art result.},
  pubstate = {prepublished},
  version = {2},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Dai et al_2021_CoAtNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\T2B5N8ML\\2106.html}
}

@online{daiWhyCanGPT2023,
  title = {Why {{Can GPT Learn In-Context}}? {{Language Models Implicitly Perform Gradient Descent}} as {{Meta-Optimizers}}},
  shorttitle = {Why {{Can GPT Learn In-Context}}?},
  author = {Dai, Damai and Sun, Yutao and Dong, Li and Hao, Yaru and Ma, Shuming and Sui, Zhifang and Wei, Furu},
  date = {2023-05-15},
  eprint = {2212.10559},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2212.10559},
  urldate = {2024-01-31},
  abstract = {Large pretrained language models have shown surprising in-context learning (ICL) ability. With a few demonstration input-label pairs, they can predict the label for an unseen input without parameter updates. Despite the great success in performance, its working mechanism still remains an open question. In this paper, we explain language models as meta-optimizers and understand in-context learning as implicit finetuning. Theoretically, we figure out that Transformer attention has a dual form of gradient descent. On top of it, we understand ICL as follows: GPT first produces meta-gradients according to the demonstration examples, and then these meta-gradients are applied to the original GPT to build an ICL model. We comprehensively compare the behaviors of in-context learning and explicit finetuning on real tasks to provide empirical evidence that supports our understanding. Experimental results show that in-context learning behaves similarly to explicit finetuning from multiple perspectives. Inspired by the dual form between Transformer attention and gradient descent, we design a momentum-based attention by analogy with gradient descent with momentum. The improved performance over vanilla attention further supports our understanding from another perspective, and more importantly, shows the potential to utilize our understanding for future model design. The code is available at \textbackslash url\{https://aka.ms/icl\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Dai et al_2023_Why Can GPT Learn In-Context.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RC3NFN3U\\2212.html}
}

@online{dalviAnalyzingRedundancyPretrained2020,
  title = {Analyzing {{Redundancy}} in {{Pretrained Transformer Models}}},
  author = {Dalvi, Fahim and Sajjad, Hassan and Durrani, Nadir and Belinkov, Yonatan},
  date = {2020-10-06},
  eprint = {2004.04010},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2004.04010},
  url = {http://arxiv.org/abs/2004.04010},
  urldate = {2024-04-18},
  abstract = {Transformer-based deep NLP models are trained using hundreds of millions of parameters, limiting their applicability in computationally constrained environments. In this paper, we study the cause of these limitations by defining a notion of Redundancy, which we categorize into two classes: General Redundancy and Task-specific Redundancy. We dissect two popular pretrained models, BERT and XLNet, studying how much redundancy they exhibit at a representation-level and at a more fine-grained neuron-level. Our analysis reveals interesting insights, such as: i) 85\% of the neurons across the network are redundant and ii) at least 92\% of them can be removed when optimizing towards a downstream task. Based on our analysis, we present an efficient feature-based transfer learning procedure, which maintains 97\% performance while using at-most 10\% of the original neurons.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Dalvi et al_2020_Analyzing Redundancy in Pretrained Transformer Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2HKLXV3K\\2004.html}
}

@article{danielczukCreating3DReconstructions,
  title = {Towards {{Creating 3D Reconstructions}} of {{Semi-Transparent Objects}}},
  author = {Danielczuk, Michael and Bucki, Nathan and Agrawal, Ayush},
  abstract = {Many semi-transparent objects are common household objects, and often used in everyday manipulation tasks, requiring that they be perceived effectively. Although object detection and recognition has been applied with good results to opaque objects, semitransparent objects typically pose problems for these algorithms. In this paper, we implement two methods for 3D reconstruction of semi-transparent objects: (1) Mask Re-projection and (2) Multiview Consistency. The first method re-projects image masks of the object from different cameras into 3D space to recreate a 3D mesh of the object. The second method implements a convolutional neural network to compute the 3D shape and pose of the object using a single input image. We also collected a fairly large dataset of transparent objects, such as cups, wine glasses and mugs, consisting of images of the objects taken at different camera poses and background lighting conditions, as well as the corresponding object masks.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\SY3EJ3RR\Danielczuk 등 - Towards Creating 3D Reconstructions of Semi-Transp.pdf}
}

@online{DanpingZouShanghai,
  title = {Danping {{Zou}} - {{Shanghai Jiao Tong University}}},
  url = {https://drone.sjtu.edu.cn/dpzou/teaching.php},
  urldate = {2023-01-26},
  file = {C:\Users\chsey\Zotero\storage\CRGQZCK7\teaching.html}
}

@online{darcetVisionTransformersNeed2024,
  title = {Vision {{Transformers Need Registers}}},
  author = {Darcet, Timothée and Oquab, Maxime and Mairal, Julien and Bojanowski, Piotr},
  date = {2024-04-12},
  eprint = {2309.16588},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2309.16588},
  urldate = {2024-06-22},
  abstract = {Transformers have recently emerged as a powerful tool for learning visual representations. In this paper, we identify and characterize artifacts in feature maps of both supervised and self-supervised ViT networks. The artifacts correspond to high-norm tokens appearing during inference primarily in low-informative background areas of images, that are repurposed for internal computations. We propose a simple yet effective solution based on providing additional tokens to the input sequence of the Vision Transformer to fill that role. We show that this solution fixes that problem entirely for both supervised and self-supervised models, sets a new state of the art for self-supervised visual models on dense visual prediction tasks, enables object discovery methods with larger models, and most importantly leads to smoother feature maps and attention maps for downstream visual processing.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\NFQW777M\Darcet 등 - 2024 - Vision Transformers Need Registers.pdf}
}

@online{dasLearningExpressivePrompting2023,
  title = {Learning {{Expressive Prompting With Residuals}} for {{Vision Transformers}}},
  author = {Das, Rajshekhar and Dukler, Yonatan and Ravichandran, Avinash and Swaminathan, Ashwin},
  date = {2023-03-27},
  eprint = {2303.15591},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.15591},
  url = {http://arxiv.org/abs/2303.15591},
  urldate = {2023-06-29},
  abstract = {Prompt learning is an efficient approach to adapt transformers by inserting learnable set of parameters into the input and intermediate representations of a pre-trained model. In this work, we present Expressive Prompts with Residuals (EXPRES) which modifies the prompt learning paradigm specifically for effective adaptation of vision transformers (ViT). Out method constructs downstream representations via learnable ``output'' tokens, that are akin to the learned class tokens of the ViT. Further for better steering of the downstream representation processed by the frozen transformer, we introduce residual learnable tokens that are added to the output of various computations. We apply EXPRES for image classification, few shot learning, and semantic segmentation, and show our method is capable of achieving state of the art prompt tuning on 3/3 categories of the VTAB benchmark. In addition to strong performance, we observe that our approach is an order of magnitude more prompt efficient than existing visual prompting baselines. We analytically show the computational benefits of our approach over weight space adaptation techniques like finetuning. Lastly we systematically corroborate the architectural design of our method via a series of ablation experiments.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Das et al_2023_Learning Expressive Prompting With Residuals for Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DNM7NJP6\\2303.html}
}

@online{dasVisualDialog2017,
  title = {Visual {{Dialog}}},
  author = {Das, Abhishek and Kottur, Satwik and Gupta, Khushi and Singh, Avi and Yadav, Deshraj and Moura, José M. F. and Parikh, Devi and Batra, Dhruv},
  date = {2017-08-01},
  eprint = {1611.08669},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1611.08669},
  url = {http://arxiv.org/abs/1611.08669},
  urldate = {2023-08-05},
  abstract = {We introduce the task of Visual Dialog, which requires an AI agent to hold a meaningful dialog with humans in natural, conversational language about visual content. Specifically, given an image, a dialog history, and a question about the image, the agent has to ground the question in image, infer context from history, and answer the question accurately. Visual Dialog is disentangled enough from a specific downstream task so as to serve as a general test of machine intelligence, while being grounded in vision enough to allow objective evaluation of individual responses and benchmark progress. We develop a novel two-person chat data-collection protocol to curate a large-scale Visual Dialog dataset (VisDial). VisDial v0.9 has been released and contains 1 dialog with 10 question-answer pairs on \textasciitilde 120k images from COCO, with a total of \textasciitilde 1.2M dialog question-answer pairs. We introduce a family of neural encoder-decoder models for Visual Dialog with 3 encoders -- Late Fusion, Hierarchical Recurrent Encoder and Memory Network -- and 2 decoders (generative and discriminative), which outperform a number of sophisticated baselines. We propose a retrieval-based evaluation protocol for Visual Dialog where the AI agent is asked to sort a set of candidate answers and evaluated on metrics such as mean-reciprocal-rank of human response. We quantify gap between machine and human performance on the Visual Dialog task via human studies. Putting it all together, we demonstrate the first 'visual chatbot'! Our dataset, code, trained models and visual chatbot are available on https://visualdialog.org},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\vision and language\\Das et al_2017_Visual Dialog.pdf;C\:\\Users\\chsey\\Zotero\\storage\\75A5SKZP\\1611.html}
}

@inproceedings{davisRelationshipPrecisionRecallROC2006,
  title = {The Relationship between {{Precision-Recall}} and {{ROC}} Curves},
  booktitle = {Proceedings of the 23rd International Conference on {{Machine}} Learning  - {{ICML}} '06},
  author = {Davis, Jesse and Goadrich, Mark},
  date = {2006},
  pages = {233--240},
  publisher = {ACM Press},
  location = {Pittsburgh, Pennsylvania},
  doi = {10.1145/1143844.1143874},
  url = {http://portal.acm.org/citation.cfm?doid=1143844.1143874},
  urldate = {2022-09-06},
  abstract = {Receiver Operator Characteristic (ROC) curves are commonly used to present results for binary decision problems in machine learning. However, when dealing with highly skewed datasets, Precision-Recall (PR) curves give a more informative picture of an algorithm’s performance. We show that a deep connection exists between ROC space and PR space, such that a curve dominates in ROC space if and only if it dominates in PR space. A corollary is the notion of an achievable PR curve, which has properties much like the convex hull in ROC space; we show an efficient algorithm for computing this curve. Finally, we also note differences in the two types of curves are significant for algorithm design. For example, in PR space it is incorrect to linearly interpolate between points. Furthermore, algorithms that optimize the area under the ROC curve are not guaranteed to optimize the area under the PR curve.},
  eventtitle = {The 23rd International Conference},
  isbn = {978-1-59593-383-6},
  langid = {english},
  file = {Y:\paper\2022 autumn intern\OOD\Davis_Goadrich_2006_The relationship between Precision-Recall and ROC curves.pdf}
}

@online{debbaghNeuralRadianceFields2023,
  title = {Neural {{Radiance Fields}} ({{NeRFs}}): {{A Review}} and {{Some Recent Developments}}},
  shorttitle = {Neural {{Radiance Fields}} ({{NeRFs}})},
  author = {Debbagh, Mohamed},
  date = {2023-04-29},
  eprint = {2305.00375},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  doi = {10.48550/arXiv.2305.00375},
  url = {http://arxiv.org/abs/2305.00375},
  urldate = {2023-06-24},
  abstract = {Neural Radiance Field (NeRF) is a framework that represents a 3D scene in the weights of a fully connected neural network, known as the Multi-Layer Perception(MLP). The method was introduced for the task of novel view synthesis and is able to achieve state-of-the-art photorealistic image renderings from a given continuous viewpoint. NeRFs have become a popular field of research as recent developments have been made that expand the performance and capabilities of the base framework. Recent developments include methods that require less images to train the model for view synthesis as well as methods that are able to generate views from unconstrained and dynamic scene representations.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\2022 winter intern\\NeRF_review\\Debbagh_2023_Neural Radiance Fields (NeRFs).pdf;C\:\\Users\\chsey\\Zotero\\storage\\2BXNI5YV\\2305.html}
}

@online{DeepAnomalyGoogle,
  title = {Deep Anomaly - {{Google}} 검색},
  url = {https://www.google.com/search?q=deep+anomlay&oq=deep+anomlay&aqs=chrome..69i57.2731j0j4&sourceid=chrome&ie=UTF-8},
  urldate = {2022-09-21},
  file = {C:\Users\chsey\Zotero\storage\226RW7YP\search.html}
}

@online{DeepAnomalyGooglea,
  title = {Deep Anomaly - {{Google}} 검색},
  url = {https://www.google.com/search?q=deep+anomlay&oq=deep+anomlay&aqs=chrome..69i57.2731j0j4&sourceid=chrome&ie=UTF-8},
  urldate = {2022-09-21}
}

@online{dehghaniScalingVisionTransformers2023,
  title = {Scaling {{Vision Transformers}} to 22 {{Billion Parameters}}},
  author = {Dehghani, Mostafa and Djolonga, Josip and Mustafa, Basil and Padlewski, Piotr and Heek, Jonathan and Gilmer, Justin and Steiner, Andreas and Caron, Mathilde and Geirhos, Robert and Alabdulmohsin, Ibrahim and Jenatton, Rodolphe and Beyer, Lucas and Tschannen, Michael and Arnab, Anurag and Wang, Xiao and Riquelme, Carlos and Minderer, Matthias and Puigcerver, Joan and Evci, Utku and Kumar, Manoj and family=Steenkiste, given=Sjoerd, prefix=van, useprefix=true and Elsayed, Gamaleldin F. and Mahendran, Aravindh and Yu, Fisher and Oliver, Avital and Huot, Fantine and Bastings, Jasmijn and Collier, Mark Patrick and Gritsenko, Alexey and Birodkar, Vighnesh and Vasconcelos, Cristina and Tay, Yi and Mensink, Thomas and Kolesnikov, Alexander and Pavetić, Filip and Tran, Dustin and Kipf, Thomas and Lučić, Mario and Zhai, Xiaohua and Keysers, Daniel and Harmsen, Jeremiah and Houlsby, Neil},
  date = {2023-02-10},
  eprint = {2302.05442},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2302.05442},
  url = {http://arxiv.org/abs/2302.05442},
  urldate = {2023-07-26},
  abstract = {The scaling of Transformers has driven breakthrough capabilities for language models. At present, the largest large language models (LLMs) contain upwards of 100B parameters. Vision Transformers (ViT) have introduced the same architecture to image and video modelling, but these have not yet been successfully scaled to nearly the same degree; the largest dense ViT contains 4B parameters (Chen et al., 2022). We present a recipe for highly efficient and stable training of a 22B-parameter ViT (ViT-22B) and perform a wide variety of experiments on the resulting model. When evaluated on downstream tasks (often with a lightweight linear model on frozen features), ViT-22B demonstrates increasing performance with scale. We further observe other interesting benefits of scale, including an improved tradeoff between fairness and performance, state-of-the-art alignment to human visual perception in terms of shape/texture bias, and improved robustness. ViT-22B demonstrates the potential for "LLM-like" scaling in vision, and provides key steps towards getting there.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Dehghani et al_2023_Scaling Vision Transformers to 22 Billion Parameters.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RJ52R7S7\\2302.html}
}

@online{deletangLanguageModelingCompression2024,
  title = {Language {{Modeling Is Compression}}},
  author = {Delétang, Grégoire and Ruoss, Anian and Duquenne, Paul-Ambroise and Catt, Elliot and Genewein, Tim and Mattern, Christopher and Grau-Moya, Jordi and Wenliang, Li Kevin and Aitchison, Matthew and Orseau, Laurent and Hutter, Marcus and Veness, Joel},
  date = {2024-03-18},
  eprint = {2309.10668},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/2309.10668},
  urldate = {2024-04-21},
  abstract = {It has long been established that predictive models can be transformed into lossless compressors and vice versa. Incidentally, in recent years, the machine learning community has focused on training increasingly large and powerful self-supervised (language) models. Since these large language models exhibit impressive predictive capabilities, they are well-positioned to be strong compressors. In this work, we advocate for viewing the prediction problem through the lens of compression and evaluate the compression capabilities of large (foundation) models. We show that large language models are powerful general-purpose predictors and that the compression viewpoint provides novel insights into scaling laws, tokenization, and in-context learning. For example, Chinchilla 70B, while trained primarily on text, compresses ImageNet patches to 43.4\% and LibriSpeech samples to 16.4\% of their raw size, beating domain-specific compressors like PNG (58.5\%) or FLAC (30.3\%), respectively. Finally, we show that the prediction-compression equivalence allows us to use any compressor (like gzip) to build a conditional generative model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Information Theory,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Delétang et al_2024_Language Modeling Is Compression.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QHLRLKGC\\2309.html}
}

@online{dengDepthsupervisedNeRFFewer2022,
  title = {Depth-Supervised {{NeRF}}: {{Fewer Views}} and {{Faster Training}} for {{Free}}},
  shorttitle = {Depth-Supervised {{NeRF}}},
  author = {Deng, Kangle and Liu, Andrew and Zhu, Jun-Yan and Ramanan, Deva},
  date = {2022-04-29},
  eprint = {2107.02791},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2107.02791},
  urldate = {2023-02-06},
  abstract = {A commonly observed failure mode of Neural Radiance Field (NeRF) is fitting incorrect geometries when given an insufficient number of input views. One potential reason is that standard volumetric rendering does not enforce the constraint that most of a scene's geometry consist of empty space and opaque surfaces. We formalize the above assumption through DS-NeRF (Depth-supervised Neural Radiance Fields), a loss for learning radiance fields that takes advantage of readily-available depth supervision. We leverage the fact that current NeRF pipelines require images with known camera poses that are typically estimated by running structure-from-motion (SFM). Crucially, SFM also produces sparse 3D points that can be used as "free" depth supervision during training: we add a loss to encourage the distribution of a ray's terminating depth matches a given 3D keypoint, incorporating depth uncertainty. DS-NeRF can render better images given fewer training views while training 2-3x faster. Further, we show that our loss is compatible with other recently proposed NeRF methods, demonstrating that depth is a cheap and easily digestible supervisory signal. And finally, we find that DS-NeRF can support other types of depth supervision such as scanned depth sensors and RGB-D reconstruction outputs.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Deng et al_2022_Depth-supervised NeRF2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5QLQB52K\\2107.html}
}

@inproceedings{dengDepthsupervisedNeRFFewer2022a,
  title = {Depth-Supervised {{NeRF}}: {{Fewer Views}} and {{Faster Training}} for {{Free}}},
  shorttitle = {Depth-Supervised {{NeRF}}},
  booktitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Deng, Kangle and Liu, Andrew and Zhu, Jun-Yan and Ramanan, Deva},
  date = {2022-06},
  pages = {12872--12881},
  publisher = {IEEE},
  location = {New Orleans, LA, USA},
  doi = {10.1109/CVPR52688.2022.01254},
  url = {https://ieeexplore.ieee.org/document/9880067/},
  urldate = {2023-01-17},
  eventtitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-66546-946-3},
  langid = {english},
  file = {Y:\paper\2022 winter intern\Deng et al_2022_Depth-supervised NeRF.pdf}
}

@inproceedings{derakhshaniBayesianPromptLearning2023,
  title = {Bayesian {{Prompt Learning}} for {{Image-Language Model Generalization}}},
  author = {Derakhshani, Mohammad Mahdi and Sanchez, Enrique and Bulat, Adrian and family=Costa, given=Victor G. Turrisi, prefix=da, useprefix=true and Snoek, Cees G. M. and Tzimiropoulos, Georgios and Martinez, Brais},
  date = {2023},
  pages = {15237--15246},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Derakhshani_Bayesian_Prompt_Learning_for_Image-Language_Model_Generalization_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Derakhshani et al_2023_Bayesian Prompt Learning for Image-Language Model Generalization.pdf}
}

@online{DescribableTexturesDataset,
  title = {Describable {{Textures Dataset}}},
  url = {https://www.robots.ox.ac.uk/~vgg/data/dtd/},
  urldate = {2022-11-15},
  file = {C:\Users\chsey\Zotero\storage\2WJZTY8F\dtd.html}
}

@online{deshmukhPengiAudioLanguage2024,
  title = {Pengi: {{An Audio Language Model}} for {{Audio Tasks}}},
  shorttitle = {Pengi},
  author = {Deshmukh, Soham and Elizalde, Benjamin and Singh, Rita and Wang, Huaming},
  date = {2024-01-18},
  eprint = {2305.11834},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2305.11834},
  urldate = {2024-07-04},
  abstract = {In the domain of audio processing, Transfer Learning has facilitated the rise of Self-Supervised Learning and Zero-Shot Learning techniques. These approaches have led to the development of versatile models capable of tackling a wide array of tasks, while delivering state-of-the-art performance. However, current models inherently lack the capacity to produce the requisite language for open-ended tasks, such as Audio Captioning or Audio Question Answering. We introduce Pengi, a novel Audio Language Model that leverages Transfer Learning by framing all audio tasks as text-generation tasks. It takes as input, an audio recording, and text, and generates free-form text as output. The input audio is represented as a sequence of continuous embeddings by an audio encoder. A text encoder does the same for the corresponding text input. Both sequences are combined as a prefix to prompt a pre-trained frozen language model. The unified architecture of Pengi enables open-ended tasks and close-ended tasks without any additional fine-tuning or task-specific extensions. When evaluated on 21 downstream tasks, our approach yields state-of-the-art performance in several of them. Our results show that connecting language models with audio models is a major step towards general-purpose audio understanding 1.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Sound,Electrical Engineering and Systems Science - Audio and Speech Processing,notion},
  file = {C:\Users\chsey\Zotero\storage\UFN5BJCS\2305.pdf}
}

@online{DetectionCovid19Chest,
  title = {Detection of {{Covid-19}} in {{Chest X-ray Image}} Using {{CLAHE}} and {{Convolutional Neural Network}} | {{IEEE Conference Publication}} | {{IEEE Xplore}}},
  url = {https://ieeexplore.ieee.org/abstract/document/9320806},
  urldate = {2022-07-09},
  file = {C:\Users\chsey\Zotero\storage\U2N5WTXV\9320806.html}
}

@online{dettmersSpQRSparseQuantizedRepresentation2023,
  title = {{{SpQR}}: {{A Sparse-Quantized Representation}} for {{Near-Lossless LLM Weight Compression}}},
  shorttitle = {{{SpQR}}},
  author = {Dettmers, Tim and Svirschevski, Ruslan and Egiazarian, Vage and Kuznedelev, Denis and Frantar, Elias and Ashkboos, Saleh and Borzunov, Alexander and Hoefler, Torsten and Alistarh, Dan},
  date = {2023-06-05},
  eprint = {2306.03078},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2306.03078},
  url = {http://arxiv.org/abs/2306.03078},
  urldate = {2024-04-16},
  abstract = {Recent advances in large language model (LLM) pretraining have led to high-quality LLMs with impressive abilities. By compressing such LLMs via quantization to 3-4 bits per parameter, they can fit into memory-limited devices such as laptops and mobile phones, enabling personalized use. However, quantization down to 3-4 bits per parameter usually leads to moderate-to-high accuracy losses, especially for smaller models in the 1-10B parameter range, which are well-suited for edge deployments. To address this accuracy issue, we introduce the Sparse-Quantized Representation (SpQR), a new compressed format and quantization technique which enables for the first time near-lossless compression of LLMs across model scales, while reaching similar compression levels to previous methods. SpQR works by identifying and isolating outlier weights, which cause particularly-large quantization errors, and storing them in higher precision, while compressing all other weights to 3-4 bits, and achieves relative accuracy losses of less than 1\% in perplexity for highly-accurate LLaMA and Falcon LLMs. This makes it possible to run 33B parameter LLM on a single 24 GB consumer GPU without any performance degradation at 15\% speedup thus making powerful LLMs available to consumer without any downsides. SpQR comes with efficient algorithms for both encoding weights into its format, as well as decoding them efficiently at runtime. Specifically, we provide an efficient GPU inference algorithm for SpQR which yields faster inference than 16-bit baselines at similar accuracy, while enabling memory compression gains of more than 4x.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Dettmers et al_2023_SpQR.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MJX5VIX5\\2306.html}
}

@online{devlinBERTPretrainingDeep2019,
  title = {{{BERT}}: {{Pre-training}} of {{Deep Bidirectional Transformers}} for {{Language Understanding}}},
  shorttitle = {{{BERT}}},
  author = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  date = {2019-05-24},
  eprint = {1810.04805},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1810.04805},
  url = {http://arxiv.org/abs/1810.04805},
  urldate = {2024-02-10},
  abstract = {We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models, BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5\% (7.7\% point absolute improvement), MultiNLI accuracy to 86.7\% (4.6\% absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Devlin et al_2019_BERT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HE63CTWI\\1810.html}
}

@online{devlinBERTPretrainingDeep2019a,
  title = {{{BERT}}: {{Pre-training}} of {{Deep Bidirectional Transformers}} for {{Language Understanding}}},
  shorttitle = {{{BERT}}},
  author = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  date = {2019-05-24},
  eprint = {1810.04805},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1810.04805},
  url = {http://arxiv.org/abs/1810.04805},
  urldate = {2023-11-17},
  abstract = {We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models, BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5\% (7.7\% point absolute improvement), MultiNLI accuracy to 86.7\% (4.6\% absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\Devlin et al_2019_BERT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WNHDES7W\\1810.html}
}

@online{dingSparseLowrankAdaptation2023,
  title = {Sparse {{Low-rank Adaptation}} of {{Pre-trained Language Models}}},
  author = {Ding, Ning and Lv, Xingtai and Wang, Qiaosen and Chen, Yulin and Zhou, Bowen and Liu, Zhiyuan and Sun, Maosong},
  date = {2023-11-20},
  eprint = {2311.11696},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2311.11696},
  url = {http://arxiv.org/abs/2311.11696},
  urldate = {2024-03-18},
  abstract = {Fine-tuning pre-trained large language models in a parameter-efficient manner is widely studied for its effectiveness and efficiency. The popular method of low-rank adaptation (LoRA) offers a notable approach, hypothesizing that the adaptation process is intrinsically low-dimensional. Although LoRA has demonstrated commendable performance, it is implemented with a fixed and unalterable intrinsic rank that might not always be the ideal choice. Recognizing the need for more flexible adaptation, we extend the methodology of LoRA to an innovative approach we call sparse low-rank adaptation (SoRA) that enables dynamic adjustments to the intrinsic rank during the adaptation process. We achieve this through the incorporation of a gate unit optimized with proximal gradient method in the training stage, controlling the cardinality of rank under the sparsity of the gate. In the subsequent inference stage, we eliminate the parameter blocks corresponding to the zeroed-out ranks, to reduce each SoRA module back to a concise yet rank-optimal LoRA. Our approach strengthens the representation power of LoRA by initializing it with a higher rank, while efficiently taming a temporarily increased number of parameters via updating in a sparse way. We further introduce a sparsifying scheduler for SoRA, aiming to examine the impact of the number of non-zero parameters on the model's memorization and generalization. Our experimental results demonstrate that SoRA can outperform other baselines even with 70\% retained parameters and 70\% training time.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Ding et al_2023_Sparse Low-rank Adaptation of Pre-trained Language Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BATQUADE\\2311.html}
}

@online{Doi101016,
  title = {Doi:10.1016/j.Cviu.2005.06.001 | {{Elsevier Enhanced Reader}}},
  shorttitle = {Doi},
  doi = {10.1016/j.cviu.2005.06.001},
  url = {https://reader.elsevier.com/reader/sd/pii/S1077314205000846?token=58F2ABE7860D75095E10EA5DF9921FABED5A26312410F2CA8B7A2E396B4F06992DFE6E513FD960E4BC4FFE054683451B&originRegion=us-east-1&originCreation=20230126081629},
  urldate = {2023-01-26},
  langid = {english},
  file = {Y:\paper\2022 winter intern\gemmetric\doi.pdf}
}

@online{donahueDeCAFDeepConvolutional2013,
  title = {{{DeCAF}}: {{A Deep Convolutional Activation Feature}} for {{Generic Visual Recognition}}},
  shorttitle = {{{DeCAF}}},
  author = {Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
  date = {2013-10-05},
  eprint = {1310.1531},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1310.1531},
  urldate = {2022-12-21},
  abstract = {We evaluate whether features extracted from the activation of a deep convolutional network trained in a fully supervised fashion on a large, fixed set of object recognition tasks can be re-purposed to novel generic tasks. Our generic tasks may differ significantly from the originally trained tasks and there may be insufficient labeled or unlabeled data to conventionally train or adapt a deep architecture to the new tasks. We investigate and visualize the semantic clustering of deep convolutional features with respect to a variety of such tasks, including scene recognition, domain adaptation, and fine-grained recognition challenges. We compare the efficacy of relying on various network levels to define a fixed feature, and report novel results that significantly outperform the state-of-the-art on several important vision challenges. We are releasing DeCAF, an open-source implementation of these deep convolutional activation features, along with all associated network parameters to enable vision researchers to be able to conduct experimentation with deep representations across a range of visual concept learning paradigms.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Donahue et al_2013_DeCAF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4GTFFTVT\\1310.html}
}

@inproceedings{dongPromptTuningInversion2023,
  title = {Prompt {{Tuning Inversion}} for {{Text-driven Image Editing Using Diffusion Models}}},
  author = {Dong, Wenkai and Xue, Song and Duan, Xiaoyue and Han, Shumin},
  date = {2023},
  pages = {7430--7440},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Dong_Prompt_Tuning_Inversion_for_Text-driven_Image_Editing_Using_Diffusion_Models_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Dong et al_2023_Prompt Tuning Inversion for Text-driven Image Editing Using Diffusion Models.pdf}
}

@online{dorflerSystemsTheoryAlgorithms2024,
  title = {Towards a {{Systems Theory}} of {{Algorithms}}},
  author = {Dörfler, Florian and He, Zhiyu and Belgioioso, Giuseppe and Bolognani, Saverio and Lygeros, John and Muehlebach, Michael},
  date = {2024-01-25},
  eprint = {2401.14029},
  eprinttype = {arXiv},
  eprintclass = {cs, eess, math},
  url = {http://arxiv.org/abs/2401.14029},
  urldate = {2024-01-29},
  abstract = {Traditionally, numerical algorithms are seen as isolated pieces of code confined to an \{\textbackslash em in silico\} existence. However, this perspective is not appropriate for many modern computational approaches in control, learning, or optimization, wherein \{\textbackslash em in vivo\} algorithms interact with their environment. Examples of such \{\textbackslash em open\} include various real-time optimization-based control strategies, reinforcement learning, decision-making architectures, online optimization, and many more. Further, even \{\textbackslash em closed\} algorithms in learning or optimization are increasingly abstracted in block diagrams with interacting dynamic modules and pipelines. In this opinion paper, we state our vision on a to-be-cultivated \{\textbackslash em systems theory of algorithms\} and argue in favour of viewing algorithms as open dynamical systems interacting with other algorithms, physical systems, humans, or databases. Remarkably, the manifold tools developed under the umbrella of systems theory also provide valuable insights into this burgeoning paradigm shift and its accompanying challenges in the algorithmic world. We survey various instances where the principles of algorithmic systems theory are being developed and outline pertinent modeling, analysis, and design challenges.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Electrical Engineering and Systems Science - Systems and Control,Mathematics - Optimization and Control,notion},
  file = {Y\:\\paper\\2024_research\\Dörfler et al_2024_Towards a Systems Theory of Algorithms.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HBLRZA3V\\2401.html}
}

@online{dosovitskiyImageWorth16x162021,
  title = {An {{Image}} Is {{Worth}} 16x16 {{Words}}: {{Transformers}} for {{Image Recognition}} at {{Scale}}},
  shorttitle = {An {{Image}} Is {{Worth}} 16x16 {{Words}}},
  author = {Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
  date = {2021-06-03},
  eprint = {2010.11929},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2010.11929},
  url = {http://arxiv.org/abs/2010.11929},
  urldate = {2022-08-10},
  abstract = {While the Transformer architecture has become the de-facto standard for natural language processing tasks, its applications to computer vision remain limited. In vision, attention is either applied in conjunction with convolutional networks, or used to replace certain components of convolutional networks while keeping their overall structure in place. We show that this reliance on CNNs is not necessary and a pure transformer applied directly to sequences of image patches can perform very well on image classification tasks. When pre-trained on large amounts of data and transferred to multiple mid-sized or small image recognition benchmarks (ImageNet, CIFAR-100, VTAB, etc.), Vision Transformer (ViT) attains excellent results compared to state-of-the-art convolutional networks while requiring substantially fewer computational resources to train.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Dosovitskiy et al_2021_An Image is Worth 16x16 Words.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FGJQTKXJ\\2010.html}
}

@online{douEmpiricalStudyTraining2022,
  title = {An {{Empirical Study}} of {{Training End-to-End Vision-and-Language Transformers}}},
  author = {Dou, Zi-Yi and Xu, Yichong and Gan, Zhe and Wang, Jianfeng and Wang, Shuohang and Wang, Lijuan and Zhu, Chenguang and Zhang, Pengchuan and Yuan, Lu and Peng, Nanyun and Liu, Zicheng and Zeng, Michael},
  date = {2022-03-17},
  eprint = {2111.02387},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.02387},
  url = {http://arxiv.org/abs/2111.02387},
  urldate = {2024-04-25},
  abstract = {Vision-and-language (VL) pre-training has proven to be highly effective on various VL downstream tasks. While recent work has shown that fully transformer-based VL models can be more efficient than previous region-feature-based methods, their performance on downstream tasks often degrades significantly. In this paper, we present METER, a Multimodal End-to-end TransformER framework, through which we investigate how to design and pre-train a fully transformer-based VL model in an end-to-end manner. Specifically, we dissect the model designs along multiple dimensions: vision encoders (e.g., CLIP-ViT, Swin transformer), text encoders (e.g., RoBERTa, DeBERTa), multimodal fusion module (e.g., merged attention vs. co-attention), architectural design (e.g., encoder-only vs. encoder-decoder), and pre-training objectives (e.g., masked image modeling). We conduct comprehensive experiments and provide insights on how to train a performant VL transformer. METER achieves an accuracy of 77.64\% on the VQAv2 test-std set using only 4M images for pre-training, surpassing the state-of-the-art region-feature-based model by 1.04\%, and outperforming the previous best fully transformer-based model by 1.6\%. Notably, when further scaled up, our best VQA model achieves an accuracy of 80.54\%. Code and pre-trained models are released at https://github.com/zdou0830/METER.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Dou et al_2022_An Empirical Study of Training End-to-End Vision-and-Language Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KHLML8U6\\2111.html}
}

@online{douillardDyToxTransformersContinual2022,
  title = {{{DyTox}}: {{Transformers}} for {{Continual Learning}} with {{DYnamic TOken eXpansion}}},
  shorttitle = {{{DyTox}}},
  author = {Douillard, Arthur and Ramé, Alexandre and Couairon, Guillaume and Cord, Matthieu},
  date = {2022-08-07},
  eprint = {2111.11326},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.11326},
  url = {http://arxiv.org/abs/2111.11326},
  urldate = {2023-12-24},
  abstract = {Deep network architectures struggle to continually learn new tasks without forgetting the previous tasks. A recent trend indicates that dynamic architectures based on an expansion of the parameters can reduce catastrophic forgetting efficiently in continual learning. However, existing approaches often require a task identifier at test-time, need complex tuning to balance the growing number of parameters, and barely share any information across tasks. As a result, they struggle to scale to a large number of tasks without significant overhead. In this paper, we propose a transformer architecture based on a dedicated encoder/decoder framework. Critically, the encoder and decoder are shared among all tasks. Through a dynamic expansion of special tokens, we specialize each forward of our decoder network on a task distribution. Our strategy scales to a large number of tasks while having negligible memory and time overheads due to strict control of the parameters expansion. Moreover, this efficient strategy doesn't need any hyperparameter tuning to control the network's expansion. Our model reaches excellent results on CIFAR100 and state-of-the-art performances on the large-scale ImageNet100 and ImageNet1000 while having less parameters than concurrent dynamic frameworks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\incremental_learning\\Douillard et al_2022_DyTox.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EIZQG828\\2111.html}
}

@inproceedings{douillardDyToxTransformersContinual2022a,
  title = {{{DyTox}}: {{Transformers}} for {{Continual Learning}} with {{DYnamic TOken eXpansion}}},
  shorttitle = {{{DyTox}}},
  booktitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Douillard, Arthur and Rame, Alexandre and Couairon, Guillaume and Cord, Matthieu},
  date = {2022-06},
  pages = {9275--9285},
  publisher = {IEEE},
  location = {New Orleans, LA, USA},
  doi = {10.1109/CVPR52688.2022.00907},
  url = {https://ieeexplore.ieee.org/document/9880199/},
  urldate = {2023-12-24},
  abstract = {Deep network architectures struggle to continually learn new tasks without forgetting the previous tasks. A recent trend indicates that dynamic architectures based on an expansion of the parameters can reduce catastrophic forgetting efficiently in continual learning. However, existing approaches often require a task identifier at test-time, need complex tuning to balance the growing number of parameters, and barely share any information across tasks. As a result, they struggle to scale to a large number of tasks without significant overhead.},
  eventtitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-66546-946-3},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\GQDFMB29\Douillard 등 - 2022 - DyTox Transformers for Continual Learning with DY.pdf}
}

@inproceedings{duCatchMeIf2016,
  title = {Catch {{Me If You Can}}: {{Detecting Pickpocket Suspects}} from {{Large-Scale Transit Records}}},
  shorttitle = {Catch {{Me If You Can}}},
  booktitle = {Proceedings of the 22nd {{ACM SIGKDD International Conference}} on {{Knowledge Discovery}} and {{Data Mining}}},
  author = {Du, Bowen and Liu, Chuanren and Zhou, Wenjun and Hou, Zhenshan and Xiong, Hui},
  year = {8월 13, 2016},
  series = {{{KDD}} '16},
  pages = {87--96},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/2939672.2939687},
  url = {https://doi.org/10.1145/2939672.2939687},
  urldate = {2023-05-24},
  abstract = {Massive data collected by automated fare collection (AFC) systems provide opportunities for studying both personal traveling behaviors and collective mobility patterns in the urban area. Existing studies on the AFC data have primarily focused on identifying passengers' movement patterns. In this paper, however, we creatively leveraged such data for identifying thieves in the public transit systems. Indeed, stopping pickpockets in the public transit systems has been critical for improving passenger satisfaction and public safety. However, it is challenging to tell thieves from regular passengers in practice. To this end, we developed a suspect detection and surveillance system, which can identify pick-pocket suspects based on their daily transit records. Specifically, we first extracted a number of features from each passenger's daily activities in the transit systems. Then, we took a two-step approach that exploits the strengths of unsupervised outlier detection and supervised classification models to identify thieves, who exhibit abnormal traveling behaviors. Experimental results demonstrated the effective- ness of our method. We also developed a prototype system with a user-friendly interface for the security personnel.},
  isbn = {978-1-4503-4232-2},
  keywords = {anomaly detection,automated fare collection,mobility patterns,public safety,travel behaviors}
}

@book{duMechanicsMechanicalWatches2012,
  title = {The {{Mechanics}} of {{Mechanical Watches}} and {{Clocks}}},
  author = {Du, Ruxu and Xie, Longhan},
  date = {2012-09-21},
  eprint = {ASi7L2MAmkgC},
  eprinttype = {googlebooks},
  publisher = {Springer Science \& Business Media},
  abstract = {"The Mechanics of Mechanical Watches and Clocks" presents historical views and mathematical models of mechanical watches and clocks. Although now over six hundred years old, mechanical watches and clocks are still popular luxury items that fascinate many people around the world. However few have examined the theory of how they work as presented in this book. The illustrations and computer animations are unique and have never been published before.It will be of significant interest to researchers in mechanical engineering, watchmakers and clockmakers, as well as people who have an engineering background and are interested in mechanical watches and clocks. It will also inspire people in other fields of science and technology, such as mechanical engineering and electronics engineering, to advance their designs.Professor Ruxu Du works at the Chinese University of Hong Kong, China. Assistant Professor Longhan Xie works at the South China University of Technology, China.},
  isbn = {978-3-642-29307-8},
  langid = {english},
  pagetotal = {182},
  keywords = {Mathematics / Probability & Statistics / Stochastic Processes,Science / Mechanics / General,Science / Mechanics / Solids,Technology & Engineering / Mechanical},
  file = {Y:\paper\management\Du_Xie_2012_The Mechanics of Mechanical Watches and Clocks.pdf}
}

@online{dwivediRepresentationSimilarityAnalysis2019,
  title = {Representation {{Similarity Analysis}} for {{Efficient Task}} Taxonomy \& {{Transfer Learning}}},
  author = {Dwivedi, Kshitij and Roig, Gemma},
  date = {2019-04-26},
  eprint = {1904.11740},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.11740},
  url = {http://arxiv.org/abs/1904.11740},
  urldate = {2023-11-21},
  abstract = {Transfer learning is widely used in deep neural network models when there are few labeled examples available. The common approach is to take a pre-trained network in a similar task and finetune the model parameters. This is usually done blindly without a pre-selection from a set of pre-trained models, or by finetuning a set of models trained on different tasks and selecting the best performing one by cross-validation. We address this problem by proposing an approach to assess the relationship between visual tasks and their task-specific models. Our method uses Representation Similarity Analysis (RSA), which is commonly used to find a correlation between neuronal responses from brain data and models. With RSA we obtain a similarity score among tasks by computing correlations between models trained on different tasks. Our method is efficient as it requires only pre-trained models, and a few images with no further training. We demonstrate the effectiveness and efficiency of our method for generating task taxonomy on Taskonomy dataset. We next evaluate the relationship of RSA with the transfer learning performance on Taskonomy tasks and a new task: Pascal VOC semantic segmentation. Our results reveal that models trained on tasks with higher similarity score show higher transfer learning performance. Surprisingly, the best transfer learning result for Pascal VOC semantic segmentation is not obtained from the pre-trained model on semantic segmentation, probably due to the domain differences, and our method successfully selects the high performing models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Dwivedi_Roig_2019_Representation Similarity Analysis for Efficient Task taxonomy & Transfer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MH6Z6VES\\1904.html}
}

@article{eaton-rosenImprovingDataAugmentation,
  title = {Improving {{Data Augmentation}} for {{Medical Image Segmentation}}},
  author = {Eaton-Rosen, Zach and Bragman, Felix and Ourselin, Sebastien and Cardoso, M Jorge},
  pages = {3},
  abstract = {Medical image segmentation is often constrained by the availability of labelled training data. ‘Data augmentation’ helps to prevent memorisation of training data and helps the network’s performance on data from outside the training set. As such, it is vital in building robust deep learning pipelines. Augmentation in medical imaging typically involves applying small transformations to images during training to create variety. However, it is also possible to use linear combinations of training images and labels to augment the dataset using the recently-proposed ‘mixup’ algorithm. Here, we apply this algorithm for use in medical imaging segmentation. We show that it increases performance in segmentation tasks, and also offer a theoretical suggestion for the efficacy of this technique.},
  langid = {english},
  file = {Y:\paper\Computer Vision\augmentation\Eaton-Rosen et al_Improving Data Augmentation for Medical Image Segmentation.pdf}
}

@online{ehretRegularizationNeRFsUsing2022,
  title = {Regularization of {{NeRFs}} Using Differential Geometry},
  author = {Ehret, Thibaud and Marí, Roger and Facciolo, Gabriele},
  date = {2022-11-30},
  eprint = {2206.14938},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.14938},
  urldate = {2023-01-20},
  abstract = {Neural radiance fields, or NeRF, represent a breakthrough in the field of novel view synthesis and 3D modeling of complex scenes from multi-view image collections. Numerous recent works have shown the importance of making NeRF models more robust, by means of regularization, in order to train with possibly inconsistent and/or very sparse data. In this work, we explore how differential geometry can provide elegant regularization tools for robustly training NeRF-like models, which are modified so as to represent continuous and infinitely differentiable functions. In particular, we present a generic framework for regularizing different types of NeRFs observations to improve the performance in challenging conditions. We also show how the same formalism can also be used to natively encourage the regularity of surfaces by means of Gaussian or mean curvatures.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Ehret et al_2022_Regularization of NeRFs using differential geometry.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WMWGPX2A\\2206.html}
}

@online{eigenPredictingDepthSurface2015,
  title = {Predicting {{Depth}}, {{Surface Normals}} and {{Semantic Labels}} with a {{Common Multi-Scale Convolutional Architecture}}},
  author = {Eigen, David and Fergus, Rob},
  date = {2015-12-16},
  eprint = {1411.4734},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1411.4734},
  url = {http://arxiv.org/abs/1411.4734},
  urldate = {2023-08-05},
  abstract = {In this paper we address three different computer vision tasks using a single basic architecture: depth prediction, surface normal estimation, and semantic labeling. We use a multiscale convolutional network that is able to adapt easily to each task using only small modifications, regressing from the input image to the output map directly. Our method progressively refines predictions using a sequence of scales, and captures many image details without any superpixels or low-level segmentation. We achieve state-of-the-art performance on benchmarks for all three tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\2.5d image understanding\\Eigen_Fergus_2015_Predicting Depth, Surface Normals and Semantic Labels with a Common Multi-Scale.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4HFQ37CD\\1411.html}
}

@article{elgendiEffectivenessImageAugmentation2021,
  title = {The {{Effectiveness}} of {{Image Augmentation}} in {{Deep Learning Networks}} for {{Detecting COVID-19}}: {{A Geometric Transformation Perspective}}},
  shorttitle = {The {{Effectiveness}} of {{Image Augmentation}} in {{Deep Learning Networks}} for {{Detecting COVID-19}}},
  author = {Elgendi, Mohamed and Nasir, Muhammad Umer and Tang, Qunfeng and Smith, David and Grenier, John-Paul and Batte, Catherine and Spieler, Bradley and Leslie, William Donald and Menon, Carlo and Fletcher, Richard Ribbon and Howard, Newton and Ward, Rabab and Parker, William and Nicolaou, Savvas},
  date = {2021},
  journaltitle = {Frontiers in Medicine},
  volume = {8},
  issn = {2296-858X},
  url = {https://www.frontiersin.org/articles/10.3389/fmed.2021.629134},
  urldate = {2022-07-09},
  abstract = {Chest X-ray imaging technology used for the early detection and screening of COVID-19 pneumonia is both accessible worldwide and affordable compared to other non-invasive technologies. Additionally, deep learning methods have recently shown remarkable results in detecting COVID-19 on chest X-rays, making it a promising screening technology for COVID-19. Deep learning relies on a large amount of data to avoid overfitting. While overfitting can result in perfect modeling on the original training dataset, on a new testing dataset it can fail to achieve high accuracy. In the image processing field, an image augmentation step (i.e., adding more training data) is often used to reduce overfitting on the training dataset, and improve prediction accuracy on the testing dataset. In this paper, we examined the impact of geometric augmentations as implemented in several recent publications for detecting COVID-19. We compared the performance of 17 deep learning algorithms with and without different geometric augmentations. We empirically examined the influence of augmentation with respect to detection accuracy, dataset diversity, augmentation methodology, and network size. Contrary to expectation, our results show that the removal of recently used geometrical augmentation steps actually improved the Matthews correlation coefficient (MCC) of 17 models. The MCC without augmentation (MCC = 0.51) outperformed four recent geometrical augmentations (MCC = 0.47 for Data Augmentation 1, MCC = 0.44 for Data Augmentation 2, MCC = 0.48 for Data Augmentation 3, and MCC = 0.49 for Data Augmentation 4). When we retrained a recently published deep learning without augmentation on the same dataset, the detection accuracy significantly increased, with a χMcNemar′s~statistic2=163.2 and a p-value of 2.23 × 10−37. This is an interesting finding that may improve current deep learning algorithms using geometrical augmentations for detecting COVID-19. We also provide clinical perspectives on geometric augmentation to consider regarding the development of a robust COVID-19 X-ray-based detector.},
  file = {Y:\paper\2022 summer intern\assignment\data augmentation\Elgendi et al_2021_The Effectiveness of Image Augmentation in Deep Learning Networks for Detecting.pdf}
}

@online{ElsevierEnhancedReader,
  title = {Elsevier {{Enhanced Reader}}},
  url = {https://reader.elsevier.com/reader/sd/pii/S0165168416300536?token=042B6A4BCA5EA3C126772F30E59674D7C7D9CE46606B8234C945A26A925CE089C38719F6F6F644BCBBF46A72F80375A0&originRegion=us-east-1&originCreation=20220926024808},
  urldate = {2022-09-26},
  file = {C:\Users\chsey\Zotero\storage\FLVAI65Z\S0165168416300536.html}
}

@online{evansInvisibleEnginesHow2016,
  type = {SSRN Scholarly Paper},
  title = {Invisible {{Engines}}: {{How Software Platforms Drive Innovation}} and {{Transform Industries}}},
  shorttitle = {Invisible {{Engines}}},
  author = {Evans, David S. and Hagiu, Andrei and Schmalensee, Richard},
  date = {2016-03-13},
  number = {2747032},
  location = {Rochester, NY},
  url = {https://papers.ssrn.com/abstract=2747032},
  urldate = {2023-12-30},
  abstract = {“Software platforms are the invisible engines that have created, touched, or transformed nearly every major industry for the past quarter century. They power everything from mobile phones and automobile navigation systems to search engines and web portals. They have been the source of enormous value to consumers and helped some entrepreneurs build great fortunes. And they are likely to drive change that will dwarf the business and technology revolution we have seen to this point. Invisible Engines examines the business dynamics and strategies used by firms that recognize the transformative power unleashed by this new revolution — a revolution that will change both new and old industries.”  Invisible Engines was written, including those words, mainly in 2004 and 2005 and published in 2006.  Timing is everything and, sometimes, even economists get it right: on January 9, 2007 Steve Jobs introduced the iPhone.  We believe Invisible Engines may still be worth reading for the enduring principles it lays out; for the lessons taught by software platforms that transformed the economy from the mid 1970s through the mid 2000s; and for its general insights into new economics of multisided platforms.  Some of the book will, no doubt, seem like watching an old movie with landline telephones and big cathode ray screens sitting or workers’ desks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {information communications and technology,mobile phones,multi-sided platforms,operating systems,software platforms,two-sided markets},
  file = {Y:\paper\management\Evans et al_2016_Invisible Engines.pdf}
}

@online{ExploringContextVisual,
  title = {Exploring Context and Visual Pattern of Relationship for Scene Graph Generation. - {{Google}} 검색},
  url = {https://www.google.com/search?q=Exploring+context+and+visual+pattern+of+relationship+for+scene+graph+generation.&oq=Exploring+context+and+visual+pattern+of+relationship+for+scene+graph+generation.&aqs=edge..69i57j0i30.787j0j1&sourceid=chrome&ie=UTF-8},
  urldate = {2023-05-30},
  file = {C:\Users\chsey\Zotero\storage\GPWFFAW3\search.html}
}

@inproceedings{fahesPODAPromptdrivenZeroshot2023,
  title = {{{PODA}}: {{Prompt-driven Zero-shot Domain Adaptation}}},
  shorttitle = {{{PODA}}},
  author = {Fahes, Mohammad and Vu, Tuan-Hung and Bursuc, Andrei and Pérez, Patrick and family=Charette, given=Raoul, prefix=de, useprefix=true},
  date = {2023},
  pages = {18623--18633},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Fahes_PODA_Prompt-driven_Zero-shot_Domain_Adaptation_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {domain adaptation,notion,zero shot},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Fahes et al_2023_PODA.pdf}
}

@online{fajtlAMNetMemorabilityEstimation2018,
  title = {{{AMNet}}: {{Memorability Estimation}} with {{Attention}}},
  shorttitle = {{{AMNet}}},
  author = {Fajtl, Jiri and Argyriou, Vasileios and Monekosso, Dorothy and Remagnino, Paolo},
  date = {2018-04-09},
  eprint = {1804.03115},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1804.03115},
  url = {http://arxiv.org/abs/1804.03115},
  urldate = {2023-08-05},
  abstract = {In this paper we present the design and evaluation of an end-to-end trainable, deep neural network with a visual attention mechanism for memorability estimation in still images. We analyze the suitability of transfer learning of deep models from image classification to the memorability task. Further on we study the impact of the attention mechanism on the memorability estimation and evaluate our network on the SUN Memorability and the LaMem datasets. Our network outperforms the existing state of the art models on both datasets in terms of the Spearman's rank correlation as well as the mean squared error, closely matching human consistency.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\memorability and intention interface\\Fajtl et al_2018_AMNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DXZNRQMR\\1804.html}
}

@online{fanDPOKReinforcementLearning2023,
  title = {{{DPOK}}: {{Reinforcement Learning}} for {{Fine-tuning Text-to-Image Diffusion Models}}},
  shorttitle = {{{DPOK}}},
  author = {Fan, Ying and Watkins, Olivia and Du, Yuqing and Liu, Hao and Ryu, Moonkyung and Boutilier, Craig and Abbeel, Pieter and Ghavamzadeh, Mohammad and Lee, Kangwook and Lee, Kimin},
  date = {2023-11-01},
  eprint = {2305.16381},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.16381},
  urldate = {2024-06-05},
  abstract = {Learning from human feedback has been shown to improve text-to-image models. These techniques first learn a reward function that captures what humans care about in the task and then improve the models based on the learned reward function. Even though relatively simple approaches (e.g., rejection sampling based on reward scores) have been investigated, fine-tuning text-to-image models with the reward function remains challenging. In this work, we propose using online reinforcement learning (RL) to fine-tune text-to-image models. We focus on diffusion models, defining the fine-tuning task as an RL problem, and updating the pre-trained text-to-image diffusion models using policy gradient to maximize the feedbacktrained reward. Our approach, coined DPOK, integrates policy optimization with KL regularization. We conduct an analysis of KL regularization for both RL fine-tuning and supervised fine-tuning. In our experiments, we show that DPOK is generally superior to supervised fine-tuning with respect to both image-text alignment and image quality. Our code is available at https://github.com/googleresearch/google-research/tree/master/dpok.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_lecture\Fan et al_2023_DPOK.pdf}
}

@online{fanFGNFullyGuided2020,
  title = {{{FGN}}: {{Fully Guided Network}} for {{Few-Shot Instance Segmentation}}},
  shorttitle = {{{FGN}}},
  author = {Fan, Zhibo and Yu, Jin-Gang and Liang, Zhihao and Ou, Jiarong and Gao, Changxin and Xia, Gui-Song and Li, Yuanqing},
  date = {2020-03-31},
  eprint = {2003.13954},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2003.13954},
  url = {http://arxiv.org/abs/2003.13954},
  urldate = {2023-11-23},
  abstract = {Few-shot instance segmentation (FSIS) conjoins the few-shot learning paradigm with general instance segmentation, which provides a possible way of tackling instance segmentation in the lack of abundant labeled data for training. This paper presents a Fully Guided Network (FGN) for few-shot instance segmentation. FGN perceives FSIS as a guided model where a so-called support set is encoded and utilized to guide the predictions of a base instance segmentation network (i.e., Mask R-CNN), critical to which is the guidance mechanism. In this view, FGN introduces different guidance mechanisms into the various key components in Mask R-CNN, including Attention-Guided RPN, Relation-Guided Detector, and Attention-Guided FCN, in order to make full use of the guidance effect from the support set and adapt better to the inter-class generalization. Experiments on public datasets demonstrate that our proposed FGN can outperform the state-of-the-art methods.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\few shot dense\\Fan et al_2020_FGN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EWIM6E49\\2003.html}
}

@inproceedings{farhadiDescribingObjectsTheir2009,
  title = {Describing Objects by Their Attributes},
  booktitle = {2009 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  author = {Farhadi, Ali and Endres, Ian and Hoiem, Derek and Forsyth, David},
  date = {2009-06},
  pages = {1778--1785},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2009.5206772},
  abstract = {We propose to shift the goal of recognition from naming to describing. Doing so allows us not only to name familiar objects, but also: to report unusual aspects of a familiar object (“spotty dog”, not just “dog”); to say something about unfamiliar objects (“hairy and four-legged”, not just “unknown”); and to learn how to recognize new objects with few or no visual examples. Rather than focusing on identity assignment, we make inferring attributes the core problem of recognition. These attributes can be semantic (“spotty”) or discriminative (“dogs have it but sheep do not”). Learning attributes presents a major new challenge: generalization across object categories, not just across instances within a category. In this paper, we also introduce a novel feature selection method for learning attributes that generalize well across categories. We support our claims by thorough evaluation that provides insights into the limitations of the standard recognition paradigm of naming and demonstrates the new abilities provided by our attribute-based framework.},
  eventtitle = {2009 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  keywords = {Cats,Computer vision,Detectors,Dogs,Leg,Motorcycles,notion,Object detection,Object recognition,Shape,Testing},
  file = {Y:\paper\computer_vision_topics_18\few shot learning\Farhadi et al_2009_Describing objects by their attributes.pdf}
}

@online{FasterRCNNRealTime,
  title = {Faster {{R-CNN}}: {{Towards Real-Time Object Detection}} with {{Region Proposal Networks}}},
  url = {https://proceedings.neurips.cc/paper/2015/hash/14bfa6bb14875e45bba028a21ed38046-Abstract.html},
  urldate = {2023-05-28}
}

@online{feichtenhoferMaskedAutoencodersSpatiotemporal2022,
  title = {Masked {{Autoencoders As Spatiotemporal Learners}}},
  author = {Feichtenhofer, Christoph and Fan, Haoqi and Li, Yanghao and He, Kaiming},
  date = {2022-10-21},
  eprint = {2205.09113},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2205.09113},
  url = {http://arxiv.org/abs/2205.09113},
  urldate = {2023-08-28},
  abstract = {This paper studies a conceptually simple extension of Masked Autoencoders (MAE) to spatiotemporal representation learning from videos. We randomly mask out spacetime patches in videos and learn an autoencoder to reconstruct them in pixels. Interestingly, we show that our MAE method can learn strong representations with almost no inductive bias on spacetime (only except for patch and positional embeddings), and spacetime-agnostic random masking performs the best. We observe that the optimal masking ratio is as high as 90\% (vs. 75\% on images), supporting the hypothesis that this ratio is related to information redundancy of the data. A high masking ratio leads to a large speedup, e.g., {$>$} 4x in wall-clock time or even more. We report competitive results on several challenging video datasets using vanilla Vision Transformers. We observe that MAE can outperform supervised pre-training by large margins. We further report encouraging results of training on real-world, uncurated Instagram data. Our study suggests that the general framework of masked autoencoding (BERT, MAE, etc.) can be a unified methodology for representation learning with minimal domain knowledge.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Feichtenhofer et al_2022_Masked Autoencoders As Spatiotemporal Learners.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4KDZDJW5\\2205.html}
}

@online{feichtenhoferSlowFastNetworksVideo2019,
  title = {{{SlowFast Networks}} for {{Video Recognition}}},
  author = {Feichtenhofer, Christoph and Fan, Haoqi and Malik, Jitendra and He, Kaiming},
  date = {2019-10-29},
  eprint = {1812.03982},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1812.03982},
  url = {http://arxiv.org/abs/1812.03982},
  urldate = {2023-08-05},
  abstract = {We present SlowFast networks for video recognition. Our model involves (i) a Slow pathway, operating at low frame rate, to capture spatial semantics, and (ii) a Fast pathway, operating at high frame rate, to capture motion at fine temporal resolution. The Fast pathway can be made very lightweight by reducing its channel capacity, yet can learn useful temporal information for video recognition. Our models achieve strong performance for both action classification and detection in video, and large improvements are pin-pointed as contributions by our SlowFast concept. We report state-of-the-art accuracy on major video recognition benchmarks, Kinetics, Charades and AVA. Code has been made available at: https://github.com/facebookresearch/SlowFast},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Feichtenhofer et al_2019_SlowFast Networks for Video Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2XWGKCLQ\\1812.html}
}

@inproceedings{fengDiverseDataAugmentation2023,
  title = {Diverse {{Data Augmentation}} with {{Diffusions}} for {{Effective Test-time Prompt Tuning}}},
  author = {Feng, Chun-Mei and Yu, Kai and Liu, Yong and Khan, Salman and Zuo, Wangmeng},
  date = {2023},
  pages = {2704--2714},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Feng_Diverse_Data_Augmentation_with_Diffusions_for_Effective_Test-time_Prompt_Tuning_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Feng et al_2023_Diverse Data Augmentation with Diffusions for Effective Test-time Prompt Tuning.pdf}
}

@online{fiftyEfficientlyIdentifyingTask2021,
  title = {Efficiently {{Identifying Task Groupings}} for {{Multi-Task Learning}}},
  author = {Fifty, Christopher and Amid, Ehsan and Zhao, Zhe and Yu, Tianhe and Anil, Rohan and Finn, Chelsea},
  date = {2021-10-25},
  eprint = {2109.04617},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2109.04617},
  urldate = {2023-11-14},
  abstract = {Multi-task learning can leverage information learned by one task to benefit the training of other tasks. Despite this capacity, naively training all tasks together in one model often degrades performance, and exhaustively searching through combinations of task groupings can be prohibitively expensive. As a result, efficiently identifying the tasks that would benefit from training together remains a challenging design question without a clear solution. In this paper, we suggest an approach to select which tasks should train together in multi-task learning models. Our method determines task groupings in a single run by training all tasks together and quantifying the effect to which one task's gradient would affect another task's loss. On the large-scale Taskonomy computer vision dataset, we find this method can decrease test loss by 10.0\% compared to simply training all tasks together while operating 11.6 times faster than a state-of-the-art task grouping method.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Fifty et al_2021_Efficiently Identifying Task Groupings for Multi-Task Learning2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V4WXRHEA\\2109.html}
}

@online{fiftyEfficientlyIdentifyingTask2021a,
  title = {Efficiently {{Identifying Task Groupings}} for {{Multi-Task Learning}}},
  author = {Fifty, Christopher and Amid, Ehsan and Zhao, Zhe and Yu, Tianhe and Anil, Rohan and Finn, Chelsea},
  date = {2021-10-25},
  eprint = {2109.04617},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2109.04617},
  urldate = {2023-11-14},
  abstract = {Multi-task learning can leverage information learned by one task to benefit the training of other tasks. Despite this capacity, naively training all tasks together in one model often degrades performance, and exhaustively searching through combinations of task groupings can be prohibitively expensive. As a result, efficiently identifying the tasks that would benefit from training together remains a challenging design question without a clear solution. In this paper, we suggest an approach to select which tasks should train together in multi-task learning models. Our method determines task groupings in a single run by training all tasks together and quantifying the effect to which one task's gradient would affect another task's loss. On the large-scale Taskonomy computer vision dataset, we find this method can decrease test loss by 10.0\% compared to simply training all tasks together while operating 11.6 times faster than a state-of-the-art task grouping method.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Fifty et al_2021_Efficiently Identifying Task Groupings for Multi-Task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KZPIJSWC\\2109.html}
}

@online{fiftyEfficientlyIdentifyingTask2021b,
  title = {Efficiently {{Identifying Task Groupings}} for {{Multi-Task Learning}}},
  author = {Fifty, Christopher and Amid, Ehsan and Zhao, Zhe and Yu, Tianhe and Anil, Rohan and Finn, Chelsea},
  date = {2021-10-25},
  eprint = {2109.04617},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2109.04617},
  url = {http://arxiv.org/abs/2109.04617},
  urldate = {2023-11-21},
  abstract = {Multi-task learning can leverage information learned by one task to benefit the training of other tasks. Despite this capacity, naively training all tasks together in one model often degrades performance, and exhaustively searching through combinations of task groupings can be prohibitively expensive. As a result, efficiently identifying the tasks that would benefit from training together remains a challenging design question without a clear solution. In this paper, we suggest an approach to select which tasks should train together in multi-task learning models. Our method determines task groupings in a single run by training all tasks together and quantifying the effect to which one task's gradient would affect another task's loss. On the large-scale Taskonomy computer vision dataset, we find this method can decrease test loss by 10.0\% compared to simply training all tasks together while operating 11.6 times faster than a state-of-the-art task grouping method.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Fifty et al_2021_Efficiently Identifying Task Groupings for Multi-Task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NKYD5WMU\\2109.html}
}

@online{FilePocketwatchCutaway1931,
  title = {File:{{Pocketwatch}} Cutaway Drawing.Jpg - {{Wikipedia}}},
  shorttitle = {File},
  date = {1931-12},
  url = {https://commons.wikimedia.org/wiki/File:Pocketwatch_cutaway_drawing.jpg},
  urldate = {2023-12-26},
  langid = {english}
}

@online{finnDeepVisualForesight2017,
  title = {Deep {{Visual Foresight}} for {{Planning Robot Motion}}},
  author = {Finn, Chelsea and Levine, Sergey},
  date = {2017-03-12},
  eprint = {1610.00696},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1610.00696},
  url = {http://arxiv.org/abs/1610.00696},
  urldate = {2023-08-05},
  abstract = {A key challenge in scaling up robot learning to many skills and environments is removing the need for human supervision, so that robots can collect their own data and improve their own performance without being limited by the cost of requesting human feedback. Model-based reinforcement learning holds the promise of enabling an agent to learn to predict the effects of its actions, which could provide flexible predictive models for a wide range of tasks and environments, without detailed human supervision. We develop a method for combining deep action-conditioned video prediction models with model-predictive control that uses entirely unlabeled training data. Our approach does not require a calibrated camera, an instrumented training set-up, nor precise sensing and actuation. Our results show that our method enables a real robot to perform nonprehensile manipulation -- pushing objects -- and can handle novel objects not seen during training.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Robotics,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\video prediction\\Finn_Levine_2017_Deep Visual Foresight for Planning Robot Motion.pdf;C\:\\Users\\chsey\\Zotero\\storage\\IGDE2Y5C\\1610.html}
}

@online{finnModelAgnosticMetaLearningFast2017,
  title = {Model-{{Agnostic Meta-Learning}} for {{Fast Adaptation}} of {{Deep Networks}}},
  author = {Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  date = {2017-07-18},
  eprint = {1703.03400},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1703.03400},
  url = {http://arxiv.org/abs/1703.03400},
  urldate = {2022-12-19},
  abstract = {We propose an algorithm for meta-learning that is model-agnostic, in the sense that it is compatible with any model trained with gradient descent and applicable to a variety of different learning problems, including classification, regression, and reinforcement learning. The goal of meta-learning is to train a model on a variety of learning tasks, such that it can solve new learning tasks using only a small number of training samples. In our approach, the parameters of the model are explicitly trained such that a small number of gradient steps with a small amount of training data from a new task will produce good generalization performance on that task. In effect, our method trains the model to be easy to fine-tune. We demonstrate that this approach leads to state-of-the-art performance on two few-shot image classification benchmarks, produces good results on few-shot regression, and accelerates fine-tuning for policy gradient reinforcement learning with neural network policies.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Finn et al_2017_Model-Agnostic Meta-Learning for Fast Adaptation of Deep Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LYZ79D2Y\\1703.html}
}

@article{flemingRecombinantUncertaintyTechnological2001,
  title = {Recombinant {{Uncertainty}} in {{Technological Search}}},
  author = {Fleming, Lee},
  date = {2001},
  journaltitle = {Management Science},
  volume = {47},
  number = {1},
  eprint = {2661563},
  eprinttype = {jstor},
  pages = {117--132},
  publisher = {INFORMS},
  issn = {0025-1909},
  url = {https://www.jstor.org/stable/2661563},
  urldate = {2023-12-06},
  abstract = {While the course of technological change is widely accepted to be highly uncertain and unpredictable, little work has identified or studied the ultimate sources and causes of that uncertainty. This paper proposes that purely technological uncertainty derives from inventors' search processes with unfamiliar components and component combinations. Experimentation with new components and new combinations leads to less useful inventions on average, but it also implies an increase in the variability that can result in both failure and breakthrough. Negative binomial count and dispersion models with patent citation data demonstrate that new combinations are indeed more variable. In contrast to predictions, however, the reuse of components has a nonmonotonic and eventually positive effect on variability.},
  file = {Y:\paper\management\Fleming_2001_Recombinant Uncertainty in Technological Search.pdf}
}

@article{flemingScienceMapTechnological2004,
  title = {Science as a Map in Technological Search},
  author = {Fleming, Lee and Sorenson, Olav},
  date = {2004},
  journaltitle = {Strategic Management Journal},
  volume = {25},
  number = {8-9},
  pages = {909--928},
  issn = {1097-0266},
  doi = {10.1002/smj.384},
  url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/smj.384},
  urldate = {2023-12-06},
  abstract = {A large body of work argues that scientific research increases the rate of technological advance, and with it economic growth. The precise mechanism through which science accelerates the rate of invention, however, remains an open question. Conceptualizing invention as a combinatorial search process, this paper argues that science alters inventors' search processes, by leading them more directly to useful combinations, eliminating fruitless paths of research, and motivating them to continue even in the face of negative feedback. These mechanisms prove most useful when inventors attempt to combine highly coupled components; therefore, the value of scientific research to invention varies systematically across applications. Empirical analyses of patent data support this thesis. Copyright © 2004 John Wiley \& Sons, Ltd.},
  langid = {english},
  keywords = {coupling,invention,recombinant search,science},
  file = {Y\:\\paper\\management\\Fleming_Sorenson_2004_Science as a map in technological search.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BWS2ZQFS\\smj.html}
}

@online{Food101MiningDiscriminative,
  title = {Food-101 -- {{Mining Discriminative Components}} with {{Random Forests}}},
  url = {https://data.vision.ee.ethz.ch/cvl/datasets_extra/food-101/},
  urldate = {2022-11-15},
  file = {C:\Users\chsey\Zotero\storage\UIG34ICF\food-101.html}
}

@online{fortDeepLearningKernel2020,
  title = {Deep Learning versus Kernel Learning: An Empirical Study of Loss Landscape Geometry and the Time Evolution of the {{Neural Tangent Kernel}}},
  shorttitle = {Deep Learning versus Kernel Learning},
  author = {Fort, Stanislav and Dziugaite, Gintare Karolina and Paul, Mansheej and Kharaghani, Sepideh and Roy, Daniel M. and Ganguli, Surya},
  date = {2020-10-28},
  eprint = {2010.15110},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2010.15110},
  urldate = {2024-09-28},
  abstract = {In suitably initialized wide networks, small learning rates transform deep neural networks (DNNs) into neural tangent kernel (NTK) machines, whose training dynamics is well-approximated by a linear weight expansion of the network at initialization. Standard training, however, diverges from its linearization in ways that are poorly understood. We study the relationship between the training dynamics of nonlinear deep networks, the geometry of the loss landscape, and the time evolution of a data-dependent NTK. We do so through a large-scale phenomenological analysis of training, synthesizing diverse measures characterizing loss landscape geometry and NTK dynamics. In multiple neural architectures and datasets, we find these diverse measures evolve in a highly correlated manner, revealing a universal picture of the deep learning process. In this picture, deep network training exhibits a highly chaotic rapid initial transient that within 2 to 3 epochs determines the final linearly connected basin of low loss containing the end point of training. During this chaotic transient, the NTK changes rapidly, learning useful features from the training data that enables it to outperform the standard initial NTK by a factor of 3 in less than 3 to 4 epochs. After this rapid chaotic transient, the NTK changes at constant velocity, and its performance matches that of full network training in 15\% to 45\% of training time. Overall, our analysis reveals a striking correlation between a diverse set of metrics over training time, governed by a rapid chaotic to stable transition in the first few epochs, that together poses challenges and opportunities for the development of more accurate theories of deep learning.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\RREUCYBR\Fort 등 - 2020 - Deep learning versus kernel learning an empirical.pdf}
}

@online{fortDeepLearningKernel2020a,
  title = {Deep Learning versus Kernel Learning: An Empirical Study of Loss Landscape Geometry and the Time Evolution of the {{Neural Tangent Kernel}}},
  shorttitle = {Deep Learning versus Kernel Learning},
  author = {Fort, Stanislav and Dziugaite, Gintare Karolina and Paul, Mansheej and Kharaghani, Sepideh and Roy, Daniel M. and Ganguli, Surya},
  date = {2020-10-28},
  eprint = {2010.15110},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2010.15110},
  urldate = {2024-09-28},
  abstract = {In suitably initialized wide networks, small learning rates transform deep neural networks (DNNs) into neural tangent kernel (NTK) machines, whose training dynamics is well-approximated by a linear weight expansion of the network at initialization. Standard training, however, diverges from its linearization in ways that are poorly understood. We study the relationship between the training dynamics of nonlinear deep networks, the geometry of the loss landscape, and the time evolution of a data-dependent NTK. We do so through a large-scale phenomenological analysis of training, synthesizing diverse measures characterizing loss landscape geometry and NTK dynamics. In multiple neural architectures and datasets, we find these diverse measures evolve in a highly correlated manner, revealing a universal picture of the deep learning process. In this picture, deep network training exhibits a highly chaotic rapid initial transient that within 2 to 3 epochs determines the final linearly connected basin of low loss containing the end point of training. During this chaotic transient, the NTK changes rapidly, learning useful features from the training data that enables it to outperform the standard initial NTK by a factor of 3 in less than 3 to 4 epochs. After this rapid chaotic transient, the NTK changes at constant velocity, and its performance matches that of full network training in 15\% to 45\% of training time. Overall, our analysis reveals a striking correlation between a diverse set of metrics over training time, governed by a rapid chaotic to stable transition in the first few epochs, that together poses challenges and opportunities for the development of more accurate theories of deep learning.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\XH423KRG\Fort 등 - 2020 - Deep learning versus kernel learning an empirical.pdf}
}

@article{fortExploringLimitsOutofDistribution2021,
  title = {Exploring the {{Limits}} of {{Out-of-Distribution Detection}}},
  author = {Fort, Stanislav and Ren, Jie and Lakshminarayanan, Balaji},
  date = {2021-06-06},
  doi = {10.48550/arXiv.2106.03004},
  url = {https://arxiv.org/abs/2106.03004v3},
  urldate = {2022-09-05},
  abstract = {Near out-of-distribution detection (OOD) is a major challenge for deep neural networks. We demonstrate that large-scale pre-trained transformers can significantly improve the state-of-the-art (SOTA) on a range of near OOD tasks across different data modalities. For instance, on CIFAR-100 vs CIFAR-10 OOD detection, we improve the AUROC from 85\% (current SOTA) to more than 96\% using Vision Transformers pre-trained on ImageNet-21k. On a challenging genomics OOD detection benchmark, we improve the AUROC from 66\% to 77\% using transformers and unsupervised pre-training. To further improve performance, we explore the few-shot outlier exposure setting where a few examples from outlier classes may be available; we show that pre-trained transformers are particularly well-suited for outlier exposure, and that the AUROC of OOD detection on CIFAR-100 vs CIFAR-10 can be improved to 98.7\% with just 1 image per OOD class, and 99.46\% with 10 images per OOD class. For multi-modal image-text pre-trained transformers such as CLIP, we explore a new way of using just the names of outlier classes as a sole source of information without any accompanying images, and show that this outperforms previous SOTA on standard vision OOD benchmark tasks.},
  langid = {english},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Fort et al_2021_Exploring the Limits of Out-of-Distribution Detection.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y8RCZTDX\\2106.html}
}

@online{FourRevolutionsPart,
  title = {Four {{Revolutions}}: {{Part}} 1: {{A Concise History Of The Quartz Revolution}} - {{Hodinkee}}},
  url = {https://www.hodinkee.com/articles/four-revolutions-quartz-revolution},
  urldate = {2023-12-26}
}

@online{frankleLinearModeConnectivity2020,
  title = {Linear {{Mode Connectivity}} and the {{Lottery Ticket Hypothesis}}},
  author = {Frankle, Jonathan and Dziugaite, Gintare Karolina and Roy, Daniel M. and Carbin, Michael},
  date = {2020-07-18},
  eprint = {1912.05671},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.1912.05671},
  url = {http://arxiv.org/abs/1912.05671},
  urldate = {2024-10-23},
  abstract = {We study whether a neural network optimizes to the same, linearly connected minimum under different samples of SGD noise (e.g., random data order and augmentation). We find that standard vision models become stable to SGD noise in this way early in training. From then on, the outcome of optimization is determined to a linearly connected region. We use this technique to study iterative magnitude pruning (IMP), the procedure used by work on the lottery ticket hypothesis to identify subnetworks that could have trained in isolation to full accuracy. We find that these subnetworks only reach full accuracy when they are stable to SGD noise, which either occurs at initialization for small-scale settings (MNIST) or early in training for large-scale settings (ResNet-50 and Inception-v3 on ImageNet).},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Frankle et al_2020_Linear Mode Connectivity and the Lottery Ticket Hypothesis.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PISL9EIR\\1912.html}
}

@article{freiIMPLICITBIASLEAKY2023,
  title = {{{IMPLICIT BIAS IN LEAKY RELU NETWORKS TRAINED ON HIGH-DIMENSIONAL DATA}}},
  author = {Frei, Spencer and Vardi, Gal and Bartlett, Peter L and Srebro, Nathan and Hu, Wei},
  date = {2023},
  abstract = {The implicit biases of gradient-based optimization algorithms are conjectured to be a major factor in the success of modern deep learning. In this work, we investigate the implicit bias of gradient flow and gradient descent in two-layer fullyconnected neural networks with leaky ReLU activations when the training data are nearly-orthogonal, a common property of high-dimensional data. For gradient flow, we leverage recent work on the implicit bias for homogeneous neural networks to show that asymptotically, gradient flow produces a neural network with rank at most two. Moreover, this network is an ℓ2-max-margin solution (in parameter space), and has a linear decision boundary that corresponds to an approximate-max-margin linear predictor. For gradient descent, provided the random initialization variance is small enough, we show that a single step of gradient descent suffices to drastically reduce the rank of the network, and that the rank remains small throughout training. We provide experiments which suggest that a small initialization scale is important for finding low-rank neural networks with gradient descent.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Frei et al_2023_IMPLICIT BIAS IN LEAKY RELU NETWORKS TRAINED ON HIGH-DIMENSIONAL DATA.pdf}
}

@article{frid-adarGANbasedSyntheticMedical2018,
  title = {{{GAN-based Synthetic Medical Image Augmentation}} for Increased {{CNN Performance}} in {{Liver Lesion Classification}}},
  author = {Frid-Adar, Maayan and Diamant, Idit and Klang, Eyal and Amitai, Michal and Goldberger, Jacob and Greenspan, Hayit},
  date = {2018-12},
  journaltitle = {Neurocomputing},
  shortjournal = {Neurocomputing},
  volume = {321},
  eprint = {1803.01229},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  pages = {321--331},
  issn = {09252312},
  doi = {10.1016/j.neucom.2018.09.013},
  url = {http://arxiv.org/abs/1803.01229},
  urldate = {2022-07-19},
  abstract = {Deep learning methods, and in particular convolutional neural networks (CNNs), have led to an enormous breakthrough in a wide range of computer vision tasks, primarily by using large-scale annotated datasets. However, obtaining such datasets in the medical domain remains a challenge. In this paper, we present methods for generating synthetic medical images using recently presented deep learning Generative Adversarial Networks (GANs). Furthermore, we show that generated medical images can be used for synthetic data augmentation, and improve the performance of CNN for medical image classification. Our novel method is demonstrated on a limited dataset of computed tomography (CT) images of 182 liver lesions (53 cysts, 64 metastases and 65 hemangiomas). We first exploit GAN architectures for synthesizing high quality liver lesion ROIs. Then we present a novel scheme for liver lesion classification using CNN. Finally, we train the CNN using classic data augmentation and our synthetic data augmentation and compare performance. In addition, we explore the quality of our synthesized examples using visualization and expert assessment. The classification performance using only classic data augmentation yielded 78.6\% sensitivity and 88.4\% specificity. By adding the synthetic data augmentation the results increased to 85.7\% sensitivity and 92.4\% specificity. We believe that this approach to synthetic data augmentation can generalize to other medical classification applications and thus support radiologists’ efforts to improve diagnosis.},
  langid = {english},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y:\paper\2022 summer intern\assignment\reproduction\Frid-Adar et al_2018_GAN-based Synthetic Medical Image Augmentation for increased CNN Performance in.pdf}
}

@inproceedings{fujitomiLBNERFLightBending2022,
  title = {{{LB-NERF}}: {{Light Bending Neural Radiance Fields}} for {{Transparent Medium}}},
  shorttitle = {{{LB-NERF}}},
  booktitle = {2022 {{IEEE International Conference}} on {{Image Processing}} ({{ICIP}})},
  author = {Fujitomi, Taku and Sakurada, Ken and Hamaguchi, Ryuhei and Shishido, Hidehiko and Onishi, Masaki and Kameda, Yoshinari},
  date = {2022-10},
  pages = {2142--2146},
  issn = {2381-8549},
  doi = {10.1109/ICIP46576.2022.9897642},
  abstract = {Neural radiance fields (NeRFs) have been proposed as methods of novel view synthesis and have been used to address various problems because of its versatility. NeRF can represent colors and densities in 3D space using neural rendering assuming a straight light path. However, a medium with a different refractive index in the scene, such as a transparent medium, causes light refraction and breaks the assumption of the straight path of light. Therefore, the NeRFs cannot be learned consistently across multi-view images. To solve this problem, this study proposes a method to learn consistent radiance fields across multiple viewpoints by introducing the light refraction effect as an offset from the straight line originating from the camera center. The experimental results quantitatively and qualitatively verified that our method can interpolate viewpoints better than the conventional NeRF method when considering the refraction of transparent objects.},
  eventtitle = {2022 {{IEEE International Conference}} on {{Image Processing}} ({{ICIP}})},
  keywords = {Bending,Cameras,Image color analysis,Learning systems,radiance fields,refraction,Refractive index,Rendering (computer graphics),Three-dimensional displays,transparent medium,view synthesis,volume rendering},
  file = {Y\:\\paper\\2022 winter intern\\Fujitomi et al_2022_LB-NERF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Z779KC9N\\stamp.html}
}

@online{FullArticleAnalysis,
  title = {Full Article: {{Analysis}} and Modeling of Client Order Flow in Limit Order Markets},
  url = {https://www.tandfonline.com/doi/full/10.1080/14697688.2022.2150282},
  urldate = {2024-09-11},
  file = {C:\Users\chsey\Zotero\storage\NSFQKD4K\14697688.2022.html}
}

@article{fusielloElementsGeometricComputer,
  title = {Elements of {{Geometric Computer Vision}}.},
  author = {Fusiello, Andrea},
  pages = {25},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA2\Fusiello_Elements of Geometric Computer Vision.pdf}
}

@online{gaalAttentionUNetBased2020,
  title = {Attention {{U-Net Based Adversarial Architectures}} for {{Chest X-ray Lung Segmentation}}},
  author = {Gaál, Gusztáv and Maga, Balázs and Lukács, András},
  date = {2020-03-23},
  eprint = {2003.10304},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2003.10304},
  urldate = {2022-07-10},
  abstract = {Chest X-ray is the most common test among medical imaging modalities. It is applied for detection and differentiation of, among others, lung cancer, tuberculosis, and pneumonia, the last with importance due to the COVID-19 disease. Integrating computer-aided detection methods into the radiologist diagnostic pipeline, greatly reduces the doctors' workload, increasing reliability and quantitative analysis. Here we present a novel deep learning approach for lung segmentation, a basic, but arduous task in the diagnostic pipeline. Our method uses state-of-the-art fully convolutional neural networks in conjunction with an adversarial critic model. It generalized well to CXR images of unseen datasets with different patient profiles, achieving a final DSC of 97.5\% on the JSRT dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\data augmentation\\pre-processing\\Gaál et al_2020_Attention U-Net Based Adversarial Architectures for Chest X-ray Lung.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EV67I2DT\\2003.html}
}

@article{gagneDayAheadHailPrediction2015,
  title = {Day-{{Ahead Hail Prediction Integrating Machine Learning}} with {{Storm-Scale Numerical Weather Models}}},
  author = {Gagne, David and McGovern, Amy and Jerald, Jerald and Coniglio, Michael and Correia, James and Xue, Ming},
  date = {2015-01-25},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {29},
  number = {2},
  pages = {3954--3960},
  issn = {2374-3468},
  doi = {10.1609/aaai.v29i2.19053},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/19053},
  urldate = {2023-05-24},
  abstract = {Hail causes billions of dollars in losses by damaging buildings, vehicles, and crops. Improving the spatial and temporal accuracy of hail forecasts would allow people to mitigate hail damage. We have developed an approach to forecasting hail that identifies potential hail storms in storm-scale numerical weather prediction models and matches them with observed hailstorms. Machine learning models, including random forests, gradient boosting trees, and linear regression, are used to predict the expected hail size from each forecast storm. The individual hail size forecasts are merged with a spatial neighborhood ensemble probability technique to produce a consensus probability of hail at least 25.4 mm in diameter. The system was evaluated during the 2014 National Oceanic and Atmospheric Administration Hazardous Weather Testbed Experimental Forecast Program and compared with a physics-based hail size model. The machine-learning-based technique shows advantages in producing smaller size errors and more reliable probability forecasts. The machine learning approaches correctly predicted the location and extent of a significant hail event in eastern Nebraska and a marginal severe hail event in Colorado.},
  issue = {2},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Gagne et al_2015_Day-Ahead Hail Prediction Integrating Machine Learning with Storm-Scale.pdf}
}

@online{gaoCapOnImageContextdrivenDenseCaptioning2022,
  title = {{{CapOnImage}}: {{Context-driven Dense-Captioning}} on {{Image}}},
  shorttitle = {{{CapOnImage}}},
  author = {Gao, Yiqi and Hou, Xinglin and Zhang, Yuanmeng and Ge, Tiezheng and Jiang, Yuning and Wang, Peng},
  date = {2022-04-27},
  eprint = {2204.12974},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2204.12974},
  urldate = {2023-05-28},
  abstract = {Existing image captioning systems are dedicated to generating narrative captions for images, which are spatially detached from the image in presentation. However, texts can also be used as decorations on the image to highlight the key points and increase the attractiveness of images. In this work, we introduce a new task called captioning on image (CapOnImage), which aims to generate dense captions at different locations of the image based on contextual information. To fully exploit the surrounding visual context to generate the most suitable caption for each location, we propose a multi-modal pre-training model with multi-level pre-training tasks that progressively learn the correspondence between texts and image locations from easy to difficult. Since the model may generate redundant captions for nearby locations, we further enhance the location embedding with neighbor locations as context. For this new task, we also introduce a large-scale benchmark called CapOnImage2M, which contains 2.1 million product images, each with an average of 4.8 spatially localized captions. Compared with other image captioning model variants, our model achieves the best results in both captioning accuracy and diversity aspects. We will make code and datasets public to facilitate future research.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Gao et al_2022_CapOnImage.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9HJGF479\\2204.html}
}

@online{gaoCapOnImageContextdrivenDenseCaptioning2022a,
  title = {{{CapOnImage}}: {{Context-driven Dense-Captioning}} on {{Image}}},
  shorttitle = {{{CapOnImage}}},
  author = {Gao, Yiqi and Hou, Xinglin and Zhang, Yuanmeng and Ge, Tiezheng and Jiang, Yuning and Wang, Peng},
  date = {2022-04-27},
  eprint = {2204.12974},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2204.12974},
  url = {http://arxiv.org/abs/2204.12974},
  urldate = {2023-05-27},
  abstract = {Existing image captioning systems are dedicated to generating narrative captions for images, which are spatially detached from the image in presentation. However, texts can also be used as decorations on the image to highlight the key points and increase the attractiveness of images. In this work, we introduce a new task called captioning on image (CapOnImage), which aims to generate dense captions at different locations of the image based on contextual information. To fully exploit the surrounding visual context to generate the most suitable caption for each location, we propose a multi-modal pre-training model with multi-level pre-training tasks that progressively learn the correspondence between texts and image locations from easy to difficult. Since the model may generate redundant captions for nearby locations, we further enhance the location embedding with neighbor locations as context. For this new task, we also introduce a large-scale benchmark called CapOnImage2M, which contains 2.1 million product images, each with an average of 4.8 spatially localized captions. Compared with other image captioning model variants, our model achieves the best results in both captioning accuracy and diversity aspects. We will make code and datasets public to facilitate future research.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\image captioning\\Gao et al_2022_CapOnImage.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LDE9Q6AA\\2204.html}
}

@inproceedings{gaoLearningJointlyShare2022,
  title = {Learning to {{Jointly Share}} and {{Prune Weights}} for {{Grounding Based Vision}} and {{Language Models}}},
  author = {Gao, Shangqian and Uzkent, Burak and Shen, Yilin and Huang, Heng and Jin, Hongxia},
  date = {2022-09-29},
  url = {https://openreview.net/forum?id=UMERaIHMwB3},
  urldate = {2024-03-13},
  abstract = {Transformers have seen growing interest in processing different modalities, including language and image data. As a result, we can process vision and language data using transformers that are architecturally similar. Leveraging this feature of transformers, we propose weight sharing across two transformer backbones and within the same transformer backbone and pruning across two backbones in a unified framework. More specifically, we investigate weight sharing and pruning for two components of the transformers: (1) Multi-Head Attention (MSA) and (2) Feed-Forward Network (FFN) layers. To jointly perform weight sharing and pruning, we propose to use a regularization term to align model weights and the desired structure during the multimodal pre-training step. The structure vectors of sharing and pruning are generated by using a hypernetwork, which can capture complex interactions between pruning and sharing across layers and modalities. We train the hypernetwork and model weights iteratively so that the learned structure evolves along with model weights. After minimizing the proposed objective in the pre-training step, we perform weight sharing and pruning and fine-tune the compressed model on downstream tasks. Finally, we perform experiments on vision and language tasks, including Referring Expression Comprehension (REC), Visual Question Answering (VQA), and Object Detection using the state-of-the-art grounding based models: MDETR and GLIP. Our experiments show that we can compress these models by \$35-40\textbackslash\%\$ by sharing and pruning MSA and FFN weights without almost any loss in accuracy.},
  eventtitle = {The {{Eleventh International Conference}} on {{Learning Representations}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Gao et al_2022_Learning to Jointly Share and Prune Weights for Grounding Based Vision and.pdf}
}

@online{gaoNeRFNeuralRadiance2022,
  title = {{{NeRF}}: {{Neural Radiance Field}} in {{3D Vision}}, {{A Comprehensive Review}}},
  shorttitle = {{{NeRF}}},
  author = {Gao, Kyle and Gao, Yina and He, Hongjie and Lu, Dening and Xu, Linlin and Li, Jonathan},
  date = {2022-12-18},
  eprint = {2210.00379},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2210.00379},
  urldate = {2023-01-09},
  abstract = {Neural Radiance Field (NeRF), a new novel view synthesis with implicit scene representation has taken the field of Computer Vision by storm. As a novel view synthesis and 3D reconstruction method, NeRF models find applications in robotics, urban mapping, autonomous navigation, virtual reality/augmented reality, and more. Since the original paper by Mildenhall et al., more than 250 preprints were published, with more than 100 eventually being accepted in tier one Computer Vision Conferences. Given NeRF popularity and the current interest in this research area, we believe it necessary to compile a comprehensive survey of NeRF papers from the past two years, which we organized into both architecture, and application based taxonomies. We also provide an introduction to the theory of NeRF based novel view synthesis, and a benchmark comparison of the performance and speed of key NeRF models. By creating this survey, we hope to introduce new researchers to NeRF, provide a helpful reference for influential works in this field, as well as motivate future research directions with our discussion section.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Gao et al_2022_NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5RM36QDJ\\2210.html}
}

@article{garcinPlNtNet300KPlant2021,
  title = {Pl@{{ntNet-300K}}: A Plant Image Dataset with High Label Ambiguity and a Long-Tailed Distribution},
  shorttitle = {Pl@{{ntNet-300K}}},
  author = {Garcin, Camille and Joly, Alexis and Bonnet, Pierre and Affouard, Antoine and Lombardo, Jean-Christophe and Chouet, Mathias and Servajean, Maximilien and Lorieul, Titouan and Salmon, Joseph},
  date = {2021-12-06},
  journaltitle = {Proceedings of the Neural Information Processing Systems Track on Datasets and Benchmarks},
  volume = {1},
  url = {https://datasets-benchmarks-proceedings.neurips.cc/paper/2021/hash/7e7757b1e12abcb736ab9a754ffb617a-Abstract-round2.html},
  urldate = {2023-05-23},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\Garcin et al_2021_Pl@ntNet-300K.pdf}
}

@online{gargWhatCanTransformers2023,
  title = {What {{Can Transformers Learn In-Context}}? {{A Case Study}} of {{Simple Function Classes}}},
  shorttitle = {What {{Can Transformers Learn In-Context}}?},
  author = {Garg, Shivam and Tsipras, Dimitris and Liang, Percy and Valiant, Gregory},
  date = {2023-08-11},
  eprint = {2208.01066},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2208.01066},
  urldate = {2024-05-16},
  abstract = {In-context learning refers to the ability of a model to condition on a prompt sequence consisting of in-context examples (input-output pairs corresponding to some task) along with a new query input, and generate the corresponding output. Crucially, in-context learning happens only at inference time without any parameter updates to the model. While large language models such as GPT-3 exhibit some ability to perform in-context learning, it is unclear what the relationship is between tasks on which this succeeds and what is present in the training data. To make progress towards understanding in-context learning, we consider the well-defined problem of training a model to in-context learn a function class (e.g., linear functions): that is, given data derived from some functions in the class, can we train a model to in-context learn "most" functions from this class? We show empirically that standard Transformers can be trained from scratch to perform in-context learning of linear functions -- that is, the trained model is able to learn unseen linear functions from in-context examples with performance comparable to the optimal least squares estimator. In fact, in-context learning is possible even under two forms of distribution shift: (i) between the training data of the model and inference-time prompts, and (ii) between the in-context examples and the query input during inference. We also show that we can train Transformers to in-context learn more complex function classes -- namely sparse linear functions, two-layer neural networks, and decision trees -- with performance that matches or exceeds task-specific learning algorithms. Our code and models are available at https://github.com/dtsip/in-context-learning .},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\Y3DWH3K3\Garg 등 - 2023 - What Can Transformers Learn In-Context A Case Stu.pdf}
}

@article{gemanVisualTuringTest2015,
  title = {Visual {{Turing}} Test for Computer Vision Systems},
  author = {Geman, Donald and Geman, Stuart and Hallonquist, Neil and Younes, Laurent},
  date = {2015-03-24},
  journaltitle = {Proceedings of the National Academy of Sciences},
  volume = {112},
  number = {12},
  pages = {3618--3623},
  publisher = {Proceedings of the National Academy of Sciences},
  doi = {10.1073/pnas.1422953112},
  url = {https://www.pnas.org/doi/10.1073/pnas.1422953112},
  urldate = {2023-05-28},
  abstract = {Today, computer vision systems are tested by their accuracy in detecting and localizing instances of objects. As an alternative, and motivated by the ability of humans to provide far richer descriptions and even tell a story about an image, we construct a “visual Turing test”: an operator-assisted device that produces a stochastic sequence of binary questions from a given test image. The query engine proposes a question; the operator either provides the correct answer or rejects the question as ambiguous; the engine proposes the next question (“just-in-time truthing”). The test is then administered to the computer-vision system, one question at a time. After the system’s answer is recorded, the system is provided the correct answer and the next question. Parsing is trivial and deterministic; the system being tested requires no natural language processing. The query engine employs statistical constraints, learned from a training set, to produce questions with essentially unpredictable answers—the answer to a question, given the history of questions and their correct answers, is nearly equally likely to be positive or negative. In this sense, the test is only about vision. The system is designed to produce streams of questions that follow natural story lines, from the instantiation of a unique object, through an exploration of its properties, and on to its relationships with other uniquely instantiated objects.},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Geman et al_2015_Visual Turing test for computer vision systems.pdf}
}

@online{gengMultimodalMaskedAutoencoders2022,
  title = {Multimodal {{Masked Autoencoders Learn Transferable Representations}}},
  author = {Geng, Xinyang and Liu, Hao and Lee, Lisa and Schuurmans, Dale and Levine, Sergey and Abbeel, Pieter},
  date = {2022-10-21},
  eprint = {2205.14204},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.14204},
  urldate = {2024-06-30},
  abstract = {Building scalable models to learn from diverse, multimodal data remains an open challenge. For vision-language data, the dominant approaches are based on contrastive learning objectives that train a separate encoder for each modality. While effective, contrastive learning approaches introduce sampling bias depending on the data augmentations used, which can degrade performance on downstream tasks. Moreover, these methods are limited to paired image-text data, and cannot leverage widely-available unpaired data. In this paper, we investigate whether a large multimodal model trained purely via masked token prediction, without using modality-specific encoders or contrastive learning, can learn transferable representations for downstream tasks. We propose a simple and scalable network architecture, the Multimodal Masked Autoencoder (M3AE), which learns a unified encoder for both vision and language data via masked token prediction. We provide an empirical study of M3AE trained on a large-scale image-text dataset, and find that M3AE is able to learn generalizable representations that transfer well to downstream tasks. Surprisingly, we find that M3AE benefits from a higher text mask ratio (50-90\%), in contrast to BERT whose standard masking ratio is 15\%, due to the joint training of two data modalities. We also provide qualitative analysis showing that the learned representation incorporates meaningful information from both image and language. Lastly, we demonstrate the scalability of M3AE with larger model size and training time, and its flexibility to train on both paired image-text data as well as unpaired data.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\VT3L8T4G\Geng 등 - 2022 - Multimodal Masked Autoencoders Learn Transferable .pdf}
}

@inproceedings{georgescuAudiovisualMaskedAutoencoders2023,
  title = {Audiovisual {{Masked Autoencoders}}},
  booktitle = {2023 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  author = {Georgescu, Mariana-Iuliana and Fonseca, Eduardo and Ionescu, Radu Tudor and Lucic, Mario and Schmid, Cordelia and Arnab, Anurag},
  date = {2023-10-01},
  pages = {16098--16108},
  publisher = {IEEE},
  location = {Paris, France},
  doi = {10.1109/ICCV51070.2023.01479},
  url = {https://ieeexplore.ieee.org/document/10377052/},
  urldate = {2024-06-17},
  eventtitle = {2023 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  isbn = {9798350307184},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\6GPLGCAG\Georgescu 등 - 2023 - Audiovisual Masked Autoencoders.pdf}
}

@online{ghiasiNASFPNLearningScalable2019,
  title = {{{NAS-FPN}}: {{Learning Scalable Feature Pyramid Architecture}} for {{Object Detection}}},
  shorttitle = {{{NAS-FPN}}},
  author = {Ghiasi, Golnaz and Lin, Tsung-Yi and Pang, Ruoming and Le, Quoc V.},
  date = {2019-04-15},
  eprint = {1904.07392},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.07392},
  url = {http://arxiv.org/abs/1904.07392},
  urldate = {2023-01-03},
  abstract = {Current state-of-the-art convolutional architectures for object detection are manually designed. Here we aim to learn a better architecture of feature pyramid network for object detection. We adopt Neural Architecture Search and discover a new feature pyramid architecture in a novel scalable search space covering all cross-scale connections. The discovered architecture, named NAS-FPN, consists of a combination of top-down and bottom-up connections to fuse features across scales. NAS-FPN, combined with various backbone models in the RetinaNet framework, achieves better accuracy and latency tradeoff compared to state-of-the-art object detection models. NAS-FPN improves mobile detection accuracy by 2 AP compared to state-of-the-art SSDLite with MobileNetV2 model in [32] and achieves 48.3 AP which surpasses Mask R-CNN [10] detection accuracy with less computation time.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Ghiasi et al_2019_NAS-FPN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5EZRFJEG\\1904.html}
}

@online{ghiasiSimpleCopyPasteStrong2021,
  title = {Simple {{Copy-Paste}} Is a {{Strong Data Augmentation Method}} for {{Instance Segmentation}}},
  author = {Ghiasi, Golnaz and Cui, Yin and Srinivas, Aravind and Qian, Rui and Lin, Tsung-Yi and Cubuk, Ekin D. and Le, Quoc V. and Zoph, Barret},
  date = {2021-06-23},
  eprint = {2012.07177},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2012.07177},
  urldate = {2022-07-03},
  abstract = {Building instance segmentation models that are data-efficient and can handle rare object categories is an important challenge in computer vision. Leveraging data augmentations is a promising direction towards addressing this challenge. Here, we perform a systematic study of the Copy-Paste augmentation ([13, 12]) for instance segmentation where we randomly paste objects onto an image. Prior studies on Copy-Paste relied on modeling the surrounding visual context for pasting the objects. However, we find that the simple mechanism of pasting objects randomly is good enough and can provide solid gains on top of strong baselines. Furthermore, we show Copy-Paste is additive with semi-supervised methods that leverage extra data through pseudo labeling (e.g. self-training). On COCO instance segmentation, we achieve 49.1 mask AP and 57.3 box AP, an improvement of +0.6 mask AP and +1.5 box AP over the previous state-of-the-art. We further demonstrate that Copy-Paste can lead to significant improvements on the LVIS benchmark. Our baseline model outperforms the LVIS 2020 Challenge winning entry by +3.6 mask AP on rare categories.},
  pubstate = {prepublished},
  version = {2},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\data augmentation\\Ghiasi et al_2021_Simple Copy-Paste is a Strong Data Augmentation Method for Instance Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\66DXJWWU\\2012.html}
}

@online{ghiasiSimpleCopyPasteStrong2021a,
  title = {Simple {{Copy-Paste}} Is a {{Strong Data Augmentation Method}} for {{Instance Segmentation}}},
  author = {Ghiasi, Golnaz and Cui, Yin and Srinivas, Aravind and Qian, Rui and Lin, Tsung-Yi and Cubuk, Ekin D. and Le, Quoc V. and Zoph, Barret},
  date = {2021-06-23},
  eprint = {2012.07177},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2012.07177},
  urldate = {2022-07-09},
  abstract = {Building instance segmentation models that are data-efficient and can handle rare object categories is an important challenge in computer vision. Leveraging data augmentations is a promising direction towards addressing this challenge. Here, we perform a systematic study of the Copy-Paste augmentation ([13, 12]) for instance segmentation where we randomly paste objects onto an image. Prior studies on Copy-Paste relied on modeling the surrounding visual context for pasting the objects. However, we find that the simple mechanism of pasting objects randomly is good enough and can provide solid gains on top of strong baselines. Furthermore, we show Copy-Paste is additive with semi-supervised methods that leverage extra data through pseudo labeling (e.g. self-training). On COCO instance segmentation, we achieve 49.1 mask AP and 57.3 box AP, an improvement of +0.6 mask AP and +1.5 box AP over the previous state-of-the-art. We further demonstrate that Copy-Paste can lead to significant improvements on the LVIS benchmark. Our baseline model outperforms the LVIS 2020 Challenge winning entry by +3.6 mask AP on rare categories.},
  pubstate = {prepublished},
  version = {2},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\segmentation\\Ghiasi et al_2021_Simple Copy-Paste is a Strong Data Augmentation Method for Instance Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QGWAIDGH\\2012.html}
}

@online{girdharImageBindOneEmbedding2023,
  title = {{{ImageBind}}: {{One Embedding Space To Bind Them All}}},
  shorttitle = {{{ImageBind}}},
  author = {Girdhar, Rohit and El-Nouby, Alaaeldin and Liu, Zhuang and Singh, Mannat and Alwala, Kalyan Vasudev and Joulin, Armand and Misra, Ishan},
  date = {2023-05-31},
  eprint = {2305.05665},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.05665},
  urldate = {2024-05-07},
  abstract = {We present IMAGEBIND, an approach to learn a joint embedding across six different modalities - images, text, audio, depth, thermal, and IMU data. We show that all combinations of paired data are not necessary to train such a joint embedding, and only image-paired data is sufficient to bind the modalities together. IMAGEBIND can leverage recent large scale vision-language models, and extends their zeroshot capabilities to new modalities just by using their natural pairing with images. It enables novel emergent applications ‘out-of-the-box’ including cross-modal retrieval, composing modalities with arithmetic, cross-modal detection and generation. The emergent capabilities improve with the strength of the image encoder and we set a new state-of-theart on emergent zero-shot recognition tasks across modalities, outperforming specialist supervised models. Finally, we show strong few-shot recognition results outperforming prior work, and that IMAGEBIND serves as a new way to evaluate vision models for visual and non-visual tasks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {Y:\paper\2024_research\Girdhar et al_2023_ImageBind.pdf}
}

@online{girdharLearningPredictableGenerative2016,
  title = {Learning a {{Predictable}} and {{Generative Vector Representation}} for {{Objects}}},
  author = {Girdhar, Rohit and Fouhey, David F. and Rodriguez, Mikel and Gupta, Abhinav},
  date = {2016-08-31},
  eprint = {1603.08637},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1603.08637},
  url = {http://arxiv.org/abs/1603.08637},
  urldate = {2023-08-05},
  abstract = {What is a good vector representation of an object? We believe that it should be generative in 3D, in the sense that it can produce new 3D objects; as well as be predictable from 2D, in the sense that it can be perceived from 2D images. We propose a novel architecture, called the TL-embedding network, to learn an embedding space with these properties. The network consists of two components: (a) an autoencoder that ensures the representation is generative; and (b) a convolutional network that ensures the representation is predictable. This enables tackling a number of tasks including voxel prediction from 2D images and 3D model retrieval. Extensive experimental analysis demonstrates the usefulness and versatility of this embedding.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\3d image understanding\\Girdhar et al_2016_Learning a Predictable and Generative Vector Representation for Objects.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EI8FMBZN\\1603.html}
}

@online{girdharOmniMAESingleModel2023,
  title = {{{OmniMAE}}: {{Single Model Masked Pretraining}} on {{Images}} and {{Videos}}},
  shorttitle = {{{OmniMAE}}},
  author = {Girdhar, Rohit and El-Nouby, Alaaeldin and Singh, Mannat and Alwala, Kalyan Vasudev and Joulin, Armand and Misra, Ishan},
  date = {2023-05-31},
  eprint = {2206.08356},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2206.08356},
  url = {http://arxiv.org/abs/2206.08356},
  urldate = {2024-07-05},
  abstract = {Transformer-based architectures have become competitive across a variety of visual domains, most notably images and videos. While prior work studies these modalities in isolation, having a common architecture suggests that one can train a single unified model for multiple visual modalities. Prior attempts at unified modeling typically use architectures tailored for vision tasks, or obtain worse performance compared to single modality models. In this work, we show that masked autoencoding can be used to train a simple Vision Transformer on images and videos, without requiring any labeled data. This single model learns visual representations that are comparable to or better than single-modality representations on both image and video benchmarks, while using a much simpler architecture. Furthermore, this model can be learned by dropping 90\% of the image and 95\% of the video patches, enabling extremely fast training of huge model architectures. In particular, we show that our single ViT-Huge model can be finetuned to achieve 86.6\% on ImageNet and 75.5\% on the challenging Something Something-v2 video benchmark, setting a new state-of-the-art.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Girdhar et al_2023_OmniMAE.pdf;C\:\\Users\\chsey\\Zotero\\storage\\N6ZG34ZI\\2206.html}
}

@online{girshickFastRCNN2015,
  title = {Fast {{R-CNN}}},
  author = {Girshick, Ross},
  date = {2015-09-27},
  eprint = {1504.08083},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1504.08083},
  url = {http://arxiv.org/abs/1504.08083},
  urldate = {2022-07-04},
  abstract = {This paper proposes a Fast Region-based Convolutional Network method (Fast R-CNN) for object detection. Fast R-CNN builds on previous work to efficiently classify object proposals using deep convolutional networks. Compared to previous work, Fast R-CNN employs several innovations to improve training and testing speed while also increasing detection accuracy. Fast R-CNN trains the very deep VGG16 network 9x faster than R-CNN, is 213x faster at test-time, and achieves a higher mAP on PASCAL VOC 2012. Compared to SPPnet, Fast R-CNN trains VGG16 3x faster, tests 10x faster, and is more accurate. Fast R-CNN is implemented in Python and C++ (using Caffe) and is available under the open-source MIT License at https://github.com/rbgirshick/fast-rcnn.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\detection\\Girshick_2015_Fast R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XX5BH357\\1504.html}
}

@online{girshickFastRCNN2015a,
  title = {Fast {{R-CNN}}},
  author = {Girshick, Ross},
  date = {2015-09-27},
  eprint = {1504.08083},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1504.08083},
  url = {http://arxiv.org/abs/1504.08083},
  urldate = {2023-08-05},
  abstract = {This paper proposes a Fast Region-based Convolutional Network method (Fast R-CNN) for object detection. Fast R-CNN builds on previous work to efficiently classify object proposals using deep convolutional networks. Compared to previous work, Fast R-CNN employs several innovations to improve training and testing speed while also increasing detection accuracy. Fast R-CNN trains the very deep VGG16 network 9x faster than R-CNN, is 213x faster at test-time, and achieves a higher mAP on PASCAL VOC 2012. Compared to SPPnet, Fast R-CNN trains VGG16 3x faster, tests 10x faster, and is more accurate. Fast R-CNN is implemented in Python and C++ (using Caffe) and is available under the open-source MIT License at https://github.com/rbgirshick/fast-rcnn.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Girshick_2015_Fast R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\N826VTJ2\\1504.html}
}

@online{girshickRCNNRichFeature2014,
  title = {R-{{CNN}}: {{Rich}} Feature Hierarchies for Accurate Object Detection and Semantic Segmentation},
  author = {Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  date = {2014-10-22},
  eprint = {1311.2524},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1311.2524},
  url = {http://arxiv.org/abs/1311.2524},
  urldate = {2022-07-04},
  abstract = {Object detection performance, as measured on the canonical PASCAL VOC dataset, has plateaued in the last few years. The best-performing methods are complex ensemble systems that typically combine multiple low-level image features with high-level context. In this paper, we propose a simple and scalable detection algorithm that improves mean average precision (mAP) by more than 30\% relative to the previous best result on VOC 2012---achieving a mAP of 53.3\%. Our approach combines two key insights: (1) one can apply high-capacity convolutional neural networks (CNNs) to bottom-up region proposals in order to localize and segment objects and (2) when labeled training data is scarce, supervised pre-training for an auxiliary task, followed by domain-specific fine-tuning, yields a significant performance boost. Since we combine region proposals with CNNs, we call our method R-CNN: Regions with CNN features. We also compare R-CNN to OverFeat, a recently proposed sliding-window detector based on a similar CNN architecture. We find that R-CNN outperforms OverFeat by a large margin on the 200-class ILSVRC2013 detection dataset. Source code for the complete system is available at http://www.cs.berkeley.edu/\textasciitilde rbg/rcnn.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\detection\\Girshick et al_2014_R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\J94G5KIA\\1311.html}
}

@article{girshickRegionBasedConvolutionalNetworks2016,
  title = {Region-{{Based Convolutional Networks}} for {{Accurate Object Detection}} and {{Segmentation}}},
  author = {Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  date = {2016-01},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {38},
  number = {1},
  pages = {142--158},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2015.2437384},
  abstract = {Object detection performance, as measured on the canonical PASCAL VOC Challenge datasets, plateaued in the final years of the competition. The best-performing methods were complex ensemble systems that typically combined multiple low-level image features with high-level context. In this paper, we propose a simple and scalable detection algorithm that improves mean average precision (mAP) by more than 50 percent relative to the previous best result on VOC 2012-achieving a mAP of 62.4 percent. Our approach combines two ideas: (1) one can apply high-capacity convolutional networks (CNNs) to bottom-up region proposals in order to localize and segment objects and (2) when labeled training data are scarce, supervised pre-training for an auxiliary task, followed by domain-specific fine-tuning, boosts performance significantly. Since we combine region proposals with CNNs, we call the resulting model an R-CNN or Region-based Convolutional Network. Source code for the complete system is available at http://www.cs.berkeley.edu/ rbg/rcnn.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  keywords = {convolutional networks,deep learning,detection,Detectors,Feature extraction,Image segmentation,notion,Object detection,Object recognition,Proposals,semantic segmentation,Support vector machines,Training,transfer learning},
  file = {Y:\paper\computer_vision_topics_18\object detection\Girshick et al_2016_Region-Based Convolutional Networks for Accurate Object Detection and.pdf}
}

@online{gkioxariMeshRCNN2020,
  title = {Mesh {{R-CNN}}},
  author = {Gkioxari, Georgia and Malik, Jitendra and Johnson, Justin},
  date = {2020-01-25},
  eprint = {1906.02739},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1906.02739},
  url = {http://arxiv.org/abs/1906.02739},
  urldate = {2023-08-05},
  abstract = {Rapid advances in 2D perception have led to systems that accurately detect objects in real-world images. However, these systems make predictions in 2D, ignoring the 3D structure of the world. Concurrently, advances in 3D shape prediction have mostly focused on synthetic benchmarks and isolated objects. We unify advances in these two areas. We propose a system that detects objects in real-world images and produces a triangle mesh giving the full 3D shape of each detected object. Our system, called Mesh R-CNN, augments Mask R-CNN with a mesh prediction branch that outputs meshes with varying topological structure by first predicting coarse voxel representations which are converted to meshes and refined with a graph convolution network operating over the mesh's vertices and edges. We validate our mesh prediction branch on ShapeNet, where we outperform prior work on single-image shape prediction. We then deploy our full Mesh R-CNN system on Pix3D, where we jointly detect objects and predict their 3D shapes.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\3d image understanding\\Gkioxari et al_2020_Mesh R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VRX2MLPC\\1906.html}
}

@article{gnyawaliCoopetitionGiantsCollaboration2011,
  title = {Co-Opetition between Giants: {{Collaboration}} with Competitors for Technological Innovation},
  author = {Gnyawali, Devi R. and Park, Byung-Jin (Robert)},
  date = {2011},
  journaltitle = {Research Policy},
  volume = {40},
  number = {5},
  pages = {650--663},
  doi = {10.1016/j.respol.2011.01.009}
}

@online{goldbergWord2vecExplainedDeriving2014,
  title = {Word2vec {{Explained}}: Deriving {{Mikolov}} et al.'s Negative-Sampling Word-Embedding Method},
  shorttitle = {Word2vec {{Explained}}},
  author = {Goldberg, Yoav and Levy, Omer},
  date = {2014-02-15},
  eprint = {1402.3722},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1402.3722},
  urldate = {2022-09-25},
  abstract = {The word2vec software of Tomas Mikolov and colleagues (https://code.google.com/p/word2vec/ ) has gained a lot of traction lately, and provides state-of-the-art word embeddings. The learning models behind the software are described in two research papers. We found the description of the models in these papers to be somewhat cryptic and hard to follow. While the motivations and presentation may be obvious to the neural-networks language-modeling crowd, we had to struggle quite a bit to figure out the rationale behind the equations. This note is an attempt to explain equation (4) (negative sampling) in "Distributed Representations of Words and Phrases and their Compositionality" by Tomas Mikolov, Ilya Sutskever, Kai Chen, Greg Corrado and Jeffrey Dean.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\artificial intelligence\\NLP\\Goldberg_Levy_2014_word2vec Explained.pdf;C\:\\Users\\chsey\\Zotero\\storage\\YXDAY35Y\\1402.html}
}

@online{gongASTAudioSpectrogram2021,
  title = {{{AST}}: {{Audio Spectrogram Transformer}}},
  shorttitle = {{{AST}}},
  author = {Gong, Yuan and Chung, Yu-An and Glass, James},
  date = {2021-07-08},
  eprint = {2104.01778},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2104.01778},
  urldate = {2024-02-02},
  abstract = {In the past decade, convolutional neural networks (CNNs) have been widely adopted as the main building block for end-to-end audio classification models, which aim to learn a direct mapping from audio spectrograms to corresponding labels. To better capture long-range global context, a recent trend is to add a self-attention mechanism on top of the CNN, forming a CNN-attention hybrid model. However, it is unclear whether the reliance on a CNN is necessary, and if neural networks purely based on attention are sufficient to obtain good performance in audio classification. In this paper, we answer the question by introducing the Audio Spectrogram Transformer (AST), the first convolution-free, purely attention-based model for audio classification. We evaluate AST on various audio classification benchmarks, where it achieves new state-of-the-art results of 0.485 mAP on AudioSet, 95.6\% accuracy on ESC-50, and 98.1\% accuracy on Speech Commands V2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Sound,notion},
  file = {Y\:\\paper\\2024_research\\Gong et al_2021_AST.pdf;C\:\\Users\\chsey\\Zotero\\storage\\R9MKTJH2\\2104.html}
}

@book{goodfellowDeepLearning2016,
  title = {Deep Learning},
  author = {Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  date = {2016},
  series = {Adaptive Computation and Machine Learning},
  publisher = {The MIT Press},
  location = {Cambridge, Massachusetts},
  isbn = {978-0-262-03561-3},
  langid = {english},
  pagetotal = {775},
  keywords = {Machine learning},
  file = {Y:\paper\textbook\Goodfellow et al_2016_Deep learning.pdf}
}

@online{goodfellowGenerativeAdversarialNetworks2014,
  title = {Generative {{Adversarial Networks}}},
  author = {Goodfellow, Ian J. and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  date = {2014-06-10},
  eprint = {1406.2661},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1406.2661},
  url = {http://arxiv.org/abs/1406.2661},
  urldate = {2023-08-05},
  abstract = {We propose a new framework for estimating generative models via an adversarial process, in which we simultaneously train two models: a generative model G that captures the data distribution, and a discriminative model D that estimates the probability that a sample came from the training data rather than G. The training procedure for G is to maximize the probability of D making a mistake. This framework corresponds to a minimax two-player game. In the space of arbitrary functions G and D, a unique solution exists, with G recovering the training data distribution and D equal to 1/2 everywhere. In the case where G and D are defined by multilayer perceptrons, the entire system can be trained with backpropagation. There is no need for any Markov chains or unrolled approximate inference networks during either training or generation of samples. Experiments demonstrate the potential of the framework through qualitative and quantitative evaluation of the generated samples.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Goodfellow et al_2014_Generative Adversarial Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RKESFDSK\\1406.html}
}

@online{GoogleHagsulGeomsaeg,
  title = {Google 학술 검색},
  url = {https://scholar.google.com/scholar?hl=ko&as_sdt=0%2C5&q=learning+with+noisy+label&btnG=},
  urldate = {2022-09-01},
  file = {C:\Users\chsey\Zotero\storage\QSV7NEPA\scholar.html}
}

@article{gouKnowledgeDistillationSurvey2021,
  title = {Knowledge {{Distillation}}: {{A Survey}}},
  shorttitle = {Knowledge {{Distillation}}},
  author = {Gou, Jianping and Yu, Baosheng and Maybank, Stephen J. and Tao, Dacheng},
  date = {2021-06-01},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {129},
  number = {6},
  pages = {1789--1819},
  issn = {1573-1405},
  doi = {10.1007/s11263-021-01453-z},
  url = {https://doi.org/10.1007/s11263-021-01453-z},
  urldate = {2024-01-29},
  abstract = {In recent years, deep neural networks have been successful in both industry and academia, especially for computer vision tasks. The great success of deep learning is mainly due to its scalability to encode large-scale data and to maneuver billions of model parameters. However, it is a challenge to deploy these cumbersome deep models on devices with limited resources, e.g., mobile phones and embedded devices, not only because of the high computational complexity but also the large storage requirements. To this end, a variety of model compression and acceleration techniques have been developed. As a representative type of model compression and acceleration, knowledge distillation effectively learns a small student model from a large teacher model. It has received rapid increasing attention from the community. This paper provides a comprehensive survey of knowledge distillation from the perspectives of knowledge categories, training schemes, teacher–student architecture, distillation algorithms, performance comparison and applications. Furthermore, challenges in knowledge distillation are briefly reviewed and comments on future research are discussed and forwarded.},
  langid = {english},
  keywords = {Deep neural networks,Knowledge distillation,Knowledge transfer,Model compression,notion,Teacher–student architecture},
  file = {Y:\paper\2024_research\Gou et al_2021_Knowledge Distillation.pdf}
}

@online{goyalAccurateLargeMinibatch2018,
  title = {Accurate, {{Large Minibatch SGD}}: {{Training ImageNet}} in 1 {{Hour}}},
  shorttitle = {Accurate, {{Large Minibatch SGD}}},
  author = {Goyal, Priya and Dollár, Piotr and Girshick, Ross and Noordhuis, Pieter and Wesolowski, Lukasz and Kyrola, Aapo and Tulloch, Andrew and Jia, Yangqing and He, Kaiming},
  date = {2018-04-30},
  eprint = {1706.02677},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1706.02677},
  urldate = {2022-09-08},
  abstract = {Deep learning thrives with large neural networks and large datasets. However, larger networks and larger datasets result in longer training times that impede research and development progress. Distributed synchronous SGD offers a potential solution to this problem by dividing SGD minibatches over a pool of parallel workers. Yet to make this scheme efficient, the per-worker workload must be large, which implies nontrivial growth in the SGD minibatch size. In this paper, we empirically show that on the ImageNet dataset large minibatches cause optimization difficulties, but when these are addressed the trained networks exhibit good generalization. Specifically, we show no loss of accuracy when training with large minibatch sizes up to 8192 images. To achieve this result, we adopt a hyper-parameter-free linear scaling rule for adjusting learning rates as a function of minibatch size and develop a new warmup scheme that overcomes optimization challenges early in training. With these simple techniques, our Caffe2-based system trains ResNet-50 with a minibatch size of 8192 on 256 GPUs in one hour, while matching small minibatch accuracy. Using commodity hardware, our implementation achieves \textasciitilde 90\% scaling efficiency when moving from 8 to 256 GPUs. Our findings enable training visual recognition models on internet-scale data with high efficiency.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Distributed Parallel and Cluster Computing,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\Goyal et al_2018_Accurate, Large Minibatch SGD.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HCXGFRQZ\\1706.html}
}

@online{goyalAccurateLargeMinibatch2018a,
  title = {Accurate, {{Large Minibatch SGD}}: {{Training ImageNet}} in 1 {{Hour}}},
  shorttitle = {Accurate, {{Large Minibatch SGD}}},
  author = {Goyal, Priya and Dollár, Piotr and Girshick, Ross and Noordhuis, Pieter and Wesolowski, Lukasz and Kyrola, Aapo and Tulloch, Andrew and Jia, Yangqing and He, Kaiming},
  date = {2018-04-30},
  eprint = {1706.02677},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.02677},
  url = {http://arxiv.org/abs/1706.02677},
  urldate = {2022-09-15},
  abstract = {Deep learning thrives with large neural networks and large datasets. However, larger networks and larger datasets result in longer training times that impede research and development progress. Distributed synchronous SGD offers a potential solution to this problem by dividing SGD minibatches over a pool of parallel workers. Yet to make this scheme efficient, the per-worker workload must be large, which implies nontrivial growth in the SGD minibatch size. In this paper, we empirically show that on the ImageNet dataset large minibatches cause optimization difficulties, but when these are addressed the trained networks exhibit good generalization. Specifically, we show no loss of accuracy when training with large minibatch sizes up to 8192 images. To achieve this result, we adopt a hyper-parameter-free linear scaling rule for adjusting learning rates as a function of minibatch size and develop a new warmup scheme that overcomes optimization challenges early in training. With these simple techniques, our Caffe2-based system trains ResNet-50 with a minibatch size of 8192 on 256 GPUs in one hour, while matching small minibatch accuracy. Using commodity hardware, our implementation achieves \textasciitilde 90\% scaling efficiency when moving from 8 to 256 GPUs. Our findings enable training visual recognition models on internet-scale data with high efficiency.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Distributed Parallel and Cluster Computing,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\Goyal et al_2018_Accurate, Large Minibatch SGD.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VLVPEXQ6\\1706.html}
}

@online{goyalLargerScaleTransformersMultilingual2021,
  title = {Larger-{{Scale Transformers}} for {{Multilingual Masked Language Modeling}}},
  author = {Goyal, Naman and Du, Jingfei and Ott, Myle and Anantharaman, Giri and Conneau, Alexis},
  date = {2021-05-02},
  eprint = {2105.00572},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2105.00572},
  urldate = {2024-08-23},
  abstract = {Recent work has demonstrated the effectiveness of cross-lingual language model pretraining for cross-lingual understanding. In this study, we present the results of two larger multilingual masked language models, with 3.5B and 10.7B parameters. Our two new models dubbed XLM-R XL and XLM-R XXL outperform XLM-R by 1.8\% and 2.4\% average accuracy on XNLI. Our model also outperforms the RoBERTa-Large model on several English tasks of the GLUE benchmark by 0.3\% on average while handling 99 more languages. This suggests pretrained models with larger capacity may obtain both strong performance on high-resource languages while greatly improving low-resource languages. We make our code and models publicly available.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {C:\Users\chsey\Zotero\storage\JPGJ66U9\Goyal 등 - 2021 - Larger-Scale Transformers for Multilingual Masked .pdf}
}

@article{goyalMakingVQAMatter,
  title = {Making the v in {{VQA Matter}}: {{Elevating}} the {{Role}} of {{Image Understanding}} in {{Visual Question Answering}}},
  author = {Goyal, Yash and Khot, Tejas and Summers-Stay, Douglas and Batra, Dhruv and Parikh, Devi},
  abstract = {Problems at the intersection of vision and language are of significant importance both as challenging research questions and for the rich set of applications they enable. However, inherent structure in our world and bias in our language tend to be a simpler signal for learning than visual modalities, resulting in models that ignore visual information, leading to an inflated sense of their capability.},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Goyal et al_Making the v in VQA Matter.pdf}
}

@article{goyalMakingVQAMatter2019,
  title = {Making the {{V}} in {{VQA Matter}}: {{Elevating}} the {{Role}} of {{Image Understanding}} in {{Visual Question Answering}}},
  shorttitle = {Making the {{V}} in {{VQA Matter}}},
  author = {Goyal, Yash and Khot, Tejas and Agrawal, Aishwarya and Summers-Stay, Douglas and Batra, Dhruv and Parikh, Devi},
  date = {2019-04-01},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {127},
  number = {4},
  pages = {398--414},
  issn = {1573-1405},
  doi = {10.1007/s11263-018-1116-0},
  url = {https://doi.org/10.1007/s11263-018-1116-0},
  urldate = {2023-05-28},
  abstract = {The problem of visual question answering (VQA) is of significant importance both as a challenging research question and for the rich set of applications it enables. In this context, however, inherent structure in our world and bias in our language tend to be a simpler signal for learning than visual modalities, resulting in VQA models that ignore visual information, leading to an inflated sense of their capability. We propose to counter these language priors for the task of VQA and make vision (the V in VQA) matter! Specifically, we balance the popular VQA dataset (Antol et al., in: ICCV, 2015) by collecting complementary images such that every question in our balanced dataset is associated with not just a single image, but rather a pair of similar images that result in two different answers to the question. Our dataset is by construction more balanced than the original VQA dataset and has approximately twice the number of image-question pairs. Our complete balanced dataset is publicly available at http://visualqa.org/as part of the 2nd iteration of the VQA Dataset and Challenge (VQA v2.0). We further benchmark a number of state-of-art VQA models on our balanced dataset. All models perform significantly worse on our balanced dataset, suggesting that these models have indeed learned to exploit language priors. This finding provides the first concrete empirical evidence for what seems to be a qualitative sense among practitioners. We also present interesting insights from analysis of the participant entries in VQA Challenge 2017, organized by us on the proposed VQA v2.0 dataset. The results of the challenge were announced in the 2nd VQA Challenge Workshop at the IEEE Conference on Computer Vision and Pattern Recognition (CVPR) 2017. Finally, our data collection protocol for identifying complementary images enables us to develop a novel interpretable model, which in addition to providing an answer to the given (image, question) pair, also provides a counter-example based explanation. Specifically, it identifies an image that is similar to the original image, but it believes has a different answer to the same question. This can help in building trust for machines among their users.},
  langid = {english},
  keywords = {Visual question answering,VQA,VQA challenge},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Goyal et al_2019_Making the V in VQA Matter.pdf}
}

@article{grettonIntroductionRKHSSimple,
  title = {Introduction to {{RKHS}}, and Some Simple Kernel Algorithms},
  author = {Gretton, Arthur},
  pages = {33},
  langid = {english},
  file = {Y:\paper\2022 autumn intern\OOD\Gretton_Introduction to RKHS, and some simple kernel algorithms.pdf}
}

@article{griesTextsComputerScience,
  title = {Texts in {{Computer Science}}},
  author = {Gries, David and Hazzan, Orit},
  pages = {938},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA2\Gries_Hazzan_Texts in Computer Science.pdf}
}

@online{griggSelfSupervisedSupervisedMethods2021,
  title = {Do {{Self-Supervised}} and {{Supervised Methods Learn Similar Visual Representations}}?},
  author = {Grigg, Tom George and Busbridge, Dan and Ramapuram, Jason and Webb, Russ},
  date = {2021-12-02},
  eprint = {2110.00528},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2110.00528},
  url = {http://arxiv.org/abs/2110.00528},
  urldate = {2023-07-19},
  abstract = {Despite the success of a number of recent techniques for visual self-supervised deep learning, there has been limited investigation into the representations that are ultimately learned. By leveraging recent advances in the comparison of neural representations, we explore in this direction by comparing a contrastive self-supervised algorithm to supervision for simple image data in a common architecture. We find that the methods learn similar intermediate representations through dissimilar means, and that the representations diverge rapidly in the final few layers. We investigate this divergence, finding that these layers strongly fit to their distinct learning objectives. We also find that the contrastive objective implicitly fits the supervised objective in intermediate layers, but that the reverse is not true. Our work particularly highlights the importance of the learned intermediate representations, and raises critical questions for auxiliary task design.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Grigg et al_2021_Do Self-Supervised and Supervised Methods Learn Similar Visual Representations.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EI5WYSRP\\2110.html}
}

@online{guibasAdaptiveFourierNeural2022,
  title = {Adaptive {{Fourier Neural Operators}}: {{Efficient Token Mixers}} for {{Transformers}}},
  shorttitle = {Adaptive {{Fourier Neural Operators}}},
  author = {Guibas, John and Mardani, Morteza and Li, Zongyi and Tao, Andrew and Anandkumar, Anima and Catanzaro, Bryan},
  date = {2022-03-27},
  eprint = {2111.13587},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.13587},
  urldate = {2022-08-09},
  abstract = {Vision transformers have delivered tremendous success in representation learning. This is primarily due to effective token mixing through self attention. However, this scales quadratically with the number of pixels, which becomes infeasible for high-resolution inputs. To cope with this challenge, we propose Adaptive Fourier Neural Operator (AFNO) as an efficient token mixer that learns to mix in the Fourier domain. AFNO is based on a principled foundation of operator learning which allows us to frame token mixing as a continuous global convolution without any dependence on the input resolution. This principle was previously used to design FNO, which solves global convolution efficiently in the Fourier domain and has shown promise in learning challenging PDEs. To handle challenges in visual representation learning such as discontinuities in images and high resolution inputs, we propose principled architectural modifications to FNO which results in memory and computational efficiency. This includes imposing a block-diagonal structure on the channel mixing weights, adaptively sharing weights across tokens, and sparsifying the frequency modes via soft-thresholding and shrinkage. The resulting model is highly parallel with a quasi-linear complexity and has linear memory in the sequence size. AFNO outperforms self-attention mechanisms for few-shot segmentation in terms of both efficiency and accuracy. For Cityscapes segmentation with the Segformer-B3 backbone, AFNO can handle a sequence size of 65k and outperforms other efficient self-attention mechanisms.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\artificial intelligence\\Guibas et al_2022_Adaptive Fourier Neural Operators.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UBZZ74TS\\2111.html}
}

@article{guoAttentionMechanismsComputer2022,
  title = {Attention Mechanisms in Computer Vision: {{A}} Survey},
  shorttitle = {Attention Mechanisms in Computer Vision},
  author = {Guo, Meng-Hao and Xu, Tian-Xing and Liu, Jiang-Jiang and Liu, Zheng-Ning and Jiang, Peng-Tao and Mu, Tai-Jiang and Zhang, Song-Hai and Martin, Ralph R. and Cheng, Ming-Ming and Hu, Shi-Min},
  date = {2022-09-01},
  journaltitle = {Computational Visual Media},
  shortjournal = {Comp. Visual Media},
  volume = {8},
  number = {3},
  pages = {331--368},
  issn = {2096-0662},
  doi = {10.1007/s41095-022-0271-y},
  url = {https://doi.org/10.1007/s41095-022-0271-y},
  urldate = {2023-08-28},
  abstract = {Humans can naturally and effectively find salient regions in complex scenes. Motivated by this observation, attention mechanisms were introduced into computer vision with the aim of imitating this aspect of the human visual system. Such an attention mechanism can be regarded as a dynamic weight adjustment process based on features of the input image. Attention mechanisms have achieved great success in many visual tasks, including image classification, object detection, semantic segmentation, video understanding, image generation, 3D vision, multimodal tasks, and self-supervised learning. In this survey, we provide a comprehensive review of various attention mechanisms in computer vision and categorize them according to approach, such as channel attention, spatial attention, temporal attention, and branch attention; a related repository https://github.com/MenghaoGuo/Awesome-Vision-Attentionsis dedicated to collecting related work. We also suggest future directions for attention mechanism research.},
  langid = {english},
  keywords = {attention,computer vision,deep learning,notion,salience,transformer},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Guo et al_2022_Attention mechanisms in computer vision.pdf}
}

@inproceedings{guoCalibrationModernNeural2017,
  title = {On {{Calibration}} of {{Modern Neural Networks}}},
  booktitle = {Proceedings of the 34th {{International Conference}} on {{Machine Learning}}},
  author = {Guo, Chuan and Pleiss, Geoff and Sun, Yu and Weinberger, Kilian Q.},
  date = {2017-07-17},
  pages = {1321--1330},
  publisher = {PMLR},
  issn = {2640-3498},
  url = {https://proceedings.mlr.press/v70/guo17a.html},
  urldate = {2022-09-01},
  abstract = {Confidence calibration – the problem of predicting probability estimates representative of the true correctness likelihood – is important for classification models in many applications. We discover that modern neural networks, unlike those from a decade ago, are poorly calibrated. Through extensive experiments, we observe that depth, width, weight decay, and Batch Normalization are important factors influencing calibration. We evaluate the performance of various post-processing calibration methods on state-of-the-art architectures with image and document classification datasets. Our analysis and experiments not only offer insights into neural network learning, but also provide a simple and straightforward recipe for practical settings: on most datasets, temperature scaling – a single-parameter variant of Platt Scaling – is surprisingly effective at calibrating predictions.},
  eventtitle = {International {{Conference}} on {{Machine Learning}}},
  langid = {english},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Guo et al_2017_On Calibration of Modern Neural Networks.pdf;Y\:\\paper\\2022 autumn intern\\OOD\\Guo et al_2017_On Calibration of Modern Neural Networks2.pdf}
}

@online{guoNeRFReNNeuralRadiance2022,
  title = {{{NeRFReN}}: {{Neural Radiance Fields}} with {{Reflections}}},
  shorttitle = {{{NeRFReN}}},
  author = {Guo, Yuan-Chen and Kang, Di and Bao, Linchao and He, Yu and Zhang, Song-Hai},
  date = {2022-04-06},
  eprint = {2111.15234},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.15234},
  urldate = {2023-01-25},
  abstract = {Neural Radiance Fields (NeRF) has achieved unprecedented view synthesis quality using coordinate-based neural scene representations. However, NeRF's view dependency can only handle simple reflections like highlights but cannot deal with complex reflections such as those from glass and mirrors. In these scenarios, NeRF models the virtual image as real geometries which leads to inaccurate depth estimation, and produces blurry renderings when the multi-view consistency is violated as the reflected objects may only be seen under some of the viewpoints. To overcome these issues, we introduce NeRFReN, which is built upon NeRF to model scenes with reflections. Specifically, we propose to split a scene into transmitted and reflected components, and model the two components with separate neural radiance fields. Considering that this decomposition is highly under-constrained, we exploit geometric priors and apply carefully-designed training strategies to achieve reasonable decomposition results. Experiments on various self-captured scenes show that our method achieves high-quality novel view synthesis and physically sound depth estimation results while enabling scene editing applications.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,nerf reflective,연구 - 대상},
  file = {Y\:\\paper\\2022 winter intern\\Guo et al_2022_NeRFReN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TU5B7P2I\\2111.html}
}

@online{guptaLVISDatasetLarge2019,
  title = {{{LVIS}}: {{A Dataset}} for {{Large Vocabulary Instance Segmentation}}},
  shorttitle = {{{LVIS}}},
  author = {Gupta, Agrim and Dollár, Piotr and Girshick, Ross},
  date = {2019-09-15},
  eprint = {1908.03195},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1908.03195},
  url = {http://arxiv.org/abs/1908.03195},
  urldate = {2023-08-05},
  abstract = {Progress on object detection is enabled by datasets that focus the research community's attention on open challenges. This process led us from simple images to complex scenes and from bounding boxes to segmentation masks. In this work, we introduce LVIS (pronounced `el-vis'): a new dataset for Large Vocabulary Instance Segmentation. We plan to collect \textasciitilde 2 million high-quality instance segmentation masks for over 1000 entry-level object categories in 164k images. Due to the Zipfian distribution of categories in natural images, LVIS naturally has a long tail of categories with few training samples. Given that state-of-the-art deep learning methods for object detection perform poorly in the low-sample regime, we believe that our dataset poses an important and exciting new scientific challenge. LVIS is available at http://www.lvisdataset.org.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image segmentation\\Gupta et al_2019_LVIS.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CWXZACZ9\\1908.html}
}

@article{guptaObservingHumanObjectInteractions2009,
  title = {Observing {{Human-Object Interactions}}: {{Using Spatial}} and {{Functional Compatibility}} for {{Recognition}}},
  shorttitle = {Observing {{Human-Object Interactions}}},
  author = {Gupta, Abhinav and Kembhavi, Aniruddha and Davis, Larry S.},
  date = {2009-10},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {31},
  number = {10},
  pages = {1775--1789},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2009.83},
  abstract = {Interpretation of images and videos containing humans interacting with different objects is a daunting task. It involves understanding scene or event, analyzing human movements, recognizing manipulable objects, and observing the effect of the human movement on those objects. While each of these perceptual tasks can be conducted independently, recognition rate improves when interactions between them are considered. Motivated by psychological studies of human perception, we present a Bayesian approach which integrates various perceptual tasks involved in understanding human-object interactions. Previous approaches to object and action recognition rely on static shape or appearance feature matching and motion analysis, respectively. Our approach goes beyond these traditional approaches and applies spatial and functional constraints on each of the perceptual elements for coherent semantic interpretation. Such constraints allow us to recognize objects and actions when the appearances are not discriminative enough. We also demonstrate the use of such constraints in recognition of actions from static images without using any motion information.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  keywords = {Action recognition,Bayesian methods,functional recognition.,Humans,Image recognition,Information analysis,Layout,Motion analysis,notion,object recognition,Object recognition,Pattern recognition,Shape,Videos},
  file = {Y:\paper\computer_vision_topics_18\contextual cues\Gupta et al_2009_Observing Human-Object Interactions.pdf}
}

@inproceedings{gurariCaptioningImagesTaken2020,
  title = {Captioning {{Images Taken}} by {{People Who Are Blind}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Gurari, Danna and Zhao, Yinan and Zhang, Meng and Bhattacharya, Nilavra},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {417--434},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58520-4_25},
  abstract = {While an important problem in the vision community is to design algorithms that can automatically caption images, few publicly-available datasets for algorithm development directly address the interests of real users. Observing that people who are blind have relied on (human-based) image captioning services to learn about images they take for nearly a decade, we introduce the first image captioning dataset to represent this real use case. This new dataset, which we call VizWiz-Captions, consists of over 39,000 images originating from people who are blind that are each paired with five captions. We analyze this dataset to (1) characterize the typical captions, (2) characterize the diversity of content found in the images, and (3) compare its content to that found in eight popular vision datasets. We also analyze modern image captioning algorithms to identify what makes this new dataset challenging for the vision community. We publicly-share the dataset with captioning challenge instructions at https://vizwiz.org.},
  isbn = {978-3-030-58520-4},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Gurari et al_2020_Captioning Images Taken by People Who Are Blind.pdf}
}

@online{guSceneGraphGeneration2019,
  title = {Scene {{Graph Generation}} with {{External Knowledge}} and {{Image Reconstruction}}},
  author = {Gu, Jiuxiang and Zhao, Handong and Lin, Zhe and Li, Sheng and Cai, Jianfei and Ling, Mingyang},
  date = {2019-04-01},
  eprint = {1904.00560},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.00560},
  url = {http://arxiv.org/abs/1904.00560},
  urldate = {2023-05-30},
  abstract = {Scene graph generation has received growing attention with the advancements in image understanding tasks such as object detection, attributes and relationship prediction,\textasciitilde\textbackslash etc. However, existing datasets are biased in terms of object and relationship labels, or often come with noisy and missing annotations, which makes the development of a reliable scene graph prediction model very challenging. In this paper, we propose a novel scene graph generation algorithm with external knowledge and image reconstruction loss to overcome these dataset issues. In particular, we extract commonsense knowledge from the external knowledge base to refine object and phrase features for improving generalizability in scene graph generation. To address the bias of noisy object annotations, we introduce an auxiliary image reconstruction path to regularize the scene graph generation network. Extensive experiments show that our framework can generate better scene graphs, achieving the state-of-the-art performance on two benchmark datasets: Visual Relationship Detection and Visual Genome datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Gu et al_2019_Scene Graph Generation with External Knowledge and Image Reconstruction.pdf;C\:\\Users\\chsey\\Zotero\\storage\\K4H2E887\\1904.html}
}

@online{han2VPTEffectiveEfficient2023,
  title = {E\textasciicircum{{2VPT}}: {{An Effective}} and {{Efficient Approach}} for {{Visual Prompt Tuning}}},
  shorttitle = {E\textasciicircum{{2VPT}}},
  author = {Han, Cheng and Wang, Qifan and Cui, Yiming and Cao, Zhiwen and Wang, Wenguan and Qi, Siyuan and Liu, Dongfang},
  date = {2023-07-25},
  eprint = {2307.13770},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2307.13770},
  urldate = {2023-10-17},
  abstract = {As the size of transformer-based models continues to grow, fine-tuning these large-scale pretrained vision models for new tasks has become increasingly parameter-intensive. Parameter-efficient learning has been developed to reduce the number of tunable parameters during fine-tuning. Although these methods show promising results, there is still a significant performance gap compared to full fine-tuning. To address this challenge, we propose an Effective and Efficient Visual Prompt Tuning (E\textasciicircum 2VPT) approach for large-scale transformer-based model adaptation. Specifically, we introduce a set of learnable key-value prompts and visual prompts into self-attention and input layers, respectively, to improve the effectiveness of model fine-tuning. Moreover, we design a prompt pruning procedure to systematically prune low importance prompts while preserving model performance, which largely enhances the model's efficiency. Empirical results demonstrate that our approach outperforms several state-of-the-art baselines on two benchmarks, with considerably low parameter usage (e.g., 0.32\% of model parameters on VTAB-1k). Our code is available at https://github.com/ChengHan111/E2VPT.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_prompt\\Han et al_2023_E^2VPT2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UTABVHJQ\\2307.html}
}

@online{haoLanguageModelsAre2022,
  title = {Language {{Models}} Are {{General-Purpose Interfaces}}},
  author = {Hao, Yaru and Song, Haoyu and Dong, Li and Huang, Shaohan and Chi, Zewen and Wang, Wenhui and Ma, Shuming and Wei, Furu},
  date = {2022-06-13},
  eprint = {2206.06336},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.06336},
  urldate = {2024-01-31},
  abstract = {Foundation models have received much attention due to their effectiveness across a broad range of downstream applications. Though there is a big convergence in terms of architecture, most pretrained models are typically still developed for specific tasks or modalities. In this work, we propose to use language models as a general-purpose interface to various foundation models. A collection of pretrained encoders perceive diverse modalities (such as vision, and language), and they dock with a language model that plays the role of a universal task layer. We propose a semi-causal language modeling objective to jointly pretrain the interface and the modular encoders. We subsume the advantages and capabilities from both causal and non-causal modeling, thereby combining the best of two worlds. Specifically, the proposed method not only inherits the capabilities of in-context learning and open-ended generation from causal language modeling, but also is conducive to finetuning because of the bidirectional encoders. More importantly, our approach seamlessly unlocks the combinations of the above capabilities, e.g., enabling in-context learning or instruction following with finetuned encoders. Experimental results across various language-only and vision-language benchmarks show that our model outperforms or is competitive with specialized models on finetuning, zero-shot generalization, and few-shot learning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2024_research\\Hao et al_2022_Language Models are General-Purpose Interfaces2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\D7IEV6BG\\2206.html}
}

@online{haoLanguageModelsAre2022a,
  title = {Language {{Models}} Are {{General-Purpose Interfaces}}},
  author = {Hao, Yaru and Song, Haoyu and Dong, Li and Huang, Shaohan and Chi, Zewen and Wang, Wenhui and Ma, Shuming and Wei, Furu},
  date = {2022-06-13},
  eprint = {2206.06336},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.06336},
  urldate = {2024-01-30},
  abstract = {Foundation models have received much attention due to their effectiveness across a broad range of downstream applications. Though there is a big convergence in terms of architecture, most pretrained models are typically still developed for specific tasks or modalities. In this work, we propose to use language models as a general-purpose interface to various foundation models. A collection of pretrained encoders perceive diverse modalities (such as vision, and language), and they dock with a language model that plays the role of a universal task layer. We propose a semi-causal language modeling objective to jointly pretrain the interface and the modular encoders. We subsume the advantages and capabilities from both causal and non-causal modeling, thereby combining the best of two worlds. Specifically, the proposed method not only inherits the capabilities of in-context learning and open-ended generation from causal language modeling, but also is conducive to finetuning because of the bidirectional encoders. More importantly, our approach seamlessly unlocks the combinations of the above capabilities, e.g., enabling in-context learning or instruction following with finetuned encoders. Experimental results across various language-only and vision-language benchmarks show that our model outperforms or is competitive with specialized models on finetuning, zero-shot generalization, and few-shot learning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Hao et al_2022_Language Models are General-Purpose Interfaces.pdf;C\:\\Users\\chsey\\Zotero\\storage\\P898BLSV\\2206.html}
}

@online{hariharanLowshotVisualRecognition2017,
  title = {Low-Shot {{Visual Recognition}} by {{Shrinking}} and {{Hallucinating Features}}},
  author = {Hariharan, Bharath and Girshick, Ross},
  date = {2017-11-04},
  eprint = {1606.02819},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1606.02819},
  url = {http://arxiv.org/abs/1606.02819},
  urldate = {2023-08-05},
  abstract = {Low-shot visual learning---the ability to recognize novel object categories from very few examples---is a hallmark of human visual intelligence. Existing machine learning approaches fail to generalize in the same way. To make progress on this foundational problem, we present a low-shot learning benchmark on complex images that mimics challenges faced by recognition systems in the wild. We then propose a) representation regularization techniques, and b) techniques to hallucinate additional training examples for data-starved classes. Together, our methods improve the effectiveness of convolutional networks in low-shot learning, improving the one-shot accuracy on novel classes by 2.3x on the challenging ImageNet dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\few shot learning\\Hariharan_Girshick_2017_Low-shot Visual Recognition by Shrinking and Hallucinating Features.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BW69GPL2\\1606.html}
}

@article{hartleyMultipleViewGeometry,
  title = {Multiple {{View Geometry}} in {{Computer Vision}}, {{Second Edition}}},
  author = {Hartley, Richard and Zisserman, Andrew},
  langid = {english},
  file = {Y:\paper\textbook\Hartley_Zisserman_Multiple View Geometry in Computer Vision, Second Edition.pdf}
}

@article{hartleyMultipleViewGeometrya,
  title = {Multiple {{View Geometry}} in {{Computer Vision}}, {{Second Edition}}},
  author = {Hartley, Richard and Zisserman, Andrew},
  pages = {673},
  langid = {english},
  keywords = {_tablet},
  file = {C:\Users\jiho\OneDrive - GIST\바탕 화면\대학공부\2022 autumn\컴퓨터 비전\SfM\Richard Hartley Andrew Zisserman - Multiple View Geometry in Computer Vision, 2nd Edition (2004).pdf}
}

@article{hastieSurprisesHighdimensionalRidgeless2022,
  title = {Surprises in High-Dimensional Ridgeless Least Squares Interpolation},
  author = {Hastie, Trevor and Montanari, Andrea and Rosset, Saharon and Tibshirani, Ryan J.},
  date = {2022-04},
  journaltitle = {The Annals of Statistics},
  volume = {50},
  number = {2},
  pages = {949--986},
  publisher = {Institute of Mathematical Statistics},
  issn = {0090-5364, 2168-8966},
  doi = {10.1214/21-AOS2133},
  url = {https://projecteuclid.org/journals/annals-of-statistics/volume-50/issue-2/Surprises-in-high-dimensional-ridgeless-least-squares-interpolation/10.1214/21-AOS2133.full},
  urldate = {2024-03-27},
  abstract = {Interpolators—estimators that achieve zero training error—have attracted growing attention in machine learning, mainly because state-of-the art neural networks appear to be models of this type. In this paper, we study minimum ℓ2 norm (“ridgeless”) interpolation least squares regression, focusing on the high-dimensional regime in which the number of unknown parameters p is of the same order as the number of samples n. We consider two different models for the feature distribution: a linear model, where the feature vectors xi∈Rp are obtained by applying a linear transform to a vector of i.i.d. entries, xi=Σ1/2zi (with zi∈Rp); and a nonlinear model, where the feature vectors are obtained by passing the input through a random one-layer neural network, xi=φ(Wzi) (with zi∈Rd, W∈Rp×d a matrix of i.i.d. entries, and φ an activation function acting componentwise on Wzi). We recover—in a precise quantitative way—several phenomena that have been observed in large-scale neural networks and kernel machines, including the “double descent” behavior of the prediction risk, and the potential benefits of overparametrization.},
  keywords = {62F12,62J02,62J05,62J07,interpolation,overparametrization,Random matrix theory,regression,Ridge regression},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Hastie et al_2022_Surprises in high-dimensional ridgeless least squares interpolation.pdf}
}

@online{heDeepResidualLearning2015,
  title = {Deep {{Residual Learning}} for {{Image Recognition}}},
  author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  date = {2015-12-10},
  eprint = {1512.03385},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1512.03385},
  url = {http://arxiv.org/abs/1512.03385},
  urldate = {2022-07-04},
  abstract = {Deeper neural networks are more difficult to train. We present a residual learning framework to ease the training of networks that are substantially deeper than those used previously. We explicitly reformulate the layers as learning residual functions with reference to the layer inputs, instead of learning unreferenced functions. We provide comprehensive empirical evidence showing that these residual networks are easier to optimize, and can gain accuracy from considerably increased depth. On the ImageNet dataset we evaluate residual nets with a depth of up to 152 layers---8x deeper than VGG nets but still having lower complexity. An ensemble of these residual nets achieves 3.57\% error on the ImageNet test set. This result won the 1st place on the ILSVRC 2015 classification task. We also present analysis on CIFAR-10 with 100 and 1000 layers. The depth of representations is of central importance for many visual recognition tasks. Solely due to our extremely deep representations, we obtain a 28\% relative improvement on the COCO object detection dataset. Deep residual nets are foundations of our submissions to ILSVRC \& COCO 2015 competitions, where we also won the 1st places on the tasks of ImageNet detection, ImageNet localization, COCO detection, and COCO segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\He et al_2015_Deep Residual Learning for Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9KUPG5HK\\1512.html}
}

@online{heDeepResidualLearning2015a,
  title = {Deep {{Residual Learning}} for {{Image Recognition}}},
  author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  date = {2015-12-10},
  eprint = {1512.03385},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1512.03385},
  url = {http://arxiv.org/abs/1512.03385},
  urldate = {2022-12-09},
  abstract = {Deeper neural networks are more difficult to train. We present a residual learning framework to ease the training of networks that are substantially deeper than those used previously. We explicitly reformulate the layers as learning residual functions with reference to the layer inputs, instead of learning unreferenced functions. We provide comprehensive empirical evidence showing that these residual networks are easier to optimize, and can gain accuracy from considerably increased depth. On the ImageNet dataset we evaluate residual nets with a depth of up to 152 layers---8x deeper than VGG nets but still having lower complexity. An ensemble of these residual nets achieves 3.57\% error on the ImageNet test set. This result won the 1st place on the ILSVRC 2015 classification task. We also present analysis on CIFAR-10 with 100 and 1000 layers. The depth of representations is of central importance for many visual recognition tasks. Solely due to our extremely deep representations, we obtain a 28\% relative improvement on the COCO object detection dataset. Deep residual nets are foundations of our submissions to ILSVRC \& COCO 2015 competitions, where we also won the 1st places on the tasks of ImageNet detection, ImageNet localization, COCO detection, and COCO segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\traditional\\PA3\\He et al_2015_Deep Residual Learning for Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y7LID6JQ\\1512.html}
}

@online{heDeepResidualLearning2015b,
  title = {Deep {{Residual Learning}} for {{Image Recognition}}},
  author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  date = {2015-12-10},
  eprint = {1512.03385},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1512.03385},
  url = {http://arxiv.org/abs/1512.03385},
  urldate = {2023-08-05},
  abstract = {Deeper neural networks are more difficult to train. We present a residual learning framework to ease the training of networks that are substantially deeper than those used previously. We explicitly reformulate the layers as learning residual functions with reference to the layer inputs, instead of learning unreferenced functions. We provide comprehensive empirical evidence showing that these residual networks are easier to optimize, and can gain accuracy from considerably increased depth. On the ImageNet dataset we evaluate residual nets with a depth of up to 152 layers---8x deeper than VGG nets but still having lower complexity. An ensemble of these residual nets achieves 3.57\% error on the ImageNet test set. This result won the 1st place on the ILSVRC 2015 classification task. We also present analysis on CIFAR-10 with 100 and 1000 layers. The depth of representations is of central importance for many visual recognition tasks. Solely due to our extremely deep representations, we obtain a 28\% relative improvement on the COCO object detection dataset. Deep residual nets are foundations of our submissions to ILSVRC \& COCO 2015 competitions, where we also won the 1st places on the tasks of ImageNet detection, ImageNet localization, COCO detection, and COCO segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image classification\\He et al_2015_Deep Residual Learning for Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\79Z9BIJ3\\1512.html}
}

@inproceedings{heDeepResidualLearning2016,
  title = {Deep {{Residual Learning}} for {{Image Recognition}}},
  booktitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  date = {2016-06},
  pages = {770--778},
  publisher = {IEEE},
  location = {Las Vegas, NV, USA},
  doi = {10.1109/CVPR.2016.90},
  url = {http://ieeexplore.ieee.org/document/7780459/},
  urldate = {2022-11-27},
  abstract = {Deeper neural networks are more difficult to train. We present a residual learning framework to ease the training of networks that are substantially deeper than those used previously. We explicitly reformulate the layers as learning residual functions with reference to the layer inputs, instead of learning unreferenced functions. We provide comprehensive empirical evidence showing that these residual networks are easier to optimize, and can gain accuracy from considerably increased depth. On the ImageNet dataset we evaluate residual nets with a depth of up to 152 layers—8× deeper than VGG nets [40] but still having lower complexity. An ensemble of these residual nets achieves 3.57\% error on the ImageNet test set. This result won the 1st place on the ILSVRC 2015 classification task. We also present analysis on CIFAR-10 with 100 and 1000 layers.},
  eventtitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-4673-8851-1},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\reading assignment 5\He et al_2016_Deep Residual Learning for Image Recognition.pdf}
}

@inproceedings{heEnhancedBoundaryLearning2021,
  title = {Enhanced {{Boundary Learning}} for {{Glass-Like Object Segmentation}}},
  author = {He, Hao and Li, Xiangtai and Cheng, Guangliang and Shi, Jianping and Tong, Yunhai and Meng, Gaofeng and Prinet, Véronique and Weng, LuBin},
  date = {2021},
  pages = {15859--15868},
  url = {https://openaccess.thecvf.com/content/ICCV2021/html/He_Enhanced_Boundary_Learning_for_Glass-Like_Object_Segmentation_ICCV_2021_paper.html?ref=https://githubhelp.com},
  urldate = {2023-02-03},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  file = {Y:\paper\2022 winter intern\transparent_segmentation\He et al_2021_Enhanced Boundary Learning for Glass-Like Object Segmentation.pdf}
}

@inproceedings{heEnhancedBoundaryLearning2021a,
  title = {Enhanced {{Boundary Learning}} for {{Glass-like Object Segmentation}}},
  booktitle = {2021 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  author = {He, Hao and Li, Xiangtai and Cheng, Guangliang and Shi, Jianping and Tong, Yunhai and Meng, Gaofeng and Prinet, Veronique and Weng, LuBin},
  date = {2021-10},
  pages = {15839--15848},
  publisher = {IEEE},
  location = {Montreal, QC, Canada},
  doi = {10.1109/ICCV48922.2021.01556},
  url = {https://ieeexplore.ieee.org/document/9710709/},
  urldate = {2023-02-03},
  abstract = {Glass-like objects such as windows, bottles, and mirrors exist widely in the real world. Sensing these objects has many applications, including robot navigation and grasping. However, this task is very challenging due to the arbitrary scenes behind glass-like objects. This paper aims to solve the glass-like object segmentation problem via enhanced boundary learning. In particular, we first propose a novel refined differential module that outputs finer boundary cues. We then introduce an edge-aware point-based graph convolution network module to model the global shape along the boundary. We use these two modules to design a decoder that generates accurate and clean segmentation results, especially on the object contours. Both modules are lightweight and effective: they can be embedded into various segmentation models. In extensive experiments on three recent glass-like object segmentation datasets, including Trans10k, MSD, and GDD, our approach establishes new state-of-the-art results. We also illustrate the strong generalization properties of our method on three generic segmentation datasets, including Cityscapes, BDD, and COCO Stuff. Code and models will be available for further research.},
  eventtitle = {2021 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  isbn = {978-1-66542-812-5},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\TESI9BR4\He 등 - 2021 - Enhanced Boundary Learning for Glass-like Object S.pdf}
}

@online{heMaskedAutoencodersAre2021,
  title = {Masked {{Autoencoders Are Scalable Vision Learners}}},
  author = {He, Kaiming and Chen, Xinlei and Xie, Saining and Li, Yanghao and Dollár, Piotr and Girshick, Ross},
  date = {2021-12-19},
  eprint = {2111.06377},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.06377},
  url = {http://arxiv.org/abs/2111.06377},
  urldate = {2024-02-12},
  abstract = {This paper shows that masked autoencoders (MAE) are scalable self-supervised learners for computer vision. Our MAE approach is simple: we mask random patches of the input image and reconstruct the missing pixels. It is based on two core designs. First, we develop an asymmetric encoder-decoder architecture, with an encoder that operates only on the visible subset of patches (without mask tokens), along with a lightweight decoder that reconstructs the original image from the latent representation and mask tokens. Second, we find that masking a high proportion of the input image, e.g., 75\%, yields a nontrivial and meaningful self-supervisory task. Coupling these two designs enables us to train large models efficiently and effectively: we accelerate training (by 3x or more) and improve accuracy. Our scalable approach allows for learning high-capacity models that generalize well: e.g., a vanilla ViT-Huge model achieves the best accuracy (87.8\%) among methods that use only ImageNet-1K data. Transfer performance in downstream tasks outperforms supervised pre-training and shows promising scaling behavior.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\He et al_2021_Masked Autoencoders Are Scalable Vision Learners.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UX2QTGPP\\2111.html}
}

@online{heMaskedAutoencodersAre2021a,
  title = {Masked {{Autoencoders Are Scalable Vision Learners}}},
  author = {He, Kaiming and Chen, Xinlei and Xie, Saining and Li, Yanghao and Dollár, Piotr and Girshick, Ross},
  date = {2021-12-19},
  eprint = {2111.06377},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.06377},
  url = {http://arxiv.org/abs/2111.06377},
  urldate = {2023-07-04},
  abstract = {This paper shows that masked autoencoders (MAE) are scalable self-supervised learners for computer vision. Our MAE approach is simple: we mask random patches of the input image and reconstruct the missing pixels. It is based on two core designs. First, we develop an asymmetric encoder-decoder architecture, with an encoder that operates only on the visible subset of patches (without mask tokens), along with a lightweight decoder that reconstructs the original image from the latent representation and mask tokens. Second, we find that masking a high proportion of the input image, e.g., 75\%, yields a nontrivial and meaningful self-supervisory task. Coupling these two designs enables us to train large models efficiently and effectively: we accelerate training (by 3x or more) and improve accuracy. Our scalable approach allows for learning high-capacity models that generalize well: e.g., a vanilla ViT-Huge model achieves the best accuracy (87.8\%) among methods that use only ImageNet-1K data. Transfer performance in downstream tasks outperforms supervised pre-training and shows promising scaling behavior.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\He et al_2021_Masked Autoencoders Are Scalable Vision Learners.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NPNFKBSK\\2111.html}
}

@online{heMaskRCNN2018,
  title = {Mask {{R-CNN}}},
  author = {He, Kaiming and Gkioxari, Georgia and Dollár, Piotr and Girshick, Ross},
  date = {2018-01-24},
  eprint = {1703.06870},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1703.06870},
  url = {http://arxiv.org/abs/1703.06870},
  urldate = {2023-08-05},
  abstract = {We present a conceptually simple, flexible, and general framework for object instance segmentation. Our approach efficiently detects objects in an image while simultaneously generating a high-quality segmentation mask for each instance. The method, called Mask R-CNN, extends Faster R-CNN by adding a branch for predicting an object mask in parallel with the existing branch for bounding box recognition. Mask R-CNN is simple to train and adds only a small overhead to Faster R-CNN, running at 5 fps. Moreover, Mask R-CNN is easy to generalize to other tasks, e.g., allowing us to estimate human poses in the same framework. We show top results in all three tracks of the COCO suite of challenges, including instance segmentation, bounding-box object detection, and person keypoint detection. Without bells and whistles, Mask R-CNN outperforms all existing, single-model entries on every task, including the COCO 2016 challenge winners. We hope our simple and effective approach will serve as a solid baseline and help ease future research in instance-level recognition. Code has been made available at: https://github.com/facebookresearch/Detectron},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image segmentation\\He et al_2018_Mask R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\67944TK7\\1703.html}
}

@online{heMaskRCNN2018a,
  title = {Mask {{R-CNN}}},
  author = {He, Kaiming and Gkioxari, Georgia and Dollár, Piotr and Girshick, Ross},
  date = {2018-01-24},
  eprint = {1703.06870},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1703.06870},
  urldate = {2022-07-21},
  abstract = {We present a conceptually simple, flexible, and general framework for object instance segmentation. Our approach efficiently detects objects in an image while simultaneously generating a high-quality segmentation mask for each instance. The method, called Mask R-CNN, extends Faster R-CNN by adding a branch for predicting an object mask in parallel with the existing branch for bounding box recognition. Mask R-CNN is simple to train and adds only a small overhead to Faster R-CNN, running at 5 fps. Moreover, Mask R-CNN is easy to generalize to other tasks, e.g., allowing us to estimate human poses in the same framework. We show top results in all three tracks of the COCO suite of challenges, including instance segmentation, boundingbox object detection, and person keypoint detection. Without bells and whistles, Mask R-CNN outperforms all existing, single-model entries on every task, including the COCO 2016 challenge winners. We hope our simple and effective approach will serve as a solid baseline and help ease future research in instance-level recognition. Code has been made available at: https://github.com/ facebookresearch/Detectron.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\He et al_2018_Mask R-CNN.pdf}
}

@online{heMaskRCNN2018b,
  title = {Mask {{R-CNN}}},
  author = {He, Kaiming and Gkioxari, Georgia and Dollár, Piotr and Girshick, Ross},
  date = {2018-01-24},
  eprint = {1703.06870},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1703.06870},
  url = {http://arxiv.org/abs/1703.06870},
  urldate = {2022-07-05},
  abstract = {We present a conceptually simple, flexible, and general framework for object instance segmentation. Our approach efficiently detects objects in an image while simultaneously generating a high-quality segmentation mask for each instance. The method, called Mask R-CNN, extends Faster R-CNN by adding a branch for predicting an object mask in parallel with the existing branch for bounding box recognition. Mask R-CNN is simple to train and adds only a small overhead to Faster R-CNN, running at 5 fps. Moreover, Mask R-CNN is easy to generalize to other tasks, e.g., allowing us to estimate human poses in the same framework. We show top results in all three tracks of the COCO suite of challenges, including instance segmentation, bounding-box object detection, and person keypoint detection. Without bells and whistles, Mask R-CNN outperforms all existing, single-model entries on every task, including the COCO 2016 challenge winners. We hope our simple and effective approach will serve as a solid baseline and help ease future research in instance-level recognition. Code has been made available at: https://github.com/facebookresearch/Detectron},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\segmentation\\He et al_2018_Mask R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UINXZZQN\\1703.html}
}

@online{heMomentumContrastUnsupervised2020,
  title = {Momentum {{Contrast}} for {{Unsupervised Visual Representation Learning}}},
  author = {He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  date = {2020-03-23},
  eprint = {1911.05722},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1911.05722},
  url = {http://arxiv.org/abs/1911.05722},
  urldate = {2023-08-05},
  abstract = {We present Momentum Contrast (MoCo) for unsupervised visual representation learning. From a perspective on contrastive learning as dictionary look-up, we build a dynamic dictionary with a queue and a moving-averaged encoder. This enables building a large and consistent dictionary on-the-fly that facilitates contrastive unsupervised learning. MoCo provides competitive results under the common linear protocol on ImageNet classification. More importantly, the representations learned by MoCo transfer well to downstream tasks. MoCo can outperform its supervised pre-training counterpart in 7 detection/segmentation tasks on PASCAL VOC, COCO, and other datasets, sometimes surpassing it by large margins. This suggests that the gap between unsupervised and supervised representation learning has been largely closed in many vision tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\self supervised learning\\He et al_2020_Momentum Contrast for Unsupervised Visual Representation Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HCSGNR9N\\1911.html}
}

@article{hendersonArchitecturalInnovationReconfiguration1990,
  title = {Architectural {{Innovation}}: {{The Reconfiguration}} of {{Existing Product Technologies}} and the {{Failure}} of {{Established Firms}}},
  shorttitle = {Architectural {{Innovation}}},
  author = {Henderson, Rebecca M. and Clark, Kim B.},
  date = {1990},
  journaltitle = {Administrative Science Quarterly},
  volume = {35},
  number = {1},
  eprint = {2393549},
  eprinttype = {jstor},
  pages = {9--30},
  publisher = {[Sage Publications, Inc., Johnson Graduate School of Management, Cornell University]},
  issn = {0001-8392},
  doi = {10.2307/2393549},
  url = {https://www.jstor.org/stable/2393549},
  urldate = {2023-12-06},
  abstract = {This paper demonstrates that the traditional categorization of innovation as either incremental or radical is incomplete and potentially misleading and does not account for the sometimes disastrous effects on industry incumbents of seemingly minor improvements in technological products. We examine such innovations more closely and, distinguishing between the components of a product and the ways they are integrated into the system that is the product "architecture," define them as innovations that change the architecture of a product without changing its components. We show that architectural innovations destroy the usefulness of the architectural knowledge of established firms, and that since architectural knowledge tends to become embedded in the structure and information-processing procedures of established organizations, this destruction is difficult for firms to recognize and hard to correct. Architectural innovation therefore presents established organizations with subtle challenges that may have significant competitive implications. We illustrate the concept's explanatory force through an empirical study of the semiconductor photolithographic alignment equipment industry, which has experienced a number of architectural innovations.},
  file = {Y:\paper\management\Henderson_Clark_1990_Architectural Innovation.pdf}
}

@online{hendricksDecouplingRoleData2021,
  title = {Decoupling the {{Role}} of {{Data}}, {{Attention}}, and {{Losses}} in {{Multimodal Transformers}}},
  author = {Hendricks, Lisa Anne and Mellor, John and Schneider, Rosalia and Alayrac, Jean-Baptiste and Nematzadeh, Aida},
  date = {2021-01-31},
  eprint = {2102.00529},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2102.00529},
  urldate = {2024-05-28},
  abstract = {Recently multimodal transformer models have gained popularity because their performance on language and vision tasks suggest they learn rich visual-linguistic representations. Focusing on zero-shot image retrieval tasks, we study three important factors which can impact the quality of learned representations: pretraining data, the attention mechanism, and loss functions. By pretraining models on six datasets, we observe that dataset noise and language similarity to our downstream task are important indicators of model performance. Through architectural analysis, we learn that models with a multimodal attention mechanism can outperform deeper models with modality specific attention mechanisms. Finally, we show that successful contrastive losses used in the self-supervised learning literature do not yield similar performance gains when used in multimodal transformers},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\QSXV97ZI\Hendricks 등 - 2021 - Decoupling the Role of Data, Attention, and Losses.pdf}
}

@online{hendricksDecouplingRoleData2021a,
  title = {Decoupling the {{Role}} of {{Data}}, {{Attention}}, and {{Losses}} in {{Multimodal Transformers}}},
  author = {Hendricks, Lisa Anne and Mellor, John and Schneider, Rosalia and Alayrac, Jean-Baptiste and Nematzadeh, Aida},
  date = {2021-01-31},
  eprint = {2102.00529},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2102.00529},
  urldate = {2024-05-29},
  abstract = {Recently multimodal transformer models have gained popularity because their performance on language and vision tasks suggest they learn rich visual-linguistic representations. Focusing on zero-shot image retrieval tasks, we study three important factors which can impact the quality of learned representations: pretraining data, the attention mechanism, and loss functions. By pretraining models on six datasets, we observe that dataset noise and language similarity to our downstream task are important indicators of model performance. Through architectural analysis, we learn that models with a multimodal attention mechanism can outperform deeper models with modality specific attention mechanisms. Finally, we show that successful contrastive losses used in the self-supervised learning literature do not yield similar performance gains when used in multimodal transformers},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\VWPSSFWT\Hendricks 등 - 2021 - Decoupling the Role of Data, Attention, and Losses.pdf}
}

@online{hendrycksBaselineDetectingMisclassified2018,
  title = {A {{Baseline}} for {{Detecting Misclassified}} and {{Out-of-Distribution Examples}} in {{Neural Networks}}},
  author = {Hendrycks, Dan and Gimpel, Kevin},
  date = {2018-10-03},
  eprint = {1610.02136},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1610.02136},
  urldate = {2022-09-05},
  abstract = {We consider the two related problems of detecting if an example is misclassified or out-of-distribution. We present a simple baseline that utilizes probabilities from softmax distributions. Correctly classified examples tend to have greater maximum softmax probabilities than erroneously classified and out-of-distribution examples, allowing for their detection. We assess performance by defining several tasks in computer vision, natural language processing, and automatic speech recognition, showing the effectiveness of this baseline across all. We then show the baseline can sometimes be surpassed, demonstrating the room for future research on these underexplored detection tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Hendrycks_Gimpel_2018_A Baseline for Detecting Misclassified and Out-of-Distribution Examples in.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8DMEK34N\\1610.html}
}

@online{hendrycksDeepAnomalyDetection2019,
  title = {Deep {{Anomaly Detection}} with {{Outlier Exposure}}},
  author = {Hendrycks, Dan and Mazeika, Mantas and Dietterich, Thomas},
  date = {2019-01-28},
  eprint = {1812.04606},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1812.04606},
  urldate = {2022-09-06},
  abstract = {It is important to detect anomalous inputs when deploying machine learning systems. The use of larger and more complex inputs in deep learning magnifies the difficulty of distinguishing between anomalous and in-distribution examples. At the same time, diverse image and text data are available in enormous quantities. We propose leveraging these data to improve deep anomaly detection by training anomaly detectors against an auxiliary dataset of outliers, an approach we call Outlier Exposure (OE). This enables anomaly detectors to generalize and detect unseen anomalies. In extensive experiments on natural language processing and small- and large-scale vision tasks, we find that Outlier Exposure significantly improves detection performance. We also observe that cutting-edge generative models trained on CIFAR-10 may assign higher likelihoods to SVHN images than to CIFAR-10 images; we use OE to mitigate this issue. We also analyze the flexibility and robustness of Outlier Exposure, and identify characteristics of the auxiliary dataset that improve performance.},
  pubstate = {prepublished},
  version = {3},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Hendrycks et al_2019_Deep Anomaly Detection with Outlier Exposure.pdf;C\:\\Users\\chsey\\Zotero\\storage\\23X7IZSR\\1812.html}
}

@online{heParameterefficientModelAdaptation2023,
  title = {Parameter-Efficient {{Model Adaptation}} for {{Vision Transformers}}},
  author = {He, Xuehai and Li, Chunyuan and Zhang, Pengchuan and Yang, Jianwei and Wang, Xin Eric},
  date = {2023-07-13},
  eprint = {2203.16329},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.16329},
  url = {http://arxiv.org/abs/2203.16329},
  urldate = {2024-03-11},
  abstract = {In computer vision, it has achieved great transfer learning performance via adapting large-scale pretrained vision models (e.g., vision transformers) to downstream tasks. Common approaches for model adaptation either update all model parameters or leverage linear probes. In this paper, we aim to study parameter-efficient model adaptation strategies for vision transformers on the image classification task. We formulate efficient model adaptation as a subspace training problem and perform a comprehensive benchmarking over different efficient adaptation methods. We conduct an empirical study on each efficient model adaptation method focusing on its performance alongside parameter cost. Furthermore, we propose a parameter-efficient model adaptation framework, which first selects submodules by measuring local intrinsic dimensions and then projects them into subspace for further decomposition via a novel Kronecker Adaptation (KAdaptation) method. We analyze and compare our method with a diverse set of baseline model adaptation methods (including state-of-the-art methods for pretrained language models). Our method performs the best in terms of the tradeoff between accuracy and parameter efficiency across 20 image classification datasets under the few-shot setting and 7 image classification datasets under the full-shot setting.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\He et al_2023_Parameter-efficient Model Adaptation for Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QGGCEY7G\\2203.html}
}

@inproceedings{herdadeImageCaptioningTransforming2019,
  title = {Image {{Captioning}}: {{Transforming Objects}} into {{Words}}},
  shorttitle = {Image {{Captioning}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Herdade, Simao and Kappeler, Armin and Boakye, Kofi and Soares, Joao},
  date = {2019},
  volume = {32},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper_files/paper/2019/hash/680390c55bbd9ce416d1d69a9ab4760d-Abstract.html},
  urldate = {2023-05-27},
  abstract = {Image captioning models typically follow an encoder-decoder architecture which uses abstract image feature vectors as input to the encoder. One of the most successful algorithms uses feature vectors extracted from the region proposals obtained from an object detector. In this work we introduce the Object Relation Transformer, that builds upon this approach by explicitly incorporating information about the spatial relationship between input detected objects through geometric attention. Quantitative and qualitative results demonstrate the importance of such geometric attention for image captioning, leading to improvements on all common captioning metrics on the MS-COCO dataset. Code is available at https://github.com/yahoo/objectrelationtransformer .},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Herdade et al_2019_Image Captioning.pdf}
}

@article{hermensBusinessCyclesJoseph1941,
  title = {Business {{Cycles}} - {{Joseph A}}. {{Schumpeter}}: {{Business Cycles}}: {{A Theoretical}}, {{Historical}} and {{Statistical Analysis}} of the {{Capitalist Process}}. {{Two}} Vols., {{New York}}: {{McGraw Hill Book Co}}. {{Pp}}. Xvi, 1095. \$10.00.},
  shorttitle = {Business {{Cycles}} - {{Joseph A}}. {{Schumpeter}}},
  author = {Hermens, F. A.},
  date = {1941-04},
  journaltitle = {The Review of Politics},
  volume = {3},
  number = {2},
  pages = {261--264},
  publisher = {Cambridge University Press},
  issn = {1748-6858, 0034-6705},
  doi = {10.1017/S0034670500001170},
  url = {https://www.cambridge.org/core/journals/review-of-politics/article/abs/business-cycles-joseph-a-schumpeter-business-cycles-a-theoretical-historical-and-statistical-analysis-of-the-capitalist-process-two-vols-new-york-mcgraw-hill-book-co-pp-xvi-1095-1000/29BBEFCD973FB078BCB64DD7C3A8233B},
  urldate = {2023-12-25},
  abstract = {//static.cambridge.org/content/id/urn\%3Acambridge.org\%3Aid\%3Aarticle\%3AS0034670500001170/resource/name/firstPage-S0034670500001170a.jpg},
  langid = {english},
  file = {Y:\paper\management\Hermens_1941_Business Cycles - Joseph A.pdf}
}

@online{hernandezScalingLawsTransfer2021,
  title = {Scaling {{Laws}} for {{Transfer}}},
  author = {Hernandez, Danny and Kaplan, Jared and Henighan, Tom and McCandlish, Sam},
  date = {2021-02-01},
  eprint = {2102.01293},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2102.01293},
  urldate = {2024-05-14},
  abstract = {We study empirical scaling laws for transfer learning between distributions in an unsupervised, fine-tuning setting. When we train increasingly large neural networks from-scratch on a fixed-size dataset, they eventually become data-limited and stop improving in performance (cross-entropy loss). When we do the same for models pre-trained on a large language dataset, the slope in performance gains is merely reduced rather than going to zero. We calculate the effective data “transferred” from pre-training by determining how much data a transformer of the same size would have required to achieve the same loss when training from scratch. In other words, we focus on units of data while holding everything else fixed. We find that the effective data transferred is described well in the low data regime by a power-law of parameter count and fine-tuning dataset size. We believe the exponents in these power-laws correspond to measures of the generality of a model and proximity of distributions (in a directed rather than symmetric sense). We find that pre-training effectively multiplies the fine-tuning dataset size. Transfer, like overall performance, scales predictably in terms of parameters, data, and compute.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Hernandez et al_2021_Scaling Laws for Transfer.pdf}
}

@inproceedings{heSingleImageSuperresolution2011,
  title = {Single Image Super-Resolution Using {{Gaussian}} Process Regression},
  booktitle = {{{CVPR}} 2011},
  author = {He, He and Siu, Wan-Chi},
  date = {2011-06},
  pages = {449--456},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2011.5995713},
  abstract = {In this paper we address the problem of producing a high-resolution image from a single low-resolution image without any external training set. We propose a framework for both magnification and deblurring using only the original low-resolution image and its blurred version. In our method, each pixel is predicted by its neighbors through the Gaussian process regression. We show that when using a proper covariance function, the Gaussian process regression can perform soft clustering of pixels based on their local structures. We further demonstrate that our algorithm can extract adequate information contained in a single low-resolution image to generate a high-resolution image with sharp edges, which is comparable to or even superior in quality to the performance of other edge-directed and example-based super-resolution algorithms. Experimental results also show that our approach maintains high-quality performance at large magnifications.},
  eventtitle = {{{CVPR}} 2011},
  keywords = {Equations,Ground penetrating radar,Image edge detection,Image resolution,Mathematical model,Strontium,Training},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\He_Siu_2011_Single image super-resolution using Gaussian process regression.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7VURHXHV\\5995713.html}
}

@incollection{heSpatialPyramidPooling2014,
  title = {Spatial {{Pyramid Pooling}} in {{Deep Convolutional Networks}} for {{Visual Recognition}}},
  author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  date = {2014},
  volume = {8691},
  eprint = {1406.4729},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {346--361},
  doi = {10.1007/978-3-319-10578-9_23},
  url = {http://arxiv.org/abs/1406.4729},
  urldate = {2022-07-04},
  abstract = {Existing deep convolutional neural networks (CNNs) require a fixed-size (e.g., 224x224) input image. This requirement is "artificial" and may reduce the recognition accuracy for the images or sub-images of an arbitrary size/scale. In this work, we equip the networks with another pooling strategy, "spatial pyramid pooling", to eliminate the above requirement. The new network structure, called SPP-net, can generate a fixed-length representation regardless of image size/scale. Pyramid pooling is also robust to object deformations. With these advantages, SPP-net should in general improve all CNN-based image classification methods. On the ImageNet 2012 dataset, we demonstrate that SPP-net boosts the accuracy of a variety of CNN architectures despite their different designs. On the Pascal VOC 2007 and Caltech101 datasets, SPP-net achieves state-of-the-art classification results using a single full-image representation and no fine-tuning. The power of SPP-net is also significant in object detection. Using SPP-net, we compute the feature maps from the entire image only once, and then pool features in arbitrary regions (sub-images) to generate fixed-length representations for training the detectors. This method avoids repeatedly computing the convolutional features. In processing test images, our method is 24-102x faster than the R-CNN method, while achieving better or comparable accuracy on Pascal VOC 2007. In ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2014, our methods rank \#2 in object detection and \#3 in image classification among all 38 teams. This manuscript also introduces the improvement made for this competition.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\detection\\He et al_2014_Spatial Pyramid Pooling in Deep Convolutional Networks for Visual Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GAGKJCGF\\1406.html}
}

@inproceedings{heUnsupervisedPromptTuning2023,
  title = {Unsupervised {{Prompt Tuning}} for {{Text-Driven Object Detection}}},
  author = {He, Weizhen and Chen, Weijie and Chen, Binbin and Yang, Shicai and Xie, Di and Lin, Luojun and Qi, Donglian and Zhuang, Yueting},
  date = {2023},
  pages = {2651--2661},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/He_Unsupervised_Prompt_Tuning_for_Text-Driven_Object_Detection_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\He et al_2023_Unsupervised Prompt Tuning for Text-Driven Object Detection.pdf}
}

@book{hillMcGrawHillDictionaryScientific2003,
  title = {{{McGraw-Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}},
  author = {Hill, McGraw},
  date = {2003},
  eprint = {xOPzO5HVFfEC},
  eprinttype = {googlebooks},
  publisher = {McGraw-Hill Education},
  abstract = {For more than a quarter of a century, this amazingly comprehensive dictionary has been a standard international reference. Containing more than 115,000 terms and 125,000 definitions--from 100 areas of science and technology--this trusted resource provides definitions written in clear, simple language, understandable to the general reader, yet is consistent with the specialized use of the term.THE NEW SIXTH EDITION:* Thoroughly revised with 5,000 NEW TERMS* Each term includes a helpful pronunciation guide* Entries are complemented by 3,000 illustrations; appendices containing biographic listings, converison tables, taxonomic classification charts, and more* The only dictionary of scientific and technical terms to be thumb-indexedInvaluable to scientists, researchers, teachers, students, as well as interested lay persons, the McGraw-Hill Dictionary of Scientific and Technical Terms is truly the single best way for anyone to gain fluency in the language of science.},
  isbn = {978-0-07-042313-8},
  langid = {english},
  pagetotal = {2400},
  keywords = {Science / Reference,Social Science / Sociology / General,Technology & Engineering / Engineering (General)}
}

@inproceedings{hintonAutoencodersMinimumDescription1993,
  title = {Autoencoders, {{Minimum Description Length}} and {{Helmholtz Free Energy}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Hinton, Geoffrey E and Zemel, Richard},
  date = {1993},
  volume = {6},
  publisher = {Morgan-Kaufmann},
  url = {https://proceedings.neurips.cc/paper/1993/hash/9e3cfc48eccf81a0d57663e129aef3cb-Abstract.html},
  urldate = {2024-04-17},
  abstract = {An autoencoder network uses a set of recognition weights to convert an  input vector into a code vector.  It then uses a set of generative weights to  convert the code vector into an approximate reconstruction of the input  vector.  We derive an objective function for training autoencoders based  on the  Minimum  Description Length  (MDL)  principle.  The aim  is  to  minimize the information required to describe both the code vector and  the reconstruction error.  We  show  that this information  is  minimized  by choosing code vectors stochastically according to a Boltzmann distri(cid:173) bution, where the generative weights define the energy of each possible  code vector given  the input vector.  Unfortunately,  if the code vectors  use distributed representations, it is exponentially expensive to compute  this Boltzmann distribution because it involves all possible code vectors.  We show that the recognition weights of an autoencoder can  be used to  compute an approximation to the Boltzmann distribution and that this ap(cid:173) proximation gives an upper bound on the description length.  Even when  this bound is poor,  it can  be used  as a  Lyapunov function for learning  both the generative and the recognition weights.  We  demonstrate that  this approach can be used to learn factorial codes.},
  keywords = {notion},
  file = {Y:\paper\2024_research\Hinton_Zemel_1993_Autoencoders, Minimum Description Length and Helmholtz Free Energy.pdf}
}

@online{hoDenoisingDiffusionProbabilistic2020,
  title = {Denoising {{Diffusion Probabilistic Models}}},
  author = {Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  date = {2020-12-16},
  eprint = {2006.11239},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2006.11239},
  url = {http://arxiv.org/abs/2006.11239},
  urldate = {2024-01-24},
  abstract = {We present high quality image synthesis results using diffusion probabilistic models, a class of latent variable models inspired by considerations from nonequilibrium thermodynamics. Our best results are obtained by training on a weighted variational bound designed according to a novel connection between diffusion probabilistic models and denoising score matching with Langevin dynamics, and our models naturally admit a progressive lossy decompression scheme that can be interpreted as a generalization of autoregressive decoding. On the unconditional CIFAR10 dataset, we obtain an Inception score of 9.46 and a state-of-the-art FID score of 3.17. On 256x256 LSUN, we obtain sample quality similar to ProgressiveGAN. Our implementation is available at https://github.com/hojonathanho/diffusion},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Ho et al_2020_Denoising Diffusion Probabilistic Models.pdf;Y\:\\research\\research_paper\\denoising-diffusion-probabilistic-models - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\EUCZ4EDX\\2006.html}
}

@online{hoDenoisingDiffusionProbabilistic2020a,
  title = {Denoising {{Diffusion Probabilistic Models}}},
  author = {Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  date = {2020-12-16},
  eprint = {2006.11239},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2006.11239},
  url = {http://arxiv.org/abs/2006.11239},
  urldate = {2024-09-15},
  abstract = {We present high quality image synthesis results using diffusion probabilistic models, a class of latent variable models inspired by considerations from nonequilibrium thermodynamics. Our best results are obtained by training on a weighted variational bound designed according to a novel connection between diffusion probabilistic models and denoising score matching with Langevin dynamics, and our models naturally admit a progressive lossy decompression scheme that can be interpreted as a generalization of autoregressive decoding. On the unconditional CIFAR10 dataset, we obtain an Inception score of 9.46 and a state-of-the-art FID score of 3.17. On 256x256 LSUN, we obtain sample quality similar to ProgressiveGAN. Our implementation is available at https://github.com/hojonathanho/diffusion},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Ho et al_2020_Denoising Diffusion Probabilistic Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\47I7U993\\2006.html}
}

@inproceedings{hoiemGeometricContextSingle2005,
  title = {Geometric Context from a Single Image},
  booktitle = {Tenth {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}}'05) {{Volume}} 1},
  author = {Hoiem, D. and Efros, A.A. and Hebert, M.},
  date = {2005-10},
  volume = {1},
  pages = {654-661 Vol. 1},
  issn = {2380-7504},
  doi = {10.1109/ICCV.2005.107},
  abstract = {Many computer vision algorithms limit their performance by ignoring the underlying 3D geometric structure in the image. We show that we can estimate the coarse geometric properties of a scene by learning appearance-based models of geometric classes, even in cluttered natural scenes. Geometric classes describe the 3D orientation of an image region with respect to the camera. We provide a multiple-hypothesis framework for robustly estimating scene structure from a single image and obtaining confidences for each geometric label. These confidences can then be used to improve the performance of many other applications. We provide a thorough quantitative evaluation of our algorithm on a set of outdoor images and demonstrate its usefulness in two applications: object detection and automatic single-view reconstruction.},
  eventtitle = {Tenth {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}}'05) {{Volume}} 1},
  keywords = {Application software,Cameras,Computer vision,Humans,Image reconstruction,Layout,notion,Object detection,Robustness,Solid modeling,Surface reconstruction},
  file = {Y:\paper\computer_vision_topics_18\2.5d image understanding\Hoiem et al_2005_Geometric context from a single image.pdf}
}

@online{houlsbyParameterEfficientTransferLearning2019,
  title = {Parameter-{{Efficient Transfer Learning}} for {{NLP}}},
  author = {Houlsby, Neil and Giurgiu, Andrei and Jastrzebski, Stanislaw and Morrone, Bruna and family=Laroussilhe, given=Quentin, prefix=de, useprefix=true and Gesmundo, Andrea and Attariyan, Mona and Gelly, Sylvain},
  date = {2019-06-13},
  eprint = {1902.00751},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1902.00751},
  url = {http://arxiv.org/abs/1902.00751},
  urldate = {2023-11-22},
  abstract = {Fine-tuning large pre-trained models is an effective transfer mechanism in NLP. However, in the presence of many downstream tasks, fine-tuning is parameter inefficient: an entire new model is required for every task. As an alternative, we propose transfer with adapter modules. Adapter modules yield a compact and extensible model; they add only a few trainable parameters per task, and new tasks can be added without revisiting previous ones. The parameters of the original network remain fixed, yielding a high degree of parameter sharing. To demonstrate adapter's effectiveness, we transfer the recently proposed BERT Transformer model to 26 diverse text classification tasks, including the GLUE benchmark. Adapters attain near state-of-the-art performance, whilst adding only a few parameters per task. On GLUE, we attain within 0.4\% of the performance of full fine-tuning, adding only 3.6\% parameters per task. By contrast, fine-tuning trains 100\% of the parameters per task.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Houlsby et al_2019_Parameter-Efficient Transfer Learning for NLP.pdf;C\:\\Users\\chsey\\Zotero\\storage\\A5CEEVHY\\1902.html}
}

@online{huangClassIncrementalLearningCLIP2024,
  title = {Class-{{Incremental Learning}} with {{CLIP}}: {{Adaptive Representation Adjustment}} and {{Parameter Fusion}}},
  shorttitle = {Class-{{Incremental Learning}} with {{CLIP}}},
  author = {Huang, Linlan and Cao, Xusheng and Lu, Haori and Liu, Xialei},
  date = {2024-07-19},
  eprint = {2407.14143},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2407.14143},
  urldate = {2024-09-12},
  abstract = {Class-incremental learning is a challenging problem, where the goal is to train a model that can classify data from an increasing number of classes over time. With the advancement of vision-language pre-trained models such as CLIP, they demonstrate good generalization ability that allows them to excel in class-incremental learning with completely frozen parameters. However, further adaptation to downstream tasks by simply fine-tuning the model leads to severe forgetting. Most existing works with pre-trained models assume that the forgetting of old classes is uniform when the model acquires new knowledge. In this paper, we propose a method named Adaptive Representation Adjustment and Parameter Fusion (RAPF). During training for new data, we measure the influence of new classes on old ones and adjust the representations, using textual features. After training, we employ a decomposed parameter fusion to further mitigate forgetting during adapter module fine-tuning. Experiments on several conventional benchmarks show that our method achieves state-of-the-art results. Our code is available at https://github.com/linlany/RAPF.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\GWGTUPLY\Huang 등 - 2024 - Class-Incremental Learning with CLIP Adaptive Rep.pdf}
}

@online{huangCrossmodalCommonRepresentation2017,
  title = {Cross-Modal {{Common Representation Learning}} by {{Hybrid Transfer Network}}},
  author = {Huang, Xin and Peng, Yuxin and Yuan, Mingkuan},
  date = {2017-06-24},
  eprint = {1706.00153},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1706.00153},
  urldate = {2024-05-27},
  abstract = {DNN-based cross-modal retrieval is a research hotspot to retrieve across different modalities as image and text, but existing methods often face the challenge of insufficient cross-modal training data. In single-modal scenario, similar problem is usually relieved by transferring knowledge from largescale auxiliary datasets (as ImageNet). Knowledge from such single-modal datasets is also very useful for cross-modal retrieval, which can provide rich general semantic information that can be shared across different modalities. However, it is challenging to transfer useful knowledge from single-modal (as image) source domain to cross-modal (as image/text) target domain. Knowledge in source domain cannot be directly transferred to both two different modalities in target domain, and the inherent cross-modal correlation contained in target domain provides key hints for cross-modal retrieval which should be preserved during transfer process. This paper proposes Cross-modal Hybrid Transfer Network (CHTN) with two subnetworks: Modalsharing transfer subnetwork utilizes the modality in both source and target domains as a bridge, for transferring knowledge to both two modalities simultaneously; Layer-sharing correlation subnetwork preserves the inherent cross-modal semantic correlation to further adapt to cross-modal retrieval task. Cross-modal data can be converted to common representation by CHTN for retrieval, and comprehensive experiments on 3 datasets show its effectiveness.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {C:\Users\chsey\Zotero\storage\CQYH2GDK\1706.pdf}
}

@online{huangDeepNetworksStochastic2016,
  title = {Deep {{Networks}} with {{Stochastic Depth}}},
  author = {Huang, Gao and Sun, Yu and Liu, Zhuang and Sedra, Daniel and Weinberger, Kilian},
  date = {2016-07-28},
  eprint = {1603.09382},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1603.09382},
  url = {http://arxiv.org/abs/1603.09382},
  urldate = {2024-04-23},
  abstract = {Very deep convolutional networks with hundreds of layers have led to significant reductions in error on competitive benchmarks. Although the unmatched expressiveness of the many layers can be highly desirable at test time, training very deep networks comes with its own set of challenges. The gradients can vanish, the forward flow often diminishes, and the training time can be painfully slow. To address these problems, we propose stochastic depth, a training procedure that enables the seemingly contradictory setup to train short networks and use deep networks at test time. We start with very deep networks but during training, for each mini-batch, randomly drop a subset of layers and bypass them with the identity function. This simple approach complements the recent success of residual networks. It reduces training time substantially and improves the test error significantly on almost all data sets that we used for evaluation. With stochastic depth we can increase the depth of residual networks even beyond 1200 layers and still yield meaningful improvements in test error (4.91\% on CIFAR-10).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,notion},
  file = {Y\:\\paper\\2024_research\\Huang et al_2016_Deep Networks with Stochastic Depth.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GXJU6JAF\\1603.html}
}

@online{huangDenselyConnectedConvolutional2018,
  title = {Densely {{Connected Convolutional Networks}}},
  author = {Huang, Gao and Liu, Zhuang and family=Maaten, given=Laurens, prefix=van der, useprefix=true and Weinberger, Kilian Q.},
  date = {2018-01-28},
  eprint = {1608.06993},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1608.06993},
  url = {http://arxiv.org/abs/1608.06993},
  urldate = {2023-08-05},
  abstract = {Recent work has shown that convolutional networks can be substantially deeper, more accurate, and efficient to train if they contain shorter connections between layers close to the input and those close to the output. In this paper, we embrace this observation and introduce the Dense Convolutional Network (DenseNet), which connects each layer to every other layer in a feed-forward fashion. Whereas traditional convolutional networks with L layers have L connections - one between each layer and its subsequent layer - our network has L(L+1)/2 direct connections. For each layer, the feature-maps of all preceding layers are used as inputs, and its own feature-maps are used as inputs into all subsequent layers. DenseNets have several compelling advantages: they alleviate the vanishing-gradient problem, strengthen feature propagation, encourage feature reuse, and substantially reduce the number of parameters. We evaluate our proposed architecture on four highly competitive object recognition benchmark tasks (CIFAR-10, CIFAR-100, SVHN, and ImageNet). DenseNets obtain significant improvements over the state-of-the-art on most of them, whilst requiring less computation to achieve high performance. Code and pre-trained models are available at https://github.com/liuzhuang13/DenseNet .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image classification\\Huang et al_2018_Densely Connected Convolutional Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\958Y277B\\1608.html}
}

@online{huangDiversityAwareMetaVisual2023,
  title = {Diversity-{{Aware Meta Visual Prompting}}},
  author = {Huang, Qidong and Dong, Xiaoyi and Chen, Dongdong and Zhang, Weiming and Wang, Feifei and Hua, Gang and Yu, Nenghai},
  date = {2023-03-14},
  eprint = {2303.08138},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.08138},
  url = {http://arxiv.org/abs/2303.08138},
  urldate = {2023-11-06},
  abstract = {We present Diversity-Aware Meta Visual Prompting\textasciitilde (DAM-VP), an efficient and effective prompting method for transferring pre-trained models to downstream tasks with frozen backbone. A challenging issue in visual prompting is that image datasets sometimes have a large data diversity whereas a per-dataset generic prompt can hardly handle the complex distribution shift toward the original pretraining data distribution properly. To address this issue, we propose a dataset Diversity-Aware prompting strategy whose initialization is realized by a Meta-prompt. Specifically, we cluster the downstream dataset into small homogeneity subsets in a diversity-adaptive way, with each subset has its own prompt optimized separately. Such a divide-and-conquer design reduces the optimization difficulty greatly and significantly boosts the prompting performance. Furthermore, all the prompts are initialized with a meta-prompt, which is learned across several datasets. It is a bootstrapped paradigm, with the key observation that the prompting knowledge learned from previous datasets could help the prompt to converge faster and perform better on a new dataset. During inference, we dynamically select a proper prompt for each input, based on the feature distance between the input and each subset. Through extensive experiments, our DAM-VP demonstrates superior efficiency and effectiveness, clearly surpassing previous prompting methods in a series of downstream datasets for different pretraining models. Our code is available at: \textbackslash url\{https://github.com/shikiw/DAM-VP\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Huang et al_2023_Diversity-Aware Meta Visual Prompting.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WPWXTZQ9\\2303.html}
}

@online{huangFrustratinglyEasyTransferability2022,
  title = {Frustratingly {{Easy Transferability Estimation}}},
  author = {Huang, Long-Kai and Wei, Ying and Rong, Yu and Yang, Qiang and Huang, Junzhou},
  date = {2022-07-06},
  eprint = {2106.09362},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.09362},
  urldate = {2024-01-05},
  abstract = {Transferability estimation has been an essential tool in selecting a pre-trained model and the layers in it for transfer learning, to transfer, so as to maximize the performance on a target task and prevent negative transfer. Existing estimation algorithms either require intensive training on target tasks or have difficulties in evaluating the transferability between layers. To this end, we propose a simple, efficient, and effective transferability measure named TransRate. Through a single pass over examples of a target task, TransRate measures the transferability as the mutual information between features of target examples extracted by a pre-trained model and their labels. We overcome the challenge of efficient mutual information estimation by resorting to coding rate that serves as an effective alternative to entropy. From the perspective of feature representation, the resulting TransRate evaluates both completeness (whether features contain sufficient information of a target task) and compactness (whether features of each class are compact enough for good generalization) of pre-trained features. Theoretically, we have analyzed the close connection of TransRate to the performance after transfer learning. Despite its extraordinary simplicity in 10 lines of codes, TransRate performs remarkably well in extensive evaluations on 32 pre-trained models and 16 downstream tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\Huang et al_2022_Frustratingly Easy Transferability Estimation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QPW7FJ97\\2106.html}
}

@online{huangLoraHubEfficientCrossTask2024,
  title = {{{LoraHub}}: {{Efficient Cross-Task Generalization}} via {{Dynamic LoRA Composition}}},
  shorttitle = {{{LoraHub}}},
  author = {Huang, Chengsong and Liu, Qian and Lin, Bill Yuchen and Pang, Tianyu and Du, Chao and Lin, Min},
  date = {2024-08-18},
  eprint = {2307.13269},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2307.13269},
  urldate = {2024-09-17},
  abstract = {Low-rank adaptations (LoRA) are often employed to fine-tune large language models (LLMs) for new tasks. This paper investigates LoRA composability for cross-task generalization and introduces LoraHub, a simple framework devised for the purposive assembly of LoRA modules trained on diverse given tasks, with the objective of achieving adaptable performance on unseen tasks. With just a few examples from a new task, LoraHub can fluidly combine multiple LoRA modules, eliminating the need for human expertise and assumptions. Notably, the composition requires neither additional model parameters nor gradients. Empirical results on the Big-Bench Hard benchmark suggest that LoraHub, while not surpassing the performance of in-context learning, offers a notable performanceefficiency trade-off in few-shot scenarios by employing a significantly reduced number of tokens per example during inference. Notably, LoraHub establishes a better upper bound compared to in-context learning when paired with different demonstration examples, demonstrating its potential for future development. Our vision is to establish a platform for LoRA modules, empowering users to share their trained LoRA modules. This collaborative approach facilitates the seamless application of LoRA modules to novel tasks, contributing to an adaptive ecosystem. Our code is available at github.com/sail-sg/lorahub, and all the pre-trained LoRA modules are released at huggingface.co/lorahub.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,notion},
  file = {C:\Users\chsey\Zotero\storage\23RYMRFF\Huang 등 - 2024 - LoraHub Efficient Cross-Task Generalization via D.pdf}
}

@online{huangUnsupervisedPromptLearning2022,
  title = {Unsupervised {{Prompt Learning}} for {{Vision-Language Models}}},
  author = {Huang, Tony and Chu, Jack and Wei, Fangyun},
  date = {2022-08-22},
  eprint = {2204.03649},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2204.03649},
  url = {http://arxiv.org/abs/2204.03649},
  urldate = {2023-06-27},
  abstract = {Contrastive vision-language models like CLIP have shown great progress in transfer learning. In the inference stage, the proper text description, also known as prompt, needs to be carefully designed to correctly classify the given images. In order to avoid laborious prompt engineering, recent works such as CoOp, CLIP-Adapter and Tip-Adapter propose to adapt vision-language models for downstream image recognition tasks on a small set of labeled data. Though promising improvements are achieved, requiring labeled data from the target datasets may restrict the scalability. In this paper, we explore a different scenario, in which the labels of the target datasets are unprovided, and we present an unsupervised prompt learning (UPL) approach to avoid prompt engineering while simultaneously improving transfer performance of CLIP-like vision-language models. As far as we know, UPL is the first work to introduce unsupervised learning into prompt learning. Experimentally, our UPL outperforms original CLIP with prompt engineering on ImageNet as well as other 10 datasets. An enhanced version of UPL is even competitive with the 8-shot CoOp and the 8-shot TIP-Adapter on most datasets. Code and models are available at https://github.com/tonyhuang2022/UPL.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Huang et al_2022_Unsupervised Prompt Learning for Vision-Language Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XV3MQ8LS\\2204.html}
}

@article{hughesTwitterAdoptionUse2009,
  title = {Twitter Adoption and Use in Mass Convergence and Emergency Events},
  author = {Hughes, Amanda Lee and Palen, Leysia},
  date = {2009},
  journaltitle = {International Journal of Emergency Management},
  shortjournal = {IJEM},
  volume = {6},
  number = {3/4},
  pages = {248},
  issn = {1471-4825, 1741-5071},
  doi = {10.1504/IJEM.2009.031564},
  url = {http://www.inderscience.com/link.php?id=31564},
  urldate = {2023-05-25},
  abstract = {This paper offers a descriptive account of Twitter (a microblogging service) across four high-profile, mass convergence events - two emergency and two national security. We statistically examine how Twitter is being used surrounding these events, and compare and contrast how that behaviour is different from more general Twitter use. Our findings suggest that Twitter messages sent during these types of events contain more displays of information broadcasting and brokerage, and we observe that general Twitter use seems to have evolved over time to offer more of an information-sharing purpose. We also provide preliminary evidence that Twitter users who join during and in apparent relation to a mass convergence or emergency event are more likely to become long-term adopters of the technology.},
  langid = {english}
}

@online{huhTrainingNeuralNetworks2024,
  title = {Training {{Neural Networks}} from {{Scratch}} with {{Parallel Low-Rank Adapters}}},
  author = {Huh, Minyoung and Cheung, Brian and Bernstein, Jeremy and Isola, Phillip and Agrawal, Pulkit},
  date = {2024-07-26},
  eprint = {2402.16828},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2402.16828},
  urldate = {2024-09-13},
  abstract = {The scalability of deep learning models is fundamentally limited by computing resources, memory, and communication. Although methods like low-rank adaptation (LoRA) have reduced the cost of model finetuning, its application in model pre-training remains largely unexplored. This paper explores extending LoRA to model pretraining, identifying the inherent constraints and limitations of standard LoRA in this context. We introduce LoRA-the-Explorer (LTE), a novel bilevel optimization algorithm designed to enable parallel training of multiple low-rank heads across computing nodes, thereby reducing the need for frequent synchronization. Our approach includes extensive experimentation on vision transformers using various vision datasets, demonstrating that LTE is competitive with standard pre-training.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\VZIB7QB9\Huh 등 - 2024 - Training Neural Networks from Scratch with Paralle.pdf}
}

@online{huLoRALowRankAdaptation2021,
  title = {{{LoRA}}: {{Low-Rank Adaptation}} of {{Large Language Models}}},
  shorttitle = {{{LoRA}}},
  author = {Hu, Edward J. and Shen, Yelong and Wallis, Phillip and Allen-Zhu, Zeyuan and Li, Yuanzhi and Wang, Shean and Wang, Lu and Chen, Weizhu},
  date = {2021-10-16},
  eprint = {2106.09685},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.09685},
  urldate = {2023-07-31},
  abstract = {An important paradigm of natural language processing consists of large-scale pre-training on general domain data and adaptation to particular tasks or domains. As we pre-train larger models, full fine-tuning, which retrains all model parameters, becomes less feasible. Using GPT-3 175B as an example -- deploying independent instances of fine-tuned models, each with 175B parameters, is prohibitively expensive. We propose Low-Rank Adaptation, or LoRA, which freezes the pre-trained model weights and injects trainable rank decomposition matrices into each layer of the Transformer architecture, greatly reducing the number of trainable parameters for downstream tasks. Compared to GPT-3 175B fine-tuned with Adam, LoRA can reduce the number of trainable parameters by 10,000 times and the GPU memory requirement by 3 times. LoRA performs on-par or better than fine-tuning in model quality on RoBERTa, DeBERTa, GPT-2, and GPT-3, despite having fewer trainable parameters, a higher training throughput, and, unlike adapters, no additional inference latency. We also provide an empirical investigation into rank-deficiency in language model adaptation, which sheds light on the efficacy of LoRA. We release a package that facilitates the integration of LoRA with PyTorch models and provide our implementations and model checkpoints for RoBERTa, DeBERTa, and GPT-2 at https://github.com/microsoft/LoRA.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Hu et al_2021_LoRA.pdf;Y\:\\research\\research_paper\\lora-low-rank-adaptation-of-large-language-models - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\HN3285FI\\2106.html}
}

@online{huOnlineConvolutionalReparameterization2022,
  title = {Online {{Convolutional Re-parameterization}}},
  author = {Hu, Mu and Feng, Junyi and Hua, Jiashen and Lai, Baisheng and Huang, Jianqiang and Gong, Xiaojin and Hua, Xiansheng},
  date = {2022-04-02},
  eprint = {2204.00826},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2204.00826},
  url = {http://arxiv.org/abs/2204.00826},
  urldate = {2022-08-26},
  abstract = {Structural re-parameterization has drawn increasing attention in various computer vision tasks. It aims at improving the performance of deep models without introducing any inference-time cost. Though efficient during inference, such models rely heavily on the complicated training-time blocks to achieve high accuracy, leading to large extra training cost. In this paper, we present online convolutional re-parameterization (OREPA), a two-stage pipeline, aiming to reduce the huge training overhead by squeezing the complex training-time block into a single convolution. To achieve this goal, we introduce a linear scaling layer for better optimizing the online blocks. Assisted with the reduced training cost, we also explore some more effective re-param components. Compared with the state-of-the-art re-param models, OREPA is able to save the training-time memory cost by about 70\% and accelerate the training speed by around 2x. Meanwhile, equipped with OREPA, the models outperform previous methods on ImageNet by up to +0.6\%.We also conduct experiments on object detection and semantic segmentation and show consistent improvements on the downstream tasks. Codes are available at https://github.com/JUGGHM/OREPA\_CVPR2022 .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\layer\\Hu et al_2022_Online Convolutional Re-parameterization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\26DTM9KG\\2204.html}
}

@article{hwangNonAutoregressiveSignLanguage,
  title = {Non-{{Autoregressive Sign Language Production}} with {{Gaussian Space}}},
  author = {Hwang, Eui Jun},
  abstract = {Sign Language Production (SLP) aims to translate spoken language expressions into sign language expressions such as a sequence of sign poses or a sign video. Previous SLP works have used an autoregressive approach to learn the relationship between spoken words and sign poses. However, since the approaches work autoregressively, the decoder unintentionally regresses to the mean and even suffers from error propagation. In this work, we propose Non-Autoregressive Sign Language Production with Gaussian space (NSLP-G), a novel SLP model that uses non-autoregressive decoding to generate sign poses. To avoid direct regression, NSLP-G makes use of two phases. The first phase is to build a pose generator capable of generating various sign poses in a continuous sign pose space. At the second phase, we use a non-autoregressive Transformer to map from the source sentence to the target distribution. To validate the results of our model, we assess the quality of produced sign poses using Fréchet Gesture Distance, Mean Absolute Error of Joint coordination and back-translation evaluation. Experimental results show that NSLP-G outperforms the state-of-the-art model on the RWTH-PHOENIX-Weather 2014T dataset.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\EIBY92RL\Hwang - Non-Autoregressive Sign Language Production with G.pdf}
}

@online{ichnowskiDexNeRFUsingNeural2021,
  title = {Dex-{{NeRF}}: {{Using}} a {{Neural Radiance Field}} to {{Grasp Transparent Objects}}},
  shorttitle = {Dex-{{NeRF}}},
  author = {Ichnowski, Jeffrey and Avigal, Yahav and Kerr, Justin and Goldberg, Ken},
  date = {2021-10-27},
  eprint = {2110.14217},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2110.14217},
  urldate = {2023-01-03},
  abstract = {The ability to grasp and manipulate transparent objects is a major challenge for robots. Existing depth cameras have difficulty detecting, localizing, and inferring the geometry of such objects. We propose using neural radiance fields (NeRF) to detect, localize, and infer the geometry of transparent objects with sufficient accuracy to find and grasp them securely. We leverage NeRF's view-independent learned density, place lights to increase specular reflections, and perform a transparency-aware depth-rendering that we feed into the Dex-Net grasp planner. We show how additional lights create specular reflections that improve the quality of the depth map, and test a setup for a robot workcell equipped with an array of cameras to perform transparent object manipulation. We also create synthetic and real datasets of transparent objects in real-world settings, including singulated objects, cluttered tables, and the top rack of a dishwasher. In each setting we show that NeRF and Dex-Net are able to reliably compute robust grasps on transparent objects, achieving 90\% and 100\% grasp success rates in physical experiments on an ABB YuMi, on objects where baseline methods fail.},
  pubstate = {prepublished},
  keywords = {68T40 (Primary) 68T45 (Secondary),Computer Science - Computer Vision and Pattern Recognition,Computer Science - Robotics},
  file = {Y\:\\paper\\2022 winter intern\\Ichnowski et al_2021_Dex-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\YG7ZI6FB\\2110.html}
}

@inproceedings{idelbayevLowRankCompressionNeural2020,
  title = {Low-{{Rank Compression}} of {{Neural Nets}}: {{Learning}} the {{Rank}} of {{Each Layer}}},
  shorttitle = {Low-{{Rank Compression}} of {{Neural Nets}}},
  booktitle = {2020 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Idelbayev, Yerlan and Carreira-Perpinan, Miguel A.},
  date = {2020-06},
  pages = {8046--8056},
  publisher = {IEEE},
  location = {Seattle, WA, USA},
  doi = {10.1109/CVPR42600.2020.00807},
  url = {https://ieeexplore.ieee.org/document/9157223/},
  urldate = {2024-03-18},
  abstract = {Neural net compression can be achieved by approximating each layer’s weight matrix by a low-rank matrix. The real difficulty in doing this is not in training the resulting neural net (made up of one low-rank matrix per layer), but in determining what the optimal rank of each layer is—effectively, an architecture search problem with one hyperparameter per layer. We show that, with a suitable formulation, this problem is amenable to a mixed discretecontinuous optimization jointly over the ranks and over the matrix elements, and give a corresponding algorithm. We show that this indeed can select ranks much better than existing approaches, making low-rank compression much more attractive than previously thought. For example, we can make a VGG network faster than a ResNet and with nearly the same classification error.},
  eventtitle = {2020 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-72817-168-5},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Idelbayev_Carreira-Perpinan_2020_Low-Rank Compression of Neural Nets.pdf}
}

@article{ihrkeEikonalRenderingEfficient,
  title = {Eikonal {{Rendering}}: {{Eﬃcient Light Transport}} in {{Refractive Objects}}},
  author = {Ihrke, Ivo and Ziegler, Gernot and Tevs, Art and Theobalt, Christian and Magnor, Marcus and Seidel, Hans-Peter},
  abstract = {We present a new method for real-time rendering of sophisticated lighting effects in and around refractive objects. It enables us to realistically display refractive objects with complex material properties, such as arbitrarily varying refractive index, inhomogeneous attenuation, as well as spatially-varying anisotropic scattering and reflectance properties. User-controlled changes of lighting positions only require a few seconds of update time. Our method is based on a set of ordinary differential equations derived from the eikonal equation, the main postulate of geometric optics. This set of equations allows for fast casting of bent light rays with the complexity of a particle tracer. Based on this concept, we also propose an efficient light propagation technique using adaptive wavefront tracing. Efficient GPU implementations for our algorithmic concepts enable us to render a combination of visual effects that were previously not reproducible in real-time.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\K823KQTZ\Ihrke 등 - Eikonal Rendering Eﬃcient Light Transport in Refr.pdf}
}

@article{ihrkeEikonalRenderingEfficient2007,
  title = {Eikonal Rendering: Efficient Light Transport in Refractive Objects},
  shorttitle = {Eikonal Rendering},
  author = {Ihrke, Ivo and Ziegler, Gernot and Tevs, Art and Theobalt, Christian and Magnor, Marcus and Seidel, Hans-Peter},
  date = {2007-07-29},
  journaltitle = {ACM Transactions on Graphics},
  shortjournal = {ACM Trans. Graph.},
  volume = {26},
  number = {3},
  pages = {59--es},
  issn = {0730-0301},
  doi = {10.1145/1276377.1276451},
  url = {https://doi.org/10.1145/1276377.1276451},
  urldate = {2023-02-02},
  abstract = {We present a new method for real-time rendering of sophisticated lighting effects in and around refractive objects. It enables us to realistically display refractive objects with complex material properties, such as arbitrarily varying refractive index, inhomogeneous attenuation, as well as spatially-varying anisotropic scattering and reflectance properties. User-controlled changes of lighting positions only require a few seconds of update time. Our method is based on a set of ordinary differential equations derived from the eikonal equation, the main postulate of geometric optics. This set of equations allows for fast casting of bent light rays with the complexity of a particle tracer. Based on this concept, we also propose an efficient light propagation technique using adaptive wavefront tracing. Efficient GPU implementations for our algorithmic concepts enable us to render a combination of visual effects that were previously not reproducible in real-time.},
  keywords = {geometric optics,light transport,real-time rendering,refractive objects}
}

@article{ihrkeEikonalRenderingEfficienta,
  title = {Eikonal {{Rendering}}: {{Eﬃcient Light Transport}} in {{Refractive Objects}}},
  author = {Ihrke, Ivo and Ziegler, Gernot and Tevs, Art and Theobalt, Christian and Magnor, Marcus and Seidel, Hans-Peter},
  abstract = {We present a new method for real-time rendering of sophisticated lighting effects in and around refractive objects. It enables us to realistically display refractive objects with complex material properties, such as arbitrarily varying refractive index, inhomogeneous attenuation, as well as spatially-varying anisotropic scattering and reflectance properties. User-controlled changes of lighting positions only require a few seconds of update time. Our method is based on a set of ordinary differential equations derived from the eikonal equation, the main postulate of geometric optics. This set of equations allows for fast casting of bent light rays with the complexity of a particle tracer. Based on this concept, we also propose an efficient light propagation technique using adaptive wavefront tracing. Efficient GPU implementations for our algorithmic concepts enable us to render a combination of visual effects that were previously not reproducible in real-time.},
  langid = {english},
  file = {Y:\paper\2022 winter intern\Ihrke et al_Eikonal Rendering.pdf}
}

@online{ilharcoEditingModelsTask2023,
  title = {Editing {{Models}} with {{Task Arithmetic}}},
  author = {Ilharco, Gabriel and Ribeiro, Marco Tulio and Wortsman, Mitchell and Gururangan, Suchin and Schmidt, Ludwig and Hajishirzi, Hannaneh and Farhadi, Ali},
  date = {2023-03-31},
  eprint = {2212.04089},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2212.04089},
  urldate = {2024-09-30},
  abstract = {Changing how pre-trained models behave—e.g., improving their performance on a downstream task or mitigating biases learned during pre-training—is a common practice when developing machine learning systems. In this work, we propose a new paradigm for steering the behavior of neural networks, centered around task vectors. A task vector specifies a direction in the weight space of a pre-trained model, such that movement in that direction improves performance on the task. We build task vectors by subtracting the weights of a pre-trained model from the weights of the same model after fine-tuning on a task. We show that these task vectors can be modified and combined together through arithmetic operations such as negation and addition, and the behavior of the resulting model is steered accordingly. Negating a task vector decreases performance on the target task, with little change in model behavior on control tasks. Moreover, adding task vectors together can improve performance on multiple tasks at once. Finally, when tasks are linked by an analogy relationship of the form “A is to B as C is to D”, combining task vectors from three of the tasks can improve performance on the fourth, even when no data from the fourth task is used for training. Overall, our experiments with several models, modalities and tasks show that task arithmetic is a simple, efficient and effective way of editing models.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\95JP7X7Z\Ilharco 등 - 2023 - Editing Models with Task Arithmetic.pdf}
}

@online{ImageClassificationUsing,
  title = {Image Classification Using {{LoRA}}},
  url = {https://huggingface.co/docs/peft/task_guides/image_classification_lora},
  urldate = {2024-01-23},
  abstract = {We’re on a journey to advance and democratize artificial intelligence through open source and open science.},
  file = {C:\Users\chsey\Zotero\storage\VPZ47XKS\image_classification_lora.html}
}

@online{imfeldTransformerFusionOptimal2024,
  title = {Transformer {{Fusion}} with {{Optimal Transport}}},
  author = {Imfeld, Moritz and Graldi, Jacopo and Giordano, Marco and Hofmann, Thomas and Anagnostidis, Sotiris and Singh, Sidak Pal},
  date = {2024-04-22},
  eprint = {2310.05719},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.2310.05719},
  url = {http://arxiv.org/abs/2310.05719},
  urldate = {2024-10-23},
  abstract = {Fusion is a technique for merging multiple independently-trained neural networks in order to combine their capabilities. Past attempts have been restricted to the case of fully-connected, convolutional, and residual networks. This paper presents a systematic approach for fusing two or more transformer-based networks exploiting Optimal Transport to (soft-)align the various architectural components. We flesh out an abstraction for layer alignment, that can generalize to arbitrary architectures - in principle - and we apply this to the key ingredients of Transformers such as multi-head self-attention, layer-normalization, and residual connections, and we discuss how to handle them via various ablation studies. Furthermore, our method allows the fusion of models of different sizes (heterogeneous fusion), providing a new and efficient way to compress Transformers. The proposed approach is evaluated on both image classification tasks via Vision Transformer and natural language modeling tasks using BERT. Our approach consistently outperforms vanilla fusion, and, after a surprisingly short finetuning, also outperforms the individual converged parent models. In our analysis, we uncover intriguing insights about the significant role of soft alignment in the case of Transformers. Our results showcase the potential of fusing multiple Transformers, thus compounding their expertise, in the budding paradigm of model fusion and recombination. Code is available at https://github.com/graldij/transformer-fusion.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Imfeld et al_2024_Transformer Fusion with Optimal Transport.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TA8ZVC8C\\2310.html}
}

@online{ImpactDigitalizationRetailers,
  title = {Impact of Digitalization on Retailers and Its Future Trends - {{ScienceDirect}}},
  url = {https://www.sciencedirect.com/science/article/pii/S2214785321046186},
  urldate = {2023-12-28},
  file = {Y:\paper\management\Impact of digitalization on retailers and its future trends - ScienceDirect.pdf}
}

@online{ImpactDigitalizationRetailersa,
  title = {Impact of Digitalization on Retailers and Its Future Trends - {{ScienceDirect}}},
  url = {https://www.sciencedirect.com/science/article/pii/S2214785321046186},
  urldate = {2023-12-28}
}

@online{ImpactDigitalTransformation,
  title = {The Impact of Digital Transformation on the Retailing Value Chain - {{ScienceDirect}}},
  url = {https://www.sciencedirect.com/science/article/pii/S0167811618300739},
  urldate = {2023-12-27},
  file = {C:\Users\chsey\Zotero\storage\GSCVEG6H\S0167811618300739.html}
}

@online{ImpactDigitalTransformationa,
  title = {The Impact of Digital Transformation on the Retailing Value Chain - {{ScienceDirect}}},
  url = {https://www.sciencedirect.com/science/article/pii/S0167811618300739},
  urldate = {2023-12-28}
}

@inproceedings{imranTwitterLifelineHumanannotated2016,
  title = {Twitter as a {{Lifeline}}: {{Human-annotated Twitter Corpora}} for {{NLP}} of {{Crisis-related Messages}}},
  shorttitle = {Twitter as a {{Lifeline}}},
  booktitle = {Proceedings of the {{Tenth International Conference}} on {{Language Resources}} and {{Evaluation}} ({{LREC}}'16)},
  author = {Imran, Muhammad and Mitra, Prasenjit and Castillo, Carlos},
  date = {2016-05},
  pages = {1638--1643},
  publisher = {European Language Resources Association (ELRA)},
  location = {Portorož, Slovenia},
  url = {https://aclanthology.org/L16-1259},
  urldate = {2023-05-25},
  abstract = {Microblogging platforms such as Twitter provide active communication channels during mass convergence and emergency events such as earthquakes, typhoons. During the sudden onset of a crisis situation, affected people post useful information on Twitter that can be used for situational awareness and other humanitarian disaster response efforts, if processed timely and effectively. Processing social media information pose multiple challenges such as parsing noisy, brief and informal messages, learning information categories from the incoming stream of messages and classifying them into different classes among others. One of the basic necessities of many of these tasks is the availability of data, in particular human-annotated data. In this paper, we present human-annotated Twitter corpora collected during 19 different crises that took place between 2013 and 2015. To demonstrate the utility of the annotations, we train machine learning classifiers. Moreover, we publish first largest word2vec word embeddings trained on 52 million crisis-related tweets. To deal with tweets language issues, we present human-annotated normalized lexical resources for different lexical variations.},
  eventtitle = {{{LREC}} 2016},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Imran et al_2016_Twitter as a Lifeline.pdf}
}

@inproceedings{imranTwitterLifelineHumanannotated2016a,
  title = {Twitter as a Lifeline: {{Human-annotated Twitter}} Corpora for {{NLP}} of Crisis-Related Messages},
  shorttitle = {Twitter as a Lifeline},
  author = {Imran, M. and Mitra, P. and Castillo, C.},
  date = {2016},
  pages = {1638--1643},
  abstract = {Microblogging platforms such as Twitter provide active communication channels during mass convergence and emergency events such as earthquakes, typhoons. During the sudden onset of a crisis situation, affected people post useful information on Twitter that can be used for situational awareness and other humanitarian disaster response efforts, if processed timely and effectively. Processing social media information pose multiple challenges such as parsing noisy, brief and informal messages, learning information categories from the incoming stream of messages and classifying them into different classes among others. One of the basic necessities of many of these tasks is the availability of data, in particular human-annotated data. In this paper, we present human-annotated Twitter corpora collected during 19 different crises that took place between 2013 and 2015. To demonstrate the utility of the annotations, we train machine learning classifiers. Moreover, we publish first largest word2vec word embeddings trained on 52 million crisis-related tweets. To deal with tweets language issues, we present human-annotated normalized lexical resources for different lexical variations.},
  eventtitle = {Proceedings of the 10th {{International Conference}} on {{Language Resources}} and {{Evaluation}}, {{LREC}} 2016},
  isbn = {978-2-9517408-9-1},
  langid = {english},
  keywords = {Disaster response,Natural language processing,Supervised classification,Twitter}
}

@online{inanModelingIntensificationSign2022,
  title = {Modeling {{Intensification}} for {{Sign Language Generation}}: {{A Computational Approach}}},
  shorttitle = {Modeling {{Intensification}} for {{Sign Language Generation}}},
  author = {İnan, Mert and Zhong, Yang and Hassan, Sabit and Quandt, Lorna and Alikhani, Malihe},
  date = {2022-03-17},
  eprint = {2203.09679},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2203.09679},
  urldate = {2023-05-03},
  abstract = {End-to-end sign language generation models do not accurately represent the prosody in sign language. A lack of temporal and spatial variations leads to poor-quality generated presentations that confuse human interpreters. In this paper, we aim to improve the prosody in generated sign languages by modeling intensification in a data-driven manner. We present different strategies grounded in linguistics of sign language that inform how intensity modifiers can be represented in gloss annotations. To employ our strategies, we first annotate a subset of the benchmark PHOENIX-14T, a German Sign Language dataset, with different levels of intensification. We then use a supervised intensity tagger to extend the annotated dataset and obtain labels for the remaining portion of it. This enhanced dataset is then used to train state-of-the-art transformer models for sign language generation. We find that our efforts in intensification modeling yield better results when evaluated with automatic metrics. Human evaluation also indicates a higher preference of the videos generated using our model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_PBL\\İnan et al_2022_Modeling Intensification for Sign Language Generation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7S8JEMS8\\2203.html}
}

@misc{Initial_reportPdf,
  title = {Initial\_report.Pdf},
  file = {C:\Users\chsey\Zotero\storage\9IM94SGK\initial_report.pdf}
}

@unpublished{InstantnerfPptx,
  title = {Instant-Nerf.Pptx},
  url = {https://docs.google.com/presentation/d/16rx53IR5mCa0MyG1HeJpUzDUht7bZYwK},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\instant-nerf.pdf}
}

@report{intuitAnualReport2005,
  title = {Anual Report},
  author = {Intuit},
  date = {2005},
  url = {https://investors.intuit.com/files/doc_financials/2005/ar/2005_annual_report.pdf},
  urldate = {2024-01-01},
  file = {C:\Users\chsey\Zotero\storage\BIAW82UX\2005_annual_report.pdf}
}

@inproceedings{ioffeBatchNormalizationAccelerating2015,
  title = {Batch {{Normalization}}: {{Accelerating Deep Network Training}} by {{Reducing Internal Covariate Shift}}},
  shorttitle = {Batch {{Normalization}}},
  booktitle = {Proceedings of the 32nd {{International Conference}} on {{Machine Learning}}},
  author = {Ioffe, Sergey and Szegedy, Christian},
  date = {2015-06-01},
  pages = {448--456},
  publisher = {PMLR},
  issn = {1938-7228},
  url = {https://proceedings.mlr.press/v37/ioffe15.html},
  urldate = {2023-05-28},
  abstract = {Training Deep Neural Networks is complicated by the fact that the distribution of each layer’s inputs changes during training, as the parameters of the previous layers change. This slows down the training by requiring lower learning rates and careful parameter initialization, and makes it notoriously hard to train models with saturating nonlinearities. We refer to this phenomenon as internal covariate shift, and address the problem by normalizing layer inputs. Our method draws its strength from making normalization a part of the model architecture and performing the normalization for each training mini-batch. Batch Normalization allows us to use much higher learning rates and be less careful about initialization, and in some cases eliminates the need for Dropout. Applied to a stateof-the-art image classification model, Batch Normalization achieves the same accuracy with 14 times fewer training steps, and beats the original model by a significant margin. Using an ensemble of batch-normalized networks, we improve upon the best published result on ImageNet classification: reaching 4.82\% top-5 test error, exceeding the accuracy of human raters.},
  eventtitle = {International {{Conference}} on {{Machine Learning}}},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Ioffe_Szegedy_2015_Batch Normalization.pdf}
}

@online{iqbalMSANetMultiSimilarityAttention2022,
  title = {{{MSANet}}: {{Multi-Similarity}} and {{Attention Guidance}} for {{Boosting Few-Shot Segmentation}}},
  shorttitle = {{{MSANet}}},
  author = {Iqbal, Ehtesham and Safarov, Sirojbek and Bang, Seongdeok},
  date = {2022-06-20},
  eprint = {2206.09667},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2206.09667},
  url = {http://arxiv.org/abs/2206.09667},
  urldate = {2023-11-23},
  abstract = {Few-shot segmentation aims to segment unseen-class objects given only a handful of densely labeled samples. Prototype learning, where the support feature yields a singleor several prototypes by averaging global and local object information, has been widely used in FSS. However, utilizing only prototype vectors may be insufficient to represent the features for all training data. To extract abundant features and make more precise predictions, we propose a Multi-Similarity and Attention Network (MSANet) including two novel modules, a multi-similarity module and an attention module. The multi-similarity module exploits multiple feature-maps of support images and query images to estimate accurate semantic relationships. The attention module instructs the network to concentrate on class-relevant information. The network is tested on standard FSS datasets, PASCAL-5i 1-shot, PASCAL-5i 5-shot, COCO-20i 1-shot, and COCO-20i 5-shot. The MSANet with the backbone of ResNet-101 achieves the state-of-the-art performance for all 4-benchmark datasets with mean intersection over union (mIoU) of 69.13\%, 73.99\%, 51.09\%, 56.80\%, respectively. Code is available at https://github.com/AIVResearch/MSANet},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\few shot dense\\Iqbal et al_2022_MSANet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\345E4QNH\\2206.html}
}

@inproceedings{izsakHowTrainBERT2021,
  title = {How to {{Train BERT}} with an {{Academic Budget}}},
  booktitle = {Proceedings of the 2021 {{Conference}} on {{Empirical Methods}} in {{Natural Language Processing}}},
  author = {Izsak, Peter and Berchansky, Moshe and Levy, Omer},
  editor = {Moens, Marie-Francine and Huang, Xuanjing and Specia, Lucia and Yih, Scott Wen-tau},
  date = {2021-01},
  pages = {10644--10652},
  publisher = {Association for Computational Linguistics},
  location = {Online and Punta Cana, Dominican Republic},
  doi = {10.18653/v1/2021.emnlp-main.831},
  url = {https://aclanthology.org/2021.emnlp-main.831},
  urldate = {2024-03-17},
  abstract = {While large language models a la BERT are used ubiquitously in NLP, pretraining them is considered a luxury that only a few well-funded industry labs can afford. How can one train such models with a more modest budget? We present a recipe for pretraining a masked language model in 24 hours using a single low-end deep learning server. We demonstrate that through a combination of software optimizations, design choices, and hyperparameter tuning, it is possible to produce models that are competitive with BERT-base on GLUE tasks at a fraction of the original pretraining cost.},
  eventtitle = {{{EMNLP}} 2021},
  keywords = {notion},
  file = {Y:\paper\2024_research\Izsak et al_2021_How to Train BERT with an Academic Budget.pdf}
}

@article{jacsoMcGrawHillDictionary2002,
  title = {{{McGraw Hill}} Dictionary of Scientific and Technical Terms},
  author = {Jacso, Peter},
  date = {2002-09-01},
  journaltitle = {Online},
  shortjournal = {Online},
  volume = {26}
}

@article{jainVideoCaptioningReview2022,
  title = {Video Captioning: A Review of Theory, Techniques and Practices},
  shorttitle = {Video Captioning},
  author = {Jain, Vanita and Al-Turjman, Fadi and Chaudhary, Gopal and Nayar, Devang and Gupta, Varun and Kumar, Aayush},
  date = {2022-10-01},
  journaltitle = {Multimedia Tools and Applications},
  shortjournal = {Multimed Tools Appl},
  volume = {81},
  number = {25},
  pages = {35619--35653},
  issn = {1573-7721},
  doi = {10.1007/s11042-021-11878-w},
  url = {https://doi.org/10.1007/s11042-021-11878-w},
  urldate = {2023-04-16},
  abstract = {In today’s world, video captioning is extensively used in various applications for specially-abled and, more specifically, visually abled persons. With advancements in technology for object detection and natural processing, there has been an instant surge infusing the above mainstream tasks. One such example of this fusion resulted in the generation of Image captions when an input image is fed to the system, and it gives a short description of what is present in the image. This fusion pertained to images and was further moved to be implemented on the Videos, with some tweaking in the current methods. This paper presents the survey of the state of art techniques of various video captioning methods. There have been many inputs provided by people worldwide in this domain; thus, there was a need to compile, study and analyze all the results and present that in a comprehensive study, which we have done in this paper. The comparison of various video captioning methods on the distinct dataset was evaluated on different parameters, which were most common and mainly used for image and video analysis. This review was done for methods used from the year 2015–2019 (year by year). The most commonly used dataset and evaluation method are also pictorially represented in a bar graph and scatter plot for each year for the respective evaluation parameter. Though a lot of analysis and research has been done on video captioning, our survey shows many problems.},
  langid = {english},
  keywords = {CNN,Encoder-decoder framework,Natural language processing,RNN,Video captioning},
  file = {Y:\paper\2023_PBL\Jain et al_2022_Video captioning.pdf}
}

@online{jangModelStockAll2024,
  title = {Model {{Stock}}: {{All}} We Need Is Just a Few Fine-Tuned Models},
  shorttitle = {Model {{Stock}}},
  author = {Jang, Dong-Hwan and Yun, Sangdoo and Han, Dongyoon},
  date = {2024-03-28},
  eprint = {2403.19522},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2403.19522},
  urldate = {2024-10-07},
  abstract = {This paper introduces an efficient fine-tuning method for large pre-trained models, offering strong in-distribution (ID) and out-ofdistribution (OOD) performance. Breaking away from traditional practices that need a multitude of fine-tuned models for averaging, our approach employs significantly fewer models to achieve final weights yet yield superior accuracy. Drawing from key insights in the weight space of fine-tuned weights, we uncover a strong link between the performance and proximity to the center of weight space. Based on this, we introduce a method that approximates a center-close weight using only two finetuned models, applicable during or after training. Our innovative layerwise weight averaging technique surpasses state-of-the-art model methods such as Model Soup, utilizing only two fine-tuned models. This strategy can be aptly coined Model Stock, highlighting its reliance on selecting a minimal number of models to draw a more optimized-averaged model. We demonstrate the efficacy of Model Stock with fine-tuned models based upon pre-trained CLIP architectures, achieving remarkable performance on both ID and OOD tasks on the standard benchmarks, all while barely bringing extra computational demands. Our code and pre-trained models are available at https://github.com/naver-ai/model-stock.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\EGP7Y92E\Jang 등 - 2024 - Model Stock All we need is just a few fine-tuned .pdf}
}

@online{jelassiVisionTransformersProvably2022,
  title = {Vision {{Transformers}} Provably Learn Spatial Structure},
  author = {Jelassi, Samy and Sander, Michael E. and Li, Yuanzhi},
  date = {2022-10-13},
  eprint = {2210.09221},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2210.09221},
  urldate = {2023-07-17},
  abstract = {Vision Transformers (ViTs) have achieved comparable or superior performance than Convolutional Neural Networks (CNNs) in computer vision. This empirical breakthrough is even more remarkable since, in contrast to CNNs, ViTs do not embed any visual inductive bias of spatial locality. Yet, recent works have shown that while minimizing their training loss, ViTs specifically learn spatially localized patterns. This raises a central question: how do ViTs learn these patterns by solely minimizing their training loss using gradient-based methods from random initialization? In this paper, we provide some theoretical justification of this phenomenon. We propose a spatially structured dataset and a simplified ViT model. In this model, the attention matrix solely depends on the positional encodings. We call this mechanism the positional attention mechanism. On the theoretical side, we consider a binary classification task and show that while the learning problem admits multiple solutions that generalize, our model implicitly learns the spatial structure of the dataset while generalizing: we call this phenomenon patch association. We prove that patch association helps to sample-efficiently transfer to downstream datasets that share the same structure as the pre-training one but differ in the features. Lastly, we empirically verify that a ViT with positional attention performs similarly to the original one on CIFAR-10/100, SVHN and ImageNet.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2022 winter intern\\Jelassi et al_2022_Vision Transformers provably learn spatial structure.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4FMGLHHM\\2210.html}
}

@inproceedings{jeonFlutteringPatternGeneration2013,
  title = {Fluttering {{Pattern Generation Using Modified Legendre Sequence}} for {{Coded Exposure Imaging}}},
  booktitle = {2013 {{IEEE International Conference}} on {{Computer Vision}}},
  author = {Jeon, Hae-Gon and Lee, Joon-Young and Han, Yudeog and Kim, Seon Joo and Kweon, In So},
  date = {2013-02},
  pages = {1001--1008},
  issn = {2380-7504},
  doi = {10.1109/ICCV.2013.128},
  abstract = {Finding a good binary sequence is critical in determining the performance of the coded exposure imaging, but previous methods mostly rely on a random search for finding the binary codes, which could easily fail to find good long sequences due to the exponentially growing search space. In this paper, we present a new computationally efficient algorithm for generating the binary sequence, which is especially well suited for longer sequences. We show that the concept of the low autocorrelation binary sequence that has been well exploited in the information theory community can be applied for generating the fluttering patterns of the shutter, propose a new measure of a good binary sequence, and present a new algorithm by modifying the Legendre sequence for the coded exposure imaging. Experiments using both synthetic and real data show that our new algorithm consistently generates better binary sequences for the coded exposure problem, yielding better deblurring and resolution enhancement results compared to the previous methods for generating the binary codes.},
  eventtitle = {2013 {{IEEE International Conference}} on {{Computer Vision}}},
  keywords = {Binary codes,Cameras,Coded Exposure,Computational Photography,Computer vision,Correlation,Deblurring,Deconvolution,Noise},
  file = {Y\:\\paper\\2022 winter intern\\Jeon et al_2013_Fluttering Pattern Generation Using Modified Legendre Sequence for Coded.pdf;C\:\\Users\\chsey\\Zotero\\storage\\T59ZH96Q\\stamp.html}
}

@inproceedings{jeongOODMAMLMetaLearningFewShot2020,
  title = {{{OOD-MAML}}: {{Meta-Learning}} for {{Few-Shot Out-of-Distribution Detection}} and {{Classification}}},
  shorttitle = {{{OOD-MAML}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Jeong, Taewon and Kim, Heeyoung},
  date = {2020},
  volume = {33},
  pages = {3907--3916},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2020/hash/28e209b61a52482a0ae1cb9f5959c792-Abstract.html},
  urldate = {2022-12-20},
  abstract = {We propose a few-shot learning method for detecting out-of-distribution (OOD) samples from classes that are unseen during training while classifying samples from seen classes using only a few labeled examples. For detecting unseen classes while generalizing to new samples of known classes, we synthesize fake samples, i.e., OOD samples, but that resemble in-distribution samples, and use them along with real samples. Our approach is based on an extension of model-agnostic meta learning (MAML) and is denoted as OOD-MAML, which not only learns a model initialization but also the initial fake samples across tasks. The learned initial fake samples can be used to quickly adapt to new tasks to form task-specific fake samples with only one or a few gradient update steps using MAML. For testing, OOD-MAML converts a K-shot N-way classification task into N sub-tasks of K-shot OOD detection with respect to each class. The joint analysis of N sub-tasks facilitates simultaneous classification and OOD detection and, furthermore, offers an advantage, in that it does not require re-training when the number of classes for a test task differs from that for training tasks; it is sufficient to simply assume as many sub-tasks as the number of classes for the test task. We also demonstrate the effective performance of OOD-MAML over benchmark datasets.},
  file = {Y:\paper\2022 autumn intern\OOD\Jeong_Kim_2020_OOD-MAML.pdf}
}

@online{jiaEgoTaskQAUnderstandingHuman2022,
  title = {{{EgoTaskQA}}: {{Understanding Human Tasks}} in {{Egocentric Videos}}},
  shorttitle = {{{EgoTaskQA}}},
  author = {Jia, Baoxiong and Lei, Ting and Zhu, Song-Chun and Huang, Siyuan},
  date = {2022-10-08},
  eprint = {2210.03929},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2210.03929},
  url = {http://arxiv.org/abs/2210.03929},
  urldate = {2023-05-23},
  abstract = {Understanding human tasks through video observations is an essential capability of intelligent agents. The challenges of such capability lie in the difficulty of generating a detailed understanding of situated actions, their effects on object states (i.e., state changes), and their causal dependencies. These challenges are further aggravated by the natural parallelism from multi-tasking and partial observations in multi-agent collaboration. Most prior works leverage action localization or future prediction as an indirect metric for evaluating such task understanding from videos. To make a direct evaluation, we introduce the EgoTaskQA benchmark that provides a single home for the crucial dimensions of task understanding through question-answering on real-world egocentric videos. We meticulously design questions that target the understanding of (1) action dependencies and effects, (2) intents and goals, and (3) agents' beliefs about others. These questions are divided into four types, including descriptive (what status?), predictive (what will?), explanatory (what caused?), and counterfactual (what if?) to provide diagnostic analyses on spatial, temporal, and causal understandings of goal-oriented tasks. We evaluate state-of-the-art video reasoning models on our benchmark and show their significant gaps between humans in understanding complex goal-oriented egocentric videos. We hope this effort will drive the vision community to move onward with goal-oriented video understanding and reasoning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\Jia et al_2022_EgoTaskQA.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XFWNE8IH\\2210.html}
}

@online{jiangHowDoesAdaptive2022,
  title = {How {{Does Adaptive Optimization Impact Local Neural Network Geometry}}?},
  author = {Jiang, Kaiqi and Malik, Dhruv and Li, Yuanzhi},
  date = {2022-11-04},
  eprint = {2211.02254},
  eprinttype = {arXiv},
  eprintclass = {cs, math, stat},
  doi = {10.48550/arXiv.2211.02254},
  url = {http://arxiv.org/abs/2211.02254},
  urldate = {2024-06-01},
  abstract = {Adaptive optimization methods are well known to achieve superior convergence relative to vanilla gradient methods. The traditional viewpoint in optimization, particularly in convex optimization, explains this improved performance by arguing that, unlike vanilla gradient schemes, adaptive algorithms mimic the behavior of a second-order method by adapting to the global geometry of the loss function. We argue that in the context of neural network optimization, this traditional viewpoint is insufficient. Instead, we advocate for a local trajectory analysis. For iterate trajectories produced by running a generic optimization algorithm OPT, we introduce \$R\textasciicircum\{\textbackslash text\{OPT\}\}\_\{\textbackslash text\{med\}\}\$, a statistic that is analogous to the condition number of the loss Hessian evaluated at the iterates. Through extensive experiments, we show that adaptive methods such as Adam bias the trajectories towards regions where \$R\textasciicircum\{\textbackslash text\{Adam\}\}\_\{\textbackslash text\{med\}\}\$ is small, where one might expect faster convergence. By contrast, vanilla gradient methods like SGD bias the trajectories towards regions where \$R\textasciicircum\{\textbackslash text\{SGD\}\}\_\{\textbackslash text\{med\}\}\$ is comparatively large. We complement these empirical observations with a theoretical result that provably demonstrates this phenomenon in the simplified setting of a two-layer linear network. We view our findings as evidence for the need of a new explanation of the success of adaptive methods, one that is different than the conventional wisdom.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Mathematics - Optimization and Control,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_lecture\\Jiang et al_2022_How Does Adaptive Optimization Impact Local Neural Network Geometry.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3MPNK9X2\\2211.html}
}

@inproceedings{jiangLowResourceTextClassification2023,
  title = {“{{Low-Resource}}” {{Text Classification}}: {{A Parameter-Free Classification Method}} with {{Compressors}}},
  shorttitle = {“{{Low-Resource}}” {{Text Classification}}},
  booktitle = {Findings of the {{Association}} for {{Computational Linguistics}}: {{ACL}} 2023},
  author = {Jiang, Zhiying and Yang, Matthew and Tsirlin, Mikhail and Tang, Raphael and Dai, Yiqin and Lin, Jimmy},
  editor = {Rogers, Anna and Boyd-Graber, Jordan and Okazaki, Naoaki},
  date = {2023-07},
  pages = {6810--6828},
  publisher = {Association for Computational Linguistics},
  location = {Toronto, Canada},
  doi = {10.18653/v1/2023.findings-acl.426},
  url = {https://aclanthology.org/2023.findings-acl.426},
  urldate = {2024-04-22},
  abstract = {Deep neural networks (DNNs) are often used for text classification due to their high accuracy. However, DNNs can be computationally intensive, requiring millions of parameters and large amounts of labeled data, which can make them expensive to use, to optimize, and to transfer to out-of-distribution (OOD) cases in practice. In this paper, we propose a non-parametric alternative to DNNs that's easy, lightweight, and universal in text classification: a combination of a simple compressor like gzip with a k-nearest-neighbor classifier. Without any training parameters, our method achieves results that are competitive with non-pretrained deep learning methods on six in-distribution datasets.It even outperforms BERT on all five OOD datasets, including four low-resource languages. Our method also excels in the few-shot setting, where labeled data are too scarce to train DNNs effectively.},
  eventtitle = {Findings 2023},
  keywords = {notion},
  file = {Y:\paper\2024_research\Jiang et al_2023_“Low-Resource” Text Classification.pdf}
}

@article{jiangSingleImageSuperResolution2017,
  title = {Single {{Image Super-Resolution}} via {{Locally Regularized Anchored Neighborhood Regression}} and {{Nonlocal Means}}},
  author = {Jiang, Junjun and Ma, Xiang and Chen, Chen and Lu, Tao and Wang, Zhongyuan and Ma, Jiayi},
  date = {2017-01},
  journaltitle = {IEEE Transactions on Multimedia},
  volume = {19},
  number = {1},
  pages = {15--26},
  issn = {1941-0077},
  doi = {10.1109/TMM.2016.2599145},
  abstract = {The goal of learning-based image super resolution (SR) is to generate a plausible and visually pleasing high-resolution (HR) image from a given low-resolution (LR) input. The SR problem is severely underconstrained, and it has to rely on examples or some strong image priors to reconstruct the missing HR image details. This paper addresses the problem of learning the mapping functions (i.e., projection matrices) between the LR and HR images based on a dictionary of LR and HR examples. Encouraged by recent developments in image prior modeling, where the state-of-the-art algorithms are formed with nonlocal self-similarity and local geometry priors, we seek an SR algorithm of similar nature that will incorporate these two priors into the learning from LR space to HR space. The nonlocal self-similarity prior takes advantage of the redundancy of similar patches in natural images, while the local geometry prior of the data space can be used to regularize the modeling of the nonlinear relationship between LR and HR spaces. Based on the above two considerations, we first apply the local geometry prior to regularize the patch representation, and then utilize the nonlocal means filter to improve the super-resolved outcome. Experimental results verify the effectiveness of the proposed algorithm compared with the state-of-the-art SR methods.},
  eventtitle = {{{IEEE Transactions}} on {{Multimedia}}},
  keywords = {Anchored neighborhood regression,Dictionaries,Electronic mail,Geometry,Image coding,Image reconstruction,Image resolution,locality geometry,neighbor embedding,nonlocal means,super-resolution (SR),Training},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Jiang et al_2017_Single Image Super-Resolution via Locally Regularized Anchored Neighborhood.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UGUSA23T\\7539698.html}
}

@online{jiaScalingVisualVisionLanguage2021,
  title = {Scaling {{Up Visual}} and {{Vision-Language Representation Learning With Noisy Text Supervision}}},
  author = {Jia, Chao and Yang, Yinfei and Xia, Ye and Chen, Yi-Ting and Parekh, Zarana and Pham, Hieu and Le, Quoc V. and Sung, Yunhsuan and Li, Zhen and Duerig, Tom},
  date = {2021-06-11},
  eprint = {2102.05918},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2102.05918},
  url = {http://arxiv.org/abs/2102.05918},
  urldate = {2024-03-21},
  abstract = {Pre-trained representations are becoming crucial for many NLP and perception tasks. While representation learning in NLP has transitioned to training on raw text without human annotations, visual and vision-language representations still rely heavily on curated training datasets that are expensive or require expert knowledge. For vision applications, representations are mostly learned using datasets with explicit class labels such as ImageNet or OpenImages. For vision-language, popular datasets like Conceptual Captions, MSCOCO, or CLIP all involve a non-trivial data collection (and cleaning) process. This costly curation process limits the size of datasets and hence hinders the scaling of trained models. In this paper, we leverage a noisy dataset of over one billion image alt-text pairs, obtained without expensive filtering or post-processing steps in the Conceptual Captions dataset. A simple dual-encoder architecture learns to align visual and language representations of the image and text pairs using a contrastive loss. We show that the scale of our corpus can make up for its noise and leads to state-of-the-art representations even with such a simple learning scheme. Our visual representation achieves strong performance when transferred to classification tasks such as ImageNet and VTAB. The aligned visual and language representations enables zero-shot image classification and also set new state-of-the-art results on Flickr30K and MSCOCO image-text retrieval benchmarks, even when compared with more sophisticated cross-attention models. The representations also enable cross-modality search with complex text and text + image queries.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Jia et al_2021_Scaling Up Visual and Vision-Language Representation Learning With Noisy Text.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AUFMDKFH\\2102.html}
}

@online{jiaVisualPromptTuning2022,
  title = {Visual {{Prompt Tuning}}},
  author = {Jia, Menglin and Tang, Luming and Chen, Bor-Chun and Cardie, Claire and Belongie, Serge and Hariharan, Bharath and Lim, Ser-Nam},
  date = {2022-07-20},
  eprint = {2203.12119},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.12119},
  url = {http://arxiv.org/abs/2203.12119},
  urldate = {2023-06-29},
  abstract = {The current modus operandi in adapting pre-trained models involves updating all the backbone parameters, ie, full fine-tuning. This paper introduces Visual Prompt Tuning (VPT) as an efficient and effective alternative to full fine-tuning for large-scale Transformer models in vision. Taking inspiration from recent advances in efficiently tuning large language models, VPT introduces only a small amount (less than 1\% of model parameters) of trainable parameters in the input space while keeping the model backbone frozen. Via extensive experiments on a wide variety of downstream recognition tasks, we show that VPT achieves significant performance gains compared to other parameter efficient tuning protocols. Most importantly, VPT even outperforms full fine-tuning in many cases across model capacities and training data scales, while reducing per-task storage cost.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Jia et al_2022_Visual Prompt Tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XY4NC66F\\2203.html}
}

@video{jimkuroseEmail2022,
  entrysubtype = {video},
  title = {2.3 {{Email}}},
  editor = {{JimKurose}},
  editortype = {director},
  date = {2022},
  url = {https://www.youtube.com/watch?v=D3GMrOMR2dk},
  urldate = {2022-09-21}
}

@video{jimkuroseNetworkEdge2022,
  entrysubtype = {video},
  title = {1.2 {{The}} Network Edge},
  editor = {{JimKurose}},
  editortype = {director},
  date = {2022},
  url = {https://www.youtube.com/watch?v=k8NmM-hImBU},
  urldate = {2022-10-20},
  file = {C:\Users\jiho\OneDrive - GIST\바탕 화면\research_archive\research_paper\1.2-the-network-edge-zotero.md}
}

@online{jinDatalessKnowledgeFusion2023,
  title = {Dataless {{Knowledge Fusion}} by {{Merging Weights}} of {{Language Models}}},
  author = {Jin, Xisen and Ren, Xiang and Preotiuc-Pietro, Daniel and Cheng, Pengxiang},
  date = {2023-10-12},
  eprint = {2212.09849},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2212.09849},
  urldate = {2024-09-23},
  abstract = {Fine-tuning pre-trained language models has become the prevalent paradigm for building downstream NLP models. Oftentimes fine-tuned models are readily available but their training data is not, due to data privacy or intellectual property concerns. This creates a barrier to fusing knowledge across individual models to yield a better single model. In this paper, we study the problem of merging individual models built on different training data sets to obtain a single model that performs well both across all data set domains and can generalize on out-of-domain data. We propose a dataless knowledge fusion method that merges models in their parameter space, guided by weights that minimize prediction differences between the merged model and the individual models. Over a battery of evaluation settings, we show that the proposed method significantly outperforms baselines such as Fisher-weighted averaging or model ensembling. Further, we find that our method is a promising alternative to multi-task learning that can preserve or sometimes improve over the individual models without access to the training data. Finally, model merging is more efficient than training a multi-task model, thus making it applicable to a wider set of scenarios.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\STJZC5KM\Jin 등 - 2023 - Dataless Knowledge Fusion by Merging Weights of La.pdf}
}

@online{jinLargeLanguageModels2024,
  title = {Large {{Language Models}} on {{Graphs}}: {{A Comprehensive Survey}}},
  shorttitle = {Large {{Language Models}} on {{Graphs}}},
  author = {Jin, Bowen and Liu, Gang and Han, Chi and Jiang, Meng and Ji, Heng and Han, Jiawei},
  date = {2024-02-01},
  eprint = {2312.02783},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2312.02783},
  urldate = {2024-08-18},
  abstract = {Large language models (LLMs), such as GPT4 and LLaMA, are creating significant advancements in natural language processing, due to their strong text encoding/decoding ability and newly found emergent capability (e.g., reasoning). While LLMs are mainly designed to process pure texts, there are many real-world scenarios where text data is associated with rich structure information in the form of graphs (e.g., academic networks, and e-commerce networks) or scenarios where graph data are paired with rich textual information (e.g., molecules with descriptions). Besides, although LLMs have shown their pure textbased reasoning ability, it is underexplored whether such ability can be generalized to graphs (i.e., graph-based reasoning). In this paper, we provide a systematic review of scenarios and techniques related to large language models on graphs. We first summarize potential scenarios of adopting LLMs on graphs into three categories, namely pure graphs, text-attributed graphs, and text-paired graphs. We then discuss detailed techniques for utilizing LLMs on graphs, including LLM as Predictor, LLM as Encoder, and LLM as Aligner, and compare the advantages and disadvantages of different schools of models. Furthermore, we discuss the real-world applications of such methods and summarize open-source codes and benchmark datasets. Finally, we conclude with potential future research directions in this fast-growing field. The related source can be found at https://github.com/PeterGriffinJin/ Awesome-Language-Model-on-Graphs.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\BFIP37UG\Jin 등 - 2024 - Large Language Models on Graphs A Comprehensive S.pdf}
}

@inproceedings{johnsonDenseCapFullyConvolutional2016,
  title = {{{DenseCap}}: {{Fully Convolutional Localization Networks}} for {{Dense Captioning}}},
  shorttitle = {{{DenseCap}}},
  author = {Johnson, Justin and Karpathy, Andrej and Fei-Fei, Li},
  date = {2016},
  pages = {4565--4574},
  url = {https://openaccess.thecvf.com/content_cvpr_2016/html/Johnson_DenseCap_Fully_Convolutional_CVPR_2016_paper.html},
  urldate = {2023-05-29},
  eventtitle = {Proceedings of the {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\dense captioning\Johnson et al_2016_DenseCap.pdf}
}

@online{joudetDeepLearningObject2018,
  title = {Deep Learning Object Detection on Dental X-Rays},
  author = {Joudet, Clement},
  date = {2018-09-06T08:38:12},
  url = {https://medium.com/@clemkoa/deep-learning-object-detection-on-dental-x-rays-8211e48e520b},
  urldate = {2022-07-09},
  abstract = {As the interest in AI and deep learning keeps growing, we see more and more practical applications, especially in healthcare where…},
  langid = {english},
  organization = {Medium},
  file = {C:\Users\chsey\Zotero\storage\NBIJNDVY\deep-learning-object-detection-on-dental-x-rays-8211e48e520b.html}
}

@online{joulinLearningVisualFeatures2015,
  title = {Learning {{Visual Features}} from {{Large Weakly Supervised Data}}},
  author = {Joulin, Armand and family=Maaten, given=Laurens, prefix=van der, useprefix=true and Jabri, Allan and Vasilache, Nicolas},
  date = {2015-11-06},
  eprint = {1511.02251},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1511.02251},
  urldate = {2023-06-29},
  abstract = {Convolutional networks trained on large supervised dataset produce visual features which form the basis for the state-of-the-art in many computer-vision problems. Further improvements of these visual features will likely require even larger manually labeled data sets, which severely limits the pace at which progress can be made. In this paper, we explore the potential of leveraging massive, weakly-labeled image collections for learning good visual features. We train convolutional networks on a dataset of 100 million Flickr photos and captions, and show that these networks produce features that perform well in a range of vision problems. We also show that the networks appropriately capture word similarity, and learn correspondences between different languages.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Joulin et al_2015_Learning Visual Features from Large Weakly Supervised Data.pdf;C\:\\Users\\chsey\\Zotero\\storage\\N7PQFKPE\\1511.html}
}

@article{jungGeneratingInstancelevelPrompts,
  title = {Generating {{Instance-level Prompts}} for {{Rehearsal-free Continual Learning}}},
  author = {Jung, Dahuin and Han, Dongyoon and Bang, Jihwan and Song, Hwanjun},
  abstract = {We introduce Domain-Adaptive Prompt (DAP), a novel method for continual learning using Vision Transformers (ViT). Prompt-based continual learning has recently gained attention due to its rehearsal-free nature. Currently, the prompt pool, which is suggested by prompt-based continual learning, is key to effectively exploiting the frozen pretrained ViT backbone in a sequence of tasks. However, we observe that the use of a prompt pool creates a domain scalability problem between pre-training and continual learning. This problem arises due to the inherent encoding of group-level instructions within the prompt pool. To address this problem, we propose DAP, a pool-free approach that generates a suitable prompt in an instance-level manner at inference time. We optimize an adaptive prompt generator that creates instance-specific fine-grained instructions required for each input, enabling enhanced model plasticity and reduced forgetting. Our experiments on seven datasets with varying degrees of domain similarity to ImageNet demonstrate the superiority of DAP over state-ofthe-art prompt-based methods. Code is publicly available at https://github.com/naver-ai/dap-cl.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\GGRWS9BP\Jung 등 - Generating Instance-level Prompts for Rehearsal-fr.pdf}
}

@inproceedings{kajiyaRenderingEquation1986,
  title = {The Rendering Equation},
  booktitle = {Proceedings of the 13th Annual Conference on {{Computer}} Graphics and Interactive Techniques  - {{SIGGRAPH}} '86},
  author = {Kajiya, James T.},
  date = {1986},
  pages = {143--150},
  publisher = {ACM Press},
  location = {Not Known},
  doi = {10.1145/15922.15902},
  url = {http://portal.acm.org/citation.cfm?doid=15922.15902},
  urldate = {2023-04-11},
  eventtitle = {The 13th Annual Conference},
  isbn = {978-0-89791-196-2},
  langid = {english},
  file = {Y:\paper\2022 winter intern\Kajiya_1986_The rendering equation.pdf}
}

@online{Kakaogyejeong,
  title = {카카오계정},
  url = {https://accounts.kakao.com/login/?continue=https%3A%2F%2Fmy.kakao.com%2Fproduct%2FEMOTICON001#login},
  urldate = {2023-11-17},
  langid = {korean-han},
  file = {C:\Users\chsey\Zotero\storage\PYEQPCQQ\login.html}
}

@online{Kakaogyejeonga,
  title = {카카오계정},
  url = {https://accounts.kakao.com/login/?continue=https%3A%2F%2Fmy.kakao.com%2Fproduct%2FEMOTICON001#login},
  urldate = {2023-11-13},
  langid = {korean-han},
  file = {C:\Users\chsey\Zotero\storage\PJSEF4XS\login.html}
}

@inproceedings{kalraDeepPolarizationCues2020,
  title = {Deep {{Polarization Cues}} for {{Transparent Object Segmentation}}},
  booktitle = {2020 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Kalra, Agastya and Taamazyan, Vage and Rao, Supreeth Krishna and Venkataraman, Kartik and Raskar, Ramesh and Kadambi, Achuta},
  date = {2020-06},
  pages = {8599--8608},
  issn = {2575-7075},
  doi = {10.1109/CVPR42600.2020.00863},
  abstract = {Segmentation of transparent objects is a hard, open problem in computer vision. Transparent objects lack texture of their own, adopting instead the texture of scene background. This paper reframes the problem of transparent object segmentation into the realm of light polarization, i.e., the rotation of light waves. We use a polarization camera to capture multi-modal imagery and couple this with a unique deep learning backbone for processing polarization input data. Our method achieves instance segmentation on cluttered, transparent objects in various scene and background conditions, demonstrating an improvement over traditional image-based approaches. As an application we use this for robotic bin picking of transparent objects.},
  eventtitle = {2020 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  keywords = {Image edge detection,Image segmentation,Machine learning,Mathematical model,Object segmentation,Robustness,Tensile stress},
  file = {Y\:\\paper\\2022 winter intern\\transparent_segmentation\\Kalra et al_2020_Deep Polarization Cues for Transparent Object Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PFTMCFT7\\stamp.html}
}

@article{kangLearningWhomShare,
  title = {Learning with {{Whom}} to {{Share}} in {{Multi-task Feature Learning}}},
  author = {Kang, Zhuoliang and Grauman, Kristen and Sha, Fei},
  abstract = {In multi-task learning (MTL), multiple tasks are learnt jointly. A major assumption for this paradigm is that all those tasks are indeed related so that the joint training is appropriate and beneficial. In this paper, we study the problem of multi-task learning of shared feature representations among tasks, while simultaneously determining “with whom” each task should share. We formulate the problem as a mixed integer programming and provide an alternating minimization technique to solve the optimization problem of jointly identifying grouping structures and parameters. The algorithm monotonically decreases the objective function and converges to a local optimum. Compared to the standard MTL paradigm where all tasks are in a single group, our algorithm improves its performance with statistical significance for three out of the four datasets we have studied. We also demonstrate its advantage over other task grouping techniques investigated in literature.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\MW6ZWMLJ\Kang 등 - Learning with Whom to Share in Multi-task Feature .pdf}
}

@inproceedings{kanKnowledgeAwarePromptTuning2023,
  title = {Knowledge-{{Aware Prompt Tuning}} for {{Generalizable Vision-Language Models}}},
  author = {Kan, Baoshuo and Wang, Teng and Lu, Wenpeng and Zhen, Xiantong and Guan, Weili and Zheng, Feng},
  date = {2023},
  pages = {15670--15680},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Kan_Knowledge-Aware_Prompt_Tuning_for_Generalizable_Vision-Language_Models_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Kan et al_2023_Knowledge-Aware Prompt Tuning for Generalizable Vision-Language Models.pdf}
}

@online{karrasStyleBasedGeneratorArchitecture2019,
  title = {A {{Style-Based Generator Architecture}} for {{Generative Adversarial Networks}}},
  author = {Karras, Tero and Laine, Samuli and Aila, Timo},
  date = {2019-03-29},
  eprint = {1812.04948},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1812.04948},
  url = {http://arxiv.org/abs/1812.04948},
  urldate = {2023-08-05},
  abstract = {We propose an alternative generator architecture for generative adversarial networks, borrowing from style transfer literature. The new architecture leads to an automatically learned, unsupervised separation of high-level attributes (e.g., pose and identity when trained on human faces) and stochastic variation in the generated images (e.g., freckles, hair), and it enables intuitive, scale-specific control of the synthesis. The new generator improves the state-of-the-art in terms of traditional distribution quality metrics, leads to demonstrably better interpolation properties, and also better disentangles the latent factors of variation. To quantify interpolation quality and disentanglement, we propose two new, automated methods that are applicable to any generator architecture. Finally, we introduce a new, highly varied and high-quality dataset of human faces.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\generative model\\Karras et al_2019_A Style-Based Generator Architecture for Generative Adversarial Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VGE85478\\1812.html}
}

@book{kauffmanOriginsOrderSelforganization1993,
  title = {The {{Origins}} of {{Order}}: {{Self-organization}} and {{Selection}} in {{Evolution}}},
  shorttitle = {The {{Origins}} of {{Order}}},
  author = {Kauffman, Stuart A.},
  date = {1993},
  eprint = {lZcSpRJz0dgC},
  eprinttype = {googlebooks},
  publisher = {Oxford University Press},
  abstract = {Stuart Kauffman here presents a brilliant new paradigm for evolutionary biology, one that extends the basic concepts of Darwinian evolution to accommodate recent findings and perspectives from the fields of biology, physics, chemistry and mathematics. The book drives to the heart of the exciting debate on the origins of life and maintenance of order in complex biological systems. It focuses on the concept of self-organization: the spontaneous emergence of order that is widely observed throughout nature Kauffman argues that self-organization plays an important role in the Darwinian process of natural selection. Yet until now no systematic effort has been made to incorporate the concept of self-organization into evolutionary theory. The construction requirements which permit complex systems to adapt are poorly understood, as is the extent to which selection itself can yield systems able to adapt more successfully. This book explores these themes. It shows how complex systems, contrary to expectations, can spontaneously exhibit stunning degrees of order, and how this order, in turn, is essential for understanding the emergence and development of life on Earth. Topics include the new biotechnology of applied molecular evolution, with its important implications for developing new drugs and vaccines; the balance between order and chaos observed in many naturally occurring systems; new insights concerning the predictive power of statistical mechanics in biology; and other major issues. Indeed, the approaches investigated here may prove to be the new center around which biological science itself will evolve. The work is written for all those interested in the cutting edge of research in the life sciences.},
  isbn = {978-0-19-507951-7},
  langid = {english},
  pagetotal = {744},
  keywords = {Medical / Oncology / General,Science / Life Sciences / Ecology,Science / Life Sciences / Evolution}
}

@online{kauflinAmericaTop50,
  title = {America's {{Top}} 50 {{Companies}} 1917-2017},
  author = {Kauflin, Jeff},
  url = {https://www.forbes.com/sites/jeffkauflin/2017/09/19/americas-top-50-companies-1917-2017/},
  urldate = {2023-12-17},
  abstract = {It's impossible to read this ranking of the nation's largest firms over the past century without a sense of awe. The U.S. economy regularly creates new business behemoths, then ruthlessly strikes them down. In the wake of this creative destruction come new jobs, wealth, industries and innovation.},
  langid = {english},
  organization = {Forbes},
  file = {C:\Users\chsey\Zotero\storage\XBPL3LUP\americas-top-50-companies-1917-2017.html}
}

@article{kautzApproximationGlossyReflection,
  title = {Approximation of {{Glossy Reﬂection}} with {{Preﬁltered Environment Maps}}},
  author = {Kautz, Jan and McCool, Michael D},
  abstract = {A method is presented that can render glossy reflections with arbitrary isotropic bidirectional reflectance distribution functions (BRDFs) at interactive rates using texture mapping. This method is based on the well-known environment map technique for specular reflections.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\PKAXW2LP\Kautz 그리고 McCool - Approximation of Glossy Reﬂection with Preﬁltered .pdf}
}

@article{kellyPrincipalPortfolios2023,
  title = {Principal {{Portfolios}}},
  author = {Kelly, Bryan and Malamud, Semyon and Pedersen, Lasse Heje},
  date = {2023},
  journaltitle = {The Journal of Finance},
  volume = {78},
  number = {1},
  pages = {347--387},
  issn = {1540-6261},
  doi = {10.1111/jofi.13199},
  url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/jofi.13199},
  urldate = {2024-09-11},
  abstract = {We propose a new asset pricing framework in which all securities' signals predict each individual return. While the literature focuses on securities' own-signal predictability, assuming equal strength across securities, our framework includes cross-predictability—leading to three main results. First, we derive the optimal strategy in closed form. It consists of eigenvectors of a “prediction matrix,” which we call “principal portfolios.” Second, we decompose the problem into alpha and beta, yielding optimal strategies with, respectively, zero and positive factor exposure. Third, we provide a new test of asset pricing models. Empirically, principal portfolios deliver significant out-of-sample alphas to standard factors in several data sets.},
  langid = {english},
  keywords = {notion},
  file = {Y\:\\paper\\2024_lecture\\Kelly et al_2023_Principal Portfolios.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3ME2ZFJD\\jofi.html}
}

@online{kendallEndtoEndLearningGeometry2017,
  title = {End-to-{{End Learning}} of {{Geometry}} and {{Context}} for {{Deep Stereo Regression}}},
  author = {Kendall, Alex and Martirosyan, Hayk and Dasgupta, Saumitro and Henry, Peter and Kennedy, Ryan and Bachrach, Abraham and Bry, Adam},
  date = {2017-03-13},
  eprint = {1703.04309},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1703.04309},
  url = {http://arxiv.org/abs/1703.04309},
  urldate = {2023-08-05},
  abstract = {We propose a novel deep learning architecture for regressing disparity from a rectified pair of stereo images. We leverage knowledge of the problem's geometry to form a cost volume using deep feature representations. We learn to incorporate contextual information using 3-D convolutions over this volume. Disparity values are regressed from the cost volume using a proposed differentiable soft argmin operation, which allows us to train our method end-to-end to sub-pixel accuracy without any additional post-processing or regularization. We evaluate our method on the Scene Flow and KITTI datasets and on KITTI we set a new state-of-the-art benchmark, while being significantly faster than competing approaches.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Neural and Evolutionary Computing,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\2.5d image understanding\\Kendall et al_2017_End-to-End Learning of Geometry and Context for Deep Stereo Regression.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DL2B7RXR\\1703.html}
}

@online{khattakMaPLeMultimodalPrompt2023,
  title = {{{MaPLe}}: {{Multi-modal Prompt Learning}}},
  shorttitle = {{{MaPLe}}},
  author = {Khattak, Muhammad Uzair and Rasheed, Hanoona and Maaz, Muhammad and Khan, Salman and Khan, Fahad Shahbaz},
  date = {2023-04-01},
  eprint = {2210.03117},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2210.03117},
  url = {http://arxiv.org/abs/2210.03117},
  urldate = {2023-06-27},
  abstract = {Pre-trained vision-language (V-L) models such as CLIP have shown excellent generalization ability to downstream tasks. However, they are sensitive to the choice of input text prompts and require careful selection of prompt templates to perform well. Inspired by the Natural Language Processing (NLP) literature, recent CLIP adaptation approaches learn prompts as the textual inputs to fine-tune CLIP for downstream tasks. We note that using prompting to adapt representations in a single branch of CLIP (language or vision) is sub-optimal since it does not allow the flexibility to dynamically adjust both representation spaces on a downstream task. In this work, we propose Multi-modal Prompt Learning (MaPLe) for both vision and language branches to improve alignment between the vision and language representations. Our design promotes strong coupling between the vision-language prompts to ensure mutual synergy and discourages learning independent uni-modal solutions. Further, we learn separate prompts across different early stages to progressively model the stage-wise feature relationships to allow rich context learning. We evaluate the effectiveness of our approach on three representative tasks of generalization to novel classes, new target datasets and unseen domain shifts. Compared with the state-of-the-art method Co-CoOp, MaPLe exhibits favorable performance and achieves an absolute gain of 3.45\% on novel classes and 2.72\% on overall harmonic-mean, averaged over 11 diverse image recognition datasets. Our code and pre-trained models are available at https://github.com/muzairkhattak/multimodal-prompt-learning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Khattak et al_2023_MaPLe2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5A3XSF5J\\2210.html}
}

@online{khattakSelfregulatingPromptsFoundational2023,
  title = {Self-Regulating {{Prompts}}: {{Foundational Model Adaptation}} without {{Forgetting}}},
  shorttitle = {Self-Regulating {{Prompts}}},
  author = {Khattak, Muhammad Uzair and Wasim, Syed Talal and Naseer, Muzammal and Khan, Salman and Yang, Ming-Hsuan and Khan, Fahad Shahbaz},
  date = {2023-08-24},
  eprint = {2307.06948},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2307.06948},
  url = {http://arxiv.org/abs/2307.06948},
  urldate = {2023-10-15},
  abstract = {Prompt learning has emerged as an efficient alternative for fine-tuning foundational models, such as CLIP, for various downstream tasks. Conventionally trained using the task-specific objective, i.e., cross-entropy loss, prompts tend to overfit downstream data distributions and find it challenging to capture task-agnostic general features from the frozen CLIP. This leads to the loss of the model's original generalization capability. To address this issue, our work introduces a self-regularization framework for prompting called PromptSRC (Prompting with Self-regulating Constraints). PromptSRC guides the prompts to optimize for both task-specific and task-agnostic general representations using a three-pronged approach by: (a) regulating prompted representations via mutual agreement maximization with the frozen model, (b) regulating with self-ensemble of prompts over the training trajectory to encode their complementary strengths, and (c) regulating with textual diversity to mitigate sample diversity imbalance with the visual branch. To the best of our knowledge, this is the first regularization framework for prompt learning that avoids overfitting by jointly attending to pre-trained model features, the training trajectory during prompting, and the textual diversity. PromptSRC explicitly steers the prompts to learn a representation space that maximizes performance on downstream tasks without compromising CLIP generalization. We perform extensive experiments on 4 benchmarks where PromptSRC overall performs favorably well compared to the existing methods. Our code and pre-trained models are publicly available at: https://github.com/muzairkhattak/PromptSRC.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_prompt\\Khattak et al_2023_Self-regulating Prompts.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XHZSVI5M\\2307.html}
}

@article{khodadadiAlgorithmsEstimatingTrends2019,
  title = {Algorithms for {{Estimating Trends}} in {{Global Temperature Volatility}}},
  author = {Khodadadi, Arash and McDonald, Daniel J.},
  date = {2019-07-17},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {33},
  number = {01},
  pages = {614--621},
  issn = {2374-3468},
  doi = {10.1609/aaai.v33i01.3301614},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/3837},
  urldate = {2023-05-24},
  abstract = {Trends in terrestrial temperature variability are perhaps more relevant for species viability than trends in mean temperature. In this paper, we develop methodology for estimating such trends using multi-resolution climate data from polar orbiting weather satellites. We derive two novel algorithms for computation that are tailored for dense, gridded observations over both space and time. We evaluate our methods with a simulation that mimics these data’s features and on a large, publicly available, global temperature dataset with the eventual goal of tracking trends in cloud reflectance temperature variability.},
  issue = {01},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Khodadadi_McDonald_2019_Algorithms for Estimating Trends in Global Temperature Volatility.pdf}
}

@inproceedings{khoslaUnderstandingPredictingImage2015,
  title = {Understanding and {{Predicting Image Memorability}} at a {{Large Scale}}},
  booktitle = {2015 {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}})},
  author = {Khosla, Aditya and Raju, Akhil S. and Torralba, Antonio and Oliva, Aude},
  date = {2015-02},
  pages = {2390--2398},
  issn = {2380-7504},
  doi = {10.1109/ICCV.2015.275},
  abstract = {Progress in estimating visual memorability has been limited by the small scale and lack of variety of benchmark data. Here, we introduce a novel experimental procedure to objectively measure human memory, allowing us to build LaMem, the largest annotated image memorability dataset to date (containing 60,000 images from diverse sources). Using Convolutional Neural Networks (CNNs), we show that fine-tuned deep features outperform all other features by a large margin, reaching a rank correlation of 0.64, near human consistency (0.68). Analysis of the responses of the high-level CNN layers shows which objects and regions are positively, and negatively, correlated with memorability, allowing us to create memorability maps for each image and provide a concrete method to perform image memorability manipulation. This work demonstrates that one can now robustly estimate the memorability of images from many different classes, positioning memorability and deep memorability features as prime candidates to estimate the utility of information for cognitive systems. Our model and data are available at: http://memorability.csail.mit.edu.},
  eventtitle = {2015 {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}})},
  keywords = {Benchmark testing,Computer vision,Correlation,Delay effects,Delays,Games,notion,Visualization},
  file = {Y:\paper\computer_vision_topics_18\memorability and intention interface\Khosla et al_2015_Understanding and Predicting Image Memorability at a Large Scale.pdf}
}

@online{kielaHatefulMemesChallenge2021,
  title = {The {{Hateful Memes Challenge}}: {{Detecting Hate Speech}} in {{Multimodal Memes}}},
  shorttitle = {The {{Hateful Memes Challenge}}},
  author = {Kiela, Douwe and Firooz, Hamed and Mohan, Aravind and Goswami, Vedanuj and Singh, Amanpreet and Ringshia, Pratik and Testuggine, Davide},
  date = {2021-04-07},
  eprint = {2005.04790},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2005.04790},
  url = {http://arxiv.org/abs/2005.04790},
  urldate = {2024-03-11},
  abstract = {This work proposes a new challenge set for multimodal classification, focusing on detecting hate speech in multimodal memes. It is constructed such that unimodal models struggle and only multimodal models can succeed: difficult examples ("benign confounders") are added to the dataset to make it hard to rely on unimodal signals. The task requires subtle reasoning, yet is straightforward to evaluate as a binary classification problem. We provide baseline performance numbers for unimodal models, as well as for multimodal models with various degrees of sophistication. We find that state-of-the-art methods perform poorly compared to humans (64.73\% vs. 84.7\% accuracy), illustrating the difficulty of the task and highlighting the challenge that this important problem poses to the community.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Kiela et al_2021_The Hateful Memes Challenge.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SCM2VGB6\\2005.html}
}

@article{kimAnatomicalRiskFactors2021,
  title = {Anatomical {{Risk Factors}} of {{Inferior Alveolar Nerve Injury Association}} with {{Surgical Extraction}} of {{Mandibular Third Molar}} in {{Korean Population}}},
  author = {Kim, Hee Jin and Jo, Ye Joon and Choi, Jun Seok and Kim, Hyo Joon and Kim, Jin and Moon, Seong Yong},
  date = {2021-01},
  journaltitle = {Applied Sciences},
  volume = {11},
  number = {2},
  pages = {816},
  publisher = {Multidisciplinary Digital Publishing Institute},
  issn = {2076-3417},
  doi = {10.3390/app11020816},
  url = {https://www.mdpi.com/2076-3417/11/2/816},
  urldate = {2022-07-03},
  abstract = {The purpose of this study was to analyze the incidence and risk factors of possible inferior alveolar nerve (IAN) injury after extraction of the mandibular third molars. A total of 6182 patients were examined for 10,310 mandibular third molar teeth. Panoramic radiography and patients’ medical records were used to analyze age, gender, and impaction pattern of the mandibular third molar. Cone beam computed tomography (CBCT) was used to investigate the detailed pathway of the inferior alveolar nerve and evaluated the presence of symptoms of nerve damage after tooth extraction. In CBCT, 6283 cases (61\%) of the inferior alveolar nerve were actually in contact with the root of the mandibular third molar. The correlation with the panoramic signs of root darkening (p {$<$} 0.001), root deflection (p {$<$} 0.001), interruption of the IAN (p {$<$} 0.001), diversion of the IAN (p {$<$} 0.001), and narrowing of the IAN (p {$<$} 0.001) had statistical significance. Of the 4708 patients who underwent surgical extraction, 31 (0.658\%) complained of nerve damage. Among them, 30 patients (0.637\%) complained of symptoms of inferior alveolar nerve damage, and 1 patient (0.02\%) complained of symptoms of lingual nerve damage. There was a significant correlation with IAN injury in cases where the roots became dark at the IAN area (p = 0.018) and there was diversion of the IAN at the root area (p = 0.041). When the narrowing of the IAN and the lingual driving pathway of the inferior alveolar nerve appeared simultaneously in CBCT, the risk of IAN injury was high.},
  issue = {2},
  langid = {english},
  keywords = {CBCT,impacted mandibular third molar,inferior alveolar nerve,third molar,third molar extraction},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Kim et al_2021_Anatomical Risk Factors of Inferior Alveolar Nerve Injury Association with.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KGQUXVEJ\\816.html}
}

@online{kimInterpretabilityFeatureAttribution2018,
  title = {Interpretability {{Beyond Feature Attribution}}: {{Quantitative Testing}} with {{Concept Activation Vectors}} ({{TCAV}})},
  shorttitle = {Interpretability {{Beyond Feature Attribution}}},
  author = {Kim, Been and Wattenberg, Martin and Gilmer, Justin and Cai, Carrie and Wexler, James and Viegas, Fernanda and Sayres, Rory},
  date = {2018-06-07},
  eprint = {1711.11279},
  eprinttype = {arXiv},
  eprintclass = {stat},
  doi = {10.48550/arXiv.1711.11279},
  url = {http://arxiv.org/abs/1711.11279},
  urldate = {2023-08-05},
  abstract = {The interpretation of deep learning models is a challenge due to their size, complexity, and often opaque internal state. In addition, many systems, such as image classifiers, operate on low-level features rather than high-level concepts. To address these challenges, we introduce Concept Activation Vectors (CAVs), which provide an interpretation of a neural net's internal state in terms of human-friendly concepts. The key idea is to view the high-dimensional internal state of a neural net as an aid, not an obstacle. We show how to use CAVs as part of a technique, Testing with CAVs (TCAV), that uses directional derivatives to quantify the degree to which a user-defined concept is important to a classification result--for example, how sensitive a prediction of "zebra" is to the presence of stripes. Using the domain of image classification as a testing ground, we describe how CAVs may be used to explore hypotheses and generate insights for a standard image classification network as well as a medical application.},
  pubstate = {prepublished},
  keywords = {notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\understanding deep CNN\\Kim et al_2018_Interpretability Beyond Feature Attribution.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BAWKEWQI\\1711.html}
}

@online{kimMultipleClassificationSplit2020,
  title = {Multiple {{Classification}} with {{Split Learning}}},
  author = {Kim, Jongwon and Shin, Sungho and Yu, Yeonguk and Lee, Junseok and Lee, Kyoobin},
  date = {2020-09-11},
  eprint = {2008.09874},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2008.09874},
  url = {http://arxiv.org/abs/2008.09874},
  urldate = {2022-06-27},
  abstract = {Privacy issues were raised in the process of training deep learning in medical, mobility, and other fields. To solve this problem, we present privacy-preserving distributed deep learning method that allow clients to learn a variety of data without direct exposure. We divided a single deep learning architecture into a common extractor, a cloud model and a local classifier for the distributed learning. First, the common extractor, which is used by local clients, extracts secure features from the input data. The secure features also take the role that the cloud model can employ various task and diverse types of data. The feature contain the most important information that helps to proceed various task. Second, the cloud model including most parts of the whole training model gets the embedded features from the massive local clients, and performs most of deep learning operations which takes severe computing cost. After the operations in cloud model finished, outputs of the cloud model send back to local clients. Finally, the local classifier determined classification results and delivers the results to local clients. When clients train models, our model does not directly expose sensitive information to exterior network. During the test, the average performance improvement was 2.63\% over the existing local training model. However, in a distributed environment, there is a possibility of inversion attack due to exposed features. For this reason, we experimented with the common extractor to prevent data restoration. The quality of restoration of the original image was tested by adjusting the depth of the common extractor. As a result, we found that the deeper the common extractor, the restoration score decreased to 89.74.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 summer intern\\Kim et al_2020_Multiple Classification with Split Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GBRGJ5ZA\\2008.html}
}

@online{kimMultiTaskNeuralProcesses2022,
  title = {Multi-{{Task Neural Processes}}},
  author = {Kim, Donggyun and Cho, Seongwoong and Lee, Wonkwang and Hong, Seunghoon},
  date = {2022-03-25},
  eprint = {2110.14953},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2110.14953},
  url = {http://arxiv.org/abs/2110.14953},
  urldate = {2024-01-29},
  abstract = {Neural Processes (NPs) consider a task as a function realized from a stochastic process and flexibly adapt to unseen tasks through inference on functions. However, naive NPs can model data from only a single stochastic process and are designed to infer each task independently. Since many real-world data represent a set of correlated tasks from multiple sources (e.g., multiple attributes and multi-sensor data), it is beneficial to infer them jointly and exploit the underlying correlation to improve the predictive performance. To this end, we propose Multi-Task Neural Processes (MTNPs), an extension of NPs designed to jointly infer tasks realized from multiple stochastic processes. We build MTNPs in a hierarchical way such that inter-task correlation is considered by conditioning all per-task latent variables on a single global latent variable. In addition, we further design our MTNPs so that they can address multi-task settings with incomplete data (i.e., not all tasks share the same set of input points), which has high practical demands in various applications. Experiments demonstrate that MTNPs can successfully model multiple tasks jointly by discovering and exploiting their correlations in various real-world data such as time series of weather attributes and pixel-aligned visual modalities. We release our code at https://github.com/GitGyun/multi\_task\_neural\_processes.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Kim et al_2022_Multi-Task Neural Processes.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6W296HDK\\2110.html}
}

@article{kimTechnologicalCapabilitiesSamsung1998,
  title = {Technological Capabilities and {{Samsung Electronics}}’ International Production Network in {{East Asia}}},
  author = {Kim, Youngsoo},
  date = {1998},
  journaltitle = {Management Decision},
  volume = {36},
  number = {8},
  pages = {517--527},
  doi = {10.1108/00251749810232592}
}

@inproceedings{kimUniversalFewshotLearning2022,
  title = {Universal {{Few-shot Learning}} of {{Dense Prediction Tasks}} with {{Visual Token Matching}}},
  author = {Kim, Donggyun and Kim, Jinwoo and Cho, Seongwoong and Luo, Chong and Hong, Seunghoon},
  date = {2022-09-29},
  url = {https://openreview.net/forum?id=88nT0j5jAn},
  urldate = {2024-02-04},
  abstract = {Dense prediction tasks are a fundamental class of problems in computer vision. As supervised methods suffer from high pixel-wise labeling cost, a few-shot learning solution that can learn any dense task from a few labeled images is desired. Yet, current few-shot learning methods target a restricted set of tasks such as semantic segmentation, presumably due to challenges in designing a general and unified model that is able to flexibly and efficiently adapt to arbitrary tasks of unseen semantics. We propose Visual Token Matching (VTM), a universal few-shot learner for arbitrary dense prediction tasks. It employs non-parametric matching on patch-level embedded tokens of images and labels that encapsulates all tasks. Also, VTM flexibly adapts to any task with a tiny amount of task-specific parameters that modulate the matching algorithm. We implement VTM as a powerful hierarchical encoder-decoder architecture involving ViT backbones where token matching is performed at multiple feature hierarchies. We experiment VTM on a challenging variant of Taskonomy dataset and observe that it robustly few-shot learns various unseen dense prediction tasks. Surprisingly, it is competitive with fully supervised baselines using only 10 labeled examples of novel tasks (\$0.004\textbackslash\%\$ of full supervision) and sometimes outperforms using \$0.1\textbackslash\%\$ of full supervision. Codes are available at https://github.com/GitGyun/visual\_token\_matching.},
  eventtitle = {The {{Eleventh International Conference}} on {{Learning Representations}}},
  langid = {english},
  file = {Y:\paper\2023 graduation\visual language\Kim et al_2022_Universal Few-shot Learning of Dense Prediction Tasks with Visual Token Matching.pdf}
}

@online{kimUniversalFewshotLearning2023,
  title = {Universal {{Few-shot Learning}} of {{Dense Prediction Tasks}} with {{Visual Token Matching}}},
  author = {Kim, Donggyun and Kim, Jinwoo and Cho, Seongwoong and Luo, Chong and Hong, Seunghoon},
  date = {2023-03-27},
  eprint = {2303.14969},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.14969},
  url = {http://arxiv.org/abs/2303.14969},
  urldate = {2023-06-29},
  abstract = {Dense prediction tasks are a fundamental class of problems in computer vision. As supervised methods suffer from high pixel-wise labeling cost, a few-shot learning solution that can learn any dense task from a few labeled images is desired. Yet, current few-shot learning methods target a restricted set of tasks such as semantic segmentation, presumably due to challenges in designing a general and unified model that is able to flexibly and efficiently adapt to arbitrary tasks of unseen semantics. We propose Visual Token Matching (VTM), a universal few-shot learner for arbitrary dense prediction tasks. It employs non-parametric matching on patch-level embedded tokens of images and labels that encapsulates all tasks. Also, VTM flexibly adapts to any task with a tiny amount of task-specific parameters that modulate the matching algorithm. We implement VTM as a powerful hierarchical encoder-decoder architecture involving ViT backbones where token matching is performed at multiple feature hierarchies. We experiment VTM on a challenging variant of Taskonomy dataset and observe that it robustly few-shot learns various unseen dense prediction tasks. Surprisingly, it is competitive with fully supervised baselines using only 10 labeled examples of novel tasks (0.004\% of full supervision) and sometimes outperforms using 0.1\% of full supervision. Codes are available at https://github.com/GitGyun/visual\_token\_matching.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Kim et al_2023_Universal Few-shot Learning of Dense Prediction Tasks with Visual Token Matching.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XV5CATMS\\2303.html}
}

@online{kimViLTVisionandLanguageTransformer2021,
  title = {{{ViLT}}: {{Vision-and-Language Transformer Without Convolution}} or {{Region Supervision}}},
  shorttitle = {{{ViLT}}},
  author = {Kim, Wonjae and Son, Bokyung and Kim, Ildoo},
  date = {2021-06-10},
  eprint = {2102.03334},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2102.03334},
  urldate = {2024-03-13},
  abstract = {Vision-and-Language Pre-training (VLP) has improved performance on various joint vision-and-language downstream tasks. Current approaches to VLP heavily rely on image feature extraction processes, most of which involve region supervision (e.g., object detection) and the convolutional architecture (e.g., ResNet). Although disregarded in the literature, we find it problematic in terms of both (1) efficiency/speed, that simply extracting input features requires much more computation than the multimodal interaction steps; and (2) expressive power, as it is upper bounded to the expressive power of the visual embedder and its predefined visual vocabulary. In this paper, we present a minimal VLP model, Vision-and-Language Transformer (ViLT), monolithic in the sense that the processing of visual inputs is drastically simplified to just the same convolution-free manner that we process textual inputs. We show that ViLT is up to tens of times faster than previous VLP models, yet with competitive or better downstream task performance. Our code and pre-trained weights are available at https://github.com/dandelin/vilt.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Kim et al_2021_ViLT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HMGUQ2RH\\2102.html}
}

@online{kindermanFoldableSuperNetsScalable2024,
  title = {Foldable {{SuperNets}}: {{Scalable Merging}} of {{Transformers}} with {{Different Initializations}} and {{Tasks}}},
  shorttitle = {Foldable {{SuperNets}}},
  author = {Kinderman, Edan and Hubara, Itay and Maron, Haggai and Soudry, Daniel},
  date = {2024-10-02},
  eprint = {2410.01483},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2410.01483},
  urldate = {2024-10-21},
  abstract = {Many recent methods aim to merge neural networks (NNs) with identical architectures trained on different tasks to obtain a single multi-task model. Most existing works tackle the simpler setup of merging NNs initialized from a common pre-trained network, where simple heuristics like weight averaging work well. This work targets a more challenging goal: merging large transformers trained on different tasks from distinct initializations. First, we demonstrate that traditional merging methods fail catastrophically in this setup. To overcome this challenge, we propose Foldable SuperNet Merge (FS-Merge), a method that optimizes a SuperNet to fuse the original models using a feature reconstruction loss. FS-Merge is simple, data-efficient, and capable of merging models of varying widths. We test FS-Merge against existing methods, including knowledge distillation, on MLPs and transformers across various settings, sizes, tasks, and modalities. FS-Merge consistently outperforms them, achieving SOTA results, particularly in limited data scenarios.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Kinderman et al_2024_Foldable SuperNets.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UBCEDKSP\\2410.html}
}

@online{kingmaAdamMethodStochastic2017,
  title = {Adam: {{A Method}} for {{Stochastic Optimization}}},
  shorttitle = {Adam},
  author = {Kingma, Diederik P. and Ba, Jimmy},
  date = {2017-01-29},
  eprint = {1412.6980},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1412.6980},
  urldate = {2022-08-03},
  abstract = {We introduce Adam, an algorithm for first-order gradient-based optimization of stochastic objective functions, based on adaptive estimates of lower-order moments. The method is straightforward to implement, is computationally efficient, has little memory requirements, is invariant to diagonal rescaling of the gradients, and is well suited for problems that are large in terms of data and/or parameters. The method is also appropriate for non-stationary objectives and problems with very noisy and/or sparse gradients. The hyper-parameters have intuitive interpretations and typically require little tuning. Some connections to related algorithms, on which Adam was inspired, are discussed. We also analyze the theoretical convergence properties of the algorithm and provide a regret bound on the convergence rate that is comparable to the best known results under the online convex optimization framework. Empirical results demonstrate that Adam works well in practice and compares favorably to other stochastic optimization methods. Finally, we discuss AdaMax, a variant of Adam based on the infinity norm.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\optimzer\\Kingma_Ba_2017_Adam.pdf;C\:\\Users\\chsey\\Zotero\\storage\\79YWC5XK\\1412.html}
}

@online{kingmaAdamMethodStochastic2017a,
  title = {Adam: {{A Method}} for {{Stochastic Optimization}}},
  shorttitle = {Adam},
  author = {Kingma, Diederik P. and Ba, Jimmy},
  date = {2017-01-29},
  eprint = {1412.6980},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1412.6980},
  urldate = {2024-04-19},
  abstract = {We introduce Adam, an algorithm for first-order gradient-based optimization of stochastic objective functions, based on adaptive estimates of lower-order moments. The method is straightforward to implement, is computationally efficient, has little memory requirements, is invariant to diagonal rescaling of the gradients, and is well suited for problems that are large in terms of data and/or parameters. The method is also appropriate for non-stationary objectives and problems with very noisy and/or sparse gradients. The hyper-parameters have intuitive interpretations and typically require little tuning. Some connections to related algorithms, on which Adam was inspired, are discussed. We also analyze the theoretical convergence properties of the algorithm and provide a regret bound on the convergence rate that is comparable to the best known results under the online convex optimization framework. Empirical results demonstrate that Adam works well in practice and compares favorably to other stochastic optimization methods. Finally, we discuss AdaMax, a variant of Adam based on the infinity norm.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Kingma_Ba_2017_Adam.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NBKG89HF\\1412.html}
}

@online{kirillovPanopticSegmentation2019,
  title = {Panoptic {{Segmentation}}},
  author = {Kirillov, Alexander and He, Kaiming and Girshick, Ross and Rother, Carsten and Dollár, Piotr},
  date = {2019-04-10},
  eprint = {1801.00868},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1801.00868},
  url = {http://arxiv.org/abs/1801.00868},
  urldate = {2023-11-18},
  abstract = {We propose and study a task we name panoptic segmentation (PS). Panoptic segmentation unifies the typically distinct tasks of semantic segmentation (assign a class label to each pixel) and instance segmentation (detect and segment each object instance). The proposed task requires generating a coherent scene segmentation that is rich and complete, an important step toward real-world vision systems. While early work in computer vision addressed related image/scene parsing tasks, these are not currently popular, possibly due to lack of appropriate metrics or associated recognition challenges. To address this, we propose a novel panoptic quality (PQ) metric that captures performance for all classes (stuff and things) in an interpretable and unified manner. Using the proposed metric, we perform a rigorous study of both human and machine performance for PS on three existing datasets, revealing interesting insights about the task. The aim of our work is to revive the interest of the community in a more unified view of image segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\Kirillov et al_2019_Panoptic Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BRYARFWV\\1801.html}
}

@online{kirillovSegmentAnything2023,
  title = {Segment {{Anything}}},
  author = {Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C. and Lo, Wan-Yen and Dollár, Piotr and Girshick, Ross},
  date = {2023-04-05},
  eprint = {2304.02643},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2304.02643},
  url = {http://arxiv.org/abs/2304.02643},
  urldate = {2023-07-16},
  abstract = {We introduce the Segment Anything (SA) project: a new task, model, and dataset for image segmentation. Using our efficient model in a data collection loop, we built the largest segmentation dataset to date (by far), with over 1 billion masks on 11M licensed and privacy respecting images. The model is designed and trained to be promptable, so it can transfer zero-shot to new image distributions and tasks. We evaluate its capabilities on numerous tasks and find that its zero-shot performance is impressive -- often competitive with or even superior to prior fully supervised results. We are releasing the Segment Anything Model (SAM) and corresponding dataset (SA-1B) of 1B masks and 11M images at https://segment-anything.com to foster research into foundation models for computer vision.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Kirillov et al_2023_Segment Anything.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5UH7KYVZ\\2304.html}
}

@article{kirkpatrickOvercomingCatastrophicForgetting2017,
  title = {Overcoming Catastrophic Forgetting in Neural Networks},
  author = {Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A. and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and Hassabis, Demis and Clopath, Claudia and Kumaran, Dharshan and Hadsell, Raia},
  date = {2017-03-28},
  journaltitle = {Proceedings of the National Academy of Sciences},
  shortjournal = {Proc. Natl. Acad. Sci. U.S.A.},
  volume = {114},
  number = {13},
  eprint = {1612.00796},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  pages = {3521--3526},
  issn = {0027-8424, 1091-6490},
  doi = {10.1073/pnas.1611835114},
  url = {http://arxiv.org/abs/1612.00796},
  urldate = {2023-12-24},
  abstract = {The ability to learn tasks in a sequential fashion is crucial to the development of artificial intelligence. Neural networks are not, in general, capable of this and it has been widely thought that catastrophic forgetting is an inevitable feature of connectionist models. We show that it is possible to overcome this limitation and train networks that can maintain expertise on tasks which they have not experienced for a long time. Our approach remembers old tasks by selectively slowing down learning on the weights important for those tasks. We demonstrate our approach is scalable and effective by solving a set of classification tasks based on the MNIST hand written digit dataset and by learning several Atari 2600 games sequentially.},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\incremental_learning\\Kirkpatrick et al_2017_Overcoming catastrophic forgetting in neural networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VRBCYNL2\\1612.html}
}

@article{kirkpatrickOvercomingCatastrophicForgetting2017a,
  title = {Overcoming Catastrophic Forgetting in Neural Networks},
  author = {Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A. and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and Hassabis, Demis and Clopath, Claudia and Kumaran, Dharshan and Hadsell, Raia},
  date = {2017-03-28},
  journaltitle = {Proceedings of the National Academy of Sciences},
  shortjournal = {Proc. Natl. Acad. Sci. U.S.A.},
  volume = {114},
  number = {13},
  eprint = {1612.00796},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  pages = {3521--3526},
  issn = {0027-8424, 1091-6490},
  doi = {10.1073/pnas.1611835114},
  url = {http://arxiv.org/abs/1612.00796},
  urldate = {2023-11-22},
  abstract = {The ability to learn tasks in a sequential fashion is crucial to the development of artificial intelligence. Neural networks are not, in general, capable of this and it has been widely thought that catastrophic forgetting is an inevitable feature of connectionist models. We show that it is possible to overcome this limitation and train networks that can maintain expertise on tasks which they have not experienced for a long time. Our approach remembers old tasks by selectively slowing down learning on the weights important for those tasks. We demonstrate our approach is scalable and effective by solving a set of classification tasks based on the MNIST hand written digit dataset and by learning several Atari 2600 games sequentially.},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Kirkpatrick et al_2017_Overcoming catastrophic forgetting in neural networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5WAAI9RQ\\1612.html}
}

@online{knodtNeuralRayTracingLearning2021,
  title = {Neural {{Ray-Tracing}}: {{Learning Surfaces}} and {{Reflectance}} for {{Relighting}} and {{View Synthesis}}},
  shorttitle = {Neural {{Ray-Tracing}}},
  author = {Knodt, Julian and Bartusek, Joe and Baek, Seung-Hwan and Heide, Felix},
  date = {2021-12-04},
  eprint = {2104.13562},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2104.13562},
  url = {http://arxiv.org/abs/2104.13562},
  urldate = {2023-01-25},
  abstract = {Recent neural rendering methods have demonstrated accurate view interpolation by predicting volumetric density and color with a neural network. Although such volumetric representations can be supervised on static and dynamic scenes, existing methods implicitly bake the complete scene light transport into a single neural network for a given scene, including surface modeling, bidirectional scattering distribution functions, and indirect lighting effects. In contrast to traditional rendering pipelines, this prohibits changing surface reflectance, illumination, or composing other objects in the scene. In this work, we explicitly model the light transport between scene surfaces and we rely on traditional integration schemes and the rendering equation to reconstruct a scene. The proposed method allows BSDF recovery with unknown light conditions and classic light transports such as pathtracing. By learning decomposed transport with surface representations established in conventional rendering methods, the method naturally facilitates editing shape, reflectance, lighting and scene composition. The method outperforms NeRV for relighting under known lighting conditions, and produces realistic reconstructions for relit and edited scenes. We validate the proposed approach for scene editing, relighting and reflectance estimation learned from synthetic and captured views on a subset of NeRV's datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Knodt et al_2021_Neural Ray-Tracing.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ENMJU6SH\\2104.html}
}

@online{kodaliRecentRapidAdvancement2022,
  title = {Recent, Rapid Advancement in Visual Question Answering Architecture: A Review},
  shorttitle = {Recent, Rapid Advancement in Visual Question Answering Architecture},
  author = {Kodali, Venkat and Berleant, Daniel},
  date = {2022-07-09},
  eprint = {2203.01322},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.01322},
  url = {http://arxiv.org/abs/2203.01322},
  urldate = {2023-05-27},
  abstract = {Understanding visual question answering is going to be crucial for numerous human activities. However, it presents major challenges at the heart of the artificial intelligence endeavor. This paper presents an update on the rapid advancements in visual question answering using images that have occurred in the last couple of years. Tremendous growth in research on improving visual question answering system architecture has been published recently, showing the importance of multimodal architectures. Several points on the benefits of visual question answering are mentioned in the review paper by Manmadhan et al. (2020), on which the present article builds, including subsequent updates in the field.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Multimedia},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\VQA\\Kodali_Berleant_2022_Recent, rapid advancement in visual question answering architecture.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V32WI2X5\\2203.html}
}

@online{kolesnikovBigTransferBiT2020,
  title = {Big {{Transfer}} ({{BiT}}): {{General Visual Representation Learning}}},
  shorttitle = {Big {{Transfer}} ({{BiT}})},
  author = {Kolesnikov, Alexander and Beyer, Lucas and Zhai, Xiaohua and Puigcerver, Joan and Yung, Jessica and Gelly, Sylvain and Houlsby, Neil},
  date = {2020-05-05},
  eprint = {1912.11370},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1912.11370},
  url = {http://arxiv.org/abs/1912.11370},
  urldate = {2023-06-27},
  abstract = {Transfer of pre-trained representations improves sample efficiency and simplifies hyperparameter tuning when training deep neural networks for vision. We revisit the paradigm of pre-training on large supervised datasets and fine-tuning the model on a target task. We scale up pre-training, and propose a simple recipe that we call Big Transfer (BiT). By combining a few carefully selected components, and transferring using a simple heuristic, we achieve strong performance on over 20 datasets. BiT performs well across a surprisingly wide range of data regimes -- from 1 example per class to 1M total examples. BiT achieves 87.5\% top-1 accuracy on ILSVRC-2012, 99.4\% on CIFAR-10, and 76.3\% on the 19 task Visual Task Adaptation Benchmark (VTAB). On small datasets, BiT attains 76.8\% on ILSVRC-2012 with 10 examples per class, and 97.0\% on CIFAR-10 with 10 examples per class. We conduct detailed analysis of the main components that lead to high transfer performance.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\Kolesnikov et al_2020_Big Transfer (BiT).pdf;C\:\\Users\\chsey\\Zotero\\storage\\YTMY7C23\\1912.html}
}

@inproceedings{kolesnikovDetectingVisualRelationships2019,
  title = {Detecting {{Visual Relationships Using Box Attention}}},
  booktitle = {2019 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision Workshop}} ({{ICCVW}})},
  author = {Kolesnikov, Alexander and Kuznetsova, Alina and Lampert, Christoph and Ferrari, Vittorio},
  date = {2019-10},
  pages = {1749--1753},
  publisher = {IEEE},
  location = {Seoul, Korea (South)},
  doi = {10.1109/ICCVW.2019.00217},
  url = {https://ieeexplore.ieee.org/document/9022364/},
  urldate = {2023-05-21},
  abstract = {We propose a new model for detecting visual relationships, such as "person riding motorcycle" or "bottle on table". This task is an important step towards comprehensive structured image understanding, going beyond detecting individual objects. Our main novelty is a Box Attention mechanism that allows to model pairwise interactions between objects using standard object detection pipelines. The resulting model is conceptually clean, expressive and relies on well-justified training and prediction procedures. Moreover, unlike previously proposed approaches, our model does not introduce any additional complex components or hyperparameters on top of those already required by the underlying detection model. We conduct an experimental evaluation on two datasets, V-COCO and Open Images, demonstrating strong quantitative and qualitative results.},
  eventtitle = {2019 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision Workshop}} ({{ICCVW}})},
  isbn = {978-1-72815-023-9},
  langid = {english},
  file = {Y:\paper\2022 winter intern\scene_graph_generation\Kolesnikov et al_2019_Detecting Visual Relationships Using Box Attention.pdf}
}

@article{kondmannDENETHORDynamicEarthNETDataset,
  title = {{{DENETHOR}}: {{The DynamicEarthNET}} Dataset for {{Harmonized}}, Inter-{{Operable}}, Analysis-{{Ready}}, Daily Crop Monitoring from Space},
  author = {Kondmann, Lukas and Toker, Aysim and Rußwurm, Marc and Camero, Andrés and Peressutti, Devis and Milcinski, Grega and Longépé, Nicolas and Mathieu, Pierre-Philippe and Davis, Timothy and Marchisio, Giovanni and Leal-Taixé, Laura and Zhu, Xiao Xiang},
  pages = {13},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\PEPAU8IH\Kondmann et al_DENETHOR.pdf}
}

@online{konecnyFederatedOptimizationDistributed2016,
  title = {Federated {{Optimization}}: {{Distributed Machine Learning}} for {{On-Device Intelligence}}},
  shorttitle = {Federated {{Optimization}}},
  author = {Konečný, Jakub and McMahan, H. Brendan and Ramage, Daniel and Richtárik, Peter},
  date = {2016-10-08},
  eprint = {1610.02527},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1610.02527},
  urldate = {2024-09-11},
  abstract = {We introduce a new and increasingly relevant setting for distributed optimization in machine learning, where the data defining the optimization are unevenly distributed over an extremely large number of nodes. The goal is to train a high-quality centralized model. We refer to this setting as Federated Optimization. In this setting, communication efficiency is of the utmost importance and minimizing the number of rounds of communication is the principal goal.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\3HHM94AD\Konečný 등 - 2016 - Federated Optimization Distributed Machine Learni.pdf}
}

@article{kopanasNeuralPointCatacaustics2022,
  title = {Neural {{Point Catacaustics}} for {{Novel-View Synthesis}} of {{Reflections}}},
  author = {Kopanas, Georgios and Leimkühler, Thomas and Rainer, Gilles and Jambon, Clément and Drettakis, George},
  date = {2022-12},
  journaltitle = {ACM Transactions on Graphics},
  shortjournal = {ACM Trans. Graph.},
  volume = {41},
  number = {6},
  eprint = {2301.01087},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--15},
  issn = {0730-0301, 1557-7368},
  doi = {10.1145/3550454.3555497},
  url = {http://arxiv.org/abs/2301.01087},
  urldate = {2023-01-25},
  abstract = {View-dependent effects such as reflections pose a substantial challenge for image-based and neural rendering algorithms. Above all, curved reflectors are particularly hard, as they lead to highly non-linear reflection flows as the camera moves. We introduce a new point-based representation to compute Neural Point Catacaustics allowing novel-view synthesis of scenes with curved reflectors, from a set of casually-captured input photos. At the core of our method is a neural warp field that models catacaustic trajectories of reflections, so complex specular effects can be rendered using efficient point splatting in conjunction with a neural renderer. One of our key contributions is the explicit representation of reflections with a reflection point cloud which is displaced by the neural warp field, and a primary point cloud which is optimized to represent the rest of the scene. After a short manual annotation step, our approach allows interactive high-quality renderings of novel views with accurate reflection flow. Additionally, the explicit representation of reflection flow supports several forms of scene manipulation in captured scenes, such as reflection editing, cloning of specular objects, reflection tracking across views, and comfortable stereo viewing. We provide the source code and other supplemental material on https://repo-sam.inria.fr/ fungraph/neural\_catacaustics/},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,nerf reflective,연구 - 대상},
  file = {Y\:\\paper\\2022 winter intern\\Kopanas et al_2022_Neural Point Catacaustics for Novel-View Synthesis of Reflections.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6M7V9XUM\\2301.html}
}

@online{krauseGeDiGenerativeDiscriminator2020,
  title = {{{GeDi}}: {{Generative Discriminator Guided Sequence Generation}}},
  shorttitle = {{{GeDi}}},
  author = {Krause, Ben and Gotmare, Akhilesh Deepak and McCann, Bryan and Keskar, Nitish Shirish and Joty, Shafiq and Socher, Richard and Rajani, Nazneen Fatema},
  date = {2020-10-22},
  eprint = {2009.06367},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2009.06367},
  urldate = {2024-05-18},
  abstract = {While large-scale language models (LMs) are able to imitate the distribution of natural language well enough to generate realistic text, it is difficult to control which regions of the distribution they generate. This is especially problematic because datasets used for training large LMs usually contain significant toxicity, hate, bias, and negativity. We propose GeDi as an efficient method for using smaller LMs as generative discriminators to guide generation from large LMs to make them safer and more controllable. GeDi guides generation at each step by computing classification probabilities for all possible next tokens via Bayes rule by normalizing over two class-conditional distributions; one conditioned on the desired attribute, or control code, and another conditioned on the undesired attribute, or anti control code. We find that GeDi gives stronger controllability than the state of the art method while also achieving generation speeds more than 30 times faster. Additionally, training GeDi on only four topics allows us to controllably generate new topics zero-shot from just a keyword, unlocking a new capability that previous controllable generation methods do not have. Lastly, we show that GeDi can make GPT-2 (1.5B parameters) significantly less toxic without sacrificing linguistic quality, making it by far the most practical existing method for detoxifying large language models while maintaining a fast generation speed.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\ITAAJKKT\Krause 등 - 2020 - GeDi Generative Discriminator Guided Sequence Gen.pdf}
}

@online{krishnaVisualGenomeConnecting2016,
  title = {Visual {{Genome}}: {{Connecting Language}} and {{Vision Using Crowdsourced Dense Image Annotations}}},
  shorttitle = {Visual {{Genome}}},
  author = {Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalantidis, Yannis and Li, Li-Jia and Shamma, David A. and Bernstein, Michael S. and Li, Fei-Fei},
  date = {2016-02-23},
  eprint = {1602.07332},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1602.07332},
  url = {http://arxiv.org/abs/1602.07332},
  urldate = {2023-05-29},
  abstract = {Despite progress in perceptual tasks such as image classification, computers still perform poorly on cognitive tasks such as image description and question answering. Cognition is core to tasks that involve not just recognizing, but reasoning about our visual world. However, models used to tackle the rich content in images for cognitive tasks are still being trained using the same datasets designed for perceptual tasks. To achieve success at cognitive tasks, models need to understand the interactions and relationships between objects in an image. When asked "What vehicle is the person riding?", computers will need to identify the objects in an image as well as the relationships riding(man, carriage) and pulling(horse, carriage) in order to answer correctly that "the person is riding a horse-drawn carriage". In this paper, we present the Visual Genome dataset to enable the modeling of such relationships. We collect dense annotations of objects, attributes, and relationships within each image to learn these models. Specifically, our dataset contains over 100K images where each image has an average of 21 objects, 18 attributes, and 18 pairwise relationships between objects. We canonicalize the objects, attributes, relationships, and noun phrases in region descriptions and questions answer pairs to WordNet synsets. Together, these annotations represent the densest and largest dataset of image descriptions, objects, attributes, relationships, and question answers.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Krishna et al_2016_Visual Genome.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2LT4QMYT\\1602.html}
}

@article{krishnaVisualGenomeConnecting2017,
  title = {Visual {{Genome}}: {{Connecting Language}} and {{Vision Using Crowdsourced Dense Image Annotations}}},
  shorttitle = {Visual {{Genome}}},
  author = {Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalantidis, Yannis and Li, Li-Jia and Shamma, David A. and Bernstein, Michael S. and Fei-Fei, Li},
  date = {2017-05-01},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {123},
  number = {1},
  pages = {32--73},
  issn = {1573-1405},
  doi = {10.1007/s11263-016-0981-7},
  url = {https://doi.org/10.1007/s11263-016-0981-7},
  urldate = {2023-05-28},
  abstract = {Despite progress in perceptual tasks such as image classification, computers still perform poorly on cognitive tasks such as image description and question answering. Cognition is core to tasks that involve not just recognizing, but reasoning about our visual world. However, models used to tackle the rich content in images for cognitive tasks are still being trained using the same datasets designed for perceptual tasks. To achieve success at cognitive tasks, models need to understand the interactions and relationships between objects in an image. When asked “What vehicle is the person riding?”, computers will need to identify the objects in an image as well as the relationships riding(man, carriage) and pulling(horse, carriage) to answer correctly that “the person is riding a horse-drawn carriage.” In this paper, we present the Visual Genome dataset to enable the modeling of such relationships. We collect dense annotations of objects, attributes, and relationships within each image to learn these models. Specifically, our dataset contains over 108K images where each image has an average of \$\$35\$\$objects, \$\$26\$\$attributes, and \$\$21\$\$pairwise relationships between objects. We canonicalize the objects, attributes, relationships, and noun phrases in region descriptions and questions answer pairs to WordNet synsets. Together, these annotations represent the densest and largest dataset of image descriptions, objects, attributes, relationships, and question answer pairs.},
  langid = {english},
  keywords = {Attributes,Computer vision,Crowdsourcing,Dataset,Image,Knowledge,Language,Objects,Question answering,Relationships,Scene graph},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Krishna et al_2017_Visual Genome.pdf}
}

@inproceedings{krizhevskyImageNetClassificationDeep2012,
  title = {{{ImageNet Classification}} with {{Deep Convolutional Neural Networks}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  date = {2012},
  volume = {25},
  publisher = {Curran Associates, Inc.},
  url = {https://papers.nips.cc/paper/2012/hash/c399862d3b9d6b76c8436e924a68c45b-Abstract.html},
  urldate = {2022-07-04},
  abstract = {We trained a large, deep convolutional neural network to classify the 1.3 million high-resolution images in the LSVRC-2010 ImageNet training set into the 1000 different classes. On the test data, we achieved top-1 and top-5 error rates of 39.7\textbackslash\% and 18.9\textbackslash\% which is considerably better than the previous state-of-the-art results. The neural network, which has 60 million parameters and 500,000 neurons, consists of five convolutional layers, some of which are followed by max-pooling layers, and two globally connected layers with a final 1000-way softmax. To make training faster, we used non-saturating neurons and a very efficient GPU implementation of convolutional nets. To reduce overfitting in the globally connected layers we employed a new regularization method that proved to be very effective.},
  keywords = {read,read_20220712},
  file = {Y:\paper\Computer Vision\classificaiton\Krizhevsky et al_2012_ImageNet Classification with Deep Convolutional Neural Networks.pdf}
}

@inproceedings{krizhevskyImageNetClassificationDeep2012a,
  title = {{{ImageNet Classification}} with {{Deep Convolutional Neural Networks}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  date = {2012},
  volume = {25},
  publisher = {Curran Associates, Inc.},
  url = {https://papers.nips.cc/paper_files/paper/2012/hash/c399862d3b9d6b76c8436e924a68c45b-Abstract.html},
  urldate = {2023-08-05},
  abstract = {We trained a large, deep convolutional neural network to classify the 1.3 million high-resolution images in the LSVRC-2010 ImageNet training set into the 1000 different classes. On the test data, we achieved top-1 and top-5 error rates of 39.7\textbackslash\% and 18.9\textbackslash\% which is considerably better than the previous state-of-the-art results. The neural network, which has 60 million parameters and 500,000 neurons, consists of five convolutional layers, some of which are followed by max-pooling layers, and two globally connected layers with a final 1000-way softmax. To make training faster, we used non-saturating neurons and a very efficient GPU implementation of convolutional nets. To reduce overfitting in the globally connected layers we employed a new regularization method that proved to be very effective.},
  keywords = {notion},
  file = {Y:\paper\computer_vision_topics_18\Krizhevsky et al_2012_ImageNet Classification with Deep Convolutional Neural Networks.pdf}
}

@article{krizhevskyLearningMultipleLayers,
  title = {Learning {{Multiple Layers}} of {{Features}} from {{Tiny Images}}},
  author = {Krizhevsky, Alex},
  pages = {60},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA3\Krizhevsky_Learning Multiple Layers of Features from Tiny Images.pdf}
}

@inproceedings{kulkarniBabyTalkUnderstanding2011,
  title = {Baby Talk: {{Understanding}} and Generating Simple Image Descriptions},
  shorttitle = {Baby Talk},
  booktitle = {{{CVPR}} 2011},
  author = {Kulkarni, Girish and Premraj, Visruth and Dhar, Sagnik and Li, Siming and Choi, Yejin and Berg, Alexander C and Berg, Tamara L},
  date = {2011-06},
  pages = {1601--1608},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2011.5995466},
  abstract = {We posit that visually descriptive language offers computer vision researchers both information about the world, and information about how people describe the world. The potential benefit from this source is made more significant due to the enormous amount of language data easily available today. We present a system to automatically generate natural language descriptions from images that exploits both statistics gleaned from parsing large quantities of text data and recognition algorithms from computer vision. The system is very effective at producing relevant sentences for images. It also generates descriptions that are notably more true to the specific image content than previous work.},
  eventtitle = {{{CVPR}} 2011},
  keywords = {Computer vision,Detectors,Image recognition,Labeling,Natural languages,notion,Object detection,Visualization},
  file = {Y:\paper\computer_vision_topics_18\vision and language\Kulkarni et al_2011_Baby talk.pdf}
}

@online{kulkarniCanonicalSurfaceMapping2019,
  title = {Canonical {{Surface Mapping}} via {{Geometric Cycle Consistency}}},
  author = {Kulkarni, Nilesh and Gupta, Abhinav and Tulsiani, Shubham},
  date = {2019-08-15},
  eprint = {1907.10043},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1907.10043},
  url = {http://arxiv.org/abs/1907.10043},
  urldate = {2023-08-05},
  abstract = {We explore the task of Canonical Surface Mapping (CSM). Specifically, given an image, we learn to map pixels on the object to their corresponding locations on an abstract 3D model of the category. But how do we learn such a mapping? A supervised approach would require extensive manual labeling which is not scalable beyond a few hand-picked categories. Our key insight is that the CSM task (pixel to 3D), when combined with 3D projection (3D to pixel), completes a cycle. Hence, we can exploit a geometric cycle consistency loss, thereby allowing us to forgo the dense manual supervision. Our approach allows us to train a CSM model for a diverse set of classes, without sparse or dense keypoint annotation, by leveraging only foreground mask labels for training. We show that our predictions also allow us to infer dense correspondence between two images, and compare the performance of our approach against several methods that predict correspondence by leveraging varying amount of supervision.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\3d image understanding\\Kulkarni et al_2019_Canonical Surface Mapping via Geometric Cycle Consistency.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CI9EXL2A\\1907.html}
}

@online{kunstnerHeavyTailedClassImbalance2024,
  title = {Heavy-{{Tailed Class Imbalance}} and {{Why Adam Outperforms Gradient Descent}} on {{Language Models}}},
  author = {Kunstner, Frederik and Yadav, Robin and Milligan, Alan and Schmidt, Mark and Bietti, Alberto},
  date = {2024-02-29},
  eprint = {2402.19449},
  eprinttype = {arXiv},
  eprintclass = {cs, math, stat},
  url = {http://arxiv.org/abs/2402.19449},
  urldate = {2024-06-01},
  abstract = {Adam has been shown to outperform gradient descent in optimizing large language transformers empirically, and by a larger margin than on other tasks, but it is unclear why this happens. We show that the heavy-tailed class imbalance found in language modeling tasks leads to difficulties in the optimization dynamics. When training with gradient descent, the loss associated with infrequent words decreases slower than the loss associated with frequent ones. As most samples come from relatively infrequent words, the average loss decreases slowly with gradient descent. On the other hand, Adam and sign-based methods do not suffer from this problem and improve predictions on all classes. To establish that this behavior is indeed caused by class imbalance, we show empirically that it persist through different architectures and data types, on language transformers, vision CNNs, and linear models. We further study this phenomenon on a linear classification with crossentropy loss, showing that heavy-tailed class imbalance leads to ill-conditioning, and that the normalization used by Adam can counteract it.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Mathematics - Optimization and Control,notion,Statistics - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\C4L7J5BL\2402.pdf}
}

@online{kunstnerNoiseNotMain2023,
  title = {Noise {{Is Not}} the {{Main Factor Behind}} the {{Gap Between SGD}} and {{Adam}} on {{Transformers}}, but {{Sign Descent Might Be}}},
  author = {Kunstner, Frederik and Chen, Jacques and Lavington, Jonathan Wilder and Schmidt, Mark},
  date = {2023-04-27},
  eprint = {2304.13960},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  doi = {10.48550/arXiv.2304.13960},
  url = {http://arxiv.org/abs/2304.13960},
  urldate = {2024-05-31},
  abstract = {The success of the Adam optimizer on a wide array of architectures has made it the default in settings where stochastic gradient descent (SGD) performs poorly. However, our theoretical understanding of this discrepancy is lagging, preventing the development of significant improvements on either algorithm. Recent work advances the hypothesis that Adam and other heuristics like gradient clipping outperform SGD on language tasks because the distribution of the error induced by sampling has heavy tails. This suggests that Adam outperform SGD because it uses a more robust gradient estimate. We evaluate this hypothesis by varying the batch size, up to the entire dataset, to control for stochasticity. We present evidence that stochasticity and heavy-tailed noise are not major factors in the performance gap between SGD and Adam. Rather, Adam performs better as the batch size increases, while SGD is less effective at taking advantage of the reduction in noise. This raises the question as to why Adam outperforms SGD in the full-batch setting. Through further investigation of simpler variants of SGD, we find that the behavior of Adam with large batches is similar to sign descent with momentum.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Mathematics - Optimization and Control,notion},
  file = {Y\:\\paper\\2024_lecture\\Kunstner et al_2023_Noise Is Not the Main Factor Behind the Gap Between SGD and Adam on.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7ZD8YZWC\\2304.html}
}

@book{kuroseComputerNetworkingTopdown2021,
  title = {Computer Networking: A Top-down Approach},
  shorttitle = {Computer Networking},
  author = {Kurose, James F. and Ross, Keith W.},
  date = {2021},
  edition = {Eighth edition},
  publisher = {Pearson},
  location = {Hoboken},
  abstract = {"Welcome to the eighth edition of Computer Networking: A Top-Down Approach. Since the publication of the first edition 16 years ago, our book has been adopted for use at many hundreds of colleges and universities, translated into 14 languages, and used by over one hundred thousand students and practitioners worldwide. We ve heard from many of these readers and have been overwhelmed by the positive response"--},
  isbn = {978-0-13-668155-7},
  langid = {english},
  keywords = {_tablet,Computer networks,Internet},
  file = {C:\Users\chsey\Zotero\storage\L4DUSSVV\Kurose_Ross_2021_Computer networking.pdf}
}

@inproceedings{kutulakosTheoryRefractiveSpecular2005,
  title = {A Theory of Refractive and Specular {{3D}} Shape by Light-Path Triangulation},
  booktitle = {Tenth {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}}'05) {{Volume}} 1},
  author = {Kutulakos, K.N. and Steger, E.},
  date = {2005-10},
  volume = {2},
  pages = {1448-1455 Vol. 2},
  issn = {2380-7504},
  doi = {10.1109/ICCV.2005.26},
  abstract = {We investigate the feasibility of reconstructing an arbitrarily-shaped specular scene (refractive or mirror-like) from one or more viewpoints. By reducing shape recovery to the problem of reconstructing individual 3D light paths that cross the image plane, we obtain three key results. First, we show how to compute the depth map of a specular scene from a single viewpoint, when the scene redirects incoming light just once. Second, for scenes where incoming light undergoes two refractions or reflections, we show that three viewpoints are sufficient to enable reconstruction in the general case. Third, we show that it is impossible to reconstruct individual light paths when light is redirected more than twice. Our analysis assumes that, for every point on the image plane, we know at least one 3D point on its light path. This leads to reconstruction algorithms that rely on an "environment matting" procedure to establish pixel-to-point correspondences along a light path. Preliminary results for a variety of scenes (mirror, glass, etc) are also presented.},
  eventtitle = {Tenth {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}}'05) {{Volume}} 1},
  keywords = {Algorithm design and analysis,Glass,Image reconstruction,Layout,Liquids,Mirrors,Optical reflection,Optical refraction,Reconstruction algorithms,Shape},
  file = {Y\:\\paper\\2022 winter intern\\Kutulakos_Steger_2005_A theory of refractive and specular 3D shape by light-path triangulation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Z2RPRW25\\stamp.html}
}

@online{kwonMaskedVisionLanguage2023,
  title = {Masked {{Vision}} and {{Language Modeling}} for {{Multi-modal Representation Learning}}},
  author = {Kwon, Gukyeong and Cai, Zhaowei and Ravichandran, Avinash and Bas, Erhan and Bhotika, Rahul and Soatto, Stefano},
  date = {2023-03-14},
  eprint = {2208.02131},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2208.02131},
  urldate = {2024-06-27},
  abstract = {In this paper, we study how to use masked signal modeling in vision and language (V+L) representation learning. Instead of developing masked language modeling (MLM) and masked image modeling (MIM) independently, we propose to build joint masked vision and language modeling, where the masked signal of one modality is reconstructed with the help from another modality. This is motivated by the nature of image-text paired data that both of the image and the text convey almost the same information but in different formats. The masked signal reconstruction of one modality conditioned on another modality can also implicitly learn cross-modal alignment between language tokens and image patches. Our experiments on various V+L tasks show that the proposed method, along with common V+L alignment losses, achieves state-of-the-art performance in the regime of millions of pre-training data. Also, we outperforms the other competitors by a significant margin in limited data scenarios.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\J3HJVPNJ\Kwon 등 - 2023 - Masked Vision and Language Modeling for Multi-moda.pdf}
}

@misc{Lab07Vision,
  title = {Lab 07 Vision Transformer},
  file = {Y:\paper\textbook\2022 AI exp lab\lab 07 vision transformer.pdf}
}

@inproceedings{lafortuneNonlinearApproximationReflectance1997,
  title = {Non-Linear Approximation of Reflectance Functions},
  booktitle = {Proceedings of the 24th Annual Conference on {{Computer}} Graphics and Interactive Techniques  - {{SIGGRAPH}} '97},
  author = {Lafortune, Eric P. F. and Foo, Sing-Choong and Torrance, Kenneth E. and Greenberg, Donald P.},
  date = {1997},
  pages = {117--126},
  publisher = {ACM Press},
  location = {Not Known},
  doi = {10.1145/258734.258801},
  url = {http://portal.acm.org/citation.cfm?doid=258734.258801},
  urldate = {2023-04-10},
  abstract = {We introduce a new class of primitive functions with non-linear parameters for representing light reflectance functions. The functions are reciprocal, energy-conserving and expressive. They can capture important phenomena such as off-specular reflection, increasing reflectance and retro-reflection. We demonstrate this by fitting sums of primitive functions to a physically-based model and to actual measurements. The resulting representation is simple, compact and uniform. It can be applied efficiently in analytical and Monte Carlo computations.},
  eventtitle = {The 24th Annual Conference},
  isbn = {978-0-89791-896-1},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\ELAMJCQQ\Lafortune 등 - 1997 - Non-linear approximation of reflectance functions.pdf}
}

@inproceedings{lakshminarayananSimpleScalablePredictive2017,
  title = {Simple and {{Scalable Predictive Uncertainty Estimation}} Using {{Deep Ensembles}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
  date = {2017},
  volume = {30},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2017/hash/9ef2ed4b7fd2c810847ffa5fa85bce38-Abstract.html},
  urldate = {2022-09-01},
  abstract = {Deep neural networks (NNs) are powerful black box predictors that have recently achieved impressive performance on a wide spectrum of tasks. Quantifying predictive uncertainty in NNs is a challenging and yet unsolved problem.  Bayesian NNs, which learn a distribution over weights, are currently the state-of-the-art for estimating predictive uncertainty; however these require significant modifications to the training procedure and are computationally expensive compared to standard (non-Bayesian)  NNs.  We propose an alternative to Bayesian NNs that is simple to implement, readily parallelizable, requires very little hyperparameter tuning, and yields high quality predictive uncertainty estimates. Through a series of experiments on classification and regression benchmarks, we demonstrate that our method produces well-calibrated uncertainty estimates which are as good or better than approximate Bayesian NNs. To assess robustness to dataset shift, we evaluate the predictive uncertainty on test examples from known and unknown distributions, and show that our method is able to express higher uncertainty on out-of-distribution examples. We demonstrate the scalability of our method by evaluating predictive uncertainty estimates on ImageNet.},
  file = {Y:\paper\2022 autumn intern\OOD\Lakshminarayanan et al_2017_Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles.pdf}
}

@article{lampertAttributeBasedClassificationZeroShot2014,
  title = {Attribute-{{Based Classification}} for {{Zero-Shot Visual Object Categorization}}},
  author = {Lampert, Christoph H. and Nickisch, Hannes and Harmeling, Stefan},
  date = {2014-03},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {36},
  number = {3},
  pages = {453--465},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2013.140},
  abstract = {We study the problem of object recognition for categories for which we have no training examples, a task also called zero–data or zero-shot learning. This situation has hardly been studied in computer vision research, even though it occurs frequently; the world contains tens of thousands of different object classes, and image collections have been formed and suitably annotated for only a few of them. To tackle the problem, we introduce attribute-based classification: Objects are identified based on a high-level description that is phrased in terms of semantic attributes, such as the object's color or shape. Because the identification of each such property transcends the specific learning task at hand, the attribute classifiers can be prelearned independently, for example, from existing image data sets unrelated to the current task. Afterward, new classes can be detected based on their attribute representation, without the need for a new training phase. In this paper, we also introduce a new data set, Animals with Attributes, of over 30,000 images of 50 animal classes, annotated with 85 semantic attributes. Extensive experiments on this and two more data sets show that attribute-based classification indeed is able to categorize images without access to any training images of the target classes.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  keywords = {Computer vision,Marine animals,notion,Object recognition,Probabilistic logic,Semantics,Training,Vectors,vision and scene understanding},
  file = {Y:\paper\computer_vision_topics_18\few shot learning\Lampert et al_2014_Attribute-Based Classification for Zero-Shot Visual Object Categorization.pdf}
}

@online{lanALBERTLiteBERT2020,
  title = {{{ALBERT}}: {{A Lite BERT}} for {{Self-supervised Learning}} of {{Language Representations}}},
  shorttitle = {{{ALBERT}}},
  author = {Lan, Zhenzhong and Chen, Mingda and Goodman, Sebastian and Gimpel, Kevin and Sharma, Piyush and Soricut, Radu},
  date = {2020-02-08},
  eprint = {1909.11942},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1909.11942},
  urldate = {2024-08-23},
  abstract = {Increasing model size when pretraining natural language representations often results in improved performance on downstream tasks. However, at some point further model increases become harder due to GPU/TPU memory limitations and longer training times. To address these problems, we present two parameterreduction techniques to lower memory consumption and increase the training speed of BERT (Devlin et al., 2019). Comprehensive empirical evidence shows that our proposed methods lead to models that scale much better compared to the original BERT. We also use a self-supervised loss that focuses on modeling inter-sentence coherence, and show it consistently helps downstream tasks with multi-sentence inputs. As a result, our best model establishes new state-of-the-art results on the GLUE, RACE, and SQuAD benchmarks while having fewer parameters compared to BERT-large. The code and the pretrained models are available at https://github.com/google-research/ALBERT.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,notion},
  file = {C:\Users\chsey\Zotero\storage\WUSF447X\Lan 등 - 2020 - ALBERT A Lite BERT for Self-supervised Learning o.pdf}
}

@inproceedings{laugesenWhatFactorsContributed2010,
  title = {What {{Factors Contributed}} to the {{Success}} of {{Apple}}'s {{iPhone}}?},
  booktitle = {2010 {{Ninth International Conference}} on {{Mobile Business}} and 2010 {{Ninth Global Mobility Roundtable}} ({{ICMB-GMR}})},
  author = {Laugesen, John and Yuan, Yufei},
  date = {2010-06},
  pages = {91--99},
  doi = {10.1109/ICMB-GMR.2010.63},
  url = {https://ieeexplore.ieee.org/document/5494782},
  urldate = {2023-12-30},
  abstract = {Unknown to most North American consumers, a mobile data and Internet service in Japan called i-mode has been highly successful in that country for the past decade. Unfortunately, mobile data services in North America have lagged behind many European and Asian countries. However, the situation changed rapidly with the iPhone, launched in the US in June 2007. Consumers lined up for days for the chance to purchase one, and over 500, 000 units sold on the first weekend. Since that time, over 42 million iPhones have been sold, arguably making it one of the most successful mobile phone products ever launched. What is it that makes the iPhone such a success? In this paper we define a set of success criteria to investigate the success of the iPhone and propose a comprehensive success model. The success model can be used by both academics and practitioners to understand the reasons why, and ways to ensure that mobile data and commerce services become successful.},
  eventtitle = {2010 {{Ninth International Conference}} on {{Mobile Business}} and 2010 {{Ninth Global Mobility Roundtable}} ({{ICMB-GMR}})},
  file = {Y:\paper\management\Laugesen_Yuan_2010_What Factors Contributed to the Success of Apple's iPhone.pdf}
}

@online{Lecture01introPdf,
  title = {Lecture01-Intro.Pdf},
  url = {https://drone.sjtu.edu.cn/dpzou/teaching/course/lecture01-intro.pdf},
  urldate = {2023-01-26},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\lecture01-intro.pdf}
}

@article{lecunGradientbasedLearningApplied1998,
  title = {Gradient-Based Learning Applied to Document Recognition},
  author = {Lecun, Y. and Bottou, L. and Bengio, Y. and Haffner, P.},
  date = {1998-11},
  journaltitle = {Proceedings of the IEEE},
  volume = {86},
  number = {11},
  pages = {2278--2324},
  issn = {1558-2256},
  doi = {10.1109/5.726791},
  abstract = {Multilayer neural networks trained with the back-propagation algorithm constitute the best example of a successful gradient based learning technique. Given an appropriate network architecture, gradient-based learning algorithms can be used to synthesize a complex decision surface that can classify high-dimensional patterns, such as handwritten characters, with minimal preprocessing. This paper reviews various methods applied to handwritten character recognition and compares them on a standard handwritten digit recognition task. Convolutional neural networks, which are specifically designed to deal with the variability of 2D shapes, are shown to outperform all other techniques. Real-life document recognition systems are composed of multiple modules including field extraction, segmentation recognition, and language modeling. A new learning paradigm, called graph transformer networks (GTN), allows such multimodule systems to be trained globally using gradient-based methods so as to minimize an overall performance measure. Two systems for online handwriting recognition are described. Experiments demonstrate the advantage of global training, and the flexibility of graph transformer networks. A graph transformer network for reading a bank cheque is also described. It uses convolutional neural network character recognizers combined with global training techniques to provide record accuracy on business and personal cheques. It is deployed commercially and reads several million cheques per day.},
  eventtitle = {Proceedings of the {{IEEE}}},
  keywords = {Character recognition,Feature extraction,Hidden Markov models,Machine learning,Multi-layer neural network,Neural networks,Optical character recognition software,Optical computing,Pattern recognition,Principal component analysis},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Lecun et al_1998_Gradient-based learning applied to document recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\A66W26Y3\\726791.html}
}

@article{leeAutomatedPredictionExtraction2022,
  title = {Automated {{Prediction}} of {{Extraction Difficulty}} and {{Inferior Alveolar Nerve Injury}} for {{Mandibular Third Molar Using}} a {{Deep Neural Network}}},
  author = {Lee, Junseok and Park, Jumi and Moon, Seong Yong and Lee, Kyoobin},
  date = {2022-01},
  journaltitle = {Applied Sciences},
  volume = {12},
  number = {1},
  pages = {475},
  publisher = {Multidisciplinary Digital Publishing Institute},
  issn = {2076-3417},
  doi = {10.3390/app12010475},
  url = {https://www.mdpi.com/2076-3417/12/1/475},
  urldate = {2022-06-27},
  abstract = {Extraction of mandibular third molars is a common procedure in oral and maxillofacial surgery. There are studies that simultaneously predict the extraction difficulty of mandibular third molar and the complications that may occur. Thus, we propose a method of automatically detecting mandibular third molars in the panoramic radiographic images and predicting the extraction difficulty and likelihood of inferior alveolar nerve (IAN) injury. Our dataset consists of 4903 panoramic radiographic images acquired from various dental hospitals. Seven dentists annotated detection and classification labels. The detection model determines the mandibular third molar in the panoramic radiographic image. The region of interest (ROI) includes the detected mandibular third molar, adjacent teeth, and IAN, which is cropped in the panoramic radiographic image. The classification models use ROI as input to predict the extraction difficulty and likelihood of IAN injury. The achieved detection performance was 99.0\% mAP over the intersection of union (IOU) 0.5. In addition, we achieved an 83.5\% accuracy for the prediction of extraction difficulty and an 81.1\% accuracy for the prediction of the likelihood of IAN injury. We demonstrated that a deep learning method can support the diagnosis for extracting the mandibular third molar.},
  issue = {1},
  langid = {english},
  keywords = {deep neural network,extraction difficulty,inferior alveolar nerve (IAN) injury,mandibular third molar,panoramic radiographic image},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\reproduction\\Lee et al_2022_Automated Prediction of Extraction Difficulty and Inferior Alveolar Nerve.pdf;C\:\\Users\\chsey\\Zotero\\storage\\M9TZDJMC\\475.html}
}

@online{leeMoAIMixtureAll2024,
  title = {{{MoAI}}: {{Mixture}} of {{All Intelligence}} for {{Large Language}} and {{Vision Models}}},
  shorttitle = {{{MoAI}}},
  author = {Lee, Byung-Kwan and Park, Beomchan and Kim, Chae Won and Ro, Yong Man},
  date = {2024-03-12},
  eprint = {2403.07508},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2403.07508},
  urldate = {2024-03-13},
  abstract = {The rise of large language models (LLMs) and instruction tuning has led to the current trend of instruction-tuned large language and vision models (LLVMs). This trend involves either meticulously curating numerous instruction tuning datasets tailored to specific objectives or enlarging LLVMs to manage vast amounts of vision language (VL) data. However, current LLVMs have disregarded the detailed and comprehensive real-world scene understanding available from specialized computer vision (CV) models in visual perception tasks such as segmentation, detection, scene graph generation (SGG), and optical character recognition (OCR). Instead, the existing LLVMs rely mainly on the large capacity and emergent capabilities of their LLM backbones. Therefore, we present a new LLVM, Mixture of All Intelligence (MoAI), which leverages auxiliary visual information obtained from the outputs of external segmentation, detection, SGG, and OCR models. MoAI operates through two newly introduced modules: MoAI-Compressor and MoAI-Mixer. After verbalizing the outputs of the external CV models, the MoAI-Compressor aligns and condenses them to efficiently use relevant auxiliary visual information for VL tasks. MoAI-Mixer then blends three types of intelligence (1) visual features, (2) auxiliary features from the external CV models, and (3) language features by utilizing the concept of Mixture of Experts. Through this integration, MoAI significantly outperforms both open-source and closed-source LLVMs in numerous zero-shot VL tasks, particularly those related to real-world scene understanding such as object existence, positions, relations, and OCR without enlarging the model size or curating extra visual instruction tuning datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Lee et al_2024_MoAI.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GCEXMB6C\\2403.html}
}

@online{leeMultiGameDecisionTransformers2022,
  title = {Multi-{{Game Decision Transformers}}},
  author = {Lee, Kuang-Huei and Nachum, Ofir and Yang, Mengjiao and Lee, Lisa and Freeman, Daniel and Xu, Winnie and Guadarrama, Sergio and Fischer, Ian and Jang, Eric and Michalewski, Henryk and Mordatch, Igor},
  date = {2022-10-15},
  eprint = {2205.15241},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.15241},
  urldate = {2024-05-08},
  abstract = {A longstanding goal of the field of AI is a method for learning a highly capable, generalist agent from diverse experience. In the subfields of vision and language, this was largely achieved by scaling up transformer-based models and training them on large, diverse datasets. Motivated by this progress, we investigate whether the same strategy can be used to produce generalist reinforcement learning agents. Specifically, we show that a single transformer-based model - with a single set of weights - trained purely offline can play a suite of up to 46 Atari games simultaneously at close-to-human performance. When trained and evaluated appropriately, we find that the same trends observed in language and vision hold, including scaling of performance with model size and rapid adaptation to new games via fine-tuning. We compare several approaches in this multi-game setting, such as online and offline RL methods and behavioral cloning, and find that our Multi-Game Decision Transformer models offer the best scalability and performance. We release the pre-trained models and code to encourage further research in this direction.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Lee et al_2022_Multi-Game Decision Transformers.pdf}
}

@online{leeParameterEfficientMultimodal2021,
  title = {Parameter {{Efficient Multimodal Transformers}} for {{Video Representation Learning}}},
  author = {Lee, Sangho and Yu, Youngjae and Kim, Gunhee and Breuel, Thomas and Kautz, Jan and Song, Yale},
  date = {2021-09-22},
  eprint = {2012.04124},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2012.04124},
  url = {http://arxiv.org/abs/2012.04124},
  urldate = {2024-02-02},
  abstract = {The recent success of Transformers in the language domain has motivated adapting it to a multimodal setting, where a new visual model is trained in tandem with an already pretrained language model. However, due to the excessive memory requirements from Transformers, existing work typically fixes the language model and train only the vision module, which limits its ability to learn cross-modal information in an end-to-end manner. In this work, we focus on reducing the parameters of multimodal Transformers in the context of audio-visual video representation learning. We alleviate the high memory requirement by sharing the parameters of Transformers across layers and modalities; we decompose the Transformer into modality-specific and modality-shared parts so that the model learns the dynamics of each modality both individually and together, and propose a novel parameter sharing scheme based on low-rank approximation. We show that our approach reduces parameters of the Transformers up to 97\$\textbackslash\%\$, allowing us to train our model end-to-end from scratch. We also propose a negative sampling approach based on an instance similarity measured on the CNN embedding space that our model learns together with the Transformers. To demonstrate our approach, we pretrain our model on 30-second clips (480 frames) from Kinetics-700 and transfer it to audio-visual classification tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Lee et al_2021_Parameter Efficient Multimodal Transformers for Video Representation Learning.pdf;Y\:\\research\\research_paper\\parameter-efficient-multimodal-transformers-for-video-representation-learning - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\D3GIECI7\\2012.html}
}

@online{leePreservationGlobalKnowledge2022,
  title = {Preservation of {{Global Knowledge}} by {{Not-True Distillation}} in {{Federated Learning}}},
  author = {Lee, Gihun and Jeong, Minchan and Shin, Yongjin and Bae, Sangmin and Yun, Se-Young},
  date = {2022-02-17},
  eprint = {2106.03097},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.03097},
  urldate = {2022-10-09},
  abstract = {In federated learning, a strong global model is collaboratively learned by aggregating clients' locally trained models. Although this precludes the need to access clients' data directly, the global model's convergence often suffers from data heterogeneity. This study starts from an analogy to continual learning and suggests that forgetting could be the bottleneck of federated learning. We observe that the global model forgets the knowledge from previous rounds, and the local training induces forgetting the knowledge outside of the local distribution. Based on our findings, we hypothesize that tackling down forgetting will relieve the data heterogeneity problem. To this end, we propose a novel and effective algorithm, Federated Not-True Distillation (FedNTD), which preserves the global perspective on locally available data only for the not-true classes. In the experiments, FedNTD shows state-of-the-art performance on various setups without compromising data privacy or incurring additional communication costs.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\intern\\Lee et al_2022_Preservation of Global Knowledge by Not-True Distillation in Federated Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ICI96AQR\\2106.html}
}

@inproceedings{leeReadonlyPromptOptimization2023,
  title = {Read-Only {{Prompt Optimization}} for {{Vision-Language Few-shot Learning}}},
  author = {Lee, Dongjun and Song, Seokwon and Suh, Jihee and Choi, Joonmyeong and Lee, Sanghyeok and Kim, Hyunwoo J.},
  date = {2023},
  pages = {1401--1411},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Lee_Read-only_Prompt_Optimization_for_Vision-Language_Few-shot_Learning_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Lee et al_2023_Read-only Prompt Optimization for Vision-Language Few-shot Learning.pdf}
}

@online{leeSimpleUnifiedFramework2018,
  title = {A {{Simple Unified Framework}} for {{Detecting Out-of-Distribution Samples}} and {{Adversarial Attacks}}},
  author = {Lee, Kimin and Lee, Kibok and Lee, Honglak and Shin, Jinwoo},
  date = {2018-10-27},
  eprint = {1807.03888},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1807.03888},
  urldate = {2022-10-03},
  abstract = {Detecting test samples drawn sufficiently far away from the training distribution statistically or adversarially is a fundamental requirement for deploying a good classifier in many real-world machine learning applications. However, deep neural networks with the softmax classifier are known to produce highly overconfident posterior distributions even for such abnormal samples. In this paper, we propose a simple yet effective method for detecting any abnormal samples, which is applicable to any pre-trained softmax neural classifier. We obtain the class conditional Gaussian distributions with respect to (low- and upper-level) features of the deep models under Gaussian discriminant analysis, which result in a confidence score based on the Mahalanobis distance. While most prior methods have been evaluated for detecting either out-of-distribution or adversarial samples, but not both, the proposed method achieves the state-of-the-art performances for both cases in our experiments. Moreover, we found that our proposed method is more robust in harsh cases, e.g., when the training dataset has noisy labels or small number of samples. Finally, we show that the proposed method enjoys broader usage by applying it to class-incremental learning: whenever out-of-distribution samples are detected, our classification rule can incorporate new classes well without further training deep models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Cryptography and Security,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Lee et al_2018_A Simple Unified Framework for Detecting Out-of-Distribution Samples and.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MUG4PG2N\\1807.html}
}

@online{leeTrainingConfidencecalibratedClassifiers2018,
  title = {Training {{Confidence-calibrated Classifiers}} for {{Detecting Out-of-Distribution Samples}}},
  author = {Lee, Kimin and Lee, Honglak and Lee, Kibok and Shin, Jinwoo},
  date = {2018-02-23},
  eprint = {1711.09325},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1711.09325},
  url = {http://arxiv.org/abs/1711.09325},
  urldate = {2022-09-13},
  abstract = {The problem of detecting whether a test sample is from in-distribution (i.e., training distribution by a classifier) or out-of-distribution sufficiently different from it arises in many real-world machine learning applications. However, the state-of-art deep neural networks are known to be highly overconfident in their predictions, i.e., do not distinguish in- and out-of-distributions. Recently, to handle this issue, several threshold-based detectors have been proposed given pre-trained neural classifiers. However, the performance of prior works highly depends on how to train the classifiers since they only focus on improving inference procedures. In this paper, we develop a novel training method for classifiers so that such inference algorithms can work better. In particular, we suggest two additional terms added to the original loss (e.g., cross entropy). The first one forces samples from out-of-distribution less confident by the classifier and the second one is for (implicitly) generating most effective training samples for the first one. In essence, our method jointly trains both classification and generative neural networks for out-of-distribution. We demonstrate its effectiveness using deep convolutional neural networks on various popular image datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Lee et al_2018_Training Confidence-calibrated Classifiers for Detecting Out-of-Distribution.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QLI657U7\\1711.html}
}

@online{leFastfoodApproximateKernel2014,
  title = {Fastfood: {{Approximate Kernel Expansions}} in {{Loglinear Time}}},
  shorttitle = {Fastfood},
  author = {Le, Quoc Viet and Sarlos, Tamas and Smola, Alexander Johannes},
  date = {2014-08-13},
  eprint = {1408.3060},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1408.3060},
  url = {http://arxiv.org/abs/1408.3060},
  urldate = {2024-04-21},
  abstract = {Despite their successes, what makes kernel methods difficult to use in many large scale problems is the fact that storing and computing the decision function is typically expensive, especially at prediction time. In this paper, we overcome this difficulty by proposing Fastfood, an approximation that accelerates such computation significantly. Key to Fastfood is the observation that Hadamard matrices, when combined with diagonal Gaussian matrices, exhibit properties similar to dense Gaussian random matrices. Yet unlike the latter, Hadamard and diagonal matrices are inexpensive to multiply and store. These two matrices can be used in lieu of Gaussian matrices in Random Kitchen Sinks proposed by Rahimi and Recht (2009) and thereby speeding up the computation for a large range of kernel functions. Specifically, Fastfood requires O(n log d) time and O(n) storage to compute n non-linear basis functions in d dimensions, a significant improvement from O(nd) computation and storage, without sacrificing accuracy. Our method applies to any translation invariant and any dot-product kernel, such as the popular RBF kernels and polynomial kernels. We prove that the approximation is unbiased and has low variance. Experiments show that we achieve similar accuracy to full kernel expansions and Random Kitchen Sinks while being 100x faster and using 1000x less memory. These improvements, especially in terms of memory usage, make kernel methods more practical for applications that have large training sets and/or require real-time prediction.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Le et al_2014_Fastfood.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2LPV6XPP\\1408.html}
}

@online{lepikhinGShardScalingGiant2020,
  title = {{{GShard}}: {{Scaling Giant Models}} with {{Conditional Computation}} and {{Automatic Sharding}}},
  shorttitle = {{{GShard}}},
  author = {Lepikhin, Dmitry and Lee, HyoukJoong and Xu, Yuanzhong and Chen, Dehao and Firat, Orhan and Huang, Yanping and Krikun, Maxim and Shazeer, Noam and Chen, Zhifeng},
  date = {2020-06-30},
  eprint = {2006.16668},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2006.16668},
  urldate = {2024-02-02},
  abstract = {Neural network scaling has been critical for improving the model quality in many real-world machine learning applications with vast amounts of training data and compute. Although this trend of scaling is affirmed to be a sure-fire approach for better model quality, there are challenges on the path such as the computation cost, ease of programming, and efficient implementation on parallel devices. GShard is a module composed of a set of lightweight annotation APIs and an extension to the XLA compiler. It provides an elegant way to express a wide range of parallel computation patterns with minimal changes to the existing model code. GShard enabled us to scale up multilingual neural machine translation Transformer model with Sparsely-Gated Mixture-of-Experts beyond 600 billion parameters using automatic sharding. We demonstrate that such a giant model can efficiently be trained on 2048 TPU v3 accelerators in 4 days to achieve far superior quality for translation from 100 languages to English compared to the prior art.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Lepikhin et al_2020_GShard.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PMKMMLN7\\2006.html}
}

@online{lesterPowerScaleParameterEfficient2021,
  title = {The {{Power}} of {{Scale}} for {{Parameter-Efficient Prompt Tuning}}},
  author = {Lester, Brian and Al-Rfou, Rami and Constant, Noah},
  date = {2021-09-02},
  eprint = {2104.08691},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2104.08691},
  urldate = {2023-08-11},
  abstract = {In this work, we explore "prompt tuning", a simple yet effective mechanism for learning "soft prompts" to condition frozen language models to perform specific downstream tasks. Unlike the discrete text prompts used by GPT-3, soft prompts are learned through backpropagation and can be tuned to incorporate signal from any number of labeled examples. Our end-to-end learned approach outperforms GPT-3's "few-shot" learning by a large margin. More remarkably, through ablations on model size using T5, we show that prompt tuning becomes more competitive with scale: as models exceed billions of parameters, our method "closes the gap" and matches the strong performance of model tuning (where all model weights are tuned). This finding is especially relevant in that large models are costly to share and serve, and the ability to reuse one frozen model for multiple downstream tasks can ease this burden. Our method can be seen as a simplification of the recently proposed "prefix tuning" of Li and Liang (2021), and we provide a comparison to this and other similar approaches. Finally, we show that conditioning a frozen model with soft prompts confers benefits in robustness to domain transfer, as compared to full model tuning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Lester et al_2021_The Power of Scale for Parameter-Efficient Prompt Tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FF5T7WCS\\2104.html}
}

@online{lesterPowerScaleParameterEfficient2021a,
  title = {The {{Power}} of {{Scale}} for {{Parameter-Efficient Prompt Tuning}}},
  author = {Lester, Brian and Al-Rfou, Rami and Constant, Noah},
  date = {2021-09-02},
  eprint = {2104.08691},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2104.08691},
  urldate = {2023-08-25},
  abstract = {In this work, we explore "prompt tuning", a simple yet effective mechanism for learning "soft prompts" to condition frozen language models to perform specific downstream tasks. Unlike the discrete text prompts used by GPT-3, soft prompts are learned through backpropagation and can be tuned to incorporate signal from any number of labeled examples. Our end-to-end learned approach outperforms GPT-3's "few-shot" learning by a large margin. More remarkably, through ablations on model size using T5, we show that prompt tuning becomes more competitive with scale: as models exceed billions of parameters, our method "closes the gap" and matches the strong performance of model tuning (where all model weights are tuned). This finding is especially relevant in that large models are costly to share and serve, and the ability to reuse one frozen model for multiple downstream tasks can ease this burden. Our method can be seen as a simplification of the recently proposed "prefix tuning" of Li and Liang (2021), and we provide a comparison to this and other similar approaches. Finally, we show that conditioning a frozen model with soft prompts confers benefits in robustness to domain transfer, as compared to full model tuning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\CJ_paper\\Lester et al_2021_The Power of Scale for Parameter-Efficient Prompt Tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4JL4ABPV\\2104.html}
}

@inproceedings{levoyLightFieldRendering1996,
  title = {Light Field Rendering},
  booktitle = {Proceedings of the 23rd Annual Conference on {{Computer}} Graphics and Interactive Techniques  - {{SIGGRAPH}} '96},
  author = {Levoy, Marc and Hanrahan, Pat},
  date = {1996},
  pages = {31--42},
  publisher = {ACM Press},
  location = {Not Known},
  doi = {10.1145/237170.237199},
  url = {http://portal.acm.org/citation.cfm?doid=237170.237199},
  urldate = {2023-01-03},
  abstract = {A number of techniques have been proposed for flying through scenes by redisplaying previously rendered or digitized views. Techniques have also been proposed for interpolating between views by warping input images, using depth information or correspondences between multiple images. In this paper, we describe a simple and robust method for generating new views from arbitrary camera positions without depth information or feature matching, simply by combining and resampling the available images. The key to this technique lies in interpreting the input images as 2D slices of a 4D function - the light field. This function completely characterizes the flow of light through unobstructed space in a static scene with fixed illumination.},
  eventtitle = {The 23rd Annual Conference},
  isbn = {978-0-89791-746-9},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\7CXXHQT2\Levoy 그리고 Hanrahan - 1996 - Light field rendering.pdf}
}

@inproceedings{levoyLightFieldRendering1996a,
  title = {Light Field Rendering},
  booktitle = {Proceedings of the 23rd Annual Conference on {{Computer}} Graphics and Interactive Techniques  - {{SIGGRAPH}} '96},
  author = {Levoy, Marc and Hanrahan, Pat},
  date = {1996},
  pages = {31--42},
  publisher = {ACM Press},
  location = {Not Known},
  doi = {10.1145/237170.237199},
  url = {http://portal.acm.org/citation.cfm?doid=237170.237199},
  urldate = {2023-01-03},
  abstract = {A number of techniques have been proposed for flying through scenes by redisplaying previously rendered or digitized views. Techniques have also been proposed for interpolating between views by warping input images, using depth information or correspondences between multiple images. In this paper, we describe a simple and robust method for generating new views from arbitrary camera positions without depth information or feature matching, simply by combining and resampling the available images. The key to this technique lies in interpreting the input images as 2D slices of a 4D function - the light field. This function completely characterizes the flow of light through unobstructed space in a static scene with fixed illumination.},
  eventtitle = {The 23rd Annual Conference},
  isbn = {978-0-89791-746-9},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\6KLD2HSY\Levoy 그리고 Hanrahan - 1996 - Light field rendering.pdf}
}

@online{liAlignFuseVision2021,
  title = {Align before {{Fuse}}: {{Vision}} and {{Language Representation Learning}} with {{Momentum Distillation}}},
  shorttitle = {Align before {{Fuse}}},
  author = {Li, Junnan and Selvaraju, Ramprasaath R. and Gotmare, Akhilesh Deepak and Joty, Shafiq and Xiong, Caiming and Hoi, Steven},
  date = {2021-10-07},
  eprint = {2107.07651},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2107.07651},
  urldate = {2024-04-15},
  abstract = {Large-scale vision and language representation learning has shown promising improvements on various vision-language tasks. Most existing methods employ a transformer-based multimodal encoder to jointly model visual tokens (region-based image features) and word tokens. Because the visual tokens and word tokens are unaligned, it is challenging for the multimodal encoder to learn image-text interactions. In this paper, we introduce a contrastive loss to ALign the image and text representations BEfore Fusing (ALBEF) them through cross-modal attention, which enables more grounded vision and language representation learning. Unlike most existing methods, our method does not require bounding box annotations nor high-resolution images. In order to improve learning from noisy web data, we propose momentum distillation, a self-training method which learns from pseudo-targets produced by a momentum model. We provide a theoretical analysis of ALBEF from a mutual information maximization perspective, showing that different training tasks can be interpreted as different ways to generate views for an image-text pair. ALBEF achieves state-of-the-art performance on multiple downstream vision-language tasks. On image-text retrieval, ALBEF outperforms methods that are pre-trained on orders of magnitude larger datasets. On VQA and NLVR\$\textasciicircum 2\$, ALBEF achieves absolute improvements of 2.37\% and 3.84\% compared to the state-of-the-art, while enjoying faster inference speed. Code and pre-trained models are available at https://github.com/salesforce/ALBEF/.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Li et al_2021_Align before Fuse.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KKI5KYVR\\2107.html}
}

@online{liangEnhancingReliabilityOutofdistribution2020,
  title = {Enhancing {{The Reliability}} of {{Out-of-distribution Image Detection}} in {{Neural Networks}}},
  author = {Liang, Shiyu and Li, Yixuan and Srikant, R.},
  date = {2020-08-30},
  eprint = {1706.02690},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1706.02690},
  url = {http://arxiv.org/abs/1706.02690},
  urldate = {2022-09-06},
  abstract = {We consider the problem of detecting out-of-distribution images in neural networks. We propose ODIN, a simple and effective method that does not require any change to a pre-trained neural network. Our method is based on the observation that using temperature scaling and adding small perturbations to the input can separate the softmax score distributions between in- and out-of-distribution images, allowing for more effective detection. We show in a series of experiments that ODIN is compatible with diverse network architectures and datasets. It consistently outperforms the baseline approach by a large margin, establishing a new state-of-the-art performance on this task. For example, ODIN reduces the false positive rate from the baseline 34.7\% to 4.3\% on the DenseNet (applied to CIFAR-10) when the true positive rate is 95\%.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Liang et al_2020_Enhancing The Reliability of Out-of-distribution Image Detection in Neural.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PZVKJRQR\\1706.html}
}

@online{liangFoundationsTrendsMultimodal2023,
  title = {Foundations and {{Trends}} in {{Multimodal Machine Learning}}: {{Principles}}, {{Challenges}}, and {{Open Questions}}},
  shorttitle = {Foundations and {{Trends}} in {{Multimodal Machine Learning}}},
  author = {Liang, Paul Pu and Zadeh, Amir and Morency, Louis-Philippe},
  date = {2023-02-20},
  eprint = {2209.03430},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2209.03430},
  urldate = {2024-02-06},
  abstract = {Multimodal machine learning is a vibrant multi-disciplinary research field that aims to design computer agents with intelligent capabilities such as understanding, reasoning, and learning through integrating multiple communicative modalities, including linguistic, acoustic, visual, tactile, and physiological messages. With the recent interest in video understanding, embodied autonomous agents, text-to-image generation, and multisensor fusion in application domains such as healthcare and robotics, multimodal machine learning has brought unique computational and theoretical challenges to the machine learning community given the heterogeneity of data sources and the interconnections often found between modalities. However, the breadth of progress in multimodal research has made it difficult to identify the common themes and open questions in the field. By synthesizing a broad range of application domains and theoretical frameworks from both historical and recent perspectives, this paper is designed to provide an overview of the computational and theoretical foundations of multimodal machine learning. We start by defining three key principles of modality heterogeneity, connections, and interactions that have driven subsequent innovations, and propose a taxonomy of six core technical challenges: representation, alignment, reasoning, generation, transference, and quantification covering historical and recent trends. Recent technical achievements will be presented through the lens of this taxonomy, allowing researchers to understand the similarities and differences across new approaches. We end by motivating several open problems for future research as identified by our taxonomy.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {Y\:\\paper\\2024_research\\Liang et al_2023_Foundations and Trends in Multimodal Machine Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\76FPN8HZ\\2209.html}
}

@article{liangHighModalityMultimodalTransformer,
  title = {High-{{Modality Multimodal Transformer}}: {{Quantifying Modality}} \& {{Interaction Heterogeneity}} for {{High-Modality Representation Learning}}},
  author = {Liang, Paul Pu and Lyu, Yiwei and Fan, Xiang and Tsaw, Jeffrey and Liu, Yudong and Mo, Shentong and Yogatama, Dani and Morency, Louis-Philippe and Salakhutdinov, Ruslan},
  abstract = {Many real-world problems are inherently multimodal, from the communicative modalities humans use such as spoken language, gestures, and paralinguistics to the force, proprioception, and visual sensors ubiquitous on robots. While there has been an explosion of interest in multimodal representation learning, these methods are still largely focused on a small set of modalities, primarily in the language, vision, and audio space. In order to accelerate generalization towards diverse and understudied modalities, this paper studies efficient representation learning for high-modality scenarios involving a large set of diverse modalities. Since adding new models for every new modality or task becomes prohibitively expensive, a critical technical challenge is heterogeneity quantification: how can we measure which modalities encode similar information and interactions in order to permit parameter sharing with previous modalities? This paper proposes two new information theoretic metrics for heterogeneity quantification: (1) modality heterogeneity studies how similar 2 modalities \{X1, X2\} are by measuring how much information can be transferred from X1 to X2, while (2) interaction heterogeneity studies how similarly pairs of modalities \{X1, X2\}, \{X3, X4\} interact by measuring how much information can be transferred from fusing \{X1, X2\} to \{X3, X4\}. We show the importance of these 2 proposed metrics in high-modality scenarios as a way to automatically prioritize the fusion of modalities that contain unique information or interactions. The result is a single model, HighMMT, that scales up to 10 modalities (text, image, audio, video, sensors, proprioception, speech, time-series, sets, and tables) and 15 tasks from 5 research areas. Not only does HighMMT outperform prior methods on the tradeoff between performance and efficiency, it also demonstrates a crucial scaling behavior: performance continues to improve with each modality added, and it transfers to entirely new modalities and tasks during fine-tuning. We release our code and benchmarks at: https://github.com/pliang279/HighMMT.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\HIABEC72\Liang 등 - High-Modality Multimodal Transformer Quantifying .pdf}
}

@online{liangHighModalityMultimodalTransformer2023,
  title = {High-{{Modality Multimodal Transformer}}: {{Quantifying Modality}} \& {{Interaction Heterogeneity}} for {{High-Modality Representation Learning}}},
  shorttitle = {High-{{Modality Multimodal Transformer}}},
  author = {Liang, Paul Pu and Lyu, Yiwei and Fan, Xiang and Tsaw, Jeffrey and Liu, Yudong and Mo, Shentong and Yogatama, Dani and Morency, Louis-Philippe and Salakhutdinov, Ruslan},
  date = {2023-06-28},
  eprint = {2203.01311},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.01311},
  url = {http://arxiv.org/abs/2203.01311},
  urldate = {2024-02-06},
  abstract = {Many real-world problems are inherently multimodal, from spoken language, gestures, and paralinguistics humans use to communicate, to force, proprioception, and visual sensors on robots. While there has been an explosion of interest in multimodal learning, these methods are focused on a small set of modalities primarily in language, vision, and audio. In order to accelerate generalization towards diverse and understudied modalities, this paper studies efficient representation learning for high-modality scenarios involving a large set of diverse modalities. Since adding new models for every new modality becomes prohibitively expensive, a critical technical challenge is heterogeneity quantification: how can we measure which modalities encode similar information and interactions in order to permit parameter sharing with previous modalities? This paper proposes two new information theoretic metrics for heterogeneity quantification: (1) modality heterogeneity studies how similar 2 modalities \{X1,X2\} are by measuring how much information can be transferred from X1 to X2, while (2) interaction heterogeneity studies how similarly pairs of modalities \{X1,X2\}, \{X3,X4\} interact by measuring how much information can be transferred from fusing \{X1,X2\} to \{X3,X4\}. We show the importance of these 2 proposed metrics as a way to automatically prioritize the fusion of modalities that contain unique information or interactions. The result is a single model, HighMMT, that scales up to 10 modalities (text, image, audio, video, sensors, proprioception, speech, time-series, sets, and tables) and 15 tasks from 5 research areas. Not only does HighMMT outperform prior methods on the tradeoff between performance and efficiency, it also demonstrates a crucial scaling behavior: performance continues to improve with each modality added, and it transfers to entirely new modalities and tasks during fine-tuning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {Y\:\\paper\\2024_research\\Liang et al_2023_High-Modality Multimodal Transformer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GQTJJ8JR\\2203.html}
}

@online{liangLessMoreTaskaware2023,
  title = {Less Is {{More}}: {{Task-aware Layer-wise Distillation}} for {{Language Model Compression}}},
  shorttitle = {Less Is {{More}}},
  author = {Liang, Chen and Zuo, Simiao and Zhang, Qingru and He, Pengcheng and Chen, Weizhu and Zhao, Tuo},
  date = {2023-06-05},
  eprint = {2210.01351},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2210.01351},
  urldate = {2024-04-17},
  abstract = {Layer-wise distillation is a powerful tool to compress large models (i.e. teacher models) into small ones (i.e., student models). The student distills knowledge from the teacher by mimicking the hidden representations of the teacher at every intermediate layer. However, layer-wise distillation is difficult. Since the student has a smaller model capacity than the teacher, it is often under-fitted. Furthermore, the hidden representations of the teacher contain redundant information that the student does not necessarily need for the target task's learning. To address these challenges, we propose a novel Task-aware layEr-wise Distillation (TED). TED designs task-aware filters to align the hidden representations of the student and the teacher at each layer. The filters select the knowledge that is useful for the target task from the hidden representations. As such, TED reduces the knowledge gap between the two models and helps the student to fit better on the target task. We evaluate TED in two scenarios: continual pre-training and fine-tuning. TED demonstrates significant and consistent improvements over existing distillation methods in both scenarios. Code is available at https://github.com/cliang1453/task-aware-distillation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Liang et al_2023_Less is More.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LE9AWQWG\\2210.html}
}

@online{liangMultimodalLearningLabeled2023,
  title = {Multimodal {{Learning Without Labeled Multimodal Data}}: {{Guarantees}} and {{Applications}}},
  shorttitle = {Multimodal {{Learning Without Labeled Multimodal Data}}},
  author = {Liang, Paul Pu and Ling, Chun Kai and Cheng, Yun and Obolenskiy, Alex and Liu, Yudong and Pandey, Rohan and Wilf, Alex and Morency, Louis-Philippe and Salakhutdinov, Ruslan},
  date = {2023-06-07},
  eprint = {2306.04539},
  eprinttype = {arXiv},
  eprintclass = {cs, math, stat},
  url = {http://arxiv.org/abs/2306.04539},
  urldate = {2024-05-07},
  abstract = {In many machine learning systems that jointly learn from multiple modalities, a core research question is to understand the nature of multimodal interactions: the emergence of new task-relevant information during learning from both modalities that was not present in either alone. We study this challenge of interaction quantification in a semi-supervised setting with only labeled unimodal data and naturally co-occurring multimodal data (e.g., unlabeled images and captions, video and corresponding audio) but when labeling them is time-consuming. Using a precise information-theoretic definition of interactions, our key contributions are the derivations of lower and upper bounds to quantify the amount of multimodal interactions in this semi-supervised setting. We propose two lower bounds based on the amount of shared information between modalities and the disagreement between separately trained unimodal classifiers, and derive an upper bound through connections to approximate algorithms for min-entropy couplings. We validate these estimated bounds and show how they accurately track true interactions. Finally, two semisupervised multimodal applications are explored based on these theoretical results: (1) analyzing the relationship between multimodal performance and estimated interactions, and (2) self-supervised learning that embraces disagreement between modalities beyond agreement as is typically done.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Information Theory,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y:\paper\2024_research\Liang et al_2023_Multimodal Learning Without Labeled Multimodal Data.pdf}
}

@online{liangQuantifyingModelingMultimodal2023,
  title = {Quantifying \& {{Modeling Multimodal Interactions}}: {{An Information Decomposition Framework}}},
  shorttitle = {Quantifying \& {{Modeling Multimodal Interactions}}},
  author = {Liang, Paul Pu and Cheng, Yun and Fan, Xiang and Ling, Chun Kai and Nie, Suzanne and Chen, Richard and Deng, Zihao and Allen, Nicholas and Auerbach, Randy and Mahmood, Faisal and Salakhutdinov, Ruslan and Morency, Louis-Philippe},
  date = {2023-12-10},
  eprint = {2302.12247},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/2302.12247},
  urldate = {2024-05-13},
  abstract = {The recent explosion of interest in multimodal applications has resulted in a wide selection of datasets and methods for representing and integrating information from different modalities. Despite these empirical advances, there remain fundamental research questions: How can we quantify the interactions that are necessary to solve a multimodal task? Subsequently, what are the most suitable multimodal models to capture these interactions? To answer these questions, we propose an information-theoretic approach to quantify the degree of redundancy, uniqueness, and synergy relating input modalities with an output task. We term these three measures as the PID statistics of a multimodal distribution (or PID for short), and introduce two new estimators for these PID statistics that scale to high-dimensional distributions. To validate PID estimation, we conduct extensive experiments on both synthetic datasets where the PID is known and on large-scale multimodal benchmarks where PID estimations are compared with human annotations. Finally, we demonstrate their usefulness in (1) quantifying interactions within multimodal datasets, (2) quantifying interactions captured by multimodal models, (3) principled approaches for model selection, and (4) three real-world case studies engaging with domain experts in pathology, mood prediction, and robotic perception where our framework helps to recommend strong multimodal models for each application.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Information Theory,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Liang et al_2023_Quantifying & Modeling Multimodal Interactions.pdf}
}

@online{liBLIP2BootstrappingLanguageImage2023,
  title = {{{BLIP-2}}: {{Bootstrapping Language-Image Pre-training}} with {{Frozen Image Encoders}} and {{Large Language Models}}},
  shorttitle = {{{BLIP-2}}},
  author = {Li, Junnan and Li, Dongxu and Savarese, Silvio and Hoi, Steven},
  date = {2023-05-01},
  eprint = {2301.12597},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2301.12597},
  url = {http://arxiv.org/abs/2301.12597},
  urldate = {2023-05-27},
  abstract = {The cost of vision-and-language pre-training has become increasingly prohibitive due to end-to-end training of large-scale models. This paper proposes BLIP-2, a generic and efficient pre-training strategy that bootstraps vision-language pre-training from off-the-shelf frozen pre-trained image encoders and frozen large language models. BLIP-2 bridges the modality gap with a lightweight Querying Transformer, which is pre-trained in two stages. The first stage bootstraps vision-language representation learning from a frozen image encoder. The second stage bootstraps vision-to-language generative learning from a frozen language model. BLIP-2 achieves state-of-the-art performance on various vision-language tasks, despite having significantly fewer trainable parameters than existing methods. For example, our model outperforms Flamingo80B by 8.7\% on zero-shot VQAv2 with 54x fewer trainable parameters. We also demonstrate the model's emerging capabilities of zero-shot image-to-text generation that can follow natural language instructions.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\Li et al_2023_BLIP-2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HILJPJUW\\2301.html}
}

@online{liExploringBenefitsVisual2023,
  title = {Exploring the {{Benefits}} of {{Visual Prompting}} in {{Differential Privacy}}},
  author = {Li, Yizhe and Tsai, Yu-Lin and Ren, Xuebin and Yu, Chia-Mu and Chen, Pin-Yu},
  date = {2023-08-30},
  eprint = {2303.12247},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.12247},
  url = {http://arxiv.org/abs/2303.12247},
  urldate = {2023-11-06},
  abstract = {Visual Prompting (VP) is an emerging and powerful technique that allows sample-efficient adaptation to downstream tasks by engineering a well-trained frozen source model. In this work, we explore the benefits of VP in constructing compelling neural network classifiers with differential privacy (DP). We explore and integrate VP into canonical DP training methods and demonstrate its simplicity and efficiency. In particular, we discover that VP in tandem with PATE, a state-of-the-art DP training method that leverages the knowledge transfer from an ensemble of teachers, achieves the state-of-the-art privacy-utility trade-off with minimum expenditure of privacy budget. Moreover, we conduct additional experiments on cross-domain image classification with a sufficient domain gap to further unveil the advantage of VP in DP. Lastly, we also conduct extensive ablation studies to validate the effectiveness and contribution of VP under DP consideration. Our code is available at (https://github.com/EzzzLi/Prompt-PATE).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Cryptography and Security,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Li et al_2023_Exploring the Benefits of Visual Prompting in Differential Privacy.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6MF4E33E\\2303.html}
}

@online{liExploringPlainVision2022,
  title = {Exploring {{Plain Vision Transformer Backbones}} for {{Object Detection}}},
  author = {Li, Yanghao and Mao, Hanzi and Girshick, Ross and He, Kaiming},
  date = {2022-06-10},
  eprint = {2203.16527},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.16527},
  url = {http://arxiv.org/abs/2203.16527},
  urldate = {2023-11-22},
  abstract = {We explore the plain, non-hierarchical Vision Transformer (ViT) as a backbone network for object detection. This design enables the original ViT architecture to be fine-tuned for object detection without needing to redesign a hierarchical backbone for pre-training. With minimal adaptations for fine-tuning, our plain-backbone detector can achieve competitive results. Surprisingly, we observe: (i) it is sufficient to build a simple feature pyramid from a single-scale feature map (without the common FPN design) and (ii) it is sufficient to use window attention (without shifting) aided with very few cross-window propagation blocks. With plain ViT backbones pre-trained as Masked Autoencoders (MAE), our detector, named ViTDet, can compete with the previous leading methods that were all based on hierarchical backbones, reaching up to 61.3 AP\_box on the COCO dataset using only ImageNet-1K pre-training. We hope our study will draw attention to research on plain-backbone detectors. Code for ViTDet is available in Detectron2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Li et al_2022_Exploring Plain Vision Transformer Backbones for Object Detection.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UIP8NGRQ\\2203.html}
}

@inproceedings{liGradientRegulatedMetaPromptLearning2023,
  title = {Gradient-{{Regulated Meta-Prompt Learning}} for {{Generalizable Vision-Language Models}}},
  author = {Li, Juncheng and Gao, Minghe and Wei, Longhui and Tang, Siliang and Zhang, Wenqiao and Li, Mengze and Ji, Wei and Tian, Qi and Chua, Tat-Seng and Zhuang, Yueting},
  date = {2023},
  pages = {2551--2562},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Li_Gradient-Regulated_Meta-Prompt_Learning_for_Generalizable_Vision-Language_Models_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Li et al_2023_Gradient-Regulated Meta-Prompt Learning for Generalizable Vision-Language Models.pdf}
}

@online{liLearningAnswerQuestions2022,
  title = {Learning to {{Answer Questions}} in {{Dynamic Audio-Visual Scenarios}}},
  author = {Li, Guangyao and Wei, Yake and Tian, Yapeng and Xu, Chenliang and Wen, Ji-Rong and Hu, Di},
  date = {2022-04-05},
  eprint = {2203.14072},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.14072},
  url = {http://arxiv.org/abs/2203.14072},
  urldate = {2024-07-05},
  abstract = {In this paper, we focus on the Audio-Visual Question Answering (AVQA) task, which aims to answer questions regarding different visual objects, sounds, and their associations in videos. The problem requires comprehensive multimodal understanding and spatio-temporal reasoning over audio-visual scenes. To benchmark this task and facilitate our study, we introduce a large-scale MUSIC-AVQA dataset, which contains more than 45K question-answer pairs covering 33 different question templates spanning over different modalities and question types. We develop several baselines and introduce a spatio-temporal grounded audio-visual network for the AVQA problem. Our results demonstrate that AVQA benefits from multisensory perception and our model outperforms recent A-, V-, and AVQA approaches. We believe that our built dataset has the potential to serve as testbed for evaluating and promoting progress in audio-visual scene understanding and spatio-temporal reasoning. Code and dataset: http://gewu-lab.github.io/MUSIC-AVQA/},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C\:\\Users\\chsey\\Zotero\\storage\\K9JVLHVF\\Li 등 - 2022 - Learning to Answer Questions in Dynamic Audio-Visu.pdf;Y\:\\paper\\2024_research\\Li et al_2022_Learning to Answer Questions in Dynamic Audio-Visual Scenarios.pdf;C\:\\Users\\chsey\\Zotero\\storage\\D5REUTAQ\\2203.html}
}

@online{liLearningForgetting2017,
  title = {Learning without {{Forgetting}}},
  author = {Li, Zhizhong and Hoiem, Derek},
  date = {2017-02-14},
  eprint = {1606.09282},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1606.09282},
  url = {http://arxiv.org/abs/1606.09282},
  urldate = {2023-08-05},
  abstract = {When building a unified vision system or gradually adding new capabilities to a system, the usual assumption is that training data for all tasks is always available. However, as the number of tasks grows, storing and retraining on such data becomes infeasible. A new problem arises where we add new capabilities to a Convolutional Neural Network (CNN), but the training data for its existing capabilities are unavailable. We propose our Learning without Forgetting method, which uses only new task data to train the network while preserving the original capabilities. Our method performs favorably compared to commonly used feature extraction and fine-tuning adaption techniques and performs similarly to multitask learning that uses original task data we assume unavailable. A more surprising observation is that Learning without Forgetting may be able to replace fine-tuning with similar old and new task datasets for improved new task performance.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\relational reasoning\\Li_Hoiem_2017_Learning without Forgetting.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y4QC5REN\\1606.html}
}

@online{liLearningForgetting2017a,
  title = {Learning without {{Forgetting}}},
  author = {Li, Zhizhong and Hoiem, Derek},
  date = {2017-02-14},
  eprint = {1606.09282},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1606.09282},
  url = {http://arxiv.org/abs/1606.09282},
  urldate = {2023-08-05},
  abstract = {When building a unified vision system or gradually adding new capabilities to a system, the usual assumption is that training data for all tasks is always available. However, as the number of tasks grows, storing and retraining on such data becomes infeasible. A new problem arises where we add new capabilities to a Convolutional Neural Network (CNN), but the training data for its existing capabilities are unavailable. We propose our Learning without Forgetting method, which uses only new task data to train the network while preserving the original capabilities. Our method performs favorably compared to commonly used feature extraction and fine-tuning adaption techniques and performs similarly to multitask learning that uses original task data we assume unavailable. A more surprising observation is that Learning without Forgetting may be able to replace fine-tuning with similar old and new task datasets for improved new task performance.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\lifelong learning\\Li_Hoiem_2017_Learning without Forgetting.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JXIGQ9MN\\1606.html}
}

@article{liLearningObjectContext2019,
  title = {Learning {{Object Context}} for {{Dense Captioning}}},
  author = {Li, Xiangyang and Jiang, Shuqiang and Han, Jungong},
  date = {2019-07-17},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {33},
  number = {01},
  pages = {8650--8657},
  issn = {2374-3468},
  doi = {10.1609/aaai.v33i01.33018650},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/4886},
  urldate = {2023-05-29},
  abstract = {Dense captioning is a challenging task which not only detects visual elements in images but also generates natural language sentences to describe them. Previous approaches do not leverage object information in images for this task. However, objects provide valuable cues to help predict the locations of caption regions as caption regions often highly overlap with objects (i.e. caption regions are usually parts of objects or combinations of them). Meanwhile, objects also provide important information for describing a target caption region as the corresponding description not only depicts its properties, but also involves its interactions with objects in the image. In this work, we propose a novel scheme with an object context encoding Long Short-Term Memory (LSTM) network to automatically learn complementary object context for each caption region, transferring knowledge from objects to caption regions. All contextual objects are arranged as a sequence and progressively fed into the context encoding module to obtain context features. Then both the learned object context features and region features are used to predict the bounding box offsets and generate the descriptions. The context learning procedure is in conjunction with the optimization of both location prediction and caption generation, thus enabling the object context encoding LSTM to capture and aggregate useful object context. Experiments on benchmark datasets demonstrate the superiority of our proposed approach over the state-of-the-art methods.},
  issue = {01},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\dense captioning\Li et al_2019_Learning Object Context for Dense Captioning.pdf}
}

@online{liMeasuringIntrinsicDimension2018,
  title = {Measuring the {{Intrinsic Dimension}} of {{Objective Landscapes}}},
  author = {Li, Chunyuan and Farkhoor, Heerad and Liu, Rosanne and Yosinski, Jason},
  date = {2018-04-24},
  eprint = {1804.08838},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1804.08838},
  url = {http://arxiv.org/abs/1804.08838},
  urldate = {2024-04-14},
  abstract = {Many recently trained neural networks employ large numbers of parameters to achieve good performance. One may intuitively use the number of parameters required as a rough gauge of the difficulty of a problem. But how accurate are such notions? How many parameters are really needed? In this paper we attempt to answer this question by training networks not in their native parameter space, but instead in a smaller, randomly oriented subspace. We slowly increase the dimension of this subspace, note at which dimension solutions first appear, and define this to be the intrinsic dimension of the objective landscape. The approach is simple to implement, computationally tractable, and produces several suggestive conclusions. Many problems have smaller intrinsic dimensions than one might suspect, and the intrinsic dimension for a given dataset varies little across a family of models with vastly different sizes. This latter result has the profound implication that once a parameter space is large enough to solve a problem, extra parameters serve directly to increase the dimensionality of the solution manifold. Intrinsic dimension allows some quantitative comparison of problem difficulty across supervised, reinforcement, and other types of learning where we conclude, for example, that solving the inverted pendulum problem is 100 times easier than classifying digits from MNIST, and playing Atari Pong from pixels is about as hard as classifying CIFAR-10. In addition to providing new cartography of the objective landscapes wandered by parameterized models, the method is a simple technique for constructively obtaining an upper bound on the minimum description length of a solution. A byproduct of this construction is a simple approach for compressing networks, in some cases by more than 100 times.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Li et al_2018_Measuring the Intrinsic Dimension of Objective Landscapes.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GLJ3YXQY\\1804.html}
}

@online{liMPLUGEffectiveEfficient2022,
  title = {{{mPLUG}}: {{Effective}} and {{Efficient Vision-Language Learning}} by {{Cross-modal Skip-connections}}},
  shorttitle = {{{mPLUG}}},
  author = {Li, Chenliang and Xu, Haiyang and Tian, Junfeng and Wang, Wei and Yan, Ming and Bi, Bin and Ye, Jiabo and Chen, Hehong and Xu, Guohai and Cao, Zheng and Zhang, Ji and Huang, Songfang and Huang, Fei and Zhou, Jingren and Si, Luo},
  date = {2022-05-25},
  eprint = {2205.12005},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.12005},
  urldate = {2024-03-13},
  abstract = {Large-scale pretrained foundation models have been an emerging paradigm for building artificial intelligence (AI) systems, which can be quickly adapted to a wide range of downstream tasks. This paper presents mPLUG, a new vision-language foundation model for both cross-modal understanding and generation. Most existing pre-trained models suffer from the problems of low computational efficiency and information asymmetry brought by the long visual sequence in cross-modal alignment. To address these problems, mPLUG introduces an effective and efficient vision-language architecture with novel cross-modal skip-connections, which creates inter-layer shortcuts that skip a certain number of layers for time-consuming full self-attention on the vision side. mPLUG is pre-trained end-to-end on large-scale image-text pairs with both discriminative and generative objectives. It achieves state-of-the-art results on a wide range of vision-language downstream tasks, such as image captioning, image-text retrieval, visual grounding and visual question answering. mPLUG also demonstrates strong zero-shot transferability when directly transferred to multiple video-language tasks.},
  pubstate = {prepublished},
  version = {2},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Li et al_2022_mPLUG.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V2FEMDQM\\2205.html}
}

@article{lindenFlyingGeeseMoving1998,
  title = {Flying {{Geese}} as {{Moving Targets}}: {{Are Korea}} and {{Taiwan Catching}} up with {{Japan}} in {{Advanced Displays}}?},
  author = {Linden, Greg and Hart, Jeffrey and Lenway, Stefanie Ann and Murtha, Thomas P.},
  date = {1998},
  journaltitle = {Industry and Innovation},
  volume = {5},
  number = {1},
  pages = {11--34},
  doi = {10.1080/13662719800000002}
}

@online{liNeural3DVideo2022,
  title = {Neural {{3D Video Synthesis}} from {{Multi-view Video}}},
  author = {Li, Tianye and Slavcheva, Mira and Zollhoefer, Michael and Green, Simon and Lassner, Christoph and Kim, Changil and Schmidt, Tanner and Lovegrove, Steven and Goesele, Michael and Newcombe, Richard and Lv, Zhaoyang},
  date = {2022-05-02},
  eprint = {2103.02597},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2103.02597},
  url = {http://arxiv.org/abs/2103.02597},
  urldate = {2023-01-24},
  abstract = {We propose a novel approach for 3D video synthesis that is able to represent multi-view video recordings of a dynamic real-world scene in a compact, yet expressive representation that enables high-quality view synthesis and motion interpolation. Our approach takes the high quality and compactness of static neural radiance fields in a new direction: to a model-free, dynamic setting. At the core of our approach is a novel time-conditioned neural radiance field that represents scene dynamics using a set of compact latent codes. We are able to significantly boost the training speed and perceptual quality of the generated imagery by a novel hierarchical training scheme in combination with ray importance sampling. Our learned representation is highly compact and able to represent a 10 second 30 FPS multiview video recording by 18 cameras with a model size of only 28MB. We demonstrate that our method can render high-fidelity wide-angle novel views at over 1K resolution, even for complex and dynamic scenes. We perform an extensive qualitative and quantitative evaluation that shows that our approach outperforms the state of the art. Project website: https://neural-3d-video.github.io/.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Li et al_2022_Neural 3D Video Synthesis from Multi-view Video.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UNRCQWNT\\2103.html}
}

@online{lingRegionawareAdaptiveInstance2021,
  title = {Region-Aware {{Adaptive Instance Normalization}} for {{Image Harmonization}}},
  author = {Ling, Jun and Xue, Han and Song, Li and Xie, Rong and Gu, Xiao},
  date = {2021-06-05},
  eprint = {2106.02853},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.02853},
  urldate = {2022-11-28},
  abstract = {Image composition plays a common but important role in photo editing. To acquire photo-realistic composite images, one must adjust the appearance and visual style of the foreground to be compatible with the background. Existing deep learning methods for harmonizing composite images directly learn an image mapping network from the composite to the real one, without explicit exploration on visual style consistency between the background and the foreground images. To ensure the visual style consistency between the foreground and the background, in this paper, we treat image harmonization as a style transfer problem. In particular, we propose a simple yet effective Region-aware Adaptive Instance Normalization (RAIN) module, which explicitly formulates the visual style from the background and adaptively applies them to the foreground. With our settings, our RAIN module can be used as a drop-in module for existing image harmonization networks and is able to bring significant improvements. Extensive experiments on the existing image harmonization benchmark datasets show the superior capability of the proposed method. Code is available at \{https://github.com/junleen/RainNet\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\traditional\\PA3\\Ling et al_2021_Region-aware Adaptive Instance Normalization for Image Harmonization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FHDSQSLY\\2106.html}
}

@inproceedings{linMicrosoftCOCOCommon2014,
  title = {Microsoft {{COCO}}: {{Common Objects}} in {{Context}}},
  shorttitle = {Microsoft {{COCO}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2014},
  author = {Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Dollár, Piotr and Zitnick, C. Lawrence},
  editor = {Fleet, David and Pajdla, Tomas and Schiele, Bernt and Tuytelaars, Tinne},
  date = {2014},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {740--755},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-319-10602-1_48},
  abstract = {We present a new dataset with the goal of advancing the state-of-the-art in object recognition by placing the question of object recognition in the context of the broader question of scene understanding. This is achieved by gathering images of complex everyday scenes containing common objects in their natural context. Objects are labeled using per-instance segmentations to aid in precise object localization. Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old. With a total of 2.5 million labeled instances in 328k images, the creation of our dataset drew upon extensive crowd worker involvement via novel user interfaces for category detection, instance spotting and instance segmentation. We present a detailed statistical analysis of the dataset in comparison to PASCAL, ImageNet, and SUN. Finally, we provide baseline performance analysis for bounding box and segmentation detection results using a Deformable Parts Model.},
  isbn = {978-3-319-10602-1},
  langid = {english},
  keywords = {Common Object,Object Category,Object Detection,Object Instance,Scene Understanding},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Lin et al_2014_Microsoft COCO.pdf}
}

@online{linMicrosoftCOCOCommon2015,
  title = {Microsoft {{COCO}}: {{Common Objects}} in {{Context}}},
  shorttitle = {Microsoft {{COCO}}},
  author = {Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Bourdev, Lubomir and Girshick, Ross and Hays, James and Perona, Pietro and Ramanan, Deva and Zitnick, C. Lawrence and Dollár, Piotr},
  date = {2015-02-20},
  eprint = {1405.0312},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1405.0312},
  url = {http://arxiv.org/abs/1405.0312},
  urldate = {2023-11-18},
  abstract = {We present a new dataset with the goal of advancing the state-of-the-art in object recognition by placing the question of object recognition in the context of the broader question of scene understanding. This is achieved by gathering images of complex everyday scenes containing common objects in their natural context. Objects are labeled using per-instance segmentations to aid in precise object localization. Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old. With a total of 2.5 million labeled instances in 328k images, the creation of our dataset drew upon extensive crowd worker involvement via novel user interfaces for category detection, instance spotting and instance segmentation. We present a detailed statistical analysis of the dataset in comparison to PASCAL, ImageNet, and SUN. Finally, we provide baseline performance analysis for bounding box and segmentation detection results using a Deformable Parts Model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\Lin et al_2015_Microsoft COCO.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XH2LUESZ\\1405.html}
}

@online{linMicrosoftCOCOCommon2015a,
  title = {Microsoft {{COCO}}: {{Common Objects}} in {{Context}}},
  shorttitle = {Microsoft {{COCO}}},
  author = {Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Bourdev, Lubomir and Girshick, Ross and Hays, James and Perona, Pietro and Ramanan, Deva and Zitnick, C. Lawrence and Dollár, Piotr},
  date = {2015-02-20},
  eprint = {1405.0312},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1405.0312},
  url = {http://arxiv.org/abs/1405.0312},
  urldate = {2023-05-29},
  abstract = {We present a new dataset with the goal of advancing the state-of-the-art in object recognition by placing the question of object recognition in the context of the broader question of scene understanding. This is achieved by gathering images of complex everyday scenes containing common objects in their natural context. Objects are labeled using per-instance segmentations to aid in precise object localization. Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old. With a total of 2.5 million labeled instances in 328k images, the creation of our dataset drew upon extensive crowd worker involvement via novel user interfaces for category detection, instance spotting and instance segmentation. We present a detailed statistical analysis of the dataset in comparison to PASCAL, ImageNet, and SUN. Finally, we provide baseline performance analysis for bounding box and segmentation detection results using a Deformable Parts Model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Lin et al_2015_Microsoft COCO.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MK8N3E9B\\1405.html}
}

@online{liPrefixTuningOptimizingContinuous2021,
  title = {Prefix-{{Tuning}}: {{Optimizing Continuous Prompts}} for {{Generation}}},
  shorttitle = {Prefix-{{Tuning}}},
  author = {Li, Xiang Lisa and Liang, Percy},
  date = {2021-01-01},
  eprint = {2101.00190},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2101.00190},
  urldate = {2023-08-25},
  abstract = {Fine-tuning is the de facto way to leverage large pretrained language models to perform downstream tasks. However, it modifies all the language model parameters and therefore necessitates storing a full copy for each task. In this paper, we propose prefix-tuning, a lightweight alternative to fine-tuning for natural language generation tasks, which keeps language model parameters frozen, but optimizes a small continuous task-specific vector (called the prefix). Prefix-tuning draws inspiration from prompting, allowing subsequent tokens to attend to this prefix as if it were "virtual tokens". We apply prefix-tuning to GPT-2 for table-to-text generation and to BART for summarization. We find that by learning only 0.1\textbackslash\% of the parameters, prefix-tuning obtains comparable performance in the full data setting, outperforms fine-tuning in low-data settings, and extrapolates better to examples with topics unseen during training.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\CJ_paper\\Li_Liang_2021_Prefix-Tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UZJCXX5D\\2101.html}
}

@online{liScalingLanguageImagePretraining2023,
  title = {Scaling {{Language-Image Pre-training}} via {{Masking}}},
  author = {Li, Yanghao and Fan, Haoqi and Hu, Ronghang and Feichtenhofer, Christoph and He, Kaiming},
  date = {2023-03-30},
  eprint = {2212.00794},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2212.00794},
  url = {http://arxiv.org/abs/2212.00794},
  urldate = {2023-07-04},
  abstract = {We present Fast Language-Image Pre-training (FLIP), a simple and more efficient method for training CLIP. Our method randomly masks out and removes a large portion of image patches during training. Masking allows us to learn from more image-text pairs given the same wall-clock time and contrast more samples per iteration with similar memory footprint. It leads to a favorable trade-off between accuracy and training time. In our experiments on 400 million image-text pairs, FLIP improves both accuracy and speed over the no-masking baseline. On a large diversity of downstream tasks, FLIP dominantly outperforms the CLIP counterparts trained on the same data. Facilitated by the speedup, we explore the scaling behavior of increasing the model size, data size, or training length, and report encouraging results and comparisons. We hope that our work will foster future research on scaling vision-language learning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Li et al_2023_Scaling Language-Image Pre-training via Masking.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NIAK35LY\\2212.html}
}

@article{liSurveySingleImage2020,
  title = {Survey of Single Image Super-Resolution Reconstruction},
  author = {Li, Kai and Yang, Shenghao and Dong, Runting and Wang, Xiaoying and Huang, Jianqiang},
  date = {2020},
  journaltitle = {IET Image Processing},
  volume = {14},
  number = {11},
  pages = {2273--2290},
  issn = {1751-9667},
  doi = {10.1049/iet-ipr.2019.1438},
  url = {https://onlinelibrary.wiley.com/doi/abs/10.1049/iet-ipr.2019.1438},
  urldate = {2022-09-28},
  abstract = {Image super-resolution reconstruction refers to a technique of recovering a high-resolution (HR) image (or multiple images) from a low-resolution (LR) degraded image (or multiple images). Due to the breakthrough progress in deep learning in other computer vision tasks, people try to introduce deep neural network and solve the problem of image super-resolution reconstruction by constructing a deep-level network for end-to-end training. The currently used deep learning models can divide the SISR model into four types: interpolation-based preprocessing-based model, original image processing based model, hierarchical feature-based model, and high-frequency detail-based model, or shared the network model. The current challenges for super-resolution reconstruction are mainly reflected in the actual application process, such as encountering an unknown scaling factor, losing paired LR–HR images, and so on.},
  langid = {english},
  keywords = {computer vision,deep neural network,deep-level network,feature extraction,GAN-based deep learning method,generative adversarial network,hierarchical feature-based model,hyperspectral imaging,image input information,image processing,image reconstruction,image resolution,interpolation,learning (artificial intelligence),LR images,LR–HR images,medical imaging,multiscale super-resolution reconstruction,network model,neural nets,or multiple images,original image processing-based model,popular CNN-based deep learning method,remote sensing,single image super-resolution reconstruction,super-resolution images},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Li et al_2020_Survey of single image super-resolution reconstruction.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5VJRMTU5\\iet-ipr.2019.html}
}

@online{liSurveyTransformersReinforcement2023,
  title = {A {{Survey}} on {{Transformers}} in {{Reinforcement Learning}}},
  author = {Li, Wenzhe and Luo, Hao and Lin, Zichuan and Zhang, Chongjie and Lu, Zongqing and Ye, Deheng},
  date = {2023-09-20},
  eprint = {2301.03044},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2301.03044},
  url = {http://arxiv.org/abs/2301.03044},
  urldate = {2024-05-08},
  abstract = {Transformer has been considered the dominating neural architecture in NLP and CV, mostly under supervised settings. Recently, a similar surge of using Transformers has appeared in the domain of reinforcement learning (RL), but it is faced with unique design choices and challenges brought by the nature of RL. However, the evolution of Transformers in RL has not yet been well unraveled. In this paper, we seek to systematically review motivations and progress on using Transformers in RL, provide a taxonomy on existing works, discuss each sub-field, and summarize future prospects.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Li et al_2023_A Survey on Transformers in Reinforcement Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\R7B3A7GF\\2301.html}
}

@online{liuDARTSDifferentiableArchitecture2019,
  title = {{{DARTS}}: {{Differentiable Architecture Search}}},
  shorttitle = {{{DARTS}}},
  author = {Liu, Hanxiao and Simonyan, Karen and Yang, Yiming},
  date = {2019-04-23},
  eprint = {1806.09055},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1806.09055},
  url = {http://arxiv.org/abs/1806.09055},
  urldate = {2023-08-05},
  abstract = {This paper addresses the scalability challenge of architecture search by formulating the task in a differentiable manner. Unlike conventional approaches of applying evolution or reinforcement learning over a discrete and non-differentiable search space, our method is based on the continuous relaxation of the architecture representation, allowing efficient search of the architecture using gradient descent. Extensive experiments on CIFAR-10, ImageNet, Penn Treebank and WikiText-2 show that our algorithm excels in discovering high-performance convolutional architectures for image classification and recurrent architectures for language modeling, while being orders of magnitude faster than state-of-the-art non-differentiable techniques. Our implementation has been made publicly available to facilitate further research on efficient architecture search algorithms.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\neural architecture search\\Liu et al_2019_DARTS.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8ZW4RQWF\\1806.html}
}

@online{liuExplicitVisualPrompting2023,
  title = {Explicit {{Visual Prompting}} for {{Low-Level Structure Segmentations}}},
  author = {Liu, Weihuang and Shen, Xi and Pun, Chi-Man and Cun, Xiaodong},
  date = {2023-03-21},
  eprint = {2303.10883},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.10883},
  url = {http://arxiv.org/abs/2303.10883},
  urldate = {2023-08-07},
  abstract = {We consider the generic problem of detecting low-level structures in images, which includes segmenting the manipulated parts, identifying out-of-focus pixels, separating shadow regions, and detecting concealed objects. Whereas each such topic has been typically addressed with a domain-specific solution, we show that a unified approach performs well across all of them. We take inspiration from the widely-used pre-training and then prompt tuning protocols in NLP and propose a new visual prompting model, named Explicit Visual Prompting (EVP). Different from the previous visual prompting which is typically a dataset-level implicit embedding, our key insight is to enforce the tunable parameters focusing on the explicit visual content from each individual image, i.e., the features from frozen patch embeddings and the input's high-frequency components. The proposed EVP significantly outperforms other parameter-efficient tuning protocols under the same amount of tunable parameters (5.7\% extra trainable parameters of each task). EVP also achieves state-of-the-art performances on diverse low-level structure segmentation tasks compared to task-specific solutions. Our code is available at: https://github.com/NiFangBaAGe/Explicit-Visual-Prompt.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Liu et al_2023_Explicit Visual Prompting for Low-Level Structure Segmentations.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FH4NN8SQ\\2303.html}
}

@inproceedings{liuExploringInterChannelCorrelation2021,
  title = {Exploring {{Inter-Channel Correlation}} for {{Diversity-Preserved Knowledge Distillation}}},
  author = {Liu, Li and Huang, Qingle and Lin, Sihao and Xie, Hongwei and Wang, Bing and Chang, Xiaojun and Liang, Xiaodan},
  date = {2021},
  pages = {8271--8280},
  url = {https://openaccess.thecvf.com/content/ICCV2021/html/Liu_Exploring_Inter-Channel_Correlation_for_Diversity-Preserved_Knowledge_Distillation_ICCV_2021_paper.html},
  urldate = {2023-10-18},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Liu et al_2021_Exploring Inter-Channel Correlation for Diversity-Preserved Knowledge.pdf}
}

@online{liuFewShotParameterEfficientFineTuning2022,
  title = {Few-{{Shot Parameter-Efficient Fine-Tuning}} Is {{Better}} and {{Cheaper}} than {{In-Context Learning}}},
  author = {Liu, Haokun and Tam, Derek and Muqeeth, Mohammed and Mohta, Jay and Huang, Tenghao and Bansal, Mohit and Raffel, Colin},
  date = {2022-08-26},
  eprint = {2205.05638},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2205.05638},
  urldate = {2023-12-24},
  abstract = {Few-shot in-context learning (ICL) enables pre-trained language models to perform a previously-unseen task without any gradient-based training by feeding a small number of training examples as part of the input. ICL incurs substantial computational, memory, and storage costs because it involves processing all of the training examples every time a prediction is made. Parameter-efficient fine-tuning (PEFT) (e.g. adapter modules, prompt tuning, sparse update methods, etc.) offers an alternative paradigm where a small set of parameters are trained to enable a model to perform the new task. In this paper, we rigorously compare few-shot ICL and PEFT and demonstrate that the latter offers better accuracy as well as dramatically lower computational costs. Along the way, we introduce a new PEFT method called (IA)\$\textasciicircum 3\$ that scales activations by learned vectors, attaining stronger performance while only introducing a relatively tiny amount of new parameters. We also propose a simple recipe based on the T0 model called T-Few that can be applied to new tasks without task-specific tuning or modifications. We validate the effectiveness of T-Few on completely unseen tasks by applying it to the RAFT benchmark, attaining super-human performance for the first time and outperforming the state-of-the-art by 6\% absolute. All of the code used in our experiments is publicly available.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Liu et al_2022_Few-Shot Parameter-Efficient Fine-Tuning is Better and Cheaper than In-Context.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FY6996H2\\2205.html}
}

@article{liuHierarchicalPromptLearning,
  title = {Hierarchical {{Prompt Learning}} for {{Multi-Task Learning}}},
  author = {Liu, Yajing and Lu, Yuning and Liu, Hao and An, Yaozu and Xu, Zhuoran and Yao, Zhuokun and Zhang, Baofeng and Xiong, Zhiwei and Gui, Chenguang},
  abstract = {Vision-language models (VLMs) can effectively transfer to various vision tasks via prompt learning. Real-world scenarios often require adapting a model to multiple similar yet distinct tasks. Existing methods focus on learning a specific prompt for each task, limiting the ability to exploit potentially shared information from other tasks. Naively training a task-shared prompt using a combination of all tasks ignores fine-grained task correlations. Significant discrepancies across tasks could cause negative transferring. Considering this, we present Hierarchical Prompt (HiPro) learning, a simple and effective method for jointly adapting a pre-trained VLM to multiple downstream tasks. Our method quantifies inter-task affinity and subsequently constructs a hierarchical task tree. Task-shared prompts learned by internal nodes explore the information within the corresponding task group, while task-individual prompts learned by leaf nodes obtain fine-grained information targeted at each task. The combination of hierarchical prompts provides high-quality content of different granularity. We evaluate HiPro on four multi-task learning datasets. The results demonstrate the effectiveness of our method.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\Liu et al_Hierarchical Prompt Learning for Multi-Task Learning.pdf}
}

@online{liuLLMQATDataFreeQuantization2023,
  title = {{{LLM-QAT}}: {{Data-Free Quantization Aware Training}} for {{Large Language Models}}},
  shorttitle = {{{LLM-QAT}}},
  author = {Liu, Zechun and Oguz, Barlas and Zhao, Changsheng and Chang, Ernie and Stock, Pierre and Mehdad, Yashar and Shi, Yangyang and Krishnamoorthi, Raghuraman and Chandra, Vikas},
  date = {2023-05-29},
  eprint = {2305.17888},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2305.17888},
  url = {http://arxiv.org/abs/2305.17888},
  urldate = {2024-04-16},
  abstract = {Several post-training quantization methods have been applied to large language models (LLMs), and have been shown to perform well down to 8-bits. We find that these methods break down at lower bit precision, and investigate quantization aware training for LLMs (LLM-QAT) to push quantization levels even further. We propose a data-free distillation method that leverages generations produced by the pre-trained model, which better preserves the original output distribution and allows quantizing any generative model independent of its training data, similar to post-training quantization methods. In addition to quantizing weights and activations, we also quantize the KV cache, which is critical for increasing throughput and support long sequence dependencies at current model sizes. We experiment with LLaMA models of sizes 7B, 13B, and 30B, at quantization levels down to 4-bits. We observe large improvements over training-free methods, especially in the low-bit settings.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Liu et al_2023_LLM-QAT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ARJJWW8C\\2305.html}
}

@online{liUnifiedFoundationModel2021,
  title = {Towards a {{Unified Foundation Model}}: {{Jointly Pre-Training Transformers}} on {{Unpaired Images}} and {{Text}}},
  shorttitle = {Towards a {{Unified Foundation Model}}},
  author = {Li, Qing and Gong, Boqing and Cui, Yin and Kondratyuk, Dan and Du, Xianzhi and Yang, Ming-Hsuan and Brown, Matthew},
  date = {2021-12-13},
  eprint = {2112.07074},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2112.07074},
  url = {http://arxiv.org/abs/2112.07074},
  urldate = {2024-02-02},
  abstract = {In this paper, we explore the possibility of building a unified foundation model that can be adapted to both vision-only and text-only tasks. Starting from BERT and ViT, we design a unified transformer consisting of modality-specific tokenizers, a shared transformer encoder, and task-specific output heads. To efficiently pre-train the proposed model jointly on unpaired images and text, we propose two novel techniques: (i) We employ the separately-trained BERT and ViT models as teachers and apply knowledge distillation to provide additional, accurate supervision signals for the joint training; (ii) We propose a novel gradient masking strategy to balance the parameter updates from the image and text pre-training losses. We evaluate the jointly pre-trained transformer by fine-tuning it on image classification tasks and natural language understanding tasks, respectively. The experiments show that the resultant unified foundation transformer works surprisingly well on both the vision-only and text-only tasks, and the proposed knowledge distillation and gradient masking strategy can effectively lift the performance to approach the level of separately-trained models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Li et al_2021_Towards a Unified Foundation Model.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CCKLUAHE\\2112.html}
}

@inproceedings{liUNIMO2EndtoEndUnified2022,
  title = {{{UNIMO-2}}: {{End-to-End Unified Vision-Language Grounded Learning}}},
  shorttitle = {{{UNIMO-2}}},
  booktitle = {Findings of the {{Association}} for {{Computational Linguistics}}: {{ACL}} 2022},
  author = {Li, Wei and Gao, Can and Niu, Guocheng and Xiao, Xinyan and Liu, Hao and Liu, Jiachen and Wu, Hua and Wang, Haifeng},
  date = {2022-05},
  pages = {3187--3201},
  publisher = {Association for Computational Linguistics},
  location = {Dublin, Ireland},
  doi = {10.18653/v1/2022.findings-acl.251},
  url = {https://aclanthology.org/2022.findings-acl.251},
  urldate = {2023-05-28},
  abstract = {Vision-Language Pre-training (VLP) has achieved impressive performance on various cross-modal downstream tasks. However, most existing methods can only learn from aligned image-caption data and rely heavily on expensive regional features, which greatly limits their scalability and performance. In this paper, we propose an end-to-end unified-modal pre-training framework, namely UNIMO-2, for joint learning on both aligned image-caption data and unaligned image-only and text-only corpus. We build a unified Transformer model to jointly learn visual representations, textual representations and semantic alignment between images and texts. In particular, we propose to conduct grounded learning on both images and texts via a sharing grounded space, which helps bridge unaligned images and texts, and align the visual and textual semantic spaces on different types of corpora. The experiments show that our grounded learning method can improve textual and visual semantic alignment for improving performance on various cross-modal tasks. Moreover, benefiting from effective joint modeling of different types of corpora, our model also achieves impressive performance on single-modal visual and textual tasks. Our code and models are public at the UNIMO project page https://unimo-ptm.github.io/.},
  eventtitle = {Findings 2022},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Li et al_2022_UNIMO-2.pdf}
}

@online{liuOpenCategoryDetection2018,
  title = {Open {{Category Detection}} with {{PAC Guarantees}}},
  author = {Liu, Si and Garrepalli, Risheek and Dietterich, Thomas G. and Fern, Alan and Hendrycks, Dan},
  date = {2018-08-01},
  eprint = {1808.00529},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1808.00529},
  urldate = {2022-12-16},
  abstract = {Open category detection is the problem of detecting "alien" test instances that belong to categories or classes that were not present in the training data. In many applications, reliably detecting such aliens is central to ensuring the safety and accuracy of test set predictions. Unfortunately, there are no algorithms that provide theoretical guarantees on their ability to detect aliens under general assumptions. Further, while there are algorithms for open category detection, there are few empirical results that directly report alien detection rates. Thus, there are significant theoretical and empirical gaps in our understanding of open category detection. In this paper, we take a step toward addressing this gap by studying a simple, but practically-relevant variant of open category detection. In our setting, we are provided with a "clean" training set that contains only the target categories of interest and an unlabeled "contaminated" training set that contains a fraction \$\textbackslash alpha\$ of alien examples. Under the assumption that we know an upper bound on \$\textbackslash alpha\$, we develop an algorithm with PAC-style guarantees on the alien detection rate, while aiming to minimize false alarms. Empirical results on synthetic and standard benchmark datasets demonstrate the regimes in which the algorithm can be effective and provide a baseline for further advancements.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Liu et al_2018_Open Category Detection with PAC Guarantees.pdf;C\:\\Users\\chsey\\Zotero\\storage\\699G3JC4\\1808.html}
}

@online{liuParameterEfficientOrthogonalFinetuning2024,
  title = {Parameter-{{Efficient Orthogonal Finetuning}} via {{Butterfly Factorization}}},
  author = {Liu, Weiyang and Qiu, Zeju and Feng, Yao and Xiu, Yuliang and Xue, Yuxuan and Yu, Longhui and Feng, Haiwen and Liu, Zhen and Heo, Juyeon and Peng, Songyou and Wen, Yandong and Black, Michael J. and Weller, Adrian and Schölkopf, Bernhard},
  date = {2024-04-28},
  eprint = {2311.06243},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2311.06243},
  urldate = {2024-05-20},
  abstract = {Large foundation models are becoming ubiquitous, but training them from scratch is prohibitively expensive. Thus, efficiently adapting these powerful models to downstream tasks is increasingly important. In this paper, we study a principled finetuning paradigm – Orthogonal Finetuning (OFT) – for downstream task adaptation. Despite demonstrating good generalizability, OFT still uses a fairly large number of trainable parameters due to the high dimensionality of orthogonal matrices. To address this, we start by examining OFT from an information transmission perspective, and then identify a few key desiderata that enable better parameterefficiency. Inspired by how the Cooley-Tukey fast Fourier transform algorithm enables efficient information transmission, we propose an efficient orthogonal parameterization using butterfly structures. We apply this parameterization to OFT, creating a novel parameter-efficient finetuning method, called Orthogonal Butterfly (BOFT). By subsuming OFT as a special case, BOFT introduces a generalized orthogonal finetuning framework. Finally, we conduct an extensive empirical study of adapting large vision transformers, large language models, and text-to-image diffusion models to various downstream tasks in vision and language.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\DQ8KEEX8\Liu 등 - 2024 - Parameter-Efficient Orthogonal Finetuning via Butt.pdf}
}

@online{liuPretrainPromptPredict2021,
  title = {Pre-Train, {{Prompt}}, and {{Predict}}: {{A Systematic Survey}} of {{Prompting Methods}} in {{Natural Language Processing}}},
  shorttitle = {Pre-Train, {{Prompt}}, and {{Predict}}},
  author = {Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
  date = {2021-07-28},
  eprint = {2107.13586},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2107.13586},
  urldate = {2023-08-11},
  abstract = {This paper surveys and organizes research works in a new paradigm in natural language processing, which we dub "prompt-based learning". Unlike traditional supervised learning, which trains a model to take in an input x and predict an output y as P(y|x), prompt-based learning is based on language models that model the probability of text directly. To use these models to perform prediction tasks, the original input x is modified using a template into a textual string prompt x' that has some unfilled slots, and then the language model is used to probabilistically fill the unfilled information to obtain a final string x, from which the final output y can be derived. This framework is powerful and attractive for a number of reasons: it allows the language model to be pre-trained on massive amounts of raw text, and by defining a new prompting function the model is able to perform few-shot or even zero-shot learning, adapting to new scenarios with few or no labeled data. In this paper we introduce the basics of this promising paradigm, describe a unified set of mathematical notations that can cover a wide variety of existing work, and organize existing work along several dimensions, e.g.the choice of pre-trained models, prompts, and tuning strategies. To make the field more accessible to interested beginners, we not only make a systematic review of existing works and a highly structured typology of prompt-based concepts, but also release other resources, e.g., a website http://pretrain.nlpedia.ai/ including constantly-updated survey, and paperlist.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Liu et al_2021_Pre-train, Prompt, and Predict.pdf;C\:\\Users\\chsey\\Zotero\\storage\\647GGG7G\\2107.html}
}

@online{liuPretrainPromptPredict2021a,
  title = {Pre-Train, {{Prompt}}, and {{Predict}}: {{A Systematic Survey}} of {{Prompting Methods}} in {{Natural Language Processing}}},
  shorttitle = {Pre-Train, {{Prompt}}, and {{Predict}}},
  author = {Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
  date = {2021-07-28},
  eprint = {2107.13586},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2107.13586},
  url = {http://arxiv.org/abs/2107.13586},
  urldate = {2023-11-22},
  abstract = {This paper surveys and organizes research works in a new paradigm in natural language processing, which we dub "prompt-based learning". Unlike traditional supervised learning, which trains a model to take in an input x and predict an output y as P(y|x), prompt-based learning is based on language models that model the probability of text directly. To use these models to perform prediction tasks, the original input x is modified using a template into a textual string prompt x' that has some unfilled slots, and then the language model is used to probabilistically fill the unfilled information to obtain a final string x, from which the final output y can be derived. This framework is powerful and attractive for a number of reasons: it allows the language model to be pre-trained on massive amounts of raw text, and by defining a new prompting function the model is able to perform few-shot or even zero-shot learning, adapting to new scenarios with few or no labeled data. In this paper we introduce the basics of this promising paradigm, describe a unified set of mathematical notations that can cover a wide variety of existing work, and organize existing work along several dimensions, e.g.the choice of pre-trained models, prompts, and tuning strategies. To make the field more accessible to interested beginners, we not only make a systematic review of existing works and a highly structured typology of prompt-based concepts, but also release other resources, e.g., a website http://pretrain.nlpedia.ai/ including constantly-updated survey, and paperlist.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Liu et al_2021_Pre-train, Prompt, and Predict.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MHDAVIKP\\2107.html}
}

@inproceedings{liuPTuningPromptTuning2022,
  title = {P-{{Tuning}}: {{Prompt Tuning Can Be Comparable}} to {{Fine-tuning Across Scales}} and {{Tasks}}},
  shorttitle = {P-{{Tuning}}},
  booktitle = {Proceedings of the 60th {{Annual Meeting}} of the {{Association}} for {{Computational Linguistics}} ({{Volume}} 2: {{Short Papers}})},
  author = {Liu, Xiao and Ji, Kaixuan and Fu, Yicheng and Tam, Weng and Du, Zhengxiao and Yang, Zhilin and Tang, Jie},
  date = {2022-05},
  pages = {61--68},
  publisher = {Association for Computational Linguistics},
  location = {Dublin, Ireland},
  doi = {10.18653/v1/2022.acl-short.8},
  url = {https://aclanthology.org/2022.acl-short.8},
  urldate = {2023-08-25},
  abstract = {Prompt tuning, which only tunes continuous prompts with a frozen language model, substantially reduces per-task storage and memory usage at training. However, in the context of NLU, prior work reveals that prompt tuning does not perform well for normal-sized pretrained models. We also find that existing methods of prompt tuning cannot handle hard sequence labeling tasks, indicating a lack of universality. We present a novel empirical finding that properly optimized prompt tuning can be universally effective across a wide range of model scales and NLU tasks. It matches the performance of finetuning while having only 0.1\%-3\% tuned parameters. Our method P-Tuning v2 is an implementation of Deep Prompt Tuning (CITATION) optimized and adapted for NLU. Given the universality and simplicity of P-Tuning v2, we believe it can serve as an alternative to finetuning and a strong baseline for future research.},
  eventtitle = {{{ACL}} 2022},
  file = {Y:\paper\2023 graduation\CJ_paper\Liu et al_2022_P-Tuning.pdf}
}

@online{liuRecentAdvancesFederated2023,
  title = {Recent {{Advances}} on {{Federated Learning}}: {{A Systematic Survey}}},
  shorttitle = {Recent {{Advances}} on {{Federated Learning}}},
  author = {Liu, Bingyan and Lv, Nuoyan and Guo, Yuanchun and Li, Yawen},
  date = {2023-01-03},
  eprint = {2301.01299},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2301.01299},
  urldate = {2024-09-19},
  abstract = {Federated learning has emerged as an effective paradigm to achieve privacy-preserving collaborative learning among different parties. Compared to traditional centralized learning that requires collecting data from each party, in federated learning, only the locally trained models or computed gradients are exchanged, without exposing any data information. As a result, it is able to protect privacy to some extent. In recent years, federated learning has become more and more prevalent and there have been many surveys for summarizing related methods in this hot research topic. However, most of them focus on a specific perspective or lack the latest research progress. In this paper, we provide a systematic survey on federated learning, aiming to review the recent advanced federated methods and applications from different aspects. Specifically, this paper includes four major contributions. First, we present a new taxonomy of federated learning in terms of the pipeline and challenges in federated scenarios. Second, we summarize federated learning methods into several categories and briefly introduce the state-of-the-art methods under these categories. Third, we overview some prevalent federated learning frameworks and introduce their features. Finally, some potential deficiencies of current methods and several future directions are discussed.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\4Q7CDB4W\Liu 등 - 2023 - Recent Advances on Federated Learning A Systemati.pdf}
}

@online{liuRoBERTaRobustlyOptimized2019,
  title = {{{RoBERTa}}: {{A Robustly Optimized BERT Pretraining Approach}}},
  shorttitle = {{{RoBERTa}}},
  author = {Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  date = {2019-07-26},
  eprint = {1907.11692},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1907.11692},
  urldate = {2024-05-10},
  abstract = {Language model pretraining has led to significant performance gains but careful comparison between different approaches is challenging. Training is computationally expensive, often done on private datasets of different sizes, and, as we will show, hyperparameter choices have significant impact on the final results. We present a replication study of BERT pretraining (Devlin et al., 2019) that carefully measures the impact of many key hyperparameters and training data size. We find that BERT was significantly undertrained, and can match or exceed the performance of every model published after it. Our best model achieves state-of-the-art results on GLUE, RACE and SQuAD. These results highlight the importance of previously overlooked design choices, and raise questions about the source of recently reported improvements. We release our models and code.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y:\paper\2024_research\Liu et al_2019_RoBERTa.pdf}
}

@online{liuSamePretrainingLoss2022,
  title = {Same {{Pre-training Loss}}, {{Better Downstream}}: {{Implicit Bias Matters}} for {{Language Models}}},
  shorttitle = {Same {{Pre-training Loss}}, {{Better Downstream}}},
  author = {Liu, Hong and Xie, Sang Michael and Li, Zhiyuan and Ma, Tengyu},
  date = {2022-10-25},
  eprint = {2210.14199},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2210.14199},
  urldate = {2024-04-14},
  abstract = {Language modeling on large-scale datasets leads to impressive performance gains on various downstream language tasks. The validation pre-training loss (or perplexity in autoregressive language modeling) is often used as the evaluation metric when developing language models since the pre-training loss tends to be well-correlated with downstream performance (which is itself difficult to evaluate comprehensively). Contrary to this conventional wisdom, this paper shows that 1) pre-training loss cannot fully explain downstream performance and 2) flatness of the model is well-correlated with downstream performance where pre-training loss is not. On simplified datasets, we identify three ways to produce models with the same (statistically optimal) pre-training loss but different downstream performance: continue pre-training after convergence, increasing the model size, and changing the training algorithm. These experiments demonstrate the existence of implicit bias of pre-training algorithms/optimizers -- among models with the same minimal pre-training loss, they implicitly prefer more transferable ones. Toward understanding this implicit bias, we prove that SGD with standard mini-batch noise implicitly prefers flatter minima in language models, and empirically observe a strong correlation between flatness and downstream performance among models with the same minimal pre-training loss. We also prove in a synthetic language setting that among the models with the minimal pre-training loss, the flattest model transfers to downstream tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Liu et al_2022_Same Pre-training Loss, Better Downstream.pdf;C\:\\Users\\chsey\\Zotero\\storage\\33WU8RY6\\2210.html}
}

@incollection{liuSSDSingleShot2016,
  title = {{{SSD}}: {{Single Shot MultiBox Detector}}},
  shorttitle = {{{SSD}}},
  author = {Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C.},
  date = {2016},
  volume = {9905},
  eprint = {1512.02325},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {21--37},
  doi = {10.1007/978-3-319-46448-0_2},
  url = {http://arxiv.org/abs/1512.02325},
  urldate = {2023-08-05},
  abstract = {We present a method for detecting objects in images using a single deep neural network. Our approach, named SSD, discretizes the output space of bounding boxes into a set of default boxes over different aspect ratios and scales per feature map location. At prediction time, the network generates scores for the presence of each object category in each default box and produces adjustments to the box to better match the object shape. Additionally, the network combines predictions from multiple feature maps with different resolutions to naturally handle objects of various sizes. Our SSD model is simple relative to methods that require object proposals because it completely eliminates proposal generation and subsequent pixel or feature resampling stage and encapsulates all computation in a single network. This makes SSD easy to train and straightforward to integrate into systems that require a detection component. Experimental results on the PASCAL VOC, MS COCO, and ILSVRC datasets confirm that SSD has comparable accuracy to methods that utilize an additional object proposal step and is much faster, while providing a unified framework for both training and inference. Compared to other single stage methods, SSD has much better accuracy, even with a smaller input image size. For \$300\textbackslash times 300\$ input, SSD achieves 72.1\% mAP on VOC2007 test at 58 FPS on a Nvidia Titan X and for \$500\textbackslash times 500\$ input, SSD achieves 75.1\% mAP, outperforming a comparable state of the art Faster R-CNN model. Code is available at https://github.com/weiliu89/caffe/tree/ssd .},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Liu et al_2016_SSD.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UH6LCDB6\\1512.html}
}

@online{liuSwinTransformerHierarchical2021,
  title = {Swin {{Transformer}}: {{Hierarchical Vision Transformer}} Using {{Shifted Windows}}},
  shorttitle = {Swin {{Transformer}}},
  author = {Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  date = {2021-08-17},
  eprint = {2103.14030},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2103.14030},
  url = {http://arxiv.org/abs/2103.14030},
  urldate = {2022-07-04},
  abstract = {This paper presents a new vision Transformer, called Swin Transformer, that capably serves as a general-purpose backbone for computer vision. Challenges in adapting Transformer from language to vision arise from differences between the two domains, such as large variations in the scale of visual entities and the high resolution of pixels in images compared to words in text. To address these differences, we propose a hierarchical Transformer whose representation is computed with \textbackslash textbf\{S\}hifted \textbackslash textbf\{win\}dows. The shifted windowing scheme brings greater efficiency by limiting self-attention computation to non-overlapping local windows while also allowing for cross-window connection. This hierarchical architecture has the flexibility to model at various scales and has linear computational complexity with respect to image size. These qualities of Swin Transformer make it compatible with a broad range of vision tasks, including image classification (87.3 top-1 accuracy on ImageNet-1K) and dense prediction tasks such as object detection (58.7 box AP and 51.1 mask AP on COCO test-dev) and semantic segmentation (53.5 mIoU on ADE20K val). Its performance surpasses the previous state-of-the-art by a large margin of +2.7 box AP and +2.6 mask AP on COCO, and +3.2 mIoU on ADE20K, demonstrating the potential of Transformer-based models as vision backbones. The hierarchical design and the shifted window approach also prove beneficial for all-MLP architectures. The code and models are publicly available at\textasciitilde\textbackslash url\{https://github.com/microsoft/Swin-Transformer\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\transformer\\Liu et al_2021_Swin Transformer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V3W2P5EU\\2103.html}
}

@online{liuSwinTransformerHierarchical2021a,
  title = {Swin {{Transformer}}: {{Hierarchical Vision Transformer}} Using {{Shifted Windows}}},
  shorttitle = {Swin {{Transformer}}},
  author = {Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  date = {2021-08-17},
  eprint = {2103.14030},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2103.14030},
  url = {http://arxiv.org/abs/2103.14030},
  urldate = {2023-10-23},
  abstract = {This paper presents a new vision Transformer, called Swin Transformer, that capably serves as a general-purpose backbone for computer vision. Challenges in adapting Transformer from language to vision arise from differences between the two domains, such as large variations in the scale of visual entities and the high resolution of pixels in images compared to words in text. To address these differences, we propose a hierarchical Transformer whose representation is computed with \textbackslash textbf\{S\}hifted \textbackslash textbf\{win\}dows. The shifted windowing scheme brings greater efficiency by limiting self-attention computation to non-overlapping local windows while also allowing for cross-window connection. This hierarchical architecture has the flexibility to model at various scales and has linear computational complexity with respect to image size. These qualities of Swin Transformer make it compatible with a broad range of vision tasks, including image classification (87.3 top-1 accuracy on ImageNet-1K) and dense prediction tasks such as object detection (58.7 box AP and 51.1 mask AP on COCO test-dev) and semantic segmentation (53.5 mIoU on ADE20K val). Its performance surpasses the previous state-of-the-art by a large margin of +2.7 box AP and +2.6 mask AP on COCO, and +3.2 mIoU on ADE20K, demonstrating the potential of Transformer-based models as vision backbones. The hierarchical design and the shifted window approach also prove beneficial for all-MLP architectures. The code and models are publicly available at\textasciitilde\textbackslash url\{https://github.com/microsoft/Swin-Transformer\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Liu et al_2021_Swin Transformer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HW42VZI9\\2103.html}
}

@online{liuSwinTransformerV22022,
  title = {Swin {{Transformer V2}}: {{Scaling Up Capacity}} and {{Resolution}}},
  shorttitle = {Swin {{Transformer V2}}},
  author = {Liu, Ze and Hu, Han and Lin, Yutong and Yao, Zhuliang and Xie, Zhenda and Wei, Yixuan and Ning, Jia and Cao, Yue and Zhang, Zheng and Dong, Li and Wei, Furu and Guo, Baining},
  date = {2022-04-11},
  eprint = {2111.09883},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.09883},
  urldate = {2023-11-10},
  abstract = {Large-scale NLP models have been shown to significantly improve the performance on language tasks with no signs of saturation. They also demonstrate amazing few-shot capabilities like that of human beings. This paper aims to explore large-scale models in computer vision. We tackle three major issues in training and application of large vision models, including training instability, resolution gaps between pre-training and fine-tuning, and hunger on labelled data. Three main techniques are proposed: 1) a residual-post-norm method combined with cosine attention to improve training stability; 2) A log-spaced continuous position bias method to effectively transfer models pre-trained using low-resolution images to downstream tasks with high-resolution inputs; 3) A self-supervised pre-training method, SimMIM, to reduce the needs of vast labeled images. Through these techniques, this paper successfully trained a 3 billion-parameter Swin Transformer V2 model, which is the largest dense vision model to date, and makes it capable of training with images of up to 1,536\$\textbackslash times\$1,536 resolution. It set new performance records on 4 representative vision tasks, including ImageNet-V2 image classification, COCO object detection, ADE20K semantic segmentation, and Kinetics-400 video action classification. Also note our training is much more efficient than that in Google's billion-level visual models, which consumes 40 times less labelled data and 40 times less training time. Code is available at \textbackslash url\{https://github.com/microsoft/Swin-Transformer\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Liu et al_2022_Swin Transformer V2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MJYIMXBE\\2111.html}
}

@online{liuZero13ZeroshotOne2023,
  title = {Zero-1-to-3: {{Zero-shot One Image}} to {{3D Object}}},
  shorttitle = {Zero-1-to-3},
  author = {Liu, Ruoshi and Wu, Rundi and Hoorick, Basile Van and Tokmakov, Pavel and Zakharov, Sergey and Vondrick, Carl},
  date = {2023-03-20},
  eprint = {2303.11328},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2303.11328},
  urldate = {2024-10-18},
  abstract = {We introduce Zero-1-to-3, a framework for changing the camera viewpoint of an object given just a single RGB image. To perform novel view synthesis in this under-constrained setting, we capitalize on the geometric priors that large-scale diffusion models learn about natural images. Our conditional diffusion model uses a synthetic dataset to learn controls of the relative camera viewpoint, which allow new images to be generated of the same object under a specified camera transformation. Even though it is trained on a synthetic dataset, our model retains a strong zero-shot generalization ability to out-of-distribution datasets as well as in-the-wild images, including impressionist paintings. Our viewpoint-conditioned diffusion approach can further be used for the task of 3D reconstruction from a single image. Qualitative and quantitative experiments show that our method significantly outperforms state-of-the-art single-view 3D reconstruction and novel view synthesis models by leveraging Internet-scale pre-training.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Robotics},
  file = {Y\:\\paper\\2024_lecture\\Liu et al_2023_Zero-1-to-3.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5ZKTY5U9\\2303.html}
}

@inproceedings{liVerySparseRandom2006,
  title = {Very Sparse Random Projections},
  booktitle = {Proceedings of the 12th {{ACM SIGKDD}} International Conference on {{Knowledge}} Discovery and Data Mining},
  author = {Li, Ping and Hastie, Trevor J. and Church, Kenneth W.},
  year = {8월 20, 2006},
  series = {{{KDD}} '06},
  pages = {287--296},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/1150402.1150436},
  url = {https://dl.acm.org/doi/10.1145/1150402.1150436},
  urldate = {2024-04-14},
  abstract = {There has been considerable interest in random projections, an approximate algorithm for estimating distances between pairs of points in a high-dimensional vector space. Let A in Rn x D be our n points in D dimensions. The method multiplies A by a random matrix R in RD x k, reducing the D dimensions down to just k for speeding up the computation. R typically consists of entries of standard normal N(0,1). It is well known that random projections preserve pairwise distances (in the expectation). Achlioptas proposed sparse random projections by replacing the N(0,1) entries in R with entries in -1,0,1 with probabilities 1/6, 2/3, 1/6, achieving a threefold speedup in processing time.We recommend using R of entries in -1,0,1 with probabilities 1/2√D, 1-1√D, 1/2√D for achieving a significant √D-fold speedup, with little loss in accuracy.},
  isbn = {978-1-59593-339-3},
  keywords = {notion,random projections,rates of convergence,sampling},
  file = {Y:\paper\2024_research\Li et al_2006_Very sparse random projections.pdf}
}

@inproceedings{liWhatDoesBERT2020,
  title = {What {{Does BERT}} with {{Vision Look At}}?},
  booktitle = {Proceedings of the 58th {{Annual Meeting}} of the {{Association}} for {{Computational Linguistics}}},
  author = {Li, Liunian Harold and Yatskar, Mark and Yin, Da and Hsieh, Cho-Jui and Chang, Kai-Wei},
  date = {2020-07},
  pages = {5265--5275},
  publisher = {Association for Computational Linguistics},
  location = {Online},
  doi = {10.18653/v1/2020.acl-main.469},
  url = {https://aclanthology.org/2020.acl-main.469},
  urldate = {2023-05-28},
  abstract = {Pre-trained visually grounded language models such as ViLBERT, LXMERT, and UNITER have achieved significant performance improvement on vision-and-language tasks but what they learn during pre-training remains unclear. In this work, we demonstrate that certain attention heads of a visually grounded language model actively ground elements of language to image regions. Specifically, some heads can map entities to image regions, performing the task known as entity grounding. Some heads can even detect the syntactic relations between non-entity words and image regions, tracking, for example, associations between verbs and regions corresponding to their arguments. We denote this ability as syntactic grounding. We verify grounding both quantitatively and qualitatively, using Flickr30K Entities as a testbed.},
  eventtitle = {{{ACL}} 2020},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\dense captioning\Li et al_2020_What Does BERT with Vision Look At.pdf}
}

@online{liWhatHappensSGD2022,
  title = {What {{Happens}} after {{SGD Reaches Zero Loss}}? --{{A Mathematical Framework}}},
  shorttitle = {What {{Happens}} after {{SGD Reaches Zero Loss}}?},
  author = {Li, Zhiyuan and Wang, Tianhao and Arora, Sanjeev},
  date = {2022-07-28},
  eprint = {2110.06914},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2110.06914},
  urldate = {2024-05-17},
  abstract = {Understanding the implicit bias of Stochastic Gradient Descent (SGD) is one of the key challenges in deep learning, especially for overparametrized models, where the local minimizers of the loss function L can form a manifold. Intuitively, with a sufficiently small learning rate η, SGD tracks Gradient Descent (GD) until it gets close to such manifold, where the gradient noise prevents further convergence. In such regime, Blanc et al. (2020) proved that SGD with label noise locally decreases a regularizer-like term, the sharpness of loss, tr[∇2L]. The current paper gives a general framework for such analysis by adapting ideas from Katzenberger (1991). It allows in principle a complete characterization for the regularization effect of SGD around such manifold—i.e., the ”implicit bias”—using a stochastic differential equation (SDE) describing the limiting dynamics of the parameters, which is determined jointly by the loss function and the noise covariance. This yields some new results: (1) a global analysis of the implicit bias valid for η−2 steps, in contrast to the local analysis of Blanc et al. (2020) that is only valid for η−1.6 steps and (2) allowing arbitrary noise covariance. As an application, we show with arbitrary large initialization, label noise SGD can always escape the kernel regime and only requires O(κ ln d) samples for learning a κ-sparse overparametrized linear model in Rd (Woodworth et al., 2020), while GD initialized in the kernel regime requires Ω(d) samples. This upper bound is minimax optimal and improves the previous O(κ2) upper bound (HaoChen et al., 2020).},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\UXH7XGUD\Li 등 - 2022 - What Happens after SGD Reaches Zero Loss --A Math.pdf}
}

@online{logeQPainQuestionAnswering2021,
  title = {Q-{{Pain}}: {{A Question Answering Dataset}} to {{Measure Social Bias}} in {{Pain Management}}},
  shorttitle = {Q-{{Pain}}},
  author = {Logé, Cécile and Ross, Emily and Dadey, David Yaw Amoah and Jain, Saahil and Saporta, Adriel and Ng, Andrew Y. and Rajpurkar, Pranav},
  date = {2021-08-03},
  eprint = {2108.01764},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2108.01764},
  url = {http://arxiv.org/abs/2108.01764},
  urldate = {2023-05-23},
  abstract = {Recent advances in Natural Language Processing (NLP), and specifically automated Question Answering (QA) systems, have demonstrated both impressive linguistic fluency and a pernicious tendency to reflect social biases. In this study, we introduce Q-Pain, a dataset for assessing bias in medical QA in the context of pain management, one of the most challenging forms of clinical decision-making. Along with the dataset, we propose a new, rigorous framework, including a sample experimental design, to measure the potential biases present when making treatment decisions. We demonstrate its use by assessing two reference Question-Answering systems, GPT-2 and GPT-3, and find statistically significant differences in treatment between intersectional race-gender subgroups, thus reaffirming the risks posed by AI in medical settings, and the need for datasets like ours to ensure safety before medical AI applications are deployed.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\Logé et al_2021_Q-Pain.pdf;C\:\\Users\\chsey\\Zotero\\storage\\769BQZG7\\2108.html}
}

@online{longFullyConvolutionalNetworks2015,
  title = {Fully {{Convolutional Networks}} for {{Semantic Segmentation}}},
  author = {Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  date = {2015-03-08},
  eprint = {1411.4038},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1411.4038},
  url = {http://arxiv.org/abs/1411.4038},
  urldate = {2023-08-05},
  abstract = {Convolutional networks are powerful visual models that yield hierarchies of features. We show that convolutional networks by themselves, trained end-to-end, pixels-to-pixels, exceed the state-of-the-art in semantic segmentation. Our key insight is to build "fully convolutional" networks that take input of arbitrary size and produce correspondingly-sized output with efficient inference and learning. We define and detail the space of fully convolutional networks, explain their application to spatially dense prediction tasks, and draw connections to prior models. We adapt contemporary classification networks (AlexNet, the VGG net, and GoogLeNet) into fully convolutional networks and transfer their learned representations by fine-tuning to the segmentation task. We then define a novel architecture that combines semantic information from a deep, coarse layer with appearance information from a shallow, fine layer to produce accurate and detailed segmentations. Our fully convolutional network achieves state-of-the-art segmentation of PASCAL VOC (20\% relative improvement to 62.2\% mean IU on 2012), NYUDv2, and SIFT Flow, while inference takes one third of a second for a typical image.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image segmentation\\Long et al_2015_Fully Convolutional Networks for Semantic Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UYXSQPF3\\1411.html}
}

@online{loshchilovSGDRStochasticGradient2017,
  title = {{{SGDR}}: {{Stochastic Gradient Descent}} with {{Warm Restarts}}},
  shorttitle = {{{SGDR}}},
  author = {Loshchilov, Ilya and Hutter, Frank},
  date = {2017-05-03},
  eprint = {1608.03983},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/1608.03983},
  urldate = {2022-12-09},
  abstract = {Restart techniques are common in gradient-free optimization to deal with multimodal functions. Partial warm restarts are also gaining popularity in gradient-based optimization to improve the rate of convergence in accelerated gradient schemes to deal with ill-conditioned functions. In this paper, we propose a simple warm restart technique for stochastic gradient descent to improve its anytime performance when training deep neural networks. We empirically study its performance on the CIFAR-10 and CIFAR-100 datasets, where we demonstrate new state-of-the-art results at 3.14\% and 16.21\%, respectively. We also demonstrate its advantages on a dataset of EEG recordings and on a downsampled version of the ImageNet dataset. Our source code is available at https://github.com/loshchil/SGDR},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,Mathematics - Optimization and Control},
  file = {Y\:\\paper\\Computer Vision\\traditional\\PA3\\Loshchilov_Hutter_2017_SGDR.pdf;C\:\\Users\\chsey\\Zotero\\storage\\I84WW9HF\\1608.html}
}

@online{lotfiNonVacuousGeneralizationBounds2024,
  title = {Non-{{Vacuous Generalization Bounds}} for {{Large Language Models}}},
  author = {Lotfi, Sanae and Finzi, Marc and Kuang, Yilun and Rudner, Tim G. J. and Goldblum, Micah and Wilson, Andrew Gordon},
  date = {2024-02-12},
  eprint = {2312.17173},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2312.17173},
  url = {http://arxiv.org/abs/2312.17173},
  urldate = {2024-04-10},
  abstract = {Modern language models can contain billions of parameters, raising the question of whether they can generalize beyond the training data or simply regurgitate their training corpora. We provide the first non-vacuous generalization bounds for pretrained large language models (LLMs), indicating that language models are capable of discovering regularities that generalize to unseen data. In particular, we derive a compression bound that is valid for the unbounded log-likelihood loss using prediction smoothing, and we extend the bound to handle subsampling, accelerating bound computation on massive datasets. To achieve the extreme level of compression required for non-vacuous generalization bounds, we devise SubLoRA, a low-dimensional non-linear parameterization. Using this approach, we find that larger models have better generalization bounds and are more compressible than smaller models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Lotfi et al_2024_Non-Vacuous Generalization Bounds for Large Language Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6N8DJXVA\\2312.html}
}

@online{lotfiPACBayesCompressionBounds2022,
  title = {{{PAC-Bayes Compression Bounds So Tight That They Can Explain Generalization}}},
  author = {Lotfi, Sanae and Finzi, Marc and Kapoor, Sanyam and Potapczynski, Andres and Goldblum, Micah and Wilson, Andrew Gordon},
  date = {2022-11-24},
  eprint = {2211.13609},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2211.13609},
  url = {http://arxiv.org/abs/2211.13609},
  urldate = {2024-04-13},
  abstract = {While there has been progress in developing non-vacuous generalization bounds for deep neural networks, these bounds tend to be uninformative about why deep learning works. In this paper, we develop a compression approach based on quantizing neural network parameters in a linear subspace, profoundly improving on previous results to provide state-of-the-art generalization bounds on a variety of tasks, including transfer learning. We use these tight bounds to better understand the role of model size, equivariance, and the implicit biases of optimization, for generalization in deep learning. Notably, we find large models can be compressed to a much greater extent than previously known, encapsulating Occam's razor. We also argue for data-independent bounds in explaining generalization.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Lotfi et al_2022_PAC-Bayes Compression Bounds So Tight That They Can Explain Generalization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PLIW9LBW\\2211.html}
}

@article{loweDistinctiveImageFeatures2004,
  title = {Distinctive {{Image Features}} from {{Scale-Invariant Keypoints}}},
  author = {Lowe, David G.},
  date = {2004-11},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {International Journal of Computer Vision},
  volume = {60},
  number = {2},
  pages = {91--110},
  issn = {0920-5691},
  doi = {10.1023/B:VISI.0000029664.99615.94},
  url = {http://link.springer.com/10.1023/B:VISI.0000029664.99615.94},
  urldate = {2022-11-04},
  abstract = {This paper presents a method for extracting distinctive invariant features from images that can be used to perform reliable matching between different views of an object or scene. The features are invariant to image scale and rotation, and are shown to provide robust matching across a substantial range of affine distortion, change in 3D viewpoint, addition of noise, and change in illumination. The features are highly distinctive, in the sense that a single feature can be correctly matched with high probability against a large database of features from many images. This paper also describes an approach to using these features for object recognition. The recognition proceeds by matching individual features to a database of features from known objects using a fast nearest-neighbor algorithm, followed by a Hough transform to identify clusters belonging to a single object, and finally performing verification through least-squares solution for consistent pose parameters. This approach to recognition can robustly identify objects among clutter and occlusion while achieving near real-time performance.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA2\Lowe_2004_Distinctive Image Features from Scale-Invariant Keypoints.pdf}
}

@online{LowRankCompressionNeural,
  title = {Low-{{Rank Compression}} of {{Neural Nets}}: {{Learning}} the {{Rank}} of {{Each Layer}} | {{IEEE Conference Publication}} | {{IEEE Xplore}}},
  url = {https://ieeexplore.ieee.org/document/9157223},
  urldate = {2024-03-18},
  keywords = {notion}
}

@online{LSUN,
  title = {{{LSUN}}},
  url = {https://www.yf.io/p/lsun},
  urldate = {2022-11-15},
  file = {C:\Users\chsey\Zotero\storage\RZIP55Z8\lsun.html}
}

@online{luHierarchicalQuestionImageCoAttention2017,
  title = {Hierarchical {{Question-Image Co-Attention}} for {{Visual Question Answering}}},
  author = {Lu, Jiasen and Yang, Jianwei and Batra, Dhruv and Parikh, Devi},
  date = {2017-01-19},
  eprint = {1606.00061},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1606.00061},
  url = {http://arxiv.org/abs/1606.00061},
  urldate = {2024-04-25},
  abstract = {A number of recent works have proposed attention models for Visual Question Answering (VQA) that generate spatial maps highlighting image regions relevant to answering the question. In this paper, we argue that in addition to modeling "where to look" or visual attention, it is equally important to model "what words to listen to" or question attention. We present a novel co-attention model for VQA that jointly reasons about image and question attention. In addition, our model reasons about the question (and consequently the image via the co-attention mechanism) in a hierarchical fashion via a novel 1-dimensional convolution neural networks (CNN). Our model improves the state-of-the-art on the VQA dataset from 60.3\% to 60.5\%, and from 61.6\% to 63.3\% on the COCO-QA dataset. By using ResNet, the performance is further improved to 62.1\% for VQA and 65.4\% for COCO-QA.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Lu et al_2017_Hierarchical Question-Image Co-Attention for Visual Question Answering.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TCQEE4WP\\1606.html}
}

@online{luIconQANewBenchmark2022,
  title = {{{IconQA}}: {{A New Benchmark}} for {{Abstract Diagram Understanding}} and {{Visual Language Reasoning}}},
  shorttitle = {{{IconQA}}},
  author = {Lu, Pan and Qiu, Liang and Chen, Jiaqi and Xia, Tony and Zhao, Yizhou and Zhang, Wei and Yu, Zhou and Liang, Xiaodan and Zhu, Song-Chun},
  date = {2022-07-25},
  eprint = {2110.13214},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2110.13214},
  url = {http://arxiv.org/abs/2110.13214},
  urldate = {2023-05-23},
  abstract = {Current visual question answering (VQA) tasks mainly consider answering human-annotated questions for natural images. However, aside from natural images, abstract diagrams with semantic richness are still understudied in visual understanding and reasoning research. In this work, we introduce a new challenge of Icon Question Answering (IconQA) with the goal of answering a question in an icon image context. We release IconQA, a large-scale dataset that consists of 107,439 questions and three sub-tasks: multi-image-choice, multi-text-choice, and filling-in-the-blank. The IconQA dataset is inspired by real-world diagram word problems that highlight the importance of abstract diagram understanding and comprehensive cognitive reasoning. Thus, IconQA requires not only perception skills like object recognition and text understanding, but also diverse cognitive reasoning skills, such as geometric reasoning, commonsense reasoning, and arithmetic reasoning. To facilitate potential IconQA models to learn semantic representations for icon images, we further release an icon dataset Icon645 which contains 645,687 colored icons on 377 classes. We conduct extensive user studies and blind experiments and reproduce a wide range of advanced VQA methods to benchmark the IconQA task. Also, we develop a strong IconQA baseline Patch-TRM that applies a pyramid cross-modal Transformer with input diagram embeddings pre-trained on the icon dataset. IconQA and Icon645 are available at https://iconqa.github.io.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\Lu et al_2022_IconQA.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VS68R4VM\\2110.html}
}

@online{luNeuralBabyTalk2018,
  title = {Neural {{Baby Talk}}},
  author = {Lu, Jiasen and Yang, Jianwei and Batra, Dhruv and Parikh, Devi},
  date = {2018-03-26},
  eprint = {1803.09845},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1803.09845},
  url = {http://arxiv.org/abs/1803.09845},
  urldate = {2023-08-05},
  abstract = {We introduce a novel framework for image captioning that can produce natural language explicitly grounded in entities that object detectors find in the image. Our approach reconciles classical slot filling approaches (that are generally better grounded in images) with modern neural captioning approaches (that are generally more natural sounding and accurate). Our approach first generates a sentence `template' with slot locations explicitly tied to specific image regions. These slots are then filled in by visual concepts identified in the regions by object detectors. The entire architecture (sentence template generation and slot filling with object detectors) is end-to-end differentiable. We verify the effectiveness of our proposed model on different image captioning tasks. On standard image captioning and novel object captioning, our model reaches state-of-the-art on both COCO and Flickr30k datasets. We also demonstrate that our model has unique advantages when the train and test distributions of scene compositions -- and hence language priors of associated captions -- are different. Code has been made available at: https://github.com/jiasenlu/NeuralBabyTalk},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\vision and language\\Lu et al_2018_Neural Baby Talk.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3X4HEJ5A\\1803.html}
}

@online{luoLabelEfficientLearning2017,
  title = {Label {{Efficient Learning}} of {{Transferable Representations}} across {{Domains}} and {{Tasks}}},
  author = {Luo, Zelun and Zou, Yuliang and Hoffman, Judy and Fei-Fei, Li},
  date = {2017-11-30},
  eprint = {1712.00123},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1712.00123},
  url = {http://arxiv.org/abs/1712.00123},
  urldate = {2023-12-23},
  abstract = {We propose a framework that learns a representation transferable across different domains and tasks in a label efficient manner. Our approach battles domain shift with a domain adversarial loss, and generalizes the embedding to novel task using a metric learning-based approach. Our model is simultaneously optimized on labeled source data and unlabeled or sparsely labeled data in the target domain. Our method shows compelling results on novel classes within a new domain even when only a few labeled examples per class are available, outperforming the prevalent fine-tuning approach. In addition, we demonstrate the effectiveness of our framework on the transfer learning task from image object recognition to video action recognition.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Luo et al_2017_Label Efficient Learning of Transferable Representations across Domains and.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6ZYI6KYA\\1712.html}
}

@online{luPretrainedTransformersUniversal2021,
  title = {Pretrained {{Transformers}} as {{Universal Computation Engines}}},
  author = {Lu, Kevin and Grover, Aditya and Abbeel, Pieter and Mordatch, Igor},
  date = {2021-06-30},
  eprint = {2103.05247},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.05247},
  urldate = {2024-05-08},
  abstract = {We investigate the capability of a transformer pretrained on natural language to generalize to other modalities with minimal finetuning – in particular, without finetuning of the self-attention and feedforward layers of the residual blocks. We consider such a model, which we call a Frozen Pretrained Transformer (FPT), and study finetuning it on a variety of sequence classification tasks spanning numerical computation, vision, and protein fold prediction. In contrast to prior works which investigate finetuning on the same modality as the pretraining dataset, we show that pretraining on natural language can improve performance and compute efficiency on non-language downstream tasks. Additionally, we perform an analysis of the architecture, comparing the performance of a random initialized transformer to a random LSTM. Combining the two insights, we find language-pretrained transformers can obtain strong performance on a variety of non-language tasks1.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Lu et al_2021_Pretrained Transformers as Universal Computation Engines.pdf}
}

@online{luTwinMergingDynamicIntegration2024,
  title = {Twin-{{Merging}}: {{Dynamic Integration}} of {{Modular Expertise}} in {{Model Merging}}},
  shorttitle = {Twin-{{Merging}}},
  author = {Lu, Zhenyi and Fan, Chenghao and Wei, Wei and Qu, Xiaoye and Chen, Dangyang and Cheng, Yu},
  date = {2024-10-14},
  eprint = {2406.15479},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.2406.15479},
  url = {http://arxiv.org/abs/2406.15479},
  urldate = {2024-10-25},
  abstract = {In the era of large language models, model merging is a promising way to combine multiple task-specific models into a single multitask model without extra training. However, two challenges remain: (a) interference between different models and (b) heterogeneous data during testing. Traditional model merging methods often show significant performance gaps compared to fine-tuned models due to these issues. Additionally, a one-size-fits-all model lacks flexibility for diverse test data, leading to performance degradation. We show that both shared and exclusive task-specific knowledge are crucial for merging performance, but directly merging exclusive knowledge hinders overall performance. In view of this, we propose Twin-Merging, a method that encompasses two principal stages: (1) modularizing knowledge into shared and exclusive components, with compression to reduce redundancy and enhance efficiency; (2) dynamically merging shared and task-specific knowledge based on the input. This approach narrows the performance gap between merged and fine-tuned models and improves adaptability to heterogeneous data. Extensive experiments on \$20\$ datasets for both language and vision tasks demonstrate the effectiveness of our method, showing an average improvement of \$28.34\textbackslash\%\$ in absolute normalized score for discriminative tasks and even surpassing the fine-tuned upper bound on the generative tasks. Our implementation is available in \textbackslash url\{https://github.com/LZY-the-boys/Twin-Merging\}},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Lu et al_2024_Twin-Merging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PU8IWKQ7\\2406.html}
}

@online{luUnifiedIOUnifiedModel2022,
  title = {Unified-{{IO}}: {{A Unified Model}} for {{Vision}}, {{Language}}, and {{Multi-Modal Tasks}}},
  shorttitle = {Unified-{{IO}}},
  author = {Lu, Jiasen and Clark, Christopher and Zellers, Rowan and Mottaghi, Roozbeh and Kembhavi, Aniruddha},
  date = {2022-10-04},
  eprint = {2206.08916},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2206.08916},
  url = {http://arxiv.org/abs/2206.08916},
  urldate = {2024-02-05},
  abstract = {We propose Unified-IO, a model that performs a large variety of AI tasks spanning classical computer vision tasks, including pose estimation, object detection, depth estimation and image generation, vision-and-language tasks such as region captioning and referring expression, to natural language processing tasks such as question answering and paraphrasing. Developing a single unified model for such a large variety of tasks poses unique challenges due to the heterogeneous inputs and outputs pertaining to each task, including RGB images, per-pixel maps, binary masks, bounding boxes, and language. We achieve this unification by homogenizing every supported input and output into a sequence of discrete vocabulary tokens. This common representation across all tasks allows us to train a single transformer-based architecture, jointly on over 90 diverse datasets in the vision and language fields. Unified-IO is the first model capable of performing all 7 tasks on the GRIT benchmark and produces strong results across 16 diverse benchmarks like NYUv2-Depth, ImageNet, VQA2.0, OK-VQA, Swig, VizWizGround, BoolQ, and SciTail, with no task-specific fine-tuning. Code and demos for Unified-IO are available at: https://unified-io.allenai.org.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Lu et al_2022_Unified-IO.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2AVJQZQ3\\2206.html}
}

@inproceedings{maenoLightFieldDistortion2013,
  title = {Light {{Field Distortion Feature}} for {{Transparent Object Recognition}}},
  booktitle = {2013 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  author = {Maeno, Kazuki and Nagahara, Hajime and Shimada, Atsushi and Taniguchi, Rin-Ichiro},
  date = {2013-06},
  pages = {2786--2793},
  publisher = {IEEE},
  location = {Portland, OR, USA},
  doi = {10.1109/CVPR.2013.359},
  url = {http://ieeexplore.ieee.org/document/6619203/},
  urldate = {2023-01-21},
  abstract = {Current object-recognition algorithms use local features, such as scale-invariant feature transform (SIFT) and speeded-up robust features (SURF), for visually learning to recognize objects. These approaches though cannot apply to transparent objects made of glass or plastic, as such objects take on the visual features of background objects, and the appearance of such objects dramatically varies with changes in scene background. Indeed, in transmitting light, transparent objects have the unique characteristic of distorting the background by refraction. In this paper, we use a single-shot light Àeld image as an input and model the distortion of the light Àeld caused by the refractive property of a transparent object. We propose a new feature, called the light Àeld distortion (LFD) feature, for identifying a transparent object. The proposal incorporates this LFD feature into the bag-of-features approach for recognizing transparent objects. We evaluated its performance in laboratory and real settings.},
  eventtitle = {2013 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-0-7695-4989-7},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\BI8AZJ2L\Maeno 등 - 2013 - Light Field Distortion Feature for Transparent Obj.pdf}
}

@online{maEurekaHumanLevelReward2024,
  title = {Eureka: {{Human-Level Reward Design}} via {{Coding Large Language Models}}},
  shorttitle = {Eureka},
  author = {Ma, Yecheng Jason and Liang, William and Wang, Guanzhi and Huang, De-An and Bastani, Osbert and Jayaraman, Dinesh and Zhu, Yuke and Fan, Linxi and Anandkumar, Anima},
  date = {2024-04-30},
  eprint = {2310.12931},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2310.12931},
  urldate = {2024-05-27},
  abstract = {Large Language Models (LLMs) have excelled as high-level semantic planners for sequential decision-making tasks. However, harnessing them to learn complex lowlevel manipulation tasks, such as dexterous pen spinning, remains an open problem. We bridge this fundamental gap and present EUREKA, a human-level reward design algorithm powered by LLMs. EUREKA exploits the remarkable zero-shot generation, code-writing, and in-context improvement capabilities of state-of-theart LLMs, such as GPT-4, to perform evolutionary optimization over reward code. The resulting rewards can then be used to acquire complex skills via reinforcement learning. Without any task-specific prompting or pre-defined reward templates, EUREKA generates reward functions that outperform expert human-engineered rewards. In a diverse suite of 29 open-source RL environments that include 10 distinct robot morphologies, EUREKA outperforms human experts on 83\% of the tasks, leading to an average normalized improvement of 52\%. The generality of EUREKA also enables a new gradient-free in-context learning approach to reinforcement learning from human feedback (RLHF), readily incorporating human inputs to improve the quality and the safety of the generated rewards without model updating. Finally, using EUREKA rewards in a curriculum learning setting, we demonstrate for the first time, a simulated Shadow Hand capable of performing pen spinning tricks, adeptly manipulating a pen in circles at rapid speed.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Computer Science - Robotics,notion},
  file = {C:\Users\chsey\Zotero\storage\38P5TN8T\Ma 등 - 2024 - Eureka Human-Level Reward Design via Coding Large.pdf}
}

@online{mahendranUnderstandingDeepImage2014,
  title = {Understanding {{Deep Image Representations}} by {{Inverting Them}}},
  author = {Mahendran, Aravindh and Vedaldi, Andrea},
  date = {2014-11-26},
  eprint = {1412.0035},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1412.0035},
  url = {http://arxiv.org/abs/1412.0035},
  urldate = {2023-08-05},
  abstract = {Image representations, from SIFT and Bag of Visual Words to Convolutional Neural Networks (CNNs), are a crucial component of almost any image understanding system. Nevertheless, our understanding of them remains limited. In this paper we conduct a direct analysis of the visual information contained in representations by asking the following question: given an encoding of an image, to which extent is it possible to reconstruct the image itself? To answer this question we contribute a general framework to invert representations. We show that this method can invert representations such as HOG and SIFT more accurately than recent alternatives while being applicable to CNNs too. We then use this technique to study the inverse of recent state-of-the-art CNN image representations for the first time. Among our findings, we show that several layers in CNNs retain photographically accurate information about the image, with different degrees of geometric and photometric invariance.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image classification\\Mahendran_Vedaldi_2014_Understanding Deep Image Representations by Inverting Them.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NAHLLQ4L\\1412.html}
}

@article{manmadhanVisualQuestionAnswering2020,
  title = {Visual Question Answering: A State-of-the-Art Review},
  shorttitle = {Visual Question Answering},
  author = {Manmadhan, Sruthy and Kovoor, Binsu C.},
  date = {2020-12-01},
  journaltitle = {Artificial Intelligence Review},
  shortjournal = {Artif Intell Rev},
  volume = {53},
  number = {8},
  pages = {5705--5745},
  issn = {1573-7462},
  doi = {10.1007/s10462-020-09832-7},
  url = {https://doi.org/10.1007/s10462-020-09832-7},
  urldate = {2023-05-28},
  abstract = {Visual question answering (VQA) is a task that has received immense consideration from two major research communities: computer vision and natural language processing. Recently it has been widely accepted as an AI-complete task which can be used as an alternative to visual turing test. In its most common form, it is a multi-modal challenging task where a computer is required to provide the correct answer for a natural language question asked about an input image. It attracts many deep learning researchers after their remarkable achievements in text, voice and vision technologies. This review extensively and critically examines the current status of VQA research in terms of step by step solution methodologies, datasets and evaluation metrics. Finally, this paper also discusses future research directions for all the above-mentioned aspects of VQA separately.},
  langid = {english},
  keywords = {Computer vision,Deep learning,Natural language processing,Visual question answering},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\VQA\Manmadhan_Kovoor_2020_Visual question answering.pdf}
}

@article{maoCLEVRERHumansDescribingPhysical2022,
  title = {{{CLEVRER-Humans}}: {{Describing Physical}} and {{Causal Events}} the {{Human Way}}},
  shorttitle = {{{CLEVRER-Humans}}},
  author = {Mao, Jiayuan and Yang, Xuelin and Zhang, Xikun and Goodman, Noah and Wu, Jiajun},
  date = {2022-12-06},
  journaltitle = {Advances in Neural Information Processing Systems},
  volume = {35},
  pages = {7755--7768},
  url = {https://proceedings.neurips.cc/paper_files/paper/2022/hash/32fea358f4811ec6d703e8c17028ce1d-Abstract-Datasets_and_Benchmarks.html},
  urldate = {2023-05-23},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\Mao et al_2022_CLEVRER-Humans.pdf}
}

@article{marrisonEvolutionQuartzCrystal1948,
  title = {The {{Evolution}} of the {{Quartz Crystal Clock}}*},
  author = {Marrison, Warren A.},
  date = {1948-07},
  journaltitle = {Bell System Technical Journal},
  volume = {27},
  number = {3},
  pages = {510--588},
  issn = {00058580},
  doi = {10.1002/j.1538-7305.1948.tb01343.x},
  url = {https://ieeexplore.ieee.org/document/6773029},
  urldate = {2023-12-26},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\47C9CQTI\Marrison - 1948 - The Evolution of the Quartz Crystal Clock.pdf}
}

@article{marrisonEvolutionQuartzCrystal1948a,
  title = {The {{Evolution}} of the {{Quartz Crystal Clock}}*},
  author = {Marrison, Warren A.},
  date = {1948},
  journaltitle = {Bell System Technical Journal},
  volume = {27},
  number = {3},
  pages = {510--588},
  issn = {1538-7305},
  doi = {10.1002/j.1538-7305.1948.tb01343.x},
  url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/j.1538-7305.1948.tb01343.x},
  urldate = {2023-12-26},
  langid = {english}
}

@online{MathematicalFonts,
  title = {Mathematical Fonts},
  url = {https://www.overleaf.com/learn/latex/Mathematical_fonts},
  urldate = {2023-02-13},
  abstract = {An online LaTeX editor that’s easy to use. No installation, real-time collaboration, version control, hundreds of LaTeX templates, and more.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\LPL2WEJJ\Mathematical_fonts.html}
}

@video{matthewotooleToRFTimeofFlightRadiance2022,
  entrysubtype = {video},
  title = {{{TöRF}}: {{Time-of-Flight Radiance Fields}} for {{Dynamic Scene View Synthesis}}},
  shorttitle = {{{TöRF}}},
  editor = {{Matthew O'Toole}},
  editortype = {director},
  date = {2022},
  url = {https://www.youtube.com/watch?v=aaJnSRxAQXc},
  urldate = {2023-01-21}
}

@article{maxLocalGlobalIllumination2010,
  title = {Local and {{Global Illumination}} in the {{Volume Rendering Integral}}},
  author = {Max, Nelson and Chen, Min},
  namea = {Herbstritt, Marc},
  nameatype = {collaborator},
  date = {2010},
  pages = {16 pages},
  publisher = {Schloss Dagstuhl - Leibniz-Zentrum fuer Informatik GmbH, Wadern/Saarbruecken, Germany},
  doi = {10.4230/DFU.SCIVIZ.2010.259},
  url = {http://drops.dagstuhl.de/opus/volltexte/2010/2709/},
  urldate = {2023-01-24},
  abstract = {This article is intended as an update of the major survey by Max [40] on optical models for direct volume rendering. It provides a brief overview of the subject scope covered by [40], and brings recent developments, such as new shadow algorithms and refraction rendering, into the perspective. In particular, we examine three fundamentals aspects of direct volume rendering, namely the volume rendering integral, local illumination models and global illumination models, in a wavelength-independent manner. We review the developments on spectral volume rendering, in which visible light are considered as a form of electromagnetic radiation, optical models are implemented in conjunction with representations of spectral power distribution. This survey can provide a basis for, and encourage, new efforts for developing and using complex illumination models to achieve better realism and perception through optical correctness.},
  langid = {english},
  keywords = {000 Computer science knowledge general works,Computer Science},
  file = {C:\Users\chsey\Zotero\storage\Y5UC4G3R\Max 그리고 Chen - 2010 - Local and Global Illumination in the Volume Render.pdf}
}

@article{maxOpticalModelsDirect,
  title = {Optical {{Models}} for {{Direct Volume Rendering}}},
  author = {Max, Nelson},
  abstract = {This tutorial survey paper reviews several different models for light interaction with volume densities of absorbing, glowing, reflecting, and/or scattering material. They are, in order of increasing realism, absorption only, emission only, emission and absorption combined, single scattering of external illumination without shadows, single scattering with shadows, and multiple scattering. For each model I give the physical assumptions, describe the applications for which it is appropriate, derive the differential or integral equations for light transport, present calculations methods for solving them, and show output images for a data set representing a cloud. Special attention is given to calculation methods for the multiple scattering model.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\P88SFXED\Max - Optical Models for Direct Volume Rendering.pdf}
}

@online{McGrawHillDictionaryScientific,
  title = {The {{McGraw-Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}, {{Seventh Edition}} ({{Mcgraw Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}) | {{BibSonomy}}},
  url = {https://www.bibsonomy.org/bibtex/257725856823161f04cb3c336cd0adee?postOwner=baisemain&intraHash=db7a65f7407e6ffad9bf28ec75f00b3e},
  urldate = {2022-09-29}
}

@online{McGrawHillDictionaryScientifica,
  title = {The {{McGraw-Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}, {{Seventh Edition}} ({{Mcgraw Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}) | {{BibSonomy}}},
  url = {https://www.bibsonomy.org/bibtex/257725856823161f04cb3c336cd0adee?postOwner=baisemain&intraHash=db7a65f7407e6ffad9bf28ec75f00b3e},
  urldate = {2022-09-29}
}

@online{McGrawHillDictionaryScientificb,
  title = {The {{McGraw-Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}, {{Seventh Edition}} ({{Mcgraw Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}) | {{BibSonomy}}},
  url = {https://www.bibsonomy.org/bibtex/257725856823161f04cb3c336cd0adee?postOwner=baisemain&intraHash=db7a65f7407e6ffad9bf28ec75f00b3e},
  urldate = {2022-09-29}
}

@online{McGrawHillDictionaryScientificc,
  title = {The {{McGraw-Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}, {{Seventh Edition}} ({{Mcgraw Hill Dictionary}} of {{Scientific}} and {{Technical Terms}}) | {{BibSonomy}}},
  url = {https://www.bibsonomy.org/bibtex/257725856823161f04cb3c336cd0adee?postOwner=baisemain&intraHash=db7a65f7407e6ffad9bf28ec75f00b3e},
  urldate = {2022-09-29}
}

@inreference{MechanicalWatch2023,
  title = {Mechanical Watch},
  booktitle = {Wikipedia},
  date = {2023-11-04T05:39:54Z},
  url = {https://en.wikipedia.org/w/index.php?title=Mechanical_watch&oldid=1183420084},
  urldate = {2023-12-26},
  abstract = {A mechanical watch is a watch that uses a clockwork mechanism to measure the passage of time, as opposed to quartz watches which function using the vibration modes of a piezoelectric quartz tuning fork, or radio watches, which are quartz watches synchronized to an atomic clock via radio waves. A mechanical watch is driven by a mainspring which must be wound either periodically by hand or via a self-winding mechanism.  Its force is transmitted through a series of gears to power the balance wheel, a weighted wheel which oscillates back and forth at a constant rate. A device called an escapement releases the watch's wheels to move forward a small amount with each swing of the balance wheel, moving the watch's hands forward at a constant rate.  The escapement is what makes the 'ticking' sound which is heard in an operating mechanical watch. Mechanical watches evolved in Europe in the 17th century from spring powered clocks, which appeared in the 15th century. Mechanical watches are typically not as accurate as quartz watches, and they eventually require periodic cleaning and calibration by a skilled watchmaker.  Since the 1970s, quartz watches have taken over most of the watch market, and mechanical watches are now mostly marketed as a luxury product, purchased for their aesthetic and luxury values, for appreciation of their fine craftsmanship, or as a status symbol.},
  langid = {english},
  annotation = {Page Version ID: 1183420084}
}

@online{mehraAnalysisTaskTransferability2023,
  title = {Analysis of {{Task Transferability}} in {{Large Pre-trained Classifiers}}},
  author = {Mehra, Akshay and Zhang, Yunbei and Hamm, Jihun},
  date = {2023-07-03},
  eprint = {2307.00823},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2307.00823},
  urldate = {2024-01-05},
  abstract = {Transfer learning transfers the knowledge acquired by a model from a source task to multiple downstream target tasks with minimal fine-tuning. The success of transfer learning at improving performance, especially with the use of large pre-trained models has made transfer learning an essential tool in the machine learning toolbox. However, the conditions under which the performance is transferable to downstream tasks are not understood very well. In this work, we analyze the transfer of performance for classification tasks, when only the last linear layer of the source model is fine-tuned on the target task. We propose a novel Task Transfer Analysis approach that transforms the source distribution (and classifier) by changing the class prior distribution, label, and feature spaces to produce a new source distribution (and classifier) and allows us to relate the loss of the downstream task (i.e., transferability) to that of the source task. Concretely, our bound explains transferability in terms of the Wasserstein distance between the transformed source and downstream task's distribution, conditional entropy between the label distributions of the two tasks, and weighted loss of the source classifier on the source task. Moreover, we propose an optimization problem for learning the transforms of the source task to minimize the upper bound on transferability. We perform a large-scale empirical study by using state-of-the-art pre-trained models and demonstrate the effectiveness of our bound and optimization at predicting transferability. The results of our experiments demonstrate how factors such as task relatedness, pretraining method, and model architecture affect transferability.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\Mehra et al_2023_Analysis of Task Transferability in Large Pre-trained Classifiers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\25M8YXZY\\2307.html}
}

@online{mehtaMobileViTLightweightGeneralpurpose2022,
  title = {{{MobileViT}}: {{Light-weight}}, {{General-purpose}}, and {{Mobile-friendly Vision Transformer}}},
  shorttitle = {{{MobileViT}}},
  author = {Mehta, Sachin and Rastegari, Mohammad},
  date = {2022-03-04},
  eprint = {2110.02178},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2110.02178},
  url = {http://arxiv.org/abs/2110.02178},
  urldate = {2022-08-26},
  abstract = {Light-weight convolutional neural networks (CNNs) are the de-facto for mobile vision tasks. Their spatial inductive biases allow them to learn representations with fewer parameters across different vision tasks. However, these networks are spatially local. To learn global representations, self-attention-based vision trans-formers (ViTs) have been adopted. Unlike CNNs, ViTs are heavy-weight. In this paper, we ask the following question: is it possible to combine the strengths of CNNs and ViTs to build a light-weight and low latency network for mobile vision tasks? Towards this end, we introduce MobileViT, a light-weight and general-purpose vision transformer for mobile devices. MobileViT presents a different perspective for the global processing of information with transformers, i.e., transformers as convolutions. Our results show that MobileViT significantly outperforms CNN- and ViT-based networks across different tasks and datasets. On the ImageNet-1k dataset, MobileViT achieves top-1 accuracy of 78.4\% with about 6 million parameters, which is 3.2\% and 6.2\% more accurate than MobileNetv3 (CNN-based) and DeIT (ViT-based) for a similar number of parameters. On the MS-COCO object detection task, MobileViT is 5.7\% more accurate than MobileNetv3 for a similar number of parameters. Our source code is open-source and available at: https://github.com/apple/ml-cvnets},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\transformer\\Mehta_Rastegari_2022_MobileViT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KBFB5EJH\\2110.html}
}

@online{meschederOccupancyNetworksLearning2019,
  title = {Occupancy {{Networks}}: {{Learning 3D Reconstruction}} in {{Function Space}}},
  shorttitle = {Occupancy {{Networks}}},
  author = {Mescheder, Lars and Oechsle, Michael and Niemeyer, Michael and Nowozin, Sebastian and Geiger, Andreas},
  date = {2019-04-30},
  eprint = {1812.03828},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1812.03828},
  url = {http://arxiv.org/abs/1812.03828},
  urldate = {2023-08-05},
  abstract = {With the advent of deep neural networks, learning-based approaches for 3D reconstruction have gained popularity. However, unlike for images, in 3D there is no canonical representation which is both computationally and memory efficient yet allows for representing high-resolution geometry of arbitrary topology. Many of the state-of-the-art learning-based 3D reconstruction approaches can hence only represent very coarse 3D geometry or are limited to a restricted domain. In this paper, we propose Occupancy Networks, a new representation for learning-based 3D reconstruction methods. Occupancy networks implicitly represent the 3D surface as the continuous decision boundary of a deep neural network classifier. In contrast to existing approaches, our representation encodes a description of the 3D output at infinite resolution without excessive memory footprint. We validate that our representation can efficiently encode 3D structure and can be inferred from various kinds of input. Our experiments demonstrate competitive results, both qualitatively and quantitatively, for the challenging tasks of 3D reconstruction from single images, noisy point clouds and coarse discrete voxel grids. We believe that occupancy networks will become a useful tool in a wide variety of learning-based 3D tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\3d image understanding\\Mescheder et al_2019_Occupancy Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5IBKWLBL\\1812.html}
}

@online{michelAreSixteenHeads2019,
  title = {Are {{Sixteen Heads Really Better}} than {{One}}?},
  author = {Michel, Paul and Levy, Omer and Neubig, Graham},
  date = {2019-11-04},
  eprint = {1905.10650},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1905.10650},
  url = {http://arxiv.org/abs/1905.10650},
  urldate = {2023-10-19},
  abstract = {Attention is a powerful and ubiquitous mechanism for allowing neural models to focus on particular salient pieces of information by taking their weighted average when making predictions. In particular, multi-headed attention is a driving force behind many recent state-of-the-art NLP models such as Transformer-based MT models and BERT. These models apply multiple attention mechanisms in parallel, with each attention "head" potentially focusing on different parts of the input, which makes it possible to express sophisticated functions beyond the simple weighted average. In this paper we make the surprising observation that even if models have been trained using multiple heads, in practice, a large percentage of attention heads can be removed at test time without significantly impacting performance. In fact, some layers can even be reduced to a single head. We further examine greedy algorithms for pruning down models, and the potential speed, memory efficiency, and accuracy improvements obtainable therefrom. Finally, we analyze the results with respect to which parts of the model are more reliant on having multiple heads, and provide precursory evidence that training dynamics play a role in the gains provided by multi-head attention.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Michel et al_2019_Are Sixteen Heads Really Better than One.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FSZ7HMGF\\1905.html}
}

@online{MigugjusigSigacongaegTOP202022,
  title = {미국주식 시가총액 TOP20 순위변화 (1995-2022 28년간)},
  date = {2022-08-07T09:11:23+09:00},
  url = {https://etfs.tistory.com/entry/historical-us-market-cap-top20},
  urldate = {2023-12-17},
  abstract = {영원한 1등은 없다 미국주식 시가총액 상위 종목들의 연도별 변화를 조사해보았다. 1995년부터 2022년까지 TOP20이 기록된 사이트를 찾아서 옮겨옴 연도별 시가총액 TOP3 종목과 Market Capitalization, 티커(Ticker, 상장코드)를 표시하였다. TOP1 M.Cap Ticker TOP2 M.Cap Ticker TOP3 M.Cap Ticker 1995 GE 92B GE Exxon 83B XOM AT\&T 81B T 1996 GE 126B GE Coca-Cola 101B KO AT\&T 98B T 1997 GE 169B GE Coca-Cola 148B KO Exxon 126B XOM 1998 GE 260B GE Microsoft 199B MSFT Coca-Cola 185B KO 1999 ..},
  langid = {korean-han},
  organization = {금융치료실},
  file = {C:\Users\chsey\Zotero\storage\MYG4ZH87\historical-us-market-cap-top20.html}
}

@inproceedings{mikolovDistributedRepresentationsWords2013,
  title = {Distributed {{Representations}} of {{Words}} and {{Phrases}} and Their {{Compositionality}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  date = {2013},
  volume = {26},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2013/hash/9aa42b31882ec039965f3c4923ce901b-Abstract.html},
  urldate = {2022-09-25},
  abstract = {The recently introduced continuous Skip-gram model is an efficient method for learning high-quality distributed vector representations that capture a large number of precise syntactic and semantic word relationships.  In this paper we present several improvements that make the Skip-gram model more expressive and enable it to learn higher quality vectors more rapidly.  We show that by subsampling frequent words we obtain significant speedup,  and also learn higher quality representations as measured by our tasks. We also introduce Negative Sampling, a simplified variant of Noise Contrastive Estimation (NCE) that learns more accurate vectors for frequent words compared to the hierarchical softmax.   An inherent limitation of word representations is their indifference to word order and their inability to represent idiomatic phrases.  For example, the meanings of Canada'' and "Air'' cannot be easily combined to obtain "Air Canada''.  Motivated by this example, we present a simple and efficient method for finding phrases, and show that their vector representations can be accurately learned by the Skip-gram model. "},
  file = {Y:\paper\artificial intelligence\NLP\Mikolov et al_2013_Distributed Representations of Words and Phrases and their Compositionality.pdf}
}

@online{mildenhallNeRFDarkHigh2021,
  title = {{{NeRF}} in the {{Dark}}: {{High Dynamic Range View Synthesis}} from {{Noisy Raw Images}}},
  shorttitle = {{{NeRF}} in the {{Dark}}},
  author = {Mildenhall, Ben and Hedman, Peter and Martin-Brualla, Ricardo and Srinivasan, Pratul and Barron, Jonathan T.},
  date = {2021-11-26},
  eprint = {2111.13679},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2111.13679},
  urldate = {2023-06-26},
  abstract = {Neural Radiance Fields (NeRF) is a technique for high quality novel view synthesis from a collection of posed input images. Like most view synthesis methods, NeRF uses tonemapped low dynamic range (LDR) as input; these images have been processed by a lossy camera pipeline that smooths detail, clips highlights, and distorts the simple noise distribution of raw sensor data. We modify NeRF to instead train directly on linear raw images, preserving the scene's full dynamic range. By rendering raw output images from the resulting NeRF, we can perform novel high dynamic range (HDR) view synthesis tasks. In addition to changing the camera viewpoint, we can manipulate focus, exposure, and tonemapping after the fact. Although a single raw image appears significantly more noisy than a postprocessed one, we show that NeRF is highly robust to the zero-mean distribution of raw noise. When optimized over many noisy raw inputs (25-200), NeRF produces a scene representation so accurate that its rendered novel views outperform dedicated single and multi-image deep raw denoisers run on the same wide baseline input images. As a result, our method, which we call RawNeRF, can reconstruct scenes from extremely noisy images captured in near-darkness.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\2022 winter intern\\Mildenhall et al_2021_NeRF in the Dark.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9F5V763U\\2111.html}
}

@online{mildenhallNeRFRepresentingScenes2020,
  title = {{{NeRF}}: {{Representing Scenes}} as {{Neural Radiance Fields}} for {{View Synthesis}}},
  shorttitle = {{{NeRF}}},
  author = {Mildenhall, Ben and Srinivasan, Pratul P. and Tancik, Matthew and Barron, Jonathan T. and Ramamoorthi, Ravi and Ng, Ren},
  date = {2020-08-03},
  eprint = {2003.08934},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2003.08934},
  url = {http://arxiv.org/abs/2003.08934},
  urldate = {2023-01-02},
  abstract = {We present a method that achieves state-of-the-art results for synthesizing novel views of complex scenes by optimizing an underlying continuous volumetric scene function using a sparse set of input views. Our algorithm represents a scene using a fully-connected (non-convolutional) deep network, whose input is a single continuous 5D coordinate (spatial location \$(x,y,z)\$ and viewing direction \$(\textbackslash theta, \textbackslash phi)\$) and whose output is the volume density and view-dependent emitted radiance at that spatial location. We synthesize views by querying 5D coordinates along camera rays and use classic volume rendering techniques to project the output colors and densities into an image. Because volume rendering is naturally differentiable, the only input required to optimize our representation is a set of images with known camera poses. We describe how to effectively optimize neural radiance fields to render photorealistic novel views of scenes with complicated geometry and appearance, and demonstrate results that outperform prior work on neural rendering and view synthesis. View synthesis results are best viewed as videos, so we urge readers to view our supplementary video for convincing comparisons.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Mildenhall et al_2020_NeRF2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9VKMLNAR\\2003.html}
}

@online{mildenhallNeRFRepresentingScenes2020a,
  title = {{{NeRF}}: {{Representing Scenes}} as {{Neural Radiance Fields}} for {{View Synthesis}}},
  shorttitle = {{{NeRF}}},
  author = {Mildenhall, Ben and Srinivasan, Pratul P. and Tancik, Matthew and Barron, Jonathan T. and Ramamoorthi, Ravi and Ng, Ren},
  date = {2020-08-03},
  eprint = {2003.08934},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2003.08934},
  url = {http://arxiv.org/abs/2003.08934},
  urldate = {2022-10-27},
  abstract = {We present a method that achieves state-of-the-art results for synthesizing novel views of complex scenes by optimizing an underlying continuous volumetric scene function using a sparse set of input views. Our algorithm represents a scene using a fully-connected (non-convolutional) deep network, whose input is a single continuous 5D coordinate (spatial location \$(x,y,z)\$ and viewing direction \$(\textbackslash theta, \textbackslash phi)\$) and whose output is the volume density and view-dependent emitted radiance at that spatial location. We synthesize views by querying 5D coordinates along camera rays and use classic volume rendering techniques to project the output colors and densities into an image. Because volume rendering is naturally differentiable, the only input required to optimize our representation is a set of images with known camera poses. We describe how to effectively optimize neural radiance fields to render photorealistic novel views of scenes with complicated geometry and appearance, and demonstrate results that outperform prior work on neural rendering and view synthesis. View synthesis results are best viewed as videos, so we urge readers to view our supplementary video for convincing comparisons.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Mildenhall et al_2020_NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KG63IKTJ\\2003.html}
}

@online{misraCrossstitchNetworksMultitask2016,
  title = {Cross-Stitch {{Networks}} for {{Multi-task Learning}}},
  author = {Misra, Ishan and Shrivastava, Abhinav and Gupta, Abhinav and Hebert, Martial},
  date = {2016-04-12},
  eprint = {1604.03539},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1604.03539},
  url = {http://arxiv.org/abs/1604.03539},
  urldate = {2023-08-05},
  abstract = {Multi-task learning in Convolutional Networks has displayed remarkable success in the field of recognition. This success can be largely attributed to learning shared representations from multiple supervisory tasks. However, existing multi-task approaches rely on enumerating multiple network architectures specific to the tasks at hand, that do not generalize. In this paper, we propose a principled approach to learn shared representations in ConvNets using multi-task learning. Specifically, we propose a new sharing unit: "cross-stitch" unit. These units combine the activations from multiple networks and can be trained end-to-end. A network with cross-stitch units can learn an optimal combination of shared and task-specific representations. Our proposed method generalizes across multiple tasks and shows dramatically improved performance over baseline methods for categories with few training examples.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\lifelong learning\\Misra et al_2016_Cross-stitch Networks for Multi-task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6UFEDKVC\\1604.html}
}

@inproceedings{misraRedWineRed2017,
  title = {From {{Red Wine}} to {{Red Tomato}}: {{Composition}} with {{Context}}},
  shorttitle = {From {{Red Wine}} to {{Red Tomato}}},
  booktitle = {2017 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Misra, Ishan and Gupta, Abhinav and Hebert, Martial},
  date = {2017-07},
  pages = {1160--1169},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2017.129},
  abstract = {Compositionality and contextuality are key building blocks of intelligence. They allow us to compose known concepts to generate new and complex ones. However, traditional learning methods do not model both these properties and require copious amounts of labeled data to learn new concepts. A large fraction of existing techniques, e.g., using late fusion, compose concepts but fail to model contextuality. For example, red in red wine is different from red in red tomatoes. In this paper, we present a simple method that respects contextuality in order to compose classifiers of known visual concepts. Our method builds upon the intuition that classifiers lie in a smooth space where compositional transforms can be modeled. We show how it can generalize to unseen combinations of concepts. Our results on composing attributes, objects as well as composing subject, predicate, and objects demonstrate its strong generalization performance compared to baselines. Finally, we present detailed analysis of our method and highlight its properties.},
  eventtitle = {2017 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  keywords = {Automobiles,Computer vision,Context modeling,notion,Training,Training data,Transforms,Visualization},
  file = {Y:\paper\computer_vision_topics_18\lifelong learning\Misra et al_2017_From Red Wine to Red Tomato.pdf}
}

@online{misraSelfSupervisedLearningPretextInvariant2019,
  title = {Self-{{Supervised Learning}} of {{Pretext-Invariant Representations}}},
  author = {Misra, Ishan and family=Maaten, given=Laurens, prefix=van der, useprefix=true},
  date = {2019-12-04},
  eprint = {1912.01991},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1912.01991},
  url = {http://arxiv.org/abs/1912.01991},
  urldate = {2023-08-05},
  abstract = {The goal of self-supervised learning from images is to construct image representations that are semantically meaningful via pretext tasks that do not require semantic annotations for a large training set of images. Many pretext tasks lead to representations that are covariant with image transformations. We argue that, instead, semantic representations ought to be invariant under such transformations. Specifically, we develop Pretext-Invariant Representation Learning (PIRL, pronounced as "pearl") that learns invariant representations based on pretext tasks. We use PIRL with a commonly used pretext task that involves solving jigsaw puzzles. We find that PIRL substantially improves the semantic quality of the learned image representations. Our approach sets a new state-of-the-art in self-supervised learning from images on several popular benchmarks for self-supervised learning. Despite being unsupervised, PIRL outperforms supervised pre-training in learning image representations for object detection. Altogether, our results demonstrate the potential of self-supervised learning of image representations with good invariance properties.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\self supervised learning\\Misra_van der Maaten_2019_Self-Supervised Learning of Pretext-Invariant Representations.pdf;C\:\\Users\\chsey\\Zotero\\storage\\78EQCDXK\\1912.html}
}

@article{mitchellAbstractionAnalogyMakingArtificial2021,
  title = {Abstraction and {{Analogy-Making}} in {{Artificial Intelligence}}},
  author = {Mitchell, Melanie},
  date = {2021-12},
  journaltitle = {Annals of the New York Academy of Sciences},
  shortjournal = {Annals of the New York Academy of Sciences},
  volume = {1505},
  number = {1},
  eprint = {2102.10717},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {79--101},
  issn = {0077-8923, 1749-6632},
  doi = {10.1111/nyas.14619},
  url = {http://arxiv.org/abs/2102.10717},
  urldate = {2023-11-17},
  abstract = {Conceptual abstraction and analogy-making are key abilities underlying humans' abilities to learn, reason, and robustly adapt their knowledge to new domains. Despite of a long history of research on constructing AI systems with these abilities, no current AI system is anywhere close to a capability of forming humanlike abstractions or analogies. This paper reviews the advantages and limitations of several approaches toward this goal, including symbolic methods, deep learning, and probabilistic program induction. The paper concludes with several proposals for designing challenge tasks and evaluation measures in order to make quantifiable and generalizable progress in this area.},
  keywords = {Computer Science - Artificial Intelligence},
  file = {Y\:\\paper\\2023 graduation\\Mitchell_2021_Abstraction and Analogy-Making in Artificial Intelligence.pdf;C\:\\Users\\chsey\\Zotero\\storage\\R96ZSSAU\\2102.html}
}

@article{mitchellAbstractionAnalogyMakingArtificial2021a,
  title = {Abstraction and {{Analogy-Making}} in {{Artificial Intelligence}}},
  author = {Mitchell, Melanie},
  date = {2021-12},
  journaltitle = {Annals of the New York Academy of Sciences},
  shortjournal = {Annals NY Academy of Science},
  volume = {1505},
  number = {1},
  eprint = {2102.10717},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {79--101},
  issn = {0077-8923, 1749-6632},
  doi = {10.1111/nyas.14619},
  url = {http://arxiv.org/abs/2102.10717},
  urldate = {2023-06-30},
  abstract = {Conceptual abstraction and analogy-making are key abilities underlying humans' abilities to learn, reason, and robustly adapt their knowledge to new domains. Despite of a long history of research on constructing AI systems with these abilities, no current AI system is anywhere close to a capability of forming humanlike abstractions or analogies. This paper reviews the advantages and limitations of several approaches toward this goal, including symbolic methods, deep learning, and probabilistic program induction. The paper concludes with several proposals for designing challenge tasks and evaluation measures in order to make quantifiable and generalizable progress in this area.},
  keywords = {Computer Science - Artificial Intelligence,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Mitchell_2021_Abstraction and Analogy-Making in Artificial Intelligence.pdf;C\:\\Users\\chsey\\Zotero\\storage\\IUHPAECE\\2102.html}
}

@article{mizrahi4MMassivelyMultimodal,
  title = {{{4M}}: {{Massively Multimodal Masked Modeling}}},
  author = {Mizrahi, David and Bachmann, Roman and Yeo, Teresa and Gao, Mingfei and Dehghan, Afshin and Zamir, Amir},
  abstract = {Current machine learning models for vision are often highly specialized and limited to a single modality and task. In contrast, recent large language models exhibit a wide range of capabilities, hinting at a possibility for similarly versatile models in computer vision. In this paper, we take a step in this direction and propose a multimodal training scheme called 4M. It consists of training a single unified Transformer encoder-decoder using a masked modeling objective across a wide range of input/output modalities – including text, images, geometric, and semantic modalities, as well as neural network feature maps. 4M achieves scalability by unifying the representation space of all modalities through mapping them into discrete tokens and performing multimodal masked modeling on a small randomized subset of tokens. 4M leads to models that exhibit several key capabilities: (1) they can perform a diverse set of vision tasks out of the box, (2) they excel when fine-tuned for unseen downstream tasks or new input modalities, and (3) they can function as a generative model that can be conditioned on arbitrary modalities, enabling a wide variety of expressive multimodal editing capabilities with remarkable flexibility.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\3G2VSJAU\Mizrahi 등 - 4M Massively Multimodal Masked Modeling.pdf}
}

@article{mohanIterativeReweightedAlgorithms,
  title = {Iterative {{Reweighted Algorithms}} for {{Matrix Rank Minimization}}},
  author = {Mohan, Karthik and Fazel, Maryam},
  abstract = {The problem of minimizing the rank of a matrix subject to affine constraints has applications in several areas including machine learning, and is known to be NP-hard. A tractable relaxation for this problem is nuclear norm (or trace norm) minimization, which is guaranteed to find the minimum rank matrix under suitable assumptions. In this paper, we propose a family of Iterative Reweighted Least Squares algorithms IRLS-p (with 0 ≤ p ≤ 1), as a computationally efficient way to improve over the performance of nuclear norm minimization. The algorithms can be viewed as (locally) minimizing certain smooth approximations to the rank function. When p = 1, we give theoretical guarantees similar to those for nuclear norm minimization, that is, recovery of low-rank matrices under certain assumptions on the operator defining the constraints. For p {$<$} 1, IRLSp shows better empirical performance in terms of recovering low-rank matrices than nuclear norm minimization. We provide an efficient implementation for IRLS-p, and also present a related family of algorithms, sIRLS-p. These algorithms exhibit competitive run times and improved recovery when compared to existing algorithms for random instances of the matrix completion problem, as well as on the MovieLens movie recommendation data set.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\GDZT63C8\Mohan 그리고 Fazel - Iterative Reweighted Algorithms for Matrix Rank Mi.pdf}
}

@article{mohanIterativeReweightedAlgorithmsa,
  title = {Iterative {{Reweighted Algorithms}} for {{Matrix Rank Minimization}}},
  author = {Mohan, Karthik and Fazel, Maryam},
  abstract = {The problem of minimizing the rank of a matrix subject to affine constraints has applications in several areas including machine learning, and is known to be NP-hard. A tractable relaxation for this problem is nuclear norm (or trace norm) minimization, which is guaranteed to find the minimum rank matrix under suitable assumptions. In this paper, we propose a family of Iterative Reweighted Least Squares algorithms IRLS-p (with 0 ≤ p ≤ 1), as a computationally efficient way to improve over the performance of nuclear norm minimization. The algorithms can be viewed as (locally) minimizing certain smooth approximations to the rank function. When p = 1, we give theoretical guarantees similar to those for nuclear norm minimization, that is, recovery of low-rank matrices under certain assumptions on the operator defining the constraints. For p {$<$} 1, IRLSp shows better empirical performance in terms of recovering low-rank matrices than nuclear norm minimization. We provide an efficient implementation for IRLS-p, and also present a related family of algorithms, sIRLS-p. These algorithms exhibit competitive run times and improved recovery when compared to existing algorithms for random instances of the matrix completion problem, as well as on the MovieLens movie recommendation data set.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Mohan_Fazel_Iterative Reweighted Algorithms for Matrix Rank Minimization.pdf}
}

@article{morisDataAugmentationApproaches2021,
  title = {Data Augmentation Approaches Using Cycle-Consistent Adversarial Networks for Improving {{COVID-19}} Screening in Portable Chest {{X-ray}} Images},
  author = {Morís, Daniel Iglesias and family=Moura Ramos, given=José Joaquim, prefix=de, useprefix=true and Buján, Jorge Novo and Hortas, Marcos Ortega},
  date = {2021-12-15},
  journaltitle = {Expert Systems with Applications},
  shortjournal = {Expert Systems with Applications},
  volume = {185},
  pages = {115681},
  issn = {0957-4174},
  doi = {10.1016/j.eswa.2021.115681},
  url = {https://www.sciencedirect.com/science/article/pii/S0957417421010666},
  urldate = {2022-07-09},
  abstract = {The current COVID-19 pandemic, that has caused more than 100 million cases as well as more than two million deaths worldwide, demands the development of fast and accurate diagnostic methods despite the lack of available samples. This disease mainly affects the respiratory system of the patients and can lead to pneumonia and to severe cases of acute respiratory syndrome that result in the formation of several pathological structures in the lungs. These pathological structures can be explored taking advantage of chest X-ray imaging. As a recommendation for the health services, portable chest X-ray devices should be used instead of conventional fixed machinery, in order to prevent the spread of the pathogen. However, portable devices present several problems (specially those related with capture quality). Moreover, the subjectivity and the fatigue of the clinicians lead to a very difficult diagnostic process. To overcome that, computer-aided methodologies can be very useful even taking into account the lack of available samples that the COVID-19 affectation shows. In this work, we propose an improvement in the performance of COVID-19 screening, taking advantage of several cycle generative adversarial networks to generate useful and relevant synthetic images to solve the lack of COVID-19 samples, in the context of poor quality and low detail datasets obtained from portable devices. For validating this proposal for improved COVID-19 screening, several experiments were conducted. The results demonstrate that this data augmentation strategy improves the performance of a previous COVID-19 screening proposal, achieving an accuracy of 98.61\% when distinguishing among NON-COVID-19 (i.e. normal control samples and samples with pathologies others than COVID-19) and genuine COVID-19 samples. It is remarkable that this methodology can be extrapolated to other pulmonary pathologies and even other medical imaging domains to overcome the data scarcity.},
  langid = {english},
  keywords = {COVID-19,CycleGAN,Data augmentation,Deep learning,Screening,X-ray portable device},
  file = {Y:\paper\2022 summer intern\assignment\data augmentation\Morís et al_2021_Data augmentation approaches using cycle-consistent adversarial networks for.pdf}
}

@online{mosbachFewshotFinetuningVs2023,
  title = {Few-Shot {{Fine-tuning}} vs. {{In-context Learning}}: {{A Fair Comparison}} and {{Evaluation}}},
  shorttitle = {Few-Shot {{Fine-tuning}} vs. {{In-context Learning}}},
  author = {Mosbach, Marius and Pimentel, Tiago and Ravfogel, Shauli and Klakow, Dietrich and Elazar, Yanai},
  date = {2023-05-30},
  eprint = {2305.16938},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.16938},
  urldate = {2023-12-24},
  abstract = {Few-shot fine-tuning and in-context learning are two alternative strategies for task adaptation of pre-trained language models. Recently, in-context learning has gained popularity over fine-tuning due to its simplicity and improved out-of-domain generalization, and because extensive evidence shows that fine-tuned models pick up on spurious correlations. Unfortunately, previous comparisons of the two approaches were done using models of different sizes. This raises the question of whether the observed weaker out-of-domain generalization of fine-tuned models is an inherent property of fine-tuning or a limitation of the experimental setup. In this paper, we compare the generalization of few-shot fine-tuning and in-context learning to challenge datasets, while controlling for the models used, the number of examples, and the number of parameters, ranging from 125M to 30B. Our results show that fine-tuned language models can in fact generalize well out-of-domain. We find that both approaches generalize similarly; they exhibit large variation and depend on properties such as model size and the number of examples, highlighting that robust task adaptation remains a challenge.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Mosbach et al_2023_Few-shot Fine-tuning vs.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LG3T9ENU\\2305.html}
}

@inproceedings{mottaghiRoleContextObject2014,
  title = {The {{Role}} of {{Context}} for {{Object Detection}} and {{Semantic Segmentation}} in the {{Wild}}},
  booktitle = {2014 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  author = {Mottaghi, Roozbeh and Chen, Xianjie and Liu, Xiaobai and Cho, Nam-Gyu and Lee, Seong-Whan and Fidler, Sanja and Urtasun, Raquel and Yuille, Alan},
  date = {2014-06},
  pages = {891--898},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2014.119},
  abstract = {In this paper we study the role of context in existing state-of-the-art detection and segmentation approaches. Towards this goal, we label every pixel of PASCAL VOC 2010 detection challenge with a semantic category. We believe this data will provide plenty of challenges to the community, as it contains 520 additional classes for semantic segmentation and object detection. Our analysis shows that nearest neighbor based approaches perform poorly on semantic segmentation of contextual classes, showing the variability of PASCAL imagery. Furthermore, improvements of existing contextual models for detection is rather modest. In order to push forward the performance in this difficult scenario, we propose a novel deformable part-based model, which exploits both local context around each candidate detection as well as global context at the level of the scene. We show that this contextual reasoning significantly helps in detecting objects at all scales.},
  eventtitle = {2014 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  keywords = {Buildings,Context,Context modeling,Image segmentation,notion,Object detection,Semantics,Vegetation},
  file = {Y:\paper\computer_vision_topics_18\contextual cues\Mottaghi et al_2014_The Role of Context for Object Detection and Semantic Segmentation in the Wild.pdf}
}

@online{mouT2IAdapterLearningAdapters2023,
  title = {{{T2I-Adapter}}: {{Learning Adapters}} to {{Dig}} out {{More Controllable Ability}} for {{Text-to-Image Diffusion Models}}},
  shorttitle = {{{T2I-Adapter}}},
  author = {Mou, Chong and Wang, Xintao and Xie, Liangbin and Wu, Yanze and Zhang, Jian and Qi, Zhongang and Shan, Ying and Qie, Xiaohu},
  date = {2023-03-20},
  eprint = {2302.08453},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2302.08453},
  url = {http://arxiv.org/abs/2302.08453},
  urldate = {2024-01-24},
  abstract = {The incredible generative ability of large-scale text-to-image (T2I) models has demonstrated strong power of learning complex structures and meaningful semantics. However, relying solely on text prompts cannot fully take advantage of the knowledge learned by the model, especially when flexible and accurate controlling (e.g., color and structure) is needed. In this paper, we aim to ``dig out" the capabilities that T2I models have implicitly learned, and then explicitly use them to control the generation more granularly. Specifically, we propose to learn simple and lightweight T2I-Adapters to align internal knowledge in T2I models with external control signals, while freezing the original large T2I models. In this way, we can train various adapters according to different conditions, achieving rich control and editing effects in the color and structure of the generation results. Further, the proposed T2I-Adapters have attractive properties of practical value, such as composability and generalization ability. Extensive experiments demonstrate that our T2I-Adapter has promising generation quality and a wide range of applications.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Mou et al_2023_T2I-Adapter.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EQGFJFRB\\2302.html}
}

@article{mullerInstantNeuralGraphics2022,
  title = {Instant {{Neural Graphics Primitives}} with a {{Multiresolution Hash Encoding}}},
  author = {Müller, Thomas and Evans, Alex and Schied, Christoph and Keller, Alexander},
  date = {2022-07},
  journaltitle = {ACM Transactions on Graphics},
  shortjournal = {ACM Trans. Graph.},
  volume = {41},
  number = {4},
  eprint = {2201.05989},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--15},
  issn = {0730-0301, 1557-7368},
  doi = {10.1145/3528223.3530127},
  url = {http://arxiv.org/abs/2201.05989},
  urldate = {2023-01-17},
  abstract = {Neural graphics primitives, parameterized by fully connected neural networks, can be costly to train and evaluate. We reduce this cost with a versatile new input encoding that permits the use of a smaller network without sacrificing quality, thus significantly reducing the number of floating point and memory access operations: a small neural network is augmented by a multiresolution hash table of trainable feature vectors whose values are optimized through stochastic gradient descent. The multiresolution structure allows the network to disambiguate hash collisions, making for a simple architecture that is trivial to parallelize on modern GPUs. We leverage this parallelism by implementing the whole system using fully-fused CUDA kernels with a focus on minimizing wasted bandwidth and compute operations. We achieve a combined speedup of several orders of magnitude, enabling training of high-quality neural graphics primitives in a matter of seconds, and rendering in tens of milliseconds at a resolution of \$\{1920\textbackslash!\textbackslash times\textbackslash!1080\}\$.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Müller et al_2022_Instant Neural Graphics Primitives with a Multiresolution Hash Encoding.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DU8U7DR7\\2201.html}
}

@article{mullerRealtimeNeuralRadiance2021,
  title = {Real-Time {{Neural Radiance Caching}} for {{Path Tracing}}},
  author = {Müller, Thomas and Rousselle, Fabrice and Novák, Jan and Keller, Alexander},
  date = {2021-08-31},
  journaltitle = {ACM Transactions on Graphics},
  shortjournal = {ACM Trans. Graph.},
  volume = {40},
  number = {4},
  eprint = {2106.12372},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--16},
  issn = {0730-0301, 1557-7368},
  doi = {10.1145/3450626.3459812},
  url = {http://arxiv.org/abs/2106.12372},
  urldate = {2023-01-29},
  abstract = {We present a real-time neural radiance caching method for path-traced global illumination. Our system is designed to handle fully dynamic scenes, and makes no assumptions about the lighting, geometry, and materials. The data-driven nature of our approach sidesteps many difficulties of caching algorithms, such as locating, interpolating, and updating cache points. Since pretraining neural networks to handle novel, dynamic scenes is a formidable generalization challenge, we do away with pretraining and instead achieve generalization via adaptation, i.e. we opt for training the radiance cache while rendering. We employ self-training to provide low-noise training targets and simulate infinite-bounce transport by merely iterating few-bounce training updates. The updates and cache queries incur a mild overhead -- about 2.6ms on full HD resolution -- thanks to a streaming implementation of the neural network that fully exploits modern hardware. We demonstrate significant noise reduction at the cost of little induced bias, and report state-of-the-art, real-time performance on a number of challenging scenarios.},
  keywords = {Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Müller et al_2021_Real-time Neural Radiance Caching for Path Tracing.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4M8EG79S\\2106.html}
}

@online{mullerTrivialAugmentTuningfreeStateoftheArt2021,
  title = {{{TrivialAugment}}: {{Tuning-free Yet State-of-the-Art Data Augmentation}}},
  shorttitle = {{{TrivialAugment}}},
  author = {Müller, Samuel G. and Hutter, Frank},
  date = {2021-08-17},
  eprint = {2103.10158},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.10158},
  urldate = {2022-07-20},
  abstract = {Automatic augmentation methods have recently become a crucial pillar for strong model performance in vision tasks. While existing automatic augmentation methods need to trade off simplicity, cost and performance, we present a most simple baseline, TrivialAugment, that outperforms previous methods for almost free. TrivialAugment is parameter-free and only applies a single augmentation to each image. Thus, TrivialAugment's effectiveness is very unexpected to us and we performed very thorough experiments to study its performance. First, we compare TrivialAugment to previous state-of-the-art methods in a variety of image classification scenarios. Then, we perform multiple ablation studies with different augmentation spaces, augmentation methods and setups to understand the crucial requirements for its performance. Additionally, we provide a simple interface to facilitate the widespread adoption of automatic augmentation methods, as well as our full code base for reproducibility. Since our work reveals a stagnation in many parts of automatic augmentation research, we end with a short proposal of best practices for sustained future progress in automatic augmentation methods.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\augmentation\\Müller_Hutter_2021_TrivialAugment.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WYIG74BF\\2103.html}
}

@online{MulrijeogGibanRendeoring,
  title = {물리적 기반 렌더링: 이론에서 구현까지},
  url = {https://pbr-book.org/3ed-2018/contents},
  urldate = {2023-01-21},
  file = {C:\Users\chsey\Zotero\storage\KRWAFQ9C\contents.html}
}

@article{murphyLimitsEconomicGrowth2022,
  title = {Limits to Economic Growth},
  author = {Murphy, Thomas W.},
  date = {2022-08},
  journaltitle = {Nature Physics},
  shortjournal = {Nat. Phys.},
  volume = {18},
  number = {8},
  pages = {844--847},
  publisher = {Nature Publishing Group},
  issn = {1745-2481},
  doi = {10.1038/s41567-022-01652-6},
  url = {https://www.nature.com/articles/s41567-022-01652-6},
  urldate = {2022-08-25},
  abstract = {Across the world, decisions on investment and policy are made under the assumption of continuous economic expansion. Fundamental physical limits may soon put an end to this phase of development, as foreshadowed by the 1972 report The Limits to Growth.},
  issue = {8},
  langid = {english},
  keywords = {Applied physics,Energy science and technology},
  file = {Y:\paper\personal interest\Murphy_2022_Limits to economic growth.pdf}
}

@inproceedings{nacsonImplicitBiasStep2022,
  title = {Implicit {{Bias}} of the {{Step Size}} in {{Linear Diagonal Neural Networks}}},
  booktitle = {Proceedings of the 39th {{International Conference}} on {{Machine Learning}}},
  author = {Nacson, Mor Shpigel and Ravichandran, Kavya and Srebro, Nathan and Soudry, Daniel},
  date = {2022-06-28},
  pages = {16270--16295},
  publisher = {PMLR},
  issn = {2640-3498},
  url = {https://proceedings.mlr.press/v162/nacson22a.html},
  urldate = {2024-03-28},
  abstract = {Focusing on diagonal linear networks as a model for understanding the implicit bias in underdetermined models, we show how the gradient descent step size can have a large qualitative effect on the implicit bias, and thus on generalization ability. In particular, we show how using large step size for non-centered data can change the implicit bias from a "kernel" type behavior to a "rich" (sparsity-inducing) regime — even when gradient flow, studied in previous works, would not escape the "kernel" regime. We do so by using dynamic stability, proving that convergence to dynamically stable global minima entails a bound on some weighted ℓ1ℓ1\textbackslash ell\_1-norm of the linear predictor, i.e. a "rich" regime. We prove this leads to good generalization in a sparse regression setting.},
  eventtitle = {International {{Conference}} on {{Machine Learning}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Nacson et al_2022_Implicit Bias of the Step Size in Linear Diagonal Neural Networks.pdf}
}

@online{najdenkoskaMetaLearningBridge2023,
  title = {Meta {{Learning}} to {{Bridge Vision}} and {{Language Models}} for {{Multimodal Few-Shot Learning}}},
  author = {Najdenkoska, Ivona and Zhen, Xiantong and Worring, Marcel},
  date = {2023-02-28},
  eprint = {2302.14794},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2302.14794},
  urldate = {2024-07-31},
  abstract = {Multimodal few-shot learning is challenging due to the large domain gap between vision and language modalities. Existing methods are trying to communicate visual concepts as prompts to frozen language models, but rely on hand-engineered task induction to reduce the hypothesis space. To make the whole process learnable, we introduce a multimodal meta-learning approach. Specifically, our approach decomposes the training of the model into a set of related multimodal few-shot tasks. We define a meta-mapper network, acting as a meta-learner, to efficiently bridge frozen large-scale vision and language models and leverage their already learned capacity. By updating the learnable parameters only of the meta-mapper, it learns to accrue shared meta-knowledge among these tasks. Thus, it can rapidly adapt to newly presented samples with only a few gradient updates. Importantly, it induces the task in a completely data-driven manner, with no need for a hand-engineered task induction. We evaluate our approach on recently proposed multimodal few-shot benchmarks, measuring how rapidly the model can bind novel visual concepts to words and answer visual questions by observing only a limited set of labeled examples. The experimental results show that our meta-learning approach outperforms the baseline across multiple datasets and various training settings while being computationally more efficient.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\LLMYHYQI\Najdenkoska 등 - 2023 - Meta Learning to Bridge Vision and Language Models.pdf}
}

@online{nakahiraMatrixDifferentiationDiagrammatic2022,
  title = {Matrix Differentiation with Diagrammatic Notation},
  author = {Nakahira, Kenji},
  date = {2022-07-10},
  eprint = {2207.04377},
  eprinttype = {arXiv},
  eprintclass = {eess, math},
  url = {http://arxiv.org/abs/2207.04377},
  urldate = {2023-05-08},
  abstract = {We propose a diagrammatic notation for matrix differentiation. Our new notation enables us to derive formulas for matrix differentiation more easily than the usual matrix (or index) notation. We demonstrate the effectiveness of our notation through several examples.},
  pubstate = {prepublished},
  keywords = {Electrical Engineering and Systems Science - Signal Processing,Mathematics - Rings and Algebras},
  file = {Y\:\\paper\\textbook\\Nakahira_2022_Matrix differentiation with diagrammatic notation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CMUCGT9X\\2207.html}
}

@online{nakkiranDeepDoubleDescent2019,
  title = {Deep {{Double Descent}}: {{Where Bigger Models}} and {{More Data Hurt}}},
  shorttitle = {Deep {{Double Descent}}},
  author = {Nakkiran, Preetum and Kaplun, Gal and Bansal, Yamini and Yang, Tristan and Barak, Boaz and Sutskever, Ilya},
  date = {2019-12-04},
  eprint = {1912.02292},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1912.02292},
  url = {http://arxiv.org/abs/1912.02292},
  urldate = {2024-04-21},
  abstract = {We show that a variety of modern deep learning tasks exhibit a "double-descent" phenomenon where, as we increase model size, performance first gets worse and then gets better. Moreover, we show that double descent occurs not just as a function of model size, but also as a function of the number of training epochs. We unify the above phenomena by defining a new complexity measure we call the effective model complexity and conjecture a generalized double descent with respect to this measure. Furthermore, our notion of model complexity allows us to identify certain regimes where increasing (even quadrupling) the number of train samples actually hurts test performance.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Nakkiran et al_2019_Deep Double Descent.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KFB5FEYH\\1912.html}
}

@article{nalepaDataAugmentationBrainTumor2019,
  title = {Data {{Augmentation}} for {{Brain-Tumor Segmentation}}: {{A Review}}},
  shorttitle = {Data {{Augmentation}} for {{Brain-Tumor Segmentation}}},
  author = {Nalepa, Jakub and Marcinkiewicz, Michal and Kawulok, Michal},
  date = {2019},
  journaltitle = {Frontiers in Computational Neuroscience},
  volume = {13},
  issn = {1662-5188},
  url = {https://www.frontiersin.org/articles/10.3389/fncom.2019.00083},
  urldate = {2022-07-20},
  abstract = {Data augmentation is a popular technique which helps improve generalization capabilities of deep neural networks, and can be perceived as implicit regularization. It plays a pivotal role in scenarios in which the amount of high-quality ground-truth data is limited, and acquiring new examples is costly and time-consuming. This is a very common problem in medical image analysis, especially tumor delineation. In this paper, we review the current advances in data-augmentation techniques applied to magnetic resonance images of brain tumors. To better understand the practical aspects of such algorithms, we investigate the papers submitted to the Multimodal Brain Tumor Segmentation Challenge (BraTS 2018 edition), as the BraTS dataset became a standard benchmark for validating existent and emerging brain-tumor detection and segmentation techniques. We verify which data augmentation approaches were exploited and what was their impact on the abilities of underlying supervised learners. Finally, we highlight the most promising research directions to follow in order to synthesize high-quality artificial brain-tumor examples which can boost the generalization abilities of deep models.},
  file = {Y:\paper\2022 summer intern\assignment\data augmentation\Nalepa et al_2019_Data Augmentation for Brain-Tumor Segmentation.pdf}
}

@online{naseryPLeaSMergingModels2024,
  title = {{{PLeaS}} -- {{Merging Models}} with {{Permutations}} and {{Least Squares}}},
  author = {Nasery, Anshul and Hayase, Jonathan and Koh, Pang Wei and Oh, Sewoong},
  date = {2024-07-02},
  eprint = {2407.02447},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2407.02447},
  urldate = {2024-09-25},
  abstract = {The democratization of machine learning systems has made the process of fine-tuning accessible to a large number of practitioners, leading to a wide range of open-source models fine-tuned on specialized tasks and datasets. Recent work has proposed to merge such models to combine their functionalities. However, prior approaches are restricted to models that are fine-tuned from the same base model. Furthermore, the final merged model is typically restricted to be of the same size as the original models. In this work, we propose a new two-step algorithm to merge models—termed PLeaS—which relaxes these constraints. First, leveraging the Permutation symmetries inherent in the two models, PLeaS partially matches nodes in each layer by maximizing alignment. Next, PLeaS computes the weights of the merged model as a layer-wise Least Squares solution to minimize the approximation error between the features of the merged model and the permuted features of the original models. into a single model of a desired size, even when the two original models are fine-tuned from different base models. We also present a variant of our method which can merge models without using data from the fine-tuning domains. We demonstrate our method to merge ResNet models trained with shared and different label spaces , and show that we can perform better than the state-of-the-art merging methods by 8 to 15 percentage points for the same target compute while merging models trained on DomainNet and fine-grained classification tasks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\WDBH58YS\Nasery 등 - 2024 - PLeaS -- Merging Models with Permutations and Leas.pdf}
}

@article{nasrollahiSuperresolutionComprehensiveSurvey2014,
  title = {Super-Resolution: A Comprehensive Survey},
  shorttitle = {Super-Resolution},
  author = {Nasrollahi, Kamal and Moeslund, Thomas B.},
  date = {2014-08},
  journaltitle = {Machine Vision and Applications},
  shortjournal = {Machine Vision and Applications},
  volume = {25},
  number = {6},
  pages = {1423--1468},
  issn = {0932-8092, 1432-1769},
  doi = {10.1007/s00138-014-0623-4},
  url = {http://link.springer.com/10.1007/s00138-014-0623-4},
  urldate = {2022-09-30},
  abstract = {Super-resolution, the process of obtaining one or more high-resolution images from one or more low-resolution observations, has been a very attractive research topic over the last two decades. It has found practical applications in many real world problems in different fields, from satellite and aerial imaging to medical image processing, to facial image analysis, text image analysis, sign and number plates reading, and biometrics recognition, to name a few. This has resulted in many research papers, each developing a new superresolution algorithm for a specific purpose. The current comprehensive survey provides an overview of most of these published works by grouping them in a broad taxonomy. For each of the groups in the taxonomy, the basic concepts of the algorithms are first explained and then the paths through which each of these groups have evolved are given in detail, by mentioning the contributions of different authors to the basic concepts of each group. Furthermore, common issues in super-resolution algorithms, such as imaging models and registration algorithms, optimization of the cost functions employed, dealing with color information, improvement factors, assessment of super-resolution algorithms, and the most commonly employed databases are discussed.},
  langid = {english},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Nasrollahi_Moeslund_2014_Super-resolution.pdf}
}

@article{nasrollahiSuperresolutionComprehensiveSurvey2014a,
  title = {Super-Resolution: A Comprehensive Survey},
  shorttitle = {Super-Resolution},
  author = {Nasrollahi, Kamal and Moeslund, Thomas B.},
  date = {2014-08},
  journaltitle = {Machine Vision and Applications},
  shortjournal = {Machine Vision and Applications},
  volume = {25},
  number = {6},
  pages = {1423--1468},
  issn = {0932-8092, 1432-1769},
  doi = {10.1007/s00138-014-0623-4},
  url = {http://link.springer.com/10.1007/s00138-014-0623-4},
  urldate = {2022-09-28},
  abstract = {Super-resolution, the process of obtaining one or more high-resolution images from one or more lowresolution observations, has been a very attractive research topic over the last two decades. It has found practical applications in many real-world problems in different fields, from satellite and aerial imaging to medical image processing, to facial image analysis, text image analysis, sign and number plates reading, and biometrics recognition, to name a few. This has resulted in many research papers, each developing a new super-resolution algorithm for a specific purpose. The current comprehensive survey provides an overview of most of these published works by grouping them in a broad taxonomy. For each of the groups in the taxonomy, the basic concepts of the algorithms are first explained and then the paths through which each of these groups have evolved are given in detail, by mentioning the contributions of different authors to the basic concepts of each group. Furthermore, common issues in super-resolution algorithms, such as imaging models and registration algorithms, optimization of the cost functions employed, dealing with color information, improvement factors, assessment of super-resolution algorithms, and the most commonly employed databases are discussed.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\super-resolution\Nasrollahi_Moeslund_2014_Super-resolution.pdf}
}

@online{NautilusSSN571,
  title = {Nautilus ({{SSN-571}})},
  url = {http://public2.nhhcaws.local/browse-by-topic/ships/submarines/uss-nautilus.html},
  urldate = {2023-12-28},
  abstract = {USS Nautilus (SSN-571) was commissioned at Groton, Connecticut, on 30 September 1954 with Commander Eugene P. Wilkinson as the boat’s first commander. The construction of Nautilus—the world’s first nuclear powered submarine—was made possible by the successful development of a nuclear propulsion plant by a group of scientists and engineers, under the leadership of Captain Hyman G. Rickover, at the Naval Reactors Branch of the Atomic Energy Commission. Following commissioning, Nautilus remained dockside for further construction and testing for the next several months. On 17 January 1955, she was underway on nuclear power. After sea trials and preliminary acceptance by the Navy, Nautilus headed south for shakedown on 10 May. While enroute to Puerto Rico, she remained submerged traveling 1,381 miles in 89.8 hours, the longest submerged cruise, to that date, by a submarine, and at the highest sustained submerged speed ever recorded for a period of more than one hour’s duration. In July and August, Nautilus conducted rigorous exercises with hunter-killer groups in Narragansett Bay, Rhode Island, and off Bermuda. She rounded out the year visiting several east coast Navy bases, a battery of torpedo firing tests, and standardization trials. The following year, Nautilus operated~out of Naval Submarine Base New London, Connecticut, where the effects of a submarine with increased speed and endurance were tested on contemporary anti-submarine warfare practices. The study found that anti-submarine practices, such as was used during World War II, were ineffective against a submarine which did not need to surface, could dive deeper, and could clear a search area in record time. In between testing, Nautilus conducted press tours and hosted several dignitaries from the Navy and Capitol Hill. On 4 February 1957, Nautilus logged her 60,000th nautical mile. It also marked another first for the boat, as the submarine was put into the Electric Boat Company Division of General Dynamics Corporation at Groton to replace the nuclear fuel core in her Westinghouse Electric submarine thermal reactor.~In early April, Nautilus operated off Bermuda with USS Seawolf (SSN-575)—the second nuclear powered submarine—before departing for the U.S. west coast on 15 May. While there, Nautilus participated in multiple exercises designed to acquaint the units of the Pacific Fleet with the capabilities of nuclear submarines. She returned to New London on 21 July. On 19 August, Nautilus departed New London for her first voyage under the Arctic polar ice pack. The 1,383 mile journey was significant, because previously U.S. submarines did not travel to the frozen northern oceans due to~diesel-electric boats could not travel freely under ice. The opening of the Arctic to Navy submarines allowed access to the previously protected waters of the Soviet Union. From the Arctic, Nautilus set sail for the eastern Atlantic to participate in NATO exercises off Norway and to visit various British and French ports. Nautilus returned to New London on 28 October where she underwent upkeep. On 25 April 1958, Nautilus was once again headed for the U.S. west coast where she made stops in San Diego, San Francisco, and Seattle. On 9 June, Nautilus departed Seattle to conduct the highly secret “Operation Sunshine,” a fully submerged transit under the North Pole. However, the first attempt was blocked by drift ice in the relatively shallow waters of the Chukchi Sea, and the submarine returned to Pearl Harbor. Her second attempt, begun on 23 July, proved successful.~Nautilus~submerged in the Barrow Sea on 1 August, transited the geographic North Pole on 3 August, and, after running submerged an additional 96 hours, surfaced off Greenland on 7 August. The commanding officer, Commander William R. Anderson, and the crew were subsequently personally congratulated by President Dwight D. Eisenhower and awarded the Presidential Unit Citation. Following fleet exercises in early 1959, Nautilus entered Portsmouth Naval Shipyard for her first complete overhaul. Updates~included the second replacement of the reactor core, overhaul of almost all machinery, new sensors, and other equipment. On 24 October 1960, Nautilus departed Portsmouth for her first deployment with Sixth Fleet in the Mediterranean. Although the deployment was relatively short, she managed to visit Rota, Spain; Valleta, Malta; and La Spezia, Italy. She returned to her homeport of New London on 16 December. By 1961, the Navy had about a dozen nuclear powered submarines in service. Nautilus continued to focus on evaluation tests for anti-submarine warfare improvements and various NATO exercises in the Atlantic. The pattern was broken in the fall of 1962, when Nautilus participated in the quarantine of Cuba during the Cuban Missile Crisis. In August 1963, Nautilus headed east again for a two month Mediterranean tour before returning to Portsmouth for an extensive overhaul. The overhaul took 27 months to complete. The submarine returned to homeport on 2 May 1966. ~Over the next six years, Nautilus participated in several fleet exercises while steaming more than 200,000 miles. In the spring of 1966, she again entered the record books when she logged her 300,000th mile underway. During the following 12 years, Nautilus was involved in a variety of developmental testing programs while continuing to serve alongside many of the more modern nuclear powered submarines she had preceded. On 9 April 1979,~Nautilus~departed Groton, on her final underway, steaming south to the Panama Canal via Guantanamo Bay and Cartagena, Columbia. From there, she cruised north and reached Mare Island Naval Shipyard, Vallejo, California, on 26 May, to begin inactivation procedures.~The ground breaking submarine~decommissioned on 3 March 1980. In recognition of her pioneering role in the practical use of nuclear power,~Nautilus~was designated a National Historic Landmark by the Secretary of the Interior on 20 May 1982. Following an extensive historic ship conversion at Mare Island, the submarine was towed to Groton, arriving on 6 July 1985. There, on 11 April 1986, 86 years to the day after the establishment of the U.S. Submarine Force, historic ship~Nautilus~and the Submarine Force Museum opened to the public as the first exhibit of its kind in the world. The unique museum ship continues to serve as a dramatic link in both Cold War-era history and the birth of the nuclear age. In October 2021, Nautilus is scheduled to receive \$36 million in upgrades to include: full blast and paint of all exterior; repairs to her superstructure; full topside decking repairs; all internal/external tanks inspected, repaired, and preserved; lighting and electrical distribution upgrades; and enhanced access to certain areas for staff members. The objective of the work is to give Nautilus 30 years of availability to the public to continue to tell her stories of the bold and courageous Sailors of U.S. submarine force. The work is scheduled to be complete in the summer of 2022. ***** Suggested Reading The Nuclear Navy Submarine Force Polar Exploration A Brief History of U.S. Navy Fleet Ballistic Missiles and Submarines The U.S. Navy in the Cold War Era,~1945–1991 Conflict and Cooperation: The U.S. and Soviet Navies in the Cold War Nuclear Navy and USS Nautilus Celebrate 60th Anniversary USS Nautilus (SSN-571) Deck Log Book—July 1958 USS Nautilus (SSN-571) Deck Log Book—August 1958 Art Exhibit A View from the Periscope Interviews with USS Nautilus (SSN-571) crewmembers Albert O. Howard Jimmy Hayes Infographic},
  langid = {american},
  file = {C:\Users\chsey\Zotero\storage\NUZ5NQ3H\uss-nautilus.html}
}

@article{navonEquivariantDeepWeight,
  title = {Equivariant {{Deep Weight Space Alignment}}},
  author = {Navon, Aviv and Shamsian, Aviv and Fetaya, Ethan and Chechik, Gal and Dym, Nadav and Maron, Haggai},
  abstract = {Permutation symmetries of deep networks make basic operations like model merging and similarity estimation challenging. In many cases, aligning the weights of the networks, i.e., finding optimal permutations between their weights, is necessary. Unfortunately, weight alignment is an NPhard problem. Prior research has mainly focused on solving relaxed versions of the alignment problem, leading to either time-consuming methods or sub-optimal solutions. To accelerate the alignment process and improve its quality, we propose a novel framework aimed at learning to solve the weight alignment problem, which we name DEEPALIGN. To that end, we first prove that weight alignment adheres to two fundamental symmetries and then, propose a deep architecture that respects these symmetries. Notably, our framework does not require any labeled data. We provide a theoretical analysis of our approach and evaluate DEEP-ALIGN on several types of network architectures and learning setups. Our experimental results indicate that a feed-forward pass with DEEP-ALIGN produces better or equivalent alignments compared to those produced by current optimization algorithms. Additionally, our alignments can be used as an effective initialization for other methods, leading to improved solutions with a significant speedup in convergence.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\W23HQ5GA\Navon 등 - Equivariant Deep Weight Space Alignment.pdf}
}

@article{neffDONeRFRealTimeRendering2021,
  title = {{{DONeRF}}: {{Towards Real-Time Rendering}} of {{Compact Neural Radiance Fields}} Using {{Depth Oracle Networks}}},
  shorttitle = {{{DONeRF}}},
  author = {Neff, Thomas and Stadlbauer, Pascal and Parger, Mathias and Kurz, Andreas and Mueller, Joerg H. and Chaitanya, Chakravarty R. Alla and Kaplanyan, Anton and Steinberger, Markus},
  date = {2021-07},
  journaltitle = {Computer Graphics Forum},
  shortjournal = {Computer Graphics Forum},
  volume = {40},
  number = {4},
  eprint = {2103.03231},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {45--59},
  issn = {0167-7055, 1467-8659},
  doi = {10.1111/cgf.14340},
  url = {http://arxiv.org/abs/2103.03231},
  urldate = {2023-01-25},
  abstract = {The recent research explosion around implicit neural representations, such as NeRF, shows that there is immense potential for implicitly storing high-quality scene and lighting information in compact neural networks. However, one major limitation preventing the use of NeRF in real-time rendering applications is the prohibitive computational cost of excessive network evaluations along each view ray, requiring dozens of petaFLOPS. In this work, we bring compact neural representations closer to practical rendering of synthetic content in real-time applications, such as games and virtual reality. We show that the number of samples required for each view ray can be significantly reduced when samples are placed around surfaces in the scene without compromising image quality. To this end, we propose a depth oracle network that predicts ray sample locations for each view ray with a single network evaluation. We show that using a classification network around logarithmically discretized and spherically warped depth values is essential to encode surface locations rather than directly estimating depth. The combination of these techniques leads to DONeRF, our compact dual network design with a depth oracle network as its first step and a locally sampled shading network for ray accumulation. With DONeRF, we reduce the inference costs by up to 48x compared to NeRF when conditioning on available ground truth depth information. Compared to concurrent acceleration methods for raymarching-based neural representations, DONeRF does not require additional memory for explicit caching or acceleration structures, and can render interactively (20 frames per second) on a single GPU.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Neff et al_2021_DONeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\E9VB2G4X\\2103.html}
}

@online{NeuralOrdinaryDifferential,
  title = {Neural {{Ordinary Differential Equations}}},
  url = {https://papers.nips.cc/paper_files/paper/2018/hash/69386f6bb1dfed68692a24c8686939b9-Abstract.html},
  urldate = {2023-05-30}
}

@online{NewsEpson,
  title = {News | {{Epson}}},
  url = {https://corporate.epson/en/news/},
  urldate = {2023-12-26},
  abstract = {2023 News Release},
  langid = {english},
  file = {Y:\paper\management\News Epson.pdf}
}

@online{neyshaburPACBayesianApproachSpectrallyNormalized2018,
  title = {A {{PAC-Bayesian Approach}} to {{Spectrally-Normalized Margin Bounds}} for {{Neural Networks}}},
  author = {Neyshabur, Behnam and Bhojanapalli, Srinadh and Srebro, Nathan},
  date = {2018-02-23},
  eprint = {1707.09564},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1707.09564},
  url = {http://arxiv.org/abs/1707.09564},
  urldate = {2024-04-14},
  abstract = {We present a generalization bound for feedforward neural networks in terms of the product of the spectral norm of the layers and the Frobenius norm of the weights. The generalization bound is derived using a PAC-Bayes analysis.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Neyshabur et al_2018_A PAC-Bayesian Approach to Spectrally-Normalized Margin Bounds for Neural.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UZ3I3BH2\\1707.html}
}

@incollection{nguyenGRITFasterBetter2022,
  title = {{{GRIT}}: {{Faster}} and {{Better Image Captioning Transformer Using Dual Visual Features}}},
  shorttitle = {{{GRIT}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2022},
  author = {Nguyen, Van-Quang and Suganuma, Masanori and Okatani, Takayuki},
  editor = {Avidan, Shai and Brostow, Gabriel and Cissé, Moustapha and Farinella, Giovanni Maria and Hassner, Tal},
  date = {2022},
  volume = {13696},
  pages = {167--184},
  publisher = {Springer Nature Switzerland},
  location = {Cham},
  doi = {10.1007/978-3-031-20059-5_10},
  url = {https://link.springer.com/10.1007/978-3-031-20059-5_10},
  urldate = {2023-05-27},
  abstract = {Current state-of-the-art methods for image captioning employ region-based features, as they provide object-level information that is essential to describe the content of images; they are usually extracted by an object detector such as Faster R-CNN. However, they have several issues, such as lack of contextual information, the risk of inaccurate detection, and the high computational cost. The first two could be resolved by additionally using grid-based features. However, how to extract and fuse these two types of features is uncharted. This paper proposes a Transformer-only neural architecture, dubbed GRIT (Grid- and Regionbased Image captioning Transformer), that effectively utilizes the two visual features to generate better captions. GRIT replaces the CNN-based detector employed in previous methods with a DETR-based one, making it computationally faster. Moreover, its monolithic design consisting only of Transformers enables end-to-end training of the model. This innovative design and the integration of the dual visual features bring about significant performance improvement. The experimental results on several image captioning benchmarks show that GRIT outperforms previous methods in inference accuracy and speed.},
  isbn = {978-3-031-20058-8 978-3-031-20059-5},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\7C457856\Nguyen 등 - 2022 - GRIT Faster and Better Image Captioning Transform.pdf}
}

@online{nilsenSourcesRadioactiveContamination2021,
  title = {Sources of {{Radioactive Contamination}} in {{Murmansk}} and {{Arkhangelsk Counties}}},
  author = {Nilsen, Thomas},
  date = {2021-08-11},
  url = {https://bellona.org/publication/sources-of-radioactive-contamination-in-murmansk-and-arkhangelsk-counties},
  urldate = {2023-12-29},
  abstract = {Detailing contamination from Soviet nuclear submarines, atomic bomb tests, radioactive waste dumping practices and even the civilian nuclear industry.},
  langid = {american},
  organization = {Bellona.org},
  file = {Y:\paper\management\Nilsen_2021_Sources of Radioactive Contamination in Murmansk and Arkhangelsk Counties.pdf}
}

@article{nishioAutomaticClassificationCOVID192020,
  title = {Automatic Classification between {{COVID-19}} Pneumonia, Non-{{COVID-19}} Pneumonia, and the Healthy on Chest {{X-ray}} Image: Combination of Data Augmentation Methods},
  shorttitle = {Automatic Classification between {{COVID-19}} Pneumonia, Non-{{COVID-19}} Pneumonia, and the Healthy on Chest {{X-ray}} Image},
  author = {Nishio, Mizuho and Noguchi, Shunjiro and Matsuo, Hidetoshi and Murakami, Takamichi},
  date = {2020-12},
  journaltitle = {Scientific Reports},
  shortjournal = {Sci Rep},
  volume = {10},
  number = {1},
  pages = {17532},
  issn = {2045-2322},
  doi = {10.1038/s41598-020-74539-2},
  url = {https://www.nature.com/articles/s41598-020-74539-2},
  urldate = {2022-08-01},
  abstract = {Abstract             This study aimed to develop and validate computer-aided diagnosis (CXDx) system for classification between COVID-19 pneumonia, non-COVID-19 pneumonia, and the healthy on chest X-ray (CXR) images. From two public datasets, 1248 CXR images were obtained, which included 215, 533, and 500 CXR images of COVID-19 pneumonia patients, non-COVID-19 pneumonia patients, and the healthy samples, respectively. The proposed CADx system utilized VGG16 as a pre-trained model and combination of conventional method and mixup as data augmentation methods. Other types of pre-trained models were compared with the VGG16-based model. Single type or no data augmentation methods were also evaluated. Splitting of training/validation/test sets was used when building and evaluating the CADx system. Three-category accuracy was evaluated for test set with 125 CXR images. The three-category accuracy of the CAD system was 83.6\% between COVID-19 pneumonia, non-COVID-19 pneumonia, and the healthy. Sensitivity for COVID-19 pneumonia was more than 90\%. The combination of conventional method and mixup was more useful than single type or no data augmentation method. In conclusion, this study was able to create an accurate CADx system for the 3-category classification. Source code of our CADx system is available as open source for COVID-19 research.},
  langid = {english},
  file = {Y:\paper\Computer Vision\augmentation\application\Nishio et al_2020_Automatic classification between COVID-19 pneumonia, non-COVID-19 pneumonia,.pdf}
}

@article{nisterEfficientSolutionFivePoint,
  title = {An {{Efﬁcient Solution}} to the {{Five-Point Relative Pose Problem}}},
  author = {Nister, David and Corporation, Sarnoff},
  abstract = {An efficient algorithmic solution to the classical five-point relative pose problem is presented. The problem is to find the possible solutions for relative camera motion between two calibrated views given five corresponding points. The algorithm consists of computing the coefficients of a tenth degree polynomial and subsequently finding its roots. It is the first algorithm well suited for numerical implementation that also corresponds to the inherent complexity of the problem. The algorithm is used in a robust hypothesise-and-test framework to estimate structure and motion in real-time.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\QUQEA8MA\Nister 그리고 Corporation - An Efﬁcient Solution to the Five-Point Relative Po.pdf}
}

@article{nisterEfficientSolutionFivepoint2004,
  title = {An Efficient Solution to the Five-Point Relative Pose Problem},
  author = {Nister, D.},
  date = {2004-06},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  shortjournal = {IEEE Trans. Pattern Anal. Machine Intell.},
  volume = {26},
  number = {6},
  pages = {756--770},
  issn = {0162-8828},
  doi = {10.1109/TPAMI.2004.17},
  url = {http://ieeexplore.ieee.org/document/1288525/},
  urldate = {2022-10-22},
  abstract = {An efficient algorithmic solution to the classical five-point relative pose problem is presented. The problem is to find the possible solutions for relative camera pose between two calibrated views given five corresponding points. The algorithm consists of computing the coefficients of a tenth degree polynomial in closed form and, subsequently, finding its roots. It is the first algorithm wellsuited for numerical implementation that also corresponds to the inherent complexity of the problem. We investigate the numerical precision of the algorithm. We also study its performance under noise in minimal as well as overdetermined cases. The performance is compared to that of the well-known 8 and 7-point methods and a 6-point scheme. The algorithm is used in a robust hypothesize-andtest framework to estimate structure and motion in real-time with low delay. The real-time system uses solely visual input and has been demonstrated at major conferences.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA2\Nister_2004_An efficient solution to the five-point relative pose problem.pdf}
}

@online{normanNuclearSubmarineSize2023,
  title = {Nuclear Submarine | {{Size}}, {{Reactor}}, {{Countries}}, \& {{Accidents}} | {{Britannica}}},
  author = {Norman, Friedemann},
  date = {2023-12-21},
  url = {https://www.britannica.com/technology/nuclear-submarine},
  urldate = {2023-12-28},
  abstract = {Nuclear submarine, submarine that relies on a nuclear reactor to drive its propulsion system. A nuclear submarine may or may not be armed with nuclear weapons. The chief advantages afforded by nuclear power are increased speed (allowing submerged submarines to keep up with fast surface ships) and},
  langid = {english}
}

@article{oelgaardAccidentsNuclearShips1996,
  title = {Accidents in Nuclear Ships},
  author = {Oelgaard, P. L.},
  date = {1996-12-01T05:00:00Z},
  url = {https://www.osti.gov/etdeweb/biblio/445202},
  urldate = {2023-12-29},
  abstract = {This report starts with a discussion of the types of nuclear vessels accidents, in particular accidents which involve the nuclear propulsion systems. Next available information on 61 reported nuclear ship events in considered. Of these 6 deals with U.S. ships, 54 with USSR ships and 1 with a French ship. The ships are in almost all cases nuclear submarines. Only events that involve the sinking of vessels, the nuclear propulsion plants, radiation exposures, fires/explosions, sea-water leaks into the submarines and sinking of vessels are considered. For each event a summary of available information is presented, and comments are added. In some cases the available information is not credible, and these events are neglected. This reduces the number of events to 5 U.S. events, 35 USSR/Russian events and 1 French event. A comparison is made between the reported Soviet accidents and information available on dumped and damaged Soviet naval reactors. It seems possible to obtain good correlation between the two types of events. An analysis is made of the accident and estimates are made of the accident probabilities which are found to be of the order of 10\{sup -3\} per ship reactor years. It if finally pointed out that the consequences of nuclear ship accidents are fairly local and does in no way not approach the magnitude of the Chernobyl accident. It is emphasized that some of the information on which this report is based, may not be correct. Consequently some of the results of the assessments made may not be correct. (au).},
  langid = {english},
  file = {Y:\paper\management\Oelgaard_1996_Accidents in nuclear ships.pdf}
}

@online{ohUnderstandingCrossDomainFewShot2022,
  title = {Understanding {{Cross-Domain Few-Shot Learning}}: {{An Experimental Study}}},
  shorttitle = {Understanding {{Cross-Domain Few-Shot Learning}}},
  author = {Oh, Jaehoon and Kim, Sungnyun and Ho, Namgyu and Kim, Jin-Hwa and Song, Hwanjun and Yun, Se-Young},
  date = {2022-02-08},
  eprint = {2202.01339},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2202.01339},
  urldate = {2022-10-09},
  abstract = {Cross-domain few-shot learning has drawn increasing attention for handling large differences between the source and target domains--an important concern in real-world scenarios. To overcome these large differences, recent works have considered exploiting small-scale unlabeled data from the target domain during the pre-training stage. This data enables self-supervised pre-training on the target domain, in addition to supervised pre-training on the source domain. In this paper, we empirically investigate scenarios under which it is advantageous to use each pre-training scheme, based on domain similarity and few-shot difficulty: performance gain of self-supervised pre-training over supervised pre-training increases when domain similarity is smaller or few-shot difficulty is lower. We further design two pre-training schemes, mixed-supervised and two-stage learning, that improve performance. In this light, we present seven findings for CD-FSL which are supported by extensive experiments and analyses on three source and eight target benchmark datasets with varying levels of domain similarity and few-shot difficulty. Our code is available at https://anonymous.4open.science/r/understandingCDFSL.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\intern\\Oh et al_2022_Understanding Cross-Domain Few-Shot Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Q2GHH683\\2202.html}
}

@article{okawaVarietiesAlternativesCatchingup2018,
  title = {Varieties and {{Alternatives}} of {{Catching-up}}: {{Asian Development}} in the {{Context}} of the 21st {{Century}} Edited by {{Yukihito Sato}} and {{Hajime Sato}}, {{London}}, {{Palgrave Macmillan}}, 2016, Xviii + 314 Pp.},
  author = {Okawa, Yoshifumi},
  date = {2018},
  journaltitle = {The Developing Economies},
  volume = {56},
  number = {1},
  pages = {68--70},
  doi = {10.1111/deve.12161}
}

@article{olahBuildingBlocksInterpretability2018,
  title = {The {{Building Blocks}} of {{Interpretability}}},
  author = {Olah, Chris and Satyanarayan, Arvind and Johnson, Ian and Carter, Shan and Schubert, Ludwig and Ye, Katherine and Mordvintsev, Alexander},
  date = {2018-03-06},
  journaltitle = {Distill},
  shortjournal = {Distill},
  volume = {3},
  number = {3},
  pages = {e10},
  issn = {2476-0757},
  doi = {10.23915/distill.00010},
  url = {https://distill.pub/2018/building-blocks},
  urldate = {2023-08-05},
  abstract = {Interpretability techniques are normally studied in isolation. We explore the powerful interfaces that arise when you combine them -- and the rich structure of this combinatorial space.},
  langid = {english},
  keywords = {notion}
}

@article{olteanuCrisisLexLexiconCollecting2014,
  title = {{{CrisisLex}}: {{A Lexicon}} for {{Collecting}} and {{Filtering Microblogged Communications}} in {{Crises}}},
  shorttitle = {{{CrisisLex}}},
  author = {Olteanu, Alexandra and Castillo, Carlos and Diaz, Fernando and Vieweg, Sarah},
  date = {2014-05-16},
  journaltitle = {Proceedings of the International AAAI Conference on Web and Social Media},
  volume = {8},
  number = {1},
  pages = {376--385},
  issn = {2334-0770},
  doi = {10.1609/icwsm.v8i1.14538},
  url = {https://ojs.aaai.org/index.php/ICWSM/article/view/14538},
  urldate = {2023-05-27},
  abstract = {Locating timely, useful information during crises and mass emergencies is critical for those forced to make potentially life-altering decisions. As the use of Twitter to broadcast useful information during such situations becomes more widespread, the problem of finding it becomes more difficult. We describe an approach toward improving the recall in the sampling of Twitter communications that can lead to greater situational awareness during crisis situations. First, we create a lexicon of crisis-related terms that frequently appear in relevant messages posted during different types of crisis situations. Next, we demonstrate how we use the lexicon to automatically identify new terms that describe a given crisis. Finally, we explain how to efficiently query Twitter to extract crisis-related messages during emergency events. In our experiments, using a crisis lexicon leads to substantial improvements in terms of recall when added to a set of crisis-specific keywords manually chosen by experts; it also helps to preserve the original distribution of message types.},
  issue = {1},
  langid = {english},
  keywords = {Adaptive Information Filtering},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\disaster\NLP\Olteanu et al_2014_CrisisLex.pdf}
}

@inproceedings{olteanuWhatExpectWhen2015,
  title = {What to {{Expect When}} the {{Unexpected Happens}}: {{Social Media Communications Across Crises}}},
  shorttitle = {What to {{Expect When}} the {{Unexpected Happens}}},
  booktitle = {Proceedings of the 18th {{ACM Conference}} on {{Computer Supported Cooperative Work}} \& {{Social Computing}}},
  author = {Olteanu, Alexandra and Vieweg, Sarah and Castillo, Carlos},
  year = {2월 28, 2015},
  series = {{{CSCW}} '15},
  pages = {994--1009},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/2675133.2675242},
  url = {https://doi.org/10.1145/2675133.2675242},
  urldate = {2023-05-26},
  abstract = {The use of social media to communicate timely information during crisis situations has become a common practice in recent years. In particular, the one-to-many nature of Twitter has created an opportunity for stakeholders to disseminate crisis-relevant messages, and to access vast amounts of information they may not otherwise have. Our goal is to understand what affected populations, response agencies and other stakeholders can expect-and not expect-from these data in various types of disaster situations. Anecdotal evidence suggests that different types of crises elicit different reactions from Twitter users, but we have yet to see whether this is in fact the case. In this paper, we investigate several crises-including natural hazards and human-induced disasters-in a systematic manner and with a consistent methodology. This leads to insights about the prevalence of different information types and sources across a variety of crisis situations.},
  isbn = {978-1-4503-2922-4},
  keywords = {emergency management,social media},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\disaster\NLP\Olteanu et al_2015_What to Expect When the Unexpected Happens.pdf}
}

@online{oordNeuralDiscreteRepresentation2018,
  title = {Neural {{Discrete Representation Learning}}},
  author = {family=Oord, given=Aaron, prefix=van den, useprefix=false and Vinyals, Oriol and Kavukcuoglu, Koray},
  date = {2018-05-30},
  eprint = {1711.00937},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1711.00937},
  urldate = {2024-05-09},
  abstract = {Learning useful representations without supervision remains a key challenge in machine learning. In this paper, we propose a simple yet powerful generative model that learns such discrete representations. Our model, the Vector QuantisedVariational AutoEncoder (VQ-VAE), differs from VAEs in two key ways: the encoder network outputs discrete, rather than continuous, codes; and the prior is learnt rather than static. In order to learn a discrete latent representation, we incorporate ideas from vector quantisation (VQ). Using the VQ method allows the model to circumvent issues of “posterior collapse” -— where the latents are ignored when they are paired with a powerful autoregressive decoder -— typically observed in the VAE framework. Pairing these representations with an autoregressive prior, the model can generate high quality images, videos, and speech as well as doing high quality speaker conversion and unsupervised learning of phonemes, providing further evidence of the utility of the learnt representations.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Oord et al_2018_Neural Discrete Representation Learning.pdf}
}

@online{oordRepresentationLearningContrastive2019,
  title = {Representation {{Learning}} with {{Contrastive Predictive Coding}}},
  author = {family=Oord, given=Aaron, prefix=van den, useprefix=false and Li, Yazhe and Vinyals, Oriol},
  date = {2019-01-22},
  eprint = {1807.03748},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1807.03748},
  urldate = {2023-06-27},
  abstract = {While supervised learning has enabled great progress in many applications, unsupervised learning has not seen such widespread adoption, and remains an important and challenging endeavor for artificial intelligence. In this work, we propose a universal unsupervised learning approach to extract useful representations from high-dimensional data, which we call Contrastive Predictive Coding. The key insight of our model is to learn such representations by predicting the future in latent space by using powerful autoregressive models. We use a probabilistic contrastive loss which induces the latent space to capture information that is maximally useful to predict future samples. It also makes the model tractable by using negative sampling. While most prior work has focused on evaluating representations for a particular modality, we demonstrate that our approach is able to learn useful representations achieving strong performance on four distinct domains: speech, images, text and reinforcement learning in 3D environments.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Oord et al_2019_Representation Learning with Contrastive Predictive Coding.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TVRSTB3S\\1807.html}
}

@online{oordRepresentationLearningContrastive2019a,
  title = {Representation {{Learning}} with {{Contrastive Predictive Coding}}},
  author = {family=Oord, given=Aaron, prefix=van den, useprefix=false and Li, Yazhe and Vinyals, Oriol},
  date = {2019-01-22},
  eprint = {1807.03748},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1807.03748},
  url = {http://arxiv.org/abs/1807.03748},
  urldate = {2023-08-05},
  abstract = {While supervised learning has enabled great progress in many applications, unsupervised learning has not seen such widespread adoption, and remains an important and challenging endeavor for artificial intelligence. In this work, we propose a universal unsupervised learning approach to extract useful representations from high-dimensional data, which we call Contrastive Predictive Coding. The key insight of our model is to learn such representations by predicting the future in latent space by using powerful autoregressive models. We use a probabilistic contrastive loss which induces the latent space to capture information that is maximally useful to predict future samples. It also makes the model tractable by using negative sampling. While most prior work has focused on evaluating representations for a particular modality, we demonstrate that our approach is able to learn useful representations achieving strong performance on four distinct domains: speech, images, text and reinforcement learning in 3D environments.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\self supervised learning\\Oord et al_2019_Representation Learning with Contrastive Predictive Coding.pdf;C\:\\Users\\chsey\\Zotero\\storage\\56R22PLW\\1807.html}
}

@online{ortiz-jimenezTaskArithmeticTangent2023,
  title = {Task {{Arithmetic}} in the {{Tangent Space}}: {{Improved Editing}} of {{Pre-Trained Models}}},
  shorttitle = {Task {{Arithmetic}} in the {{Tangent Space}}},
  author = {Ortiz-Jimenez, Guillermo and Favero, Alessandro and Frossard, Pascal},
  date = {2023-11-21},
  eprint = {2305.12827},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.12827},
  urldate = {2024-09-13},
  abstract = {Task arithmetic has recently emerged as a cost-effective and scalable approach to edit pre-trained models directly in weight space: By adding the fine-tuned weights of different tasks, the model’s performance can be improved on these tasks, while negating them leads to task forgetting. Yet, our understanding of the effectiveness of task arithmetic and its underlying principles remains limited. We present a comprehensive study of task arithmetic in vision-language models and show that weight disentanglement is the crucial factor that makes it effective. This property arises during pre-training and manifests when distinct directions in weight space govern separate, localized regions in function space associated with the tasks. Notably, we show that fine-tuning models in their tangent space by linearizing them amplifies weight disentanglement. This leads to substantial performance improvements across multiple task arithmetic benchmarks and diverse models. Building on these findings, we provide theoretical and empirical analyses of the neural tangent kernel (NTK) of these models and establish a compelling link between task arithmetic and the spatial localization of the NTK eigenfunctions. Overall, our work uncovers novel insights into the fundamental mechanisms of task arithmetic and offers a more reliable and effective approach to edit pre-trained models through the NTK linearization.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\Y6YXSJ2M\Ortiz-Jimenez 등 - 2023 - Task Arithmetic in the Tangent Space Improved Edi.pdf}
}

@article{osborneLASSOItsDual2000,
  title = {On the {{LASSO}} and Its {{Dual}}},
  author = {Osborne, Michael R. and Presnell, Brett and Turlach, Berwin A.},
  date = {2000-06-01},
  journaltitle = {Journal of Computational and Graphical Statistics},
  volume = {9},
  number = {2},
  pages = {319--337},
  publisher = {Taylor \& Francis},
  issn = {1061-8600},
  doi = {10.1080/10618600.2000.10474883},
  url = {https://www.tandfonline.com/doi/abs/10.1080/10618600.2000.10474883},
  urldate = {2024-04-11},
  abstract = {Proposed by Tibshirani, the least absolute shrinkage and selection operator (LASSO) estimates a vector of regression coefficients by minimizing the residual sum of squares subject to a constraint on the l 1-norm of the coefficient vector. The LASSO estimator typically has one or more zero elements and thus shares characteristics of both shrinkage estimation and variable selection. In this article we treat the LASSO as a convex programming problem and derive its dual. Consideration of the primal and dual problems together leads to important new insights into the characteristics of the LASSO estimator and to an improved method for estimating its covariance matrix. Using these results we also develop an efficient algorithm for computing LASSO estimates which is usable even in cases where the number of regressors exceeds the number of observations. An S-Plus library based on this algorithm is available from StatLib.},
  keywords = {Convex programming,Dual problem,notion,Partial least squares,Penalized regression,Quadratic programming,Regression,Shrinkage,Subset selection,Variable selection},
  file = {Y:\paper\2024_research\Osborne et al_2000_On the LASSO and its Dual.pdf}
}

@online{ostapenkoModularLLMsBuilding2024,
  title = {Towards {{Modular LLMs}} by {{Building}} and {{Reusing}} a {{Library}} of {{LoRAs}}},
  author = {Ostapenko, Oleksiy and Su, Zhan and Ponti, Edoardo Maria and Charlin, Laurent and Roux, Nicolas Le and Pereira, Matheus and Caccia, Lucas and Sordoni, Alessandro},
  date = {2024-05-17},
  eprint = {2405.11157},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2405.11157},
  urldate = {2024-09-13},
  abstract = {The growing number of parameter-efficient adaptations of a base large language model (LLM) calls for studying whether we can reuse such trained adapters to improve performance for new tasks. We study how to best build a library of adapters given multi-task data and devise techniques for both zero-shot and supervised task generalization through routing in such library. We benchmark existing approaches to build this library and introduce model-based clustering, MBC, a method that groups tasks based on the similarity of their adapter parameters, indirectly optimizing for transfer across the multi-task dataset. To re-use the library, we present a novel zero-shot routing mechanism, Arrow, which enables dynamic selection of the most relevant adapters for new inputs without the need for retraining. We experiment with several LLMs, such as Phi-2 and Mistral, on a wide array of held-out tasks, verifying that MBC-based adapters and Arrow routing lead to superior generalization to new tasks. We make steps towards creating modular, adaptable LLMs that can match or outperform traditional joint training.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\QSJ7H82V\Ostapenko 등 - 2024 - Towards Modular LLMs by Building and Reusing a Lib.pdf}
}

@article{oviedoFastInterpretableClassification2019,
  title = {Fast and Interpretable Classification of Small {{X-ray}} Diffraction Datasets Using Data Augmentation and Deep Neural Networks},
  author = {Oviedo, Felipe and Ren, Zekun and Sun, Shijing and Settens, Charles and Liu, Zhe and Hartono, Noor Titan Putri and Ramasamy, Savitha and DeCost, Brian L. and Tian, Siyu I. P. and Romano, Giuseppe and Gilad Kusne, Aaron and Buonassisi, Tonio},
  date = {2019-05-17},
  journaltitle = {npj Computational Materials},
  shortjournal = {npj Comput Mater},
  volume = {5},
  number = {1},
  pages = {1--9},
  publisher = {Nature Publishing Group},
  issn = {2057-3960},
  doi = {10.1038/s41524-019-0196-x},
  url = {https://www.nature.com/articles/s41524-019-0196-x},
  urldate = {2022-07-09},
  abstract = {X-ray diffraction (XRD) data acquisition and analysis is among the most time-consuming steps in the development cycle of novel thin-film materials. We propose a machine learning-enabled approach to predict crystallographic dimensionality and space group from a limited number of thin-film XRD patterns. We overcome the scarce data problem intrinsic to novel materials development by coupling a supervised machine learning approach with a model-agnostic, physics-informed data augmentation strategy using simulated data from the Inorganic Crystal Structure Database (ICSD) and experimental data. As a test case, 115 thin-film metal-halides spanning three dimensionalities and seven space groups are synthesized and classified. After testing various algorithms, we develop and implement an all convolutional neural network, with cross-validated accuracies for dimensionality and space group classification of 93 and 89\%, respectively. We propose average class activation maps, computed from a global average pooling layer, to allow high model interpretability by human experimentalists, elucidating the root causes of misclassification. Finally, we systematically evaluate the maximum XRD pattern step size (data acquisition rate) before loss of predictive accuracy occurs, and determine it to be 0.16° 2θ, which enables an XRD pattern to be obtained and classified in 5.5\,min or less.},
  issue = {1},
  langid = {english},
  keywords = {Characterization and analytical techniques,Computational methods,Synthesis and processing},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Oviedo et al_2019_Fast and interpretable classification of small X-ray diffraction datasets using.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8WQTNN97\\s41524-019-0196-x.html}
}

@online{oymakRoleAttentionPrompttuning2023,
  title = {On the {{Role}} of {{Attention}} in {{Prompt-tuning}}},
  author = {Oymak, Samet and Rawat, Ankit Singh and Soltanolkotabi, Mahdi and Thrampoulidis, Christos},
  date = {2023-06-06},
  eprint = {2306.03435},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2306.03435},
  url = {http://arxiv.org/abs/2306.03435},
  urldate = {2024-05-20},
  abstract = {Prompt-tuning is an emerging strategy to adapt large language models (LLM) to downstream tasks by learning a (soft-)prompt parameter from data. Despite its success in LLMs, there is limited theoretical understanding of the power of prompt-tuning and the role of the attention mechanism in prompting. In this work, we explore prompt-tuning for one-layer attention architectures and study contextual mixture-models where each input token belongs to a context-relevant or -irrelevant set. We isolate the role of prompt-tuning through a self-contained prompt-attention model. Our contributions are as follows: (1) We show that softmax-prompt-attention is provably more expressive than softmax-self-attention and linear-prompt-attention under our contextual data model. (2) We analyze the initial trajectory of gradient descent and show that it learns the prompt and prediction head with near-optimal sample complexity and demonstrate how prompt can provably attend to sparse context-relevant tokens. (3) Assuming a known prompt but an unknown prediction head, we characterize the exact finite sample performance of prompt-attention which reveals the fundamental performance limits and the precise benefit of the context information. We also provide experiments that verify our theoretical insights on real datasets and demonstrate how prompt-tuning enables the model to attend to context-relevant information.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {C\:\\Users\\chsey\\Zotero\\storage\\5M97NXBM\\Oymak 등 - 2023 - On the Role of Attention in Prompt-tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6KSN2L7M\\2306.html}
}

@online{padmakumarExploringRoleTask2022,
  title = {Exploring the {{Role}} of {{Task Transferability}} in {{Large-Scale Multi-Task Learning}}},
  author = {Padmakumar, Vishakh and Lausen, Leonard and Ballesteros, Miguel and Zha, Sheng and He, He and Karypis, George},
  date = {2022-07-12},
  eprint = {2204.11117},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2204.11117},
  urldate = {2024-01-05},
  abstract = {Recent work has found that multi-task training with a large number of diverse tasks can uniformly improve downstream performance on unseen target tasks. In contrast, literature on task transferability has established that the choice of intermediate tasks can heavily affect downstream task performance. In this work, we aim to disentangle the effect of scale and relatedness of tasks in multi-task representation learning. We find that, on average, increasing the scale of multi-task learning, in terms of the number of tasks, indeed results in better learned representations than smaller multi-task setups. However, if the target tasks are known ahead of time, then training on a smaller set of related tasks is competitive to the large-scale multi-task training at a reduced computational cost.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\Padmakumar et al_2022_Exploring the Role of Task Transferability in Large-Scale Multi-Task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VTN5X7JL\\2204.html}
}

@online{palZeroShotTaskTransfer2019,
  title = {Zero-{{Shot Task Transfer}}},
  author = {Pal, Arghya and Balasubramanian, Vineeth N.},
  date = {2019-03-04},
  eprint = {1903.01092},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1903.01092},
  url = {http://arxiv.org/abs/1903.01092},
  urldate = {2023-11-21},
  abstract = {In this work, we present a novel meta-learning algorithm, i.e. TTNet, that regresses model parameters for novel tasks for which no ground truth is available (zero-shot tasks). In order to adapt to novel zero-shot tasks, our meta-learner learns from the model parameters of known tasks (with ground truth) and the correlation of known tasks to zero-shot tasks. Such intuition finds its foothold in cognitive science, where a subject (human baby) can adapt to a novel-concept (depth understanding) by correlating it with old concepts (hand movement or self-motion), without receiving explicit supervision. We evaluated our model on the Taskonomy dataset, with four tasks as zero-shot: surface-normal, room layout, depth, and camera pose estimation. These tasks were chosen based on the data acquisition complexity and the complexity associated with the learning process using a deep network. Our proposed methodology out-performs state-of-the-art models (which use ground truth)on each of our zero-shot tasks, showing promise on zero-shot task transfer. We also conducted extensive experiments to study the various choices of our methodology, as well as showed how the proposed method can also be used in transfer learning. To the best of our knowledge, this is the firstsuch effort on zero-shot learning in the task space.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Pal_Balasubramanian_2019_Zero-Shot Task Transfer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\56DPBKL6\\1903.html}
}

@online{panActiveNeRFLearningWhere2022,
  title = {{{ActiveNeRF}}: {{Learning}} Where to {{See}} with {{Uncertainty Estimation}}},
  shorttitle = {{{ActiveNeRF}}},
  author = {Pan, Xuran and Lai, Zihang and Song, Shiji and Huang, Gao},
  date = {2022-09-18},
  eprint = {2209.08546},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2209.08546},
  urldate = {2023-01-20},
  abstract = {Recently, Neural Radiance Fields (NeRF) has shown promising performances on reconstructing 3D scenes and synthesizing novel views from a sparse set of 2D images. Albeit effective, the performance of NeRF is highly influenced by the quality of training samples. With limited posed images from the scene, NeRF fails to generalize well to novel views and may collapse to trivial solutions in unobserved regions. This makes NeRF impractical under resource-constrained scenarios. In this paper, we present a novel learning framework, ActiveNeRF, aiming to model a 3D scene with a constrained input budget. Specifically, we first incorporate uncertainty estimation into a NeRF model, which ensures robustness under few observations and provides an interpretation of how NeRF understands the scene. On this basis, we propose to supplement the existing training set with newly captured samples based on an active learning scheme. By evaluating the reduction of uncertainty given new inputs, we select the samples that bring the most information gain. In this way, the quality of novel view synthesis can be improved with minimal additional resources. Extensive experiments validate the performance of our model on both realistic and synthetic scenes, especially with scarcer training data. Code will be released at \textbackslash url\{https://github.com/LeapLabTHU/ActiveNeRF\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Pan et al_2022_ActiveNeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\N36PH6SN\\2209.html}
}

@article{panettaTuftsDentalDatabase2022,
  title = {Tufts {{Dental Database}}: {{A Multimodal Panoramic X-Ray Dataset}} for {{Benchmarking Diagnostic Systems}}},
  shorttitle = {Tufts {{Dental Database}}},
  author = {Panetta, Karen and Rajendran, Rahul and Ramesh, Aruna and Rao, Shishir and Agaian, Sos},
  date = {2022-04},
  journaltitle = {IEEE journal of biomedical and health informatics},
  shortjournal = {IEEE J Biomed Health Inform},
  volume = {26},
  number = {4},
  eprint = {34606466},
  eprinttype = {pmid},
  pages = {1650--1659},
  issn = {2168-2208},
  doi = {10.1109/JBHI.2021.3117575},
  abstract = {The application of Artificial Intelligence in dental healthcare has a very promising role due to the abundance of imagery and non-imagery-based clinical data. Expert analysis of dental radiographs can provide crucial information for clinical diagnosis and treatment. In recent years, Convolutional Neural Networks have achieved the highest accuracy in various benchmarks, including analyzing dental X-ray images to improve clinical care quality. The Tufts Dental Database, a new X-ray panoramic radiography image dataset, has been presented in this paper. This dataset consists of 1000 panoramic dental radiography images with expert labeling of abnormalities and teeth. The classification of radiography images was performed based on five different levels: anatomical location, peripheral characteristics, radiodensity, effects on the surrounding structure, and the abnormality category. This first-of-its-kind multimodal dataset also includes the radiologist's expertise captured in the form of eye-tracking and think-aloud protocol. The contributions of this work are 1) publicly available dataset that can help researchers to incorporate human expertise into AI and achieve more robust and accurate abnormality detection; 2) a benchmark performance analysis for various state-of-the-art systems for dental radiograph image enhancement and image segmentation using deep learning; 3) an in-depth review of various panoramic dental image datasets, along with segmentation and detection systems. The release of this dataset aims to propel the development of AI-powered automated abnormality detection and classification in dental panoramic radiographs, enhance tooth segmentation algorithms, and the ability to distill the radiologist's expertise into AI.},
  langid = {english},
  keywords = {Artificial Intelligence,Benchmarking,Humans,Radiography Panoramic,Tooth,X-Rays},
  file = {Y:\paper\2022 summer intern\assignment\data augmentation\dataset\Panetta et al_2022_Tufts Dental Database.pdf}
}

@inproceedings{panSamplingNeuralRadiance2022,
  title = {Sampling {{Neural Radiance Fields}} for {{Refractive Objects}}},
  booktitle = {{{SIGGRAPH Asia}} 2022 {{Technical Communications}}},
  author = {Pan, Jen-I. and Su, Jheng-Wei and Hsiao, Kai-Wen and Yen, Ting-Yu and Chu, Hung-Kuo},
  date = {2022-12-06},
  eprint = {2211.14799},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--4},
  doi = {10.1145/3550340.3564234},
  url = {http://arxiv.org/abs/2211.14799},
  urldate = {2023-01-30},
  abstract = {Recently, differentiable volume rendering in neural radiance fields (NeRF) has gained a lot of popularity, and its variants have attained many impressive results. However, existing methods usually assume the scene is a homogeneous volume so that a ray is cast along the straight path. In this work, the scene is instead a heterogeneous volume with a piecewise-constant refractive index, where the path will be curved if it intersects the different refractive indices. For novel view synthesis of refractive objects, our NeRF-based framework aims to optimize the radiance fields of bounded volume and boundary from multi-view posed images with refractive object silhouettes. To tackle this challenging problem, the refractive index of a scene is reconstructed from silhouettes. Given the refractive index, we extend the stratified and hierarchical sampling techniques in NeRF to allow drawing samples along a curved path tracked by the Eikonal equation. The results indicate that our framework outperforms the state-of-the-art method both quantitatively and qualitatively, demonstrating better performance on the perceptual similarity metric and an apparent improvement in the rendering quality on several synthetic and real scenes.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Pan et al_2022_Sampling Neural Radiance Fields for Refractive Objects3.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TSPEHHYR\\2211.html}
}

@inproceedings{panSamplingNeuralRadiance2022a,
  title = {Sampling {{Neural Radiance Fields}} for {{Refractive Objects}}},
  booktitle = {{{SIGGRAPH Asia}} 2022 {{Technical Communications}}},
  author = {Pan, Jen-I. and Su, Jheng-Wei and Hsiao, Kai-Wen and Yen, Ting-Yu and Chu, Hung-Kuo},
  date = {2022-12-06},
  eprint = {2211.14799},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--4},
  doi = {10.1145/3550340.3564234},
  url = {http://arxiv.org/abs/2211.14799},
  urldate = {2023-01-27},
  abstract = {Recently, differentiable volume rendering in neural radiance fields (NeRF) has gained a lot of popularity, and its variants have attained many impressive results. However, existing methods usually assume the scene is a homogeneous volume so that a ray is cast along the straight path. In this work, the scene is instead a heterogeneous volume with a piecewise-constant refractive index, where the path will be curved if it intersects the different refractive indices. For novel view synthesis of refractive objects, our NeRF-based framework aims to optimize the radiance fields of bounded volume and boundary from multi-view posed images with refractive object silhouettes. To tackle this challenging problem, the refractive index of a scene is reconstructed from silhouettes. Given the refractive index, we extend the stratified and hierarchical sampling techniques in NeRF to allow drawing samples along a curved path tracked by the Eikonal equation. The results indicate that our framework outperforms the state-of-the-art method both quantitatively and qualitatively, demonstrating better performance on the perceptual similarity metric and an apparent improvement in the rendering quality on several synthetic and real scenes.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Pan et al_2022_Sampling Neural Radiance Fields for Refractive Objects2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\B8A26K6G\\2211.html}
}

@inproceedings{panSamplingNeuralRadiance2022b,
  title = {Sampling {{Neural Radiance Fields}} for {{Refractive Objects}}},
  booktitle = {{{SIGGRAPH Asia}} 2022 {{Technical Communications}}},
  author = {Pan, Jen-I. and Su, Jheng-Wei and Hsiao, Kai-Wen and Yen, Ting-Yu and Chu, Hung-Kuo},
  date = {2022-12-06},
  eprint = {2211.14799},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--4},
  doi = {10.1145/3550340.3564234},
  url = {http://arxiv.org/abs/2211.14799},
  urldate = {2023-01-26},
  abstract = {Recently, differentiable volume rendering in neural radiance fields (NeRF) has gained a lot of popularity, and its variants have attained many impressive results. However, existing methods usually assume the scene is a homogeneous volume so that a ray is cast along the straight path. In this work, the scene is instead a heterogeneous volume with a piecewise-constant refractive index, where the path will be curved if it intersects the different refractive indices. For novel view synthesis of refractive objects, our NeRF-based framework aims to optimize the radiance fields of bounded volume and boundary from multi-view posed images with refractive object silhouettes. To tackle this challenging problem, the refractive index of a scene is reconstructed from silhouettes. Given the refractive index, we extend the stratified and hierarchical sampling techniques in NeRF to allow drawing samples along a curved path tracked by the Eikonal equation. The results indicate that our framework outperforms the state-of-the-art method both quantitatively and qualitatively, demonstrating better performance on the perceptual similarity metric and an apparent improvement in the rendering quality on several synthetic and real scenes.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Pan et al_2022_Sampling Neural Radiance Fields for Refractive Objects.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y8TI7B8V\\2211.html}
}

@online{panUnderstandingWhyAdam2023,
  title = {Toward {{Understanding Why Adam Converges Faster Than SGD}} for {{Transformers}}},
  author = {Pan, Yan and Li, Yuanzhi},
  date = {2023-05-31},
  eprint = {2306.00204},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2306.00204},
  url = {http://arxiv.org/abs/2306.00204},
  urldate = {2024-06-01},
  abstract = {While stochastic gradient descent (SGD) is still the most popular optimization algorithm in deep learning, adaptive algorithms such as Adam have established empirical advantages over SGD in some deep learning applications such as training transformers. However, it remains a question that why Adam converges significantly faster than SGD in these scenarios. In this paper, we propose one explanation of why Adam converges faster than SGD using a new concept directional sharpness. We argue that the performance of optimization algorithms is closely related to the directional sharpness of the update steps, and show SGD has much worse directional sharpness compared to adaptive algorithms. We further observe that only a small fraction of the coordinates causes the bad sharpness and slow convergence of SGD, and propose to use coordinate-wise clipping as a solution to SGD and other optimization algorithms. We demonstrate the effect of coordinate-wise clipping on sharpness reduction and speeding up the convergence of optimization algorithms under various settings. We show that coordinate-wise clipping improves the local loss reduction when only a small fraction of the coordinates has bad sharpness. We conclude that the sharpness reduction effect of adaptive coordinate-wise scaling is the reason for Adam's success in practice and suggest the use of coordinate-wise clipping as a universal technique to speed up deep learning optimization.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_lecture\\Pan_Li_2023_Toward Understanding Why Adam Converges Faster Than SGD for Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9YFWGHW9\\2306.html}
}

@online{PapersCodeSimple,
  title = {Papers with {{Code}} - {{Simple Copy-Paste}} Is a {{Strong Data Augmentation Method}} for {{Instance Segmentation}}},
  url = {https://paperswithcode.com/paper/simple-copy-paste-is-a-strong-data},
  urldate = {2022-07-09},
  abstract = {🏆 SOTA for Instance Segmentation on LVIS v1.0 val (mask AP metric)},
  langid = {english}
}

@article{parkDeepLearningBased2022,
  title = {Deep {{Learning Based Detection}} of {{Missing Tooth Regions}} for {{Dental Implant Planning}} in {{Panoramic Radiographic Images}}},
  author = {Park, Jumi and Lee, Junseok and Moon, Seongyong and Lee, Kyoobin},
  date = {2022-01},
  journaltitle = {Applied Sciences},
  volume = {12},
  number = {3},
  pages = {1595},
  publisher = {Multidisciplinary Digital Publishing Institute},
  issn = {2076-3417},
  doi = {10.3390/app12031595},
  url = {https://www.mdpi.com/2076-3417/12/3/1595},
  urldate = {2022-06-27},
  abstract = {Dental implantation is a surgical procedure in oral and maxillofacial surgery. Detecting missing tooth regions is essential for planning dental implant placement. This study proposes an automated method that detects regions of missing teeth in panoramic radiographic images. Tooth instance segmentation is required to accurately detect a missing tooth region in panoramic radiographic images containing obstacles, such as dental appliances or restoration. Therefore, we constructed a dataset that contains 455 panoramic radiographic images and annotations for tooth instance segmentation and missing tooth region detection. First, the segmentation model segments teeth into the panoramic radiographic image and generates teeth masks. Second, a detection model uses the teeth masks as input to predict regions of missing teeth. Finally, the detection model identifies the position and number of missing teeth in the panoramic radiographic image. We achieved 92.14\% mean Average Precision (mAP) for tooth instance segmentation and 59.09\% mAP for missing tooth regions detection. As a result, this method assists diagnosis by clinicians to detect missing teeth regions for implant placement.},
  issue = {3},
  langid = {english},
  keywords = {dental implant,dental implant placement,missing tooth regions detection,panoramic radiographic image,tooth instance segmentation},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\reproduction\\Park et al_2022_Deep Learning Based Detection of Missing Tooth Regions for Dental Implant.pdf;C\:\\Users\\chsey\\Zotero\\storage\\P9LTJ6UT\\1595.html}
}

@online{parkRepresentationReliabilityIts2023,
  title = {Representation {{Reliability}} and {{Its Impact}} on {{Downstream Tasks}}},
  author = {Park, Young-Jin and Wang, Hao and Ardeshir, Shervin and Azizan, Navid},
  date = {2023-05-31},
  eprint = {2306.00206},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2306.00206},
  url = {http://arxiv.org/abs/2306.00206},
  urldate = {2024-03-21},
  abstract = {Self-supervised pre-trained models extract general-purpose representations from data, and quantifying how reliable they are is crucial because many downstream models use these representations as input for their own tasks. To this end, we first introduce a formal definition of representation reliability: the representation for a given test input is considered to be reliable if the downstream models built on top of that representation can consistently generate accurate predictions for that test point. It is desired to estimate the representation reliability without knowing the downstream tasks a priori. We provide a negative result showing that existing frameworks for uncertainty quantification in supervised learning are not suitable for this purpose. As an alternative, we propose an ensemble-based method for quantifying representation reliability, based on the concept of neighborhood consistency in the representation spaces across various pre-trained models. More specifically, the key insight is to use shared neighboring points as anchors to align different representation spaces. We demonstrate through comprehensive numerical experiments that our method is capable of predicting representation reliability with high accuracy.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Park et al_2023_Representation Reliability and Its Impact on Downstream Tasks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3X4NX5XW\\2306.html}
}

@online{paszkePyTorchImperativeStyle2019,
  title = {{{PyTorch}}: {{An Imperative Style}}, {{High-Performance Deep Learning Library}}},
  shorttitle = {{{PyTorch}}},
  author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Köpf, Andreas and Yang, Edward and DeVito, Zach and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
  date = {2019-12-03},
  eprint = {1912.01703},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.1912.01703},
  url = {http://arxiv.org/abs/1912.01703},
  urldate = {2024-11-07},
  abstract = {Deep learning frameworks have often focused on either usability or speed, but not both. PyTorch is a machine learning library that shows that these two goals are in fact compatible: it provides an imperative and Pythonic programming style that supports code as a model, makes debugging easy and is consistent with other popular scientific computing libraries, while remaining efficient and supporting hardware accelerators such as GPUs. In this paper, we detail the principles that drove the implementation of PyTorch and how they are reflected in its architecture. We emphasize that every aspect of PyTorch is a regular Python program under the full control of its user. We also explain how the careful and pragmatic implementation of the key components of its runtime enables them to work together to achieve compelling performance. We demonstrate the efficiency of individual subsystems, as well as the overall speed of PyTorch on several common benchmarks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Computer Science - Mathematical Software,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Paszke et al_2019_PyTorch.pdf;C\:\\Users\\chsey\\Zotero\\storage\\FTNSEVMF\\1912.html}
}

@online{pathakFourCastNetGlobalDatadriven2022,
  title = {{{FourCastNet}}: {{A Global Data-driven High-resolution Weather Model}} Using {{Adaptive Fourier Neural Operators}}},
  shorttitle = {{{FourCastNet}}},
  author = {Pathak, Jaideep and Subramanian, Shashank and Harrington, Peter and Raja, Sanjeev and Chattopadhyay, Ashesh and Mardani, Morteza and Kurth, Thorsten and Hall, David and Li, Zongyi and Azizzadenesheli, Kamyar and Hassanzadeh, Pedram and Kashinath, Karthik and Anandkumar, Animashree},
  date = {2022-02-22},
  eprint = {2202.11214},
  eprinttype = {arXiv},
  eprintclass = {physics},
  url = {http://arxiv.org/abs/2202.11214},
  urldate = {2022-08-09},
  abstract = {FourCastNet, short for Fourier Forecasting Neural Network, is a global data-driven weather forecasting model that provides accurate short to medium-range global predictions at \$0.25\textasciicircum\{\textbackslash circ\}\$ resolution. FourCastNet accurately forecasts high-resolution, fast-timescale variables such as the surface wind speed, precipitation, and atmospheric water vapor. It has important implications for planning wind energy resources, predicting extreme weather events such as tropical cyclones, extra-tropical cyclones, and atmospheric rivers. FourCastNet matches the forecasting accuracy of the ECMWF Integrated Forecasting System (IFS), a state-of-the-art Numerical Weather Prediction (NWP) model, at short lead times for large-scale variables, while outperforming IFS for variables with complex fine-scale structure, including precipitation. FourCastNet generates a week-long forecast in less than 2 seconds, orders of magnitude faster than IFS. The speed of FourCastNet enables the creation of rapid and inexpensive large-ensemble forecasts with thousands of ensemble-members for improving probabilistic forecasting. We discuss how data-driven deep learning models such as FourCastNet are a valuable addition to the meteorology toolkit to aid and augment NWP models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Physics - Atmospheric and Oceanic Physics},
  file = {Y\:\\paper\\artificial intelligence\\Pathak et al_2022_FourCastNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SV8DQXHE\\2202.html}
}

@article{peiGroupSparseBayesian2018,
  title = {Group {{Sparse Bayesian Learning}} for {{Active Surveillance}} on {{Epidemic Dynamics}}},
  author = {Pei, Hongbin and Yang, Bo and Liu, Jiming and Dong, Lei},
  date = {2018-04-25},
  journaltitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
  volume = {32},
  number = {1},
  issn = {2374-3468},
  doi = {10.1609/aaai.v32i1.11344},
  url = {https://ojs.aaai.org/index.php/AAAI/article/view/11344},
  urldate = {2023-05-24},
  abstract = {Predicting epidemic dynamics is of great value in understanding and controlling diffusion processes, such as infectious disease spread and information propagation. This task is intractable, especially when surveillance resources are very limited. To address the challenge, we study the problem of active surveillance, i.e., how to identify a small portion of system components as sentinels to effect monitoring, such that the epidemic dynamics of an entire system can be readily predicted from the partial data collected by such sentinels. We propose a novel measure, the gamma value, to identify the sentinels by modeling a sentinel network with row sparsity structure. We design a flexible group sparse Bayesian learning algorithm to mine the sentinel network suitable for handling both linear and non-linear dynamical systems by using the expectation maximization method and variational approximation. The efficacy of the proposed algorithm is theoretically analyzed and empirically validated using both synthetic and real-world data.},
  issue = {1},
  langid = {english},
  keywords = {Diffusion},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Pei et al_2018_Group Sparse Bayesian Learning for Active Surveillance on Epidemic Dynamics.pdf}
}

@online{pengBEiTV2Masked2022,
  title = {{{BEiT}} v2: {{Masked Image Modeling}} with {{Vector-Quantized Visual Tokenizers}}},
  shorttitle = {{{BEiT}} V2},
  author = {Peng, Zhiliang and Dong, Li and Bao, Hangbo and Ye, Qixiang and Wei, Furu},
  date = {2022-10-03},
  eprint = {2208.06366},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2208.06366},
  url = {http://arxiv.org/abs/2208.06366},
  urldate = {2024-02-08},
  abstract = {Masked image modeling (MIM) has demonstrated impressive results in self-supervised representation learning by recovering corrupted image patches. However, most existing studies operate on low-level image pixels, which hinders the exploitation of high-level semantics for representation models. In this work, we propose to use a semantic-rich visual tokenizer as the reconstruction target for masked prediction, providing a systematic way to promote MIM from pixel-level to semantic-level. Specifically, we propose vector-quantized knowledge distillation to train the tokenizer, which discretizes a continuous semantic space to compact codes. We then pretrain vision Transformers by predicting the original visual tokens for the masked image patches. Furthermore, we introduce a patch aggregation strategy which associates discrete image patches to enhance global semantic representation. Experiments on image classification and semantic segmentation show that BEiT v2 outperforms all compared MIM methods. On ImageNet-1K (224 size), the base-size BEiT v2 achieves 85.5\% top-1 accuracy for fine-tuning and 80.1\% top-1 accuracy for linear probing. The large-size BEiT v2 obtains 87.3\% top-1 accuracy for ImageNet-1K (224 size) fine-tuning, and 56.7\% mIoU on ADE20K for semantic segmentation. The code and pretrained models are available at https://aka.ms/beitv2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Peng et al_2022_BEiT v2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CGZ4WM7I\\2208.html}
}

@online{pengBEiTV2Masked2022a,
  title = {{{BEiT}} v2: {{Masked Image Modeling}} with {{Vector-Quantized Visual Tokenizers}}},
  shorttitle = {{{BEiT}} V2},
  author = {Peng, Zhiliang and Dong, Li and Bao, Hangbo and Ye, Qixiang and Wei, Furu},
  date = {2022-10-03},
  eprint = {2208.06366},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2208.06366},
  url = {http://arxiv.org/abs/2208.06366},
  urldate = {2023-09-18},
  abstract = {Masked image modeling (MIM) has demonstrated impressive results in self-supervised representation learning by recovering corrupted image patches. However, most existing studies operate on low-level image pixels, which hinders the exploitation of high-level semantics for representation models. In this work, we propose to use a semantic-rich visual tokenizer as the reconstruction target for masked prediction, providing a systematic way to promote MIM from pixel-level to semantic-level. Specifically, we propose vector-quantized knowledge distillation to train the tokenizer, which discretizes a continuous semantic space to compact codes. We then pretrain vision Transformers by predicting the original visual tokens for the masked image patches. Furthermore, we introduce a patch aggregation strategy which associates discrete image patches to enhance global semantic representation. Experiments on image classification and semantic segmentation show that BEiT v2 outperforms all compared MIM methods. On ImageNet-1K (224 size), the base-size BEiT v2 achieves 85.5\% top-1 accuracy for fine-tuning and 80.1\% top-1 accuracy for linear probing. The large-size BEiT v2 obtains 87.3\% top-1 accuracy for ImageNet-1K (224 size) fine-tuning, and 56.7\% mIoU on ADE20K for semantic segmentation. The code and pretrained models are available at https://aka.ms/beitv2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Peng et al_2022_BEiT v2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\IZHKZ6CC\\2208.html}
}

@online{pengKosmos2GroundingMultimodal2023,
  title = {Kosmos-2: {{Grounding Multimodal Large Language Models}} to the {{World}}},
  shorttitle = {Kosmos-2},
  author = {Peng, Zhiliang and Wang, Wenhui and Dong, Li and Hao, Yaru and Huang, Shaohan and Ma, Shuming and Wei, Furu},
  date = {2023-07-13},
  eprint = {2306.14824},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2306.14824},
  urldate = {2024-01-30},
  abstract = {We introduce Kosmos-2, a Multimodal Large Language Model (MLLM), enabling new capabilities of perceiving object descriptions (e.g., bounding boxes) and grounding text to the visual world. Specifically, we represent refer expressions as links in Markdown, i.e., ``[text span](bounding boxes)'', where object descriptions are sequences of location tokens. Together with multimodal corpora, we construct large-scale data of grounded image-text pairs (called GrIT) to train the model. In addition to the existing capabilities of MLLMs (e.g., perceiving general modalities, following instructions, and performing in-context learning), Kosmos-2 integrates the grounding capability into downstream applications. We evaluate Kosmos-2 on a wide range of tasks, including (i) multimodal grounding, such as referring expression comprehension, and phrase grounding, (ii) multimodal referring, such as referring expression generation, (iii) perception-language tasks, and (iv) language understanding and generation. This work lays out the foundation for the development of Embodiment AI and sheds light on the big convergence of language, multimodal perception, action, and world modeling, which is a key step toward artificial general intelligence. Code and pretrained models are available at https://aka.ms/kosmos-2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Peng et al_2023_Kosmos-2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V97QGTR8\\2306.html}
}

@online{pereraImageMemorabilityPrediction2019,
  title = {Is {{Image Memorability Prediction Solved}}?},
  author = {Perera, Shay and Tal, Ayellet and Zelnik-Manor, Lihi},
  date = {2019-01-31},
  eprint = {1901.11420},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1901.11420},
  url = {http://arxiv.org/abs/1901.11420},
  urldate = {2023-08-05},
  abstract = {This paper deals with the prediction of the memorability of a given image. We start by proposing an algorithm that reaches human-level performance on the LaMem dataset - the only large scale benchmark for memorability prediction. The suggested algorithm is based on three observations we make regarding convolutional neural networks (CNNs) that affect memorability prediction. Having reached human-level performance we were humbled, and asked ourselves whether indeed we have resolved memorability prediction - and answered this question in the negative. We studied a few factors and made some recommendations that should be taken into account when designing the next benchmark.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\memorability and intention interface\\Perera et al_2019_Is Image Memorability Prediction Solved.pdf;C\:\\Users\\chsey\\Zotero\\storage\\35E769T8\\1901.html}
}

@online{perezFiLMVisualReasoning2017,
  title = {{{FiLM}}: {{Visual Reasoning}} with a {{General Conditioning Layer}}},
  shorttitle = {{{FiLM}}},
  author = {Perez, Ethan and Strub, Florian and family=Vries, given=Harm, prefix=de, useprefix=true and Dumoulin, Vincent and Courville, Aaron},
  date = {2017-12-18},
  eprint = {1709.07871},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1709.07871},
  url = {http://arxiv.org/abs/1709.07871},
  urldate = {2023-12-22},
  abstract = {We introduce a general-purpose conditioning method for neural networks called FiLM: Feature-wise Linear Modulation. FiLM layers influence neural network computation via a simple, feature-wise affine transformation based on conditioning information. We show that FiLM layers are highly effective for visual reasoning - answering image-related questions which require a multi-step, high-level process - a task which has proven difficult for standard deep learning methods that do not explicitly model reasoning. Specifically, we show on visual reasoning tasks that FiLM layers 1) halve state-of-the-art error for the CLEVR benchmark, 2) modulate features in a coherent manner, 3) are robust to ablations and architectural modifications, and 4) generalize well to challenging, new data from few examples or even zero-shot.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\Perez et al_2017_FiLM.pdf;C\:\\Users\\chsey\\Zotero\\storage\\U4YV8HM5\\1709.html}
}

@online{perezFiLMVisualReasoning2017a,
  title = {{{FiLM}}: {{Visual Reasoning}} with a {{General Conditioning Layer}}},
  shorttitle = {{{FiLM}}},
  author = {Perez, Ethan and Strub, Florian and family=Vries, given=Harm, prefix=de, useprefix=true and Dumoulin, Vincent and Courville, Aaron},
  date = {2017-12-18},
  eprint = {1709.07871},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1709.07871},
  url = {http://arxiv.org/abs/1709.07871},
  urldate = {2024-04-14},
  abstract = {We introduce a general-purpose conditioning method for neural networks called FiLM: Feature-wise Linear Modulation. FiLM layers influence neural network computation via a simple, feature-wise affine transformation based on conditioning information. We show that FiLM layers are highly effective for visual reasoning - answering image-related questions which require a multi-step, high-level process - a task which has proven difficult for standard deep learning methods that do not explicitly model reasoning. Specifically, we show on visual reasoning tasks that FiLM layers 1) halve state-of-the-art error for the CLEVR benchmark, 2) modulate features in a coherent manner, 3) are robust to ablations and architectural modifications, and 4) generalize well to challenging, new data from few examples or even zero-shot.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Perez et al_2017_FiLM.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CKYXHHZI\\1709.html}
}

@article{petersenHttpMatrixcookbookCom,
  title = {[ {{http://matrixcookbook.com}} ]},
  author = {Petersen, Kaare Brandt and Pedersen, Michael Syskind},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\FWP4CD9A\Petersen 그리고 Pedersen - [ httpmatrixcookbook.com ].pdf}
}

@article{pharrPhysicallyBasedRendering,
  title = {Physically {{Based Rendering}}: {{From Theory}} to {{Implementation}}},
  author = {Pharr, Matt},
  langid = {english},
  file = {Y:\paper\textbook\Pharr_Physically Based Rendering.pdf}
}

@book{pharrPhysicallyBasedRendering2017,
  title = {Physically Based Rendering: From Theory to Implementation},
  shorttitle = {Physically Based Rendering},
  author = {Pharr, Matt and Jakob, Wenzel and Humphreys, Greg},
  date = {2017},
  edition = {Third edition},
  publisher = {Morgan Kaufmann Publishers/Elsevier},
  location = {Cambridge, MA},
  isbn = {978-0-12-800645-0},
  langid = {english},
  pagetotal = {1233},
  keywords = {Computer graphics,Digital techniques,Dreidimensionale Computergrafik,Image processing,Realistische Computergrafik,Rendering,Three-dimensional display systems},
  annotation = {OCLC: ocn936532273},
  file = {C:\Users\chsey\Zotero\storage\JW7D2I2F\Pharr 등 - 2017 - Physically based rendering from theory to impleme.pdf}
}

@online{phuongFormalAlgorithmsTransformers2022,
  title = {Formal {{Algorithms}} for {{Transformers}}},
  author = {Phuong, Mary and Hutter, Marcus},
  date = {2022-07-19},
  eprint = {2207.09238},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2207.09238},
  urldate = {2022-07-25},
  abstract = {This document aims to be a self-contained, mathematically precise overview of transformer architectures and algorithms (*not* results). It covers what transformers are, how they are trained, what they are used for, their key architectural components, and a preview of the most prominent models. The reader is assumed to be familiar with basic ML terminology and simpler neural network architectures such as MLPs.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing},
  file = {Y\:\\paper\\Computer Vision\\transformer\\Phuong_Hutter_2022_Formal Algorithms for Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DVYK3GI3\\2207.html}
}

@inproceedings{pontiCombiningParameterefficientModules2023,
  title = {Combining {{Parameter-efficient Modules}} for {{Task-level Generalisation}}},
  booktitle = {Proceedings of the 17th {{Conference}} of the {{European Chapter}} of the {{Association}} for {{Computational Linguistics}}},
  author = {Ponti, Edoardo Maria and Sordoni, Alessandro and Bengio, Yoshua and Reddy, Siva},
  editor = {Vlachos, Andreas and Augenstein, Isabelle},
  date = {2023-05},
  pages = {687--702},
  publisher = {Association for Computational Linguistics},
  location = {Dubrovnik, Croatia},
  doi = {10.18653/v1/2023.eacl-main.49},
  url = {https://aclanthology.org/2023.eacl-main.49},
  urldate = {2024-09-18},
  abstract = {A modular design encourages neural models to disentangle and recombine different facets of knowledge to generalise more systematically to new tasks. In this work, we assume that each task is associated with a subset of latent skills from an (arbitrary size) inventory. In turn, each skill corresponds to a parameter-efficient (sparse / low-rank) model adapter. By jointly learning adapters and a routing function that allocates skills to each task, the full network is instantiated as the average of the parameters of active skills. We propose several inductive biases that encourage re-usage and composition of the skills, including variable-size skill allocation and a dual-speed learning rate. We evaluate our latent-skill model in two main settings: 1) multitask reinforcement learning for instruction following on 8 levels of the BabyAI platform; and 2) few-shot fine-tuning of language models on 160 NLP tasks of the CrossFit benchmark. We find that the modular design of our network enhances sample efficiency in reinforcement learning and few-shot generalisation in supervised learning, compared to a series of baselines. These include models where parameters are fully shared, task-specific, conditionally generated (HyperFormer), or sparse mixture-of-experts (TaskMoE).},
  eventtitle = {{{EACL}} 2023},
  keywords = {notion},
  file = {Y:\paper\2024_research\Ponti et al_2023_Combining Parameter-efficient Modules for Task-level Generalisation.pdf}
}

@online{PrincipalPortfoliosKELLY,
  title = {Principal {{Portfolios}} - {{KELLY}} - 2023 - {{The Journal}} of {{Finance}} - {{Wiley Online Library}}},
  url = {https://onlinelibrary.wiley.com/doi/full/10.1111/jofi.13199},
  urldate = {2024-09-11}
}

@online{purushwalkamTaskDrivenModularNetworks2019,
  title = {Task-{{Driven Modular Networks}} for {{Zero-Shot Compositional Learning}}},
  author = {Purushwalkam, Senthil and Nickel, Maximilian and Gupta, Abhinav and Ranzato, Marc'Aurelio},
  date = {2019-05-14},
  eprint = {1905.05908},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1905.05908},
  url = {http://arxiv.org/abs/1905.05908},
  urldate = {2023-08-05},
  abstract = {One of the hallmarks of human intelligence is the ability to compose learned knowledge into novel concepts which can be recognized without a single training example. In contrast, current state-of-the-art methods require hundreds of training examples for each possible category to build reliable and accurate classifiers. To alleviate this striking difference in efficiency, we propose a task-driven modular architecture for compositional reasoning and sample efficient learning. Our architecture consists of a set of neural network modules, which are small fully connected layers operating in semantic concept space. These modules are configured through a gating function conditioned on the task to produce features representing the compatibility between the input image and the concept under consideration. This enables us to express tasks as a combination of sub-tasks and to generalize to unseen categories by reweighting a set of small modules. Furthermore, the network can be trained efficiently as it is fully differentiable and its modules operate on small sub-spaces. We focus our study on the problem of compositional zero-shot classification of object-attribute categories. We show in our experiments that current evaluation metrics are flawed as they only consider unseen object-attribute pairs. When extending the evaluation to the generalized setting which accounts also for pairs seen during training, we discover that naive baseline methods perform similarly or better than current approaches. However, our modular network is able to outperform all existing approaches on two widely-used benchmark datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\few shot learning\\Purushwalkam et al_2019_Task-Driven Modular Networks for Zero-Shot Compositional Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5VXMUHLG\\1905.html}
}

@online{purushwalkamTaskDrivenModularNetworks2019a,
  title = {Task-{{Driven Modular Networks}} for {{Zero-Shot Compositional Learning}}},
  author = {Purushwalkam, Senthil and Nickel, Maximilian and Gupta, Abhinav and Ranzato, Marc'Aurelio},
  date = {2019-05-14},
  eprint = {1905.05908},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1905.05908},
  url = {http://arxiv.org/abs/1905.05908},
  urldate = {2023-08-05},
  abstract = {One of the hallmarks of human intelligence is the ability to compose learned knowledge into novel concepts which can be recognized without a single training example. In contrast, current state-of-the-art methods require hundreds of training examples for each possible category to build reliable and accurate classifiers. To alleviate this striking difference in efficiency, we propose a task-driven modular architecture for compositional reasoning and sample efficient learning. Our architecture consists of a set of neural network modules, which are small fully connected layers operating in semantic concept space. These modules are configured through a gating function conditioned on the task to produce features representing the compatibility between the input image and the concept under consideration. This enables us to express tasks as a combination of sub-tasks and to generalize to unseen categories by reweighting a set of small modules. Furthermore, the network can be trained efficiently as it is fully differentiable and its modules operate on small sub-spaces. We focus our study on the problem of compositional zero-shot classification of object-attribute categories. We show in our experiments that current evaluation metrics are flawed as they only consider unseen object-attribute pairs. When extending the evaluation to the generalized setting which accounts also for pairs seen during training, we discover that naive baseline methods perform similarly or better than current approaches. However, our modular network is able to outperform all existing approaches on two widely-used benchmark datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\relational reasoning\\Purushwalkam et al_2019_Task-Driven Modular Networks for Zero-Shot Compositional Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\93JV5N34\\1905.html}
}

@inproceedings{qian3DReconstructionTransparent2016,
  title = {{{3D Reconstruction}} of {{Transparent Objects}} with {{Position-Normal Consistency}}},
  booktitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Qian, Yiming and Gong, Minglun and Yang, Yee-Hong},
  date = {2016-06},
  pages = {4369--4377},
  publisher = {IEEE},
  location = {Las Vegas, NV, USA},
  doi = {10.1109/CVPR.2016.473},
  url = {http://ieeexplore.ieee.org/document/7780842/},
  urldate = {2023-01-21},
  abstract = {Estimating the shape of transparent and refractive objects is one of the few open problems in 3D reconstruction. Under the assumption that the rays refract only twice when traveling through the object, we present the first approach to simultaneously reconstructing the 3D positions and normals of the object’s surface at both refraction locations. Our acquisition setup requires only two cameras and one monitor, which serves as the light source. After acquiring the ray-ray correspondences between each camera and the monitor, we solve an optimization function which enforces a new position-normal consistency constraint. That is, the 3D positions of surface points shall agree with the normals required to refract the rays under Snell’s law. Experimental results using both synthetic and real data demonstrate the robustness and accuracy of the proposed approach.},
  eventtitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-4673-8851-1},
  langid = {english},
  file = {Y:\paper\2022 winter intern\Qian et al_2016_3D Reconstruction of Transparent Objects with Position-Normal Consistency.pdf}
}

@inproceedings{qiAttentiveRelationalNetworks2019,
  title = {Attentive {{Relational Networks}} for {{Mapping Images}} to {{Scene Graphs}}},
  booktitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Qi, Mengshi and Li, Weijian and Yang, Zhengyuan and Wang, Yunhong and Luo, Jiebo},
  date = {2019-06},
  pages = {3952--3961},
  publisher = {IEEE},
  location = {Long Beach, CA, USA},
  doi = {10.1109/CVPR.2019.00408},
  url = {https://ieeexplore.ieee.org/document/8954105/},
  urldate = {2023-05-30},
  abstract = {Scene graph generation refers to the task of automatically mapping an image into a semantic structural graph, which requires correctly labeling each extracted object and their interaction relationships. Despite the recent success in object detection using deep learning techniques, inferring complex contextual relationships and structured graph representations from visual data remains a challenging topic. In this study, we propose a novel Attentive Relational Network that consists of two key modules with an object detection backbone to approach this problem. The first module is a semantic transformation module utilized to capture semantic embedded relation features, by translating visual features and linguistic features into a common semantic space. The other module is a graph self-attention module introduced to embed a joint graph representation through assigning various importance weights to neighboring nodes. Finally, accurate scene graphs are produced by the relation inference module to recognize all entities and the corresponding relations. We evaluate our proposed method on the widely-adopted Visual Genome Dataset, and the results demonstrate the effectiveness and superiority of our model.},
  eventtitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-72813-293-8},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\K9DMYC4V\Qi 등 - 2019 - Attentive Relational Networks for Mapping Images t.pdf}
}

@online{qinExploringUniversalIntrinsic2022,
  title = {Exploring {{Universal Intrinsic Task Subspace}} via {{Prompt Tuning}}},
  author = {Qin, Yujia and Wang, Xiaozhi and Su, Yusheng and Lin, Yankai and Ding, Ning and Yi, Jing and Chen, Weize and Liu, Zhiyuan and Li, Juanzi and Hou, Lei and Li, Peng and Sun, Maosong and Zhou, Jie},
  date = {2022-11-25},
  eprint = {2110.07867},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2110.07867},
  url = {http://arxiv.org/abs/2110.07867},
  urldate = {2024-03-18},
  abstract = {Why can pre-trained language models (PLMs) learn universal representations and effectively adapt to broad NLP tasks differing a lot superficially? In this work, we empirically find evidence indicating that the adaptations of PLMs to various few-shot tasks can be reparameterized as optimizing only a few free parameters in a unified low-dimensional intrinsic task subspace, which may help us understand why PLMs could easily adapt to various NLP tasks with small-scale data. To find such a subspace and examine its universality, we propose an analysis pipeline called intrinsic prompt tuning (IPT). Specifically, we resort to the recent success of prompt tuning and decompose the soft prompts of multiple NLP tasks into the same low-dimensional nonlinear subspace, then we learn to adapt the PLM to unseen data or tasks by only tuning parameters in this subspace. In the experiments, we study diverse few-shot NLP tasks and surprisingly find that in a 250-dimensional subspace found with 100 tasks, by only tuning 250 free parameters, we can recover 97\% and 83\% of the full prompt tuning performance for 100 seen tasks (using different training data) and 20 unseen tasks, respectively, showing great generalization ability of the found intrinsic task subspace. Besides being an analysis tool, IPT could further help us improve the prompt tuning stability.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Qin et al_2022_Exploring Universal Intrinsic Task Subspace via Prompt Tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\G7PE35SP\\2110.html}
}

@online{qiPointNetDeepLearning2017,
  title = {{{PointNet}}: {{Deep Learning}} on {{Point Sets}} for {{3D Classification}} and {{Segmentation}}},
  shorttitle = {{{PointNet}}},
  author = {Qi, Charles R. and Su, Hao and Mo, Kaichun and Guibas, Leonidas J.},
  date = {2017-04-10},
  eprint = {1612.00593},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1612.00593},
  url = {http://arxiv.org/abs/1612.00593},
  urldate = {2023-08-05},
  abstract = {Point cloud is an important type of geometric data structure. Due to its irregular format, most researchers transform such data to regular 3D voxel grids or collections of images. This, however, renders data unnecessarily voluminous and causes issues. In this paper, we design a novel type of neural network that directly consumes point clouds and well respects the permutation invariance of points in the input. Our network, named PointNet, provides a unified architecture for applications ranging from object classification, part segmentation, to scene semantic parsing. Though simple, PointNet is highly efficient and effective. Empirically, it shows strong performance on par or even better than state of the art. Theoretically, we provide analysis towards understanding of what the network has learnt and why the network is robust with respect to input perturbation and corruption.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\3d image understanding\\Qi et al_2017_PointNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Z6RLSYLJ\\1612.html}
}

@online{qiPointNetDeepLearning2017a,
  title = {{{PointNet}}: {{Deep Learning}} on {{Point Sets}} for {{3D Classification}} and {{Segmentation}}},
  shorttitle = {{{PointNet}}},
  author = {Qi, Charles R. and Su, Hao and Mo, Kaichun and Guibas, Leonidas J.},
  date = {2017-04-10},
  eprint = {1612.00593},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1612.00593},
  urldate = {2023-06-26},
  abstract = {Point cloud is an important type of geometric data structure. Due to its irregular format, most researchers transform such data to regular 3D voxel grids or collections of images. This, however, renders data unnecessarily voluminous and causes issues. In this paper, we design a novel type of neural network that directly consumes point clouds and well respects the permutation invariance of points in the input. Our network, named PointNet, provides a unified architecture for applications ranging from object classification, part segmentation, to scene semantic parsing. Though simple, PointNet is highly efficient and effective. Empirically, it shows strong performance on par or even better than state of the art. Theoretically, we provide analysis towards understanding of what the network has learnt and why the network is robust with respect to input perturbation and corruption.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Qi et al_2017_PointNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7UH4CE5N\\1612.html}
}

@online{qiuLookingGlassNeural2023,
  title = {Looking {{Through}} the {{Glass}}: {{Neural Surface Reconstruction Against High Specular Reflections}}},
  shorttitle = {Looking {{Through}} the {{Glass}}},
  author = {Qiu, Jiaxiong and Jiang, Peng-Tao and Zhu, Yifan and Yin, Ze-Xin and Cheng, Ming-Ming and Ren, Bo},
  date = {2023-04-17},
  eprint = {2304.08706},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2304.08706},
  urldate = {2023-04-20},
  abstract = {Neural implicit methods have achieved high-quality 3D object surfaces under slight specular highlights. However, high specular reflections (HSR) often appear in front of target objects when we capture them through glasses. The complex ambiguity in these scenes violates the multi-view consistency, then makes it challenging for recent methods to reconstruct target objects correctly. To remedy this issue, we present a novel surface reconstruction framework, NeuS-HSR, based on implicit neural rendering. In NeuS-HSR, the object surface is parameterized as an implicit signed distance function (SDF). To reduce the interference of HSR, we propose decomposing the rendered image into two appearances: the target object and the auxiliary plane. We design a novel auxiliary plane module by combining physical assumptions and neural networks to generate the auxiliary plane appearance. Extensive experiments on synthetic and real-world datasets demonstrate that NeuS-HSR outperforms state-of-the-art approaches for accurate and robust target surface reconstruction against HSR. Code is available at https://github.com/JiaxiongQ/NeuS-HSR.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\surface normal\\Qiu et al_2023_Looking Through the Glass.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XL3C6FX4\\2304.html}
}

@online{rabanserFailingLoudlyEmpirical2019,
  title = {Failing {{Loudly}}: {{An Empirical Study}} of {{Methods}} for {{Detecting Dataset Shift}}},
  shorttitle = {Failing {{Loudly}}},
  author = {Rabanser, Stephan and Günnemann, Stephan and Lipton, Zachary C.},
  date = {2019-10-28},
  eprint = {1810.11953},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1810.11953},
  urldate = {2022-09-13},
  abstract = {We might hope that when faced with unexpected inputs, well-designed software systems would fire off warnings. Machine learning (ML) systems, however, which depend strongly on properties of their inputs (e.g. the i.i.d. assumption), tend to fail silently. This paper explores the problem of building ML systems that fail loudly, investigating methods for detecting dataset shift, identifying exemplars that most typify the shift, and quantifying shift malignancy. We focus on several datasets and various perturbations to both covariates and label distributions with varying magnitudes and fractions of data affected. Interestingly, we show that across the dataset shifts that we explore, a two-sample-testing-based approach, using pre-trained classifiers for dimensionality reduction, performs best. Moreover, we demonstrate that domain-discriminating approaches tend to be helpful for characterizing shifts qualitatively and determining if they are harmful.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Rabanser et al_2019_Failing Loudly.pdf;C\:\\Users\\chsey\\Zotero\\storage\\N6Z5DZVT\\1810.html}
}

@online{rabbyBeyondPixelsComprehensiveReview2023,
  title = {{{BeyondPixels}}: {{A Comprehensive Review}} of the {{Evolution}} of {{Neural Radiance Fields}}},
  shorttitle = {{{BeyondPixels}}},
  author = {Rabby, AKM Shahariar Azad and Zhang, Chengcui},
  date = {2023-06-05},
  eprint = {2306.03000},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2306.03000},
  url = {http://arxiv.org/abs/2306.03000},
  urldate = {2023-06-24},
  abstract = {Neural rendering combines ideas from classical computer graphics and machine learning to synthesize images from real-world observations. NeRF, short for Neural Radiance Fields, is a recent innovation that uses AI algorithms to create 3D objects from 2D images. By leveraging an interpolation approach, NeRF can produce new 3D reconstructed views of complicated scenes. Rather than directly restoring the whole 3D scene geometry, NeRF generates a volumetric representation called a ``radiance field,'' which is capable of creating color and density for every point within the relevant 3D space. The broad appeal and notoriety of NeRF make it imperative to examine the existing research on the topic comprehensively. While previous surveys on 3D rendering have primarily focused on traditional computer vision-based or deep learning-based approaches, only a handful of them discuss the potential of NeRF. However, such surveys have predominantly focused on NeRF's early contributions and have not explored its full potential. NeRF is a relatively new technique continuously being investigated for its capabilities and limitations. This survey reviews recent advances in NeRF and categorizes them according to their architectural designs, especially in the field of novel view synthesis.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Rabby_Zhang_2023_BeyondPixels.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UJNBW82M\\2306.html}
}

@online{rabeSelfattentionDoesNot2022,
  title = {Self-Attention {{Does Not Need}} \${{O}}(N\textasciicircum 2)\$ {{Memory}}},
  author = {Rabe, Markus N. and Staats, Charles},
  date = {2022-10-10},
  eprint = {2112.05682},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.05682},
  urldate = {2024-05-05},
  abstract = {We present a very simple algorithm for attention that requires \$O(1)\$ memory with respect to sequence length and an extension to self-attention that requires \$O(\textbackslash log n)\$ memory. This is in contrast with the frequently stated belief that self-attention requires \$O(n\textasciicircum 2)\$ memory. While the time complexity is still \$O(n\textasciicircum 2)\$, device memory rather than compute capability is often the limiting factor on modern accelerators. Thus, reducing the memory requirements of attention allows processing of longer sequences than might otherwise be feasible. We provide a practical implementation for accelerators that requires \$O(\textbackslash sqrt\{n\})\$ memory, is numerically stable, and is within a few percent of the runtime of the standard implementation of attention. We also demonstrate how to differentiate the function while remaining memory-efficient. For sequence length 16384, the memory overhead of self-attention is reduced by 59X for inference and by 32X for differentiation.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y:\paper\2024_research\Rabe_Staats_2022_Self-attention Does Not Need $O(n^2)$ Memory.pdf}
}

@article{radfordLanguageModelsAre,
  title = {Language {{Models}} Are {{Unsupervised Multitask Learners}}},
  author = {Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
  abstract = {Natural language processing tasks, such as question answering, machine translation, reading comprehension, and summarization, are typically approached with supervised learning on taskspecific datasets. We demonstrate that language models begin to learn these tasks without any explicit supervision when trained on a new dataset of millions of webpages called WebText. When conditioned on a document plus questions, the answers generated by the language model reach 55 F1 on the CoQA dataset - matching or exceeding the performance of 3 out of 4 baseline systems without using the 127,000+ training examples. The capacity of the language model is essential to the success of zero-shot task transfer and increasing it improves performance in a log-linear fashion across tasks. Our largest model, GPT-2, is a 1.5B parameter Transformer that achieves state of the art results on 7 out of 8 tested language modeling datasets in a zero-shot setting but still underfits WebText. Samples from the model reflect these improvements and contain coherent paragraphs of text. These findings suggest a promising path towards building language processing systems which learn to perform tasks from their naturally occurring demonstrations.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\FTLQSSG9\Radford 등 - Language Models are Unsupervised Multitask Learner.pdf}
}

@inproceedings{radfordLanguageModelsAre2019,
  title = {Language {{Models}} Are {{Unsupervised Multitask Learners}}},
  author = {Radford, Alec and Wu, Jeff and Child, R. and Luan, D. and Amodei, Dario and Sutskever, I.},
  date = {2019},
  url = {https://www.semanticscholar.org/paper/Language-Models-are-Unsupervised-Multitask-Learners-Radford-Wu/9405cc0d6169988371b2755e573cc28650d14dfe},
  urldate = {2024-05-10},
  abstract = {Natural language processing tasks, such as question answering, machine translation, reading comprehension, and summarization, are typically approached with supervised learning on taskspecific datasets. We demonstrate that language models begin to learn these tasks without any explicit supervision when trained on a new dataset of millions of webpages called WebText. When conditioned on a document plus questions, the answers generated by the language model reach 55 F1 on the CoQA dataset matching or exceeding the performance of 3 out of 4 baseline systems without using the 127,000+ training examples. The capacity of the language model is essential to the success of zero-shot task transfer and increasing it improves performance in a log-linear fashion across tasks. Our largest model, GPT-2, is a 1.5B parameter Transformer that achieves state of the art results on 7 out of 8 tested language modeling datasets in a zero-shot setting but still underfits WebText. Samples from the model reflect these improvements and contain coherent paragraphs of text. These findings suggest a promising path towards building language processing systems which learn to perform tasks from their naturally occurring demonstrations.},
  keywords = {notion},
  file = {Y:\paper\2024_research\Radford et al_2019_Language Models are Unsupervised Multitask Learners.pdf}
}

@online{radfordLearningTransferableVisual2021,
  title = {Learning {{Transferable Visual Models From Natural Language Supervision}}},
  author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
  date = {2021-02-26},
  eprint = {2103.00020},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.00020},
  urldate = {2023-05-06},
  abstract = {State-of-the-art computer vision systems are trained to predict a fixed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efficient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of fine-grained object classification. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset specific training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Radford et al_2021_Learning Transferable Visual Models From Natural Language Supervision.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SFHPJFUR\\2103.html}
}

@online{radfordLearningTransferableVisual2021a,
  title = {Learning {{Transferable Visual Models From Natural Language Supervision}}},
  author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
  date = {2021-02-26},
  eprint = {2103.00020},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2103.00020},
  url = {http://arxiv.org/abs/2103.00020},
  urldate = {2023-06-27},
  abstract = {State-of-the-art computer vision systems are trained to predict a fixed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efficient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of fine-grained object classification. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset specific training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Radford et al_2021_Learning Transferable Visual Models From Natural Language Supervision.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TKHQEB27\\2103.html}
}

@online{radfordUnsupervisedRepresentationLearning2016,
  title = {Unsupervised {{Representation Learning}} with {{Deep Convolutional Generative Adversarial Networks}}},
  author = {Radford, Alec and Metz, Luke and Chintala, Soumith},
  date = {2016-01-07},
  eprint = {1511.06434},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1511.06434},
  url = {http://arxiv.org/abs/1511.06434},
  urldate = {2023-08-05},
  abstract = {In recent years, supervised learning with convolutional networks (CNNs) has seen huge adoption in computer vision applications. Comparatively, unsupervised learning with CNNs has received less attention. In this work we hope to help bridge the gap between the success of CNNs for supervised learning and unsupervised learning. We introduce a class of CNNs called deep convolutional generative adversarial networks (DCGANs), that have certain architectural constraints, and demonstrate that they are a strong candidate for unsupervised learning. Training on various image datasets, we show convincing evidence that our deep convolutional adversarial pair learns a hierarchy of representations from object parts to scenes in both the generator and discriminator. Additionally, we use the learned features for novel tasks - demonstrating their applicability as general image representations.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\generative model\\Radford et al_2016_Unsupervised Representation Learning with Deep Convolutional Generative.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VPWBJEIA\\1511.html}
}

@online{rafailovYourLanguageModel2024,
  title = {From \$r\$ to \${{Q}}\textasciicircum *\$: {{Your Language Model}} Is {{Secretly}} a {{Q-Function}}},
  shorttitle = {From \$r\$ to \${{Q}}\textasciicircum *\$},
  author = {Rafailov, Rafael and Hejna, Joey and Park, Ryan and Finn, Chelsea},
  date = {2024-04-18},
  eprint = {2404.12358},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2404.12358},
  urldate = {2024-05-27},
  abstract = {Reinforcement Learning From Human Feedback (RLHF) has been a critical to the success of the latest generation of generative AI models. In response to the complex nature of the classical RLHF pipeline, direct alignment algorithms such as Direct Preference Optimization (DPO) have emerged as an alternative approach. Although DPO solves the same objective as the standard RLHF setup, there is a mismatch between the two approaches. Standard RLHF deploys reinforcement learning in a specific token-level MDP, while DPO is derived as a bandit problem in which the whole response of the model is treated as a single arm. In this work we rectify this difference, first we theoretically show that we can derive DPO in the token-level MDP as a general inverse Q-learning algorithm, which satisfies the Bellman equation. Using our theoretical results, we provide three concrete empirical insights. First, we show that because of its token level interpretation, DPO is able to perform some type of credit assignment. Next, we prove that under the token level formulation, classical search-based algorithms, such as MCTS, which have recently been applied to the language generation space, are equivalent to likelihood-based search on a DPO policy. Empirically we show that a simple beam search yields meaningful improvement over the base DPO policy. Finally, we show how the choice of reference policy causes implicit rewards to decline during training. We conclude by discussing applications of our work, including information elicitation in multi-tun dialogue, reasoning, agentic applications and end-to-end training of multi-model systems.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\5FMGBJSG\Rafailov 등 - 2024 - From $r$ to $Q^$ Your Language Model is Secretly.pdf}
}

@online{raffelExploringLimitsTransfer2023,
  title = {Exploring the {{Limits}} of {{Transfer Learning}} with a {{Unified Text-to-Text Transformer}}},
  author = {Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
  date = {2023-09-19},
  eprint = {1910.10683},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1910.10683},
  urldate = {2024-09-26},
  abstract = {Transfer learning, where a model is first pre-trained on a data-rich task before being fine-tuned on a downstream task, has emerged as a powerful technique in natural language processing (NLP). The effectiveness of transfer learning has given rise to a diversity of approaches, methodology, and practice. In this paper, we explore the landscape of transfer learning techniques for NLP by introducing a unified framework that converts all text-based language problems into a text-to-text format. Our systematic study compares pre-training objectives, architectures, unlabeled data sets, transfer approaches, and other factors on dozens of language understanding tasks. By combining the insights from our exploration with scale and our new ``Colossal Clean Crawled Corpus'', we achieve state-of-the-art results on many benchmarks covering summarization, question answering, text classification, and more. To facilitate future work on transfer learning for NLP, we release our data set, pre-trained models, and code.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\YG8MKDC6\Raffel 등 - 2023 - Exploring the Limits of Transfer Learning with a U.pdf}
}

@article{ramamoorthiPrecomputationBasedRendering2007,
  title = {Precomputation-{{Based Rendering}}},
  author = {Ramamoorthi, Ravi},
  date = {2007},
  journaltitle = {Foundations and Trends® in Computer Graphics and Vision},
  shortjournal = {FNT in Computer Graphics and Vision},
  volume = {3},
  number = {4},
  pages = {281--369},
  issn = {1572-2740, 1572-2759},
  doi = {10.1561/0600000021},
  url = {http://www.nowpublishers.com/article/Details/CGV-021},
  urldate = {2023-04-10},
  abstract = {High quality image synthesis is a long-standing goal in computer graphics. Complex lighting, reflection, shadow and global illumination effects can be rendered with modern image synthesis algorithms, but those methods are focused on offline computation of a single image. They are far from interactive, and the image must be recomputed from scratch when any aspect of the scene changes. On the other hand, real-time rendering often fixes the object geometry and other attributes, such as relighting a static image for lighting design. In these cases, the final image or rendering is a linear combination of basis images or radiance distributions due to individual lights. We can therefore precompute offline solutions to each individual light or lighting basis function, combining them efficiently for real-time image synthesis. Precomputationbased relighting and radiance transfer has a long history with a spurt of renewed interest, including adoption in commercial video games, due to recent mathematical developments and hardware advances. In this survey, we describe the mathematical foundations, history, current research and future directions for precomputation-based rendering.},
  langid = {english},
  file = {Y:\paper\2022 winter intern\Ramamoorthi_2007_Precomputation-Based Rendering.pdf}
}

@online{ranftlVisionTransformersDense2021,
  title = {Vision {{Transformers}} for {{Dense Prediction}}},
  author = {Ranftl, René and Bochkovskiy, Alexey and Koltun, Vladlen},
  date = {2021-03-24},
  eprint = {2103.13413},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.13413},
  urldate = {2023-07-01},
  abstract = {We introduce dense vision transformers, an architecture that leverages vision transformers in place of convolutional networks as a backbone for dense prediction tasks. We assemble tokens from various stages of the vision transformer into image-like representations at various resolutions and progressively combine them into full-resolution predictions using a convolutional decoder. The transformer backbone processes representations at a constant and relatively high resolution and has a global receptive field at every stage. These properties allow the dense vision transformer to provide finer-grained and more globally coherent predictions when compared to fully-convolutional networks. Our experiments show that this architecture yields substantial improvements on dense prediction tasks, especially when a large amount of training data is available. For monocular depth estimation, we observe an improvement of up to 28\% in relative performance when compared to a state-of-the-art fully-convolutional network. When applied to semantic segmentation, dense vision transformers set a new state of the art on ADE20K with 49.02\% mIoU. We further show that the architecture can be fine-tuned on smaller datasets such as NYUv2, KITTI, and Pascal Context where it also sets the new state of the art. Our models are available at https://github.com/intel-isl/DPT.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Ranftl et al_2021_Vision Transformers for Dense Prediction.pdf;C\:\\Users\\chsey\\Zotero\\storage\\A52DGNTC\\2103.html}
}

@article{raskarCodedExposurePhotography,
  title = {Coded {{Exposure Photography}}: {{Motion Deblurring}} Using {{Fluttered Shutter}}},
  author = {Raskar, Ramesh and Agrawal, Amit and Tumblin, Jack},
  pages = {10},
  abstract = {In a conventional single-exposure photograph, moving objects or moving cameras cause motion blur. The exposure time defines a temporal box filter that smears the moving object across the image by convolution. This box filter destroys important high-frequency spatial details so that deblurring via deconvolution becomes an illposed problem.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\reading assignment 1\Raskar et al_Coded Exposure Photography.pdf}
}

@inproceedings{raskarCodedExposurePhotography2006,
  title = {Coded Exposure Photography: {{Motion}} Deblurring Using Fluttered Shutter},
  shorttitle = {Coded Exposure Photography},
  author = {Raskar, R. and Agrawal, A. and Tumblin, J.},
  date = {2006},
  pages = {795--804},
  doi = {10.1145/1179352.1141957},
  abstract = {In a conventional single-exposure photograph, moving objects or moving cameras cause motion blur. The exposure time defines a temporal box filter that smears the moving object across the image by convolution. This box filter destroys important high-frequency spatial details so that deblurring via deconvolution becomes an ill-posed problem.Rather than leaving the shutter open for the entire exposure duration, we "flutter" the camera's shutter open and closed during the chosen exposure time with a binary pseudo-random sequence. The flutter changes the box filter to a broad-band filter that preserves high-frequency spatial details in the blurred image and the corresponding deconvolution becomes a well-posed problem. We demonstrate that manually-specified point spread functions are sufficient for several challenging cases of motion-blur removal including extremely large motions, textured backgrounds and partial occluders. Copyright © 2006 by the Association for Computing Machinery, Inc.},
  eventtitle = {{{ACM SIGGRAPH}} 2006 {{Papers}}, {{SIGGRAPH}} '06},
  isbn = {978-1-59593-364-5},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\3TNGQATM\display.html}
}

@inproceedings{rastgooSignLanguageProduction2021,
  title = {Sign {{Language Production}}: {{A Review}}},
  shorttitle = {Sign {{Language Production}}},
  booktitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition Workshops}} ({{CVPRW}})},
  author = {Rastgoo, Razieh and Kiani, Kourosh and Escalera, Sergio and Sabokrou, Mohammad},
  date = {2021-06},
  pages = {3446--3456},
  publisher = {IEEE},
  location = {Nashville, TN, USA},
  doi = {10.1109/CVPRW53098.2021.00384},
  url = {https://ieeexplore.ieee.org/document/9522839/},
  urldate = {2023-05-08},
  abstract = {Sign Language is the dominant yet non-primary form of communication language used in the deaf and hearingimpaired community. To make an easy and mutual communication between the hearing-impaired and the hearing communities, building a robust system capable of translating the spoken language into sign language and vice versa is fundamental. To this end, sign language recognition and production are two necessary parts for making such a two-way system. Sign language recognition and production need to cope with some critical challenges. In this survey, we review recent advances in Sign Language Production (SLP) and related areas using deep learning. This survey aims to briefly summarize recent achievements in SLP, discussing their advantages, limitations, and future directions of research.},
  eventtitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition Workshops}} ({{CVPRW}})},
  isbn = {978-1-66544-899-4},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\K7K4GCM7\Rastgoo 등 - 2021 - Sign Language Production A Review.pdf}
}

@inproceedings{rastgooSignLanguageProduction2021a,
  title = {Sign {{Language Production}}: {{A Review}}},
  shorttitle = {Sign {{Language Production}}},
  booktitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition Workshops}} ({{CVPRW}})},
  author = {Rastgoo, Razieh and Kiani, Kourosh and Escalera, Sergio and Sabokrou, Mohammad},
  date = {2021-06},
  pages = {3446--3456},
  publisher = {IEEE},
  location = {Nashville, TN, USA},
  doi = {10.1109/CVPRW53098.2021.00384},
  url = {https://ieeexplore.ieee.org/document/9522839/},
  urldate = {2023-05-09},
  abstract = {Sign Language is the dominant yet non-primary form of communication language used in the deaf and hearingimpaired community. To make an easy and mutual communication between the hearing-impaired and the hearing communities, building a robust system capable of translating the spoken language into sign language and vice versa is fundamental. To this end, sign language recognition and production are two necessary parts for making such a two-way system. Sign language recognition and production need to cope with some critical challenges. In this survey, we review recent advances in Sign Language Production (SLP) and related areas using deep learning. This survey aims to briefly summarize recent achievements in SLP, discussing their advantages, limitations, and future directions of research.},
  eventtitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition Workshops}} ({{CVPRW}})},
  isbn = {978-1-66544-899-4},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\Q84Y7SSJ\Rastgoo 등 - 2021 - Sign Language Production A Review.pdf}
}

@inproceedings{rastgooSignLanguageProduction2021b,
  title = {Sign {{Language Production}}: {{A Review}}},
  shorttitle = {Sign {{Language Production}}},
  author = {Rastgoo, Razieh and Kiani, Kourosh and Escalera, Sergio and Sabokrou, Mohammad},
  date = {2021},
  pages = {3451--3461},
  url = {https://openaccess.thecvf.com/content/CVPR2021W/ChaLearn/html/Rastgoo_Sign_Language_Production_A_Review_CVPRW_2021_paper.html},
  urldate = {2023-05-09},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  langid = {english},
  file = {Y:\paper\2023_PBL\Rastgoo et al_2021_Sign Language Production.pdf}
}

@online{redmonYOLO9000BetterFaster2016,
  title = {{{YOLO9000}}: {{Better}}, {{Faster}}, {{Stronger}}},
  shorttitle = {{{YOLO9000}}},
  author = {Redmon, Joseph and Farhadi, Ali},
  date = {2016-12-25},
  eprint = {1612.08242},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1612.08242},
  url = {http://arxiv.org/abs/1612.08242},
  urldate = {2023-08-05},
  abstract = {We introduce YOLO9000, a state-of-the-art, real-time object detection system that can detect over 9000 object categories. First we propose various improvements to the YOLO detection method, both novel and drawn from prior work. The improved model, YOLOv2, is state-of-the-art on standard detection tasks like PASCAL VOC and COCO. At 67 FPS, YOLOv2 gets 76.8 mAP on VOC 2007. At 40 FPS, YOLOv2 gets 78.6 mAP, outperforming state-of-the-art methods like Faster RCNN with ResNet and SSD while still running significantly faster. Finally we propose a method to jointly train on object detection and classification. Using this method we train YOLO9000 simultaneously on the COCO detection dataset and the ImageNet classification dataset. Our joint training allows YOLO9000 to predict detections for object classes that don't have labelled detection data. We validate our approach on the ImageNet detection task. YOLO9000 gets 19.7 mAP on the ImageNet detection validation set despite only having detection data for 44 of the 200 classes. On the 156 classes not in COCO, YOLO9000 gets 16.0 mAP. But YOLO can detect more than just 200 classes; it predicts detections for more than 9000 different object categories. And it still runs in real-time.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Redmon_Farhadi_2016_YOLO9000.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3J7R5VHV\\1612.html}
}

@online{redmonYouOnlyLook2016,
  title = {You {{Only Look Once}}: {{Unified}}, {{Real-Time Object Detection}}},
  shorttitle = {You {{Only Look Once}}},
  author = {Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  date = {2016-05-09},
  eprint = {1506.02640},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1506.02640},
  url = {http://arxiv.org/abs/1506.02640},
  urldate = {2023-08-05},
  abstract = {We present YOLO, a new approach to object detection. Prior work on object detection repurposes classifiers to perform detection. Instead, we frame object detection as a regression problem to spatially separated bounding boxes and associated class probabilities. A single neural network predicts bounding boxes and class probabilities directly from full images in one evaluation. Since the whole detection pipeline is a single network, it can be optimized end-to-end directly on detection performance. Our unified architecture is extremely fast. Our base YOLO model processes images in real-time at 45 frames per second. A smaller version of the network, Fast YOLO, processes an astounding 155 frames per second while still achieving double the mAP of other real-time detectors. Compared to state-of-the-art detection systems, YOLO makes more localization errors but is far less likely to predict false detections where nothing exists. Finally, YOLO learns very general representations of objects. It outperforms all other detection methods, including DPM and R-CNN, by a wide margin when generalizing from natural images to artwork on both the Picasso Dataset and the People-Art Dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Redmon et al_2016_You Only Look Once.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EYVRR7CP\\1506.html}
}

@online{redmonYouOnlyLook2016a,
  title = {You {{Only Look Once}}: {{Unified}}, {{Real-Time Object Detection}}},
  shorttitle = {You {{Only Look Once}}},
  author = {Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  date = {2016-05-09},
  eprint = {1506.02640},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1506.02640},
  urldate = {2022-07-25},
  abstract = {We present YOLO, a new approach to object detection. Prior work on object detection repurposes classifiers to perform detection. Instead, we frame object detection as a regression problem to spatially separated bounding boxes and associated class probabilities. A single neural network predicts bounding boxes and class probabilities directly from full images in one evaluation. Since the whole detection pipeline is a single network, it can be optimized end-to-end directly on detection performance. Our unified architecture is extremely fast. Our base YOLO model processes images in real-time at 45 frames per second. A smaller version of the network, Fast YOLO, processes an astounding 155 frames per second while still achieving double the mAP of other real-time detectors. Compared to state-of-the-art detection systems, YOLO makes more localization errors but is far less likely to predict false detections where nothing exists. Finally, YOLO learns very general representations of objects. It outperforms all other detection methods, including DPM and R-CNN, by a wide margin when generalizing from natural images to artwork on both the Picasso Dataset and the People-Art Dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\detection\\Redmon et al_2016_You Only Look Once.pdf;C\:\\Users\\chsey\\Zotero\\storage\\73LR9R5U\\1506.html}
}

@article{reinartzImpactDigitalTransformation2019,
  title = {The Impact of Digital Transformation on the Retailing Value Chain},
  author = {Reinartz, Werner and Wiegand, Nico and Imschloss, Monika},
  date = {2019-09-01},
  journaltitle = {International Journal of Research in Marketing},
  shortjournal = {International Journal of Research in Marketing},
  series = {Marketing {{Perspectives}} on {{Digital Business Models}}},
  volume = {36},
  number = {3},
  pages = {350--366},
  issn = {0167-8116},
  doi = {10.1016/j.ijresmar.2018.12.002},
  url = {https://www.sciencedirect.com/science/article/pii/S0167811618300739},
  urldate = {2023-12-28},
  abstract = {Consumers have traditionally made purchase decisions at the store shelf, giving institutional brick-and-mortar retailers great power to learn about and influence behaviors and preferences. With the rise of e-commerce, mobile shopping, and most recently smart technologies, new competitors threaten this long-standing supremacy. Adopting a value-creation perspective, we analyze how digitization started the erosion of institutional retailing as the primary interface to the customer. We develop a framework that identifies five new sources of value creation and propose how these advance and transform competition for this interface. Depending on the importance of the new sources of value creation (in different purchase situations), stationary retailing may prevail as an important interaction point in a multichannel decision journey. However, increasing diffusion of branded-product platforms including connected devices and online retail platforms is shifting this authority to new players. For the parties involved in this multilayered competition, acknowledging the changes and actively managing their position in the evolving eco-systems is crucial.},
  keywords = {Brands,Customer interface,Digitization,Platforms,Retailing}
}

@article{reinartzImpactDigitalTransformation2019a,
  title = {The Impact of Digital Transformation on the Retailing Value Chain},
  author = {Reinartz, Werner and Wiegand, Nico and Imschloss, Monika},
  date = {2019-09-01},
  journaltitle = {International Journal of Research in Marketing},
  shortjournal = {International Journal of Research in Marketing},
  series = {Marketing {{Perspectives}} on {{Digital Business Models}}},
  volume = {36},
  number = {3},
  pages = {350--366},
  issn = {0167-8116},
  doi = {10.1016/j.ijresmar.2018.12.002},
  url = {https://www.sciencedirect.com/science/article/pii/S0167811618300739},
  urldate = {2023-12-28},
  abstract = {Consumers have traditionally made purchase decisions at the store shelf, giving institutional brick-and-mortar retailers great power to learn about and influence behaviors and preferences. With the rise of e-commerce, mobile shopping, and most recently smart technologies, new competitors threaten this long-standing supremacy. Adopting a value-creation perspective, we analyze how digitization started the erosion of institutional retailing as the primary interface to the customer. We develop a framework that identifies five new sources of value creation and propose how these advance and transform competition for this interface. Depending on the importance of the new sources of value creation (in different purchase situations), stationary retailing may prevail as an important interaction point in a multichannel decision journey. However, increasing diffusion of branded-product platforms including connected devices and online retail platforms is shifting this authority to new players. For the parties involved in this multilayered competition, acknowledging the changes and actively managing their position in the evolving eco-systems is crucial.},
  keywords = {Brands,Customer interface,Digitization,Platforms,Retailing}
}

@inproceedings{reiserKiloNeRFSpeedingNeural2021,
  title = {KiloNeRF: Speeding Up Neural Radiance Fields With Thousands of Tiny MLPs},
  shorttitle = {KiloNeRF},
  author = {Reiser, Christian and Peng, Songyou and Liao, Yiyi and Geiger, Andreas},
  date = {2021},
  pages = {14335--14345},
  url = {https://openaccess.thecvf.com/content/ICCV2021/html/Reiser_KiloNeRF_Speeding_Up_Neural_Radiance_Fields_With_Thousands_of_Tiny_ICCV_2021_paper.html},
  urldate = {2023-01-02},
  eventtitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
  langid = {korean-han},
  file = {Y:\paper\2022 winter intern\Reiser et al_2021_KiloNeRF.pdf}
}

@online{renExploringModelsData2015,
  title = {Exploring {{Models}} and {{Data}} for {{Image Question Answering}}},
  author = {Ren, Mengye and Kiros, Ryan and Zemel, Richard},
  date = {2015-05-08},
  eprint = {1505.02074},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1505.02074},
  urldate = {2023-05-28},
  abstract = {This work aims to address the problem of image-based question-answering (QA) with new models and datasets. In our work, we propose to use neural networks and visual semantic embeddings, without intermediate stages such as object detection and image segmentation, to predict answers to simple questions about images. Our model performs 1.8 times better than the only published results on an existing image QA dataset. We also present a question generation algorithm that converts image descriptions, which are widely available, into QA form. We used this algorithm to produce an order-of-magnitude larger dataset, with more evenly distributed answers. A suite of baseline results on this new dataset are also presented.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\VQA\\Ren et al_2015_Exploring Models and Data for Image Question Answering.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5V3XJ9N9\\1505.html}
}

@inproceedings{renFasterRCNNRealTime2015,
  title = {Faster {{R-CNN}}: {{Towards Real-Time Object Detection}} with {{Region Proposal Networks}}},
  shorttitle = {Faster {{R-CNN}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  date = {2015},
  volume = {28},
  publisher = {Curran Associates, Inc.},
  url = {https://papers.nips.cc/paper/2015/hash/14bfa6bb14875e45bba028a21ed38046-Abstract.html},
  urldate = {2022-08-03},
  abstract = {State-of-the-art object detection networks depend on region proposal algorithms to hypothesize object locations. Advances like SPPnet and Fast R-CNN have reduced the running time of these detection networks, exposing region proposal computation as a bottleneck. In this work, we introduce a Region Proposal Network (RPN) that shares full-image convolutional features with the detection network, thus enabling nearly cost-free region proposals. An RPN is a fully-convolutional network that simultaneously predicts object bounds and objectness scores at each position. RPNs are trained end-to-end to generate high-quality region proposals, which are used by Fast R-CNN for detection. With a simple alternating optimization, RPN and Fast R-CNN can be trained to share convolutional features. For the very deep VGG-16 model, our detection system has a frame rate of 5fps (including all steps) on a GPU, while achieving state-of-the-art object detection accuracy on PASCAL VOC 2007 (73.2\% mAP) and 2012 (70.4\% mAP) using 300 proposals per image. Code is available at https://github.com/ShaoqingRen/faster\_rcnn.},
  file = {Y:\paper\Computer Vision\detection\Ren et al_2015_Faster R-CNN.pdf}
}

@inproceedings{renFasterRCNNRealTime2015a,
  title = {Faster {{R-CNN}}: {{Towards Real-Time Object Detection}} with {{Region Proposal Networks}}},
  shorttitle = {Faster {{R-CNN}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  date = {2015},
  volume = {28},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper_files/paper/2015/hash/14bfa6bb14875e45bba028a21ed38046-Abstract.html},
  urldate = {2023-05-28},
  abstract = {State-of-the-art object detection networks depend on region proposal algorithms to hypothesize object locations. Advances like SPPnet and Fast R-CNN have reduced the running time of these detection networks, exposing region proposal computation as a bottleneck. In this work, we introduce a Region Proposal Network (RPN) that shares full-image convolutional features with the detection network, thus enabling nearly cost-free region proposals. An RPN is a fully-convolutional network that simultaneously predicts object bounds and objectness scores at each position. RPNs are trained end-to-end to generate high-quality region proposals, which are used by Fast R-CNN for detection. With a simple alternating optimization, RPN and Fast R-CNN can be trained to share convolutional features. For the very deep VGG-16 model, our detection system has a frame rate of 5fps (including all steps) on a GPU, while achieving state-of-the-art object detection accuracy on PASCAL VOC 2007 (73.2\% mAP) and 2012 (70.4\% mAP) using 300 proposals per image. Code is available at https://github.com/ShaoqingRen/faster\_rcnn.},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Ren et al_2015_Faster R-CNN.pdf}
}

@online{renFasterRCNNRealTime2016,
  title = {Faster {{R-CNN}}: {{Towards Real-Time Object Detection}} with {{Region Proposal Networks}}},
  shorttitle = {Faster {{R-CNN}}},
  author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  date = {2016-01-06},
  eprint = {1506.01497},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1506.01497},
  url = {http://arxiv.org/abs/1506.01497},
  urldate = {2023-08-05},
  abstract = {State-of-the-art object detection networks depend on region proposal algorithms to hypothesize object locations. Advances like SPPnet and Fast R-CNN have reduced the running time of these detection networks, exposing region proposal computation as a bottleneck. In this work, we introduce a Region Proposal Network (RPN) that shares full-image convolutional features with the detection network, thus enabling nearly cost-free region proposals. An RPN is a fully convolutional network that simultaneously predicts object bounds and objectness scores at each position. The RPN is trained end-to-end to generate high-quality region proposals, which are used by Fast R-CNN for detection. We further merge RPN and Fast R-CNN into a single network by sharing their convolutional features---using the recently popular terminology of neural networks with 'attention' mechanisms, the RPN component tells the unified network where to look. For the very deep VGG-16 model, our detection system has a frame rate of 5fps (including all steps) on a GPU, while achieving state-of-the-art object detection accuracy on PASCAL VOC 2007, 2012, and MS COCO datasets with only 300 proposals per image. In ILSVRC and COCO 2015 competitions, Faster R-CNN and RPN are the foundations of the 1st-place winning entries in several tracks. Code has been made publicly available.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Ren et al_2016_Faster R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\C88XQNFA\\1506.html}
}

@online{renFasterRCNNRealTime2016a,
  title = {Faster {{R-CNN}}: {{Towards Real-Time Object Detection}} with {{Region Proposal Networks}}},
  shorttitle = {Faster {{R-CNN}}},
  author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  date = {2016-01-06},
  eprint = {1506.01497},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1506.01497},
  url = {http://arxiv.org/abs/1506.01497},
  urldate = {2022-07-04},
  abstract = {State-of-the-art object detection networks depend on region proposal algorithms to hypothesize object locations. Advances like SPPnet and Fast R-CNN have reduced the running time of these detection networks, exposing region proposal computation as a bottleneck. In this work, we introduce a Region Proposal Network (RPN) that shares full-image convolutional features with the detection network, thus enabling nearly cost-free region proposals. An RPN is a fully convolutional network that simultaneously predicts object bounds and objectness scores at each position. The RPN is trained end-to-end to generate high-quality region proposals, which are used by Fast R-CNN for detection. We further merge RPN and Fast R-CNN into a single network by sharing their convolutional features---using the recently popular terminology of neural networks with 'attention' mechanisms, the RPN component tells the unified network where to look. For the very deep VGG-16 model, our detection system has a frame rate of 5fps (including all steps) on a GPU, while achieving state-of-the-art object detection accuracy on PASCAL VOC 2007, 2012, and MS COCO datasets with only 300 proposals per image. In ILSVRC and COCO 2015 competitions, Faster R-CNN and RPN are the foundations of the 1st-place winning entries in several tracks. Code has been made publicly available.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Ren et al_2016_Faster R-CNN.pdf;C\:\\Users\\chsey\\Zotero\\storage\\L8EU5G5C\\1506.html}
}

@online{renSimpleFixMahalanobis2021,
  title = {A {{Simple Fix}} to {{Mahalanobis Distance}} for {{Improving Near-OOD Detection}}},
  author = {Ren, Jie and Fort, Stanislav and Liu, Jeremiah and Roy, Abhijit Guha and Padhy, Shreyas and Lakshminarayanan, Balaji},
  date = {2021-06-16},
  eprint = {2106.09022},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2106.09022},
  url = {http://arxiv.org/abs/2106.09022},
  urldate = {2022-09-07},
  abstract = {Mahalanobis distance (MD) is a simple and popular post-processing method for detecting out-of-distribution (OOD) inputs in neural networks. We analyze its failure modes for near-OOD detection and propose a simple fix called relative Mahalanobis distance (RMD) which improves performance and is more robust to hyperparameter choice. On a wide selection of challenging vision, language, and biology OOD benchmarks (CIFAR-100 vs CIFAR-10, CLINC OOD intent detection, Genomics OOD), we show that RMD meaningfully improves upon MD performance (by up to 15\% AUROC on genomics OOD).},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Ren et al_2021_A Simple Fix to Mahalanobis Distance for Improving Near-OOD Detection.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RM5MNA6H\\2106.html}
}

@online{rhinehartFirstPersonActivityForecasting2017,
  title = {First-{{Person Activity Forecasting}} with {{Online Inverse Reinforcement Learning}}},
  author = {Rhinehart, Nicholas and Kitani, Kris M.},
  date = {2017-08-06},
  eprint = {1612.07796},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1612.07796},
  url = {http://arxiv.org/abs/1612.07796},
  urldate = {2023-08-05},
  abstract = {We address the problem of incrementally modeling and forecasting long-term goals of a first-person camera wearer: what the user will do, where they will go, and what goal they seek. In contrast to prior work in trajectory forecasting, our algorithm, DARKO, goes further to reason about semantic states (will I pick up an object?), and future goal states that are far in terms of both space and time. DARKO learns and forecasts from first-person visual observations of the user's daily behaviors via an Online Inverse Reinforcement Learning (IRL) approach. Classical IRL discovers only the rewards in a batch setting, whereas DARKO discovers the states, transitions, rewards, and goals of a user from streaming data. Among other results, we show DARKO forecasts goals better than competing methods in both noisy and ideal settings, and our approach is theoretically and empirically no-regret.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\video prediction\\Rhinehart_Kitani_2017_First-Person Activity Forecasting with Online Inverse Reinforcement Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RDM69JDP\\1612.html}
}

@online{rombachHighResolutionImageSynthesis2022,
  title = {High-{{Resolution Image Synthesis}} with {{Latent Diffusion Models}}},
  author = {Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Björn},
  date = {2022-04-13},
  eprint = {2112.10752},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2112.10752},
  url = {http://arxiv.org/abs/2112.10752},
  urldate = {2024-01-25},
  abstract = {By decomposing the image formation process into a sequential application of denoising autoencoders, diffusion models (DMs) achieve state-of-the-art synthesis results on image data and beyond. Additionally, their formulation allows for a guiding mechanism to control the image generation process without retraining. However, since these models typically operate directly in pixel space, optimization of powerful DMs often consumes hundreds of GPU days and inference is expensive due to sequential evaluations. To enable DM training on limited computational resources while retaining their quality and flexibility, we apply them in the latent space of powerful pretrained autoencoders. In contrast to previous work, training diffusion models on such a representation allows for the first time to reach a near-optimal point between complexity reduction and detail preservation, greatly boosting visual fidelity. By introducing cross-attention layers into the model architecture, we turn diffusion models into powerful and flexible generators for general conditioning inputs such as text or bounding boxes and high-resolution synthesis becomes possible in a convolutional manner. Our latent diffusion models (LDMs) achieve a new state of the art for image inpainting and highly competitive performance on various tasks, including unconditional image generation, semantic scene synthesis, and super-resolution, while significantly reducing computational requirements compared to pixel-based DMs. Code is available at https://github.com/CompVis/latent-diffusion .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Rombach et al_2022_High-Resolution Image Synthesis with Latent Diffusion Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TESHYVPA\\2112.html}
}

@online{rombachHighResolutionImageSynthesis2022a,
  title = {High-{{Resolution Image Synthesis}} with {{Latent Diffusion Models}}},
  author = {Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Björn},
  date = {2022-04-13},
  eprint = {2112.10752},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2112.10752},
  url = {http://arxiv.org/abs/2112.10752},
  urldate = {2023-08-25},
  abstract = {By decomposing the image formation process into a sequential application of denoising autoencoders, diffusion models (DMs) achieve state-of-the-art synthesis results on image data and beyond. Additionally, their formulation allows for a guiding mechanism to control the image generation process without retraining. However, since these models typically operate directly in pixel space, optimization of powerful DMs often consumes hundreds of GPU days and inference is expensive due to sequential evaluations. To enable DM training on limited computational resources while retaining their quality and flexibility, we apply them in the latent space of powerful pretrained autoencoders. In contrast to previous work, training diffusion models on such a representation allows for the first time to reach a near-optimal point between complexity reduction and detail preservation, greatly boosting visual fidelity. By introducing cross-attention layers into the model architecture, we turn diffusion models into powerful and flexible generators for general conditioning inputs such as text or bounding boxes and high-resolution synthesis becomes possible in a convolutional manner. Our latent diffusion models (LDMs) achieve a new state of the art for image inpainting and highly competitive performance on various tasks, including unconditional image generation, semantic scene synthesis, and super-resolution, while significantly reducing computational requirements compared to pixel-based DMs. Code is available at https://github.com/CompVis/latent-diffusion .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Rombach et al_2022_High-Resolution Image Synthesis with Latent Diffusion Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EPMXFYM9\\2112.html}
}

@article{ronnebergerUNetConvolutionalNetworks2015,
  title = {U-{{Net}}: {{Convolutional Networks}} for {{Biomedical Image Segmentation}}},
  shorttitle = {U-{{Net}}},
  author = {Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  date = {2015-05-18},
  doi = {10.48550/arXiv.1505.04597},
  url = {https://arxiv.org/abs/1505.04597v1},
  urldate = {2022-12-09},
  abstract = {There is large consent that successful training of deep networks requires many thousand annotated training samples. In this paper, we present a network and training strategy that relies on the strong use of data augmentation to use the available annotated samples more efficiently. The architecture consists of a contracting path to capture context and a symmetric expanding path that enables precise localization. We show that such a network can be trained end-to-end from very few images and outperforms the prior best method (a sliding-window convolutional network) on the ISBI challenge for segmentation of neuronal structures in electron microscopic stacks. Using the same network trained on transmitted light microscopy images (phase contrast and DIC) we won the ISBI cell tracking challenge 2015 in these categories by a large margin. Moreover, the network is fast. Segmentation of a 512x512 image takes less than a second on a recent GPU. The full implementation (based on Caffe) and the trained networks are available at http://lmb.informatik.uni-freiburg.de/people/ronneber/u-net .},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA3\Ronneberger et al_2015_U-Net.pdf}
}

@book{rudinRealComplexAnalysis1987,
  title = {Real and Complex Analysis},
  author = {Rudin, Walter},
  date = {1987},
  edition = {3rd ed},
  publisher = {McGraw-Hill},
  location = {New York},
  isbn = {978-0-07-054234-1},
  langid = {english},
  pagetotal = {416},
  keywords = {Mathematical analysis},
  file = {Y:\paper\textbook\Rudin_1987_Real and complex analysis.pdf}
}

@online{russakovskyImageNetLargeScale2015,
  title = {{{ImageNet Large Scale Visual Recognition Challenge}}},
  author = {Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and Berg, Alexander C. and Fei-Fei, Li},
  date = {2015-01-29},
  eprint = {1409.0575},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1409.0575},
  url = {http://arxiv.org/abs/1409.0575},
  urldate = {2022-12-09},
  abstract = {The ImageNet Large Scale Visual Recognition Challenge is a benchmark in object category classification and detection on hundreds of object categories and millions of images. The challenge has been run annually from 2010 to present, attracting participation from more than fifty institutions. This paper describes the creation of this benchmark dataset and the advances in object recognition that have been possible as a result. We discuss the challenges of collecting large-scale ground truth annotation, highlight key breakthroughs in categorical object recognition, provide a detailed analysis of the current state of the field of large-scale image classification and object detection, and compare the state-of-the-art computer vision accuracy with human accuracy. We conclude with lessons learned in the five years of the challenge, and propose future directions and improvements.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,I.4.8,I.5.2},
  file = {Y\:\\paper\\Computer Vision\\traditional\\PA3\\Russakovsky et al_2015_ImageNet Large Scale Visual Recognition Challenge.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HRZMN77K\\1409.html}
}

@online{russakovskyImageNetLargeScale2015a,
  title = {{{ImageNet Large Scale Visual Recognition Challenge}}},
  author = {Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and Berg, Alexander C. and Fei-Fei, Li},
  date = {2015-01-29},
  eprint = {1409.0575},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1409.0575},
  url = {http://arxiv.org/abs/1409.0575},
  urldate = {2023-11-19},
  abstract = {The ImageNet Large Scale Visual Recognition Challenge is a benchmark in object category classification and detection on hundreds of object categories and millions of images. The challenge has been run annually from 2010 to present, attracting participation from more than fifty institutions. This paper describes the creation of this benchmark dataset and the advances in object recognition that have been possible as a result. We discuss the challenges of collecting large-scale ground truth annotation, highlight key breakthroughs in categorical object recognition, provide a detailed analysis of the current state of the field of large-scale image classification and object detection, and compare the state-of-the-art computer vision accuracy with human accuracy. We conclude with lessons learned in the five years of the challenge, and propose future directions and improvements.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,I.4.8,I.5.2},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Russakovsky et al_2015_ImageNet Large Scale Visual Recognition Challenge.pdf;C\:\\Users\\chsey\\Zotero\\storage\\YKWMSMX9\\1409.html}
}

@article{rustowiczCropClassificationMultiTemporal,
  title = {Crop {{Classiﬁcation}} with {{Multi-Temporal Satellite Imagery}}},
  author = {Rustowicz, Rose M},
  pages = {6},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\QCS5353Y\Rustowicz_Crop Classiﬁcation with Multi-Temporal Satellite Imagery.pdf}
}

@online{rusuProgressiveNeuralNetworks2022,
  title = {Progressive {{Neural Networks}}},
  author = {Rusu, Andrei A. and Rabinowitz, Neil C. and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  date = {2022-10-22},
  eprint = {1606.04671},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1606.04671},
  urldate = {2023-12-23},
  abstract = {Learning to solve complex sequences of tasks--while both leveraging transfer and avoiding catastrophic forgetting--remains a key obstacle to achieving human-level intelligence. The progressive networks approach represents a step forward in this direction: they are immune to forgetting and can leverage prior knowledge via lateral connections to previously learned features. We evaluate this architecture extensively on a wide variety of reinforcement learning tasks (Atari and 3D maze games), and show that it outperforms common baselines based on pretraining and finetuning. Using a novel sensitivity measure, we demonstrate that transfer occurs at both low-level sensory and high-level control layers of the learned policy.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Rusu et al_2022_Progressive Neural Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XMPCADUN\\1606.html}
}

@online{rusuProgressiveNeuralNetworks2022a,
  title = {Progressive {{Neural Networks}}},
  author = {Rusu, Andrei A. and Rabinowitz, Neil C. and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  date = {2022-10-22},
  eprint = {1606.04671},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1606.04671},
  url = {http://arxiv.org/abs/1606.04671},
  urldate = {2023-12-23},
  abstract = {Learning to solve complex sequences of tasks--while both leveraging transfer and avoiding catastrophic forgetting--remains a key obstacle to achieving human-level intelligence. The progressive networks approach represents a step forward in this direction: they are immune to forgetting and can leverage prior knowledge via lateral connections to previously learned features. We evaluate this architecture extensively on a wide variety of reinforcement learning tasks (Atari and 3D maze games), and show that it outperforms common baselines based on pretraining and finetuning. Using a novel sensitivity measure, we demonstrate that transfer occurs at both low-level sensory and high-level control layers of the learned policy.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Rusu et al_2022_Progressive Neural Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NJHK23BK\\1606.html}
}

@online{safranOptimizationBasedSeparationsNeural2023,
  title = {Optimization-{{Based Separations}} for {{Neural Networks}}},
  author = {Safran, Itay and Lee, Jason D.},
  date = {2023-02-02},
  eprint = {2112.02393},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.02393},
  urldate = {2024-03-06},
  abstract = {Depth separation results propose a possible theoretical explanation for the benefits of deep neural networks over shallower architectures, establishing that the former possess superior approximation capabilities. However, there are no known results in which the deeper architecture leverages this advantage into a provable optimization guarantee. We prove that when the data are generated by a distribution with radial symmetry which satisfies some mild assumptions, gradient descent can efficiently learn ball indicator functions using a depth 2 neural network with two layers of sigmoidal activations, and where the hidden layer is held fixed throughout training. By building on and refining existing techniques for approximation lower bounds of neural networks with a single layer of non-linearities, we show that there are \$d\$-dimensional radial distributions on the data such that ball indicators cannot be learned efficiently by any algorithm to accuracy better than \$\textbackslash Omega(d\textasciicircum\{-4\})\$, nor by a standard gradient descent implementation to accuracy better than a constant. These results establish what is to the best of our knowledge, the first optimization-based separations where the approximation benefits of the stronger architecture provably manifest in practice. Our proof technique introduces new tools and ideas that may be of independent interest in the theoretical study of both the approximation and optimization of neural networks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Safran_Lee_2023_Optimization-Based Separations for Neural Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\47L75T3P\\2112.html}
}

@article{saitoPrecisionRecallPlotMore2015,
  title = {The {{Precision-Recall Plot Is More Informative}} than the {{ROC Plot When Evaluating Binary Classifiers}} on {{Imbalanced Datasets}}},
  author = {Saito, Takaya and Rehmsmeier, Marc},
  editor = {Brock, Guy},
  date = {2015-03-04},
  journaltitle = {PLOS ONE},
  shortjournal = {PLoS ONE},
  volume = {10},
  number = {3},
  pages = {e0118432},
  issn = {1932-6203},
  doi = {10.1371/journal.pone.0118432},
  url = {https://dx.plos.org/10.1371/journal.pone.0118432},
  urldate = {2022-09-27},
  langid = {english},
  file = {Y:\paper\2022 autumn intern\OOD\Saito_Rehmsmeier_2015_The Precision-Recall Plot Is More Informative than the ROC Plot When Evaluating.pdf}
}

@online{salehTaxonomyComputationalModels2015,
  title = {Toward a {{Taxonomy}} and {{Computational Models}} of {{Abnormalities}} in {{Images}}},
  author = {Saleh, Babak and Elgammal, Ahmed and Feldman, Jacob and Farhadi, Ali},
  date = {2015-12-04},
  eprint = {1512.01325},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  doi = {10.48550/arXiv.1512.01325},
  url = {http://arxiv.org/abs/1512.01325},
  urldate = {2023-08-05},
  abstract = {The human visual system can spot an abnormal image, and reason about what makes it strange. This task has not received enough attention in computer vision. In this paper we study various types of atypicalities in images in a more comprehensive way than has been done before. We propose a new dataset of abnormal images showing a wide range of atypicalities. We design human subject experiments to discover a coarse taxonomy of the reasons for abnormality. Our experiments reveal three major categories of abnormality: object-centric, scene-centric, and contextual. Based on this taxonomy, we propose a comprehensive computational model that can predict all different types of abnormality in images and outperform prior arts in abnormality recognition.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Human-Computer Interaction,Computer Science - Information Theory,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\visual common sense reasoning\\Saleh et al_2015_Toward a Taxonomy and Computational Models of Abnormalities in Images.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WSNV8YYN\\1512.html}
}

@online{santoroSimpleNeuralNetwork2017,
  title = {A Simple Neural Network Module for Relational Reasoning},
  author = {Santoro, Adam and Raposo, David and Barrett, David G. T. and Malinowski, Mateusz and Pascanu, Razvan and Battaglia, Peter and Lillicrap, Timothy},
  date = {2017-06-05},
  eprint = {1706.01427},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.01427},
  url = {http://arxiv.org/abs/1706.01427},
  urldate = {2023-08-05},
  abstract = {Relational reasoning is a central component of generally intelligent behavior, but has proven difficult for neural networks to learn. In this paper we describe how to use Relation Networks (RNs) as a simple plug-and-play module to solve problems that fundamentally hinge on relational reasoning. We tested RN-augmented networks on three tasks: visual question answering using a challenging dataset called CLEVR, on which we achieve state-of-the-art, super-human performance; text-based question answering using the bAbI suite of tasks; and complex reasoning about dynamic physical systems. Then, using a curated dataset called Sort-of-CLEVR we show that powerful convolutional networks do not have a general capacity to solve relational questions, but can gain this capacity when augmented with RNs. Our work shows how a deep learning architecture equipped with an RN module can implicitly discover and learn to reason about entities and their relations.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\relational reasoning\\Santoro et al_2017_A simple neural network module for relational reasoning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\C6AKBNPD\\1706.html}
}

@inproceedings{santurkarHowDoesBatch2018,
  title = {How {{Does Batch Normalization Help Optimization}}?},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Santurkar, Shibani and Tsipras, Dimitris and Ilyas, Andrew and Madry, Aleksander},
  date = {2018},
  volume = {31},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2018/hash/905056c1ac1dad141560467e0a99e1cf-Abstract.html},
  urldate = {2022-07-09},
  abstract = {Batch Normalization (BatchNorm) is a widely adopted technique that enables faster and more stable training of deep neural networks (DNNs). Despite its pervasiveness, the exact reasons for BatchNorm's effectiveness are still poorly understood. The popular belief is that this effectiveness stems from controlling the change of the layers' input distributions during training to reduce the so-called "internal covariate shift". In this work, we demonstrate that such distributional stability of layer inputs has little to do with the success of BatchNorm. Instead, we uncover a more fundamental impact of BatchNorm on the training process: it makes the optimization landscape significantly smoother. This smoothness induces a more predictive and stable behavior of the gradients, allowing for faster training.},
  file = {Y:\paper\Computer Vision\temporary\Santurkar et al_2018_How Does Batch Normalization Help Optimization.pdf}
}

@online{saundersProgressiveTransformersEndtoEnd2020,
  title = {Progressive {{Transformers}} for {{End-to-End Sign Language Production}}},
  author = {Saunders, Ben and Camgoz, Necati Cihan and Bowden, Richard},
  date = {2020-07-20},
  eprint = {2004.14874},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2004.14874},
  url = {http://arxiv.org/abs/2004.14874},
  urldate = {2023-05-03},
  abstract = {The goal of automatic Sign Language Production (SLP) is to translate spoken language to a continuous stream of sign language video at a level comparable to a human translator. If this was achievable, then it would revolutionise Deaf hearing communications. Previous work on predominantly isolated SLP has shown the need for architectures that are better suited to the continuous domain of full sign sequences. In this paper, we propose Progressive Transformers, a novel architecture that can translate from discrete spoken language sentences to continuous 3D skeleton pose outputs representing sign language. We present two model configurations, an end-to-end network that produces sign direct from text and a stacked network that utilises a gloss intermediary. Our transformer network architecture introduces a counter that enables continuous sequence generation at training and inference. We also provide several data augmentation processes to overcome the problem of drift and improve the performance of SLP models. We propose a back translation evaluation mechanism for SLP, presenting benchmark quantitative results on the challenging RWTH-PHOENIX-Weather-2014T(PHOENIX14T) dataset and setting baselines for future research.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023_PBL\\Saunders et al_2020_Progressive Transformers for End-to-End Sign Language Production.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MWB4EPHX\\2004.html}
}

@inproceedings{scharsteinTaxonomyEvaluationDense2001,
  title = {A Taxonomy and Evaluation of Dense Two-Frame Stereo Correspondence Algorithms},
  booktitle = {Proceedings {{IEEE Workshop}} on {{Stereo}} and {{Multi-Baseline Vision}} ({{SMBV}} 2001)},
  author = {Scharstein, D. and Szeliski, R. and Zabih, R.},
  date = {2001},
  pages = {131--140},
  publisher = {IEEE Comput. Soc},
  location = {Kauai, HI, USA},
  doi = {10.1109/SMBV.2001.988771},
  url = {http://ieeexplore.ieee.org/document/988771/},
  urldate = {2022-10-03},
  abstract = {Stereo matching is one of the most active research areas in computer vision. While a large number of algorithms for stereo correspondence have been developed, relatively little work has been done on characterizing their performance. In this paper, we present a taxonomy of dense, two-frame stereo methods. Our taxonomy is designed to assess the different components and design decisions made in individual stereo algorithms. Using this taxonomy, we compare existing stereo methods and present experiments evaluating the performance of many different variants. In order to establish a common software platform and a collection of data sets for easy evaluation, we have designed a stand-alone, flexible C++ implementation that enables the evaluation of individual components and that can easily be extended to include new algorithms. We have also produced several new multi-frame stereo data sets with ground truth and are making both the code and data sets available on the Web. Finally, we include a comparative evaluation of a large set of today’s best-performing stereo algorithms.},
  eventtitle = {{{IEEE Workshop}} on {{Stereo}} and {{Multi-Baseline Vision}} ({{SMBV}} 2001)},
  isbn = {978-0-7695-1327-0},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\reading assignment 2\Scharstein et al_2001_A taxonomy and evaluation of dense two-frame stereo correspondence algorithms.pdf}
}

@book{schmidtWristwatchHandbookComprehensive2016,
  title = {The {{Wristwatch Handbook}}: {{A Comprehensive Guide}} to {{Mechanical Wristwatches}}},
  shorttitle = {The {{Wristwatch Handbook}}},
  author = {Schmidt, Ryan},
  date = {2016-10-14},
  publisher = {Acc Art Books},
  abstract = {A fantastic reference work for the novice or the seasoned watch enthusiastFully illustrated with 470 color photographsBrand-Agnostic. Features a vast array of timepieces from over 90 manufacturersDespite the functional obsolescence of the mechanical wristwatch (our phones and computers tell more accurate time) the early 21st Century has seen a boom in the development, production, and appreciation of all things horological. Whether it is presented to the collector as an alternative investment, as a feat of micro-mechanical technology, or as a showcase of artisanal mastery, the mechanical wristwatch has never possessed more forms, functions or facets than it does today. The Wristwatch Handbook is written from the epicenter of a renaissance, a place in time between the Quartz revolution and the rise of the smart device - where the mechanical wristwatch is the antidote to the microprocessor and the permanent buzz of your inbox. From the multi-axis tourbillon, to the split-second chronograph, to the sidereal sky chart, The Wristwatch Handbook covers it all and does so with more than 470 rich illustrations from over 90 of the World's leading brands.The book is separated into two sections. The first section provides the reader with a comprehensive understanding of the mechanical movement. Its chapters explore power, transmission, distribution and regulation illustrating the basic concepts before considering the innovation and complexity that takes place further toward the cutting edge. From the fifty-day power reserve, to the constant force mechanism, and the 1,000Hz mechanical escapement, section 1 will allow the reader to understand and appreciate what is happening beneath the dial of their watch. Section two allows the reader to take this understanding and apply it to the vast range of complications (functions) that exist in modern horology. Each chapter showcases a distinct category of complication. For example, the regatta timer, pulsometer, and monopusher chronograph join a host of others in a chapter entitled 'Recording Lapses of Time'; The power reserve indicator, dynamograph, and crown position indicator are featured in a chapter for 'Power and Performance Indication'; The moon phase indicator, annual calendar, and planetarium can be found in the 'Astronomical Complications' chapter. Once the functional categories are exhausted, the final three chapters explore whimsical complications that have little regard for practical function, novelty time indication, and the 'super-complicated' watch - a rare breed of timepiece that houses an intimidating host of complications featured throughout the book. Upon completion of The Wristwatch Handbook the reader will be able to identify even the most exotic complication from across the room, and be able to share their appreciation and understanding of what makes it so useful and compelling. The Wristwatch Handbook is "brand agnostic", using only those watches that most aptly illustrate the given subject-matter. As a consequence the book places equal emphasis on the classic and the cutting edge, on watches produced in large volume or exclusive runs, by industry-leading technology or at the hand of a master. In doing so the book provides an unparalleled range of watches from over 90 brands, allowing the reader to determine for themselves which brands, complications, and styles they will build their collection from.},
  isbn = {978-1-85149-829-1},
  langid = {english},
  pagetotal = {352}
}

@incollection{schonbergerPixelwiseViewSelection2016,
  title = {Pixelwise {{View Selection}} for {{Unstructured Multi-View Stereo}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2016},
  author = {Schönberger, Johannes L. and Zheng, Enliang and Frahm, Jan-Michael and Pollefeys, Marc},
  editor = {Leibe, Bastian and Matas, Jiri and Sebe, Nicu and Welling, Max},
  date = {2016},
  volume = {9907},
  pages = {501--518},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-319-46487-9_31},
  url = {http://link.springer.com/10.1007/978-3-319-46487-9_31},
  urldate = {2023-02-17},
  abstract = {This work presents a Multi-View Stereo system for robust and efficient dense modeling from unstructured image collections. Our core contributions are the joint estimation of depth and normal information, pixelwise view selection using photometric and geometric priors, and a multi-view geometric consistency term for the simultaneous refinement and image-based depth and normal fusion. Experiments on benchmarks and large-scale Internet photo collections demonstrate stateof-the-art performance in terms of accuracy, completeness, and efficiency.},
  isbn = {978-3-319-46486-2 978-3-319-46487-9},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\52Z4GJ94\Schönberger 등 - 2016 - Pixelwise View Selection for Unstructured Multi-Vi.pdf}
}

@online{schulmanProximalPolicyOptimization2017,
  title = {Proximal {{Policy Optimization Algorithms}}},
  author = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  date = {2017-08-28},
  eprint = {1707.06347},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1707.06347},
  url = {http://arxiv.org/abs/1707.06347},
  urldate = {2024-05-27},
  abstract = {We propose a new family of policy gradient methods for reinforcement learning, which alternate between sampling data through interaction with the environment, and optimizing a "surrogate" objective function using stochastic gradient ascent. Whereas standard policy gradient methods perform one gradient update per data sample, we propose a novel objective function that enables multiple epochs of minibatch updates. The new methods, which we call proximal policy optimization (PPO), have some of the benefits of trust region policy optimization (TRPO), but they are much simpler to implement, more general, and have better sample complexity (empirically). Our experiments test PPO on a collection of benchmark tasks, including simulated robotic locomotion and Atari game playing, and we show that PPO outperforms other online policy gradient methods, and overall strikes a favorable balance between sample complexity, simplicity, and wall-time.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Schulman et al_2017_Proximal Policy Optimization Algorithms.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4FFN9ZMK\\1707.html}
}

@article{schumpeterBUSINESSCYCLESTheoretical,
  title = {{{BUSINESS CYCLES}}. {{A Theoretical}}, {{Historical}} and {{Statistical Analysis}} of the {{Capitalist Process}}.},
  author = {Schumpeter, Joseph},
  langid = {english}
}

@book{schumpeterBusinessCyclesTheoretical2006,
  title = {Business {{Cycles}}: {{A Theoretical}}, {{Historical}}, and {{Statistical Analysis}} of the {{Capitalist Process}}},
  shorttitle = {Business {{Cycles}}},
  author = {Schumpeter, Joseph A.},
  date = {2006},
  eprint = {dd4eAQAAMAAJ},
  eprinttype = {googlebooks},
  publisher = {Martino Pub.},
  abstract = {Schumpeter is without doubt one of the most influential economists of the 20th century. Business Cycles [1939] is considered his great work. We reprint the first edition published in 1939 in two volumes. In "Business Cycles" Schumpeter focuses powerfully on the historical role of technological innovation in accounting for the high degree of instability in capitalists societies. He aims to analyze empirically the actual process of economic development using historical and statistical material based on the theoretical framework he developed in earlier writings. He tried to integrate theory and history primarily by means of statistics. It is because he adopted the method of filling in the statistical contours with detailed industrial history that "Business Cycles" comprises two large volumes. A Classic work, not otherwise available in the original two volume format.},
  isbn = {978-1-57898-556-2},
  langid = {english},
  pagetotal = {474}
}

@online{ScienceMapTechnological,
  title = {Science as a Map in Technological Search - {{Fleming}} - 2004 - {{Strategic Management Journal}} - {{Wiley Online Library}}},
  url = {https://onlinelibrary.wiley.com/doi/10.1002/smj.384},
  urldate = {2023-12-06}
}

@online{SeikoQuartzAstron,
  title = {Seiko {{Quartz Astron 35SQ}} | {{About}} | {{Epson}}},
  url = {https://corporate.epson/en/about/history/milestone-products/1969-12-35sq.html},
  urldate = {2023-12-26},
  abstract = {The Seiko Quartz Astron 35SQ is etched in the annals of horological history as the world's first quartz watch.},
  langid = {english}
}

@article{selvarajuGradCAMVisualExplanations2020,
  title = {Grad-{{CAM}}: {{Visual Explanations}} from {{Deep Networks}} via {{Gradient-based Localization}}},
  shorttitle = {Grad-{{CAM}}},
  author = {Selvaraju, Ramprasaath R. and Cogswell, Michael and Das, Abhishek and Vedantam, Ramakrishna and Parikh, Devi and Batra, Dhruv},
  date = {2020-02},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {128},
  number = {2},
  eprint = {1610.02391},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {336--359},
  issn = {0920-5691, 1573-1405},
  doi = {10.1007/s11263-019-01228-7},
  url = {http://arxiv.org/abs/1610.02391},
  urldate = {2023-08-05},
  abstract = {We propose a technique for producing "visual explanations" for decisions from a large class of CNN-based models, making them more transparent. Our approach - Gradient-weighted Class Activation Mapping (Grad-CAM), uses the gradients of any target concept, flowing into the final convolutional layer to produce a coarse localization map highlighting important regions in the image for predicting the concept. Grad-CAM is applicable to a wide variety of CNN model-families: (1) CNNs with fully-connected layers, (2) CNNs used for structured outputs, (3) CNNs used in tasks with multimodal inputs or reinforcement learning, without any architectural changes or re-training. We combine Grad-CAM with fine-grained visualizations to create a high-resolution class-discriminative visualization and apply it to off-the-shelf image classification, captioning, and visual question answering (VQA) models, including ResNet-based architectures. In the context of image classification models, our visualizations (a) lend insights into their failure modes, (b) are robust to adversarial images, (c) outperform previous methods on localization, (d) are more faithful to the underlying model and (e) help achieve generalization by identifying dataset bias. For captioning and VQA, we show that even non-attention based models can localize inputs. We devise a way to identify important neurons through Grad-CAM and combine it with neuron names to provide textual explanations for model decisions. Finally, we design and conduct human studies to measure if Grad-CAM helps users establish appropriate trust in predictions from models and show that Grad-CAM helps untrained users successfully discern a 'stronger' nodel from a 'weaker' one even when both make identical predictions. Our code is available at https://github.com/ramprs/grad-cam/, along with a demo at http://gradcam.cloudcv.org, and a video at youtu.be/COjUB9Izk6E.},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\understanding deep CNN\\Selvaraju et al_2020_Grad-CAM2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CWJ28D99\\1610.html}
}

@article{seoDevelopmentOperationTrajectory2022,
  title = {Development of an Operation Trajectory Design Algorithm for Control of Multiple {{0D}} Parameters Using Deep Reinforcement Learning in {{KSTAR}}},
  author = {Seo, J. and Na, Y.-S. and Kim, B. and Lee, C.Y. and Park, M.S. and Park, S.J. and Lee, Y.H.},
  date = {2022-08-01},
  journaltitle = {Nuclear Fusion},
  shortjournal = {Nucl. Fusion},
  volume = {62},
  number = {8},
  pages = {086049},
  issn = {0029-5515, 1741-4326},
  doi = {10.1088/1741-4326/ac79be},
  url = {https://iopscience.iop.org/article/10.1088/1741-4326/ac79be},
  urldate = {2024-05-08},
  abstract = {This work develops an artificially intelligent (AI) tokamak operation design algorithm that provides an adequate operation trajectory to control multiple plasma parameters simultaneously into different targets. An AI is trained with the reinforcement learning technique in the data-driven tokamak simulator, searching for the best action policy to get a higher reward. By setting the reward function to increase as the achieved βp, q95, and li are close to the given target values, the AI tries to properly determine the plasma current and boundary shape to reach the given targets. After training the AI with various targets and conditions in the simulation environment, we demonstrated that we could successfully achieve the target plasma states with the AI-designed operation trajectory in a real KSTAR experiment. The developed algorithm would replace the human task of searching for an operation setting for given objectives, provide clues for developing advanced operation scenarios, and serve as a basis for the autonomous operation of a fusion reactor.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Seo et al_2022_Development of an operation trajectory design algorithm for control of multiple.pdf}
}

@report{sezenerRapidEfficientLearning2021,
  type = {preprint},
  title = {A Rapid and Efficient Learning Rule for Biological Neural Circuits},
  author = {Sezener, Eren and Grabska-Barwińska, Agnieszka and Kostadinov, Dimitar and Beau, Maxime and Krishnagopal, Sanjukta and Budden, David and Hutter, Marcus and Veness, Joel and Botvinick, Matthew and Clopath, Claudia and Häusser, Michael and Latham, Peter E.},
  date = {2021-03-12},
  institution = {Neuroscience},
  doi = {10.1101/2021.03.10.434756},
  url = {http://biorxiv.org/lookup/doi/10.1101/2021.03.10.434756},
  urldate = {2022-08-26},
  abstract = {Abstract                        The dominant view in neuroscience is that changes in synaptic weights underlie learning. It is unclear, however, how the brain is able to determine which synapses should change, and by how much. This uncertainty stands in sharp contrast to deep learning, where changes in weights are explicitly engineered to optimize performance. However, the main tool for that, backpropagation, has two problems. One is neuro-science related: it is not biologically plausible. The other is inherent: networks trained with this rule tend to forget old tasks when learning new ones. Here we introduce the Dendritic Gated Network (DGN), a variant of the Gated Linear Network, which offers a biologically plausible alternative to backpropagation. DGNs combine dendritic ‘gating’ (whereby interneurons target dendrites to shape neuronal responses) with local learning rules to yield provably efficient performance. They are significantly more data efficient than conventional artificial networks, and are highly resistant to forgetting. Consequently, they perform well on a variety of tasks, in some cases better than backpropagation. Importantly, DGNs have structural and functional similarities to the cerebellum, a link that we strengthen by using             in vivo             two-photon calcium imaging to show that single interneurons suppress activity in individual dendritic branches of Purkinje cells, a key feature of the model. Thus, DGNs leverage targeted dendritic inhibition and local learning – two features ubiquitous in the brain – to achieve fast and efficient learning.},
  langid = {english},
  file = {Y:\paper\Computer Vision\layer\Sezener et al_2021_A rapid and efficient learning rule for biological neural circuits.pdf}
}

@inproceedings{shahADEPTAdapterbasedEfficient2023,
  title = {{{ADEPT}}: {{Adapter-based Efficient Prompt Tuning Approach}} for {{Language Models}}},
  shorttitle = {{{ADEPT}}},
  booktitle = {Proceedings of {{The Fourth Workshop}} on {{Simple}} and {{Efficient Natural Language Processing}} ({{SustaiNLP}})},
  author = {Shah, Aditya and Thapa, Surendrabikram and Jain, Aneesh and Huang, Lifu},
  date = {2023-07},
  pages = {121--128},
  publisher = {Association for Computational Linguistics},
  location = {Toronto, Canada (Hybrid)},
  doi = {10.18653/v1/2023.sustainlp-1.8},
  url = {https://aclanthology.org/2023.sustainlp-1.8},
  urldate = {2023-08-11},
  eventtitle = {Sustainlp 2023},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\prompt\Shah et al_2023_ADEPT.pdf}
}

@inproceedings{shakarianReducingGangViolence2014,
  title = {Reducing Gang Violence through Network Influence Based Targeting of Social Programs},
  booktitle = {Proceedings of the 20th {{ACM SIGKDD}} International Conference on {{Knowledge}} Discovery and Data Mining},
  author = {Shakarian, Paulo and Salmento, Joseph and Pulleyblank, William and Bertetto, John},
  year = {8월 24, 2014},
  series = {{{KDD}} '14},
  pages = {1829--1836},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/2623330.2623331},
  url = {https://doi.org/10.1145/2623330.2623331},
  urldate = {2023-05-24},
  abstract = {In this paper, we study a variant of the social network maximum influence problem and its application to intelligently approaching individual gang members with incentives to leave a gang. The goal is to identify individuals who when influenced to leave gangs will propagate this action. We study this emerging application by exploring specific facets of the problem that must be addressed when modeling this particular situation. We formulate a new influence maximization variant - the "social incentive influence" (SII) problem and study it both formally and in the context of the law-enforcement domain. Using new techniques from unconstrained submodular maximization, we develop an approximation algorithm for SII and present a suite of experimental results - including tests on real-world police data from Chicago.},
  isbn = {978-1-4503-2956-9},
  keywords = {complex networks,network diffusion,propagation in networks}
}

@article{shannonMathematicalTheoryCommunication1948,
  title = {A Mathematical Theory of Communication},
  author = {Shannon, C. E.},
  date = {1948-07},
  journaltitle = {The Bell System Technical Journal},
  volume = {27},
  number = {3},
  pages = {379--423},
  issn = {0005-8580},
  doi = {10.1002/j.1538-7305.1948.tb01338.x},
  abstract = {The recent development of various methods of modulation such as PCM and PPM which exchange bandwidth for signal-to-noise ratio has intensified the interest in a general theory of communication. A basis for such a theory is contained in the important papers of Nyquist1 and Hartley2 on this subject. In the present paper we will extend the theory to include a number of new factors, in particular the effect of noise in the channel, and the savings possible due to the statistical structure of the original message and due to the nature of the final destination of the information.},
  eventtitle = {The {{Bell System Technical Journal}}},
  file = {C\:\\Users\\jiho\\OneDrive - GIST\\바탕 화면\\resesrch\\zotero_pdfs\\personal interest\\Shannon_1948_A mathematical theory of communication_annotated.pdf;Y\:\\paper\\personal interest\\Shannon_1948_A mathematical theory of communication.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TN2GQSV9\\6773024.html}
}

@online{shaoPolarimetricInverseRendering2022,
  title = {Polarimetric {{Inverse Rendering}} for {{Transparent Shapes Reconstruction}}},
  author = {Shao, Mingqi and Xia, Chongkun and Duan, Dongxu and Wang, Xueqian},
  date = {2022-08-24},
  eprint = {2208.11836},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2208.11836},
  urldate = {2023-02-10},
  abstract = {In this work, we propose a novel method for the detailed reconstruction of transparent objects by exploiting polarimetric cues. Most of the existing methods usually lack sufficient constraints and suffer from the over-smooth problem. Hence, we introduce polarization information as a complementary cue. We implicitly represent the object's geometry as a neural network, while the polarization render is capable of rendering the object's polarization images from the given shape and illumination configuration. Direct comparison of the rendered polarization images to the real-world captured images will have additional errors due to the transmission in the transparent object. To address this issue, the concept of reflection percentage which represents the proportion of the reflection component is introduced. The reflection percentage is calculated by a ray tracer and then used for weighting the polarization loss. We build a polarization dataset for multi-view transparent shapes reconstruction to verify our method. The experimental results show that our method is capable of recovering detailed shapes and improving the reconstruction quality of transparent objects. Our dataset and code will be publicly available at https://github.com/shaomq2187/TransPIR.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Shao et al_2022_Polarimetric Inverse Rendering for Transparent Shapes Reconstruction.pdf;C\:\\Users\\chsey\\Zotero\\storage\\2XL6K9JR\\2208.html}
}

@article{shaoRegionObjectRelationAwareDense2022,
  title = {Region-{{Object Relation-Aware Dense Captioning}} via {{Transformer}}},
  author = {Shao, Zhuang and Han, Jungong and Marnerides, Demetris and Debattista, Kurt},
  date = {2022},
  journaltitle = {IEEE Transactions on Neural Networks and Learning Systems},
  pages = {1--12},
  issn = {2162-2388},
  doi = {10.1109/TNNLS.2022.3152990},
  abstract = {Dense captioning provides detailed captions of complex visual scenes. While a number of successes have been achieved in recent years, there are still two broad limitations: 1) most existing methods adopt an encoder-decoder framework, where the contextual information is sequentially encoded using long short-term memory (LSTM). However, the forget gate mechanism of LSTM makes it vulnerable when dealing with a long sequence and 2) the vast majority of prior arts consider regions of interests (RoIs) equally important, thus failing to focus on more informative regions. The consequence is that the generated captions cannot highlight important contents of the image, which does not seem natural. To overcome these limitations, in this article, we propose a novel end-to-end transformer-based dense image captioning architecture, termed the transformer-based dense captioner (TDC). TDC learns the mapping between images and their dense captions via a transformer, prioritizing more informative regions. To this end, we present a novel unit, named region-object correlation score unit (ROCSU), to measure the importance of each region, where the relationships between detected objects and the region, alongside the confidence scores of detected objects within the region, are taken into account. Extensive experimental results and ablation studies on the standard dense-captioning datasets demonstrate the superiority of the proposed method to the state-of-the-art methods.},
  eventtitle = {{{IEEE Transactions}} on {{Neural Networks}} and {{Learning Systems}}},
  keywords = {Decoding,Dense image captioning,Feature extraction,Object detection,region-object correlation score unit (ROCSU),Task analysis,Training,transformer-based dense image captioner.,Transformers,Visualization},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\dense captioning\Shao et al_2022_Region-Object Relation-Aware Dense Captioning via Transformer.pdf}
}

@online{sharifzadehImprovingVisualRelation2020,
  title = {Improving {{Visual Relation Detection}} Using {{Depth Maps}}},
  author = {Sharifzadeh, Sahand and Baharlou, Sina Moayed and Berrendorf, Max and Koner, Rajat and Tresp, Volker},
  date = {2020-10-17},
  eprint = {1905.00966},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1905.00966},
  urldate = {2023-05-21},
  abstract = {Visual relation detection methods rely on object information extracted from RGB images such as 2D bounding boxes, feature maps, and predicted class probabilities. We argue that depth maps can additionally provide valuable information on object relations, e.g. helping to detect not only spatial relations, such as standing behind, but also non-spatial relations, such as holding. In this work, we study the effect of using different object features with a focus on depth maps. To enable this study, we release a new synthetic dataset of depth maps, VG-Depth, as an extension to Visual Genome (VG). We also note that given the highly imbalanced distribution of relations in VG, typical evaluation metrics for visual relation detection cannot reveal improvements of under-represented relations. To address this problem, we propose using an additional metric, calling it Macro Recall@K, and demonstrate its remarkable performance on VG. Finally, our experiments confirm that by effective utilization of depth maps within a simple, yet competitive framework, the performance of visual relation detection can be improved by a margin of up to 8\%.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Sharifzadeh et al_2020_Improving Visual Relation Detection using Depth Maps.pdf;C\:\\Users\\chsey\\Zotero\\storage\\YHLP6Y9Y\\1905.html}
}

@online{shettyNotUsingCar2018,
  title = {Not {{Using}} the {{Car}} to {{See}} the {{Sidewalk}}: {{Quantifying}} and {{Controlling}} the {{Effects}} of {{Context}} in {{Classification}} and {{Segmentation}}},
  shorttitle = {Not {{Using}} the {{Car}} to {{See}} the {{Sidewalk}}},
  author = {Shetty, Rakshith and Schiele, Bernt and Fritz, Mario},
  date = {2018-12-17},
  eprint = {1812.06707},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1812.06707},
  url = {http://arxiv.org/abs/1812.06707},
  urldate = {2023-08-05},
  abstract = {Importance of visual context in scene understanding tasks is well recognized in the computer vision community. However, to what extent the computer vision models for image classification and semantic segmentation are dependent on the context to make their predictions is unclear. A model overly relying on context will fail when encountering objects in context distributions different from training data and hence it is important to identify these dependencies before we can deploy the models in the real-world. We propose a method to quantify the sensitivity of black-box vision models to visual context by editing images to remove selected objects and measuring the response of the target models. We apply this methodology on two tasks, image classification and semantic segmentation, and discover undesirable dependency between objects and context, for example that "sidewalk" segmentation relies heavily on "cars" being present in the image. We propose an object removal based data augmentation solution to mitigate this dependency and increase the robustness of classification and segmentation models to contextual variations. Our experiments show that the proposed data augmentation helps these models improve the performance in out-of-context scenarios, while preserving the performance on regular data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\contextual cues\\Shetty et al_2018_Not Using the Car to See the Sidewalk.pdf;C\:\\Users\\chsey\\Zotero\\storage\\U37RNQGD\\1812.html}
}

@online{shiArtificialIntelligenceSocial2020,
  title = {Artificial {{Intelligence}} for {{Social Good}}: {{A Survey}}},
  shorttitle = {Artificial {{Intelligence}} for {{Social Good}}},
  author = {Shi, Zheyuan Ryan and Wang, Claire and Fang, Fei},
  date = {2020-01-06},
  eprint = {2001.01818},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2001.01818},
  urldate = {2023-05-24},
  abstract = {Artificial intelligence for social good (AI4SG) is a research theme that aims to use and advance artificial intelligence to address societal issues and improve the well-being of the world. AI4SG has received lots of attention from the research community in the past decade with several successful applications. Building on the most comprehensive collection of the AI4SG literature to date with over 1000 contributed papers, we provide a detailed account and analysis of the work under the theme in the following ways. (1) We quantitatively analyze the distribution and trend of the AI4SG literature in terms of application domains and AI techniques used. (2) We propose three conceptual methods to systematically group the existing literature and analyze the eight AI4SG application domains in a unified framework. (3) We distill five research topics that represent the common challenges in AI4SG across various application domains. (4) We discuss five issues that, we hope, can shed light on the future development of the AI4SG research.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computers and Society},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\AI_for_social_good\\Shi et al_2020_Artificial Intelligence for Social Good.pdf;C\:\\Users\\chsey\\Zotero\\storage\\L2ITR65M\\2001.html}
}

@article{shinGeometryGuidedThreeDimensional2017,
  title = {Geometry {{Guided Three-Dimensional Propagation}} for {{Depth From Small Motion}}},
  author = {Shin, Seunghak and Im, Sunghoon and Shim, Inwook and Jeon, Hae-Gon and Kweon, In So},
  date = {2017-02},
  journaltitle = {IEEE Signal Processing Letters},
  volume = {24},
  number = {12},
  pages = {1857--1861},
  issn = {1558-2361},
  doi = {10.1109/LSP.2017.2761557},
  abstract = {In this letter, we present an accurate Depth from Small Motion approach, which reconstructs three-dimensional (3-D) depth from image sequences with extremely narrow baselines. We start with estimating sparse 3-D points and camera poses via the structure from motion method. For dense depth reconstruction, we propose a novel depth propagation using a geometric guidance term that considers not only the geometric constraint from the surface normal, but also color consistency. In addition, we propose an accurate surface normal estimation method with a multiple range search so that the normal vector can guide the direction of the depth propagation precisely. The major benefit of our depth propagation method is that it obtains detailed structures of a scene without fronto-parallel bias. We validate our method using various indoor and outdoor datasets, and both qualitative and quantitative experimental results show that our new algorithm consistently generates better 3-D depth information than the results of existing state-of-the-art methods.},
  eventtitle = {{{IEEE Signal Processing Letters}}},
  keywords = {Cameras,Depth from small motion,depth propagation,Estimation,Feature extraction,Image color analysis,Image reconstruction,surface normal estimation,Surface reconstruction,three-dimensional (3-D) reconstruction,Three-dimensional displays},
  file = {Y\:\\paper\\2022 winter intern\\Shin et al_2017_Geometry Guided Three-Dimensional Propagation for Depth From Small Motion.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7QTC6B2J\\stamp.html}
}

@online{shoeybiMegatronLMTrainingMultiBillion2020,
  title = {Megatron-{{LM}}: {{Training Multi-Billion Parameter Language Models Using Model Parallelism}}},
  shorttitle = {Megatron-{{LM}}},
  author = {Shoeybi, Mohammad and Patwary, Mostofa and Puri, Raul and LeGresley, Patrick and Casper, Jared and Catanzaro, Bryan},
  date = {2020-03-13},
  eprint = {1909.08053},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1909.08053},
  urldate = {2024-04-28},
  abstract = {Recent work in language modeling demonstrates that training large transformer models advances the state of the art in Natural Language Processing applications. However, very large models can be quite difficult to train due to memory constraints. In this work, we present our techniques for training very large transformer models and implement a simple, efficient intra-layer model parallel approach that enables training transformer models with billions of parameters. Our approach does not require a new compiler or library changes, is orthogonal and complimentary to pipeline model parallelism, and can be fully implemented with the insertion of a few communication operations in native PyTorch. We illustrate this approach by converging transformer based models up to 8.3 billion parameters using 512 GPUs. We sustain 15.1 PetaFLOPs across the entire application with 76\% scaling efficiency when compared to a strong single GPU baseline that sustains 39 TeraFLOPs, which is 30\% of peak FLOPs. To demonstrate that large language models can further advance the state of the art (SOTA), we train an 8.3 billion parameter transformer language model similar to GPT-2 and a 3.9 billion parameter model similar to BERT. We show that careful attention to the placement of layer normalization in BERT-like models is critical to achieving increased performance as the model size grows. Using the GPT-2 model we achieve SOTA results on the WikiText103 (10.8 compared to SOTA perplexity of 15.8) and LAMBADA (66.5\% compared to SOTA accuracy of 63.2\%) datasets. Our BERT model achieves SOTA results on the RACE dataset (90.9\% compared to SOTA accuracy of 89.4\%).},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y:\paper\2024_research\Shoeybi et al_2020_Megatron-LM.pdf}
}

@inproceedings{shottonTextonBoostJointAppearance2006,
  title = {{{TextonBoost}}: {{Joint Appearance}}, {{Shape}} and {{Context Modeling}} for {{Multi-class Object Recognition}} and {{Segmentation}}},
  shorttitle = {{{TextonBoost}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2006},
  author = {Shotton, Jamie and Winn, John and Rother, Carsten and Criminisi, Antonio},
  editor = {Leonardis, Aleš and Bischof, Horst and Pinz, Axel},
  date = {2006},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {1--15},
  publisher = {Springer},
  location = {Berlin, Heidelberg},
  doi = {10.1007/11744023_1},
  abstract = {This paper proposes a new approach to learning a discriminative model of object classes, incorporating appearance, shape and context information efficiently. The learned model is used for automatic visual recognition and semantic segmentation of photographs. Our discriminative model exploits novel features, based on textons, which jointly model shape and texture. Unary classification and feature selection is achieved using shared boosting to give an efficient classifier which can be applied to a large number of classes. Accurate image segmentation is achieved by incorporating these classifiers in a conditional random field. Efficient training of the model on very large datasets is achieved by exploiting both random feature selection and piecewise training methods.},
  isbn = {978-3-540-33833-8},
  langid = {english},
  keywords = {Class Label,Conditional Random Field,Context Modeling,Object Class,Training Image},
  file = {Y:\paper\2023 graduation\Shotton et al_2006_TextonBoost.pdf}
}

@online{shrivastavaTrainingRegionbasedObject2016,
  title = {Training {{Region-based Object Detectors}} with {{Online Hard Example Mining}}},
  author = {Shrivastava, Abhinav and Gupta, Abhinav and Girshick, Ross},
  date = {2016-04-12},
  eprint = {1604.03540},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1604.03540},
  url = {http://arxiv.org/abs/1604.03540},
  urldate = {2023-08-05},
  abstract = {The field of object detection has made significant advances riding on the wave of region-based ConvNets, but their training procedure still includes many heuristics and hyperparameters that are costly to tune. We present a simple yet surprisingly effective online hard example mining (OHEM) algorithm for training region-based ConvNet detectors. Our motivation is the same as it has always been -- detection datasets contain an overwhelming number of easy examples and a small number of hard examples. Automatic selection of these hard examples can make training more effective and efficient. OHEM is a simple and intuitive algorithm that eliminates several heuristics and hyperparameters in common use. But more importantly, it yields consistent and significant boosts in detection performance on benchmarks like PASCAL VOC 2007 and 2012. Its effectiveness increases as datasets become larger and more difficult, as demonstrated by the results on the MS COCO dataset. Moreover, combined with complementary advances in the field, OHEM leads to state-of-the-art results of 78.9\% and 76.3\% mAP on PASCAL VOC 2007 and 2012 respectively.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\object detection\\Shrivastava et al_2016_Training Region-based Object Detectors with Online Hard Example Mining.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GUYRLVKR\\1604.html}
}

@inproceedings{shtedritskiWhatDoesCLIP2023,
  title = {What Does {{CLIP}} Know about a Red Circle? {{Visual}} Prompt Engineering for {{VLMs}}},
  shorttitle = {What Does {{CLIP}} Know about a Red Circle?},
  author = {Shtedritski, Aleksandar and Rupprecht, Christian and Vedaldi, Andrea},
  date = {2023},
  pages = {11987--11997},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Shtedritski_What_does_CLIP_know_about_a_red_circle_Visual_prompt_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Shtedritski et al_2023_What does CLIP know about a red circle.pdf}
}

@online{shuTestTimePromptTuning2022,
  title = {Test-{{Time Prompt Tuning}} for {{Zero-Shot Generalization}} in {{Vision-Language Models}}},
  author = {Shu, Manli and Nie, Weili and Huang, De-An and Yu, Zhiding and Goldstein, Tom and Anandkumar, Anima and Xiao, Chaowei},
  date = {2022-09-15},
  eprint = {2209.07511},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2209.07511},
  urldate = {2024-09-10},
  abstract = {Pre-trained vision-language models (e.g., CLIP) have shown promising zero-shot generalization in many downstream tasks with properly designed text prompts. Instead of relying on hand-engineered prompts, recent works learn prompts using the training data from downstream tasks. While effective, training on domainspecific data reduces a model’s generalization capability to unseen new domains. In this work, we propose test-time prompt tuning (TPT), a method that can learn adaptive prompts on the fly with a single test sample. For image classification, TPT optimizes the prompt by minimizing the entropy with confidence selection so that the model has consistent predictions across different augmented views of each test sample. In evaluating generalization to natural distribution shifts, TPT improves the zero-shot top-1 accuracy of CLIP by 3.6\% on average, surpassing previous prompt tuning approaches that require additional task-specific training data. In evaluating cross-dataset generalization with unseen categories, TPT performs on par with the state-of-the-art approaches that use additional training data. Project page: https://azshue.github.io/TPT/.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\4IFFZSJW\Shu 등 - 2022 - Test-Time Prompt Tuning for Zero-Shot Generalizati.pdf}
}

@incollection{sidorovTextCapsDatasetImage2020,
  title = {{{TextCaps}}: {{A Dataset}} for {{Image Captioning}} with {{Reading Comprehension}}},
  shorttitle = {{{TextCaps}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Sidorov, Oleksii and Hu, Ronghang and Rohrbach, Marcus and Singh, Amanpreet},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  volume = {12347},
  pages = {742--758},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58536-5_44},
  url = {https://link.springer.com/10.1007/978-3-030-58536-5_44},
  urldate = {2023-05-28},
  abstract = {Image descriptions can help visually impaired people to quickly understand the image content. While we made significant progress in automatically describing images and optical character recognition, current approaches are unable to include written text in their descriptions, although text is omnipresent in human environments and frequently critical to understand our surroundings. To study how to comprehend text in the context of an image we collect a novel dataset, TextCaps, with 145k captions for 28k images. Our dataset challenges a model to recognize text, relate it to its visual context, and decide what part of the text to copy or paraphrase, requiring spatial, semantic, and visual reasoning between multiple text tokens and visual entities, such as objects. We study baselines and adapt existing approaches to this new task, which we refer to as image captioning with reading comprehension. Our analysis with automatic and human studies shows that our new TextCaps dataset provides many new technical challenges over previous datasets.},
  isbn = {978-3-030-58535-8 978-3-030-58536-5},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Sidorov et al_2020_TextCaps.pdf}
}

@online{SIGGRAPH2015Course,
  title = {{{SIGGRAPH}} 2015 {{Course}}: {{Physically Based Shading}} in {{Theory}} and {{Practice}}},
  url = {https://blog.selfshadow.com/publications/s2015-shading-course/#course_content},
  urldate = {2023-04-11},
  file = {C:\Users\chsey\Zotero\storage\IFV88ZAY\s2015-shading-course.html}
}

@book{silberschatzDatabaseSystemConcepts2020,
  title = {Database System Concepts},
  author = {Silberschatz, Abraham and Korth, Henry F. and Sudarshan, S.},
  date = {2020},
  edition = {Seventh edition},
  publisher = {McGraw-Hill},
  location = {New York, NY},
  isbn = {978-0-07-802215-9 978-1-260-51504-6},
  langid = {english},
  pagetotal = {1344},
  keywords = {Database management},
  file = {C:\Users\chsey\Zotero\storage\ZJ67G6SG\Silberschatz et al_2020_Database system concepts.pdf}
}

@online{simonyanTwoStreamConvolutionalNetworks2014,
  title = {Two-{{Stream Convolutional Networks}} for {{Action Recognition}} in {{Videos}}},
  author = {Simonyan, Karen and Zisserman, Andrew},
  date = {2014-11-12},
  eprint = {1406.2199},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1406.2199},
  url = {http://arxiv.org/abs/1406.2199},
  urldate = {2023-08-05},
  abstract = {We investigate architectures of discriminatively trained deep Convolutional Networks (ConvNets) for action recognition in video. The challenge is to capture the complementary information on appearance from still frames and motion between frames. We also aim to generalise the best performing hand-crafted features within a data-driven learning framework. Our contribution is three-fold. First, we propose a two-stream ConvNet architecture which incorporates spatial and temporal networks. Second, we demonstrate that a ConvNet trained on multi-frame dense optical flow is able to achieve very good performance in spite of limited training data. Finally, we show that multi-task learning, applied to two different action classification datasets, can be used to increase the amount of training data and improve the performance on both. Our architecture is trained and evaluated on the standard video actions benchmarks of UCF-101 and HMDB-51, where it is competitive with the state of the art. It also exceeds by a large margin previous attempts to use deep nets for video classification.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Simonyan_Zisserman_2014_Two-Stream Convolutional Networks for Action Recognition in Videos.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8R3IT5ZH\\1406.html}
}

@online{simonyanVeryDeepConvolutional2015,
  title = {Very {{Deep Convolutional Networks}} for {{Large-Scale Image Recognition}}},
  author = {Simonyan, Karen and Zisserman, Andrew},
  date = {2015-04-10},
  eprint = {1409.1556},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1409.1556},
  url = {http://arxiv.org/abs/1409.1556},
  urldate = {2023-08-05},
  abstract = {In this work we investigate the effect of the convolutional network depth on its accuracy in the large-scale image recognition setting. Our main contribution is a thorough evaluation of networks of increasing depth using an architecture with very small (3x3) convolution filters, which shows that a significant improvement on the prior-art configurations can be achieved by pushing the depth to 16-19 weight layers. These findings were the basis of our ImageNet Challenge 2014 submission, where our team secured the first and the second places in the localisation and classification tracks respectively. We also show that our representations generalise well to other datasets, where they achieve state-of-the-art results. We have made our two best-performing ConvNet models publicly available to facilitate further research on the use of deep visual representations in computer vision.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\image classification\\Simonyan_Zisserman_2015_Very Deep Convolutional Networks for Large-Scale Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Y9ACZBNP\\1409.html}
}

@online{simonyanVGGVeryDeep2015,
  title = {{{VGG}}: {{Very Deep Convolutional Networks}} for {{Large-Scale Image Recognition}}},
  author = {Simonyan, Karen and Zisserman, Andrew},
  date = {2015-04-10},
  eprint = {1409.1556},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1409.1556},
  urldate = {2022-08-09},
  abstract = {In this work we investigate the effect of the convolutional network depth on its accuracy in the large-scale image recognition setting. Our main contribution is a thorough evaluation of networks of increasing depth using an architecture with very small (3x3) convolution filters, which shows that a significant improvement on the prior-art configurations can be achieved by pushing the depth to 16-19 weight layers. These findings were the basis of our ImageNet Challenge 2014 submission, where our team secured the first and the second places in the localisation and classification tracks respectively. We also show that our representations generalise well to other datasets, where they achieve state-of-the-art results. We have made our two best-performing ConvNet models publicly available to facilitate further research on the use of deep visual representations in computer vision.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Simonyan_Zisserman_2015_VGG.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8RBH9B7U\\1409.html}
}

@online{singhEffectivenessMAEPrepretraining2023,
  title = {The Effectiveness of {{MAE}} Pre-Pretraining for Billion-Scale Pretraining},
  author = {Singh, Mannat and Duval, Quentin and Alwala, Kalyan Vasudev and Fan, Haoqi and Aggarwal, Vaibhav and Adcock, Aaron and Joulin, Armand and Dollár, Piotr and Feichtenhofer, Christoph and Girshick, Ross and Girdhar, Rohit and Misra, Ishan},
  date = {2023-03-23},
  eprint = {2303.13496},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2303.13496},
  urldate = {2023-08-28},
  abstract = {This paper revisits the standard pretrain-then-finetune paradigm used in computer vision for visual recognition tasks. Typically, state-of-the-art foundation models are pretrained using large scale (weakly) supervised datasets with billions of images. We introduce an additional pre-pretraining stage that is simple and uses the self-supervised MAE technique to initialize the model. While MAE has only been shown to scale with the size of models, we find that it scales with the size of the training dataset as well. Thus, our MAE-based pre-pretraining scales with both model and data size making it applicable for training foundation models. Pre-pretraining consistently improves both the model convergence and the downstream transfer performance across a range of model scales (millions to billions of parameters), and dataset sizes (millions to billions of images). We measure the effectiveness of pre-pretraining on 10 different visual recognition tasks spanning image classification, video recognition, object detection, low-shot classification and zero-shot recognition. Our largest model achieves new state-of-the-art results on iNaturalist-18 (91.3\%), 1-shot ImageNet-1k (62.1\%), and zero-shot transfer on Food-101 (96.0\%). Our study reveals that model initialization plays a significant role, even for web-scale pretraining with billions of images.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Singh et al_2023_The effectiveness of MAE pre-pretraining for billion-scale pretraining.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4SKB2FBP\\2303.html}
}

@inproceedings{singhFLAVAFoundationalLanguage2022,
  title = {{{FLAVA}}: {{A Foundational Language And Vision Alignment Model}}},
  shorttitle = {{{FLAVA}}},
  booktitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Singh, Amanpreet and Hu, Ronghang and Goswami, Vedanuj and Couairon, Guillaume and Galuba, Wojciech and Rohrbach, Marcus and Kiela, Douwe},
  date = {2022-06},
  pages = {15617--15629},
  publisher = {IEEE},
  location = {New Orleans, LA, USA},
  doi = {10.1109/CVPR52688.2022.01519},
  url = {https://ieeexplore.ieee.org/document/9880206/},
  urldate = {2024-02-02},
  abstract = {State-of-the-art vision and vision-and-language models rely on large-scale visio-linguistic pretraining for obtaining good performance on a variety of downstream tasks. Generally, such models are often either cross-modal (contrastive) or multi-modal (with earlier fusion) but not both; and they often only target specific modalities or tasks. A promising direction would be to use a single holistic universal model, as a “foundation”, that targets all modalities at once—a true vision and language foundation model should be good at vision tasks, language tasks, and cross- and multi-modal vision and language tasks. We introduce FLAVA as such a model and demonstrate impressive performance on a wide range of 35 tasks spanning these target modalities.},
  eventtitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-66546-946-3},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Singh et al_2022_FLAVA.pdf}
}

@online{singhFLAVAFoundationalLanguage2022a,
  title = {{{FLAVA}}: {{A Foundational Language And Vision Alignment Model}}},
  shorttitle = {{{FLAVA}}},
  author = {Singh, Amanpreet and Hu, Ronghang and Goswami, Vedanuj and Couairon, Guillaume and Galuba, Wojciech and Rohrbach, Marcus and Kiela, Douwe},
  date = {2022-03-29},
  eprint = {2112.04482},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.04482},
  urldate = {2024-04-15},
  abstract = {State-of-the-art vision and vision-and-language models rely on large-scale visio-linguistic pretraining for obtaining good performance on a variety of downstream tasks. Generally, such models are often either cross-modal (contrastive) or multi-modal (with earlier fusion) but not both; and they often only target specific modalities or tasks. A promising direction would be to use a single holistic universal model, as a "foundation", that targets all modalities at once -- a true vision and language foundation model should be good at vision tasks, language tasks, and cross- and multi-modal vision and language tasks. We introduce FLAVA as such a model and demonstrate impressive performance on a wide range of 35 tasks spanning these target modalities.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Singh et al_2022_FLAVA2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KG7HZBTE\\2112.html}
}

@online{SingleImageSuperResolutionBenchmark,
  title = {Single-{{Image Super-Resolution}}: {{A Benchmark}} | {{SpringerLink}}},
  url = {https://link.springer.com/chapter/10.1007/978-3-319-10593-2_25},
  urldate = {2022-09-26},
  file = {C:\Users\chsey\Zotero\storage\YGE6V6W8\978-3-319-10593-2_25.html}
}

@online{snellPrototypicalNetworksFewshot2017,
  title = {Prototypical {{Networks}} for {{Few-shot Learning}}},
  author = {Snell, Jake and Swersky, Kevin and Zemel, Richard S.},
  date = {2017-06-19},
  eprint = {1703.05175},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1703.05175},
  url = {http://arxiv.org/abs/1703.05175},
  urldate = {2023-08-05},
  abstract = {We propose prototypical networks for the problem of few-shot classification, where a classifier must generalize to new classes not seen in the training set, given only a small number of examples of each new class. Prototypical networks learn a metric space in which classification can be performed by computing distances to prototype representations of each class. Compared to recent approaches for few-shot learning, they reflect a simpler inductive bias that is beneficial in this limited-data regime, and achieve excellent results. We provide an analysis showing that some simple design decisions can yield substantial improvements over recent approaches involving complicated architectural choices and meta-learning. We further extend prototypical networks to zero-shot learning and achieve state-of-the-art results on the CU-Birds dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\few shot learning\\Snell et al_2017_Prototypical Networks for Few-shot Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UU4QBWRR\\1703.html}
}

@article{songDynamicCapabilitiesSamsung2016,
  title = {Dynamic {{Capabilities}} at {{Samsung}}: {{Optimizing Internal Co-Opetition}}},
  author = {Song, Jaeyong and Lee, Kyungmook and Khanna, Tarun},
  date = {2016},
  journaltitle = {California Management Review},
  volume = {58},
  number = {4},
  pages = {118--140},
  doi = {10.1525/cmr.2016.58.4.118}
}

@article{soodDeepReinforcementLearning,
  title = {Deep {{Reinforcement Learning}} for {{Optimal Portfolio Allocation}}: {{A Comparative Study}} with {{Mean-Variance Optimization}}},
  author = {Sood, Srijan and Papasotiriou, Kassiani and Vaiciulis, Marius and Balch, Tucker},
  abstract = {Portfolio Management is the process of overseeing a group of investments, referred to as a portfolio, with the objective of achieving predetermined investment goals and objectives. Portfolio Optimization is a key component that involves allocating the portfolio assets so as to maximize returns while minimizing risk taken. Portfolio optimization is typically carried out by financial professionals who use a combination of quantitative techniques and investment expertise to make decisions about the portfolio allocation.},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\ZATARBEU\Sood 등 - Deep Reinforcement Learning for Optimal Portfolio .pdf}
}

@inproceedings{srinivasanNeRVNeuralReflectance2021,
  title = {{{NeRV}}: {{Neural Reflectance}} and {{Visibility Fields}} for {{Relighting}} and {{View Synthesis}}},
  shorttitle = {{{NeRV}}},
  booktitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Srinivasan, Pratul P. and Deng, Boyang and Zhang, Xiuming and Tancik, Matthew and Mildenhall, Ben and Barron, Jonathan T.},
  date = {2021-06},
  pages = {7491--7500},
  publisher = {IEEE},
  location = {Nashville, TN, USA},
  doi = {10.1109/CVPR46437.2021.00741},
  url = {https://ieeexplore.ieee.org/document/9578828/},
  urldate = {2023-04-08},
  abstract = {We present a method that takes as input a set of images of a scene illuminated by unconstrained known lighting, and produces as output a 3D representation that can be rendered from novel viewpoints under arbitrary lighting conditions. Our method represents the scene as a continuous volumetric function parameterized as MLPs whose inputs are a 3D location and whose outputs are the following scene properties at that input location: volume density, surface normal, material parameters, distance to the first surface intersection in any direction, and visibility of the external environment in any direction. Together, these allow us to render novel views of the object under arbitrary lighting, including indirect illumination effects. The predicted visibility and surface intersection fields are critical to our model’s ability to simulate direct and indirect illumination during training, because the brute-force techniques used by prior work are intractable for lighting conditions outside of controlled setups with a single light. Our method outperforms alternative approaches for recovering relightable 3D scene representations, and performs well in complex lighting settings that have posed a significant challenge to prior work.},
  eventtitle = {2021 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-66544-509-2},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\SHSAWVKT\Srinivasan_NeRV_Neural_Reflectance_and_Visibility_Fields_for_Relighting_and_View_CVPR_2021_paper.pdf}
}

@online{staffOndemandCRMLeadership2015,
  title = {On-Demand {{CRM}} Leadership Is Polarising, Study Finds},
  author = {Staff, Wise Marketer},
  date = {2015-05-01T15:00:00+00:00},
  url = {https://thewisemarketer.com/on-demand-crm-leadership-is-polarising-study-finds-4-2/},
  urldate = {2024-01-01},
  abstract = {On-demand CRM leadership is polarising, study finds The appeal for on-demand CRM applications was strong in 2004, generating some US\$300 million in revenue. But IDC has found a particularly high revenue concentration among a very few vendors, with the top five vendors accounting for 81.6\% of the total market. The new IDC report, 'Worldwide On-demand},
  langid = {american},
  organization = {The Wise Marketer}
}

@online{standleyWhichTasksShould2020,
  title = {Which {{Tasks Should Be Learned Together}} in {{Multi-task Learning}}?},
  author = {Standley, Trevor and Zamir, Amir R. and Chen, Dawn and Guibas, Leonidas and Malik, Jitendra and Savarese, Silvio},
  date = {2020-09-02},
  eprint = {1905.07553},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1905.07553},
  url = {http://arxiv.org/abs/1905.07553},
  urldate = {2023-11-21},
  abstract = {Many computer vision applications require solving multiple tasks in real-time. A neural network can be trained to solve multiple tasks simultaneously using multi-task learning. This can save computation at inference time as only a single network needs to be evaluated. Unfortunately, this often leads to inferior overall performance as task objectives can compete, which consequently poses the question: which tasks should and should not be learned together in one network when employing multi-task learning? We study task cooperation and competition in several different learning settings and propose a framework for assigning tasks to a few neural networks such that cooperating tasks are computed by the same neural network, while competing tasks are computed by different networks. Our framework offers a time-accuracy trade-off and can produce better accuracy using less inference time than not only a single large multi-task neural network but also many single-task networks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Standley et al_2020_Which Tasks Should Be Learned Together in Multi-task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TYSQZCNQ\\1905.html}
}

@article{stefaniniShowTellSurvey2023,
  title = {From {{Show}} to {{Tell}}: {{A Survey}} on {{Deep Learning-Based Image Captioning}}},
  shorttitle = {From {{Show}} to {{Tell}}},
  author = {Stefanini, Matteo and Cornia, Marcella and Baraldi, Lorenzo and Cascianelli, Silvia and Fiameni, Giuseppe and Cucchiara, Rita},
  date = {2023-01},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {45},
  number = {1},
  pages = {539--559},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2022.3148210},
  abstract = {Connecting Vision and Language plays an essential role in Generative Intelligence. For this reason, large research efforts have been devoted to image captioning, i.e. describing images with syntactically and semantically meaningful sentences. Starting from 2015 the task has generally been addressed with pipelines composed of a visual encoder and a language model for text generation. During these years, both components have evolved considerably through the exploitation of object regions, attributes, the introduction of multi-modal connections, fully-attentive approaches, and BERT-like early-fusion strategies. However, regardless of the impressive results, research in image captioning has not reached a conclusive answer yet. This work aims at providing a comprehensive overview of image captioning approaches, from visual encoding and text generation to training strategies, datasets, and evaluation metrics. In this respect, we quantitatively compare many relevant state-of-the-art approaches to identify the most impactful technical innovations in architectures and training strategies. Moreover, many variants of the problem and its open challenges are discussed. The final goal of this work is to serve as a tool for understanding the existing literature and highlighting the future directions for a research area where Computer Vision and Natural Language Processing can find an optimal synergy.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  keywords = {Additives,Convolutional neural networks,deep learning,Feature extraction,Image captioning,Image coding,survey,Task analysis,Training,vision-and-language,Visualization},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\image captioning\\Stefanini et al_2023_From Show to Tell.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9SZDPXG8\\9706348.html}
}

@article{steingardApplyingAISocial2023,
  title = {Applying {{AI}} for Social Good: {{Aligning}} Academic Journal Ratings with the {{United Nations Sustainable Development Goals}} ({{SDGs}})},
  shorttitle = {Applying {{AI}} for Social Good},
  author = {Steingard, David and Balduccini, Marcello and Sinha, Akanksha},
  date = {2023-04-01},
  journaltitle = {AI \& SOCIETY},
  shortjournal = {AI \& Soc},
  volume = {38},
  number = {2},
  pages = {613--629},
  issn = {1435-5655},
  doi = {10.1007/s00146-022-01459-2},
  url = {https://doi.org/10.1007/s00146-022-01459-2},
  urldate = {2023-05-24},
  abstract = {This paper offers three contributions to the burgeoning movements of AI for Social Good (AI4SG) and AI and the United Nations Sustainable Development Goals (SDGs). First, we introduce the SDG-Intense Evaluation framework (SDGIE) that aims to situate variegated automated/AI models in a larger ecosystem of computational approaches to advance the SDGs. To foster knowledge collaboration for solving complex social and environmental problems encompassed by the SDGs, the SDGIE framework details a benchmark structure of data-algorithm-output to effectively standardize AI approaches to the SDGs. Second, as a specific instantiation of the SDGIE framework, the SDG Impact Intensity Model (SDGIIM) is theoretically and operationally established. SDGIIM embeds expert decision-making and SDG keyword banks in textual data processing to determine overall SDG “impact intensity.” Ideally, SDGIIM can be applied to textual data sets from any sector or discipline: academia, business, government, non-profit, civil society, etc. Third, the SDGIIM instantiation is applied to the specific domain of academic journal rating systems as a case study. Traditionally, academic journals have been evaluated on loosely conceived and empirically shaky notions of ‘quality.’ Aligned with the trend of AI4SG and broader calls to action, ‘impact’ is rapidly becoming the primary normative consideration for assessing academic journals. We hypothesize and demonstrate that SDGIIM is capable of producing evaluations aligned with experts’ expectations of SDG impact intensity; the consistent analysis and rating of textual data sets that embody the SDGs with varying degrees of meaning and, ultimately, promote positive impact on the actual material conditions of the world.},
  langid = {english},
  keywords = {AI for social good (AI4SG),Computational sustainability,Journal ratings,SDG impact intensity,Sustainable AI,Sustainable development goals},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Steingard et al_2023_Applying AI for social good.pdf}
}

@online{stoicaZipItMergingModels2024,
  title = {{{ZipIt}}! {{Merging Models}} from {{Different Tasks}} without {{Training}}},
  author = {Stoica, George and Bolya, Daniel and Bjorner, Jakob and Ramesh, Pratik and Hearn, Taylor and Hoffman, Judy},
  date = {2024-03-12},
  eprint = {2305.03053},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2305.03053},
  urldate = {2024-09-11},
  abstract = {Typical deep visual recognition models are capable of performing the one task they were trained on. In this paper, we tackle the extremely difficult problem of combining distinct models with different initializations, each solving a separate task, into one multi-task model without any additional training. Prior work in model merging permutes one model to the space of the other then averages them together. While this works for models trained on the same task, we find that this fails to account for the differences in models trained on disjoint tasks. Thus, we introduce “ZipIt!”, a general method for merging two arbitrary models of the same architecture that incorporates two simple strategies. First, in order to account for features that aren’t shared between models, we expand the model merging problem to allow for merging features within each model by defining a general “zip” operation. Second, we add support for partially zipping the models up until a specified layer, naturally creating a multi-head model. We find that these two changes combined account for 20-60\% improvement over prior work, making it more feasible to merge models trained on disjoint tasks without retraining.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\9C8DLTNR\Stoica 등 - 2024 - ZipIt! Merging Models from Different Tasks without.pdf}
}

@article{stollText2SignSignLanguage2020,
  title = {{{Text2Sign}}: {{Towards Sign Language Production Using Neural Machine Translation}} and {{Generative Adversarial Networks}}},
  shorttitle = {{{Text2Sign}}},
  author = {Stoll, Stephanie and Camgoz, Necati Cihan and Hadfield, Simon and Bowden, Richard},
  date = {2020-04-01},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {128},
  number = {4},
  pages = {891--908},
  issn = {1573-1405},
  doi = {10.1007/s11263-019-01281-2},
  url = {https://doi.org/10.1007/s11263-019-01281-2},
  urldate = {2023-05-02},
  abstract = {We present a novel approach to automatic Sign Language Production using recent developments in Neural Machine Translation (NMT), Generative Adversarial Networks, and motion generation. Our system is capable of producing sign videos from spoken language sentences. Contrary to current approaches that are dependent on heavily annotated data, our approach requires minimal gloss and skeletal level annotations for training. We achieve this by breaking down the task into dedicated sub-processes. We first translate spoken language sentences into sign pose sequences by combining an NMT network with a Motion Graph. The resulting pose information is then used to condition a generative model that produces photo realistic sign language video sequences. This is the first approach to continuous sign video generation that does not use a classical graphical avatar. We evaluate the translation abilities of our approach on the PHOENIX14T Sign Language Translation dataset. We set a baseline for text-to-gloss translation, reporting a BLEU-4 score of 16.34/15.26 on dev/test sets. We further demonstrate the video generation capabilities of our approach for both multi-signer and high-definition settings qualitatively and quantitatively using broadcast quality assessment metrics.},
  langid = {english},
  keywords = {Generative adversarial networks,Neural machine translation,Sign language production},
  file = {Y:\paper\2023_PBL\Stoll et al_2020_Text2Sign.pdf}
}

@inproceedings{stollThereBackAgain2022,
  title = {There and {{Back Again}}: {{3D Sign Language Generation}} from {{Text Using Back-Translation}}},
  shorttitle = {There and {{Back Again}}},
  booktitle = {2022 {{International Conference}} on {{3D Vision}} ({{3DV}})},
  author = {Stoll, Stephanie and Mustafa, Armin and Guillemaut, Jean-Yves},
  date = {2022-09},
  pages = {187--196},
  issn = {2475-7888},
  doi = {10.1109/3DV57658.2022.00031},
  abstract = {We introduce the first method to automatically generate 3D mesh sequences from text, inspired by the challenging problem of Sign Language Production (SLP). The approach only requires simple 2D annotations for training, which can be automatically extracted from video. Rather than incorporating high-definition or motion capture data, we propose back-translation as a powerful paradigm for supervision: By first addressing the arguably simpler problem of translating 2D pose sequences to text, we can leverage this to drive a transformer-based architecture to translate text to 2D poses. These are then used to drive a 3D mesh generator. Our mesh generator Pose2Mesh uses temporal information, to enforce temporal coherence and significantly reduce processing time. The approach is evaluated by generating 2D pose, and 3D mesh sequences in DGS (German Sign Language) from German language sentences. An extensive analysis of the approach and its sub-networks is conducted, reporting BLEU and ROUGE scores, as well as Mean 2D Joint Distance. Our proposed Text2Pose model outperforms the current state-of-the-art in SLP, and we establish the first benchmark for the complex task of text-to-3D-mesh-sequence generation with our Text2Mesh model.},
  eventtitle = {2022 {{International Conference}} on {{3D Vision}} ({{3DV}})},
  keywords = {Assistive technologies,Body Model,Coherence,Gesture recognition,Natural Language Processing,Production,Sign Language Production,Three-dimensional displays,Training,Transformers},
  file = {Y\:\\paper\\2023_PBL\\Stoll et al_2022_There and Back Again.pdf;C\:\\Users\\chsey\\Zotero\\storage\\59ZT6ISP\\stamp.html}
}

@online{StreetViewHouse,
  title = {The {{Street View House Numbers}} ({{SVHN}}) {{Dataset}}},
  url = {http://ufldl.stanford.edu/housenumbers/},
  urldate = {2022-11-15},
  file = {C:\Users\chsey\Zotero\storage\5CBVTWBJ\housenumbers.html}
}

@online{strezoskiLearningTaskRelatedness2019,
  title = {Learning {{Task Relatedness}} in {{Multi-Task Learning}} for {{Images}} in {{Context}}},
  author = {Strezoski, Gjorgji and family=Noord, given=Nanne, prefix=van, useprefix=true and Worring, Marcel},
  date = {2019-04-05},
  eprint = {1904.03011},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1904.03011},
  urldate = {2023-05-26},
  abstract = {Multimedia applications often require concurrent solutions to multiple tasks. These tasks hold clues to each-others solutions, however as these relations can be complex this remains a rarely utilized property. When task relations are explicitly defined based on domain knowledge multi-task learning (MTL) offers such concurrent solutions, while exploiting relatedness between multiple tasks performed over the same dataset. In most cases however, this relatedness is not explicitly defined and the domain expert knowledge that defines it is not available. To address this issue, we introduce Selective Sharing, a method that learns the inter-task relatedness from secondary latent features while the model trains. Using this insight, we can automatically group tasks and allow them to share knowledge in a mutually beneficial way. We support our method with experiments on 5 datasets in classification, regression, and ranking tasks and compare to strong baselines and state-of-the-art approaches showing a consistent improvement in terms of accuracy and parameter counts. In addition, we perform an activation region analysis showing how Selective Sharing affects the learned representation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\AI_for_social_good\\Strezoski et al_2019_Learning Task Relatedness in Multi-Task Learning for Images in Context.pdf;C\:\\Users\\chsey\\Zotero\\storage\\B4SB8RGU\\1904.html}
}

@online{sunAutoregressiveModelBeats2024,
  title = {Autoregressive {{Model Beats Diffusion}}: {{Llama}} for {{Scalable Image Generation}}},
  shorttitle = {Autoregressive {{Model Beats Diffusion}}},
  author = {Sun, Peize and Jiang, Yi and Chen, Shoufa and Zhang, Shilong and Peng, Bingyue and Luo, Ping and Yuan, Zehuan},
  date = {2024-06-10},
  eprint = {2406.06525},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2406.06525},
  urldate = {2024-06-11},
  abstract = {We introduce LlamaGen, a new family of image generation models that apply original “next-token prediction” paradigm of large language models to visual generation domain. It is an affirmative answer to whether vanilla autoregressive models, e.g., Llama, without inductive biases on visual signals can achieve state-of-the-art image generation performance if scaling properly. We reexamine design spaces of image tokenizers, scalability properties of image generation models, and their training data quality. The outcome of this exploration consists of: (1) An image tokenizer with downsample ratio of 16, reconstruction quality of 0.94 rFID and codebook usage of 97\% on ImageNet benchmark. (2) A series of class-conditional image generation models ranging from 111M to 3.1B parameters, achieving 2.18 FID on ImageNet 256×256 benchmarks, outperforming the popular diffusion models such as LDM, DiT. (3) A text-conditional image generation model with 775M parameters, from two-stage training on LAION-COCO and high aesthetics quality images, demonstrating competitive performance of visual quality and text alignment. (4) We verify the effectiveness of LLM serving frameworks in optimizing the inference speed of image generation models and achieve 326\% - 414\% speedup. We release all models and codes to facilitate open-source community of visual generation and multimodal foundation models.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\BS6AYQLN\Sun 등 - 2024 - Autoregressive Model Beats Diffusion Llama for Sc.pdf}
}

@online{sunDirectVoxelGrid2022,
  title = {Direct {{Voxel Grid Optimization}}: {{Super-fast Convergence}} for {{Radiance Fields Reconstruction}}},
  shorttitle = {Direct {{Voxel Grid Optimization}}},
  author = {Sun, Cheng and Sun, Min and Chen, Hwann-Tzong},
  date = {2022-06-03},
  eprint = {2111.11215},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.11215},
  url = {http://arxiv.org/abs/2111.11215},
  urldate = {2023-04-09},
  abstract = {We present a super-fast convergence approach to reconstructing the per-scene radiance field from a set of images that capture the scene with known poses. This task, which is often applied to novel view synthesis, is recently revolutionized by Neural Radiance Field (NeRF) for its state-of-the-art quality and flexibility. However, NeRF and its variants require a lengthy training time ranging from hours to days for a single scene. In contrast, our approach achieves NeRF-comparable quality and converges rapidly from scratch in less than 15 minutes with a single GPU. We adopt a representation consisting of a density voxel grid for scene geometry and a feature voxel grid with a shallow network for complex view-dependent appearance. Modeling with explicit and discretized volume representations is not new, but we propose two simple yet non-trivial techniques that contribute to fast convergence speed and high-quality output. First, we introduce the post-activation interpolation on voxel density, which is capable of producing sharp surfaces in lower grid resolution. Second, direct voxel density optimization is prone to suboptimal geometry solutions, so we robustify the optimization process by imposing several priors. Finally, evaluation on five inward-facing benchmarks shows that our method matches, if not surpasses, NeRF's quality, yet it only takes about 15 minutes to train from scratch for a new scene.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Sun et al_2022_Direct Voxel Grid Optimization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AZUAC5EF\\2111.html}
}

@online{sungEmpiricalStudyMultimodal2023,
  title = {An {{Empirical Study}} of {{Multimodal Model Merging}}},
  author = {Sung, Yi-Lin and Li, Linjie and Lin, Kevin and Gan, Zhe and Bansal, Mohit and Wang, Lijuan},
  date = {2023-10-11},
  eprint = {2304.14933},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2304.14933},
  urldate = {2024-09-23},
  abstract = {Model merging (e.g., via interpolation or task arithmetic) fuses multiple models trained on different tasks to generate a multi-task solution. The technique has been proven successful in previous studies, where the models are trained on similar tasks and with the same initialization. In this paper, we expand on this concept to a multimodal setup by merging transformers trained on different modalities. Furthermore, we conduct our study for a novel goal where we can merge vision, language, and cross-modal transformers of a modality-specific architecture to create a parameter-efficient modality-agnostic architecture. Through comprehensive experiments, we systematically investigate the key factors impacting model performance after merging, including initialization, merging mechanisms, and model architectures. We also propose two metrics that assess the distance between weights to be merged and can serve as an indicator of the merging outcomes. Our analysis leads to an effective training recipe for matching the performance of the modality-agnostic baseline (i.e., pre-trained from scratch) via model merging. Our method also outperforms naive merging significantly on various tasks, with improvements of 3\% on VQA, 7\% on COCO retrieval, 25\% on NLVR2, 14\% on Flickr30k and 3\% on ADE20k. Our code is available at https://github.com/ylsung/vl-merging},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\HD9F6B3L\Sung 등 - 2023 - An Empirical Study of Multimodal Model Merging.pdf}
}

@online{sunImprovedDirectVoxel2022,
  title = {Improved {{Direct Voxel Grid Optimization}} for {{Radiance Fields Reconstruction}}},
  author = {Sun, Cheng and Sun, Min and Chen, Hwann-Tzong},
  date = {2022-07-01},
  eprint = {2206.05085},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.05085},
  urldate = {2023-04-09},
  abstract = {In this technical report, we improve the DVGO framework (called DVGOv2), which is based on Pytorch and uses the simplest dense grid representation. First, we re-implement part of the Pytorch operations with cuda, achieving 2-3x speedup. The cuda extension is automatically compiled just in time. Second, we extend DVGO to support Forward-facing and Unbounded Inward-facing capturing. Third, we improve the space time complexity of the distortion loss proposed by mip-NeRF 360 from O(N\textasciicircum 2) to O(N). The distortion loss improves our quality and training speed. Our efficient implementation could allow more future works to benefit from the loss.},
  pubstate = {prepublished},
  keywords = {Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Sun et al_2022_Improved Direct Voxel Grid Optimization for Radiance Fields Reconstruction.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4HT7EEI3\\2206.html}
}

@online{sunSingularValueFinetuning2022,
  title = {Singular {{Value Fine-tuning}}: {{Few-shot Segmentation}} Requires {{Few-parameters Fine-tuning}}},
  shorttitle = {Singular {{Value Fine-tuning}}},
  author = {Sun, Yanpeng and Chen, Qiang and He, Xiangyu and Wang, Jian and Feng, Haocheng and Han, Junyu and Ding, Errui and Cheng, Jian and Li, Zechao and Wang, Jingdong},
  date = {2022-10-10},
  eprint = {2206.06122},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2206.06122},
  url = {http://arxiv.org/abs/2206.06122},
  urldate = {2023-08-07},
  abstract = {Freezing the pre-trained backbone has become a standard paradigm to avoid overfitting in few-shot segmentation. In this paper, we rethink the paradigm and explore a new regime: \{\textbackslash em fine-tuning a small part of parameters in the backbone\}. We present a solution to overcome the overfitting problem, leading to better model generalization on learning novel classes. Our method decomposes backbone parameters into three successive matrices via the Singular Value Decomposition (SVD), then \{\textbackslash em only fine-tunes the singular values\} and keeps others frozen. The above design allows the model to adjust feature representations on novel classes while maintaining semantic clues within the pre-trained backbone. We evaluate our \{\textbackslash em Singular Value Fine-tuning (SVF)\} approach on various few-shot segmentation methods with different backbones. We achieve state-of-the-art results on both Pascal-5\$\textasciicircum i\$ and COCO-20\$\textasciicircum i\$ across 1-shot and 5-shot settings. Hopefully, this simple baseline will encourage researchers to rethink the role of backbone fine-tuning in few-shot settings. The source code and models will be available at https://github.com/syp2ysy/SVF.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Sun et al_2022_Singular Value Fine-tuning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QPQ6M72T\\2206.html}
}

@online{sunVideoBERTJointModel2019,
  title = {{{VideoBERT}}: {{A Joint Model}} for {{Video}} and {{Language Representation Learning}}},
  shorttitle = {{{VideoBERT}}},
  author = {Sun, Chen and Myers, Austin and Vondrick, Carl and Murphy, Kevin and Schmid, Cordelia},
  date = {2019-09-11},
  eprint = {1904.01766},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.01766},
  url = {http://arxiv.org/abs/1904.01766},
  urldate = {2024-01-30},
  abstract = {Self-supervised learning has become increasingly important to leverage the abundance of unlabeled data available on platforms like YouTube. Whereas most existing approaches learn low-level representations, we propose a joint visual-linguistic model to learn high-level features without any explicit supervision. In particular, inspired by its recent success in language modeling, we build upon the BERT model to learn bidirectional joint distributions over sequences of visual and linguistic tokens, derived from vector quantization of video data and off-the-shelf speech recognition outputs, respectively. We use VideoBERT in numerous tasks, including action classification and video captioning. We show that it can be applied directly to open-vocabulary classification, and confirm that large amounts of training data and cross-modal information are critical to performance. Furthermore, we outperform the state-of-the-art on video captioning, and quantitative results verify that the model learns high-level semantic features.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Sun et al_2019_VideoBERT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HP434WCQ\\1904.html}
}

@online{sunVideoBERTJointModel2019a,
  title = {{{VideoBERT}}: {{A Joint Model}} for {{Video}} and {{Language Representation Learning}}},
  shorttitle = {{{VideoBERT}}},
  author = {Sun, Chen and Myers, Austin and Vondrick, Carl and Murphy, Kevin and Schmid, Cordelia},
  date = {2019-09-11},
  eprint = {1904.01766},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.01766},
  url = {http://arxiv.org/abs/1904.01766},
  urldate = {2023-08-05},
  abstract = {Self-supervised learning has become increasingly important to leverage the abundance of unlabeled data available on platforms like YouTube. Whereas most existing approaches learn low-level representations, we propose a joint visual-linguistic model to learn high-level features without any explicit supervision. In particular, inspired by its recent success in language modeling, we build upon the BERT model to learn bidirectional joint distributions over sequences of visual and linguistic tokens, derived from vector quantization of video data and off-the-shelf speech recognition outputs, respectively. We use VideoBERT in numerous tasks, including action classification and video captioning. We show that it can be applied directly to open-vocabulary classification, and confirm that large amounts of training data and cross-modal information are critical to performance. Furthermore, we outperform the state-of-the-art on video captioning, and quantitative results verify that the model learns high-level semantic features.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\vision and language\\Sun et al_2019_VideoBERT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\L6Z95I36\\1904.html}
}

@online{SuperresolutionComprehensiveSurvey,
  title = {Super-Resolution: A Comprehensive Survey | {{SpringerLink}}},
  url = {https://link.springer.com/article/10.1007/s00138-014-0623-4},
  urldate = {2022-09-30},
  file = {C:\Users\chsey\Zotero\storage\LIY99LV4\s00138-014-0623-4.html}
}

@online{SuttonBartoBook,
  title = {Sutton \& {{Barto Book}}: {{Reinforcement Learning}}: {{An Introduction}}},
  url = {http://incompleteideas.net/book/the-book-2nd.html},
  urldate = {2024-03-11},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\NTZEZIRB\the-book-2nd.html}
}

@book{suttonReinforcementLearningIntroduction2018,
  title = {Reinforcement Learning: An Introduction},
  shorttitle = {Reinforcement Learning},
  author = {Sutton, Richard S. and Barto, Andrew G.},
  date = {2018},
  series = {Adaptive Computation and Machine Learning Series},
  edition = {Second edition},
  publisher = {The MIT Press},
  location = {Cambridge, Massachusetts},
  abstract = {"Reinforcement learning, one of the most active research areas in artificial intelligence, is a computational approach to learning whereby an agent tries to maximize the total amount of reward it receives while interacting with a complex, uncertain environment. In Reinforcement Learning, Richard Sutton and Andrew Barto provide a clear and simple account of the field's key ideas and algorithms."--},
  isbn = {978-0-262-03924-6},
  langid = {english},
  pagetotal = {526},
  keywords = {notion,Reinforcement learning},
  file = {Y:\paper\2024_research\Sutton_Barto_2018_Reinforcement learning.pdf}
}

@book{suttonReinforcementLearningIntroduction2020,
  title = {Reinforcement Learning: An Introduction},
  shorttitle = {Reinforcement Learning},
  author = {Sutton, Richard S. and Barto, Andrew},
  date = {2020},
  series = {Adaptive Computation and Machine Learning},
  edition = {Second edition},
  publisher = {The MIT Press},
  location = {Cambridge, Massachusetts London, England},
  abstract = {"Reinforcement learning, one of the most active research areas in artificial intelligence, is a computational approach to learning whereby an agent tries to maximize the total amount of reward it receives while interacting with a complex, uncertain environment. In Reinforcement Learning, Richard Sutton and Andrew Barto provide a clear and simple account of the field's key ideas and algorithms."--},
  isbn = {978-0-262-03924-6},
  langid = {english},
  pagetotal = {526},
  keywords = {notion}
}

@online{szegedyGoingDeeperConvolutions2014,
  title = {Going {{Deeper}} with {{Convolutions}}},
  author = {Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  date = {2014-09-16},
  eprint = {1409.4842},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1409.4842},
  urldate = {2022-09-15},
  abstract = {We propose a deep convolutional neural network architecture codenamed "Inception", which was responsible for setting the new state of the art for classification and detection in the ImageNet Large-Scale Visual Recognition Challenge 2014 (ILSVRC 2014). The main hallmark of this architecture is the improved utilization of the computing resources inside the network. This was achieved by a carefully crafted design that allows for increasing the depth and width of the network while keeping the computational budget constant. To optimize quality, the architectural decisions were based on the Hebbian principle and the intuition of multi-scale processing. One particular incarnation used in our submission for ILSVRC 2014 is called GoogLeNet, a 22 layers deep network, the quality of which is assessed in the context of classification and detection.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Szegedy et al_2014_Going Deeper with Convolutions.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TBYDTCP5\\1409.html}
}

@online{tagliasacchiVolumeRenderingDigest2022,
  title = {Volume {{Rendering Digest}} (for {{NeRF}})},
  author = {Tagliasacchi, Andrea and Mildenhall, Ben},
  date = {2022-08-29},
  eprint = {2209.02417},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2209.02417},
  urldate = {2023-01-20},
  abstract = {Neural Radiance Fields employ simple volume rendering as a way to overcome the challenges of differentiating through ray-triangle intersections by leveraging a probabilistic notion of visibility. This is achieved by assuming the scene is composed by a cloud of light-emitting particles whose density changes in space. This technical report summarizes the derivations for differentiable volume rendering. It is a condensed version of previous reports, but rewritten in the context of NeRF, and adopting its commonly used notation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,I.3,I.4},
  file = {Y\:\\paper\\2022 winter intern\\Tagliasacchi_Mildenhall_2022_Volume Rendering Digest (for NeRF).pdf;C\:\\Users\\chsey\\Zotero\\storage\\I4ZJ7MNK\\2209.html}
}

@online{tancikFourierFeaturesLet2020,
  title = {Fourier {{Features Let Networks Learn High Frequency Functions}} in {{Low Dimensional Domains}}},
  author = {Tancik, Matthew and Srinivasan, Pratul P. and Mildenhall, Ben and Fridovich-Keil, Sara and Raghavan, Nithin and Singhal, Utkarsh and Ramamoorthi, Ravi and Barron, Jonathan T. and Ng, Ren},
  date = {2020-06-18},
  eprint = {2006.10739},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2006.10739},
  url = {http://arxiv.org/abs/2006.10739},
  urldate = {2023-01-11},
  abstract = {We show that passing input points through a simple Fourier feature mapping enables a multilayer perceptron (MLP) to learn high-frequency functions in low-dimensional problem domains. These results shed light on recent advances in computer vision and graphics that achieve state-of-the-art results by using MLPs to represent complex 3D objects and scenes. Using tools from the neural tangent kernel (NTK) literature, we show that a standard MLP fails to learn high frequencies both in theory and in practice. To overcome this spectral bias, we use a Fourier feature mapping to transform the effective NTK into a stationary kernel with a tunable bandwidth. We suggest an approach for selecting problem-specific Fourier features that greatly improves the performance of MLPs for low-dimensional regression tasks relevant to the computer vision and graphics communities.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\Tancik et al_2020_Fourier Features Let Networks Learn High Frequency Functions in Low Dimensional.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ZLTJ8I6R\\2006.html}
}

@online{tanEfficientDetScalableEfficient2020,
  title = {{{EfficientDet}}: {{Scalable}} and {{Efficient Object Detection}}},
  shorttitle = {{{EfficientDet}}},
  author = {Tan, Mingxing and Pang, Ruoming and Le, Quoc V.},
  date = {2020-07-27},
  eprint = {1911.09070},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  doi = {10.48550/arXiv.1911.09070},
  url = {http://arxiv.org/abs/1911.09070},
  urldate = {2022-07-25},
  abstract = {Model efficiency has become increasingly important in computer vision. In this paper, we systematically study neural network architecture design choices for object detection and propose several key optimizations to improve efficiency. First, we propose a weighted bi-directional feature pyramid network (BiFPN), which allows easy and fast multiscale feature fusion; Second, we propose a compound scaling method that uniformly scales the resolution, depth, and width for all backbone, feature network, and box/class prediction networks at the same time. Based on these optimizations and better backbones, we have developed a new family of object detectors, called EfficientDet, which consistently achieve much better efficiency than prior art across a wide spectrum of resource constraints. In particular, with single model and single-scale, our EfficientDet-D7 achieves state-of-the-art 55.1 AP on COCO test-dev with 77M parameters and 410B FLOPs, being 4x - 9x smaller and using 13x - 42x fewer FLOPs than previous detectors. Code is available at https://github.com/google/automl/tree/master/efficientdet.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Tan et al_2020_EfficientDet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GCQI6QFA\\1911.html}
}

@online{tanEfficientDetScalableEfficient2020a,
  title = {{{EfficientDet}}: {{Scalable}} and {{Efficient Object Detection}}},
  shorttitle = {{{EfficientDet}}},
  author = {Tan, Mingxing and Pang, Ruoming and Le, Quoc V.},
  date = {2020-07-27},
  eprint = {1911.09070},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  doi = {10.48550/arXiv.1911.09070},
  url = {http://arxiv.org/abs/1911.09070},
  urldate = {2022-07-04},
  abstract = {Model efficiency has become increasingly important in computer vision. In this paper, we systematically study neural network architecture design choices for object detection and propose several key optimizations to improve efficiency. First, we propose a weighted bi-directional feature pyramid network (BiFPN), which allows easy and fast multiscale feature fusion; Second, we propose a compound scaling method that uniformly scales the resolution, depth, and width for all backbone, feature network, and box/class prediction networks at the same time. Based on these optimizations and better backbones, we have developed a new family of object detectors, called EfficientDet, which consistently achieve much better efficiency than prior art across a wide spectrum of resource constraints. In particular, with single model and single-scale, our EfficientDet-D7 achieves state-of-the-art 55.1 AP on COCO test-dev with 77M parameters and 410B FLOPs, being 4x - 9x smaller and using 13x - 42x fewer FLOPs than previous detectors. Code is available at https://github.com/google/automl/tree/master/efficientdet.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Electrical Engineering and Systems Science - Image and Video Processing},
  file = {Y\:\\paper\\Computer Vision\\detection\\Tan et al_2020_EfficientDet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AERCA3S6\\1911.html}
}

@online{tanEfficientNetRethinkingModel2020,
  title = {{{EfficientNet}}: {{Rethinking Model Scaling}} for {{Convolutional Neural Networks}}},
  shorttitle = {{{EfficientNet}}},
  author = {Tan, Mingxing and Le, Quoc V.},
  date = {2020-09-11},
  eprint = {1905.11946},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1905.11946},
  url = {http://arxiv.org/abs/1905.11946},
  urldate = {2022-07-04},
  abstract = {Convolutional Neural Networks (ConvNets) are commonly developed at a fixed resource budget, and then scaled up for better accuracy if more resources are available. In this paper, we systematically study model scaling and identify that carefully balancing network depth, width, and resolution can lead to better performance. Based on this observation, we propose a new scaling method that uniformly scales all dimensions of depth/width/resolution using a simple yet highly effective compound coefficient. We demonstrate the effectiveness of this method on scaling up MobileNets and ResNet. To go even further, we use neural architecture search to design a new baseline network and scale it up to obtain a family of models, called EfficientNets, which achieve much better accuracy and efficiency than previous ConvNets. In particular, our EfficientNet-B7 achieves state-of-the-art 84.3\% top-1 accuracy on ImageNet, while being 8.4x smaller and 6.1x faster on inference than the best existing ConvNet. Our EfficientNets also transfer well and achieve state-of-the-art accuracy on CIFAR-100 (91.7\%), Flowers (98.8\%), and 3 other transfer learning datasets, with an order of magnitude fewer parameters. Source code is at https://github.com/tensorflow/tpu/tree/master/models/official/efficientnet.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Tan_Le_2020_EfficientNet.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XWEDJM7B\\1905.html}
}

@online{tanEfficientNetV2SmallerModels2021,
  title = {{{EfficientNetV2}}: {{Smaller Models}} and {{Faster Training}}},
  shorttitle = {{{EfficientNetV2}}},
  author = {Tan, Mingxing and Le, Quoc V.},
  date = {2021-06-23},
  eprint = {2104.00298},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2104.00298},
  urldate = {2022-07-04},
  abstract = {This paper introduces EfficientNetV2, a new family of convolutional networks that have faster training speed and better parameter efficiency than previous models. To develop this family of models, we use a combination of training-aware neural architecture search and scaling, to jointly optimize training speed and parameter efficiency. The models were searched from the search space enriched with new ops such as Fused-MBConv. Our experiments show that EfficientNetV2 models train much faster than state-of-the-art models while being up to 6.8x smaller. Our training can be further sped up by progressively increasing the image size during training, but it often causes a drop in accuracy. To compensate for this accuracy drop, we propose to adaptively adjust regularization (e.g., dropout and data augmentation) as well, such that we can achieve both fast training and good accuracy. With progressive learning, our EfficientNetV2 significantly outperforms previous models on ImageNet and CIFAR/Cars/Flowers datasets. By pretraining on the same ImageNet21k, our EfficientNetV2 achieves 87.3\% top-1 accuracy on ImageNet ILSVRC2012, outperforming the recent ViT by 2.0\% accuracy while training 5x-11x faster using the same computing resources. Code will be available at https://github.com/google/automl/tree/master/efficientnetv2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Tan_Le_2021_EfficientNetV2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\52JKQWFL\\2104.html}
}

@online{tanEfficientNetV2SmallerModels2021a,
  title = {{{EfficientNetV2}}: {{Smaller Models}} and {{Faster Training}}},
  shorttitle = {{{EfficientNetV2}}},
  author = {Tan, Mingxing and Le, Quoc V.},
  date = {2021-06-23},
  eprint = {2104.00298},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2104.00298},
  urldate = {2022-06-30},
  abstract = {This paper introduces EfficientNetV2, a new family of convolutional networks that have faster training speed and better parameter efficiency than previous models. To develop this family of models, we use a combination of training-aware neural architecture search and scaling, to jointly optimize training speed and parameter efficiency. The models were searched from the search space enriched with new ops such as Fused-MBConv. Our experiments show that EfficientNetV2 models train much faster than state-of-the-art models while being up to 6.8x smaller. Our training can be further sped up by progressively increasing the image size during training, but it often causes a drop in accuracy. To compensate for this accuracy drop, we propose to adaptively adjust regularization (e.g., dropout and data augmentation) as well, such that we can achieve both fast training and good accuracy. With progressive learning, our EfficientNetV2 significantly outperforms previous models on ImageNet and CIFAR/Cars/Flowers datasets. By pretraining on the same ImageNet21k, our EfficientNetV2 achieves 87.3\% top-1 accuracy on ImageNet ILSVRC2012, outperforming the recent ViT by 2.0\% accuracy while training 5x-11x faster using the same computing resources. Code will be available at https://github.com/google/automl/tree/master/efficientnetv2.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\classificaiton\\Tan_Le_2021_EfficientNetV2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7FEZ9RFE\\2104.html}
}

@online{tangCoDi2InContextInterleaved2023,
  title = {{{CoDi-2}}: {{In-Context}}, {{Interleaved}}, and {{Interactive Any-to-Any Generation}}},
  shorttitle = {{{CoDi-2}}},
  author = {Tang, Zineng and Yang, Ziyi and Khademi, Mahmoud and Liu, Yang and Zhu, Chenguang and Bansal, Mohit},
  date = {2023-11-30},
  eprint = {2311.18775},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  doi = {10.48550/arXiv.2311.18775},
  url = {http://arxiv.org/abs/2311.18775},
  urldate = {2024-06-24},
  abstract = {We present CoDi-2, a versatile and interactive Multimodal Large Language Model (MLLM) that can follow complex multimodal interleaved instructions, conduct in-context learning (ICL), reason, chat, edit, etc., in an any-to-any input-output modality paradigm. By aligning modalities with language for both encoding and generation, CoDi-2 empowers Large Language Models (LLMs) to not only understand complex modality-interleaved instructions and in-context examples, but also autoregressively generate grounded and coherent multimodal outputs in the continuous feature space. To train CoDi-2, we build a large-scale generation dataset encompassing in-context multimodal instructions across text, vision, and audio. CoDi-2 demonstrates a wide range of zero-shot capabilities for multimodal generation, such as in-context learning, reasoning, and compositionality of any-to-any modality generation through multi-round interactive conversation. CoDi-2 surpasses previous domain-specific models on tasks such as subject-driven image generation, vision transformation, and audio editing. CoDi-2 signifies a substantial breakthrough in developing a comprehensive multimodal foundation model adept at interpreting in-context language-vision-audio interleaved instructions and producing multimodal outputs.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Sound,Electrical Engineering and Systems Science - Audio and Speech Processing,notion},
  file = {Y\:\\paper\\2024_research\\Tang et al_2023_CoDi-2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\L2XNQ6D4\\2311.html}
}

@online{tangMergingMultiTaskModels2024,
  title = {Merging {{Multi-Task Models}} via {{Weight-Ensembling Mixture}} of {{Experts}}},
  author = {Tang, Anke and Shen, Li and Luo, Yong and Yin, Nan and Zhang, Lefei and Tao, Dacheng},
  date = {2024-06-07},
  eprint = {2402.00433},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2402.00433},
  urldate = {2024-10-22},
  abstract = {Merging various task-specific Transformer-based models trained on different tasks into a single unified model can execute all the tasks concurrently. Previous methods, exemplified by task arithmetic, have been proven to be both effective and scalable. Existing methods have primarily focused on seeking a static optimal solution within the original model parameter space. A notable challenge is mitigating the interference between parameters of different models, which can substantially deteriorate performance. In this paper, we propose to merge most of the parameters while upscaling the MLP of the Transformer layers to a weight-ensembling mixture of experts (MoE) module, which can dynamically integrate shared and task-specific knowledge based on the input, thereby providing a more flexible solution that can adapt to the specific needs of each instance. Our key insight is that by identifying and separating shared knowledge and task-specific knowledge, and then dynamically integrating them, we can mitigate the parameter interference problem to a great extent. We conduct the conventional multi-task model merging experiments and evaluate the generalization and robustness of our method. The results demonstrate the effectiveness of our method and provide a comprehensive understanding of our method. The code is available at https://github.com/tanganke/weight-ensembling\_MoE},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Tang et al_2024_Merging Multi-Task Models via Weight-Ensembling Mixture of Experts.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8WTJCG2H\\2402.html}
}

@online{tangParameterEfficientMultitask2024,
  title = {Parameter {{Efficient Multi-task Model Fusion}} with {{Partial Linearization}}},
  author = {Tang, Anke and Shen, Li and Luo, Yong and Zhan, Yibing and Hu, Han and Du, Bo and Chen, Yixin and Tao, Dacheng},
  date = {2024-03-11},
  eprint = {2310.04742},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2310.04742},
  urldate = {2024-09-23},
  abstract = {Large pre-trained models have enabled significant advances in machine learning and served as foundation components. Model fusion methods, such as task arithmetic, have been proven to be powerful and scalable to incorporate fine-tuned weights from different tasks into a multi-task model. However, efficiently finetuning large pre-trained models on multiple downstream tasks remains challenging, leading to inefficient multi-task model fusion. In this work, we propose a novel method to improve multi-task fusion for parameter-efficient fine-tuning techniques like LoRA fine-tuning. Specifically, our approach partially linearizes only the adapter modules and applies task arithmetic over the linearized adapters. This allows us to leverage the the advantages of model fusion over linearized finetuning, while still performing fine-tuning and inference efficiently. We demonstrate that our partial linearization technique enables a more effective fusion of multiple tasks into a single model, outperforming standard adapter tuning and task arithmetic alone. Experimental results demonstrate the capabilities of our proposed partial linearization technique to effectively construct unified multi-task models via the fusion of fine-tuned task vectors. We evaluate performance over an increasing number of tasks and find that our approach outperforms standard parameter-efficient fine-tuning techniques. The results highlight the benefits of partial linearization for scalable and efficient multi-task model fusion.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\7EFJJQZV\Tang 등 - 2024 - Parameter Efficient Multi-task Model Fusion with P.pdf}
}

@online{tangUnbiasedSceneGraph2020,
  title = {Unbiased {{Scene Graph Generation}} from {{Biased Training}}},
  author = {Tang, Kaihua and Niu, Yulei and Huang, Jianqiang and Shi, Jiaxin and Zhang, Hanwang},
  date = {2020-03-11},
  eprint = {2002.11949},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2002.11949},
  url = {http://arxiv.org/abs/2002.11949},
  urldate = {2023-05-29},
  abstract = {Today's scene graph generation (SGG) task is still far from practical, mainly due to the severe training bias, e.g., collapsing diverse "human walk on / sit on / lay on beach" into "human on beach". Given such SGG, the down-stream tasks such as VQA can hardly infer better scene structures than merely a bag of objects. However, debiasing in SGG is not trivial because traditional debiasing methods cannot distinguish between the good and bad bias, e.g., good context prior (e.g., "person read book" rather than "eat") and bad long-tailed bias (e.g., "near" dominating "behind / in front of"). In this paper, we present a novel SGG framework based on causal inference but not the conventional likelihood. We first build a causal graph for SGG, and perform traditional biased training with the graph. Then, we propose to draw the counterfactual causality from the trained graph to infer the effect from the bad bias, which should be removed. In particular, we use Total Direct Effect (TDE) as the proposed final predicate score for unbiased SGG. Note that our framework is agnostic to any SGG model and thus can be widely applied in the community who seeks unbiased predictions. By using the proposed Scene Graph Diagnosis toolkit on the SGG benchmark Visual Genome and several prevailing models, we observed significant improvements over the previous state-of-the-art methods.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Tang et al_2020_Unbiased Scene Graph Generation from Biased Training.pdf;C\:\\Users\\chsey\\Zotero\\storage\\H9G43R9F\\2002.html}
}

@inproceedings{tangWhenPromptbasedIncremental2023,
  title = {When {{Prompt-based Incremental Learning Does Not Meet Strong Pretraining}}},
  author = {Tang, Yu-Ming and Peng, Yi-Xing and Zheng, Wei-Shi},
  date = {2023},
  pages = {1706--1716},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Tang_When_Prompt-based_Incremental_Learning_Does_Not_Meet_Strong_Pretraining_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion,Pretraining},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Tang et al_2023_When Prompt-based Incremental Learning Does Not Meet Strong Pretraining.pdf}
}

@inproceedings{tayebiSpatiallyEmbeddedCooffence2014,
  title = {Spatially Embedded Co-Offence Prediction Using Supervised Learning},
  booktitle = {Proceedings of the 20th {{ACM SIGKDD}} International Conference on {{Knowledge}} Discovery and Data Mining},
  author = {Tayebi, Mohammad A. and Ester, Martin and Glässer, Uwe and Brantingham, Patricia L.},
  year = {8월 24, 2014},
  series = {{{KDD}} '14},
  pages = {1789--1798},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/2623330.2623353},
  url = {https://doi.org/10.1145/2623330.2623353},
  urldate = {2023-05-24},
  abstract = {Crime reduction and prevention strategies are essential to increase public safety and reduce the crime costs to society. Law enforcement agencies have long realized the importance of analyzing co-offending networks---networks of offenders who have committed crimes together---for this purpose. Although network structure can contribute significantly to co-offence prediction, research in this area is very limited. Here we address this important problem by proposing a framework for co-offence prediction using supervised learning. Considering the available information about offenders, we introduce social, geographic, geo-social and similarity feature sets which are used for classifying potential negative and positive pairs of offenders. Similar to other social networks, co-offending networks also suffer from a highly skewed distribution of positive and negative pairs. To address the class imbalance problem, we identify three types of criminal cooperation opportunities which help to reduce the class imbalance ratio significantly, while keeping half of the co-offences. The proposed framework is evaluated on a large crime dataset for the Province of British Columbia, Canada. Our experimental evaluation of four different feature sets show that the novel geo-social features are the best predictors. Overall, we experimentally show the high effectiveness of the proposed co-offence prediction framework. We believe that our framework will not only allow law enforcement agencies to improve their crime reduction and prevention strategies, but also offers new criminological insights into criminal link formation between offenders.},
  isbn = {978-1-4503-2956-9},
  keywords = {co-offence prediction,link prediction,social network}
}

@article{tewariAdvancesNeuralRendering2022,
  title = {Advances in {{Neural Rendering}}},
  author = {Tewari, A. and Thies, J. and Mildenhall, B. and Srinivasan, P. and Tretschk, E. and Yifan, W. and Lassner, C. and Sitzmann, V. and Martin-Brualla, R. and Lombardi, S. and Simon, T. and Theobalt, C. and Nießner, M. and Barron, J. T. and Wetzstein, G. and Zollhöfer, M. and Golyanik, V.},
  date = {2022},
  journaltitle = {Computer Graphics Forum},
  volume = {41},
  number = {2},
  pages = {703--735},
  issn = {1467-8659},
  doi = {10.1111/cgf.14507},
  url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/cgf.14507},
  urldate = {2023-01-02},
  abstract = {Synthesizing photo-realistic images and videos is at the heart of computer graphics and has been the focus of decades of research. Traditionally, synthetic images of a scene are generated using rendering algorithms such as rasterization or ray tracing, which take specifically defined representations of geometry and material properties as input. Collectively, these inputs define the actual scene and what is rendered, and are referred to as the scene representation (where a scene consists of one or more objects). Example scene representations are triangle meshes with accompanied textures (e.g., created by an artist), point clouds (e.g., from a depth sensor), volumetric grids (e.g., from a CT scan), or implicit surface functions (e.g., truncated signed distance fields). The reconstruction of such a scene representation from observations using differentiable rendering losses is known as inverse graphics or inverse rendering. Neural rendering is closely related, and combines ideas from classical computer graphics and machine learning to create algorithms for synthesizing images from real-world observations. Neural rendering is a leap forward towards the goal of synthesizing photo-realistic image and video content. In recent years, we have seen immense progress in this field through hundreds of publications that show different ways to inject learnable components into the rendering pipeline. This state-of-the-art report on advances in neural rendering focuses on methods that combine classical rendering principles with learned 3D scene representations, often now referred to as neural scene representations. A key advantage of these methods is that they are 3D-consistent by design, enabling applications such as novel viewpoint synthesis of a captured scene. In addition to methods that handle static scenes, we cover neural scene representations for modeling non-rigidly deforming objects and scene editing and composition. While most of these approaches are scene-specific, we also discuss techniques that generalize across object classes and can be used for generative tasks. In addition to reviewing these state-of-the-art methods, we provide an overview of fundamental concepts and definitions used in the current literature. We conclude with a discussion on open challenges and social implications.},
  langid = {english},
  file = {Y\:\\paper\\2022 winter intern\\Tewari et al_2022_Advances in Neural Rendering.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AYRPVEZZ\\cgf.html}
}

@article{thomeeYFCC100MNewData2016,
  title = {{{YFCC100M}}: {{The New Data}} in {{Multimedia Research}}},
  shorttitle = {{{YFCC100M}}},
  author = {Thomee, Bart and Shamma, David A. and Friedland, Gerald and Elizalde, Benjamin and Ni, Karl and Poland, Douglas and Borth, Damian and Li, Li-Jia},
  date = {2016-01-25},
  journaltitle = {Communications of the ACM},
  shortjournal = {Commun. ACM},
  volume = {59},
  number = {2},
  eprint = {1503.01817},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {64--73},
  issn = {0001-0782, 1557-7317},
  doi = {10.1145/2812802},
  url = {http://arxiv.org/abs/1503.01817},
  urldate = {2023-05-29},
  abstract = {We present the Yahoo Flickr Creative Commons 100 Million Dataset (YFCC100M), the largest public multimedia collection that has ever been released. The dataset contains a total of 100 million media objects, of which approximately 99.2 million are photos and 0.8 million are videos, all of which carry a Creative Commons license. Each media object in the dataset is represented by several pieces of metadata, e.g. Flickr identifier, owner name, camera, title, tags, geo, media source. The collection provides a comprehensive snapshot of how photos and videos were taken, described, and shared over the years, from the inception of Flickr in 2004 until early 2014. In this article we explain the rationale behind its creation, as well as the implications the dataset has for science, research, engineering, and development. We further present several new challenges in multimedia research that can now be expanded upon with our dataset.},
  keywords = {Computer Science - Computers and Society,Computer Science - Multimedia,H.3.7},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Thomee et al_2016_YFCC100M.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CYBH5FXZ\\1503.html}
}

@inproceedings{timorImplicitRegularizationRank2023,
  title = {Implicit {{Regularization Towards Rank Minimization}} in {{ReLU Networks}}},
  booktitle = {Proceedings of {{The}} 34th {{International Conference}} on {{Algorithmic Learning Theory}}},
  author = {Timor, Nadav and Vardi, Gal and Shamir, Ohad},
  date = {2023-02-13},
  pages = {1429--1459},
  publisher = {PMLR},
  issn = {2640-3498},
  url = {https://proceedings.mlr.press/v201/timor23a.html},
  urldate = {2024-04-03},
  abstract = {We study the conjectured relationship between the implicit~regularization in neural~networks, trained with gradient-based methods, and rank~minimization of their weight~matrices. Previously, it was proved that for linear~networks (of depth~\$2\$ and vector-valued~outputs), gradient~flow~(GF) w.r.t. the square~loss acts as a rank~minimization~heuristic. However, understanding to what extent this generalizes to nonlinear~networks is an open~problem. In this paper, we focus on nonlinear~ReLU~networks, providing several new positive and negative results. On the negative side, we prove (and demonstrate empirically) that, unlike the linear~case, GF on ReLU~networks may no~longer tend to minimize~ranks, in a rather~strong sense (even approximately, for “most” datasets of size~\$2\$). On the positive side, we reveal that ReLU~networks of sufficient~depth are provably biased towards low-rank~solutions in several reasonable settings.},
  eventtitle = {International {{Conference}} on {{Algorithmic Learning Theory}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Timor et al_2023_Implicit Regularization Towards Rank Minimization in ReLU Networks.pdf}
}

@online{tolstikhinMLPMixerAllMLPArchitecture2021,
  title = {{{MLP-Mixer}}: {{An}} All-{{MLP Architecture}} for {{Vision}}},
  shorttitle = {{{MLP-Mixer}}},
  author = {Tolstikhin, Ilya and Houlsby, Neil and Kolesnikov, Alexander and Beyer, Lucas and Zhai, Xiaohua and Unterthiner, Thomas and Yung, Jessica and Steiner, Andreas and Keysers, Daniel and Uszkoreit, Jakob and Lucic, Mario and Dosovitskiy, Alexey},
  date = {2021-06-11},
  eprint = {2105.01601},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2105.01601},
  url = {http://arxiv.org/abs/2105.01601},
  urldate = {2023-10-24},
  abstract = {Convolutional Neural Networks (CNNs) are the go-to model for computer vision. Recently, attention-based networks, such as the Vision Transformer, have also become popular. In this paper we show that while convolutions and attention are both sufficient for good performance, neither of them are necessary. We present MLP-Mixer, an architecture based exclusively on multi-layer perceptrons (MLPs). MLP-Mixer contains two types of layers: one with MLPs applied independently to image patches (i.e. "mixing" the per-location features), and one with MLPs applied across patches (i.e. "mixing" spatial information). When trained on large datasets, or with modern regularization schemes, MLP-Mixer attains competitive scores on image classification benchmarks, with pre-training and inference cost comparable to state-of-the-art models. We hope that these results spark further research beyond the realms of well established CNNs and Transformers.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Tolstikhin et al_2021_MLP-Mixer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\B4FTTA89\\2105.html}
}

@article{tomasevAISocialGood2020,
  title = {{{AI}} for Social Good: Unlocking the Opportunity for Positive Impact},
  shorttitle = {{{AI}} for Social Good},
  author = {Tomašev, Nenad and Cornebise, Julien and Hutter, Frank and Mohamed, Shakir and Picciariello, Angela and Connelly, Bec and Belgrave, Danielle C. M. and Ezer, Daphne and family=Haert, given=Fanny Cachat, prefix=van der, useprefix=false and Mugisha, Frank and Abila, Gerald and Arai, Hiromi and Almiraat, Hisham and Proskurnia, Julia and Snyder, Kyle and Otake-Matsuura, Mihoko and Othman, Mustafa and Glasmachers, Tobias and family=Wever, given=Wilfried, prefix=de, useprefix=false and Teh, Yee Whye and Khan, Mohammad Emtiyaz and Winne, Ruben De and Schaul, Tom and Clopath, Claudia},
  date = {2020-05-18},
  journaltitle = {Nature Communications},
  shortjournal = {Nat Commun},
  volume = {11},
  number = {1},
  pages = {2468},
  publisher = {Nature Publishing Group},
  issn = {2041-1723},
  doi = {10.1038/s41467-020-15871-z},
  url = {https://www.nature.com/articles/s41467-020-15871-z},
  urldate = {2023-05-24},
  abstract = {Advances in machine learning (ML) and artificial intelligence (AI) present an opportunity to build better tools and solutions to help address some of the world’s most pressing challenges, and deliver positive social impact in accordance with the priorities outlined in the United Nations’ 17 Sustainable Development Goals (SDGs). The AI for Social Good (AI4SG) movement aims to establish interdisciplinary partnerships centred around AI applications towards SDGs. We provide a set of guidelines for establishing successful long-term collaborations between AI researchers and application-domain experts, relate them to existing AI4SG projects and identify key opportunities for future AI applications targeted towards social good.},
  issue = {1},
  langid = {english},
  keywords = {Developing world,Ethics},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Tomašev et al_2020_AI for social good.pdf}
}

@online{TorchVisionObjectDetection,
  title = {{{TorchVision Object Detection Finetuning Tutorial}} — {{PyTorch Tutorials}} 1.12.0+cu102 Documentation},
  url = {https://pytorch.org/tutorials/intermediate/torchvision_tutorial.html},
  urldate = {2022-07-05}
}

@article{torralba80MillionTiny2008,
  title = {80 {{Million Tiny Images}}: {{A Large Data Set}} for {{Nonparametric Object}} and {{Scene Recognition}}},
  shorttitle = {80 {{Million Tiny Images}}},
  author = {Torralba, A. and Fergus, R. and Freeman, W.T.},
  date = {2008-11},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  shortjournal = {IEEE Trans. Pattern Anal. Mach. Intell.},
  volume = {30},
  number = {11},
  pages = {1958--1970},
  issn = {0162-8828},
  doi = {10.1109/TPAMI.2008.128},
  url = {http://ieeexplore.ieee.org/document/4531741/},
  urldate = {2022-12-17},
  abstract = {With the advent of the Internet, billions of images are now freely available online and constitute a dense sampling of the visual world. Using a variety of non-parametric methods, we explore this world with the aid of a large dataset of 79,302,017 images collected from the Web. Motivated by psychophysical results showing the remarkable tolerance of the human visual system to degradations in image resolution, the images in the dataset are stored as 32 × 32 color images. Each image is loosely labeled with one of the 75,062 non-abstract nouns in English, as listed in the Wordnet lexical database. Hence the image database gives a comprehensive coverage of all object categories and scenes. The semantic information from Wordnet can be used in conjunction with nearest-neighbor methods to perform object classification over a range of semantic levels minimizing the effects of labeling noise. For certain classes that are particularly prevalent in the dataset, such as people, we are able to demonstrate a recognition performance comparable to class-specific Viola-Jones style detectors.},
  langid = {english},
  file = {Y:\paper\2022 autumn intern\OOD\Torralba et al_2008_80 Million Tiny Images.pdf}
}

@article{torralbaContextualPrimingObject,
  title = {Contextual {{Priming}} for {{Object Detection}}},
  author = {Torralba, Antonio},
  abstract = {There is general consensus that context can be a rich source of information about an object’s identity, location and scale. In fact, the structure of many real-world scenes is governed by strong configurational rules akin to those that apply to a single object. Here we introduce a simple framework for modeling the relationship between context and object properties based on the correlation between the statistics of low-level features across the entire scene and the objects that it contains. The resulting scheme serves as an effective procedure for object priming, context driven focus of attention and automatic scale-selection on real-world scenes.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\computer_vision_topics_18\contextual cues\Torralba_Contextual Priming for Object Detection.pdf}
}

@online{touvronFixingTraintestResolution2022,
  title = {Fixing the Train-Test Resolution Discrepancy},
  author = {Touvron, Hugo and Vedaldi, Andrea and Douze, Matthijs and Jégou, Hervé},
  date = {2022-01-20},
  eprint = {1906.06423},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1906.06423},
  urldate = {2022-07-26},
  abstract = {Data-augmentation is key to the training of neural networks for image classification. This paper first shows that existing augmentations induce a significant discrepancy between the typical size of the objects seen by the classifier at train and test time. We experimentally validate that, for a target test resolution, using a lower train resolution offers better classification at test time. We then propose a simple yet effective and efficient strategy to optimize the classifier performance when the train and test resolutions differ. It involves only a computationally cheap fine-tuning of the network at the test resolution. This enables training strong classifiers using small training images. For instance, we obtain 77.1\% top-1 accuracy on ImageNet with a ResNet-50 trained on 128x128 images, and 79.8\% with one trained on 224x224 image. In addition, if we use extra training data we get 82.5\% with the ResNet-50 train with 224x224 images. Conversely, when training a ResNeXt-101 32x48d pre-trained in weakly-supervised fashion on 940 million public images at resolution 224x224 and further optimizing for test resolution 320x320, we obtain a test top-1 accuracy of 86.4\% (top-5: 98.0\%) (single-crop). To the best of our knowledge this is the highest ImageNet single-crop, top-1 and top-5 accuracy to date.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\data augmentation\\pre-processing\\Touvron et al_2022_Fixing the train-test resolution discrepancy.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UE3AQ4FD\\1906.html}
}

@online{touvronGoingDeeperImage2021,
  title = {Going Deeper with {{Image Transformers}}},
  author = {Touvron, Hugo and Cord, Matthieu and Sablayrolles, Alexandre and Synnaeve, Gabriel and Jégou, Hervé},
  date = {2021-04-07},
  eprint = {2103.17239},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.17239},
  urldate = {2024-04-28},
  abstract = {Transformers have been recently adapted for large scale image classification, achieving high scores shaking up the long supremacy of convolutional neural networks. However the optimization of image transformers has been little studied so far. In this work, we build and optimize deeper transformer networks for image classification. In particular, we investigate the interplay of architecture and optimization of such dedicated transformers. We make two transformers architecture changes that significantly improve the accuracy of deep transformers. This leads us to produce models whose performance does not saturate early with more depth, for instance we obtain 86.5\% top-1 accuracy on Imagenet when training with no external data, we thus attain the current SOTA with less FLOPs and parameters. Moreover, our best model establishes the new state of the art on Imagenet with Reassessed labels and Imagenet-V2 / match frequency, in the setting with no additional training data. We share our code and models1.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y:\paper\2024_research\Touvron et al_2021_Going deeper with Image Transformers.pdf}
}

@online{touvronTrainingDataefficientImage2021,
  title = {Training Data-Efficient Image Transformers \& Distillation through Attention},
  author = {Touvron, Hugo and Cord, Matthieu and Douze, Matthijs and Massa, Francisco and Sablayrolles, Alexandre and Jégou, Hervé},
  date = {2021-01-15},
  eprint = {2012.12877},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2012.12877},
  url = {http://arxiv.org/abs/2012.12877},
  urldate = {2023-06-28},
  abstract = {Recently, neural networks purely based on attention were shown to address image understanding tasks such as image classification. However, these visual transformers are pre-trained with hundreds of millions of images using an expensive infrastructure, thereby limiting their adoption. In this work, we produce a competitive convolution-free transformer by training on Imagenet only. We train them on a single computer in less than 3 days. Our reference vision transformer (86M parameters) achieves top-1 accuracy of 83.1\% (single-crop evaluation) on ImageNet with no external data. More importantly, we introduce a teacher-student strategy specific to transformers. It relies on a distillation token ensuring that the student learns from the teacher through attention. We show the interest of this token-based distillation, especially when using a convnet as a teacher. This leads us to report results competitive with convnets for both Imagenet (where we obtain up to 85.2\% accuracy) and when transferring to other tasks. We share our code and models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Touvron et al_2021_Training data-efficient image transformers & distillation through attention.pdf;C\:\\Users\\chsey\\Zotero\\storage\\K8EX8QZS\\2012.html}
}

@online{TradeCompetitionMigration,
  title = {Trade Competition and Migration: {{Evidence}} from the Quartz Crisis - {{ScienceDirect}}},
  url = {https://www.sciencedirect.com/science/article/pii/S002219962200085X},
  urldate = {2023-12-26},
  file = {C:\Users\chsey\Zotero\storage\3H5FILRX\S002219962200085X.html}
}

@online{tranLearningSpatiotemporalFeatures2015,
  title = {Learning {{Spatiotemporal Features}} with {{3D Convolutional Networks}}},
  author = {Tran, Du and Bourdev, Lubomir and Fergus, Rob and Torresani, Lorenzo and Paluri, Manohar},
  date = {2015-10-06},
  eprint = {1412.0767},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1412.0767},
  url = {http://arxiv.org/abs/1412.0767},
  urldate = {2023-08-05},
  abstract = {We propose a simple, yet effective approach for spatiotemporal feature learning using deep 3-dimensional convolutional networks (3D ConvNets) trained on a large scale supervised video dataset. Our findings are three-fold: 1) 3D ConvNets are more suitable for spatiotemporal feature learning compared to 2D ConvNets; 2) A homogeneous architecture with small 3x3x3 convolution kernels in all layers is among the best performing architectures for 3D ConvNets; and 3) Our learned features, namely C3D (Convolutional 3D), with a simple linear classifier outperform state-of-the-art methods on 4 different benchmarks and are comparable with current best methods on the other 2 benchmarks. In addition, the features are compact: achieving 52.8\% accuracy on UCF101 dataset with only 10 dimensions and also very efficient to compute due to the fast inference of ConvNets. Finally, they are conceptually very simple and easy to train and use.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Tran et al_2015_Learning Spatiotemporal Features with 3D Convolutional Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JZCASCXS\\1412.html}
}

@online{tranVideoClassificationChannelSeparated2019,
  title = {Video {{Classification}} with {{Channel-Separated Convolutional Networks}}},
  author = {Tran, Du and Wang, Heng and Torresani, Lorenzo and Feiszli, Matt},
  date = {2019-11-18},
  eprint = {1904.02811},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.02811},
  url = {http://arxiv.org/abs/1904.02811},
  urldate = {2023-08-05},
  abstract = {Group convolution has been shown to offer great computational savings in various 2D convolutional architectures for image classification. It is natural to ask: 1) if group convolution can help to alleviate the high computational cost of video classification networks; 2) what factors matter the most in 3D group convolutional networks; and 3) what are good computation/accuracy trade-offs with 3D group convolutional networks. This paper studies the effects of different design choices in 3D group convolutional networks for video classification. We empirically demonstrate that the amount of channel interactions plays an important role in the accuracy of 3D group convolutional networks. Our experiments suggest two main findings. First, it is a good practice to factorize 3D convolutions by separating channel interactions and spatiotemporal interactions as this leads to improved accuracy and lower computational cost. Second, 3D channel-separated convolutions provide a form of regularization, yielding lower training accuracy but higher test accuracy compared to 3D convolutions. These two empirical findings lead us to design an architecture -- Channel-Separated Convolutional Network (CSN) -- which is simple, efficient, yet accurate. On Sports1M, Kinetics, and Something-Something, our CSNs are comparable with or better than the state-of-the-art while being 2-3 times more efficient.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Tran et al_2019_Video Classification with Channel-Separated Convolutional Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5DQZG9DQ\\1904.html}
}

@online{tsimpoukelliMultimodalFewShotLearning2021,
  title = {Multimodal {{Few-Shot Learning}} with {{Frozen Language Models}}},
  author = {Tsimpoukelli, Maria and Menick, Jacob and Cabi, Serkan and Eslami, S. M. Ali and Vinyals, Oriol and Hill, Felix},
  date = {2021-07-03},
  eprint = {2106.13884},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.13884},
  urldate = {2024-07-31},
  abstract = {When trained at sufficient scale, auto-regressive language models exhibit the notable ability to learn a new language task after being prompted with just a few examples. Here, we present a simple, yet effective, approach for transferring this few-shot learning ability to a multimodal setting (vision and language). Using aligned image and caption data, we train a vision encoder to represent each image as a sequence of continuous embeddings, such that a pre-trained, frozen language model prompted with this prefix generates the appropriate caption. The resulting system is a multimodal few-shot learner, with the surprising ability to learn a variety of new tasks when conditioned on examples, represented as a sequence of multiple interleaved image and text embeddings. We demonstrate that it can rapidly learn words for new objects and novel visual categories, do visual question-answering with only a handful of examples, and make use of outside knowledge, by measuring a single model on a variety of established and new benchmarks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\7VLCTILG\2106.pdf}
}

@article{twinamTradeCompetitionMigration2022,
  title = {Trade Competition and Migration: {{Evidence}} from the Quartz Crisis},
  shorttitle = {Trade Competition and Migration},
  author = {Twinam, Tate},
  date = {2022-09-01},
  journaltitle = {Journal of International Economics},
  shortjournal = {Journal of International Economics},
  volume = {138},
  pages = {103653},
  issn = {0022-1996},
  doi = {10.1016/j.jinteco.2022.103653},
  url = {https://www.sciencedirect.com/science/article/pii/S002219962200085X},
  urldate = {2023-12-26},
  abstract = {Foreign competition and technological change can both present threats to domestic industries, potentially resulting in out-migration from cities and regions where these industries are spatially agglomerated. In this paper, I study the migration effects of one such trade shock: The quartz crisis, which devastated the globally dominant Swiss watch industry in the 1970s. Using a differences-in-differences strategy, I show that this trade shock led to a rapid loss of population in affected areas, and a long-run change in growth patterns. This contrasts with many other studies of large trade shocks, which find little migration response. I highlight three key factors that distinguish this shock from others and may explain the divergence: (1) the crisis negatively impacted a key export industry while generating no offsetting gains, (2) the affected labor markets were highly non-diversified, and (3) the affected workers were highly mobile.},
  keywords = {Migration,Technological change,Trade competition},
  file = {Y:\paper\management\Twinam_2022_Trade competition and migration3.pdf}
}

@article{twinamTradeCompetitionMigration2022a,
  title = {Trade Competition and Migration: {{Evidence}} from the Quartz Crisis},
  shorttitle = {Trade Competition and Migration},
  author = {Twinam, Tate},
  date = {2022-09-01},
  journaltitle = {Journal of International Economics},
  shortjournal = {Journal of International Economics},
  volume = {138},
  pages = {103653},
  issn = {0022-1996},
  doi = {10.1016/j.jinteco.2022.103653},
  url = {https://www.sciencedirect.com/science/article/pii/S002219962200085X},
  urldate = {2023-12-26},
  abstract = {Foreign competition and technological change can both present threats to domestic industries, potentially resulting in out-migration from cities and regions where these industries are spatially agglomerated. In this paper, I study the migration effects of one such trade shock: The quartz crisis, which devastated the globally dominant Swiss watch industry in the 1970s. Using a differences-in-differences strategy, I show that this trade shock led to a rapid loss of population in affected areas, and a long-run change in growth patterns. This contrasts with many other studies of large trade shocks, which find little migration response. I highlight three key factors that distinguish this shock from others and may explain the divergence: (1) the crisis negatively impacted a key export industry while generating no offsetting gains, (2) the affected labor markets were highly non-diversified, and (3) the affected workers were highly mobile.},
  keywords = {Migration,Technological change,Trade competition}
}

@online{TwitterAdoptionUse,
  title = {Twitter Adoption and Use in Mass Convergence and Emergency Events | {{International Journal}} of {{Emergency Management}}},
  url = {https://www.inderscienceonline.com/doi/abs/10.1504/IJEM.2009.031564},
  urldate = {2023-05-25}
}

@online{TwitterLifelineHumanannotated,
  title = {Twitter as a {{Lifeline}}: {{Human-annotated Twitter Corpora}} for {{NLP}} of {{Crisis-related Messages}} - {{ACL Anthology}}},
  url = {https://aclanthology.org/L16-1259/},
  urldate = {2023-05-25}
}

@online{u.s.navyNautilusSSN571,
  title = {Nautilus ({{SSN-571}})},
  author = {U.S.NAVY},
  url = {http://public1.nhhcaws.local/browse-by-topic/ships/submarines/uss-nautilus.html},
  urldate = {2023-12-28},
  abstract = {USS Nautilus (SSN-571) was commissioned at Groton, Connecticut, on 30 September 1954 with Commander Eugene P. Wilkinson as the boat’s first commander. The construction of Nautilus—the world’s first nuclear powered submarine—was made possible by the successful development of a nuclear propulsion plant by a group of scientists and engineers, under the leadership of Captain Hyman G. Rickover, at the Naval Reactors Branch of the Atomic Energy Commission. Following commissioning, Nautilus remained dockside for further construction and testing for the next several months. On 17 January 1955, she was underway on nuclear power. After sea trials and preliminary acceptance by the Navy, Nautilus headed south for shakedown on 10 May. While enroute to Puerto Rico, she remained submerged traveling 1,381 miles in 89.8 hours, the longest submerged cruise, to that date, by a submarine, and at the highest sustained submerged speed ever recorded for a period of more than one hour’s duration. In July and August, Nautilus conducted rigorous exercises with hunter-killer groups in Narragansett Bay, Rhode Island, and off Bermuda. She rounded out the year visiting several east coast Navy bases, a battery of torpedo firing tests, and standardization trials. The following year, Nautilus operated~out of Naval Submarine Base New London, Connecticut, where the effects of a submarine with increased speed and endurance were tested on contemporary anti-submarine warfare practices. The study found that anti-submarine practices, such as was used during World War II, were ineffective against a submarine which did not need to surface, could dive deeper, and could clear a search area in record time. In between testing, Nautilus conducted press tours and hosted several dignitaries from the Navy and Capitol Hill. On 4 February 1957, Nautilus logged her 60,000th nautical mile. It also marked another first for the boat, as the submarine was put into the Electric Boat Company Division of General Dynamics Corporation at Groton to replace the nuclear fuel core in her Westinghouse Electric submarine thermal reactor.~In early April, Nautilus operated off Bermuda with USS Seawolf (SSN-575)—the second nuclear powered submarine—before departing for the U.S. west coast on 15 May. While there, Nautilus participated in multiple exercises designed to acquaint the units of the Pacific Fleet with the capabilities of nuclear submarines. She returned to New London on 21 July. On 19 August, Nautilus departed New London for her first voyage under the Arctic polar ice pack. The 1,383 mile journey was significant, because previously U.S. submarines did not travel to the frozen northern oceans due to~diesel-electric boats could not travel freely under ice. The opening of the Arctic to Navy submarines allowed access to the previously protected waters of the Soviet Union. From the Arctic, Nautilus set sail for the eastern Atlantic to participate in NATO exercises off Norway and to visit various British and French ports. Nautilus returned to New London on 28 October where she underwent upkeep. On 25 April 1958, Nautilus was once again headed for the U.S. west coast where she made stops in San Diego, San Francisco, and Seattle. On 9 June, Nautilus departed Seattle to conduct the highly secret “Operation Sunshine,” a fully submerged transit under the North Pole. However, the first attempt was blocked by drift ice in the relatively shallow waters of the Chukchi Sea, and the submarine returned to Pearl Harbor. Her second attempt, begun on 23 July, proved successful.~Nautilus~submerged in the Barrow Sea on 1 August, transited the geographic North Pole on 3 August, and, after running submerged an additional 96 hours, surfaced off Greenland on 7 August. The commanding officer, Commander William R. Anderson, and the crew were subsequently personally congratulated by President Dwight D. Eisenhower and awarded the Presidential Unit Citation. Following fleet exercises in early 1959, Nautilus entered Portsmouth Naval Shipyard for her first complete overhaul. Updates~included the second replacement of the reactor core, overhaul of almost all machinery, new sensors, and other equipment. On 24 October 1960, Nautilus departed Portsmouth for her first deployment with Sixth Fleet in the Mediterranean. Although the deployment was relatively short, she managed to visit Rota, Spain; Valleta, Malta; and La Spezia, Italy. She returned to her homeport of New London on 16 December. By 1961, the Navy had about a dozen nuclear powered submarines in service. Nautilus continued to focus on evaluation tests for anti-submarine warfare improvements and various NATO exercises in the Atlantic. The pattern was broken in the fall of 1962, when Nautilus participated in the quarantine of Cuba during the Cuban Missile Crisis. In August 1963, Nautilus headed east again for a two month Mediterranean tour before returning to Portsmouth for an extensive overhaul. The overhaul took 27 months to complete. The submarine returned to homeport on 2 May 1966. ~Over the next six years, Nautilus participated in several fleet exercises while steaming more than 200,000 miles. In the spring of 1966, she again entered the record books when she logged her 300,000th mile underway. During the following 12 years, Nautilus was involved in a variety of developmental testing programs while continuing to serve alongside many of the more modern nuclear powered submarines she had preceded. On 9 April 1979,~Nautilus~departed Groton, on her final underway, steaming south to the Panama Canal via Guantanamo Bay and Cartagena, Columbia. From there, she cruised north and reached Mare Island Naval Shipyard, Vallejo, California, on 26 May, to begin inactivation procedures.~The ground breaking submarine~decommissioned on 3 March 1980. In recognition of her pioneering role in the practical use of nuclear power,~Nautilus~was designated a National Historic Landmark by the Secretary of the Interior on 20 May 1982. Following an extensive historic ship conversion at Mare Island, the submarine was towed to Groton, arriving on 6 July 1985. There, on 11 April 1986, 86 years to the day after the establishment of the U.S. Submarine Force, historic ship~Nautilus~and the Submarine Force Museum opened to the public as the first exhibit of its kind in the world. The unique museum ship continues to serve as a dramatic link in both Cold War-era history and the birth of the nuclear age. In October 2021, Nautilus is scheduled to receive \$36 million in upgrades to include: full blast and paint of all exterior; repairs to her superstructure; full topside decking repairs; all internal/external tanks inspected, repaired, and preserved; lighting and electrical distribution upgrades; and enhanced access to certain areas for staff members. The objective of the work is to give Nautilus 30 years of availability to the public to continue to tell her stories of the bold and courageous Sailors of U.S. submarine force. The work is scheduled to be complete in the summer of 2022. ***** Suggested Reading The Nuclear Navy Submarine Force Polar Exploration A Brief History of U.S. Navy Fleet Ballistic Missiles and Submarines The U.S. Navy in the Cold War Era,~1945–1991 Conflict and Cooperation: The U.S. and Soviet Navies in the Cold War Nuclear Navy and USS Nautilus Celebrate 60th Anniversary USS Nautilus (SSN-571) Deck Log Book—July 1958 USS Nautilus (SSN-571) Deck Log Book—August 1958 Art Exhibit A View from the Periscope Interviews with USS Nautilus (SSN-571) crewmembers Albert O. Howard Jimmy Hayes Infographic},
  langid = {american},
  file = {C:\Users\chsey\Zotero\storage\H8DXSJS3\uss-nautilus.html}
}

@online{u.s.navyNuclearNavy,
  title = {The {{Nuclear Navy}}},
  author = {U.S.NAVY},
  url = {https://www.history.navy.mil/content/history/nhhc/browse-by-topic/exploration-and-innovation/nuclear-navy.html},
  urldate = {2023-12-28},
  abstract = {The Nuclear Navy is a term coined to describe vessels powered by nuclear reactors. Incorporating nuclear energy to naval vessels revolutionized naval warfare. The general idea of nuclear ships was that they would not have to make regular stops for fuel like conventional vessels, making them only limited by supplies and crew endurance. The Navy recognized the benefits of nuclear energy for propulsion purposes and began research. From its humble beginnings, the Navy has produced many of the world’s first nuclear propelled vessels, from aircraft carriers to submarines. Shortly after World War II, the Navy sought to develop secondary uses for nuclear energy and reactors. Navy Captain Hyman Rickover, an electrical engineer and proponent of the research, sought to use nuclear reactors for the production of electricity. Rickover led the effort to pursue and manufacture the first nuclear-powered submarine,~USS~Nautilus~(SSN-571). In June 1952, construction began on~Nautilus~and on 17 January 1955~Nautilus~became the first submarine underway on nuclear power.~Nautilus~would later become the first to complete a fully submerged transit under the North Pole as part of “Operation Sunshine.” After the success of~Nautilus, research into nuclear powered surface vessels began. Construction began in 1954 on the first nuclear-powered aircraft carrier,~USS~Enterprise~(CVN-65), and the ship was commissioned 25 November 1961.~Enterprise~would go on to complete 25 deployments during its 51 years of service. Today, all submarines and aircraft carriers are powered by nuclear propulsion. The~Naval Nuclear Power Training Command~in Goose Creek, South Carolina, trains today’s nuclear operators. *****},
  langid = {american},
  file = {C:\Users\chsey\Zotero\storage\MJL3P2N5\nuclear-navy.html}
}

@online{u.s.navyRickoverHyman,
  title = {Rickover, {{Hyman G}}.},
  author = {U.S.NAVY},
  url = {http://public1.nhhcaws.local/research/library/research-guides/modern-biographical-files-ndl/modern-bios-r/rickover-hyman-g.html},
  urldate = {2023-12-29},
  abstract = {Admiral Hyman G. Rickover, the father of the nuclear Navy, was born in Makow, Poland (then part of the Russian Empire), on 27 January 1900. At the age of 6, he came to the United States, settling in Chicago. Rickover entered the U.S. Naval Academy in 1918 and was commissioned an ensign in June 1922. Following sea duty aboard the destroyer USS La Vallette (DD-315) and the battleship USS Nevada (BB-36), he attended Columbia University, where he earned a master of science degree in electrical engineering. From 1929 to 1933, Rickover qualified for submarine duty and command aboard the submarines USS S-9 (SS-114) and USS S- 48 (SS-159). In June 1937, he assumed command of the minesweeper USS Finch (AM-9). Later that year, he was selected as an engineering duty officer and spent the remainder of his career serving in that specialty. During World War II, Admiral Rickover served as head of the Electrical Section of the Bureau of Ships and later as commanding officer of Naval Repair Base, Okinawa. In 1946, he was assigned to the U.S. Atomic Energy Commission (AEC) Laboratory at Oak Ridge, Tennessee, and, in early 1949, to the Division of Reactor Development, AEC. As director of the Naval Reactors Branch, Admiral Rickover developed the world's first nuclear-powered submarine, USS Nautilus (SSN-571), which went to sea in 1955. In the years that followed, Admiral Rickover directed all aspects of building and operating the nuclear fleet. Admiral Rickover's numerous medals and decorations include the Distinguished Service Medal, Legion of Merit, Navy Commendation Medal, and the World War II Victory Medal. In recognition of his wartime service, he was made Honorary Commander of the Military Division of the Most Excellent Order of the British Empire. Admiral Rickover was twice awarded the Congressional Gold Medal for exceptional public service. In 1980, President Jimmy Carter presented Admiral Rickover with the Presidential Medal of Freedom, the nation's highest non-military honor, for his contributions to world peace. Admiral Rickover retired from the United States Navy on 31 January 1982, after more than 63 years of service to his country and to 13 Presidents. His name is memorialized in Rickover Hall at the Naval Academy, and two attack submarines, the now-decommissioned USS Hyman G.~Rickover (SSN-709) and Pre-Commissioning Unit Hyman G. Rickover (SSN-795). Admiral Rickover died on 8 July 1986 and is buried at Arlington National Cemetery. The engineering honor society Tau Beta Pi named Admiral Rickover as one of the “Top Ten Engineers of the Twentieth Century” in December 1999.},
  langid = {american},
  file = {C:\Users\chsey\Zotero\storage\LCB4HIPF\rickover-hyman-g.html}
}

@online{u.s.navyStrategicDeterrence,
  title = {Strategic {{Deterrence}}},
  author = {U.S.NAVY},
  url = {https://www.history.navy.mil/browse-by-topic/wars-conflicts-and-operations/cold-war/strategic-deterrence.html},
  urldate = {2023-12-28},
  abstract = {The goal of strategic deterrence is to dissuade adversaries from launching a nuclear attack. The U.S. Navy’s submarine-launched ballistic missiles (SLBMs) play a key role in the strategic deterrence mission by providing the U.S. with a second-strike capability. Hidden at sea on nuclear-powered ballistic missile submarines (SSBNs), SLBMs can survive an initial nuclear attack and launch in retaliation. This guaranteed retaliation is a powerful deterrent to opponents considering a first strike. In fact, the Navy’s SSBNs have long been recognized by the Department of Defense (DOD) as the most survivable leg of the United States’ nuclear triad, also composed of strategic bombers and land-based intercontinental ballistic missiles. During the Cold War, the U.S. Navy rapidly developed the Navy’s first SLBM, the Polaris A1 missile, in response to the Soviet Union’s accelerating nuclear program. Chief of Naval Operations Arleigh Burke paved the way for this achievement by prioritizing the development of a fleet ballistic missile for sea launch. In late 1955, Burke established the Special Projects Office dedicated to this mission and appointed Admiral William “Red” Raborn as its director. After only four years of testing and development, converted high-speed cargo ship Observation Island executed the first at-sea launch of a Polaris test missile on 27 August 1959. As the U.S. Navy engineered the Polaris missile, it also built nuclear-powered ballistic missile submarines to create a deterrent force. From 1959 to 1967, the Navy commissioned 41 SSBNs, each capable of carrying 16 Polaris missiles and operated by rotating Blue and Gold crews. Known as the 41 for Freedom submarines, these vessels comprised five classes of submarines: the Washington­-class, the Ethan Allen-class, the Lafayette-class, the James Madison-class, and the Benjamin Franklin­-class. The first of the 41 for Freedom submarines was George Washington (SSBN-598), which made history by successfully launching the first Polaris A1 missile from a submerged position on 20 June 1960. Two more generations of Polaris missiles, the A2 and A3, followed in 1962 and 1964. The successor to Polaris, the Poseidon (C3) missile, became operational on 31 March 1971, when James Madison (SSBN-627) began a deterrent patrol carrying 16 Poseidon missiles. The Poseidon missile’s greatest advancement was its multiple warheads, which could attack separate targets. Of the Navy’s 41 for Freedom submarines, 31 were converted to carry Poseidon missiles. The introduction of two new SLBMs with considerably longer ranges and payloads—the Trident I (C4) in 1979 and Trident II (D5) in 1990—transitioned the Navy through the end of the Cold War and into the era of modern strategic deterrence. Eighteen Ohio-class SSBNs, commissioned between 1981 and 1997, replaced the original 41 for Freedom SSBNs and became the largest submarines built by the U.S. Navy. However, in the 2000s the Navy converted the first four Ohio-class SSBNs to guided missile submarines (SSGNs) after the 1994 Nuclear Posture Review recommended the U.S. only needed 14 SSBNs to meet strategic deterrence needs. In addition, the DOD has permanently reduced the Ohio-class submarines’ SLBM capacity from 24 SLBMs to 20 in compliance with U.S.-Russia strategic nuclear arms control limits. As adversaries expand their nuclear capabilities, the Navy is now prioritizing the Columbia-class program: a minimum of 12 new SSBNs to replace the aging Ohio-class SSBNs. Columbia (SSBN-826), the first Columbia-class SSBN, was laid down on 1 October 2020 and is expected to become operational in 2031. ***},
  langid = {american}
}

@article{ulyanovDeepImagePrior2020,
  title = {Deep {{Image Prior}}},
  author = {Ulyanov, Dmitry and Vedaldi, Andrea and Lempitsky, Victor},
  date = {2020-07},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {128},
  number = {7},
  eprint = {1711.10925},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  pages = {1867--1888},
  issn = {0920-5691, 1573-1405},
  doi = {10.1007/s11263-020-01303-4},
  url = {http://arxiv.org/abs/1711.10925},
  urldate = {2023-07-26},
  abstract = {Deep convolutional networks have become a popular tool for image generation and restoration. Generally, their excellent performance is imputed to their ability to learn realistic image priors from a large number of example images. In this paper, we show that, on the contrary, the structure of a generator network is sufficient to capture a great deal of low-level image statistics prior to any learning. In order to do so, we show that a randomly-initialized neural network can be used as a handcrafted prior with excellent results in standard inverse problems such as denoising, super-resolution, and inpainting. Furthermore, the same prior can be used to invert deep neural representations to diagnose them, and to restore images based on flash-no flash input pairs. Apart from its diverse applications, our approach highlights the inductive bias captured by standard generator network architectures. It also bridges the gap between two very popular families of image restoration methods: learning-based methods using deep convolutional networks and learning-free methods based on handcrafted image priors such as self-similarity. Code and supplementary material are available at https://dmitryulyanov.github.io/deep\_image\_prior .},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Ulyanov et al_2020_Deep Image Prior.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ENFQJYWR\\1711.html}
}

@inproceedings{umriDetectionCovid19Chest2020,
  title = {Detection of {{Covid-19}} in {{Chest X-ray Image}} Using {{CLAHE}} and {{Convolutional Neural Network}}},
  booktitle = {2020 2nd {{International Conference}} on {{Cybernetics}} and {{Intelligent System}} ({{ICORIS}})},
  author = {Umri, Buyut Khoirul and Wafa Akhyari, Muhammad and Kusrini, Kusrini},
  date = {2020-10},
  pages = {1--5},
  doi = {10.1109/ICORIS50180.2020.9320806},
  abstract = {In 2019, the COVID-19 virus has spread to various parts of the world including Indonesia. This global pandemic becomes a lethal outbreak since there is no vaccine to treat or prevent transmission of the virus. Rapid Test is selected as an essential method to detect Covid-19 in Indonesia because the price is fairly cheap compared to the SWAB test. The increase in Covid-19 patients tends to lead to limited capacity for the Covid-19 test available at the hospital so that the latest technology to detect and overcome this pandemic issue is needed. Thus, the present research aims to examine the total of 100 X-Ray chest images of the Covid-19 patients and 100 X-ray normal chest images. The application of Contrast Limited Adaptive Histogram Equalization (CLAHE) and Convolutional Neural Networks (CNN) methods are implemented to analyze the dataset with two scenarios in obtaining the detection results. The results of this research reveal that the application of CLAHE is likely to affect Covid-19 detection accuracy using CNN. Also, the application of the CNN basic model shows significant results compared to the application of VGG16 transfer learning.},
  eventtitle = {2020 2nd {{International Conference}} on {{Cybernetics}} and {{Intelligent System}} ({{ICORIS}})},
  keywords = {Adaptation models,Chest X-ray,CLAHE,CNN,Convolutional neural networks,Covid-19,COVID-19,Detection,Histograms,Lung,Viruses (medical),X-ray imaging},
  file = {Y\:\\paper\\2022 summer intern\\assignment\\data augmentation\\pre-processing\\Umri et al_2020_Detection of Covid-19 in Chest X-ray Image using CLAHE and Convolutional Neural.pdf;C\:\\Users\\chsey\\Zotero\\storage\\F6RDES24\\9320806.html}
}

@online{UnilmBeit3README,
  title = {Unilm/Beit3/{{README}}.Md at Master · Microsoft/Unilm},
  url = {https://github.com/microsoft/unilm/blob/master/beit3/README.md},
  urldate = {2024-02-06},
  abstract = {Large-scale Self-supervised Pre-training Across Tasks, Languages, and Modalities - microsoft/unilm},
  langid = {english},
  organization = {GitHub}
}

@online{vasilisHowTrainStateOfTheArt,
  title = {How to {{Train State-Of-The-Art Models Using TorchVision}}’s {{Latest Primitives}}},
  author = {Vasilis, Vryniotis},
  url = {https://pytorch.org/blog/how-to-train-state-of-the-art-models-using-torchvision-latest-primitives/},
  urldate = {2022-11-18},
  langid = {english},
  organization = {pytorch},
  file = {C:\Users\chsey\Zotero\storage\ZEQBWL65\how-to-train-state-of-the-art-models-using-torchvision-latest-primitives.html}
}

@online{vaswaniAttentionAllYou2017,
  title = {Attention {{Is All You Need}}},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, Lukasz and Polosukhin, Illia},
  date = {2017-12-05},
  eprint = {1706.03762},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.03762},
  url = {http://arxiv.org/abs/1706.03762},
  urldate = {2022-08-10},
  abstract = {The dominant sequence transduction models are based on complex recurrent or convolutional neural networks in an encoder-decoder configuration. The best performing models also connect the encoder and decoder through an attention mechanism. We propose a new simple network architecture, the Transformer, based solely on attention mechanisms, dispensing with recurrence and convolutions entirely. Experiments on two machine translation tasks show these models to be superior in quality while being more parallelizable and requiring significantly less time to train. Our model achieves 28.4 BLEU on the WMT 2014 English-to-German translation task, improving over the existing best results, including ensembles by over 2 BLEU. On the WMT 2014 English-to-French translation task, our model establishes a new single-model state-of-the-art BLEU score of 41.8 after training for 3.5 days on eight GPUs, a small fraction of the training costs of the best models from the literature. We show that the Transformer generalizes well to other tasks by applying it successfully to English constituency parsing both with large and limited training data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Vaswani et al_2017_Attention Is All You Need.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MMRIU89S\\1706.html}
}

@online{vaswaniAttentionAllYou2017a,
  title = {Attention {{Is All You Need}}},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, Lukasz and Polosukhin, Illia},
  date = {2017-12-05},
  eprint = {1706.03762},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.03762},
  url = {http://arxiv.org/abs/1706.03762},
  urldate = {2023-07-18},
  abstract = {The dominant sequence transduction models are based on complex recurrent or convolutional neural networks in an encoder-decoder configuration. The best performing models also connect the encoder and decoder through an attention mechanism. We propose a new simple network architecture, the Transformer, based solely on attention mechanisms, dispensing with recurrence and convolutions entirely. Experiments on two machine translation tasks show these models to be superior in quality while being more parallelizable and requiring significantly less time to train. Our model achieves 28.4 BLEU on the WMT 2014 English-to-German translation task, improving over the existing best results, including ensembles by over 2 BLEU. On the WMT 2014 English-to-French translation task, our model establishes a new single-model state-of-the-art BLEU score of 41.8 after training for 3.5 days on eight GPUs, a small fraction of the training costs of the best models from the literature. We show that the Transformer generalizes well to other tasks by applying it successfully to English constituency parsing both with large and limited training data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Vaswani et al_2017_Attention Is All You Need2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SZJHTPNK\\1706.html}
}

@inproceedings{vaswaniAttentionAllYou2017b,
  title = {Attention Is {{All}} You {{Need}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, Łukasz and Polosukhin, Illia},
  date = {2017},
  volume = {30},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper_files/paper/2017/hash/3f5ee243547dee91fbd053c1c4a845aa-Abstract.html},
  urldate = {2023-05-28},
  abstract = {The dominant sequence transduction models are based on complex recurrent orconvolutional neural networks in an encoder and decoder configuration. The best performing such models also connect the encoder and decoder through an attentionm echanisms.  We propose a novel, simple network architecture based solely onan attention mechanism, dispensing with recurrence and convolutions entirely.Experiments on two machine translation tasks show these models to be superiorin quality while being more parallelizable and requiring significantly less timeto train. Our single model with 165 million parameters, achieves 27.5 BLEU onEnglish-to-German translation, improving over the existing best ensemble result by over 1 BLEU. On English-to-French translation, we outperform the previoussingle state-of-the-art with model by 0.7 BLEU, achieving a BLEU score of 41.1.},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Vaswani et al_2017_Attention is All you Need.pdf}
}

@online{vaswaniAttentionAllYou2017c,
  title = {Attention {{Is All You Need}}},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, Lukasz and Polosukhin, Illia},
  date = {2017-12-05},
  eprint = {1706.03762},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.03762},
  url = {http://arxiv.org/abs/1706.03762},
  urldate = {2022-07-04},
  abstract = {The dominant sequence transduction models are based on complex recurrent or convolutional neural networks in an encoder-decoder configuration. The best performing models also connect the encoder and decoder through an attention mechanism. We propose a new simple network architecture, the Transformer, based solely on attention mechanisms, dispensing with recurrence and convolutions entirely. Experiments on two machine translation tasks show these models to be superior in quality while being more parallelizable and requiring significantly less time to train. Our model achieves 28.4 BLEU on the WMT 2014 English-to-German translation task, improving over the existing best results, including ensembles by over 2 BLEU. On the WMT 2014 English-to-French translation task, our model establishes a new single-model state-of-the-art BLEU score of 41.8 after training for 3.5 days on eight GPUs, a small fraction of the training costs of the best models from the literature. We show that the Transformer generalizes well to other tasks by applying it successfully to English constituency parsing both with large and limited training data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\transformer\\Vaswani et al_2017_Attention Is All You Need.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LUNPHQYF\\1706.html}
}

@online{vaswaniAttentionAllYou2023,
  title = {Attention {{Is All You Need}}},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, Lukasz and Polosukhin, Illia},
  date = {2023-08-01},
  eprint = {1706.03762},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1706.03762},
  url = {http://arxiv.org/abs/1706.03762},
  urldate = {2023-11-17},
  abstract = {The dominant sequence transduction models are based on complex recurrent or convolutional neural networks in an encoder-decoder configuration. The best performing models also connect the encoder and decoder through an attention mechanism. We propose a new simple network architecture, the Transformer, based solely on attention mechanisms, dispensing with recurrence and convolutions entirely. Experiments on two machine translation tasks show these models to be superior in quality while being more parallelizable and requiring significantly less time to train. Our model achieves 28.4 BLEU on the WMT 2014 English-to-German translation task, improving over the existing best results, including ensembles by over 2 BLEU. On the WMT 2014 English-to-French translation task, our model establishes a new single-model state-of-the-art BLEU score of 41.8 after training for 3.5 days on eight GPUs, a small fraction of the training costs of the best models from the literature. We show that the Transformer generalizes well to other tasks by applying it successfully to English constituency parsing both with large and limited training data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Vaswani et al_2023_Attention Is All You Need.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BPYRT3XK\\1706.html}
}

@book{vedaldiComputerVisionECCV2020,
  title = {Computer {{Vision}} – {{ECCV}} 2020: 16th {{European Conference}}, {{Glasgow}}, {{UK}}, {{August}} 23–28, 2020, {{Proceedings}}, {{Part XXVII}}},
  shorttitle = {Computer {{Vision}} – {{ECCV}} 2020},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  volume = {12372},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58583-9},
  url = {https://link.springer.com/10.1007/978-3-030-58583-9},
  urldate = {2022-07-20},
  isbn = {978-3-030-58582-2 978-3-030-58583-9},
  langid = {english},
  file = {Y:\paper\Computer Vision\augmentation\Vedaldi et al_2020_Computer Vision – ECCV 2020.pdf}
}

@online{verbinRefNeRFStructuredViewDependent2021,
  title = {Ref-{{NeRF}}: {{Structured View-Dependent Appearance}} for {{Neural Radiance Fields}}},
  shorttitle = {Ref-{{NeRF}}},
  author = {Verbin, Dor and Hedman, Peter and Mildenhall, Ben and Zickler, Todd and Barron, Jonathan T. and Srinivasan, Pratul P.},
  date = {2021-12-07},
  eprint = {2112.03907},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.03907},
  urldate = {2023-01-25},
  abstract = {Neural Radiance Fields (NeRF) is a popular view synthesis technique that represents a scene as a continuous volumetric function, parameterized by multilayer perceptrons that provide the volume density and view-dependent emitted radiance at each location. While NeRF-based techniques excel at representing fine geometric structures with smoothly varying view-dependent appearance, they often fail to accurately capture and reproduce the appearance of glossy surfaces. We address this limitation by introducing Ref-NeRF, which replaces NeRF's parameterization of view-dependent outgoing radiance with a representation of reflected radiance and structures this function using a collection of spatially-varying scene properties. We show that together with a regularizer on normal vectors, our model significantly improves the realism and accuracy of specular reflections. Furthermore, we show that our model's internal representation of outgoing radiance is interpretable and useful for scene editing.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Verbin et al_2021_Ref-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JF2D3U8X\\2112.html}
}

@online{verbinRefNeRFStructuredViewDependent2021a,
  title = {Ref-{{NeRF}}: {{Structured View-Dependent Appearance}} for {{Neural Radiance Fields}}},
  shorttitle = {Ref-{{NeRF}}},
  author = {Verbin, Dor and Hedman, Peter and Mildenhall, Ben and Zickler, Todd and Barron, Jonathan T. and Srinivasan, Pratul P.},
  date = {2021-12-07},
  eprint = {2112.03907},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2112.03907},
  urldate = {2023-01-18},
  abstract = {Neural Radiance Fields (NeRF) is a popular view synthesis technique that represents a scene as a continuous volumetric function, parameterized by multilayer perceptrons that provide the volume density and view-dependent emitted radiance at each location. While NeRF-based techniques excel at representing fine geometric structures with smoothly varying view-dependent appearance, they often fail to accurately capture and reproduce the appearance of glossy surfaces. We address this limitation by introducing Ref-NeRF, which replaces NeRF's parameterization of view-dependent outgoing radiance with a representation of reflected radiance and structures this function using a collection of spatially-varying scene properties. We show that together with a regularizer on normal vectors, our model significantly improves the realism and accuracy of specular reflections. Furthermore, we show that our model's internal representation of outgoing radiance is interpretable and useful for scene editing.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,nerf reflective,연구 - 대상},
  file = {Y\:\\paper\\2022 winter intern\\Verbin et al_2021_Ref-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HC8UVBD5\\2112.html}
}

@online{Vid2SeqPretrainedVisual2023,
  title = {{{Vid2Seq}}: A Pretrained Visual Language Model for Describing Multi-Event Videos},
  shorttitle = {{{Vid2Seq}}},
  date = {2023-03-17},
  url = {https://ai.googleblog.com/2023/03/vid2seq-pretrained-visual-language.html},
  urldate = {2023-04-16},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\SAX575SG\vid2seq-pretrained-visual-language.html}
}

@inproceedings{vinyalsShowTellNeural2015,
  title = {Show and Tell: {{A}} Neural Image Caption Generator},
  shorttitle = {Show and Tell},
  booktitle = {2015 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Vinyals, Oriol and Toshev, Alexander and Bengio, Samy and Erhan, Dumitru},
  date = {2015-06},
  pages = {3156--3164},
  publisher = {IEEE},
  location = {Boston, MA, USA},
  doi = {10.1109/CVPR.2015.7298935},
  url = {http://ieeexplore.ieee.org/document/7298935/},
  urldate = {2023-05-27},
  abstract = {Automatically describing the content of an image is a fundamental problem in artificial intelligence that connects computer vision and natural language processing. In this paper, we present a generative model based on a deep recurrent architecture that combines recent advances in computer vision and machine translation and that can be used to generate natural sentences describing an image. The model is trained to maximize the likelihood of the target description sentence given the training image. Experiments on several datasets show the accuracy of the model and the fluency of the language it learns solely from image descriptions. Our model is often quite accurate, which we verify both qualitatively and quantitatively. For instance, while the current state-of-the-art BLEU-1 score (the higher the better) on the Pascal dataset is 25, our approach yields 59, to be compared to human performance around 69. We also show BLEU-1 score improvements on Flickr30k, from 56 to 66, and on SBU, from 19 to 28. Lastly, on the newly released COCO dataset, we achieve a BLEU-4 of 27.7, which is the current state-of-the-art.},
  eventtitle = {2015 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-4673-6964-0},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\FLJQUYUX\Vinyals 등 - 2015 - Show and tell A neural image caption generator.pdf}
}

@online{voraNeSFNeuralSemantic2021,
  title = {{{NeSF}}: {{Neural Semantic Fields}} for {{Generalizable Semantic Segmentation}} of {{3D Scenes}}},
  shorttitle = {{{NeSF}}},
  author = {Vora, Suhani and Radwan, Noha and Greff, Klaus and Meyer, Henning and Genova, Kyle and Sajjadi, Mehdi S. M. and Pot, Etienne and Tagliasacchi, Andrea and Duckworth, Daniel},
  date = {2021-12-02},
  eprint = {2111.13260},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.13260},
  urldate = {2023-04-09},
  abstract = {We present NeSF, a method for producing 3D semantic fields from posed RGB images alone. In place of classical 3D representations, our method builds on recent work in implicit neural scene representations wherein 3D structure is captured by point-wise functions. We leverage this methodology to recover 3D density fields upon which we then train a 3D semantic segmentation model supervised by posed 2D semantic maps. Despite being trained on 2D signals alone, our method is able to generate 3D-consistent semantic maps from novel camera poses and can be queried at arbitrary 3D points. Notably, NeSF is compatible with any method producing a density field, and its accuracy improves as the quality of the density field improves. Our empirical analysis demonstrates comparable quality to competitive 2D and 3D semantic segmentation baselines on complex, realistically rendered synthetic scenes. Our method is the first to offer truly dense 3D scene segmentations requiring only 2D supervision for training, and does not require any semantic input for inference on novel scenes. We encourage the readers to visit the project website.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Robotics},
  file = {Y\:\\paper\\2022 winter intern\\Vora et al_2021_NeSF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GS2CFHCI\\2111.html}
}

@online{walkerPoseKnowsVideo2017,
  title = {The {{Pose Knows}}: {{Video Forecasting}} by {{Generating Pose Futures}}},
  shorttitle = {The {{Pose Knows}}},
  author = {Walker, Jacob and Marino, Kenneth and Gupta, Abhinav and Hebert, Martial},
  date = {2017-04-28},
  eprint = {1705.00053},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1705.00053},
  url = {http://arxiv.org/abs/1705.00053},
  urldate = {2023-08-05},
  abstract = {Current approaches in video forecasting attempt to generate videos directly in pixel space using Generative Adversarial Networks (GANs) or Variational Autoencoders (VAEs). However, since these approaches try to model all the structure and scene dynamics at once, in unconstrained settings they often generate uninterpretable results. Our insight is to model the forecasting problem at a higher level of abstraction. Specifically, we exploit human pose detectors as a free source of supervision and break the video forecasting problem into two discrete steps. First we explicitly model the high level structure of active objects in the scene---humans---and use a VAE to model the possible future movements of humans in the pose space. We then use the future poses generated as conditional information to a GAN to predict the future frames of the video in pixel space. By using the structured space of pose as an intermediate representation, we sidestep the problems that GANs have in generating video pixels directly. We show through quantitative and qualitative evaluation that our method outperforms state-of-the-art methods for video prediction.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\video prediction\\Walker et al_2017_The Pose Knows.pdf;C\:\\Users\\chsey\\Zotero\\storage\\6B535GR2\\1705.html}
}

@online{walkerUncertainFutureForecasting2016,
  title = {An {{Uncertain Future}}: {{Forecasting}} from {{Static Images}} Using {{Variational Autoencoders}}},
  shorttitle = {An {{Uncertain Future}}},
  author = {Walker, Jacob and Doersch, Carl and Gupta, Abhinav and Hebert, Martial},
  date = {2016-06-25},
  eprint = {1606.07873},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1606.07873},
  url = {http://arxiv.org/abs/1606.07873},
  urldate = {2023-08-05},
  abstract = {In a given scene, humans can often easily predict a set of immediate future events that might happen. However, generalized pixel-level anticipation in computer vision systems is difficult because machine learning struggles with the ambiguity inherent in predicting the future. In this paper, we focus on predicting the dense trajectory of pixels in a scene, specifically what will move in the scene, where it will travel, and how it will deform over the course of one second. We propose a conditional variational autoencoder as a solution to this problem. In this framework, direct inference from the image shapes the distribution of possible trajectories, while latent variables encode any necessary information that is not available in the image. We show that our method is able to successfully predict events in a wide variety of scenes and can produce multiple different predictions when the future is ambiguous. Our algorithm is trained on thousands of diverse, realistic videos and requires absolutely no human labeling. In addition to non-semantic action prediction, we find that our method learns a representation that is applicable to semantic vision tasks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\video prediction\\Walker et al_2016_An Uncertain Future.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MY6F6LZC\\1606.html}
}

@online{walkeThereCaseDiesels2018,
  title = {There's a {{Case}} for {{Diesels}}},
  author = {Walke, Michael and Krusz, Austin},
  date = {2018-06-01T00:00:00-0400},
  url = {https://www.usni.org/magazines/proceedings/2018/june/theres-case-diesels},
  urldate = {2023-12-28},
  abstract = {Since the USS Nautilus (SSN-571) set sail in 1954, nuclear power has been the defining characteristic of the U.S. Navy’s undersea dominance. The performance advantages of nuclear submarines over conventional, diesel-electric submarines are considerable, however force structure, procurement, and fiscal sustainability have created challenges for total reliance on nuclear power. Meanwhile, rapid strategic and technological changes, such as the shift to littoral conflict or the extreme stealth of air independent propulsion (AIP) submarines, have eroded the nuclear advantage. The U.S. Navy would do well to consider augmenting its current submarine force with quiet, inexpensive, and highly capable diesel-electric submarines.},
  langid = {english},
  organization = {U.S. Naval Institute},
  file = {C:\Users\chsey\Zotero\storage\B5R3BY22\theres-case-diesels.html}
}

@online{wangActionsTransformations2016,
  title = {Actions \textasciitilde{} {{Transformations}}},
  author = {Wang, Xiaolong and Farhadi, Ali and Gupta, Abhinav},
  date = {2016-07-26},
  eprint = {1512.00795},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1512.00795},
  url = {http://arxiv.org/abs/1512.00795},
  urldate = {2023-08-05},
  abstract = {What defines an action like "kicking ball"? We argue that the true meaning of an action lies in the change or transformation an action brings to the environment. In this paper, we propose a novel representation for actions by modeling an action as a transformation which changes the state of the environment before the action happens (precondition) to the state after the action (effect). Motivated by recent advancements of video representation using deep learning, we design a Siamese network which models the action as a transformation on a high-level feature space. We show that our model gives improvements on standard action recognition datasets including UCF101 and HMDB51. More importantly, our approach is able to generalize beyond learned action categories and shows significant performance improvement on cross-category generalization on our new ACT dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Wang et al_2016_Actions ~ Transformations.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XGCQJIPS\\1512.html}
}

@inproceedings{wangExploringContextVisual2019,
  title = {Exploring {{Context}} and {{Visual Pattern}} of {{Relationship}} for {{Scene Graph Generation}}},
  booktitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Wang, Wenbin and Wang, Ruiping and Shan, Shiguang and Chen, Xilin},
  date = {2019-06},
  pages = {8180--8189},
  publisher = {IEEE},
  location = {Long Beach, CA, USA},
  doi = {10.1109/CVPR.2019.00838},
  url = {https://ieeexplore.ieee.org/document/8953893/},
  urldate = {2023-05-30},
  abstract = {Relationship is the core of scene graph, but its prediction is far from satisfying because of its complex visual diversity. To alleviate this problem, we treat relationship as an abstract object, exploring not only significative visual pattern but contextual information for it, which are two key aspects when considering object recognition. Our observation on current datasets reveals that there exists intimate association among relationships. Therefore, inspired by the successful application of context to object-oriented tasks, we especially construct context for relationships where all of them are gathered so that the recognition could benefit from their association. Moreover, accurate recognition needs discriminative visual pattern for object, and so does relationship. In order to discover effective pattern for relationship, traditional relationship feature extraction methods such as using union region or combination of subject-object feature pairs are replaced with our proposed intersection region which focuses on more essential parts. Therefore, we present our so-called Relationship Context - InterSeCtion Region (CISC) method. Experiments for scene graph generation on Visual Genome dataset and visual relationship prediction on VRD dataset indicate that both the relationship context and intersection region improve performances and realize anticipated functions.},
  eventtitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-72813-293-8},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\FSD32RHJ\Wang 등 - 2019 - Exploring Context and Visual Pattern of Relationsh.pdf}
}

@online{wangFoundationTransformers2022,
  title = {Foundation {{Transformers}}},
  author = {Wang, Hongyu and Ma, Shuming and Huang, Shaohan and Dong, Li and Wang, Wenhui and Peng, Zhiliang and Wu, Yu and Bajaj, Payal and Singhal, Saksham and Benhaim, Alon and Patra, Barun and Liu, Zhun and Chaudhary, Vishrav and Song, Xia and Wei, Furu},
  date = {2022-10-19},
  eprint = {2210.06423},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2210.06423},
  urldate = {2024-02-08},
  abstract = {A big convergence of model architectures across language, vision, speech, and multimodal is emerging. However, under the same name "Transformers", the above areas use different implementations for better performance, e.g., Post-LayerNorm for BERT, and Pre-LayerNorm for GPT and vision Transformers. We call for the development of Foundation Transformer for true general-purpose modeling, which serves as a go-to architecture for various tasks and modalities with guaranteed training stability. In this work, we introduce a Transformer variant, named Magneto, to fulfill the goal. Specifically, we propose Sub-LayerNorm for good expressivity, and the initialization strategy theoretically derived from DeepNet for stable scaling up. Extensive experiments demonstrate its superior performance and better stability than the de facto Transformer variants designed for various applications, including language modeling (i.e., BERT, and GPT), machine translation, vision pretraining (i.e., BEiT), speech recognition, and multimodal pretraining (i.e., BEiT-3).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2022_Foundation Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WJ3TS4XD\\2210.html}
}

@online{wangFrustratinglySimpleFewShot2020,
  title = {Frustratingly {{Simple Few-Shot Object Detection}}},
  author = {Wang, Xin and Huang, Thomas E. and Darrell, Trevor and Gonzalez, Joseph E. and Yu, Fisher},
  date = {2020-03-15},
  eprint = {2003.06957},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2003.06957},
  url = {http://arxiv.org/abs/2003.06957},
  urldate = {2023-11-23},
  abstract = {Detecting rare objects from a few examples is an emerging problem. Prior works show meta-learning is a promising approach. But, fine-tuning techniques have drawn scant attention. We find that fine-tuning only the last layer of existing detectors on rare classes is crucial to the few-shot object detection task. Such a simple approach outperforms the meta-learning methods by roughly 2\textasciitilde 20 points on current benchmarks and sometimes even doubles the accuracy of the prior methods. However, the high variance in the few samples often leads to the unreliability of existing benchmarks. We revise the evaluation protocols by sampling multiple groups of training examples to obtain stable comparisons and build new benchmarks based on three datasets: PASCAL VOC, COCO and LVIS. Again, our fine-tuning approach establishes a new state of the art on the revised benchmarks. The code as well as the pretrained models are available at https://github.com/ucbdrive/few-shot-object-detection.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\few shot dense\\Wang et al_2020_Frustratingly Simple Few-Shot Object Detection.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3D7IQJGB\\2003.html}
}

@online{wangGLUEMultiTaskBenchmark2019,
  title = {{{GLUE}}: {{A Multi-Task Benchmark}} and {{Analysis Platform}} for {{Natural Language Understanding}}},
  shorttitle = {{{GLUE}}},
  author = {Wang, Alex and Singh, Amanpreet and Michael, Julian and Hill, Felix and Levy, Omer and Bowman, Samuel R.},
  date = {2019-02-22},
  eprint = {1804.07461},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1804.07461},
  urldate = {2024-02-27},
  abstract = {For natural language understanding (NLU) technology to be maximally useful, both practically and as a scientific object of study, it must be general: it must be able to process language in a way that is not exclusively tailored to any one specific task or dataset. In pursuit of this objective, we introduce the General Language Understanding Evaluation benchmark (GLUE), a tool for evaluating and analyzing the performance of models across a diverse range of existing NLU tasks. GLUE is model-agnostic, but it incentivizes sharing knowledge across tasks because certain tasks have very limited training data. We further provide a hand-crafted diagnostic test suite that enables detailed linguistic analysis of NLU models. We evaluate baselines based on current methods for multi-task and transfer learning and find that they do not immediately give substantial improvements over the aggregate performance of training a separate model per task, indicating room for improvement in developing general and robust NLU systems.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language},
  file = {Y\:\\paper\\2024_research\\Wang et al_2019_GLUE.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LWSAMF4W\\1804.html}
}

@inproceedings{wangHurricaneSandyTwitter2015,
  title = {The {{Hurricane Sandy Twitter Corpus}}},
  author = {Wang, Haoyu and Hovy, E. and Dredze, Mark},
  date = {2015},
  url = {https://www.semanticscholar.org/paper/The-Hurricane-Sandy-Twitter-Corpus-Wang-Hovy/bf7f220a2908268a7a1c432a2c2efd81afed6808},
  urldate = {2023-05-27},
  abstract = {The growing use of social media has made it a critical component of disaster response and recovery efforts. Both in terms of preparedness and response, public health officials and first responders have turned to automated tools to assist with organizing and visualizing large streams of social media. In turn, this has spurred new research into algorithms for information extraction, event detection and organization, and information visualization. One challenge of these efforts has been the lack of a common corpus for disaster response on which researchers can compare and contrast their work. This paper describes the Hurricane Sandy Twitter Corpus: 6.5 million geotagged Twitter posts from the geographic area and time period of the 2012 Hurricane Sandy.},
  eventtitle = {{{AAAI Workshop}}: {{WWW}} and {{Public Health Intelligence}}}
}

@online{wangImageForeignLanguage2022,
  title = {Image as a {{Foreign Language}}: {{BEiT Pretraining}} for {{All Vision}} and {{Vision-Language Tasks}}},
  shorttitle = {Image as a {{Foreign Language}}},
  author = {Wang, Wenhui and Bao, Hangbo and Dong, Li and Bjorck, Johan and Peng, Zhiliang and Liu, Qiang and Aggarwal, Kriti and Mohammed, Owais Khan and Singhal, Saksham and Som, Subhojit and Wei, Furu},
  date = {2022-08-30},
  eprint = {2208.10442},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2208.10442},
  urldate = {2024-01-30},
  abstract = {A big convergence of language, vision, and multimodal pretraining is emerging. In this work, we introduce a general-purpose multimodal foundation model BEiT-3, which achieves state-of-the-art transfer performance on both vision and vision-language tasks. Specifically, we advance the big convergence from three aspects: backbone architecture, pretraining task, and model scaling up. We introduce Multiway Transformers for general-purpose modeling, where the modular architecture enables both deep fusion and modality-specific encoding. Based on the shared backbone, we perform masked "language" modeling on images (Imglish), texts (English), and image-text pairs ("parallel sentences") in a unified manner. Experimental results show that BEiT-3 obtains state-of-the-art performance on object detection (COCO), semantic segmentation (ADE20K), image classification (ImageNet), visual reasoning (NLVR2), visual question answering (VQAv2), image captioning (COCO), and cross-modal retrieval (Flickr30K, COCO).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2024_research\\Wang et al_2022_Image as a Foreign Language.pdf;C\:\\Users\\chsey\\Zotero\\storage\\A8ZRB84E\\2208.html}
}

@online{wangImageForeignLanguage2022a,
  title = {Image as a {{Foreign Language}}: {{BEiT Pretraining}} for {{All Vision}} and {{Vision-Language Tasks}}},
  shorttitle = {Image as a {{Foreign Language}}},
  author = {Wang, Wenhui and Bao, Hangbo and Dong, Li and Bjorck, Johan and Peng, Zhiliang and Liu, Qiang and Aggarwal, Kriti and Mohammed, Owais Khan and Singhal, Saksham and Som, Subhojit and Wei, Furu},
  date = {2022-08-30},
  eprint = {2208.10442},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2208.10442},
  url = {http://arxiv.org/abs/2208.10442},
  urldate = {2023-07-03},
  abstract = {A big convergence of language, vision, and multimodal pretraining is emerging. In this work, we introduce a general-purpose multimodal foundation model BEiT-3, which achieves state-of-the-art transfer performance on both vision and vision-language tasks. Specifically, we advance the big convergence from three aspects: backbone architecture, pretraining task, and model scaling up. We introduce Multiway Transformers for general-purpose modeling, where the modular architecture enables both deep fusion and modality-specific encoding. Based on the shared backbone, we perform masked "language" modeling on images (Imglish), texts (English), and image-text pairs ("parallel sentences") in a unified manner. Experimental results show that BEiT-3 obtains state-of-the-art performance on object detection (COCO), semantic segmentation (ADE20K), image classification (ImageNet), visual reasoning (NLVR2), visual question answering (VQAv2), image captioning (COCO), and cross-modal retrieval (Flickr30K, COCO).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2022_Image as a Foreign Language2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JW8ARU5V\\2208.html}
}

@inproceedings{wangImageForeignLanguage2023,
  title = {Image as a {{Foreign Language}}: {{BEIT Pretraining}} for {{Vision}} and {{Vision-Language Tasks}}},
  shorttitle = {Image as a {{Foreign Language}}},
  booktitle = {2023 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Wang, Wenhui and Bao, Hangbo and Dong, Li and Bjorck, Johan and Peng, Zhiliang and Liu, Qiang and Aggarwal, Kriti and Mohammed, Owais Khan and Singhal, Saksham and Som, Subhojit and Wei, Furu},
  date = {2023-06},
  pages = {19175--19186},
  publisher = {IEEE},
  location = {Vancouver, BC, Canada},
  doi = {10.1109/CVPR52729.2023.01838},
  url = {https://ieeexplore.ieee.org/document/10205465/},
  urldate = {2024-02-08},
  eventtitle = {2023 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {9798350301298},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\PLYPPP4T\Wang 등 - 2023 - Image as a Foreign Language BEIT Pretraining for .pdf}
}

@online{wangImplicitBiasSGD2023,
  title = {Implicit Bias of {{SGD}} in \${{L}}\_\{2\}\$-Regularized Linear {{DNNs}}: {{One-way}} Jumps from High to Low Rank},
  shorttitle = {Implicit Bias of {{SGD}} in \${{L}}\_\{2\}\$-Regularized Linear {{DNNs}}},
  author = {Wang, Zihan and Jacot, Arthur},
  date = {2023-09-29},
  eprint = {2305.16038},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2305.16038},
  urldate = {2024-10-27},
  abstract = {The \$L\_\{2\}\$-regularized loss of Deep Linear Networks (DLNs) with more than one hidden layers has multiple local minima, corresponding to matrices with different ranks. In tasks such as matrix completion, the goal is to converge to the local minimum with the smallest rank that still fits the training data. While rank-underestimating minima can be avoided since they do not fit the data, GD might get stuck at rank-overestimating minima. We show that with SGD, there is always a probability to jump from a higher rank minimum to a lower rank one, but the probability of jumping back is zero. More precisely, we define a sequence of sets \$B\_\{1\}\textbackslash subset B\_\{2\}\textbackslash subset\textbackslash cdots\textbackslash subset B\_\{R\}\$ so that \$B\_\{r\}\$ contains all minima of rank \$r\$ or less (and not more) that are absorbing for small enough ridge parameters \$\textbackslash lambda\$ and learning rates \$\textbackslash eta\$: SGD has prob. 0 of leaving \$B\_\{r\}\$, and from any starting point there is a non-zero prob. for SGD to go in \$B\_\{r\}\$.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Wang_Jacot_2023_Implicit bias of SGD in $L_ 2 $-regularized linear DNNs.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LG9KG2UF\\2305.html}
}

@inproceedings{wangImprovingZeroShotGeneralization2023,
  title = {Improving {{Zero-Shot Generalization}} for {{CLIP}} with {{Synthesized Prompts}}},
  author = {Wang, Zhengbo and Liang, Jian and He, Ran and Xu, Nan and Wang, Zilei and Tan, Tieniu},
  date = {2023},
  pages = {3032--3042},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Wang_Improving_Zero-Shot_Generalization_for_CLIP_with_Synthesized_Prompts_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Wang et al_2023_Improving Zero-Shot Generalization for CLIP with Synthesized Prompts.pdf}
}

@online{wangLearningRobustGlobal2019,
  title = {Learning {{Robust Global Representations}} by {{Penalizing Local Predictive Power}}},
  author = {Wang, Haohan and Ge, Songwei and Xing, Eric P. and Lipton, Zachary C.},
  date = {2019-11-04},
  eprint = {1905.13549},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1905.13549},
  url = {http://arxiv.org/abs/1905.13549},
  urldate = {2023-11-14},
  abstract = {Despite their renowned predictive power on i.i.d. data, convolutional neural networks are known to rely more on high-frequency patterns that humans deem superficial than on low-frequency patterns that agree better with intuitions about what constitutes category membership. This paper proposes a method for training robust convolutional networks by penalizing the predictive power of the local representations learned by earlier layers. Intuitively, our networks are forced to discard predictive signals such as color and texture that can be gleaned from local receptive fields and to rely instead on the global structures of the image. Across a battery of synthetic and benchmark domain adaptation tasks, our method confers improved generalization out of the domain. Also, to evaluate cross-domain transfer, we introduce ImageNet-Sketch, a new dataset consisting of sketch-like images, that matches the ImageNet classification validation set in categories and scale.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Wang et al_2019_Learning Robust Global Representations by Penalizing Local Predictive Power.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9B37MYVB\\1905.html}
}

@article{wangLowrankMatrixRecovery2021,
  title = {Low-Rank Matrix Recovery via Regularized Nuclear Norm Minimization},
  author = {Wang, Wendong and Zhang, Feng and Wang, Jianjun},
  date = {2021-09-01},
  journaltitle = {Applied and Computational Harmonic Analysis},
  shortjournal = {Applied and Computational Harmonic Analysis},
  volume = {54},
  pages = {1--19},
  issn = {1063-5203},
  doi = {10.1016/j.acha.2021.03.001},
  url = {https://www.sciencedirect.com/science/article/pii/S1063520321000208},
  urldate = {2024-04-11},
  abstract = {In this paper, we theoretically investigate the low-rank matrix recovery problem in the context of the unconstrained regularized nuclear norm minimization (RNNM) framework. Our theoretical findings show that, the RNNM method is able to provide a robust recovery of any matrix X (not necessary to be exactly low-rank) from its few noisy measurements b=A(X)+n with a bounded constraint ‖n‖2≤ϵ, provided that the tk-order restricted isometry constant (RIC) of A satisfies a certain constraint related to t{$>$}0. Specifically, the obtained recovery condition in the case of t{$>$}4/3 is found to be same with the sharp condition established previously by Cai and Zhang [10] to guarantee the exact recovery of any rank-k matrix via the constrained nuclear norm minimization method. More importantly, to the best of our knowledge, we are the first to establish the tk-order RIC based coefficient estimate of the robust null space property in the case of 0},
  keywords = {Low-rank matrix recovery,notion,Regularized nuclear norm minimization,Restricted isometry property,Robust null space property},
  file = {Y\:\\paper\\2024_research\\Wang et al_2021_Low-rank matrix recovery via regularized nuclear norm minimization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QNWL2GQ2\\S1063520321000208.html}
}

@online{wangLowShotLearningImaginary2018,
  title = {Low-{{Shot Learning}} from {{Imaginary Data}}},
  author = {Wang, Yu-Xiong and Girshick, Ross and Hebert, Martial and Hariharan, Bharath},
  date = {2018-04-02},
  eprint = {1801.05401},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1801.05401},
  url = {http://arxiv.org/abs/1801.05401},
  urldate = {2023-08-05},
  abstract = {Humans can quickly learn new visual concepts, perhaps because they can easily visualize or imagine what novel objects look like from different views. Incorporating this ability to hallucinate novel instances of new concepts might help machine vision systems perform better low-shot learning, i.e., learning concepts from few examples. We present a novel approach to low-shot learning that uses this idea. Our approach builds on recent progress in meta-learning ("learning to learn") by combining a meta-learner with a "hallucinator" that produces additional training examples, and optimizing both models jointly. Our hallucinator can be incorporated into a variety of meta-learners and provides significant gains: up to a 6 point boost in classification accuracy when only a single training example is available, yielding state-of-the-art performance on the challenging ImageNet low-shot classification benchmark.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\few shot learning\\Wang et al_2018_Low-Shot Learning from Imaginary Data.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PCKK9UXJ\\1801.html}
}

@online{wangLowShotLearningImaginary2018a,
  title = {Low-{{Shot Learning}} from {{Imaginary Data}}},
  author = {Wang, Yu-Xiong and Girshick, Ross and Hebert, Martial and Hariharan, Bharath},
  date = {2018-04-02},
  eprint = {1801.05401},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1801.05401},
  url = {http://arxiv.org/abs/1801.05401},
  urldate = {2023-08-05},
  abstract = {Humans can quickly learn new visual concepts, perhaps because they can easily visualize or imagine what novel objects look like from different views. Incorporating this ability to hallucinate novel instances of new concepts might help machine vision systems perform better low-shot learning, i.e., learning concepts from few examples. We present a novel approach to low-shot learning that uses this idea. Our approach builds on recent progress in meta-learning ("learning to learn") by combining a meta-learner with a "hallucinator" that produces additional training examples, and optimizing both models jointly. Our hallucinator can be incorporated into a variety of meta-learners and provides significant gains: up to a 6 point boost in classification accuracy when only a single training example is available, yielding state-of-the-art performance on the challenging ImageNet low-shot classification benchmark.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\relational reasoning\\Wang et al_2018_Low-Shot Learning from Imaginary Data.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KWNVNCZG\\1801.html}
}

@online{wangMiniLMDeepSelfAttention2020,
  title = {{{MiniLM}}: {{Deep Self-Attention Distillation}} for {{Task-Agnostic Compression}} of {{Pre-Trained Transformers}}},
  shorttitle = {{{MiniLM}}},
  author = {Wang, Wenhui and Wei, Furu and Dong, Li and Bao, Hangbo and Yang, Nan and Zhou, Ming},
  date = {2020-04-05},
  eprint = {2002.10957},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2002.10957},
  urldate = {2024-02-06},
  abstract = {Pre-trained language models (e.g., BERT (Devlin et al., 2018) and its variants) have achieved remarkable success in varieties of NLP tasks. However, these models usually consist of hundreds of millions of parameters which brings challenges for fine-tuning and online serving in real-life applications due to latency and capacity constraints. In this work, we present a simple and effective approach to compress large Transformer (Vaswani et al., 2017) based pre-trained models, termed as deep self-attention distillation. The small model (student) is trained by deeply mimicking the self-attention module, which plays a vital role in Transformer networks, of the large model (teacher). Specifically, we propose distilling the self-attention module of the last Transformer layer of the teacher, which is effective and flexible for the student. Furthermore, we introduce the scaled dot-product between values in the self-attention module as the new deep self-attention knowledge, in addition to the attention distributions (i.e., the scaled dot-product of queries and keys) that have been used in existing works. Moreover, we show that introducing a teacher assistant (Mirzadeh et al., 2019) also helps the distillation of large pre-trained Transformer models. Experimental results demonstrate that our monolingual model outperforms state-of-the-art baselines in different parameter size of student models. In particular, it retains more than 99\% accuracy on SQuAD 2.0 and several GLUE benchmark tasks using 50\% of the Transformer parameters and computations of the teacher model. We also obtain competitive results in applying deep self-attention distillation to multilingual pre-trained models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2020_MiniLM.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3Y4BVBZP\\2002.html}
}

@online{wangMiniLMv2MultiHeadSelfAttention2021,
  title = {{{MiniLMv2}}: {{Multi-Head Self-Attention Relation Distillation}} for {{Compressing Pretrained Transformers}}},
  shorttitle = {{{MiniLMv2}}},
  author = {Wang, Wenhui and Bao, Hangbo and Huang, Shaohan and Dong, Li and Wei, Furu},
  date = {2021-06-27},
  eprint = {2012.15828},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2012.15828},
  urldate = {2024-02-06},
  abstract = {We generalize deep self-attention distillation in MiniLM (Wang et al., 2020) by only using self-attention relation distillation for task-agnostic compression of pretrained Transformers. In particular, we define multi-head self-attention relations as scaled dot-product between the pairs of query, key, and value vectors within each self-attention module. Then we employ the above relational knowledge to train the student model. Besides its simplicity and unified principle, more favorably, there is no restriction in terms of the number of student's attention heads, while most previous work has to guarantee the same head number between teacher and student. Moreover, the fine-grained self-attention relations tend to fully exploit the interaction knowledge learned by Transformer. In addition, we thoroughly examine the layer selection strategy for teacher models, rather than just relying on the last layer as in MiniLM. We conduct extensive experiments on compressing both monolingual and multilingual pretrained models. Experimental results demonstrate that our models distilled from base-size and large-size teachers (BERT, RoBERTa and XLM-R) outperform the state-of-the-art.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2021_MiniLMv2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QNK42M5R\\2012.html}
}

@online{wangMultitaskPromptTuning2023,
  title = {Multitask {{Prompt Tuning Enables Parameter-Efficient Transfer Learning}}},
  author = {Wang, Zhen and Panda, Rameswar and Karlinsky, Leonid and Feris, Rogerio and Sun, Huan and Kim, Yoon},
  date = {2023-03-05},
  eprint = {2303.02861},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.02861},
  url = {http://arxiv.org/abs/2303.02861},
  urldate = {2024-09-17},
  abstract = {Prompt tuning, in which a base pretrained model is adapted to each task via conditioning on learned prompt vectors, has emerged as a promising approach for efficiently adapting large language models to multiple downstream tasks. However, existing methods typically learn soft prompt vectors from scratch, and it has not been clear how to exploit the rich cross-task knowledge with prompt vectors in a multitask learning setting. We propose multitask prompt tuning (MPT), which first learns a single transferable prompt by distilling knowledge from multiple task-specific source prompts. We then learn multiplicative low rank updates to this shared prompt to efficiently adapt it to each downstream target task. Extensive experiments on 23 NLP datasets demonstrate that our proposed approach outperforms the state-of-the-art methods, including the full finetuning baseline in some cases, despite only tuning 0.035\% as many task-specific parameters.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2023_Multitask Prompt Tuning Enables Parameter-Efficient Transfer Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EZUKJZ7J\\2303.html}
}

@online{wangNeuSLearningNeural2023,
  title = {{{NeuS}}: {{Learning Neural Implicit Surfaces}} by {{Volume Rendering}} for {{Multi-view Reconstruction}}},
  shorttitle = {{{NeuS}}},
  author = {Wang, Peng and Liu, Lingjie and Liu, Yuan and Theobalt, Christian and Komura, Taku and Wang, Wenping},
  date = {2023-02-01},
  eprint = {2106.10689},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.10689},
  urldate = {2023-04-20},
  abstract = {We present a novel neural surface reconstruction method, called NeuS, for reconstructing objects and scenes with high fidelity from 2D image inputs. Existing neural surface reconstruction approaches, such as DVR and IDR, require foreground mask as supervision, easily get trapped in local minima, and therefore struggle with the reconstruction of objects with severe self-occlusion or thin structures. Meanwhile, recent neural methods for novel view synthesis, such as NeRF and its variants, use volume rendering to produce a neural scene representation with robustness of optimization, even for highly complex objects. However, extracting high-quality surfaces from this learned implicit representation is difficult because there are not sufficient surface constraints in the representation. In NeuS, we propose to represent a surface as the zero-level set of a signed distance function (SDF) and develop a new volume rendering method to train a neural SDF representation. We observe that the conventional volume rendering method causes inherent geometric errors (i.e. bias) for surface reconstruction, and therefore propose a new formulation that is free of bias in the first order of approximation, thus leading to more accurate surface reconstruction even without the mask supervision. Experiments on the DTU dataset and the BlendedMVS dataset show that NeuS outperforms the state-of-the-arts in high-quality surface reconstruction, especially for objects and scenes with complex structures and self-occlusion.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\surface normal\\Wang et al_2023_NeuS.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MF6ASMEZ\\2106.html}
}

@online{wangNeuSLearningNeural2023a,
  title = {{{NeuS}}: {{Learning Neural Implicit Surfaces}} by {{Volume Rendering}} for {{Multi-view Reconstruction}}},
  shorttitle = {{{NeuS}}},
  author = {Wang, Peng and Liu, Lingjie and Liu, Yuan and Theobalt, Christian and Komura, Taku and Wang, Wenping},
  date = {2023-02-01},
  eprint = {2106.10689},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.10689},
  urldate = {2023-04-20},
  abstract = {We present a novel neural surface reconstruction method, called NeuS, for reconstructing objects and scenes with high fidelity from 2D image inputs. Existing neural surface reconstruction approaches, such as DVR and IDR, require foreground mask as supervision, easily get trapped in local minima, and therefore struggle with the reconstruction of objects with severe self-occlusion or thin structures. Meanwhile, recent neural methods for novel view synthesis, such as NeRF and its variants, use volume rendering to produce a neural scene representation with robustness of optimization, even for highly complex objects. However, extracting high-quality surfaces from this learned implicit representation is difficult because there are not sufficient surface constraints in the representation. In NeuS, we propose to represent a surface as the zero-level set of a signed distance function (SDF) and develop a new volume rendering method to train a neural SDF representation. We observe that the conventional volume rendering method causes inherent geometric errors (i.e. bias) for surface reconstruction, and therefore propose a new formulation that is free of bias in the first order of approximation, thus leading to more accurate surface reconstruction even without the mask supervision. Experiments on the DTU dataset and the BlendedMVS dataset show that NeuS outperforms the state-of-the-arts in high-quality surface reconstruction, especially for objects and scenes with complex structures and self-occlusion.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Wang et al_2023_NeuS.pdf;C\:\\Users\\chsey\\Zotero\\storage\\E8RNASS6\\2106.html}
}

@online{wangONEPEACEExploringOne2023,
  title = {{{ONE-PEACE}}: {{Exploring One General Representation Model Toward Unlimited Modalities}}},
  shorttitle = {{{ONE-PEACE}}},
  author = {Wang, Peng and Wang, Shijie and Lin, Junyang and Bai, Shuai and Zhou, Xiaohuan and Zhou, Jingren and Wang, Xinggang and Zhou, Chang},
  date = {2023-05-18},
  eprint = {2305.11172},
  eprinttype = {arXiv},
  eprintclass = {cs, eess},
  url = {http://arxiv.org/abs/2305.11172},
  urldate = {2024-03-13},
  abstract = {In this work, we explore a scalable way for building a general representation model toward unlimited modalities. We release ONE-PEACE, a highly extensible model with 4B parameters that can seamlessly align and integrate representations across vision, audio, and language modalities. The architecture of ONE-PEACE comprises modality adapters, shared self-attention layers, and modality FFNs. This design allows for the easy extension of new modalities by adding adapters and FFNs, while also enabling multi-modal fusion through self-attention layers. To pretrain ONE-PEACE, we develop two modality-agnostic pretraining tasks, cross-modal aligning contrast and intra-modal denoising contrast, which align the semantic space of different modalities and capture fine-grained details within modalities concurrently. With the scaling-friendly architecture and pretraining tasks, ONE-PEACE has the potential to expand to unlimited modalities. Without using any vision or language pretrained model for initialization, ONE-PEACE achieves leading results on a wide range of uni-modal and multi-modal tasks, including image classification (ImageNet), semantic segmentation (ADE20K), audio-text retrieval (AudioCaps, Clotho), audio classification (ESC-50, FSD50K, VGGSound), audio question answering (AVQA), image-text retrieval (MSCOCO, Flickr30K), and visual grounding (RefCOCO/+/g). Code is available at https://github.com/OFA-Sys/ONE-PEACE.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Sound,Electrical Engineering and Systems Science - Audio and Speech Processing,notion},
  file = {Y\:\\paper\\2024_research\\Wang et al_2023_ONE-PEACE.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ATNKHMH4\\2305.html}
}

@online{wangOntargetAdaptation2021,
  title = {On-Target {{Adaptation}}},
  author = {Wang, Dequan and Liu, Shaoteng and Ebrahimi, Sayna and Shelhamer, Evan and Darrell, Trevor},
  date = {2021-09-02},
  eprint = {2109.01087},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2109.01087},
  url = {http://arxiv.org/abs/2109.01087},
  urldate = {2024-01-09},
  abstract = {Domain adaptation seeks to mitigate the shift between training on the \textbackslash emph\{source\} domain and testing on the \textbackslash emph\{target\} domain. Most adaptation methods rely on the source data by joint optimization over source data and target data. Source-free methods replace the source data with a source model by fine-tuning it on target. Either way, the majority of the parameter updates for the model representation and the classifier are derived from the source, and not the target. However, target accuracy is the goal, and so we argue for optimizing as much as possible on the target data. We show significant improvement by on-target adaptation, which learns the representation purely from target data while taking only the source predictions for supervision. In the long-tailed classification setting, we show further improvement by on-target class distribution learning, which learns the (im)balance of classes from target data.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\Wang et al_2021_On-target Adaptation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\29ZRVFX4\\2109.html}
}

@online{wangReviewLargeVision2023,
  title = {Review of {{Large Vision Models}} and {{Visual Prompt Engineering}}},
  author = {Wang, Jiaqi and Liu, Zhengliang and Zhao, Lin and Wu, Zihao and Ma, Chong and Yu, Sigang and Dai, Haixing and Yang, Qiushi and Liu, Yiheng and Zhang, Songyao and Shi, Enze and Pan, Yi and Zhang, Tuo and Zhu, Dajiang and Li, Xiang and Jiang, Xi and Ge, Bao and Yuan, Yixuan and Shen, Dinggang and Liu, Tianming and Zhang, Shu},
  date = {2023-07-03},
  eprint = {2307.00855},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2307.00855},
  urldate = {2023-08-11},
  abstract = {Visual prompt engineering is a fundamental technology in the field of visual and image Artificial General Intelligence, serving as a key component for achieving zero-shot capabilities. As the development of large vision models progresses, the importance of prompt engineering becomes increasingly evident. Designing suitable prompts for specific visual tasks has emerged as a meaningful research direction. This review aims to summarize the methods employed in the computer vision domain for large vision models and visual prompt engineering, exploring the latest advancements in visual prompt engineering. We present influential large models in the visual domain and a range of prompt engineering methods employed on these models. It is our hope that this review provides a comprehensive and systematic description of prompt engineering methods based on large visual models, offering valuable insights for future researchers in their exploration of this field.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\prompt\\Wang et al_2023_Review of Large Vision Models and Visual Prompt Engineering.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SDRZPE8N\\2307.html}
}

@online{wangSOLOSegmentingObjects2020,
  title = {{{SOLO}}: {{Segmenting Objects}} by {{Locations}}},
  shorttitle = {{{SOLO}}},
  author = {Wang, Xinlong and Kong, Tao and Shen, Chunhua and Jiang, Yuning and Li, Lei},
  date = {2020-07-19},
  eprint = {1912.04488},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1912.04488},
  urldate = {2022-07-25},
  abstract = {We present a new, embarrassingly simple approach to instance segmentation in images. Compared to many other dense prediction tasks, e.g., semantic segmentation, it is the arbitrary number of instances that have made instance segmentation much more challenging. In order to predict a mask for each instance, mainstream approaches either follow the 'detect-thensegment' strategy as used by Mask R-CNN, or predict category masks first then use clustering techniques to group pixels into individual instances. We view the task of instance segmentation from a completely new perspective by introducing the notion of "instance categories", which assigns categories to each pixel within an instance according to the instance's location and size, thus nicely converting instance mask segmentation into a classification-solvable problem. Now instance segmentation is decomposed into two classification tasks. We demonstrate a much simpler and flexible instance segmentation framework with strong performance, achieving on par accuracy with Mask R-CNN and outperforming recent singleshot instance segmenters in accuracy. We hope that this very simple and strong framework can serve as a baseline for many instance-level recognition tasks besides instance segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\segmentation\\Wang et al_2020_SOLO.pdf;C\:\\Users\\chsey\\Zotero\\storage\\GIRL4FNW\\1912.html}
}

@inproceedings{wangSOLOv2DynamicFast2020,
  title = {{{SOLOv2}}: {{Dynamic}} and {{Fast Instance Segmentation}}},
  shorttitle = {{{SOLOv2}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Wang, Xinlong and Zhang, Rufeng and Kong, Tao and Li, Lei and Shen, Chunhua},
  date = {2020},
  volume = {33},
  pages = {17721--17732},
  publisher = {Curran Associates, Inc.},
  url = {https://proceedings.neurips.cc/paper/2020/hash/cd3afef9b8b89558cd56638c3631868a-Abstract.html},
  urldate = {2022-07-25},
  abstract = {In this work, we design a simple, direct, and fast framework for instance segmentation with strong performance. To this end, we propose a novel and effective approach, termed SOLOv2, following the principle of the SOLO method [32]. First, our new framework is empowered by an efficient and holistic instance mask representation scheme, which dynamically segments each instance in the image, without resorting to bounding box detection. Specifically, the object mask generation is decoupled into a mask kernel prediction and mask feature learning, which are responsible for generating convolution kernels and the feature maps to be convolved with, respectively. Second, SOLOv2 significantly reduces inference overhead with our novel matrix non-maximum suppression (NMS) technique. Our Matrix NMS performs NMS with parallel matrix operations in one shot, and yields better results. We demonstrate that the proposed SOLOv2 achieves the state-of-the- art performance with high efficiency, making it suitable for both mobile and cloud applications. A light-weight version of SOLOv2 executes at 31.3 FPS and yields 37.1\% AP on COCO test-dev. Moreover, our state-of-the-art results in object detection (from our mask byproduct) and panoptic segmentation show the potential of SOLOv2 to serve as a new strong baseline for many instance-level recognition tasks. Code is available at https://git.io/AdelaiDet},
  file = {Y:\paper\Computer Vision\segmentation\Wang et al_2020_SOLOv2.pdf}
}

@online{wangTentFullyTesttime2021,
  title = {Tent: {{Fully Test-time Adaptation}} by {{Entropy Minimization}}},
  shorttitle = {Tent},
  author = {Wang, Dequan and Shelhamer, Evan and Liu, Shaoteng and Olshausen, Bruno and Darrell, Trevor},
  date = {2021-03-18},
  eprint = {2006.10726},
  eprinttype = {arXiv},
  doi = {10.48550/arXiv.2006.10726},
  url = {http://arxiv.org/abs/2006.10726},
  urldate = {2024-11-05},
  abstract = {A model must adapt itself to generalize to new and different data during testing. In this setting of fully test-time adaptation the model has only the test data and its own parameters. We propose to adapt by test entropy minimization (tent): we optimize the model for confidence as measured by the entropy of its predictions. Our method estimates normalization statistics and optimizes channel-wise affine transformations to update online on each batch. Tent reduces generalization error for image classification on corrupted ImageNet and CIFAR-10/100 and reaches a new state-of-the-art error on ImageNet-C. Tent handles source-free domain adaptation on digit recognition from SVHN to MNIST/MNIST-M/USPS, on semantic segmentation from GTA to Cityscapes, and on the VisDA-C benchmark. These results are achieved in one epoch of test-time optimization without altering training.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\EMPTY_COLLECTION_NAME\\Wang et al_2021_Tent.pdf;C\:\\Users\\chsey\\Zotero\\storage\\IC8LSAY2\\2006.html}
}

@online{wangYOLOv7TrainableBagoffreebies2022,
  title = {{{YOLOv7}}: {{Trainable}} Bag-of-Freebies Sets New State-of-the-Art for Real-Time Object Detectors},
  shorttitle = {{{YOLOv7}}},
  author = {Wang, Chien-Yao and Bochkovskiy, Alexey and Liao, Hong-Yuan Mark},
  date = {2022-07-06},
  eprint = {2207.02696},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2207.02696},
  urldate = {2022-07-25},
  abstract = {YOLOv7 surpasses all known object detectors in both speed and accuracy in the range from 5 FPS to 160 FPS and has the highest accuracy 56.8\% AP among all known real-time object detectors with 30 FPS or higher on GPU V100. YOLOv7-E6 object detector (56 FPS V100, 55.9\% AP) outperforms both transformer-based detector SWIN-L Cascade-Mask R-CNN (9.2 FPS A100, 53.9\% AP) by 509\% in speed and 2\% in accuracy, and convolutional-based detector ConvNeXt-XL Cascade-Mask R-CNN (8.6 FPS A100, 55.2\% AP) by 551\% in speed and 0.7\% AP in accuracy, as well as YOLOv7 outperforms: YOLOR, YOLOX, Scaled-YOLOv4, YOLOv5, DETR, Deformable DETR, DINO-5scale-R50, ViT-Adapter-B and many other object detectors in speed and accuracy. Moreover, we train YOLOv7 only on MS COCO dataset from scratch without using any other datasets or pre-trained weights. Source code is released in https://github.com/WongKinYiu/yolov7.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\Computer Vision\\detection\\Wang et al_2022_YOLOv7.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AB8TM39J\\2207.html}
}

@online{wangZeroshotRecognitionSemantic2018,
  title = {Zero-Shot {{Recognition}} via {{Semantic Embeddings}} and {{Knowledge Graphs}}},
  author = {Wang, Xiaolong and Ye, Yufei and Gupta, Abhinav},
  date = {2018-04-08},
  eprint = {1803.08035},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1803.08035},
  url = {http://arxiv.org/abs/1803.08035},
  urldate = {2023-08-05},
  abstract = {We consider the problem of zero-shot recognition: learning a visual classifier for a category with zero training examples, just using the word embedding of the category and its relationship to other categories, which visual data are provided. The key to dealing with the unfamiliar or novel category is to transfer knowledge obtained from familiar classes to describe the unfamiliar class. In this paper, we build upon the recently introduced Graph Convolutional Network (GCN) and propose an approach that uses both semantic embeddings and the categorical relationships to predict the classifiers. Given a learned knowledge graph (KG), our approach takes as input semantic embeddings for each node (representing visual category). After a series of graph convolutions, we predict the visual classifier for each category. During training, the visual classifiers for a few categories are given to learn the GCN parameters. At test time, these filters are used to predict the visual classifiers of unseen categories. We show that our approach is robust to noise in the KG. More importantly, our approach provides significant improvement in performance compared to the current state-of-the-art results (from 2 \textasciitilde{} 3\% on some metrics to whopping 20\% on a few).},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\few shot learning\\Wang et al_2018_Zero-shot Recognition via Semantic Embeddings and Knowledge Graphs.pdf;C\:\\Users\\chsey\\Zotero\\storage\\K7LVMEW6\\1803.html}
}

@article{wassanImpactDigitalizationRetailers2022,
  title = {Impact of Digitalization on Retailers and Its Future Trends},
  author = {Wassan, Sobia and Gulati, Kamal and Ghosh, Ambarish and family=rafiqi, given=Ishtiyaq, prefix=shafi, useprefix=true and Mammani, Basavaraj S and Tabbassum, Sadia and family=Khaja Mohiddin, given=Md., given-i={{Md}}},
  date = {2022-01-01},
  journaltitle = {Materials Today: Proceedings},
  shortjournal = {Materials Today: Proceedings},
  series = {{{CMAE}}'21},
  volume = {51},
  pages = {803--809},
  issn = {2214-7853},
  doi = {10.1016/j.matpr.2021.06.238},
  url = {https://www.sciencedirect.com/science/article/pii/S2214785321046186},
  urldate = {2023-12-28},
  abstract = {People in today's world are getting used to buying the products they need to shop online. They don't need to go much more than beyond to shop online. They can easily access online stores or put mobile devices in place and arrange what you want. Our research is about online vs offline purchasing preference. What customers prefer to buy online or offline? And also, we demonstrate the future scenario of the retail market. So that we explore the online-offline model prediction in the future scenario followed by Barbara thau. We took sales data from national china bureau statistics. We analyze the sales of more than 6~years of data for the research. Our claim is an assumption, so we use a hypothesis model for the proof of our Claims. As well as we discuss the factor of purchasing behavior from the customer for consumer goods. Our claim is an assumption, so we use a hypothesis model for the proof of our Claims. As well as we discuss the factor of purchasing behavior from the customer for consumer goods. As we find our analysis results are positive so we make some business solution suggestions for our business people in suggestions and conclusions.},
  keywords = {Offline sales,Online sales,Online stores,Purchasing behavior,Retailor sales}
}

@article{wassermanHowInternetTransformed2011,
  title = {How the {{Internet}} Transformed the Software Industry},
  author = {Wasserman, Anthony I.},
  date = {2011-07},
  journaltitle = {Journal of Internet Services and Applications},
  shortjournal = {J Internet Serv Appl},
  volume = {2},
  number = {1},
  pages = {11--22},
  publisher = {SpringerOpen},
  issn = {1869-0238},
  doi = {10.1007/s13174-011-0019-x},
  url = {https://jisajournal.springeropen.com/articles/10.1007/s13174-011-0019-x},
  urldate = {2023-12-27},
  abstract = {The growth of the Internet has had a huge impact on the software industry, from the ease of creating new businesses to the processes that companies use to develop, distribute, and support their products. Software architectures and platforms for web applications differ significantly from traditional desktop and client-server applications, and require a new generation of programming languages and development tools. Developers make extensive use of open source software, particularly at the infrastructure level of their applications. Development teams can easily use Internet-based tools for collaboration, thus facilitating distributed organizations. Product marketing now emphasizes attracting prospective customers to the company’s website. Companies can release products over the Internet, or provide a hosted web application, both of which are more efficient and less expensive ways to sell their products. Companies can also support their products over the Internet through online discussion forums, often with users helping one another. Ongoing advances in mobile and cloud computing, styles of user interaction, and software business models are certain to have a large effect, leading to innovative new products from both new and established companies.},
  issue = {1},
  langid = {english},
  file = {Y:\paper\management\Wasserman_2011_How the Internet transformed the software industry.pdf}
}

@online{WatchmakingDanielsGeorge,
  title = {Watchmaking: {{Daniels}}, {{George}}: 9780856677045: {{Amazon}}.Com: {{Books}}},
  url = {https://www.amazon.com/Watchmaking-George-Daniels/dp/0856677043/ref=sr_1_1?keywords=Watchmaking&qid=1703584683&s=books&sr=1-1},
  urldate = {2023-12-26},
  file = {C:\Users\chsey\Zotero\storage\AFTP8LX7\ref=sr_1_1.html}
}

@inproceedings{weberDetectingNaturalDisasters2020,
  title = {Detecting {{Natural Disasters}}, {{Damage}}, and {{Incidents}} in the {{Wild}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Weber, Ethan and Marzo, Nuria and Papadopoulos, Dim P. and Biswas, Aritro and Lapedriza, Agata and Ofli, Ferda and Imran, Muhammad and Torralba, Antonio},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {331--350},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58529-7_20},
  abstract = {Responding to natural disasters, such as earthquakes, floods, and wildfires, is a laborious task performed by on-the-ground emergency responders and analysts. Social media has emerged as a low-latency data source to quickly understand disaster situations. While most studies on social media are limited to text, images offer more information for understanding disaster and incident scenes. However, no large-scale image datasets for incident detection exists. In this work, we present the Incidents Dataset, which contains 446,684 images annotated by humans that cover 43 incidents across a variety of scenes. We employ a baseline classification model that mitigates false-positive errors and we perform image filtering experiments on millions of social media images from Flickr and Twitter. Through these experiments, we show how the Incidents Dataset can be used to detect images with incidents in the wild. Code, data, and models are available online at http://incidentsdataset.csail.mit.edu.},
  isbn = {978-3-030-58529-7},
  langid = {english},
  keywords = {Disaster analysis,Image classification,Image dataset,Incident detection,Scene understanding,Social media,Visual recognition},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\disaster\Weber et al_2020_Detecting Natural Disasters, Damage, and Incidents in the Wild.pdf}
}

@inproceedings{weberDetectingNaturalDisasters2020a,
  title = {Detecting {{Natural Disasters}}, {{Damage}}, and {{Incidents}} in the {{Wild}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Weber, Ethan and Marzo, Nuria and Papadopoulos, Dim P. and Biswas, Aritro and Lapedriza, Agata and Ofli, Ferda and Imran, Muhammad and Torralba, Antonio},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {331--350},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58529-7_20},
  abstract = {Responding to natural disasters, such as earthquakes, floods, and wildfires, is a laborious task performed by on-the-ground emergency responders and analysts. Social media has emerged as a low-latency data source to quickly understand disaster situations. While most studies on social media are limited to text, images offer more information for understanding disaster and incident scenes. However, no large-scale image datasets for incident detection exists. In this work, we present the Incidents Dataset, which contains 446,684 images annotated by humans that cover 43 incidents across a variety of scenes. We employ a baseline classification model that mitigates false-positive errors and we perform image filtering experiments on millions of social media images from Flickr and Twitter. Through these experiments, we show how the Incidents Dataset can be used to detect images with incidents in the wild. Code, data, and models are available online at http://incidentsdataset.csail.mit.edu.},
  isbn = {978-3-030-58529-7},
  langid = {english},
  keywords = {Disaster analysis,Image classification,Image dataset,Incident detection,Scene understanding,Social media,Visual recognition},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\Weber et al_2020_Detecting Natural Disasters, Damage, and Incidents in the Wild.pdf}
}

@article{weberIncidents1MLargeScaleDataset2023,
  title = {{{Incidents1M}}: {{A Large-Scale Dataset}} of {{Images With Natural Disasters}}, {{Damage}}, and {{Incidents}}},
  shorttitle = {{{Incidents1M}}},
  author = {Weber, Ethan and Papadopoulos, Dim P. and Lapedriza, Agata and Ofli, Ferda and Imran, Muhammad and Torralba, Antonio},
  date = {2023-04},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume = {45},
  number = {4},
  pages = {4768--4781},
  issn = {1939-3539},
  doi = {10.1109/TPAMI.2022.3191996},
  abstract = {Natural disasters, such as floods, tornadoes, or wildfires, are increasingly pervasive as the Earth undergoes global warming. It is difficult to predict when and where an incident will occur, so timely emergency response is critical to saving the lives of those endangered by destructive events. Fortunately, technology can play a role in these situations. Social media posts can be used as a low-latency data source to understand the progression and aftermath of a disaster, yet parsing this data is tedious without automated methods. Prior work has mostly focused on text-based filtering, yet image and video-based filtering remains largely unexplored. In this work, we present the Incidents1M Dataset, a large-scale multi-label dataset which contains 977,088 images, with 43 incident and 49 place categories. We provide details of the dataset construction, statistics and potential biases; introduce and train a model for incident detection; and perform image-filtering experiments on millions of images on Flickr and Twitter. We also present some applications on incident analysis to encourage and enable future work in computer vision for humanitarian aid. Code, data, and models are available at http://incidentsdataset.csail.mit.edu.},
  eventtitle = {{{IEEE Transactions}} on {{Pattern Analysis}} and {{Machine Intelligence}}},
  keywords = {Computational modeling,Data models,disaster analysis,Disasters,Global warming,Image analysis,image dataset,incident detection,Satellites,scene understanding,social media,Social networking (online),Task analysis,Training,Visual recognition,Visualization},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\AI_for_social_good\disaster\Weber et al_2023_Incidents1M.pdf}
}

@online{wederRemovingObjectsNeural2022,
  title = {Removing {{Objects From Neural Radiance Fields}}},
  author = {Weder, Silvan and Garcia-Hernando, Guillermo and Monszpart, Aron and Pollefeys, Marc and Brostow, Gabriel and Firman, Michael and Vicente, Sara},
  date = {2022-12-22},
  eprint = {2212.11966},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2212.11966},
  urldate = {2023-01-25},
  abstract = {Neural Radiance Fields (NeRFs) are emerging as a ubiquitous scene representation that allows for novel view synthesis. Increasingly, NeRFs will be shareable with other people. Before sharing a NeRF, though, it might be desirable to remove personal information or unsightly objects. Such removal is not easily achieved with the current NeRF editing frameworks. We propose a framework to remove objects from a NeRF representation created from an RGB-D sequence. Our NeRF inpainting method leverages recent work in 2D image inpainting and is guided by a user-provided mask. Our algorithm is underpinned by a confidence based view selection procedure. It chooses which of the individual 2D inpainted images to use in the creation of the NeRF, so that the resulting inpainted NeRF is 3D consistent. We show that our method for NeRF editing is effective for synthesizing plausible inpaintings in a multi-view coherent manner. We validate our approach using a new and still-challenging dataset for the task of NeRF inpainting.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Weder et al_2022_Removing Objects From Neural Radiance Fields.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RLWG6E4M\\2212.html}
}

@online{WeightsBiases,
  title = {Weights \& {{Biases}}},
  url = {https://wandb.ai/choi-scholarg/20241025_rankmin_matching_unimodal/runs/c9qa4ixb},
  urldate = {2024-10-24},
  abstract = {Weights \& Biases, developer tools for machine learning},
  langid = {english},
  organization = {W\&B},
  keywords = {notion}
}

@online{WeightsBiases2024,
  title = {Weights \& {{Biases}}},
  date = {2024-06-07},
  url = {https://wandb.ai/site},
  urldate = {2024-06-07},
  abstract = {Weights \& Biases, developer tools for machine learning},
  langid = {english},
  organization = {W\&B},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\WWWBV7KM\img2dataset.html}
}

@online{wenContrastiveCrossModalKnowledge2022,
  title = {Contrastive {{Cross-Modal Knowledge Sharing Pre-training}} for {{Vision-Language Representation Learning}} and {{Retrieval}}},
  author = {Wen, Keyu and Tan, Zhenshan and Cheng, Qingrong and Chen, Cheng and Gu, Xiaodong},
  date = {2022-07-08},
  eprint = {2207.00733},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2207.00733},
  url = {http://arxiv.org/abs/2207.00733},
  urldate = {2024-02-02},
  abstract = {Recently, the cross-modal pre-training task has been a hotspot because of its wide application in various down-streaming researches including retrieval, captioning, question answering and so on. However, exiting methods adopt a one-stream pre-training model to explore the united vision-language representation for conducting cross-modal retrieval, which easily suffer from the calculation explosion. Moreover, although the conventional double-stream structures are quite efficient, they still lack the vital cross-modal interactions, resulting in low performances. Motivated by these challenges, we put forward a Contrastive Cross-Modal Knowledge Sharing Pre-training (COOKIE) to grasp the joint text-image representations. Structurally, COOKIE adopts the traditional double-stream structure because of the acceptable time consumption. To overcome the inherent defects of double-stream structure as mentioned above, we elaborately design two effective modules. Concretely, the first module is a weight-sharing transformer that builds on the head of the visual and textual encoders, aiming to semantically align text and image. This design enables visual and textual paths focus on the same semantics. The other one is three specially designed contrastive learning, aiming to share knowledge between different models. The shared cross-modal knowledge develops the study of unimodal representation greatly, promoting the single-modal retrieval tasks. Extensive experimental results on multi-modal matching researches that includes cross-modal retrieval, text matching, and image retrieval reveal the superiors in calculation efficiency and statistical indicators of our pre-training model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Wen et al_2022_Contrastive Cross-Modal Knowledge Sharing Pre-training for Vision-Language.pdf;C\:\\Users\\chsey\\Zotero\\storage\\D65PCBFA\\2207.html}
}

@article{wenSurveyFederatedLearning2023,
  title = {A Survey on Federated Learning: Challenges and Applications},
  shorttitle = {A Survey on Federated Learning},
  author = {Wen, Jie and Zhang, Zhixia and Lan, Yang and Cui, Zhihua and Cai, Jianghui and Zhang, Wensheng},
  date = {2023-02-01},
  journaltitle = {International Journal of Machine Learning and Cybernetics},
  shortjournal = {Int. J. Mach. Learn. \& Cyber.},
  volume = {14},
  number = {2},
  pages = {513--535},
  issn = {1868-808X},
  doi = {10.1007/s13042-022-01647-y},
  url = {https://doi.org/10.1007/s13042-022-01647-y},
  urldate = {2024-09-10},
  abstract = {Federated learning (FL) is a secure distributed machine learning paradigm that addresses the issue of data silos in building a joint model. Its unique distributed training mode and the advantages of security aggregation mechanism are very suitable for various practical applications with strict privacy requirements. However, with the deployment of FL mode into practical application, some bottlenecks appear in the FL training process, which affects the performance and efficiency of the FL model in practical applications. Therefore, more researchers have paid attention to the challenges of FL and sought for various effective research methods to solve these current bottlenecks. And various research achievements of FL have been made to promote the intelligent development of all application areas with privacy restriction. This paper systematically introduces the current researches in FL from five aspects: the basics knowledge of FL, privacy and security protection mechanisms in FL, communication overhead challenges and heterogeneity problems of FL. Furthermore, we make a comprehensive summary of the research in practical applications and prospect the future research directions of FL.},
  langid = {english},
  keywords = {Artificial Intelligence,Federated learning,Machine learning,notion,Personalized federated learning,Privacy protection},
  file = {Y:\paper\2024_research\Wen et al_2023_A survey on federated learning.pdf}
}

@online{wettigShouldYouMask2023,
  title = {Should {{You Mask}} 15\% in {{Masked Language Modeling}}?},
  author = {Wettig, Alexander and Gao, Tianyu and Zhong, Zexuan and Chen, Danqi},
  date = {2023-02-10},
  eprint = {2202.08005},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2202.08005},
  url = {http://arxiv.org/abs/2202.08005},
  urldate = {2024-03-04},
  abstract = {Masked language models (MLMs) conventionally mask 15\% of tokens due to the belief that more masking would leave insufficient context to learn good representations; this masking rate has been widely used, regardless of model sizes or masking strategies. In this work, we revisit this important choice of MLM pre-training. We first establish that 15\% is not universally optimal, and larger models should adopt a higher masking rate. Specifically, we find that masking 40\% outperforms 15\% for BERT-large size models on GLUE and SQuAD. Interestingly, an extremely high masking rate of 80\% can still preserve 95\% fine-tuning performance and most of the accuracy in linguistic probing, challenging the conventional wisdom about the role of the masking rate. We then examine the interplay between masking rates and masking strategies and find that uniform masking requires a higher masking rate compared to sophisticated masking strategies such as span or PMI masking. Finally, we argue that increasing the masking rate has two distinct effects: it leads to more corruption, which makes the prediction task more difficult; it also enables more predictions, which benefits optimization. Using this framework, we revisit BERT's 80-10-10 corruption strategy. Together, our results contribute to a better understanding of MLM pre-training.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Wettig et al_2023_Should You Mask 15% in Masked Language Modeling.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ZRL3ASQ9\\2202.html}
}

@inproceedings{whittedImprovedIlluminationModel2005,
  title = {An Improved Illumination Model for Shaded Display},
  booktitle = {{{ACM SIGGRAPH}} 2005 {{Courses}}},
  author = {Whitted, Turner},
  year = {7월 31, 2005},
  series = {{{SIGGRAPH}} '05},
  pages = {4--es},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/1198555.1198743},
  url = {https://doi.org/10.1145/1198555.1198743},
  urldate = {2023-05-30},
  abstract = {To accurately render a two-dimensional image of a three-dimensional scene, global illumination information that affects the intensity of each pixel of the image must be known at the time the intensity is calculated. In a simplified form, this information is stored in a tree of "rays" extending from the viewer to the first surface encountered and from there to other surfaces and to the light sources. A visible surface algorithm creates this tree for each pixel of the display and passes it to the shader. The shader then traverses the tree to determine the intensity of the light received by the viewer. Consideration of all of these factors allows the shader to accurately simulate true reflection, shadows, and refraction, as well as the effects simulated by conventional shaders. Anti-aliasing is included as an integral part of the visibility calculations. Surfaces displayed include curved as well as polygonal surfaces.},
  isbn = {978-1-4503-7833-8},
  keywords = {computer animation,computer graphics,raster displays,shading,visible surface algorithms},
  file = {Y:\paper\2022 winter intern\Whitted_2005_An improved illumination model for shaded display.pdf}
}

@online{wightmanResNetStrikesBack2021,
  title = {{{ResNet}} Strikes Back: {{An}} Improved Training Procedure in Timm},
  shorttitle = {{{ResNet}} Strikes Back},
  author = {Wightman, Ross and Touvron, Hugo and Jégou, Hervé},
  date = {2021-10-01},
  eprint = {2110.00476},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2110.00476},
  urldate = {2022-10-08},
  abstract = {The influential Residual Networks designed by He et al. remain the gold-standard architecture in numerous scientific publications. They typically serve as the default architecture in studies, or as baselines when new architectures are proposed. Yet there has been significant progress on best practices for training neural networks since the inception of the ResNet architecture in 2015. Novel optimization \& data-augmentation have increased the effectiveness of the training recipes. In this paper, we re-evaluate the performance of the vanilla ResNet-50 when trained with a procedure that integrates such advances. We share competitive training settings and pre-trained models in the timm open-source library, with the hope that they will serve as better baselines for future work. For instance, with our more demanding training setting, a vanilla ResNet-50 reaches 80.4\% top-1 accuracy at resolution 224x224 on ImageNet-val without extra data or distillation. We also report the performance achieved with popular models with our training procedure.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Wightman et al_2021_ResNet strikes back.pdf;C\:\\Users\\chsey\\Zotero\\storage\\Z2XXL5F8\\2110.html}
}

@inproceedings{williamsBroadCoverageChallengeCorpus2018,
  title = {A {{Broad-Coverage Challenge Corpus}} for {{Sentence Understanding}} through {{Inference}}},
  booktitle = {Proceedings of the 2018 {{Conference}} of the {{North American Chapter}} of the {{Association}} for {{Computational Linguistics}}: {{Human Language Technologies}}, {{Volume}} 1 ({{Long Papers}})},
  author = {Williams, Adina and Nangia, Nikita and Bowman, Samuel},
  editor = {Walker, Marilyn and Ji, Heng and Stent, Amanda},
  date = {2018-06},
  pages = {1112--1122},
  publisher = {Association for Computational Linguistics},
  location = {New Orleans, Louisiana},
  doi = {10.18653/v1/N18-1101},
  url = {https://aclanthology.org/N18-1101},
  urldate = {2024-05-01},
  abstract = {This paper introduces the Multi-Genre Natural Language Inference (MultiNLI) corpus, a dataset designed for use in the development and evaluation of machine learning models for sentence understanding. At 433k examples, this resource is one of the largest corpora available for natural language inference (a.k.a. recognizing textual entailment), improving upon available resources in both its coverage and difficulty. MultiNLI accomplishes this by offering data from ten distinct genres of written and spoken English, making it possible to evaluate systems on nearly the full complexity of the language, while supplying an explicit setting for evaluating cross-genre domain adaptation. In addition, an evaluation using existing machine learning models designed for the Stanford NLI corpus shows that it represents a substantially more difficult task than does that corpus, despite the two showing similar levels of inter-annotator agreement.},
  eventtitle = {{{NAACL-HLT}} 2018},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Williams et al_2018_A Broad-Coverage Challenge Corpus for Sentence Understanding through Inference.pdf}
}

@online{williamsNonnegativeDecompositionMultivariate2010,
  title = {Nonnegative {{Decomposition}} of {{Multivariate Information}}},
  author = {Williams, Paul L. and Beer, Randall D.},
  date = {2010-04-14},
  eprint = {1004.2515},
  eprinttype = {arXiv},
  eprintclass = {math-ph, physics:physics, q-bio},
  doi = {10.48550/arXiv.1004.2515},
  url = {http://arxiv.org/abs/1004.2515},
  urldate = {2024-05-19},
  abstract = {Of the various attempts to generalize information theory to multiple variables, the most widely utilized, interaction information, suffers from the problem that it is sometimes negative. Here we reconsider from first principles the general structure of the information that a set of sources provides about a given variable. We begin with a new definition of redundancy as the minimum information that any source provides about each possible outcome of the variable, averaged over all possible outcomes. We then show how this measure of redundancy induces a lattice over sets of sources that clarifies the general structure of multivariate information. Finally, we use this redundancy lattice to propose a definition of partial information atoms that exhaustively decompose the Shannon information in a multivariate system in terms of the redundancy between synergies of subsets of the sources. Unlike interaction information, the atoms of our partial information decomposition are never negative and always support a clear interpretation as informational quantities. Our analysis also demonstrates how the negativity of interaction information can be explained by its confounding of redundancy and synergy.},
  pubstate = {prepublished},
  keywords = {94A15,Computer Science - Information Theory,Mathematical Physics,notion,Physics - Biological Physics,Physics - Data Analysis Statistics and Probability,Quantitative Biology - Neurons and Cognition,Quantitative Biology - Quantitative Methods},
  file = {Y\:\\paper\\2024_research\\Williams_Beer_2010_Nonnegative Decomposition of Multivariate Information.pdf;C\:\\Users\\chsey\\Zotero\\storage\\S6JRNZGW\\1004.html}
}

@online{wilsonMarginalValueAdaptive2018,
  title = {The {{Marginal Value}} of {{Adaptive Gradient Methods}} in {{Machine Learning}}},
  author = {Wilson, Ashia C. and Roelofs, Rebecca and Stern, Mitchell and Srebro, Nathan and Recht, Benjamin},
  date = {2018-05-21},
  eprint = {1705.08292},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1705.08292},
  urldate = {2024-05-30},
  abstract = {Adaptive optimization methods, which perform local optimization with a metric constructed from the history of iterates, are becoming increasingly popular for training deep neural networks. Examples include AdaGrad, RMSProp, and Adam. We show that for simple overparameterized problems, adaptive methods often find drastically different solutions than gradient descent (GD) or stochastic gradient descent (SGD). We construct an illustrative binary classification problem where the data is linearly separable, GD and SGD achieve zero test error, and AdaGrad, Adam, and RMSProp attain test errors arbitrarily close to half. We additionally study the empirical generalization capability of adaptive methods on several stateof-the-art deep learning models. We observe that the solutions found by adaptive methods generalize worse (often significantly worse) than SGD, even when these solutions have better training performance. These results suggest that practitioners should reconsider the use of adaptive methods to train neural networks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y:\paper\2024_lecture\Wilson et al_2018_The Marginal Value of Adaptive Gradient Methods in Machine Learning.pdf}
}

@online{wm.K27JamsuhamWeonjaro,
  title = {K-27 잠수함 원자로 사고, 1968년},
  author = {Wm., Johnston},
  url = {https://www.johnstonsarchive.net/nuclear/radevents/1968USSR6.html},
  urldate = {2023-12-29},
  file = {C:\Users\chsey\Zotero\storage\ZBL9X38J\1968USSR6.html}
}

@inproceedings{woodworthKernelRichRegimes2020,
  title = {Kernel and {{Rich Regimes}} in {{Overparametrized Models}}},
  booktitle = {Proceedings of {{Thirty Third Conference}} on {{Learning Theory}}},
  author = {Woodworth, Blake and Gunasekar, Suriya and Lee, Jason D. and Moroshko, Edward and Savarese, Pedro and Golan, Itay and Soudry, Daniel and Srebro, Nathan},
  date = {2020-07-15},
  pages = {3635--3673},
  publisher = {PMLR},
  issn = {2640-3498},
  url = {https://proceedings.mlr.press/v125/woodworth20a.html},
  urldate = {2024-03-28},
  abstract = {A recent line of work studies overparametrized neural networks in the “kernel regime,” i.e.~when  during training the network behaves as a kernelized linear predictor, and thus, training with gradient descent has the effect of finding the corresponding minimum RKHS norm solution.  This stands in contrast to other studies which demonstrate how gradient descent on overparametrized  networks can induce rich implicit biases that are not RKHS norms.  Building on an observation by \textbackslash citet\{chizat2018note\}, we show how the \textbackslash textbf\{\textbackslash textit\{scale of the initialization\}\} controls the transition between the “kernel” (aka lazy) and “rich” (aka active) regimes and affects generalization properties in multilayer homogeneous models. We provide a complete and detailed analysis for a family of simple depth-\$D\$ linear networks that exhibit an interesting and meaningful transition between the kernel and rich regimes, and highlight an interesting role for the \textbackslash emph\{width\}  of the models. We further demonstrate this transition empirically for matrix factorization and multilayer non-linear networks.},
  eventtitle = {Conference on {{Learning Theory}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Woodworth et al_2020_Kernel and Rich Regimes in Overparametrized Models.pdf}
}

@online{woodworthKernelRichRegimes2020a,
  title = {Kernel and {{Rich Regimes}} in {{Overparametrized Models}}},
  author = {Woodworth, Blake and Gunasekar, Suriya and Lee, Jason D. and Moroshko, Edward and Savarese, Pedro and Golan, Itay and Soudry, Daniel and Srebro, Nathan},
  date = {2020-07-27},
  eprint = {2002.09277},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.2002.09277},
  url = {http://arxiv.org/abs/2002.09277},
  urldate = {2024-03-28},
  abstract = {A recent line of work studies overparametrized neural networks in the "kernel regime," i.e. when the network behaves during training as a kernelized linear predictor, and thus training with gradient descent has the effect of finding the minimum RKHS norm solution. This stands in contrast to other studies which demonstrate how gradient descent on overparametrized multilayer networks can induce rich implicit biases that are not RKHS norms. Building on an observation by Chizat and Bach, we show how the scale of the initialization controls the transition between the "kernel" (aka lazy) and "rich" (aka active) regimes and affects generalization properties in multilayer homogeneous models. We also highlight an interesting role for the width of a model in the case that the predictor is not identically zero at initialization. We provide a complete and detailed analysis for a family of simple depth-\$D\$ models that already exhibit an interesting and meaningful transition between the kernel and rich regimes, and we also demonstrate this transition empirically for more complex matrix factorization models and multilayer non-linear networks.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Woodworth et al_2020_Kernel and Rich Regimes in Overparametrized Models.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5VW92RD2\\2002.html}
}

@online{WorldwideCustomerRelationship,
  title = {Worldwide {{Customer Relationship Management Applications Software Forecast}}, 2022–2026},
  url = {https://www.idc.com/getdoc.jsp?containerId=US49202922},
  urldate = {2024-01-01},
  abstract = {IDC examines consumer markets by devices, applications, networks, and services to provide complete solutions for succeeding in these expanding markets.},
  organization = {IDC: The premier global market intelligence company}
}

@online{wortsmanModelSoupsAveraging2022,
  title = {Model Soups: Averaging Weights of Multiple Fine-Tuned Models Improves Accuracy without Increasing Inference Time},
  shorttitle = {Model Soups},
  author = {Wortsman, Mitchell and Ilharco, Gabriel and Gadre, Samir Yitzhak and Roelofs, Rebecca and Gontijo-Lopes, Raphael and Morcos, Ari S. and Namkoong, Hongseok and Farhadi, Ali and Carmon, Yair and Kornblith, Simon and Schmidt, Ludwig},
  date = {2022-07-01},
  eprint = {2203.05482},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2203.05482},
  url = {http://arxiv.org/abs/2203.05482},
  urldate = {2024-02-10},
  abstract = {The conventional recipe for maximizing model accuracy is to (1) train multiple models with various hyperparameters and (2) pick the individual model which performs best on a held-out validation set, discarding the remainder. In this paper, we revisit the second step of this procedure in the context of fine-tuning large pre-trained models, where fine-tuned models often appear to lie in a single low error basin. We show that averaging the weights of multiple models fine-tuned with different hyperparameter configurations often improves accuracy and robustness. Unlike a conventional ensemble, we may average many models without incurring any additional inference or memory costs -- we call the results "model soups." When fine-tuning large pre-trained models such as CLIP, ALIGN, and a ViT-G pre-trained on JFT, our soup recipe provides significant improvements over the best model in a hyperparameter sweep on ImageNet. The resulting ViT-G model, which attains 90.94\% top-1 accuracy on ImageNet, achieved a new state of the art. Furthermore, we show that the model soup approach extends to multiple image classification and natural language processing tasks, improves out-of-distribution performance, and improves zero-shot performance on new downstream tasks. Finally, we analytically relate the performance similarity of weight-averaging and logit-ensembling to flatness of the loss and confidence of the predictions, and validate this relation empirically. Code is available at https://github.com/mlfoundations/model-soups.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Wortsman et al_2022_Model soups.pdf;C\:\\Users\\chsey\\Zotero\\storage\\U8QY26PK\\2203.html}
}

@online{wuCharacterizingOvercomingGreedy2022,
  title = {Characterizing and Overcoming the Greedy Nature of Learning in Multi-Modal Deep Neural Networks},
  author = {Wu, Nan and Jastrzębski, Stanisław and Cho, Kyunghyun and Geras, Krzysztof J.},
  date = {2022-09-16},
  eprint = {2202.05306},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2202.05306},
  urldate = {2024-05-29},
  abstract = {We hypothesize that due to the greedy nature of learning in multi-modal deep neural networks, these models tend to rely on just one modality while under-fitting the other modalities. Such behavior is counter-intuitive and hurts the models’ generalization, as we observe empirically. To estimate the model’s dependence on each modality, we compute the gain on the accuracy when the model has access to it in addition to another modality. We refer to this gain as the conditional utilization rate. In the experiments, we consistently observe an imbalance in conditional utilization rates between modalities, across multiple tasks and architectures. Since conditional utilization rate cannot be computed efficiently during training, we introduce a proxy for it based on the pace at which the model learns from each modality, which we refer to as the conditional learning speed. We propose an algorithm to balance the conditional learning speeds between modalities during training and demonstrate that it indeed addresses the issue of greedy learning.1 The proposed algorithm improves the model’s generalization on three datasets: Colored MNIST, ModelNet40, and NVIDIA Dynamic Hand Gesture.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\IA4YZXBX\Wu 등 - 2022 - Characterizing and overcoming the greedy nature of.pdf}
}

@online{wuDIVeRRealtimeAccurate2022,
  title = {{{DIVeR}}: {{Real-time}} and {{Accurate Neural Radiance Fields}} with {{Deterministic Integration}} for {{Volume Rendering}}},
  shorttitle = {{{DIVeR}}},
  author = {Wu, Liwen and Lee, Jae Yong and Bhattad, Anand and Wang, Yuxiong and Forsyth, David},
  date = {2022-05-18},
  eprint = {2111.10427},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.10427},
  url = {http://arxiv.org/abs/2111.10427},
  urldate = {2023-01-24},
  abstract = {DIVeR builds on the key ideas of NeRF and its variants -- density models and volume rendering -- to learn 3D object models that can be rendered realistically from small numbers of images. In contrast to all previous NeRF methods, DIVeR uses deterministic rather than stochastic estimates of the volume rendering integral. DIVeR's representation is a voxel based field of features. To compute the volume rendering integral, a ray is broken into intervals, one per voxel; components of the volume rendering integral are estimated from the features for each interval using an MLP, and the components are aggregated. As a result, DIVeR can render thin translucent structures that are missed by other integrators. Furthermore, DIVeR's representation has semantics that is relatively exposed compared to other such methods -- moving feature vectors around in the voxel space results in natural edits. Extensive qualitative and quantitative comparisons to current state-of-the-art methods show that DIVeR produces models that (1) render at or above state-of-the-art quality, (2) are very small without being baked, (3) render very fast without being baked, and (4) can be edited in natural ways.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Wu et al_2022_DIVeR2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AMMAREH2\\2111.html}
}

@online{wuDIVeRRealtimeAccurate2022a,
  title = {{{DIVeR}}: {{Real-time}} and {{Accurate Neural Radiance Fields}} with {{Deterministic Integration}} for {{Volume Rendering}}},
  shorttitle = {{{DIVeR}}},
  author = {Wu, Liwen and Lee, Jae Yong and Bhattad, Anand and Wang, Yuxiong and Forsyth, David},
  date = {2022-05-18},
  eprint = {2111.10427},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.10427},
  urldate = {2023-01-24},
  abstract = {DIVeR builds on the key ideas of NeRF and its variants -- density models and volume rendering -- to learn 3D object models that can be rendered realistically from small numbers of images. In contrast to all previous NeRF methods, DIVeR uses deterministic rather than stochastic estimates of the volume rendering integral. DIVeR's representation is a voxel based field of features. To compute the volume rendering integral, a ray is broken into intervals, one per voxel; components of the volume rendering integral are estimated from the features for each interval using an MLP, and the components are aggregated. As a result, DIVeR can render thin translucent structures that are missed by other integrators. Furthermore, DIVeR's representation has semantics that is relatively exposed compared to other such methods -- moving feature vectors around in the voxel space results in natural edits. Extensive qualitative and quantitative comparisons to current state-of-the-art methods show that DIVeR produces models that (1) render at or above state-of-the-art quality, (2) are very small without being baked, (3) render very fast without being baked, and (4) can be edited in natural ways.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Wu et al_2022_DIVeR.pdf;C\:\\Users\\chsey\\Zotero\\storage\\S5AXNTBZ\\2111.html}
}

@inproceedings{wuDoFNeRFDepthofFieldMeets2022,
  title = {{{DoF-NeRF}}: {{Depth-of-Field Meets Neural Radiance Fields}}},
  shorttitle = {{{DoF-NeRF}}},
  booktitle = {Proceedings of the 30th {{ACM International Conference}} on {{Multimedia}}},
  author = {Wu, Zijin and Li, Xingyi and Peng, Juewen and Lu, Hao and Cao, Zhiguo and Zhong, Weicai},
  date = {2022-10-10},
  eprint = {2208.00945},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1718--1729},
  doi = {10.1145/3503161.3548088},
  url = {http://arxiv.org/abs/2208.00945},
  urldate = {2023-04-20},
  abstract = {Neural Radiance Field (NeRF) and its variants have exhibited great success on representing 3D scenes and synthesizing photo-realistic novel views. However, they are generally based on the pinhole camera model and assume all-in-focus inputs. This limits their applicability as images captured from the real world often have finite depth-of-field (DoF). To mitigate this issue, we introduce DoF-NeRF, a novel neural rendering approach that can deal with shallow DoF inputs and can simulate DoF effect. In particular, it extends NeRF to simulate the aperture of lens following the principles of geometric optics. Such a physical guarantee allows DoF-NeRF to operate views with different focus configurations. Benefiting from explicit aperture modeling, DoF-NeRF also enables direct manipulation of DoF effect by adjusting virtual aperture and focus parameters. It is plug-and-play and can be inserted into NeRF-based frameworks. Experiments on synthetic and real-world datasets show that, DoF-NeRF not only performs comparably with NeRF in the all-in-focus setting, but also can synthesize all-in-focus novel views conditioned on shallow DoF inputs. An interesting application of DoF-NeRF to DoF rendering is also demonstrated. The source code will be made available at https://github.com/zijinwuzijin/DoF-NeRF.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\surface normal\\Wu et al_2022_DoF-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\TQDK79BZ\\2208.html}
}

@online{wuGRiTGenerativeRegiontotext2022,
  title = {{{GRiT}}: {{A Generative Region-to-text Transformer}} for {{Object Understanding}}},
  shorttitle = {{{GRiT}}},
  author = {Wu, Jialian and Wang, Jianfeng and Yang, Zhengyuan and Gan, Zhe and Liu, Zicheng and Yuan, Junsong and Wang, Lijuan},
  date = {2022-11-30},
  eprint = {2212.00280},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2212.00280},
  urldate = {2023-05-29},
  abstract = {This paper presents a Generative RegIon-to-Text transformer, GRiT, for object understanding. The spirit of GRiT is to formulate object understanding as {$<$}region, text{$>$} pairs, where region locates objects and text describes objects. For example, the text in object detection denotes class names while that in dense captioning refers to descriptive sentences. Specifically, GRiT consists of a visual encoder to extract image features, a foreground object extractor to localize objects, and a text decoder to generate open-set object descriptions. With the same model architecture, GRiT can understand objects via not only simple nouns, but also rich descriptive sentences including object attributes or actions. Experimentally, we apply GRiT to object detection and dense captioning tasks. GRiT achieves 60.4 AP on COCO 2017 test-dev for object detection and 15.5 mAP on Visual Genome for dense captioning. Code is available at https://github.com/JialianW/GRiT},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Wu et al_2022_GRiT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V4QJ4TRH\\2212.html}
}

@online{wuLongTermFeatureBanks2019,
  title = {Long-{{Term Feature Banks}} for {{Detailed Video Understanding}}},
  author = {Wu, Chao-Yuan and Feichtenhofer, Christoph and Fan, Haoqi and He, Kaiming and Krähenbühl, Philipp and Girshick, Ross},
  date = {2019-04-17},
  eprint = {1812.05038},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1812.05038},
  url = {http://arxiv.org/abs/1812.05038},
  urldate = {2023-08-05},
  abstract = {To understand the world, we humans constantly need to relate the present to the past, and put events in context. In this paper, we enable existing video models to do the same. We propose a long-term feature bank---supportive information extracted over the entire span of a video---to augment state-of-the-art video models that otherwise would only view short clips of 2-5 seconds. Our experiments demonstrate that augmenting 3D convolutional networks with a long-term feature bank yields state-of-the-art results on three challenging video datasets: AVA, EPIC-Kitchens, and Charades.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\action recognition\\Wu et al_2019_Long-Term Feature Banks for Detailed Video Understanding.pdf;C\:\\Users\\chsey\\Zotero\\storage\\UUKIIE5G\\1812.html}
}

@online{wuMixtureLoRAExperts2024,
  title = {Mixture of {{LoRA Experts}}},
  author = {Wu, Xun and Huang, Shaohan and Wei, Furu},
  date = {2024-04-21},
  eprint = {2404.13628},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2404.13628},
  url = {http://arxiv.org/abs/2404.13628},
  urldate = {2024-07-15},
  abstract = {LoRA has gained widespread acceptance in the fine-tuning of large pre-trained models to cater to a diverse array of downstream tasks, showcasing notable effectiveness and efficiency, thereby solidifying its position as one of the most prevalent fine-tuning techniques. Due to the modular nature of LoRA's plug-and-play plugins, researchers have delved into the amalgamation of multiple LoRAs to empower models to excel across various downstream tasks. Nonetheless, extant approaches for LoRA fusion grapple with inherent challenges. Direct arithmetic merging may result in the loss of the original pre-trained model's generative capabilities or the distinct identity of LoRAs, thereby yielding suboptimal outcomes. On the other hand, Reference tuning-based fusion exhibits limitations concerning the requisite flexibility for the effective combination of multiple LoRAs. In response to these challenges, this paper introduces the Mixture of LoRA Experts (MoLE) approach, which harnesses hierarchical control and unfettered branch selection. The MoLE approach not only achieves superior LoRA fusion performance in comparison to direct arithmetic merging but also retains the crucial flexibility for combining LoRAs effectively. Extensive experimental evaluations conducted in both the Natural Language Processing (NLP) and Vision \& Language (V\&L) domains substantiate the efficacy of MoLE.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Computer Science - Multimedia,notion},
  file = {Y\:\\paper\\2024_research\\Wu et al_2024_Mixture of LoRA Experts.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EZX5BL99\\2404.html}
}

@online{wuOmniSMoLABoostingGeneralist2024,
  title = {Omni-{{SMoLA}}: {{Boosting Generalist Multimodal Models}} with {{Soft Mixture}} of {{Low-rank Experts}}},
  shorttitle = {Omni-{{SMoLA}}},
  author = {Wu, Jialin and Hu, Xia and Wang, Yaqing and Pang, Bo and Soricut, Radu},
  date = {2024-04-02},
  eprint = {2312.00968},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2312.00968},
  urldate = {2024-06-16},
  abstract = {Large multi-modal models (LMMs) exhibit remarkable performance across numerous tasks. However, generalist LMMs often suffer from performance degradation when tuned over a large collection of tasks. Recent research suggests that Mixture of Experts (MoE) architectures are useful for instruction tuning, but for LMMs of parameter size around O(50-100B), the prohibitive cost of replicating and storing the expert models severely limits the number of experts we can use. We propose Omni-SMoLA, an architecture that uses the Soft MoE approach to (softly) mix many multimodal low rank experts, and avoids introducing a significant number of new parameters compared to conventional MoE models. The core intuition here is that the large model provides a foundational backbone, while different lightweight experts residually learn specialized knowledge, either per-modality or multimodally. Extensive experiments demonstrate that the SMoLA approach helps improve the generalist performance across a broad range of generative vision-and-language tasks, achieving new SoTA generalist performance that often matches or outperforms single specialized LMM baselines, as well as new SoTA specialist performance.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {C:\Users\chsey\Zotero\storage\8AG3PFKT\Wu 등 - 2024 - Omni-SMoLA Boosting Generalist Multimodal Models .pdf}
}

@online{wuUnleashingPowerVisual2023,
  title = {Unleashing the {{Power}} of {{Visual Prompting At}} the {{Pixel Level}}},
  author = {Wu, Junyang and Li, Xianhang and Wei, Chen and Wang, Huiyu and Yuille, Alan and Zhou, Yuyin and Xie, Cihang},
  date = {2023-03-29},
  eprint = {2212.10556},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2212.10556},
  url = {http://arxiv.org/abs/2212.10556},
  urldate = {2023-11-06},
  abstract = {This paper presents a simple and effective visual prompting method for adapting pre-trained models to downstream recognition tasks. Our method includes two key designs. First, rather than directly adding together the prompt and the image, we treat the prompt as an extra and independent learnable component. We show that the strategy of reconciling the prompt and the image matters, and find that warping the prompt around a properly shrinked image empirically works the best. Second, we re-introduce two "old tricks" commonly used in building transferable adversarial examples, i.e., input diversity and gradient normalization, into visual prompting. These techniques improve optimization and enable the prompt to generalize better. We provide extensive experimental results to demonstrate the effectiveness of our method. Using a CLIP model, our prompting method sets a new record of 82.8\% average accuracy across 12 popular classification datasets, substantially surpassing the prior art by +5.6\%. It is worth noting that this prompting performance already outperforms linear probing by +2.1\% and can even match fully fine-tuning in certain datasets. In addition, our prompting method shows competitive performance across different data scales and against distribution shifts. The code is publicly available at https://github.com/UCSC-VLAA/EVP.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_prompt\\Wu et al_2023_Unleashing the Power of Visual Prompting At the Pixel Level.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MBR53Y2M\\2212.html}
}

@online{wuUnsupervisedFeatureLearning2018,
  title = {Unsupervised {{Feature Learning}} via {{Non-Parametric Instance-level Discrimination}}},
  author = {Wu, Zhirong and Xiong, Yuanjun and Yu, Stella and Lin, Dahua},
  date = {2018-05-04},
  eprint = {1805.01978},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1805.01978},
  url = {http://arxiv.org/abs/1805.01978},
  urldate = {2023-08-05},
  abstract = {Neural net classifiers trained on data with annotated class labels can also capture apparent visual similarity among categories without being directed to do so. We study whether this observation can be extended beyond the conventional domain of supervised learning: Can we learn a good feature representation that captures apparent similarity among instances, instead of classes, by merely asking the feature to be discriminative of individual instances? We formulate this intuition as a non-parametric classification problem at the instance-level, and use noise-contrastive estimation to tackle the computational challenges imposed by the large number of instance classes. Our experimental results demonstrate that, under unsupervised learning settings, our method surpasses the state-of-the-art on ImageNet classification by a large margin. Our method is also remarkable for consistently improving test performance with more training data and better network architectures. By fine-tuning the learned feature, we further obtain competitive results for semi-supervised learning and object detection tasks. Our non-parametric model is highly compact: With 128 features per image, our method requires only 600MB storage for a million images, enabling fast nearest neighbour retrieval at the run time.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\self supervised learning\\Wu et al_2018_Unsupervised Feature Learning via Non-Parametric Instance-level Discrimination.pdf;C\:\\Users\\chsey\\Zotero\\storage\\37BRT4TM\\1805.html}
}

@inproceedings{wuWhyPromptTuning2023,
  title = {Why {{Is Prompt Tuning}} for {{Vision-Language Models Robust}} to {{Noisy Labels}}?},
  author = {Wu, Cheng-En and Tian, Yu and Yu, Haichao and Wang, Heng and Morgado, Pedro and Hu, Yu Hen and Yang, Linjie},
  date = {2023},
  pages = {15488--15497},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Wu_Why_Is_Prompt_Tuning_for_Vision-Language_Models_Robust_to_Noisy_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Wu et al_2023_Why Is Prompt Tuning for Vision-Language Models Robust to Noisy Labels.pdf}
}

@article{wyss-gallifentMATH401MATH431Linear,
  title = {{{MATH401}}/{{MATH431}}: {{Linear Algebra Review}}},
  author = {Wyss-Gallifent, Justin},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\QAA94T84\Wyss-Gallifent - MATH401MATH431 Linear Algebra Review.pdf}
}

@article{wyss-gallifentMATH4312DGraphics,
  title = {{{MATH431}}: {{2D Graphics Basics}}},
  author = {Wyss-Gallifent, Justin},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\VWLMYN7X\Wyss-Gallifent - MATH431 2D Graphics Basics.pdf}
}

@article{wyss-gallifentMATH431GeometricAlgebra,
  title = {{{MATH431}}: {{Geometric Algebra}}},
  author = {Wyss-Gallifent, Justin},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\MHZX4BPC\Wyss-Gallifent - MATH431 Geometric Algebra.pdf}
}

@article{wyss-gallifentMATH431RealProjective,
  title = {{{MATH431}}: {{Real Projective}} 3-{{Space}}},
  author = {Wyss-Gallifent, Justin},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\UMD_vision\Wyss-Gallifent_MATH431.pdf}
}

@article{wyss-gallifentMATH431RealProjectivea,
  title = {{{MATH431}}: {{Real Projective}} 2-{{Space}}},
  author = {Wyss-Gallifent, Justin},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\FWLWEW5J\Wyss-Gallifent - MATH431 Real Projective 2-Space.pdf}
}

@online{xiaoFlorence2AdvancingUnified2023,
  title = {Florence-2: {{Advancing}} a {{Unified Representation}} for a {{Variety}} of {{Vision Tasks}}},
  shorttitle = {Florence-2},
  author = {Xiao, Bin and Wu, Haiping and Xu, Weijian and Dai, Xiyang and Hu, Houdong and Lu, Yumao and Zeng, Michael and Liu, Ce and Yuan, Lu},
  date = {2023-11-10},
  eprint = {2311.06242},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2311.06242},
  url = {http://arxiv.org/abs/2311.06242},
  urldate = {2024-03-21},
  abstract = {We introduce Florence-2, a novel vision foundation model with a unified, prompt-based representation for a variety of computer vision and vision-language tasks. While existing large vision models excel in transfer learning, they struggle to perform a diversity of tasks with simple instructions, a capability that implies handling the complexity of various spatial hierarchy and semantic granularity. Florence-2 was designed to take text-prompt as task instructions and generate desirable results in text forms, whether it be captioning, object detection, grounding or segmentation. This multi-task learning setup demands large-scale, high-quality annotated data. To this end, we co-developed FLD-5B that consists of 5.4 billion comprehensive visual annotations on 126 million images, using an iterative strategy of automated image annotation and model refinement. We adopted a sequence-to-sequence structure to train Florence-2 to perform versatile and comprehensive vision tasks. Extensive evaluations on numerous tasks demonstrated Florence-2 to be a strong vision foundation model contender with unprecedented zero-shot and fine-tuning capabilities.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Xiao et al_2023_Florence-2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\DIP7I9IA\\2311.html}
}

@online{xieDiffFitUnlockingTransferability2023,
  title = {{{DiffFit}}: {{Unlocking Transferability}} of {{Large Diffusion Models}} via {{Simple Parameter-Efficient Fine-Tuning}}},
  shorttitle = {{{DiffFit}}},
  author = {Xie, Enze and Yao, Lewei and Shi, Han and Liu, Zhili and Zhou, Daquan and Liu, Zhaoqiang and Li, Jiawei and Li, Zhenguo},
  date = {2023-07-27},
  eprint = {2304.06648},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2304.06648},
  url = {http://arxiv.org/abs/2304.06648},
  urldate = {2023-10-15},
  abstract = {Diffusion models have proven to be highly effective in generating high-quality images. However, adapting large pre-trained diffusion models to new domains remains an open challenge, which is critical for real-world applications. This paper proposes DiffFit, a parameter-efficient strategy to fine-tune large pre-trained diffusion models that enable fast adaptation to new domains. DiffFit is embarrassingly simple that only fine-tunes the bias term and newly-added scaling factors in specific layers, yet resulting in significant training speed-up and reduced model storage costs. Compared with full fine-tuning, DiffFit achieves 2\$\textbackslash times\$ training speed-up and only needs to store approximately 0.12\textbackslash\% of the total model parameters. Intuitive theoretical analysis has been provided to justify the efficacy of scaling factors on fast adaptation. On 8 downstream datasets, DiffFit achieves superior or competitive performances compared to the full fine-tuning while being more efficient. Remarkably, we show that DiffFit can adapt a pre-trained low-resolution generative model to a high-resolution one by adding minimal cost. Among diffusion-based methods, DiffFit sets a new state-of-the-art FID of 3.02 on ImageNet 512\$\textbackslash times\$512 benchmark by fine-tuning only 25 epochs from a public pre-trained ImageNet 256\$\textbackslash times\$256 checkpoint while being 30\$\textbackslash times\$ more training efficient than the closest competitor.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\iccv_2023_prompt\\Xie et al_2023_DiffFit.pdf;C\:\\Users\\chsey\\Zotero\\storage\\ZQUDCY8M\\2304.html}
}

@online{xieExploringRandomlyWired2019,
  title = {Exploring {{Randomly Wired Neural Networks}} for {{Image Recognition}}},
  author = {Xie, Saining and Kirillov, Alexander and Girshick, Ross and He, Kaiming},
  date = {2019-04-08},
  eprint = {1904.01569},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.01569},
  url = {http://arxiv.org/abs/1904.01569},
  urldate = {2023-08-05},
  abstract = {Neural networks for image recognition have evolved through extensive manual design from simple chain-like models to structures with multiple wiring paths. The success of ResNets and DenseNets is due in large part to their innovative wiring plans. Now, neural architecture search (NAS) studies are exploring the joint optimization of wiring and operation types, however, the space of possible wirings is constrained and still driven by manual design despite being searched. In this paper, we explore a more diverse set of connectivity patterns through the lens of randomly wired neural networks. To do this, we first define the concept of a stochastic network generator that encapsulates the entire network generation process. Encapsulation provides a unified view of NAS and randomly wired networks. Then, we use three classical random graph models to generate randomly wired graphs for networks. The results are surprising: several variants of these random generators yield network instances that have competitive accuracy on the ImageNet benchmark. These results suggest that new efforts focusing on designing better network generators may lead to new breakthroughs by exploring less constrained search spaces with more room for novel design.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\neural architecture search\\Xie et al_2019_Exploring Randomly Wired Neural Networks for Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7QY8JJKI\\1904.html}
}

@online{xieSegmentingTransparentObject2021,
  title = {Segmenting {{Transparent Object}} in the {{Wild}} with {{Transformer}}},
  author = {Xie, Enze and Wang, Wenjia and Wang, Wenhai and Sun, Peize and Xu, Hang and Liang, Ding and Luo, Ping},
  date = {2021-02-23},
  eprint = {2101.08461},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2101.08461},
  url = {http://arxiv.org/abs/2101.08461},
  urldate = {2023-02-03},
  abstract = {This work presents a new fine-grained transparent object segmentation dataset, termed Trans10K-v2, extending Trans10K-v1, the first large-scale transparent object segmentation dataset. Unlike Trans10K-v1 that only has two limited categories, our new dataset has several appealing benefits. (1) It has 11 fine-grained categories of transparent objects, commonly occurring in the human domestic environment, making it more practical for real-world application. (2) Trans10K-v2 brings more challenges for the current advanced segmentation methods than its former version. Furthermore, a novel transformer-based segmentation pipeline termed Trans2Seg is proposed. Firstly, the transformer encoder of Trans2Seg provides the global receptive field in contrast to CNN's local receptive field, which shows excellent advantages over pure CNN architectures. Secondly, by formulating semantic segmentation as a problem of dictionary look-up, we design a set of learnable prototypes as the query of Trans2Seg's transformer decoder, where each prototype learns the statistics of one category in the whole dataset. We benchmark more than 20 recent semantic segmentation methods, demonstrating that Trans2Seg significantly outperforms all the CNN-based methods, showing the proposed algorithm's potential ability to solve transparent object segmentation.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\transparent_segmentation\\Xie et al_2021_Segmenting Transparent Object in the Wild with Transformer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NZ6LSGHE\\2101.html}
}

@online{xieSelftrainingNoisyStudent2020,
  title = {Self-Training with {{Noisy Student}} Improves {{ImageNet}} Classification},
  author = {Xie, Qizhe and Luong, Minh-Thang and Hovy, Eduard and Le, Quoc V.},
  date = {2020-06-19},
  eprint = {1911.04252},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1911.04252},
  url = {http://arxiv.org/abs/1911.04252},
  urldate = {2022-07-09},
  abstract = {We present Noisy Student Training, a semi-supervised learning approach that works well even when labeled data is abundant. Noisy Student Training achieves 88.4\% top-1 accuracy on ImageNet, which is 2.0\% better than the state-of-the-art model that requires 3.5B weakly labeled Instagram images. On robustness test sets, it improves ImageNet-A top-1 accuracy from 61.0\% to 83.7\%, reduces ImageNet-C mean corruption error from 45.7 to 28.3, and reduces ImageNet-P mean flip rate from 27.8 to 12.2. Noisy Student Training extends the idea of self-training and distillation with the use of equal-or-larger student models and noise added to the student during learning. On ImageNet, we first train an EfficientNet model on labeled images and use it as a teacher to generate pseudo labels for 300M unlabeled images. We then train a larger EfficientNet as a student model on the combination of labeled and pseudo labeled images. We iterate this process by putting back the student as the teacher. During the learning of the student, we inject noise such as dropout, stochastic depth, and data augmentation via RandAugment to the student so that the student generalizes better than the teacher. Models are available at https://github.com/tensorflow/tpu/tree/master/models/official/efficientnet. Code is available at https://github.com/google-research/noisystudent.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\Computer Vision\\augmentation\\Xie et al_2020_Self-training with Noisy Student improves ImageNet classification.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HULHLUJ2\\1911.html}
}

@online{xieVectorQuantizedDiffusion2023,
  title = {Vector {{Quantized Diffusion Model}} with {{CodeUnet}} for {{Text-to-Sign Pose Sequences Generation}}},
  author = {Xie, Pan and Zhang, Qipeng and Li, Zexian and Tang, Hao and Du, Yao and Hu, Xiaohui},
  date = {2023-02-12},
  eprint = {2208.09141},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2208.09141},
  urldate = {2023-05-16},
  abstract = {Sign Language Production (SLP) aims to translate spoken languages into sign sequences automatically. The core process of SLP is to transform sign gloss sequences into their corresponding sign pose sequences (G2P). Most existing G2P models usually perform this conditional long-range generation in an autoregressive manner, which inevitably leads to an accumulation of errors. To address this issue, we propose a vector quantized diffusion method for conditional pose sequences generation, called PoseVQ-Diffusion, which is an iterative non-autoregressive method. Specifically, we first introduce a vector quantized variational autoencoder (Pose-VQVAE) model to represent a pose sequence as a sequence of latent codes. Then we model the latent discrete space by an extension of the recently developed diffusion architecture. To better leverage the spatial-temporal information, we introduce a novel architecture, namely CodeUnet, to generate higher quality pose sequence in the discrete space. Moreover, taking advantage of the learned codes, we develop a novel sequential k-nearest-neighbours method to predict the variable lengths of pose sequences for corresponding gloss sequences. Consequently, compared with the autoregressive G2P models, our model has a faster sampling speed and produces significantly better results. Compared with previous non-autoregressive G2P methods, PoseVQ-Diffusion improves the predicted results with iterative refinements, thus achieving state-of-the-art results on the SLP evaluation benchmark.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_PBL\\Xie et al_2023_Vector Quantized Diffusion Model with CodeUnet for Text-to-Sign Pose Sequences.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NPR2W88E\\2208.html}
}

@software{XrayImageSegmentation2022,
  title = {X-Ray Image Segmentation},
  date = {2022-06-21T08:06:35Z},
  origdate = {2018-05-01T19:06:14Z},
  url = {https://github.com/IvisionLab/dental-image},
  urldate = {2022-07-09},
  abstract = {Panoramic X-ray image segmentation},
  organization = {Intelligent Vision Research Lab}
}

@online{xuBridgeTowerBuildingBridges2024,
  title = {{{BridgeTower}}: {{Building Bridges Between Encoders}} in {{Vision-Language Representation Learning}}},
  shorttitle = {{{BridgeTower}}},
  author = {Xu, Xiao and Wu, Chenfei and Rosenman, Shachar and Lal, Vasudev and Che, Wanxiang and Duan, Nan},
  date = {2024-03-26},
  eprint = {2206.08657},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.08657},
  urldate = {2024-06-14},
  abstract = {Vision-Language (VL) models with the TWO-TOWER architecture have dominated visual-language representation learning in recent years. Current VL models either use lightweight unimodal encoders and learn to extract, align and fuse both modalities simultaneously in a deep cross-modal encoder, or feed the last-layer uni-modal representations from the deep pre-trained uni-modal encoders into the top cross-modal encoder. Both approaches potentially restrict vision-language representation learning and limit model performance. In this paper, we propose BRIDGETOWER, which introduces multiple bridge layers that build a connection between the top layers of uni-modal encoders and each layer of the cross-modal encoder. This enables effective bottom-up cross-modal alignment and fusion between visual and textual representations of different semantic levels of pre-trained uni-modal encoders in the cross-modal encoder. Pre-trained with only 4M images, BRIDGETOWER achieves state-of-the-art performance on various downstream vision-language tasks. In particular, on the VQAv2 test-std set, BRIDGETOWER achieves an accuracy of 78.73\%, outperforming the previous state-of-the-art model METER by 1.09\% with the same pre-training data and almost negligible additional parameters and computational costs. Notably, when further scaling the model, BRIDGETOWER achieves an accuracy of 81.15\%, surpassing models that are pre-trained on orders-ofmagnitude larger datasets. Code and checkpoints are available at https://github.com/microsoft/BridgeTower.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\RL64LCVF\Xu 등 - 2024 - BridgeTower Building Bridges Between Encoders in .pdf}
}

@online{xuBridgeTowerBuildingBridges2024a,
  title = {{{BridgeTower}}: {{Building Bridges Between Encoders}} in {{Vision-Language Representation Learning}}},
  shorttitle = {{{BridgeTower}}},
  author = {Xu, Xiao and Wu, Chenfei and Rosenman, Shachar and Lal, Vasudev and Che, Wanxiang and Duan, Nan},
  date = {2024-03-26},
  eprint = {2206.08657},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2206.08657},
  urldate = {2024-06-14},
  abstract = {Vision-Language (VL) models with the TWO-TOWER architecture have dominated visual-language representation learning in recent years. Current VL models either use lightweight unimodal encoders and learn to extract, align and fuse both modalities simultaneously in a deep cross-modal encoder, or feed the last-layer uni-modal representations from the deep pre-trained uni-modal encoders into the top cross-modal encoder. Both approaches potentially restrict vision-language representation learning and limit model performance. In this paper, we propose BRIDGETOWER, which introduces multiple bridge layers that build a connection between the top layers of uni-modal encoders and each layer of the cross-modal encoder. This enables effective bottom-up cross-modal alignment and fusion between visual and textual representations of different semantic levels of pre-trained uni-modal encoders in the cross-modal encoder. Pre-trained with only 4M images, BRIDGETOWER achieves state-of-the-art performance on various downstream vision-language tasks. In particular, on the VQAv2 test-std set, BRIDGETOWER achieves an accuracy of 78.73\%, outperforming the previous state-of-the-art model METER by 1.09\% with the same pre-training data and almost negligible additional parameters and computational costs. Notably, when further scaling the model, BRIDGETOWER achieves an accuracy of 81.15\%, surpassing models that are pre-trained on orders-ofmagnitude larger datasets. Code and checkpoints are available at https://github.com/microsoft/BridgeTower.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\M7RTW939\Xu 등 - 2024 - BridgeTower Building Bridges Between Encoders in .pdf}
}

@online{xuDemystifyingCLIPData2024,
  title = {Demystifying {{CLIP Data}}},
  author = {Xu, Hu and Xie, Saining and Tan, Xiaoqing Ellen and Huang, Po-Yao and Howes, Russell and Sharma, Vasu and Li, Shang-Wen and Ghosh, Gargi and Zettlemoyer, Luke and Feichtenhofer, Christoph},
  date = {2024-04-07},
  eprint = {2309.16671},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2309.16671},
  urldate = {2024-04-24},
  abstract = {Contrastive Language-Image Pre-training (CLIP) is an approach that has advanced research and applications in computer vision, fueling modern recognition systems and generative models. We believe that the main ingredient to the success of CLIP is its data and not the model architecture or pre-training objective. However, CLIP only provides very limited information about its data and how it has been collected, leading to works that aim to reproduce CLIP's data by filtering with its model parameters. In this work, we intend to reveal CLIP's data curation approach and in our pursuit of making it open to the community introduce Metadata-Curated Language-Image Pre-training (MetaCLIP). MetaCLIP takes a raw data pool and metadata (derived from CLIP's concepts) and yields a balanced subset over the metadata distribution. Our experimental study rigorously isolates the model and training settings, concentrating solely on data. MetaCLIP applied to CommonCrawl with 400M image-text data pairs outperforms CLIP's data on multiple standard benchmarks. In zero-shot ImageNet classification, MetaCLIP achieves 70.8\% accuracy, surpassing CLIP's 68.3\% on ViT-B models. Scaling to 1B data, while maintaining the same training budget, attains 72.4\%. Our observations hold across various model sizes, exemplified by ViT-H achieving 80.5\%, without any bells-and-whistles. Curation code and training data distribution on metadata is made available at https://github.com/facebookresearch/MetaCLIP.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Xu et al_2024_Demystifying CLIP Data.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HRMRANE4\\2309.html}
}

@online{xuMultimodalLearningTransformers2023,
  title = {Multimodal {{Learning}} with {{Transformers}}: {{A Survey}}},
  shorttitle = {Multimodal {{Learning}} with {{Transformers}}},
  author = {Xu, Peng and Zhu, Xiatian and Clifton, David A.},
  date = {2023-05-09},
  eprint = {2206.06488},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2206.06488},
  url = {http://arxiv.org/abs/2206.06488},
  urldate = {2024-01-25},
  abstract = {Transformer is a promising neural network learner, and has achieved great success in various machine learning tasks. Thanks to the recent prevalence of multimodal applications and big data, Transformer-based multimodal learning has become a hot topic in AI research. This paper presents a comprehensive survey of Transformer techniques oriented at multimodal data. The main contents of this survey include: (1) a background of multimodal learning, Transformer ecosystem, and the multimodal big data era, (2) a theoretical review of Vanilla Transformer, Vision Transformer, and multimodal Transformers, from a geometrically topological perspective, (3) a review of multimodal Transformer applications, via two important paradigms, i.e., for multimodal pretraining and for specific multimodal tasks, (4) a summary of the common challenges and designs shared by the multimodal Transformer models and applications, and (5) a discussion of open problems and potential research directions for the community.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Xu et al_2023_Multimodal Learning with Transformers.pdf;Y\:\\research\\research_paper\\multimodal-learning-with-transformers-a-survey - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\D2V3B8QD\\2206.html}
}

@online{xuPointNeRFPointbasedNeural2023,
  title = {Point-{{NeRF}}: {{Point-based Neural Radiance Fields}}},
  shorttitle = {Point-{{NeRF}}},
  author = {Xu, Qiangeng and Xu, Zexiang and Philip, Julien and Bi, Sai and Shu, Zhixin and Sunkavalli, Kalyan and Neumann, Ulrich},
  date = {2023-03-15},
  eprint = {2201.08845},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2201.08845},
  urldate = {2023-06-26},
  abstract = {Volumetric neural rendering methods like NeRF generate high-quality view synthesis results but are optimized per-scene leading to prohibitive reconstruction time. On the other hand, deep multi-view stereo methods can quickly reconstruct scene geometry via direct network inference. Point-NeRF combines the advantages of these two approaches by using neural 3D point clouds, with associated neural features, to model a radiance field. Point-NeRF can be rendered efficiently by aggregating neural point features near scene surfaces, in a ray marching-based rendering pipeline. Moreover, Point-NeRF can be initialized via direct inference of a pre-trained deep network to produce a neural point cloud; this point cloud can be finetuned to surpass the visual quality of NeRF with 30X faster training time. Point-NeRF can be combined with other 3D reconstruction methods and handles the errors and outliers in such methods via a novel pruning and growing mechanism. The experiments on the DTU, the NeRF Synthetics , the ScanNet and the Tanks and Temples datasets demonstrate Point-NeRF can surpass the existing methods and achieve the state-of-the-art results.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\Xu et al_2023_Point-NeRF.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JKCZ5KIN\\2201.html}
}

@inproceedings{xuPromptingDecisionTransformer2022,
  title = {Prompting {{Decision Transformer}} for {{Few-Shot Policy Generalization}}},
  booktitle = {Proceedings of the 39th {{International Conference}} on {{Machine Learning}}},
  author = {Xu, Mengdi and Shen, Yikang and Zhang, Shun and Lu, Yuchen and Zhao, Ding and Tenenbaum, Joshua and Gan, Chuang},
  date = {2022-06-28},
  pages = {24631--24645},
  publisher = {PMLR},
  issn = {2640-3498},
  url = {https://proceedings.mlr.press/v162/xu22g.html},
  urldate = {2024-05-07},
  abstract = {Human can leverage prior experience and learn novel tasks from a handful of demonstrations. In contrast to offline meta-reinforcement learning, which aims to achieve quick adaptation through better algorithm design, we investigate the effect of architecture inductive bias on the few-shot learning capability. We propose a Prompt-based Decision Transformer (Prompt-DT), which leverages the sequential modeling ability of the Transformer architecture and the prompt framework to achieve few-shot adaptation in offline RL. We design the trajectory prompt, which contains segments of the few-shot demonstrations, and encodes task-specific information to guide policy generation. Our experiments in five MuJoCo control benchmarks show that Prompt-DT is a strong few-shot learner without any extra finetuning on unseen target tasks. Prompt-DT outperforms its variants and strong meta offline RL baselines by a large margin with a trajectory prompt containing only a few timesteps. Prompt-DT is also robust to prompt length changes and can generalize to out-of-distribution (OOD) environments. Project page: \textbackslash href\{https://mxu34.github.io/PromptDT/\}\{https://mxu34.github.io/PromptDT/\}.},
  eventtitle = {International {{Conference}} on {{Machine Learning}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Xu et al_2022_Prompting Decision Transformer for Few-Shot Policy Generalization.pdf}
}

@inproceedings{xuSelfCalibratedCrossAttention2023,
  title = {Self-{{Calibrated Cross Attention Network}} for {{Few-Shot Segmentation}}},
  author = {Xu, Qianxiong and Zhao, Wenting and Lin, Guosheng and Long, Cheng},
  date = {2023},
  pages = {655--665},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Xu_Self-Calibrated_Cross_Attention_Network_for_Few-Shot_Segmentation_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion,Segmentation},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Xu et al_2023_Self-Calibrated Cross Attention Network for Few-Shot Segmentation.pdf}
}

@online{xuTensorGPTEfficientCompression2023,
  title = {{{TensorGPT}}: {{Efficient Compression}} of the {{Embedding Layer}} in {{LLMs}} Based on the {{Tensor-Train Decomposition}}},
  shorttitle = {{{TensorGPT}}},
  author = {Xu, Mingxue and Xu, Yao Lei and Mandic, Danilo P.},
  date = {2023-07-02},
  eprint = {2307.00526},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  doi = {10.48550/arXiv.2307.00526},
  url = {http://arxiv.org/abs/2307.00526},
  urldate = {2024-04-16},
  abstract = {High-dimensional token embeddings underpin Large Language Models (LLMs), as they can capture subtle semantic information and significantly enhance the modelling of complex language patterns. However, the associated high dimensionality also introduces considerable model parameters, and a prohibitively high model storage. To address this issue, this work proposes an approach based on the Tensor-Train Decomposition (TTD), where each token embedding is treated as a Matrix Product State (MPS) that can be efficiently computed in a distributed manner. The experimental results on GPT-2 demonstrate that, through our approach, the embedding layer can be compressed by a factor of up to 38.40 times, and when the compression factor is 3.31 times, even produced a better performance than the original GPT-2 model.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,Mathematics - Numerical Analysis,notion},
  file = {Y\:\\paper\\2024_research\\Xu et al_2023_TensorGPT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\9U8G7VZ9\\2307.html}
}

@article{xuTrainingFreePretrainedModel,
  title = {Training-{{Free Pretrained Model Merging}}},
  author = {Xu, Zhengqi and Yuan, Ke and Wang, Huiqiong and Wang, Yong and Song, Mingli and Song, Jie},
  abstract = {Recently, model merging techniques have surfaced as a solution to combine multiple single-talent models into a single multi-talent model. However, previous endeavors in this field have either necessitated additional training or finetuning processes, or require that the models possess the same pre-trained initialization. In this work, we identify a common drawback in prior works w.r.t. the inconsistency of unit similarity in the weight space and the activation space. To address this inconsistency, we propose an innovative model merging framework, coined as merging under dual-space constraints (MuDSC). Specifically, instead of solely maximizing the objective of a single space, we advocate for the exploration of permutation matrices situated in a region with a unified high similarity in the dual space, achieved through the linear combination of activation and weight similarity matrices. In order to enhance usability, we have also incorporated adaptations for group structure, including MultiHead Attention and Group Normalization. Comprehensive experimental comparisons demonstrate that MuDSC can significantly boost the performance of merged models with various task combinations and architectures. Furthermore, the visualization of the merged model within the multi-task loss landscape reveals that MuDSC enables the merged model to reside in the overlapping segment, featuring a unified lower loss for each task. Our code is publicly available at https://github.com/zju-vipa/training\_free\_model\_merging.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\P66UTIM4\Xu 등 - Training-Free Pretrained Model Merging.pdf}
}

@online{xuVASA1LifelikeAudioDriven2024,
  title = {{{VASA-1}}: {{Lifelike Audio-Driven Talking Faces Generated}} in {{Real Time}}},
  shorttitle = {{{VASA-1}}},
  author = {Xu, Sicheng and Chen, Guojun and Guo, Yu-Xiao and Yang, Jiaolong and Li, Chong and Zang, Zhenyu and Zhang, Yizhong and Tong, Xin and Guo, Baining},
  date = {2024-04-16},
  eprint = {2404.10667},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2404.10667},
  urldate = {2024-04-24},
  abstract = {We introduce VASA, a framework for generating lifelike talking faces with appealing visual affective skills (VAS) given a single static image and a speech audio clip. Our premiere model, VASA-1, is capable of not only producing lip movements that are exquisitely synchronized with the audio, but also capturing a large spectrum of facial nuances and natural head motions that contribute to the perception of authenticity and liveliness. The core innovations include a holistic facial dynamics and head movement generation model that works in a face latent space, and the development of such an expressive and disentangled face latent space using videos. Through extensive experiments including evaluation on a set of new metrics, we show that our method significantly outperforms previous methods along various dimensions comprehensively. Our method not only delivers high video quality with realistic facial and head dynamics but also supports the online generation of 512x512 videos at up to 40 FPS with negligible starting latency. It paves the way for real-time engagements with lifelike avatars that emulate human conversational behaviors.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Xu et al_2024_VASA-1.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NVD3ATFE\\2404.html}
}

@online{yadavTIESMergingResolvingInterference2023,
  title = {{{TIES-Merging}}: {{Resolving Interference When Merging Models}}},
  shorttitle = {{{TIES-Merging}}},
  author = {Yadav, Prateek and Tam, Derek and Choshen, Leshem and Raffel, Colin and Bansal, Mohit},
  date = {2023-10-27},
  eprint = {2306.01708},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2306.01708},
  urldate = {2024-10-26},
  abstract = {Transfer learning - i.e., further fine-tuning a pre-trained model on a downstream task - can confer significant advantages, including improved downstream performance, faster convergence, and better sample efficiency. These advantages have led to a proliferation of task-specific fine-tuned models, which typically can only perform a single task and do not benefit from one another. Recently, model merging techniques have emerged as a solution to combine multiple task-specific models into a single multitask model without performing additional training. However, existing merging methods often ignore the interference between parameters of different models, resulting in large performance drops when merging multiple models. In this paper, we demonstrate that prior merging techniques inadvertently lose valuable information due to two major sources of interference: (a) interference due to redundant parameter values and (b) disagreement on the sign of a given parameter's values across models. To address this, we propose our method, TRIM, ELECT SIGN \& MERGE (TIES-Merging), which introduces three novel steps when merging models: (1) resetting parameters that only changed a small amount during fine-tuning, (2) resolving sign conflicts, and (3) merging only the parameters that are in alignment with the final agreed-upon sign. We find that TIES-Merging outperforms several existing methods in diverse settings covering a range of modalities, domains, number of tasks, model sizes, architectures, and fine-tuning settings. We further analyze the impact of different types of interference on model parameters, and highlight the importance of resolving sign interference. Our code is available at https://github.com/prateeky2806/ties-merging},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Yadav et al_2023_TIES-Merging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JHNTSM3D\\2306.html}
}

@online{yadavTIESMergingResolvingInterference2023a,
  title = {{{TIES-Merging}}: {{Resolving Interference When Merging Models}}},
  shorttitle = {{{TIES-Merging}}},
  author = {Yadav, Prateek and Tam, Derek and Choshen, Leshem and Raffel, Colin and Bansal, Mohit},
  date = {2023-10-26},
  eprint = {2306.01708},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2306.01708},
  urldate = {2024-09-12},
  abstract = {Transfer learning - i.e., further fine-tuning a pre-trained model on a downstream task - can confer significant advantages, including improved downstream performance, faster convergence, and better sample efficiency. These advantages have led to a proliferation of task-specific fine-tuned models, which typically can only perform a single task and do not benefit from one another. Recently, model merging techniques have emerged as a solution to combine multiple task-specific models into a single multitask model without performing additional training. However, existing merging methods often ignore the interference between parameters of different models, resulting in large performance drops when merging multiple models. In this paper, we demonstrate that prior merging techniques inadvertently lose valuable information due to two major sources of interference: (a) interference due to redundant parameter values and (b) disagreement on the sign of a given parameter's values across models. To address this, we propose our method, TRIM, ELECT SIGN \& MERGE (TIES-Merging), which introduces three novel steps when merging models: (1) resetting parameters that only changed a small amount during fine-tuning, (2) resolving sign conflicts, and (3) merging only the parameters that are in alignment with the final agreed-upon sign. We find that TIES-Merging outperforms several existing methods in diverse settings covering a range of modalities, domains, number of tasks, model sizes, architectures, and fine-tuning settings. We further analyze the impact of different types of interference on model parameters, and highlight the importance of resolving sign interference. Our code is available at https://github.com/prateeky2806/ties-merging},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\9HIGUJGM\Yadav 등 - 2023 - TIES-Merging Resolving Interference When Merging .pdf}
}

@inproceedings{yanEffectivePrioritizingWater2013,
  title = {Towards Effective Prioritizing Water Pipe Replacement and Rehabilitation},
  booktitle = {Proceedings of the {{Twenty-Third}} International Joint Conference on {{Artificial Intelligence}}},
  author = {Yan, Junchi and Wang, Yu and Zhou, Ke and Huang, Jin and Tian, Chunhua and Zha, Hongyuan and Dong, Weishan},
  year = {8월 3, 2013},
  series = {{{IJCAI}} '13},
  pages = {2931--2937},
  publisher = {AAAI Press},
  location = {Beijing, China},
  abstract = {Water pipe failures can not only have a great impact on people's daily life but also cause significant waste of water which is an essential and precious resource to human beings. As a result, preventative maintenance for water pipes, particularly in urban-scale networks, is of great importance for a sustainable society. To achieve effective replacement and rehabilitation, failure prediction aims to proactively find those 'most-likely-to-fail' pipes becomes vital and has been attracting more attention from both academia and industry, especially from the civil engineering field. This paper presents an already-deployed industrial computational system for pipe failure prediction. As an alternative to risk matrix methods often depending on ad-hoc domain heuristics, learning based methods are adopted using the attributes with respect to physical, environmental, operational conditions and etc. Further challenge arises in practice when lacking of profile attributes. A dive into the failure records shows that the failure event sequences typically exhibit temporal clustering patterns, which motivates us to use the stochastic process to tackle the failure prediction task. Specifically, the failure sequence is formulated as a self-exciting stochastic process which is, to our best knowledge, a novel formulation for pipe failure prediction. And we show that it outperforms a baseline assuming the failure risk grows linearly with aging. Broad new problems and research points for the machine learning community are also introduced for future work.},
  isbn = {978-1-57735-633-2}
}

@inproceedings{yanFastGradientawareUpsampling2010,
  title = {Fast Gradient-Aware Upsampling for Cartoon Video},
  booktitle = {2010 {{International Conference}} on {{Image Analysis}} and {{Signal Processing}}},
  author = {Yan, Xing and Shen, Jianbing},
  date = {2010-04},
  pages = {636--639},
  issn = {2156-0129},
  doi = {10.1109/IASP.2010.5476190},
  abstract = {In this paper, we propose a novel fast gradient-aware upsampling approach for cartoon animation. The advantage of our method is that we don't need any prior knowledge and deconvolution stage to deblur the estimated result like existing methods. The low-resolution input video is initially upsampled to the desired high-resolution by a fast bicubic interpolation approach. After that, the gradient transformation is applied to the initially upsampled video frame. Finally, energy optimization is employed to recover additional fine details and structures. Our method is easy to implement and runs very fast. Moreover, in order to increase or decrease the sharpness of the reconstructed high resolution image, the user just needs to adjust one parameterg . Thus, our approach is suitable for the task of cartoon video upsampling.},
  eventtitle = {2010 {{International Conference}} on {{Image Analysis}} and {{Signal Processing}}},
  keywords = {Animation,Computer science,Gradient transformation,Image reconstruction,Image resolution,Information technology,Interpolation,Optimization,Signal resolution,Strontium,Transform coding,Upsampling,Video compression},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Yan_Shen_2010_Fast gradient-aware upsampling for cartoon video.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RU8JWCYS\\5476190.html}
}

@online{yangAdaMergingAdaptiveModel2024,
  title = {{{AdaMerging}}: {{Adaptive Model Merging}} for {{Multi-Task Learning}}},
  shorttitle = {{{AdaMerging}}},
  author = {Yang, Enneng and Wang, Zhenyi and Shen, Li and Liu, Shiwei and Guo, Guibing and Wang, Xingwei and Tao, Dacheng},
  date = {2024-05-28},
  eprint = {2310.02575},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2310.02575},
  urldate = {2024-10-29},
  abstract = {Multi-task learning (MTL) aims to empower a model to tackle multiple tasks simultaneously. A recent development known as task arithmetic has revealed that several models, each fine-tuned for distinct tasks, can be directly merged into a single model to execute MTL without necessitating a retraining process using the initial training data. Nevertheless, this direct addition of models often leads to a significant deterioration in the overall performance of the merged model. This decline occurs due to potential conflicts and intricate correlations among the multiple tasks. Consequently, the challenge emerges of how to merge pre-trained models more effectively without using their original training data. This paper introduces an innovative technique called Adaptive Model Merging (AdaMerging). This approach aims to autonomously learn the coefficients for model merging, either in a task-wise or layer-wise manner, without relying on the original training data. Specifically, our AdaMerging method operates as an automatic, unsupervised task arithmetic scheme. It leverages entropy minimization on unlabeled test samples from the multi-task setup as a surrogate objective function to iteratively refine the merging coefficients of the multiple models. Our experimental findings across eight tasks demonstrate the efficacy of the AdaMerging scheme we put forth. Compared to the current state-of-the-art task arithmetic merging scheme, AdaMerging showcases a remarkable 11\textbackslash\% improvement in performance. Notably, AdaMerging also exhibits superior generalization capabilities when applied to unseen downstream tasks. Furthermore, it displays a significantly enhanced robustness to data distribution shifts that may occur during the testing phase.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Yang et al_2024_AdaMerging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\I4AC5SUT\\2310.html}
}

@online{yangAdaMergingAdaptiveModel2024a,
  title = {{{AdaMerging}}: {{Adaptive Model Merging}} for {{Multi-Task Learning}}},
  shorttitle = {{{AdaMerging}}},
  author = {Yang, Enneng and Wang, Zhenyi and Shen, Li and Liu, Shiwei and Guo, Guibing and Wang, Xingwei and Tao, Dacheng},
  date = {2024-05-28},
  eprint = {2310.02575},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2310.02575},
  urldate = {2024-10-29},
  abstract = {Multi-task learning (MTL) aims to empower a model to tackle multiple tasks simultaneously. A recent development known as task arithmetic has revealed that several models, each fine-tuned for distinct tasks, can be directly merged into a single model to execute MTL without necessitating a retraining process using the initial training data. Nevertheless, this direct addition of models often leads to a significant deterioration in the overall performance of the merged model. This decline occurs due to potential conflicts and intricate correlations among the multiple tasks. Consequently, the challenge emerges of how to merge pre-trained models more effectively without using their original training data. This paper introduces an innovative technique called Adaptive Model Merging (AdaMerging). This approach aims to autonomously learn the coefficients for model merging, either in a task-wise or layer-wise manner, without relying on the original training data. Specifically, our AdaMerging method operates as an automatic, unsupervised task arithmetic scheme. It leverages entropy minimization on unlabeled test samples from the multi-task setup as a surrogate objective function to iteratively refine the merging coefficients of the multiple models. Our experimental findings across eight tasks demonstrate the efficacy of the AdaMerging scheme we put forth. Compared to the current state-of-the-art task arithmetic merging scheme, AdaMerging showcases a remarkable 11\textbackslash\% improvement in performance. Notably, AdaMerging also exhibits superior generalization capabilities when applied to unseen downstream tasks. Furthermore, it displays a significantly enhanced robustness to data distribution shifts that may occur during the testing phase.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Yang et al_2024_AdaMerging2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\34PQKJP4\\2310.html}
}

@inproceedings{yangComprehensiveSemiSupervisedMultiModal2019,
  title = {Comprehensive {{Semi-Supervised Multi-Modal Learning}}},
  booktitle = {Proceedings of the {{Twenty-Eighth International Joint Conference}} on {{Artificial Intelligence}}},
  author = {Yang, Yang and Wang, Ke-Tao and Zhan, De-Chuan and Xiong, Hui and Jiang, Yuan},
  date = {2019-08},
  pages = {4092--4098},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},
  location = {Macao, China},
  doi = {10.24963/ijcai.2019/568},
  url = {https://www.ijcai.org/proceedings/2019/568},
  urldate = {2024-05-29},
  abstract = {Multi-modal learning refers to the process of learning a precise model to represent the joint representations of different modalities. Despite its promise for multi-modal learning, the co-regularization method is based on the consistency principle with a sufficient assumption, which usually does not hold for real-world multi-modal data. Indeed, due to the modal insufficiency in real-world applications, there are divergences among heterogeneous modalities. This imposes a critical challenge for multi-modal learning. To this end, in this paper, we propose a novel Comprehensive Multi-Modal Learning (CMML) framework, which can strike a balance between the consistency and divergency modalities by considering the insufficiency in one unified framework. Specifically, we utilize an instance level attention mechanism to weight the sufficiency for each instance on different modalities. Moreover, novel diversity regularization and robust consistency metrics are designed for discovering insufficient modalities. Our empirical studies show the superior performances of CMML on real-world data in terms of various criteria.},
  eventtitle = {Twenty-{{Eighth International Joint Conference}} on {{Artificial Intelligence}} \{\vphantom\}{{IJCAI-19}}\vphantom\{\}},
  isbn = {978-0-9992411-4-1},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\GWXL8Q2X\Yang 등 - 2019 - Comprehensive Semi-Supervised Multi-Modal Learning.pdf}
}

@online{yangDenseCaptioningJoint2017,
  title = {Dense {{Captioning}} with {{Joint Inference}} and {{Visual Context}}},
  author = {Yang, Linjie and Tang, Kevin and Yang, Jianchao and Li, Li-Jia},
  date = {2017-08-07},
  eprint = {1611.06949},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1611.06949},
  url = {http://arxiv.org/abs/1611.06949},
  urldate = {2023-05-28},
  abstract = {Dense captioning is a newly emerging computer vision topic for understanding images with dense language descriptions. The goal is to densely detect visual concepts (e.g., objects, object parts, and interactions between them) from images, labeling each with a short descriptive phrase. We identify two key challenges of dense captioning that need to be properly addressed when tackling the problem. First, dense visual concept annotations in each image are associated with highly overlapping target regions, making accurate localization of each visual concept challenging. Second, the large amount of visual concepts makes it hard to recognize each of them by appearance alone. We propose a new model pipeline based on two novel ideas, joint inference and context fusion, to alleviate these two challenges. We design our model architecture in a methodical manner and thoroughly evaluate the variations in architecture. Our final model, compact and efficient, achieves state-of-the-art accuracy on Visual Genome for dense captioning with a relative gain of 73\textbackslash\% compared to the previous best algorithm. Qualitative experiments also reveal the semantic capabilities of our model in dense captioning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Yang et al_2017_Dense Captioning with Joint Inference and Visual Context.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VUE38N97\\1611.html}
}

@online{yangDepthAnythingUnleashing2024,
  title = {Depth {{Anything}}: {{Unleashing}} the {{Power}} of {{Large-Scale Unlabeled Data}}},
  shorttitle = {Depth {{Anything}}},
  author = {Yang, Lihe and Kang, Bingyi and Huang, Zilong and Xu, Xiaogang and Feng, Jiashi and Zhao, Hengshuang},
  date = {2024-01-19},
  eprint = {2401.10891},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2401.10891},
  urldate = {2024-03-13},
  abstract = {This work presents Depth Anything, a highly practical solution for robust monocular depth estimation. Without pursuing novel technical modules, we aim to build a simple yet powerful foundation model dealing with any images under any circumstances. To this end, we scale up the dataset by designing a data engine to collect and automatically annotate large-scale unlabeled data (\textasciitilde 62M), which significantly enlarges the data coverage and thus is able to reduce the generalization error. We investigate two simple yet effective strategies that make data scaling-up promising. First, a more challenging optimization target is created by leveraging data augmentation tools. It compels the model to actively seek extra visual knowledge and acquire robust representations. Second, an auxiliary supervision is developed to enforce the model to inherit rich semantic priors from pre-trained encoders. We evaluate its zero-shot capabilities extensively, including six public datasets and randomly captured photos. It demonstrates impressive generalization ability. Further, through fine-tuning it with metric depth information from NYUv2 and KITTI, new SOTAs are set. Our better depth model also results in a better depth-conditioned ControlNet. Our models are released at https://github.com/LiheYoung/Depth-Anything.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Yang et al_2024_Depth Anything.pdf;C\:\\Users\\chsey\\Zotero\\storage\\AFPGDTZ4\\2401.html}
}

@incollection{yangFashionCaptioningGenerating2020,
  title = {Fashion {{Captioning}}: {{Towards Generating Accurate Descriptions}} with {{Semantic Rewards}}},
  shorttitle = {Fashion {{Captioning}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2020},
  author = {Yang, Xuewen and Zhang, Heming and Jin, Di and Liu, Yingru and Wu, Chi-Hao and Tan, Jianchao and Xie, Dongliang and Wang, Jue and Wang, Xin},
  editor = {Vedaldi, Andrea and Bischof, Horst and Brox, Thomas and Frahm, Jan-Michael},
  date = {2020},
  volume = {12358},
  pages = {1--17},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-030-58601-0_1},
  url = {https://link.springer.com/10.1007/978-3-030-58601-0_1},
  urldate = {2023-05-28},
  isbn = {978-3-030-58600-3 978-3-030-58601-0},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Yang et al_2020_Fashion Captioning.pdf}
}

@inproceedings{yangOneShotGenerativeDomain2023,
  title = {One-{{Shot Generative Domain Adaptation}}},
  author = {Yang, Ceyuan and Shen, Yujun and Zhang, Zhiyi and Xu, Yinghao and Zhu, Jiapeng and Wu, Zhirong and Zhou, Bolei},
  date = {2023},
  pages = {7733--7742},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Yang_One-Shot_Generative_Domain_Adaptation_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {domain adaptation,notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Yang et al_2023_One-Shot Generative Domain Adaptation.pdf}
}

@online{yangPanopticSceneGraph2022,
  title = {Panoptic {{Scene Graph Generation}}},
  author = {Yang, Jingkang and Ang, Yi Zhe and Guo, Zujin and Zhou, Kaiyang and Zhang, Wayne and Liu, Ziwei},
  date = {2022-07-22},
  eprint = {2207.11247},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2207.11247},
  url = {http://arxiv.org/abs/2207.11247},
  urldate = {2023-04-24},
  abstract = {Existing research addresses scene graph generation (SGG) -- a critical technology for scene understanding in images -- from a detection perspective, i.e., objects are detected using bounding boxes followed by prediction of their pairwise relationships. We argue that such a paradigm causes several problems that impede the progress of the field. For instance, bounding box-based labels in current datasets usually contain redundant classes like hairs, and leave out background information that is crucial to the understanding of context. In this work, we introduce panoptic scene graph generation (PSG), a new problem task that requires the model to generate a more comprehensive scene graph representation based on panoptic segmentations rather than rigid bounding boxes. A high-quality PSG dataset, which contains 49k well-annotated overlapping images from COCO and Visual Genome, is created for the community to keep track of its progress. For benchmarking, we build four two-stage baselines, which are modified from classic methods in SGG, and two one-stage baselines called PSGTR and PSGFormer, which are based on the efficient Transformer-based detector, i.e., DETR. While PSGTR uses a set of queries to directly learn triplets, PSGFormer separately models the objects and relations in the form of queries from two Transformer decoders, followed by a prompting-like relation-object matching mechanism. In the end, we share insights on open challenges and future directions.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Multimedia},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Yang et al_2022_Panoptic Scene Graph Generation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KH4KQUT2\\2207.html}
}

@online{yangRepresentationSurgeryMultiTask2024,
  title = {Representation {{Surgery}} for {{Multi-Task Model Merging}}},
  author = {Yang, Enneng and Shen, Li and Wang, Zhenyi and Guo, Guibing and Chen, Xiaojun and Wang, Xingwei and Tao, Dacheng},
  date = {2024-05-28},
  eprint = {2402.02705},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2402.02705},
  urldate = {2024-10-29},
  abstract = {Multi-task learning (MTL) compresses the information from multiple tasks into a unified backbone to improve computational efficiency and generalization. Recent work directly merges multiple independently trained models to perform MTL instead of collecting their raw data for joint training, greatly expanding the application scenarios of MTL. However, by visualizing the representation distribution of existing model merging schemes, we find that the merged model often suffers from the dilemma of representation bias. That is, there is a significant discrepancy in the representation distribution between the merged and individual models, resulting in poor performance of merged MTL. In this paper, we propose a representation surgery solution called "Surgery" to reduce representation bias in the merged model. Specifically, Surgery is a lightweight task-specific module that takes the representation of the merged model as input and attempts to output the biases contained in the representation from the merged model. We then designed an unsupervised optimization objective that updates the Surgery module by minimizing the distance between the merged model's representation and the individual model's representation. Extensive experiments demonstrate significant MTL performance improvements when our Surgery module is applied to state-of-the-art (SOTA) model merging schemes.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Yang et al_2024_Representation Surgery for Multi-Task Model Merging.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V36DPNPS\\2402.html}
}

@incollection{yangSingleImageSuperResolutionBenchmark2014,
  title = {Single-{{Image Super-Resolution}}: {{A Benchmark}}},
  shorttitle = {Single-{{Image Super-Resolution}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2014},
  author = {Yang, Chih-Yuan and Ma, Chao and Yang, Ming-Hsuan},
  editor = {Fleet, David and Pajdla, Tomas and Schiele, Bernt and Tuytelaars, Tinne},
  date = {2014},
  volume = {8692},
  pages = {372--386},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-319-10593-2_25},
  url = {http://link.springer.com/10.1007/978-3-319-10593-2_25},
  urldate = {2022-09-26},
  abstract = {Single-image super-resolution is of great importance for vision applications, and numerous algorithms have been proposed in recent years. Despite the demonstrated success, these results are often generated based on different assumptions using different datasets and metrics. In this paper, we present a systematic benchmark evaluation for state-of-the-art single-image super-resolution algorithms. In addition to quantitative evaluations based on conventional full-reference metrics, human subject studies are carried out to evaluate image quality based on visual perception. The benchmark evaluations demonstrate the performance and limitations of state-of-the-art algorithms which sheds light on future research in single-image super-resolution.},
  isbn = {978-3-319-10592-5 978-3-319-10593-2},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\super-resolution\Yang et al_2014_Single-Image Super-Resolution.pdf}
}

@incollection{yangSingleImageSuperResolutionBenchmark2014a,
  title = {Single-{{Image Super-Resolution}}: {{A Benchmark}}},
  shorttitle = {Single-{{Image Super-Resolution}}},
  booktitle = {Computer {{Vision}} – {{ECCV}} 2014},
  author = {Yang, Chih-Yuan and Ma, Chao and Yang, Ming-Hsuan},
  editor = {Fleet, David and Pajdla, Tomas and Schiele, Bernt and Tuytelaars, Tinne},
  date = {2014},
  volume = {8692},
  pages = {372--386},
  publisher = {Springer International Publishing},
  location = {Cham},
  doi = {10.1007/978-3-319-10593-2_25},
  url = {http://link.springer.com/10.1007/978-3-319-10593-2_25},
  urldate = {2022-09-26},
  abstract = {Single-image super-resolution is of great importance for vision applications, and numerous algorithms have been proposed in recent years. Despite the demonstrated success, these results are often generated based on different assumptions using different datasets and metrics. In this paper, we present a systematic benchmark evaluation for state-of-the-art single-image super-resolution algorithms. In addition to quantitative evaluations based on conventional full-reference metrics, human subject studies are carried out to evaluate image quality based on visual perception. The benchmark evaluations demonstrate the performance and limitations of state-of-the-art algorithms which sheds light on future research in single-image super-resolution.},
  isbn = {978-3-319-10592-5 978-3-319-10593-2},
  langid = {english},
  file = {Y:\paper\EMPTY_COLLECTION_NAME\Yang et al_2014_Single-Image Super-Resolution.pdf}
}

@inproceedings{yangStackedAttentionNetworks2016,
  title = {Stacked {{Attention Networks}} for {{Image Question Answering}}},
  booktitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Yang, Zichao and He, Xiaodong and Gao, Jianfeng and Deng, Li and Smola, Alex},
  date = {2016-06},
  pages = {21--29},
  publisher = {IEEE},
  location = {Las Vegas, NV, USA},
  doi = {10.1109/CVPR.2016.10},
  url = {http://ieeexplore.ieee.org/document/7780379/},
  urldate = {2023-05-28},
  abstract = {This paper presents stacked attention networks (SANs) that learn to answer natural language questions from images. SANs use semantic representation of a question as query to search for the regions in an image that are related to the answer. We argue that image question answering (QA) often requires multiple steps of reasoning. Thus, we develop a multiple-layer SAN in which we query an image multiple times to infer the answer progressively. Experiments conducted on four image QA data sets demonstrate that the proposed SANs significantly outperform previous state-of-the-art approaches. The visualization of the attention layers illustrates the progress that the SAN locates the relevant visual clues that lead to the answer of the question layer-by-layer.},
  eventtitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-4673-8851-1},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\599PDGQ6\Yang 등 - 2016 - Stacked Attention Networks for Image Question Answ.pdf}
}

@online{yangTraceNormRegularised2017,
  title = {Trace {{Norm Regularised Deep Multi-Task Learning}}},
  author = {Yang, Yongxin and Hospedales, Timothy M.},
  date = {2017-02-16},
  eprint = {1606.04038},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1606.04038},
  url = {http://arxiv.org/abs/1606.04038},
  urldate = {2023-12-23},
  abstract = {We propose a framework for training multiple neural networks simultaneously. The parameters from all models are regularised by the tensor trace norm, so that each neural network is encouraged to reuse others' parameters if possible -- this is the main motivation behind multi-task learning. In contrast to many deep multi-task learning models, we do not predefine a parameter sharing strategy by specifying which layers have tied parameters. Instead, our framework considers sharing for all shareable layers, and the sharing strategy is learned in a data-driven way.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\multi-task learning\\Yang_Hospedales_2017_Trace Norm Regularised Deep Multi-Task Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\R8HC6H73\\1606.html}
}

@online{yangUniPADUniversalPretraining2023,
  title = {{{UniPAD}}: {{A Universal Pre-training Paradigm}} for {{Autonomous Driving}}},
  shorttitle = {{{UniPAD}}},
  author = {Yang, Honghui and Zhang, Sha and Huang, Di and Wu, Xiaoyang and Zhu, Haoyi and He, Tong and Tang, Shixiang and Zhao, Hengshuang and Qiu, Qibo and Lin, Binbin and He, Xiaofei and Ouyang, Wanli},
  date = {2023-10-12},
  eprint = {2310.08370},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2310.08370},
  urldate = {2024-03-13},
  abstract = {In the context of autonomous driving, the significance of effective feature learning is widely acknowledged. While conventional 3D self-supervised pre-training methods have shown widespread success, most methods follow the ideas originally designed for 2D images. In this paper, we present UniPAD, a novel self-supervised learning paradigm applying 3D volumetric differentiable rendering. UniPAD implicitly encodes 3D space, facilitating the reconstruction of continuous 3D shape structures and the intricate appearance characteristics of their 2D projections. The flexibility of our method enables seamless integration into both 2D and 3D frameworks, enabling a more holistic comprehension of the scenes. We manifest the feasibility and effectiveness of UniPAD by conducting extensive experiments on various downstream 3D tasks. Our method significantly improves lidar-, camera-, and lidar-camera-based baseline by 9.1, 7.7, and 6.9 NDS, respectively. Notably, our pre-training pipeline achieves 73.2 NDS for 3D object detection and 79.4 mIoU for 3D semantic segmentation on the nuScenes validation set, achieving state-of-the-art results in comparison with previous methods. The code will be available at https://github.com/Nightmare-n/UniPAD.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2024_research\\Yang et al_2023_UniPAD.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8P2CPHHK\\2310.html}
}

@online{yangVisualCuriosityLearning2018,
  title = {Visual {{Curiosity}}: {{Learning}} to {{Ask Questions}} to {{Learn Visual Recognition}}},
  shorttitle = {Visual {{Curiosity}}},
  author = {Yang, Jianwei and Lu, Jiasen and Lee, Stefan and Batra, Dhruv and Parikh, Devi},
  date = {2018-10-01},
  eprint = {1810.00912},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1810.00912},
  url = {http://arxiv.org/abs/1810.00912},
  urldate = {2023-08-05},
  abstract = {In an open-world setting, it is inevitable that an intelligent agent (e.g., a robot) will encounter visual objects, attributes or relationships it does not recognize. In this work, we develop an agent empowered with visual curiosity, i.e. the ability to ask questions to an Oracle (e.g., human) about the contents in images (e.g., What is the object on the left side of the red cube?) and build visual recognition model based on the answers received (e.g., Cylinder). In order to do this, the agent must (1) understand what it recognizes and what it does not, (2) formulate a valid, unambiguous and informative language query (a question) to ask the Oracle, (3) derive the parameters of visual classifiers from the Oracle response and (4) leverage the updated visual classifiers to ask more clarified questions. Specifically, we propose a novel framework and formulate the learning of visual curiosity as a reinforcement learning problem. In this framework, all components of our agent, visual recognition module (to see), question generation policy (to ask), answer digestion module (to understand) and graph memory module (to memorize), are learned entirely end-to-end to maximize the reward derived from the scene graph obtained by the agent as a consequence of the dialog with the Oracle. Importantly, the question generation policy is disentangled from the visual recognition system and specifics of the environment. Consequently, we demonstrate a sort of double generalization. Our question generation policy generalizes to new environments and a new pair of eyes, i.e., new visual system. Trained on a synthetic dataset, our results show that our agent learns new visual concepts significantly faster than several heuristic baselines, even when tested on synthetic environments with novel objects, as well as in a realistic environment.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Robotics,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\vision and language\\Yang et al_2018_Visual Curiosity.pdf;C\:\\Users\\chsey\\Zotero\\storage\\D3LRA8NX\\1810.html}
}

@online{yarotskyStructureUniversalFormulas2023,
  title = {Structure of Universal Formulas},
  author = {Yarotsky, Dmitry},
  date = {2023-11-07},
  eprint = {2311.03910},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/2311.03910},
  urldate = {2024-03-06},
  abstract = {By universal formulas we understand parameterized analytic expressions that have a fixed complexity, but nevertheless can approximate any continuous function on a compact set. There exist various examples of such formulas, including some in the form of neural networks. In this paper we analyze the essential structural elements of these highly expressive models. We introduce a hierarchy of expressiveness classes connecting the global approximability property to the weaker property of infinite VC dimension, and prove a series of classification results for several increasingly complex functional families. In particular, we introduce a general family of polynomially-exponentially-algebraic functions that, as we prove, is subject to polynomial constraints. As a consequence, we show that fixed-size neural networks with not more than one layer of neurons having transcendental activations (e.g., sine or standard sigmoid) cannot in general approximate functions on arbitrary finite sets. On the other hand, we give examples of functional families, including two-hidden-layer neural networks, that approximate functions on arbitrary finite sets, but fail to do that on the whole domain of definition.},
  pubstate = {prepublished},
  keywords = {Computer Science - Data Structures and Algorithms,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,Mathematics - Classical Analysis and ODEs,notion},
  file = {Y\:\\paper\\2024_research\\Yarotsky_2023_Structure of universal formulas.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3PA5ISD8\\2311.html}
}

@inproceedings{yatskarSituationRecognitionVisual2016,
  title = {Situation {{Recognition}}: {{Visual Semantic Role Labeling}} for {{Image Understanding}}},
  shorttitle = {Situation {{Recognition}}},
  booktitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Yatskar, Mark and Zettlemoyer, Luke and Farhadi, Ali},
  date = {2016-06},
  pages = {5534--5542},
  issn = {1063-6919},
  doi = {10.1109/CVPR.2016.597},
  abstract = {This paper introduces situation recognition, the problem of producing a concise summary of the situation an image depicts including: (1) the main activity (e.g., clipping), (2) the participating actors, objects, substances, and locations (e.g., man, shears, sheep, wool, and field) and most importantly (3) the roles these participants play in the activity (e.g., the man is clipping, the shears are his tool, the wool is being clipped from the sheep, and the clipping is in a field). We use FrameNet, a verb and role lexicon developed by linguists, to define a large space of possible situations and collect a large-scale dataset containing over 500 activities, 1,700 roles, 11,000 objects, 125,000 images, and 200,000 unique situations. We also introduce structured prediction baselines and show that, in activity-centric images, situation-driven prediction of objects and activities outperforms independent object and activity recognition.},
  eventtitle = {2016 {{IEEE Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  keywords = {Image recognition,Labeling,notion,Semantics,Spraying,Visualization,Wool},
  file = {Y:\paper\computer_vision_topics_18\visual common sense reasoning\Yatskar et al_2016_Situation Recognition.pdf}
}

@inproceedings{yatskarStatingObviousExtracting2016,
  title = {Stating the {{Obvious}}: {{Extracting Visual Common Sense Knowledge}}},
  shorttitle = {Stating the {{Obvious}}},
  booktitle = {Proceedings of the 2016 {{Conference}} of the {{North American Chapter}} of the {{Association}} for {{Computational Linguistics}}: {{Human Language Technologies}}},
  author = {Yatskar, Mark and Ordonez, Vicente and Farhadi, Ali},
  date = {2016-06},
  pages = {193--198},
  publisher = {Association for Computational Linguistics},
  location = {San Diego, California},
  doi = {10.18653/v1/N16-1023},
  url = {https://aclanthology.org/N16-1023},
  urldate = {2023-08-05},
  eventtitle = {{{NAACL-HLT}} 2016},
  keywords = {notion},
  file = {Y:\paper\computer_vision_topics_18\visual common sense reasoning\Yatskar et al_2016_Stating the Obvious.pdf}
}

@online{yinContextAttributeGrounded2019,
  title = {Context and {{Attribute Grounded Dense Captioning}}},
  author = {Yin, Guojun and Sheng, Lu and Liu, Bin and Yu, Nenghai and Wang, Xiaogang and Shao, Jing},
  date = {2019-04-02},
  eprint = {1904.01410},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1904.01410},
  url = {http://arxiv.org/abs/1904.01410},
  urldate = {2023-05-29},
  abstract = {Dense captioning aims at simultaneously localizing semantic regions and describing these regions-of-interest (ROIs) with short phrases or sentences in natural language. Previous studies have shown remarkable progresses, but they are often vulnerable to the aperture problem that a caption generated by the features inside one ROI lacks contextual coherence with its surrounding context in the input image. In this work, we investigate contextual reasoning based on multi-scale message propagations from the neighboring contents to the target ROIs. To this end, we design a novel end-to-end context and attribute grounded dense captioning framework consisting of 1) a contextual visual mining module and 2) a multi-level attribute grounded description generation module. Knowing that captions often co-occur with the linguistic attributes (such as who, what and where), we also incorporate an auxiliary supervision from hierarchical linguistic attributes to augment the distinctiveness of the learned captions. Extensive experiments and ablation studies on Visual Genome dataset demonstrate the superiority of the proposed model in comparison to state-of-the-art methods.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Yin et al_2019_Context and Attribute Grounded Dense Captioning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\BQ2C6MTR\\1904.html}
}

@online{yinContextAttributeGrounded2019a,
  title = {Context and {{Attribute Grounded Dense Captioning}}},
  author = {Yin, Guojun and Sheng, Lu and Liu, Bin and Yu, Nenghai and Wang, Xiaogang and Shao, Jing},
  date = {2019-04-02},
  eprint = {1904.01410},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1904.01410},
  urldate = {2023-05-29},
  abstract = {Dense captioning aims at simultaneously localizing semantic regions and describing these regions-of-interest (ROIs) with short phrases or sentences in natural language. Previous studies have shown remarkable progresses, but they are often vulnerable to the aperture problem that a caption generated by the features inside one ROI lacks contextual coherence with its surrounding context in the input image. In this work, we investigate contextual reasoning based on multi-scale message propagations from the neighboring contents to the target ROIs. To this end, we design a novel end-to-end context and attribute grounded dense captioning framework consisting of 1) a contextual visual mining module and 2) a multi-level attribute grounded description generation module. Knowing that captions often co-occur with the linguistic attributes (such as who, what and where), we also incorporate an auxiliary supervision from hierarchical linguistic attributes to augment the distinctiveness of the learned captions. Extensive experiments and ablation studies on Visual Genome dataset demonstrate the superiority of the proposed model in comparison to state-of-the-art methods.},
  pubstate = {prepublished},
  version = {1},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\dense captioning\\Yin et al_2019_Context and Attribute Grounded Dense Captioning2.pdf;C\:\\Users\\chsey\\Zotero\\storage\\JVCEBWE8\\1904.html}
}

@inproceedings{yinVS100ParameterEfficient2023,
  title = {1\% {{VS}} 100\%: {{Parameter-Efficient Low Rank Adapter}} for {{Dense Predictions}}},
  shorttitle = {1\% {{VS}} 100\%},
  author = {Yin, Dongshuo and Yang, Yiran and Wang, Zhechao and Yu, Hongfeng and Wei, Kaiwen and Sun, Xian},
  date = {2023},
  pages = {20116--20126},
  url = {https://openaccess.thecvf.com/content/CVPR2023/html/Yin_1_VS_100_Parameter-Efficient_Low_Rank_Adapter_for_Dense_Predictions_CVPR_2023_paper.html},
  urldate = {2023-08-07},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\prompt\Yin et al_2023_1% VS 100%.pdf}
}

@inproceedings{yooAccurateMultivariateStock2021,
  title = {Accurate {{Multivariate Stock Movement Prediction}} via {{Data-Axis Transformer}} with {{Multi-Level Contexts}}},
  booktitle = {Proceedings of the 27th {{ACM SIGKDD Conference}} on {{Knowledge Discovery}} \& {{Data Mining}}},
  author = {Yoo, Jaemin and Soun, Yejun and Park, Yong-chan and Kang, U},
  year = {8월 14, 2021},
  series = {{{KDD}} '21},
  pages = {2037--2045},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/3447548.3467297},
  url = {https://dl.acm.org/doi/10.1145/3447548.3467297},
  urldate = {2024-09-10},
  abstract = {How can we efficiently correlate multiple stocks for accurate stock movement prediction? Stock movement prediction has received growing interest in data mining and machine learning communities due to its substantial impact on financial markets. One way to improve the prediction accuracy is to utilize the correlations between multiple stocks, getting a reliable evidence regardless of the random noises of individual prices. However, it has been challenging to acquire accurate correlations between stocks because of their asymmetric and dynamic nature which is also influenced by the global movement of a market. In this work, we propose DTML (Data-axis Transformer with Multi-Level contexts), a novel approach for stock movement prediction that learns the correlations between stocks in an end-to-end way. DTML makes asymmetric and dynamic correlations by a) learning temporal correlations within each stock, b) generating multi-level contexts based on a global market context, and c) utilizing a transformer encoder for learning inter-stock correlations. DTML achieves the state-of-the-art accuracy on six datasets collected from various stock markets from US, China, Japan, and UK, making up to 13.8\%p higher profits than the best competitors and the annualized return of 44.4\% on investment simulation.},
  isbn = {978-1-4503-8332-5},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\CJ_paper\Yoo et al_2021_Accurate Multivariate Stock Movement Prediction via Data-Axis Transformer with.pdf}
}

@inproceedings{yooAccurateMultivariateStock2021a,
  title = {Accurate {{Multivariate Stock Movement Prediction}} via {{Data-Axis Transformer}} with {{Multi-Level Contexts}}},
  booktitle = {Proceedings of the 27th {{ACM SIGKDD Conference}} on {{Knowledge Discovery}} \& {{Data Mining}}},
  author = {Yoo, Jaemin and Soun, Yejun and Park, Yong-chan and Kang, U},
  date = {2021-08-14},
  pages = {2037--2045},
  publisher = {ACM},
  location = {Virtual Event Singapore},
  doi = {10.1145/3447548.3467297},
  url = {https://dl.acm.org/doi/10.1145/3447548.3467297},
  urldate = {2024-09-11},
  eventtitle = {{{KDD}} '21: {{The}} 27th {{ACM SIGKDD Conference}} on {{Knowledge Discovery}} and {{Data Mining}}},
  isbn = {978-1-4503-8332-5},
  langid = {english}
}

@online{yooImprovingVisualPrompt2023,
  title = {Improving {{Visual Prompt Tuning}} for {{Self-supervised Vision Transformers}}},
  author = {Yoo, Seungryong and Kim, Eunji and Jung, Dahuin and Lee, Jungbeom and Yoon, Sungroh},
  date = {2023-06-08},
  eprint = {2306.05067},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2306.05067},
  urldate = {2023-07-26},
  abstract = {Visual Prompt Tuning (VPT) is an effective tuning method for adapting pretrained Vision Transformers (ViTs) to downstream tasks. It leverages extra learnable tokens, known as prompts, which steer the frozen pretrained ViTs. Although VPT has demonstrated its applicability with supervised vision transformers, it often underperforms with self-supervised ones. Through empirical observations, we deduce that the effectiveness of VPT hinges largely on the ViT blocks with which the prompt tokens interact. Specifically, VPT shows improved performance on image classification tasks for MAE and MoCo v3 when the prompt tokens are inserted into later blocks rather than the first block. These observations suggest that there exists an optimal location of blocks for the insertion of prompt tokens. Unfortunately, identifying the optimal blocks for prompts within each self-supervised ViT for diverse future scenarios is a costly process. To mitigate this problem, we propose a simple yet effective method that learns a gate for each ViT block to adjust its intervention into the prompt tokens. With our method, prompt tokens are selectively influenced by blocks that require steering for task adaptation. Our method outperforms VPT variants in FGVC and VTAB image classification and ADE20K semantic segmentation. The code is available at https://github.com/ryongithub/GatedPromptTuning.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Yoo et al_2023_Improving Visual Prompt Tuning for Self-supervised Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\RFPG2JL6\\2306.html}
}

@inproceedings{yooImprovingVisualPrompt2023a,
  title = {Improving Visual Prompt Tuning for Self-Supervised Vision Transformers},
  booktitle = {Proceedings of the 40th {{International Conference}} on {{Machine Learning}}},
  author = {Yoo, Seungryong and Kim, Eunji and Jung, Dahuin and Lee, Jungbeom and Yoon, Sungroh},
  year = {7월 23, 2023},
  series = {{{ICML}}'23},
  volume = {202},
  pages = {40075--40092},
  publisher = {JMLR.org},
  location = {Honolulu, Hawaii, USA},
  abstract = {Visual Prompt Tuning (VPT) is an effective tuning method for adapting pretrained Vision Transformers (ViTs) to downstream tasks. It leverages extra learnable tokens, known as prompts, which steer the frozen pretrained ViTs. Although VPT has demonstrated its applicability with supervised vision transformers, it often underperforms with self-supervised ones. Through empirical observations, we deduce that the effectiveness of VPT hinges largely on the ViT blocks with which the prompt tokens interact. Specifically, VPT shows improved performance on image classification tasks for MAE and MoCo v3 when the prompt tokens are inserted into later blocks rather than the first block. These observations suggest that there exists an optimal location of blocks for the insertion of prompt tokens. Unfortunately, identifying the optimal blocks for prompts within each self-supervised ViT for diverse future scenarios is a costly process. To mitigate this problem, we propose a simple yet effective method that learns a gate for each ViT block to adjust its intervention into the prompt tokens. With our method, prompt tokens are selectively influenced by blocks that require steering for task adaptation. Our method outperforms VPT variants in FGVC and VTAB image classification and ADE20K semantic segmentation. The code is available at https://github.com/ryongithub/GatedPromptTuning.}
}

@online{youLogMEPracticalAssessment2021,
  title = {{{LogME}}: {{Practical Assessment}} of {{Pre-trained Models}} for {{Transfer Learning}}},
  shorttitle = {{{LogME}}},
  author = {You, Kaichao and Liu, Yong and Wang, Jianmin and Long, Mingsheng},
  date = {2021-06-23},
  eprint = {2102.11005},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2102.11005},
  url = {http://arxiv.org/abs/2102.11005},
  urldate = {2024-01-05},
  abstract = {This paper studies task adaptive pre-trained model selection, an underexplored problem of assessing pre-trained models for the target task and select best ones from the model zoo \textbackslash emph\{without fine-tuning\}. A few pilot works addressed the problem in transferring supervised pre-trained models to classification tasks, but they cannot handle emerging unsupervised pre-trained models or regression tasks. In pursuit of a practical assessment method, we propose to estimate the maximum value of label evidence given features extracted by pre-trained models. Unlike the maximum likelihood, the maximum evidence is \textbackslash emph\{immune to over-fitting\}, while its expensive computation can be dramatically reduced by our carefully designed algorithm. The Logarithm of Maximum Evidence (LogME) can be used to assess pre-trained models for transfer learning: a pre-trained model with a high LogME value is likely to have good transfer performance. LogME is \textbackslash emph\{fast, accurate, and general\}, characterizing itself as the first practical method for assessing pre-trained models. Compared with brute-force fine-tuning, LogME brings at most \$3000\textbackslash times\$ speedup in wall-clock time and requires only \$1\textbackslash\%\$ memory footprint. It outperforms prior methods by a large margin in their setting and is applicable to new settings. It is general enough for diverse pre-trained models (supervised pre-trained and unsupervised pre-trained), downstream tasks (classification and regression), and modalities (vision and language). Code is available at this repository: \textbackslash href\{https://github.com/thuml/LogME\}\{https://github.com/thuml/LogME\}.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\You et al_2021_LogME.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7GKIUDYL\\2102.html}
}

@inproceedings{yuanIsomerIsomerousTransformer2023,
  title = {Isomer: {{Isomerous Transformer}} for {{Zero-shot Video Object Segmentation}}},
  shorttitle = {Isomer},
  author = {Yuan, Yichen and Wang, Yifan and Wang, Lijun and Zhao, Xiaoqi and Lu, Huchuan and Wang, Yu and Su, Weibo and Zhang, Lei},
  date = {2023},
  pages = {966--976},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Yuan_Isomer_Isomerous_Transformer_for_Zero-shot_Video_Object_Segmentation_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Yuan et al_2023_Isomer.pdf}
}

@online{yuanLanguageBiasVisual2021,
  title = {Language Bias in {{Visual Question Answering}}: {{A Survey}} and {{Taxonomy}}},
  shorttitle = {Language Bias in {{Visual Question Answering}}},
  author = {Yuan, Desen},
  date = {2021-11-16},
  eprint = {2111.08531},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2111.08531},
  urldate = {2023-05-28},
  abstract = {Visual question answering (VQA) is a challenging task, which has attracted more and more attention in the field of computer vision and natural language processing. However, the current visual question answering has the problem of language bias, which reduces the robustness of the model and has an adverse impact on the practical application of visual question answering. In this paper, we conduct a comprehensive review and analysis of this field for the first time, and classify the existing methods according to three categories, including enhancing visual information, weakening language priors, data enhancement and training strategies. At the same time, the relevant representative methods are introduced, summarized and analyzed in turn. The causes of language bias are revealed and classified. Secondly, this paper introduces the datasets mainly used for testing, and reports the experimental results of various existing methods. Finally, we discuss the possible future research directions in this field.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2023_nips_dataset_track\\related_works_references\\visual to natural language\\VQA\\Yuan_2021_Language bias in Visual Question Answering.pdf;C\:\\Users\\chsey\\Zotero\\storage\\U4CQGVFB\\2111.html}
}

@article{yueImageSuperresolutionTechniques2016,
  title = {Image Super-Resolution: {{The}} Techniques, Applications, and Future},
  shorttitle = {Image Super-Resolution},
  author = {Yue, Linwei and Shen, Huanfeng and Li, Jie and Yuan, Qiangqiang and Zhang, Hongyan and Zhang, Liangpei},
  date = {2016-11-01},
  journaltitle = {Signal Processing},
  shortjournal = {Signal Processing},
  volume = {128},
  pages = {389--408},
  issn = {0165-1684},
  doi = {10.1016/j.sigpro.2016.05.002},
  url = {https://www.sciencedirect.com/science/article/pii/S0165168416300536},
  urldate = {2022-09-26},
  abstract = {Super-resolution (SR) technique reconstructs a higher-resolution image or sequence from the observed LR images. As SR has been developed for more than three decades, both multi-frame and single-frame SR have significant applications in our daily life. This paper aims to provide a review of SR from the perspective of techniques and applications, and especially the main contributions in recent years. Regularized SR methods are most commonly employed in the last decade. Technical details are discussed in this article, including reconstruction models, parameter selection methods, optimization algorithms and acceleration strategies. Moreover, an exhaustive summary of the current applications using SR techniques has been presented. Lastly, the article discusses the current obstacles for future research.},
  langid = {english},
  keywords = {Applications,Regularized framework,Resolution enhancement,Super resolution},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Yue et al_2016_Image super-resolution.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KK262997\\S0165168416300536.html}
}

@online{yuMMOEMixtureMultimodal2023,
  title = {{{MMOE}}: {{Mixture}} of {{Multimodal Interaction Experts}}},
  shorttitle = {{{MMOE}}},
  author = {Yu, Haofei and Liang, Paul Pu and Salakhutdinov, Ruslan and Morency, Louis-Philippe},
  date = {2023-11-16},
  eprint = {2311.09580},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2311.09580},
  urldate = {2024-05-13},
  abstract = {Multimodal machine learning, which studies the information and interactions across various input modalities, has made significant advancements in understanding the relationship between images and descriptive text. However, this is just a portion of the potential multimodal interactions seen in the real world and does not include new interactions between conflicting utterances and gestures in predicting sarcasm, for example. Notably, the current methods for capturing shared information often do not extend well to these more nuanced interactions, sometimes performing as low as 50\% in binary classification. In this paper, we address this problem via a new approach called MMOE, which stands for a mixture of multimodal interaction experts. Our method automatically classifies data points from unlabeled multimodal datasets by their interaction type and employs specialized models for each specific interaction. Based on our experiments, this approach improves performance on these challenging interactions by more than 10\%, leading to an overall increase of 2\% for tasks like sarcasm prediction. As a result, interaction quantification provides new insights for dataset analysis and yields simple approaches that obtain stateof-the-art performance.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,notion},
  file = {Y:\paper\2024_research\Yu et al_2023_MMOE.pdf}
}

@online{yuPlenOctreesRealtimeRendering2021,
  title = {{{PlenOctrees}} for {{Real-time Rendering}} of {{Neural Radiance Fields}}},
  author = {Yu, Alex and Li, Ruilong and Tancik, Matthew and Li, Hao and Ng, Ren and Kanazawa, Angjoo},
  date = {2021-08-17},
  eprint = {2103.14024},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2103.14024},
  urldate = {2023-02-06},
  abstract = {We introduce a method to render Neural Radiance Fields (NeRFs) in real time using PlenOctrees, an octree-based 3D representation which supports view-dependent effects. Our method can render 800x800 images at more than 150 FPS, which is over 3000 times faster than conventional NeRFs. We do so without sacrificing quality while preserving the ability of NeRFs to perform free-viewpoint rendering of scenes with arbitrary geometry and view-dependent effects. Real-time performance is achieved by pre-tabulating the NeRF into a PlenOctree. In order to preserve view-dependent effects such as specularities, we factorize the appearance via closed-form spherical basis functions. Specifically, we show that it is possible to train NeRFs to predict a spherical harmonic representation of radiance, removing the viewing direction as an input to the neural network. Furthermore, we show that PlenOctrees can be directly optimized to further minimize the reconstruction loss, which leads to equal or better quality compared to competing methods. Moreover, this octree optimization step can be used to reduce the training time, as we no longer need to wait for the NeRF training to converge fully. Our real-time neural rendering approach may potentially enable new applications such as 6-DOF industrial and product visualizations, as well as next generation AR/VR systems. PlenOctrees are amenable to in-browser rendering as well; please visit the project page for the interactive online demo, as well as video and code: https://alexyu.net/plenoctrees},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Yu et al_2021_PlenOctrees for Real-time Rendering of Neural Radiance Fields.pdf;C\:\\Users\\chsey\\Zotero\\storage\\HRQVQLLD\\2103.html}
}

@online{yuPlenoxelsRadianceFields2021,
  title = {Plenoxels: {{Radiance Fields}} without {{Neural Networks}}},
  shorttitle = {Plenoxels},
  author = {Yu, Alex and Fridovich-Keil, Sara and Tancik, Matthew and Chen, Qinhong and Recht, Benjamin and Kanazawa, Angjoo},
  date = {2021-12-09},
  eprint = {2112.05131},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2112.05131},
  url = {http://arxiv.org/abs/2112.05131},
  urldate = {2023-01-04},
  abstract = {We introduce Plenoxels (plenoptic voxels), a system for photorealistic view synthesis. Plenoxels represent a scene as a sparse 3D grid with spherical harmonics. This representation can be optimized from calibrated images via gradient methods and regularization without any neural components. On standard, benchmark tasks, Plenoxels are optimized two orders of magnitude faster than Neural Radiance Fields with no loss in visual quality.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Yu et al_2021_Plenoxels.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7XLU7X3K\\2112.html}
}

@article{yuProgressiveGlassSegmentation2022,
  title = {Progressive {{Glass Segmentation}}},
  author = {Yu, Letian and Mei, Haiyang and Dong, Wen and Wei, Ziqi and Zhu, Li and Wang, Yuxin and Yang, Xin},
  date = {2022},
  journaltitle = {IEEE Transactions on Image Processing},
  volume = {31},
  pages = {2920--2933},
  issn = {1941-0042},
  doi = {10.1109/TIP.2022.3162709},
  abstract = {Glass is very common in the real world. Influenced by the uncertainty about the glass region and the varying complex scenes behind the glass, the existence of glass poses severe challenges to many computer vision tasks, making glass segmentation as an important computer vision task. Glass does not have its own visual appearances but only transmit/reflect the appearances of its surroundings, making it fundamentally different from other common objects. To address such a challenging task, existing methods typically explore and combine useful cues from different levels of features in the deep network. As there exists a characteristic gap between level-different features, i.e., deep layer features embed more high-level semantics and are better at locating the target objects while shallow layer features have larger spatial sizes and keep richer and more detailed low-level information, fusing these features naively thus would lead to a sub-optimal solution. In this paper, we approach the effective features fusion towards accurate glass segmentation in two steps. First, we attempt to bridge the characteristic gap between different levels of features by developing a Discriminability Enhancement (DE) module which enables level-specific features to be a more discriminative representation, alleviating the features incompatibility for fusion. Second, we design a Focus-and-Exploration Based Fusion (FEBF) module to richly excavate useful information in the fusion process by highlighting the common and exploring the difference between level-different features. Combining these two steps, we construct a Progressive Glass Segmentation Network (PGSNet) which uses multiple DE and FEBF modules to progressively aggregate features from high-level to low-level, implementing a coarse-to-fine glass segmentation. In addition, we build the first home-scene-oriented glass segmentation dataset for advancing household robot applications and in-depth research on this topic. Extensive experiments demonstrate that our method outperforms 26 cutting-edge models on three challenging datasets under four standard metrics. The code and dataset will be made publicly available.},
  eventtitle = {{{IEEE Transactions}} on {{Image Processing}}},
  keywords = {Aggregates,Bridges,dataset,deep neural network,Feature extraction,fusion strategy,Glass,Glass segmentation,Image segmentation,Semantics,Task analysis},
  file = {Y\:\\paper\\2022 winter intern\\transparent_segmentation\\Yu et al_2022_Progressive Glass Segmentation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\3G9RYSTZ\\9748016.html}
}

@inproceedings{yuSelectionClassconditionalFilters2021,
  title = {Selection of {{Class-conditional Filters}} for {{Semantic Shifted OOD Detection}}},
  booktitle = {2021 18th {{International Conference}} on {{Ubiquitous Robots}} ({{UR}})},
  author = {Yu, Yeonguk and Shin, Sungho and Kim, Jongwon and Lee, Kyoobin},
  date = {2021-07},
  pages = {43--47},
  issn = {2325-033X},
  doi = {10.1109/UR52253.2021.9494630},
  abstract = {Deep neural networks have been deployed in a wide range of applications with remarkable performance but can be easily fooled with data that are out-of-distribution (OOD). Recent works have proposed detection methods for OOD benchmarks consisting of small image datasets from separate domains (i.e. object classification dataset for training samples and digit classification dataset for OOD samples). However, these methods fail for OOD benchmarks consisting of image datasets from the same domain (i.e. Korean food classification dataset for training samples and Italian food classification dataset for OOD samples). To solve this issue, we propose an OOD detection framework that utilizes two simple operations: counting to find class-wise highly activated filters in the last convolution layer, and summation to calculate the confidence score by summation of the activation of highly activated filters. The proposed framework is based on our assumption that given an OOD sample from the same domain, the CNN model will produce similar feature maps through all its filters, while some differences might be found in the feature map from highly activated filters. We show that our method achieves the highest performance for OOD benchmarks consisting of the Food101 dataset, which provides meaningful insights on how this issue, that has been encountered in recent works, can be effectively addressed.},
  eventtitle = {2021 18th {{International Conference}} on {{Ubiquitous Robots}} ({{UR}})},
  keywords = {Benchmark testing,Convolution,Deep learning,Robots,Semantics,Task analysis,Training},
  file = {Y\:\\paper\\2022 autumn intern\\internal paper\\Yu et al_2021_Selection of Class-conditional Filters for Semantic Shifted OOD Detection.pdf;C\:\\Users\\chsey\\Zotero\\storage\\MD8S6DCV\\9494630.html}
}

@online{zadouriPushingMixtureExperts2023,
  title = {Pushing {{Mixture}} of {{Experts}} to the {{Limit}}: {{Extremely Parameter Efficient MoE}} for {{Instruction Tuning}}},
  shorttitle = {Pushing {{Mixture}} of {{Experts}} to the {{Limit}}},
  author = {Zadouri, Ted and Üstün, Ahmet and Ahmadian, Arash and Ermiş, Beyza and Locatelli, Acyr and Hooker, Sara},
  date = {2023-09-11},
  eprint = {2309.05444},
  eprinttype = {arXiv},
  url = {http://arxiv.org/abs/2309.05444},
  urldate = {2024-10-26},
  abstract = {The Mixture of Experts (MoE) is a widely known neural architecture where an ensemble of specialized sub-models optimizes overall performance with a constant computational cost. However, conventional MoEs pose challenges at scale due to the need to store all experts in memory. In this paper, we push MoE to the limit. We propose extremely parameter-efficient MoE by uniquely combining MoE architecture with lightweight experts.Our MoE architecture outperforms standard parameter-efficient fine-tuning (PEFT) methods and is on par with full fine-tuning by only updating the lightweight experts -- less than 1\% of an 11B parameters model. Furthermore, our method generalizes to unseen tasks as it does not depend on any prior task knowledge. Our research underscores the versatility of the mixture of experts architecture, showcasing its ability to deliver robust performance even when subjected to rigorous parameter constraints. Our code used in all the experiments is publicly available here: https://github.com/for-ai/parameter-efficient-moe.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Zadouri et al_2023_Pushing Mixture of Experts to the Limit.pdf;C\:\\Users\\chsey\\Zotero\\storage\\E7CK4PG4\\2309.html}
}

@online{zagoruykoWideResidualNetworks2017,
  title = {Wide {{Residual Networks}}},
  author = {Zagoruyko, Sergey and Komodakis, Nikos},
  date = {2017-06-14},
  eprint = {1605.07146},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/1605.07146},
  urldate = {2022-11-14},
  abstract = {Deep residual networks were shown to be able to scale up to thousands of layers and still have improving performance. However, each fraction of a percent of improved accuracy costs nearly doubling the number of layers, and so training very deep residual networks has a problem of diminishing feature reuse, which makes these networks very slow to train. To tackle these problems, in this paper we conduct a detailed experimental study on the architecture of ResNet blocks, based on which we propose a novel architecture where we decrease depth and increase width of residual networks. We call the resulting network structures wide residual networks (WRNs) and show that these are far superior over their commonly used thin and very deep counterparts. For example, we demonstrate that even a simple 16-layer-deep wide residual network outperforms in accuracy and efficiency all previous deep residual networks, including thousand-layer-deep networks, achieving new state-of-the-art results on CIFAR, SVHN, COCO, and significant improvements on ImageNet. Our code and models are available at https://github.com/szagoruyko/wide-residual-networks},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing},
  file = {Y\:\\paper\\artificial intelligence\\Zagoruyko_Komodakis_2017_Wide Residual Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XS5AMKEL\\1605.html}
}

@online{zakenBitFitSimpleParameterefficient2022,
  title = {{{BitFit}}: {{Simple Parameter-efficient Fine-tuning}} for {{Transformer-based Masked Language-models}}},
  shorttitle = {{{BitFit}}},
  author = {Zaken, Elad Ben and Ravfogel, Shauli and Goldberg, Yoav},
  date = {2022-09-05},
  eprint = {2106.10199},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.10199},
  urldate = {2023-07-25},
  abstract = {We introduce BitFit, a sparse-finetuning method where only the bias-terms of the model (or a subset of them) are being modified. We show that with small-to-medium training data, applying BitFit on pre-trained BERT models is competitive with (and sometimes better than) fine-tuning the entire model. For larger data, the method is competitive with other sparse fine-tuning methods. Besides their practical utility, these findings are relevant for the question of understanding the commonly-used process of finetuning: they support the hypothesis that finetuning is mainly about exposing knowledge induced by language-modeling training, rather than learning new task-specific linguistic knowledge.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zaken et al_2022_BitFit.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WCRIPKX6\\2106.html}
}

@article{zamirTaskonomyDisentanglingTask,
  title = {Taskonomy: {{Disentangling Task Transfer Learning}}, {{Supp}}.},
  author = {Zamir, Amir R and Sax, Sasha and Shen, William and Guibas, Leonidas and Malik, Jitendra and Savarese, Silvio},
  abstract = {The following items are provided in the supplementary material: 1. Higher-order transfer experiments. 2. A tiny-data taxonomy. 3. Optimal transfer policies for selected tasks. 4. Our networks as feature extractors on MIT Places. 5. BIP Solver as API. 6. Significance testing of taxonomy. 7. Qualitative results of network output. 8. Agglomerative clustering of tasks. 9. Analysis of transitive transfers. 10. Experimental setup details. 11. Task dictionary definition and discussion.},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\background\Zamir et al_Taskonomy.pdf}
}

@online{zamirTaskonomyDisentanglingTask2018,
  title = {Taskonomy: {{Disentangling Task Transfer Learning}}},
  shorttitle = {Taskonomy},
  author = {Zamir, Amir and Sax, Alexander and Shen, William and Guibas, Leonidas and Malik, Jitendra and Savarese, Silvio},
  date = {2018-04-23},
  eprint = {1804.08328},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1804.08328},
  url = {http://arxiv.org/abs/1804.08328},
  urldate = {2023-07-04},
  abstract = {Do visual tasks have a relationship, or are they unrelated? For instance, could having surface normals simplify estimating the depth of an image? Intuition answers these questions positively, implying existence of a structure among visual tasks. Knowing this structure has notable values; it is the concept underlying transfer learning and provides a principled way for identifying redundancies across tasks, e.g., to seamlessly reuse supervision among related tasks or solve many tasks in one system without piling up the complexity. We proposes a fully computational approach for modeling the structure of space of visual tasks. This is done via finding (first and higher-order) transfer learning dependencies across a dictionary of twenty six 2D, 2.5D, 3D, and semantic tasks in a latent space. The product is a computational taxonomic map for task transfer learning. We study the consequences of this structure, e.g. nontrivial emerged relationships, and exploit them to reduce the demand for labeled data. For example, we show that the total number of labeled datapoints needed for solving a set of 10 tasks can be reduced by roughly 2/3 (compared to training independently) while keeping the performance nearly the same. We provide a set of tools for computing and probing this taxonomical structure including a solver that users can employ to devise efficient supervision policies for their use cases.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,Computer Science - Robotics,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zamir et al_2018_Taskonomy.pdf;C\:\\Users\\chsey\\Zotero\\storage\\7EG8J44B\\1804.html}
}

@online{zeilerVisualizingUnderstandingConvolutional2013,
  title = {Visualizing and {{Understanding Convolutional Networks}}},
  author = {Zeiler, Matthew D. and Fergus, Rob},
  date = {2013-11-28},
  eprint = {1311.2901},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1311.2901},
  url = {http://arxiv.org/abs/1311.2901},
  urldate = {2023-08-05},
  abstract = {Large Convolutional Network models have recently demonstrated impressive classification performance on the ImageNet benchmark. However there is no clear understanding of why they perform so well, or how they might be improved. In this paper we address both issues. We introduce a novel visualization technique that gives insight into the function of intermediate feature layers and the operation of the classifier. We also perform an ablation study to discover the performance contribution from different model layers. This enables us to find model architectures that outperform Krizhevsky \textbackslash etal on the ImageNet classification benchmark. We show our ImageNet model generalizes well to other datasets: when the softmax classifier is retrained, it convincingly beats the current state-of-the-art results on Caltech-101 and Caltech-256 datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\understanding deep CNN\\Zeiler_Fergus_2013_Visualizing and Understanding Convolutional Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\LH5HSJBM\\1311.html}
}

@online{zeilerVisualizingUnderstandingConvolutional2013a,
  title = {Visualizing and {{Understanding Convolutional Networks}}},
  author = {Zeiler, Matthew D. and Fergus, Rob},
  date = {2013-11-28},
  eprint = {1311.2901},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1311.2901},
  url = {http://arxiv.org/abs/1311.2901},
  urldate = {2022-12-19},
  abstract = {Large Convolutional Network models have recently demonstrated impressive classification performance on the ImageNet benchmark. However there is no clear understanding of why they perform so well, or how they might be improved. In this paper we address both issues. We introduce a novel visualization technique that gives insight into the function of intermediate feature layers and the operation of the classifier. We also perform an ablation study to discover the performance contribution from different model layers. This enables us to find model architectures that outperform Krizhevsky \textbackslash etal on the ImageNet classification benchmark. We show our ImageNet model generalizes well to other datasets: when the softmax classifier is retrained, it convincingly beats the current state-of-the-art results on Caltech-101 and Caltech-256 datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 autumn intern\\OOD\\Zeiler_Fergus_2013_Visualizing and Understanding Convolutional Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5SAJRZYA\\1311.html}
}

@online{zellersNeuralMotifsScene2018,
  title = {Neural {{Motifs}}: {{Scene Graph Parsing}} with {{Global Context}}},
  shorttitle = {Neural {{Motifs}}},
  author = {Zellers, Rowan and Yatskar, Mark and Thomson, Sam and Choi, Yejin},
  date = {2018-03-29},
  eprint = {1711.06640},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1711.06640},
  url = {http://arxiv.org/abs/1711.06640},
  urldate = {2023-05-21},
  abstract = {We investigate the problem of producing structured graph representations of visual scenes. Our work analyzes the role of motifs: regularly appearing substructures in scene graphs. We present new quantitative insights on such repeated structures in the Visual Genome dataset. Our analysis shows that object labels are highly predictive of relation labels but not vice-versa. We also find that there are recurring patterns even in larger subgraphs: more than 50\% of graphs contain motifs involving at least two relations. Our analysis motivates a new baseline: given object detections, predict the most frequent relation between object pairs with the given labels, as seen in the training set. This baseline improves on the previous state-of-the-art by an average of 3.6\% relative improvement across evaluation settings. We then introduce Stacked Motif Networks, a new architecture designed to capture higher order motifs in scene graphs that further improves over our strong baseline by an average 7.1\% relative gain. Our code is available at github.com/rowanz/neural-motifs.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Zellers et al_2018_Neural Motifs.pdf;C\:\\Users\\chsey\\Zotero\\storage\\CUW398VE\\1711.html}
}

@online{zellersRecognitionCognitionVisual2019,
  title = {From {{Recognition}} to {{Cognition}}: {{Visual Commonsense Reasoning}}},
  shorttitle = {From {{Recognition}} to {{Cognition}}},
  author = {Zellers, Rowan and Bisk, Yonatan and Farhadi, Ali and Choi, Yejin},
  date = {2019-03-26},
  eprint = {1811.10830},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1811.10830},
  url = {http://arxiv.org/abs/1811.10830},
  urldate = {2023-08-05},
  abstract = {Visual understanding goes well beyond object recognition. With one glance at an image, we can effortlessly imagine the world beyond the pixels: for instance, we can infer people's actions, goals, and mental states. While this task is easy for humans, it is tremendously difficult for today's vision systems, requiring higher-order cognition and commonsense reasoning about the world. We formalize this task as Visual Commonsense Reasoning. Given a challenging question about an image, a machine must answer correctly and then provide a rationale justifying its answer. Next, we introduce a new dataset, VCR, consisting of 290k multiple choice QA problems derived from 110k movie scenes. The key recipe for generating non-trivial and high-quality problems at scale is Adversarial Matching, a new approach to transform rich annotations into multiple choice questions with minimal bias. Experimental results show that while humans find VCR easy (over 90\% accuracy), state-of-the-art vision models struggle (\textasciitilde 45\%). To move towards cognition-level understanding, we present a new reasoning engine, Recognition to Cognition Networks (R2C), that models the necessary layered inferences for grounding, contextualization, and reasoning. R2C helps narrow the gap between humans and machines (\textasciitilde 65\%); still, the challenge is far from solved, and we provide analysis that suggests avenues for future work.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\visual common sense reasoning\\Zellers et al_2019_From Recognition to Cognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\QLU49R9J\\1811.html}
}

@online{zengExpressivePowerLowRank2024,
  title = {The {{Expressive Power}} of {{Low-Rank Adaptation}}},
  author = {Zeng, Yuchen and Lee, Kangwook},
  date = {2024-03-17},
  eprint = {2310.17513},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/2310.17513},
  urldate = {2024-05-02},
  abstract = {Low-Rank Adaptation (LoRA), a parameter-efficient fine-tuning method that leverages low-rank adaptation of weight matrices, has emerged as a prevalent technique for fine-tuning pre-trained models such as large language models and diffusion models. Despite its huge success in practice, the theoretical underpinnings of LoRA have largely remained unexplored. This paper takes the first step to bridge this gap by theoretically analyzing the expressive power of LoRA. We prove that, for fully connected neural networks, LoRA can adapt any model \$f\$ to accurately represent any smaller target model \$\textbackslash overline\{f\}\$ if LoRA-rank \$\textbackslash geq(\textbackslash text\{width of \}f) \textbackslash times \textbackslash frac\{\textbackslash text\{depth of \}\textbackslash overline\{f\}\}\{\textbackslash text\{depth of \}f\}\$. We also quantify the approximation error when LoRA-rank is lower than the threshold. For Transformer networks, we show any model can be adapted to a target model of the same size with rank-\$(\textbackslash frac\{\textbackslash text\{embedding size\}\}\{2\})\$ LoRA adapters.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computation and Language,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y:\paper\2024_research\Zeng_Lee_2024_The Expressive Power of Low-Rank Adaptation.pdf}
}

@online{zenkeContinualLearningSynaptic2017,
  title = {Continual {{Learning Through Synaptic Intelligence}}},
  author = {Zenke, Friedemann and Poole, Ben and Ganguli, Surya},
  date = {2017-06-12},
  eprint = {1703.04200},
  eprinttype = {arXiv},
  eprintclass = {cs, q-bio, stat},
  url = {http://arxiv.org/abs/1703.04200},
  urldate = {2023-12-24},
  abstract = {While deep learning has led to remarkable advances across diverse applications, it struggles in domains where the data distribution changes over the course of learning. In stark contrast, biological neural networks continually adapt to changing domains, possibly by leveraging complex molecular machinery to solve many tasks simultaneously. In this study, we introduce intelligent synapses that bring some of this biological complexity into artificial neural networks. Each synapse accumulates task relevant information over time, and exploits this information to rapidly store new memories without forgetting old ones. We evaluate our approach on continual learning of classification tasks, and show that it dramatically reduces forgetting while maintaining computational efficiency.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Quantitative Biology - Neurons and Cognition,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\incremental_learning\\Zenke et al_2017_Continual Learning Through Synaptic Intelligence.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8NZ7THLT\\1703.html}
}

@online{zhaiLargescaleStudyRepresentation2020,
  title = {A {{Large-scale Study}} of {{Representation Learning}} with the {{Visual Task Adaptation Benchmark}}},
  author = {Zhai, Xiaohua and Puigcerver, Joan and Kolesnikov, Alexander and Ruyssen, Pierre and Riquelme, Carlos and Lucic, Mario and Djolonga, Josip and Pinto, Andre Susano and Neumann, Maxim and Dosovitskiy, Alexey and Beyer, Lucas and Bachem, Olivier and Tschannen, Michael and Michalski, Marcin and Bousquet, Olivier and Gelly, Sylvain and Houlsby, Neil},
  date = {2020-02-21},
  eprint = {1910.04867},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1910.04867},
  url = {http://arxiv.org/abs/1910.04867},
  urldate = {2024-01-12},
  abstract = {Representation learning promises to unlock deep learning for the long tail of vision tasks without expensive labelled datasets. Yet, the absence of a unified evaluation for general visual representations hinders progress. Popular protocols are often too constrained (linear classification), limited in diversity (ImageNet, CIFAR, Pascal-VOC), or only weakly related to representation quality (ELBO, reconstruction error). We present the Visual Task Adaptation Benchmark (VTAB), which defines good representations as those that adapt to diverse, unseen tasks with few examples. With VTAB, we conduct a large-scale study of many popular publicly-available representation learning algorithms. We carefully control confounders such as architecture and tuning budget. We address questions like: How effective are ImageNet representations beyond standard natural datasets? How do representations trained via generative and discriminative models compare? To what extent can self-supervision replace labels? And, how close are we to general visual representations?},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\transfer_learning\\Zhai et al_2020_A Large-scale Study of Representation Learning with the Visual Task Adaptation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\56XKYNZW\\1910.html}
}

@online{zhaiLargescaleStudyRepresentation2020a,
  title = {A {{Large-scale Study}} of {{Representation Learning}} with the {{Visual Task Adaptation Benchmark}}},
  author = {Zhai, Xiaohua and Puigcerver, Joan and Kolesnikov, Alexander and Ruyssen, Pierre and Riquelme, Carlos and Lucic, Mario and Djolonga, Josip and Pinto, Andre Susano and Neumann, Maxim and Dosovitskiy, Alexey and Beyer, Lucas and Bachem, Olivier and Tschannen, Michael and Michalski, Marcin and Bousquet, Olivier and Gelly, Sylvain and Houlsby, Neil},
  date = {2020-02-21},
  eprint = {1910.04867},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  url = {http://arxiv.org/abs/1910.04867},
  urldate = {2023-07-07},
  abstract = {Representation learning promises to unlock deep learning for the long tail of vision tasks without expensive labelled datasets. Yet, the absence of a unified evaluation for general visual representations hinders progress. Popular protocols are often too constrained (linear classification), limited in diversity (ImageNet, CIFAR, Pascal-VOC), or only weakly related to representation quality (ELBO, reconstruction error). We present the Visual Task Adaptation Benchmark (VTAB), which defines good representations as those that adapt to diverse, unseen tasks with few examples. With VTAB, we conduct a large-scale study of many popular publicly-available representation learning algorithms. We carefully control confounders such as architecture and tuning budget. We address questions like: How effective are ImageNet representations beyond standard natural datasets? How do representations trained via generative and discriminative models compare? To what extent can self-supervision replace labels? And, how close are we to general visual representations?},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zhai et al_2020_A Large-scale Study of Representation Learning with the Visual Task Adaptation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\8XVS86MP\\1910.html}
}

@online{zhaiLiTZeroShotTransfer2022,
  title = {{{LiT}}: {{Zero-Shot Transfer}} with {{Locked-image}} Text {{Tuning}}},
  shorttitle = {{{LiT}}},
  author = {Zhai, Xiaohua and Wang, Xiao and Mustafa, Basil and Steiner, Andreas and Keysers, Daniel and Kolesnikov, Alexander and Beyer, Lucas},
  date = {2022-06-22},
  eprint = {2111.07991},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2111.07991},
  url = {http://arxiv.org/abs/2111.07991},
  urldate = {2023-09-11},
  abstract = {This paper presents contrastive-tuning, a simple method employing contrastive training to align image and text models while still taking advantage of their pre-training. In our empirical study we find that locked pre-trained image models with unlocked text models work best. We call this instance of contrastive-tuning "Locked-image Tuning" (LiT), which just teaches a text model to read out good representations from a pre-trained image model for new tasks. A LiT model gains the capability of zero-shot transfer to new vision tasks, such as image classification or retrieval. The proposed LiT is widely applicable; it works reliably with multiple pre-training methods (supervised and unsupervised) and across diverse architectures (ResNet, Vision Transformers and MLP-Mixer) using three different image-text datasets. With the transformer-based pre-trained ViT-g/14 model, the LiT model achieves 85.2\% zero-shot transfer accuracy on the ImageNet test set, and 82.5\% on the challenging out-of-distribution ObjectNet test set.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zhai et al_2022_LiT.pdf;C\:\\Users\\chsey\\Zotero\\storage\\WZ8XIYQF\\2111.html}
}

@online{zhaiScalingVisionTransformers2022,
  title = {Scaling {{Vision Transformers}}},
  author = {Zhai, Xiaohua and Kolesnikov, Alexander and Houlsby, Neil and Beyer, Lucas},
  date = {2022-06-20},
  eprint = {2106.04560},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2106.04560},
  urldate = {2023-08-11},
  abstract = {Attention-based neural networks such as the Vision Transformer (ViT) have recently attained state-of-the-art results on many computer vision benchmarks. Scale is a primary ingredient in attaining excellent results, therefore, understanding a model's scaling properties is a key to designing future generations effectively. While the laws for scaling Transformer language models have been studied, it is unknown how Vision Transformers scale. To address this, we scale ViT models and data, both up and down, and characterize the relationships between error rate, data, and compute. Along the way, we refine the architecture and training of ViT, reducing memory consumption and increasing accuracy of the resulting models. As a result, we successfully train a ViT model with two billion parameters, which attains a new state-of-the-art on ImageNet of 90.45\% top-1 accuracy. The model also performs well for few-shot transfer, for example, reaching 84.86\% top-1 accuracy on ImageNet with only 10 examples per class.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zhai et al_2022_Scaling Vision Transformers.pdf;C\:\\Users\\chsey\\Zotero\\storage\\XDQLB6MW\\2106.html}
}

@inproceedings{zhaiScalingVisionTransformers2022a,
  title = {Scaling {{Vision Transformers}}},
  booktitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Zhai, Xiaohua and Kolesnikov, Alexander and Houlsby, Neil and Beyer, Lucas},
  date = {2022-06},
  pages = {1204--1213},
  publisher = {IEEE},
  location = {New Orleans, LA, USA},
  doi = {10.1109/CVPR52688.2022.01179},
  url = {https://ieeexplore.ieee.org/document/9880094/},
  urldate = {2022-11-08},
  abstract = {Attention-based neural networks such as the Vision Transformer (ViT) have recently attained state-of-the-art results on many computer vision benchmarks. Scale is a primary ingredient in attaining excellent results, therefore, understanding a model’s scaling properties is a key to designing future generations effectively. While the laws for scaling Transformer language models have been studied, it is unknown how Vision Transformers scale. To address this, we scale ViT models and data, both up and down, and characterize the relationships between error rate, data, and compute. Along the way, we refine the architecture and training of ViT, reducing memory consumption and increasing accuracy of the resulting models. As a result, we successfully train a ViT model with two billion parameters, which attains a new state-of-the-art on ImageNet of 90.45\% top-1 accuracy. The model also performs well for few-shot transfer, for example, reaching 84.86\% top-1 accuracy on ImageNet with only 10 examples per class.},
  eventtitle = {2022 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-66546-946-3},
  langid = {english},
  file = {Y:\paper\artificial intelligence\Zhai et al_2022_Scaling Vision Transformers.pdf}
}

@online{zhangAdaLoRAAdaptiveBudget2023,
  title = {{{AdaLoRA}}: {{Adaptive Budget Allocation}} for {{Parameter-Efficient Fine-Tuning}}},
  shorttitle = {{{AdaLoRA}}},
  author = {Zhang, Qingru and Chen, Minshuo and Bukharin, Alexander and Karampatziakis, Nikos and He, Pengcheng and Cheng, Yu and Chen, Weizhu and Zhao, Tuo},
  date = {2023-12-20},
  eprint = {2303.10512},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2303.10512},
  urldate = {2024-03-22},
  abstract = {Fine-tuning large pre-trained language models on downstream tasks has become an important paradigm in NLP. However, common practice fine-tunes all of the parameters in a pre-trained model, which becomes prohibitive when a large number of downstream tasks are present. Therefore, many fine-tuning methods are proposed to learn incremental updates of pre-trained weights in a parameter efficient way, e.g., low-rank increments. These methods often evenly distribute the budget of incremental updates across all pre-trained weight matrices, and overlook the varying importance of different weight parameters. As a consequence, the fine-tuning performance is suboptimal. To bridge this gap, we propose AdaLoRA, which adaptively allocates the parameter budget among weight matrices according to their importance score. In particular, AdaLoRA parameterizes the incremental updates in the form of singular value decomposition. Such a novel approach allows us to effectively prune the singular values of unimportant updates, which is essentially to reduce their parameter budget but circumvent intensive exact SVD computations. We conduct extensive experiments with several pre-trained models on natural language processing, question answering, and natural language generation to validate the effectiveness of AdaLoRA. Results demonstrate that AdaLoRA manifests notable improvement over baselines, especially in the low budget settings. Our code is publicly available at https://github.com/QingruZhang/AdaLoRA .},
  pubstate = {prepublished},
  keywords = {Computer Science - Computation and Language,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Zhang et al_2023_AdaLoRA.pdf;C\:\\Users\\chsey\\Zotero\\storage\\93EULG9R\\2303.html}
}

@inproceedings{zhangAddingConditionalControl2023,
  title = {Adding {{Conditional Control}} to {{Text-to-Image Diffusion Models}}},
  booktitle = {2023 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  author = {Zhang, Lvmin and Rao, Anyi and Agrawala, Maneesh},
  date = {2023-10-01},
  pages = {3813--3824},
  publisher = {IEEE},
  location = {Paris, France},
  doi = {10.1109/ICCV51070.2023.00355},
  url = {https://ieeexplore.ieee.org/document/10377881/},
  urldate = {2024-01-24},
  eventtitle = {2023 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  isbn = {9798350307184},
  langid = {english},
  file = {C:\Users\chsey\Zotero\storage\6KCBLCLK\Zhang 등 - 2023 - Adding Conditional Control to Text-to-Image Diffus.pdf}
}

@online{zhangAddingConditionalControl2023a,
  title = {Adding {{Conditional Control}} to {{Text-to-Image Diffusion Models}}},
  author = {Zhang, Lvmin and Rao, Anyi and Agrawala, Maneesh},
  date = {2023-11-26},
  eprint = {2302.05543},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2302.05543},
  urldate = {2024-01-24},
  abstract = {We present ControlNet, a neural network architecture to add spatial conditioning controls to large, pretrained text-to-image diffusion models. ControlNet locks the production-ready large diffusion models, and reuses their deep and robust encoding layers pretrained with billions of images as a strong backbone to learn a diverse set of conditional controls. The neural architecture is connected with "zero convolutions" (zero-initialized convolution layers) that progressively grow the parameters from zero and ensure that no harmful noise could affect the finetuning. We test various conditioning controls, eg, edges, depth, segmentation, human pose, etc, with Stable Diffusion, using single or multiple conditions, with or without prompts. We show that the training of ControlNets is robust with small ({$<$}50k) and large ({$>$}1m) datasets. Extensive results show that ControlNet may facilitate wider applications to control image diffusion models.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics,Computer Science - Human-Computer Interaction,Computer Science - Multimedia},
  file = {Y\:\\paper\\2023 graduation\\visual language\\Zhang et al_2023_Adding Conditional Control to Text-to-Image Diffusion Models.pdf;Y\:\\research\\research_paper\\adding-conditional-control-to-text-to-image-diffusion-models - New Note.md;C\:\\Users\\chsey\\Zotero\\storage\\IQ348RVT\\2302.html}
}

@inproceedings{zhangDETADenoisedTask2023,
  title = {{{DETA}}: {{Denoised Task Adaptation}} for {{Few-Shot Learning}}},
  shorttitle = {{{DETA}}},
  author = {Zhang, Ji and Gao, Lianli and Luo, Xu and Shen, Hengtao and Song, Jingkuan},
  date = {2023},
  pages = {11541--11551},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Zhang_DETA_Denoised_Task_Adaptation_for_Few-Shot_Learning_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Zhang et al_2023_DETA.pdf}
}

@online{zhangFineGrainedSceneGraph2022,
  title = {Fine-{{Grained Scene Graph Generation}} with {{Data Transfer}}},
  author = {Zhang, Ao and Yao, Yuan and Chen, Qianyu and Ji, Wei and Liu, Zhiyuan and Sun, Maosong and Chua, Tat-Seng},
  date = {2022-07-20},
  eprint = {2203.11654},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2203.11654},
  urldate = {2023-05-21},
  abstract = {Scene graph generation (SGG) is designed to extract (subject, predicate, object) triplets in images. Recent works have made a steady progress on SGG, and provide useful tools for high-level vision and language understanding. However, due to the data distribution problems including long-tail distribution and semantic ambiguity, the predictions of current SGG models tend to collapse to several frequent but uninformative predicates (e.g., on, at), which limits practical application of these models in downstream tasks. To deal with the problems above, we propose a novel Internal and External Data Transfer (IETrans) method, which can be applied in a plug-and-play fashion and expanded to large SGG with 1,807 predicate classes. Our IETrans tries to relieve the data distribution problem by automatically creating an enhanced dataset that provides more sufficient and coherent annotations for all predicates. By training on the enhanced dataset, a Neural Motif model doubles the macro performance while maintaining competitive micro performance. The code and data are publicly available at https://github.com/waxnkw/IETrans-SGG.pytorch.},
  pubstate = {prepublished},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Zhang et al_2022_Fine-Grained Scene Graph Generation with Data Transfer.pdf;C\:\\Users\\chsey\\Zotero\\storage\\EKDRZVS5\\2203.html}
}

@article{zhangNeRFactorNeuralFactorization2021,
  title = {{{NeRFactor}}: {{Neural Factorization}} of {{Shape}} and {{Reflectance Under}} an {{Unknown Illumination}}},
  shorttitle = {{{NeRFactor}}},
  author = {Zhang, Xiuming and Srinivasan, Pratul P. and Deng, Boyang and Debevec, Paul and Freeman, William T. and Barron, Jonathan T.},
  date = {2021-12},
  journaltitle = {ACM Transactions on Graphics},
  shortjournal = {ACM Trans. Graph.},
  volume = {40},
  number = {6},
  eprint = {2106.01970},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--18},
  issn = {0730-0301, 1557-7368},
  doi = {10.1145/3478513.3480496},
  url = {http://arxiv.org/abs/2106.01970},
  urldate = {2023-02-02},
  abstract = {We address the problem of recovering the shape and spatially-varying reflectance of an object from multi-view images (and their camera poses) of an object illuminated by one unknown lighting condition. This enables the rendering of novel views of the object under arbitrary environment lighting and editing of the object's material properties. The key to our approach, which we call Neural Radiance Factorization (NeRFactor), is to distill the volumetric geometry of a Neural Radiance Field (NeRF) [Mildenhall et al. 2020] representation of the object into a surface representation and then jointly refine the geometry while solving for the spatially-varying reflectance and environment lighting. Specifically, NeRFactor recovers 3D neural fields of surface normals, light visibility, albedo, and Bidirectional Reflectance Distribution Functions (BRDFs) without any supervision, using only a re-rendering loss, simple smoothness priors, and a data-driven BRDF prior learned from real-world BRDF measurements. By explicitly modeling light visibility, NeRFactor is able to separate shadows from albedo and synthesize realistic soft or hard shadows under arbitrary lighting conditions. NeRFactor is able to recover convincing 3D models for free-viewpoint relighting in this challenging and underconstrained capture setup for both synthetic and real scenes. Qualitative and quantitative experiments show that NeRFactor outperforms classic and deep learning-based state of the art across various tasks. Our videos, code, and data are available at people.csail.mit.edu/xiuming/projects/nerfactor/.},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Graphics},
  file = {Y\:\\paper\\2022 winter intern\\Zhang et al_2021_NeRFactor.pdf;C\:\\Users\\chsey\\Zotero\\storage\\NHLG8PCZ\\2106.html}
}

@article{zhangSingleImageSuperResolution2012,
  title = {Single {{Image Super-Resolution With Non-Local Means}} and {{Steering Kernel Regression}}},
  author = {Zhang, Kaibing and Gao, Xinbo and Tao, Dacheng and Li, Xuelong},
  date = {2012-11},
  journaltitle = {IEEE Transactions on Image Processing},
  volume = {21},
  number = {11},
  pages = {4544--4556},
  issn = {1941-0042},
  doi = {10.1109/TIP.2012.2208977},
  abstract = {Image super-resolution (SR) reconstruction is essentially an ill-posed problem, so it is important to design an effective prior. For this purpose, we propose a novel image SR method by learning both non-local and local regularization priors from a given low-resolution image. The non-local prior takes advantage of the redundancy of similar patches in natural images, while the local prior assumes that a target pixel can be estimated by a weighted average of its neighbors. Based on the above considerations, we utilize the non-local means filter to learn a non-local prior and the steering kernel regression to learn a local prior. By assembling the two complementary regularization terms, we propose a maximum a posteriori probability framework for SR recovery. Thorough experimental results suggest that the proposed SR method can reconstruct higher quality results both quantitatively and perceptually.},
  eventtitle = {{{IEEE Transactions}} on {{Image Processing}}},
  keywords = {Image reconstruction,Image resolution,Image super-resolution,Interpolation,Kernel,non-local means,PSNR,regularization prior,self-similarity,steering kernel regression,Strontium,Vectors},
  file = {Y\:\\paper\\Computer Vision\\traditional\\super-resolution\\Zhang et al_2012_Single Image Super-Resolution With Non-Local Means and Steering Kernel.pdf;C\:\\Users\\chsey\\Zotero\\storage\\SX3W7UJT\\6241428.html}
}

@inproceedings{zhangSpatiotemporalCompressiveSensing2009,
  title = {Spatio-Temporal Compressive Sensing and Internet Traffic Matrices},
  booktitle = {Proceedings of the {{ACM SIGCOMM}} 2009 Conference on {{Data}} Communication},
  author = {Zhang, Yin and Roughan, Matthew and Willinger, Walter and Qiu, Lili},
  year = {8월 16, 2009},
  series = {{{SIGCOMM}} '09},
  pages = {267--278},
  publisher = {Association for Computing Machinery},
  location = {New York, NY, USA},
  doi = {10.1145/1592568.1592600},
  url = {https://dl.acm.org/doi/10.1145/1592568.1592600},
  urldate = {2024-04-11},
  abstract = {Many basic network engineering tasks (e.g., traffic engineering, capacity planning, anomaly detection) rely heavily on the availability and accuracy of traffic matrices. However, in practice it is challenging to reliably measure traffic matrices. Missing values are common. This observation brings us into the realm of compressive sensing, a generic technique for dealing with missing values that exploits the presence of structure and redundancy in many real-world systems. Despite much recent progress made in compressive sensing, existing compressive-sensing solutions often perform poorly for traffic matrix interpolation, because real traffic matrices rarely satisfy the technical conditions required for these solutions. To address this problem, we develop a novel spatio-temporal compressive sensing framework with two key components: (i) a new technique called Sparsity Regularized Matrix Factorization (SRMF) that leverages the sparse or low-rank nature of real-world traffic matrices and their spatio-temporal properties, and (ii) a mechanism for combining low-rank approximations with local interpolation procedures. We illustrate our new framework and demonstrate its superior performance in problems involving interpolation with real traffic matrices where we can successfully replace up to 98\% of the values. Evaluation in applications such as network tomography, traffic prediction, and anomaly detection confirms the flexibility and effectiveness of our approach.},
  isbn = {978-1-60558-594-9},
  keywords = {anomaly detection,compressive sensing,interpolation,notion,prediction,tomography,traffic matrix},
  file = {Y:\paper\2024_research\Zhang et al_2009_Spatio-temporal compressive sensing and internet traffic matrices.pdf}
}

@article{zhangSurveySparseRepresentation2015,
  title = {A {{Survey}} of {{Sparse Representation}}: {{Algorithms}} and {{Applications}}},
  shorttitle = {A {{Survey}} of {{Sparse Representation}}},
  author = {Zhang, Zheng and Xu, Yong and Yang, Jian and Li, Xuelong and Zhang, David},
  date = {2015},
  journaltitle = {IEEE Access},
  shortjournal = {IEEE Access},
  volume = {3},
  pages = {490--530},
  issn = {2169-3536},
  doi = {10.1109/ACCESS.2015.2430359},
  url = {https://ieeexplore.ieee.org/document/7102696/},
  urldate = {2024-05-19},
  abstract = {Sparse representation has attracted much attention from researchers in fields of signal processing, image processing, computer vision, and pattern recognition. Sparse representation also has a good reputation in both theoretical research and practical applications. Many different algorithms have been proposed for sparse representation. The main purpose of this paper is to provide a comprehensive study and an updated review on sparse representation and to supply guidance for researchers. The taxonomy of sparse representation methods can be studied from various viewpoints. For example, in terms of different norm minimizations used in sparsity constraints, the methods can be roughly categorized into five groups: 1) sparse representation with l0-norm minimization; 2) sparse representation with lp-norm (0 {$<$} p {$<$} 1) minimization; 3) sparse representation with l1-norm minimization; 4) sparse representation with l2,1-norm minimization; and 5) sparse representation with l2-norm minimization. In this paper, a comprehensive overview of sparse representation is provided. The available sparse representation algorithms can also be empirically categorized into four groups: 1) greedy strategy approximation; 2) constrained optimization; 3) proximity algorithm-based optimization; and 4) homotopy algorithm-based sparse representation. The rationales of different algorithms in each category are analyzed and a wide range of sparse representation applications are summarized, which could sufficiently reveal the potential nature of the sparse representation theory. In particular, an experimentally comparative study of these sparse representation algorithms was presented.},
  langid = {english},
  keywords = {notion},
  file = {C:\Users\chsey\Zotero\storage\NM4JRLZL\Zhang 등 - 2015 - A Survey of Sparse Representation Algorithms and .pdf}
}

@online{zhangWhyAreAdaptive2020,
  title = {Why Are {{Adaptive Methods Good}} for {{Attention Models}}?},
  author = {Zhang, Jingzhao and Karimireddy, Sai Praneeth and Veit, Andreas and Kim, Seungyeon and Reddi, Sashank J. and Kumar, Sanjiv and Sra, Suvrit},
  date = {2020-10-23},
  eprint = {1912.03194},
  eprinttype = {arXiv},
  eprintclass = {cs, math},
  url = {http://arxiv.org/abs/1912.03194},
  urldate = {2024-06-01},
  abstract = {While stochastic gradient descent (SGD) is still the de facto algorithm in deep learning, adaptive methods like Clipped SGD/Adam have been observed to outperform SGD across important tasks, such as attention models. The settings under which SGD performs poorly in comparison to adaptive methods are not well understood yet. In this paper, we provide empirical and theoretical evidence that a heavy-tailed distribution of the noise in stochastic gradients is one cause of SGD’s poor performance. We provide the first tight upper and lower convergence bounds for adaptive gradient methods under heavy-tailed noise. Further, we demonstrate how gradient clipping plays a key role in addressing heavy-tailed gradient noise. Subsequently, we show how clipping can be applied in practice by developing an adaptive coordinate-wise clipping algorithm (ACClip) and demonstrate its superior performance on BERT pretraining and finetuning tasks.},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,Mathematics - Optimization and Control,notion},
  file = {Y:\paper\2024_lecture\Zhang et al_2020_Why are Adaptive Methods Good for Attention Models.pdf}
}

@inproceedings{zhanProduct1MWeaklySupervised2021,
  title = {{{Product1M}}: {{Towards Weakly Supervised Instance-Level Product Retrieval}} via {{Cross-Modal Pretraining}}},
  shorttitle = {{{Product1M}}},
  booktitle = {2021 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  author = {Zhan, Xunlin and Wu, Yangxin and Dong, Xiao and Wei, Yunchao and Lu, Minlong and Zhang, Yichi and Xu, Hang and Liang, Xiaodan},
  date = {2021-10},
  pages = {11762--11771},
  publisher = {IEEE},
  location = {Montreal, QC, Canada},
  doi = {10.1109/ICCV48922.2021.01157},
  url = {https://ieeexplore.ieee.org/document/9710435/},
  urldate = {2024-03-12},
  abstract = {Nowadays, customer’s demands for E-commerce are more diversified, which introduces more complications to the product retrieval industry. Previous methods are either subject to single-modal input or perform supervised imagelevel product retrieval, thus fail to accommodate real-life scenarios where enormous weakly annotated multi-modal data are present. In this paper, we investigate a more realistic setting that aims to perform weakly-supervised multimodal instance-level product retrieval among fine-grained product categories. To promote the study of this challenging task, we contribute Product1M, one of the largest multimodal cosmetic datasets for real-world instance-level retrieval. Notably, Product1M contains over 1 million imagecaption pairs and consists of two sample types, i.e., singleproduct and multi-product samples, which encompass a wide variety of cosmetics brands. In addition to the great diversity, Product1M enjoys several appealing characteristics including fine-grained categories, complex combinations, and fuzzy correspondence that well mimic the realworld scenes. Moreover, we propose a novel model named Cross-modal contrAstive Product Transformer for instancelevel prodUct REtrieval (CAPTURE), that excels in capturing the potential synergy between multi-modal inputs via a hybrid-stream transformer in a self-supervised manner. CAPTURE generates discriminative instance features via masked multi-modal learning as well as cross-modal contrastive pretraining and it outperforms several SOTA crossmodal baselines. Extensive ablation studies well demonstrate the effectiveness and the generalization capacity of our model. Dataset and codes are available at https: //github.com/zhanxlin/Product1M .},
  eventtitle = {2021 {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}} ({{ICCV}})},
  isbn = {978-1-66542-812-5},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2024_research\Zhan et al_2021_Product1M.pdf}
}

@inproceedings{zhaoDataAugmentationUsing2019,
  title = {Data {{Augmentation Using Learned Transformations}} for {{One-Shot Medical Image Segmentation}}},
  booktitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  author = {Zhao, Amy and Balakrishnan, Guha and Durand, Fredo and Guttag, John V. and Dalca, Adrian V.},
  date = {2019-06},
  pages = {8535--8545},
  publisher = {IEEE},
  location = {Long Beach, CA, USA},
  doi = {10.1109/CVPR.2019.00874},
  url = {https://ieeexplore.ieee.org/document/8953991/},
  urldate = {2022-07-20},
  abstract = {Image segmentation is an important task in many medical applications. Methods based on convolutional neural networks attain state-of-the-art accuracy; however, they typically rely on supervised training with large labeled datasets. Labeling medical images requires significant expertise and time, and typical hand-tuned approaches for data augmentation fail to capture the complex variations in such images.},
  eventtitle = {2019 {{IEEE}}/{{CVF Conference}} on {{Computer Vision}} and {{Pattern Recognition}} ({{CVPR}})},
  isbn = {978-1-72813-293-8},
  langid = {english},
  file = {Y:\paper\2022 summer intern\assignment\data augmentation\Zhao et al_2019_Data Augmentation Using Learned Transformations for One-Shot Medical Image.pdf}
}

@inproceedings{zhaoGenerativePromptModel2023,
  title = {Generative {{Prompt Model}} for {{Weakly Supervised Object Localization}}},
  author = {Zhao, Yuzhong and Ye, Qixiang and Wu, Weijia and Shen, Chunhua and Wan, Fang},
  date = {2023},
  pages = {6351--6361},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Zhao_Generative_Prompt_Model_for_Weakly_Supervised_Object_Localization_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Zhao et al_2023_Generative Prompt Model for Weakly Supervised Object Localization.pdf}
}

@online{zhaoUnleashingTexttoImageDiffusion2023,
  title = {Unleashing {{Text-to-Image Diffusion Models}} for {{Visual Perception}}},
  author = {Zhao, Wenliang and Rao, Yongming and Liu, Zuyan and Liu, Benlin and Zhou, Jie and Lu, Jiwen},
  date = {2023-03-03},
  eprint = {2303.02153},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.02153},
  url = {http://arxiv.org/abs/2303.02153},
  urldate = {2023-08-25},
  abstract = {Diffusion models (DMs) have become the new trend of generative models and have demonstrated a powerful ability of conditional synthesis. Among those, text-to-image diffusion models pre-trained on large-scale image-text pairs are highly controllable by customizable prompts. Unlike the unconditional generative models that focus on low-level attributes and details, text-to-image diffusion models contain more high-level knowledge thanks to the vision-language pre-training. In this paper, we propose VPD (Visual Perception with a pre-trained Diffusion model), a new framework that exploits the semantic information of a pre-trained text-to-image diffusion model in visual perception tasks. Instead of using the pre-trained denoising autoencoder in a diffusion-based pipeline, we simply use it as a backbone and aim to study how to take full advantage of the learned knowledge. Specifically, we prompt the denoising decoder with proper textual inputs and refine the text features with an adapter, leading to a better alignment to the pre-trained stage and making the visual contents interact with the text prompts. We also propose to utilize the cross-attention maps between the visual features and the text features to provide explicit guidance. Compared with other pre-training methods, we show that vision-language pre-trained diffusion models can be faster adapted to downstream visual perception tasks using the proposed VPD. Extensive experiments on semantic segmentation, referring image segmentation and depth estimation demonstrates the effectiveness of our method. Notably, VPD attains 0.254 RMSE on NYUv2 depth estimation and 73.3\% oIoU on RefCOCO-val referring image segmentation, establishing new records on these two benchmarks. Code is available at https://github.com/wl-zhao/VPD},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\2023 graduation\\visual language\\background\\Zhao et al_2023_Unleashing Text-to-Image Diffusion Models for Visual Perception.pdf;C\:\\Users\\chsey\\Zotero\\storage\\4QDANU33\\2303.html}
}

@article{zhaoVideoTextVisual2022,
  title = {Towards {{Video Text Visual Question Answering}}: {{Benchmark}} and {{Baseline}}},
  shorttitle = {Towards {{Video Text Visual Question Answering}}},
  author = {Zhao, Minyi and Li, Bingjia and Wang, Jie and Li, Wanqing and Zhou, Wenjing and Zhang, Lan and Xuyang, Shijie and Yu, Zhihang and Yu, Xinkun and Li, Guangze and Dai, Aobotao and Zhou, Shuigeng},
  date = {2022-12-06},
  journaltitle = {Advances in Neural Information Processing Systems},
  volume = {35},
  pages = {35549--35562},
  url = {https://proceedings.neurips.cc/paper_files/paper/2022/hash/e726197ffd401df4013cd9f81007b5cf-Abstract-Datasets_and_Benchmarks.html},
  urldate = {2023-05-23},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\Zhao et al_2022_Towards Video Text Visual Question Answering.pdf}
}

@online{zhengPrototypebasedEmbeddingNetwork2023,
  title = {Prototype-Based {{Embedding Network}} for {{Scene Graph Generation}}},
  author = {Zheng, Chaofan and Lyu, Xinyu and Gao, Lianli and Dai, Bo and Song, Jingkuan},
  date = {2023-03-13},
  eprint = {2303.07096},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2303.07096},
  url = {http://arxiv.org/abs/2303.07096},
  urldate = {2023-05-21},
  abstract = {Current Scene Graph Generation (SGG) methods explore contextual information to predict relationships among entity pairs. However, due to the diverse visual appearance of numerous possible subject-object combinations, there is a large intra-class variation within each predicate category, e.g., "man-eating-pizza, giraffe-eating-leaf", and the severe inter-class similarity between different classes, e.g., "man-holding-plate, man-eating-pizza", in model's latent space. The above challenges prevent current SGG methods from acquiring robust features for reliable relation prediction. In this paper, we claim that the predicate's category-inherent semantics can serve as class-wise prototypes in the semantic space for relieving the challenges. To the end, we propose the Prototype-based Embedding Network (PE-Net), which models entities/predicates with prototype-aligned compact and distinctive representations and thereby establishes matching between entity pairs and predicates in a common embedding space for relation recognition. Moreover, Prototype-guided Learning (PL) is introduced to help PE-Net efficiently learn such entitypredicate matching, and Prototype Regularization (PR) is devised to relieve the ambiguous entity-predicate matching caused by the predicate's semantic overlap. Extensive experiments demonstrate that our method gains superior relation recognition capability on SGG, achieving new state-of-the-art performances on both Visual Genome and Open Images datasets.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Zheng et al_2023_Prototype-based Embedding Network for Scene Graph Generation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5GVRXEP7\\2303.html}
}

@article{zhouClassIncrementalLearningSurvey2024,
  title = {Class-{{Incremental Learning}}: {{A Survey}}},
  shorttitle = {Class-{{Incremental Learning}}},
  author = {Zhou, Da-Wei and Wang, Qi-Wei and Qi, Zhi-Hong and Ye, Han-Jia and Zhan, De-Chuan and Liu, Ziwei},
  date = {2024},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  shortjournal = {IEEE Trans. Pattern Anal. Mach. Intell.},
  eprint = {2302.03648},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--20},
  issn = {0162-8828, 2160-9292, 1939-3539},
  doi = {10.1109/TPAMI.2024.3429383},
  url = {http://arxiv.org/abs/2302.03648},
  urldate = {2024-09-12},
  abstract = {Deep models, e.g., CNNs and Vision Transformers, have achieved impressive achievements in many vision tasks in the closed world. However, novel classes emerge from time to time in our ever-changing world, requiring a learning system to acquire new knowledge continually. Class-Incremental Learning (CIL) enables the learner to incorporate the knowledge of new classes incrementally and build a universal classifier among all seen classes. Correspondingly, when directly training the model with new class instances, a fatal problem occurs — the model tends to catastrophically forget the characteristics of former ones, and its performance drastically degrades. There have been numerous efforts to tackle catastrophic forgetting in the machine learning community. In this paper, we survey comprehensively recent advances in class-incremental learning and summarize these methods from several aspects. We also provide a rigorous and unified evaluation of 17 methods in benchmark image classification tasks to find out the characteristics of different algorithms empirically. Furthermore, we notice that the current comparison protocol ignores the influence of memory budget in model storage, which may result in unfair comparison and biased results. Hence, we advocate fair comparison by aligning the memory budget in evaluation, as well as several memory-agnostic performance measures. The source code is available at https://github.com/zhoudw-zdw/CIL\_Survey/.},
  langid = {english},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning},
  file = {C:\Users\chsey\Zotero\storage\XW3FWGIG\Zhou 등 - 2024 - Class-Incremental Learning A Survey.pdf}
}

@article{zhouClassIncrementalLearningSurvey2024a,
  title = {Class-{{Incremental Learning}}: {{A Survey}}},
  shorttitle = {Class-{{Incremental Learning}}},
  author = {Zhou, Da-Wei and Wang, Qi-Wei and Qi, Zhi-Hong and Ye, Han-Jia and Zhan, De-Chuan and Liu, Ziwei},
  date = {2024},
  journaltitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  shortjournal = {IEEE Trans. Pattern Anal. Mach. Intell.},
  eprint = {2302.03648},
  eprinttype = {arXiv},
  eprintclass = {cs},
  pages = {1--20},
  issn = {0162-8828, 2160-9292, 1939-3539},
  doi = {10.1109/TPAMI.2024.3429383},
  url = {http://arxiv.org/abs/2302.03648},
  urldate = {2024-09-12},
  abstract = {Deep models, e.g., CNNs and Vision Transformers, have achieved impressive achievements in many vision tasks in the closed world. However, novel classes emerge from time to time in our ever-changing world, requiring a learning system to acquire new knowledge continually. Class-Incremental Learning (CIL) enables the learner to incorporate the knowledge of new classes incrementally and build a universal classifier among all seen classes. Correspondingly, when directly training the model with new class instances, a fatal problem occurs -- the model tends to catastrophically forget the characteristics of former ones, and its performance drastically degrades. There have been numerous efforts to tackle catastrophic forgetting in the machine learning community. In this paper, we survey comprehensively recent advances in class-incremental learning and summarize these methods from several aspects. We also provide a rigorous and unified evaluation of 17 methods in benchmark image classification tasks to find out the characteristics of different algorithms empirically. Furthermore, we notice that the current comparison protocol ignores the influence of memory budget in model storage, which may result in unfair comparison and biased results. Hence, we advocate fair comparison by aligning the memory budget in evaluation, as well as several memory-agnostic performance measures. The source code is available at https://github.com/zhoudw-zdw/CIL\_Survey/},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Zhou et al_2024_Class-Incremental Learning.pdf;C\:\\Users\\chsey\\Zotero\\storage\\X9Z7KL7U\\2302.html}
}

@online{zhouExpandableSubspaceEnsemble2024,
  title = {Expandable {{Subspace Ensemble}} for {{Pre-Trained Model-Based Class-Incremental Learning}}},
  author = {Zhou, Da-Wei and Sun, Hai-Long and Ye, Han-Jia and Zhan, De-Chuan},
  date = {2024-03-18},
  eprint = {2403.12030},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2403.12030},
  url = {http://arxiv.org/abs/2403.12030},
  urldate = {2024-09-12},
  abstract = {Class-Incremental Learning (CIL) requires a learning system to continually learn new classes without forgetting. Despite the strong performance of Pre-Trained Models (PTMs) in CIL, a critical issue persists: learning new classes often results in the overwriting of old ones. Excessive modification of the network causes forgetting, while minimal adjustments lead to an inadequate fit for new classes. As a result, it is desired to figure out a way of efficient model updating without harming former knowledge. In this paper, we propose ExpAndable Subspace Ensemble (EASE) for PTM-based CIL. To enable model updating without conflict, we train a distinct lightweight adapter module for each new task, aiming to create task-specific subspaces. These adapters span a high-dimensional feature space, enabling joint decision-making across multiple subspaces. As data evolves, the expanding subspaces render the old class classifiers incompatible with new-stage spaces. Correspondingly, we design a semantic-guided prototype complement strategy that synthesizes old classes' new features without using any old class instance. Extensive experiments on seven benchmark datasets verify EASE's state-of-the-art performance. Code is available at: https://github.com/sun-hailong/CVPR24-Ease},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {Y\:\\paper\\2024_research\\Zhou et al_2024_Expandable Subspace Ensemble for Pre-Trained Model-Based Class-Incremental.pdf;C\:\\Users\\chsey\\Zotero\\storage\\VUFEC64D\\2403.html}
}

@online{zhouLearningDeepFeatures2015,
  title = {Learning {{Deep Features}} for {{Discriminative Localization}}},
  author = {Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  date = {2015-12-13},
  eprint = {1512.04150},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1512.04150},
  url = {http://arxiv.org/abs/1512.04150},
  urldate = {2023-08-05},
  abstract = {In this work, we revisit the global average pooling layer proposed in [13], and shed light on how it explicitly enables the convolutional neural network to have remarkable localization ability despite being trained on image-level labels. While this technique was previously proposed as a means for regularizing training, we find that it actually builds a generic localizable deep representation that can be applied to a variety of tasks. Despite the apparent simplicity of global average pooling, we are able to achieve 37.1\% top-5 error for object localization on ILSVRC 2014, which is remarkably close to the 34.2\% top-5 error achieved by a fully supervised CNN approach. We demonstrate that our network is able to localize the discriminative image regions on a variety of tasks despite not being trained for them},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\understanding deep CNN\\Zhou et al_2015_Learning Deep Features for Discriminative Localization.pdf;C\:\\Users\\chsey\\Zotero\\storage\\96CA6J78\\1512.html}
}

@online{zhouNonVacuousGeneralizationBounds2019,
  title = {Non-{{Vacuous Generalization Bounds}} at the {{ImageNet Scale}}: {{A PAC-Bayesian Compression Approach}}},
  shorttitle = {Non-{{Vacuous Generalization Bounds}} at the {{ImageNet Scale}}},
  author = {Zhou, Wenda and Veitch, Victor and Austern, Morgane and Adams, Ryan P. and Orbanz, Peter},
  date = {2019-02-24},
  eprint = {1804.05862},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1804.05862},
  url = {http://arxiv.org/abs/1804.05862},
  urldate = {2024-04-14},
  abstract = {Modern neural networks are highly overparameterized, with capacity to substantially overfit to training data. Nevertheless, these networks often generalize well in practice. It has also been observed that trained networks can often be "compressed" to much smaller representations. The purpose of this paper is to connect these two empirical observations. Our main technical result is a generalization bound for compressed networks based on the compressed size. Combined with off-the-shelf compression algorithms, the bound leads to state of the art generalization guarantees; in particular, we provide the first non-vacuous generalization guarantees for realistic architectures applied to the ImageNet classification problem. As additional evidence connecting compression and generalization, we show that compressibility of models that tend to overfit is limited: We establish an absolute limit on expected compressibility as a function of expected generalization error, where the expectations are over the random choice of training examples. The bounds are complemented by empirical results that show an increase in overfitting implies an increase in the number of bits required to describe a trained network.},
  pubstate = {prepublished},
  keywords = {Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\2024_research\\Zhou et al_2019_Non-Vacuous Generalization Bounds at the ImageNet Scale.pdf;C\:\\Users\\chsey\\Zotero\\storage\\KM3AZS8C\\1804.html}
}

@online{zhouRevisitingClassIncrementalLearning2024,
  title = {Revisiting {{Class-Incremental Learning}} with {{Pre-Trained Models}}: {{Generalizability}} and {{Adaptivity}} Are {{All You Need}}},
  shorttitle = {Revisiting {{Class-Incremental Learning}} with {{Pre-Trained Models}}},
  author = {Zhou, Da-Wei and Cai, Zi-Wen and Ye, Han-Jia and Zhan, De-Chuan and Liu, Ziwei},
  date = {2024-08-05},
  eprint = {2303.07338},
  eprinttype = {arXiv},
  eprintclass = {cs},
  url = {http://arxiv.org/abs/2303.07338},
  urldate = {2024-09-19},
  abstract = {Class-incremental learning (CIL) aims to adapt to emerging new classes without forgetting old ones. Traditional CIL models are trained from scratch to continually acquire knowledge as data evolves. Recently, pre-training has achieved substantial progress, making vast pre-trained models (PTMs) accessible for CIL. Contrary to traditional methods, PTMs possess generalizable embeddings, which can be easily transferred for CIL. In this work, we revisit CIL with PTMs and argue that the core factors in CIL are adaptivity for model updating and generalizability for knowledge transferring. 1) We first reveal that frozen PTM can already provide generalizable embeddings for CIL. Surprisingly, a simple baseline (SimpleCIL) which continually sets the classifiers of PTM to prototype features can beat state-of-the-art even without training on the downstream task. 2) Due to the distribution gap between pre-trained and downstream datasets, PTM can be further cultivated with adaptivity via model adaptation. We propose AdaPt and mERge (APER), which aggregates the embeddings of PTM and adapted models for classifier construction. APER is a general framework that can be orthogonally combined with any parameter-efficient tuning method, which holds the advantages of PTM's generalizability and adapted model's adaptivity. 3) Additionally, considering previous ImageNet-based benchmarks are unsuitable in the era of PTM due to data overlapping, we propose four new benchmarks for assessment, namely ImageNet-A, ObjectNet, OmniBenchmark, and VTAB. Extensive experiments validate the effectiveness of APER with a unified and concise framework. Code is available at https://github.com/zhoudw-zdw/RevisitingCIL},
  langid = {english},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion},
  file = {C:\Users\chsey\Zotero\storage\K2NXWHEH\Zhou 등 - 2024 - Revisiting Class-Incremental Learning with Pre-Tra.pdf}
}

@online{zhouUnsupervisedLearningDepth2017,
  title = {Unsupervised {{Learning}} of {{Depth}} and {{Ego-Motion}} from {{Video}}},
  author = {Zhou, Tinghui and Brown, Matthew and Snavely, Noah and Lowe, David G.},
  date = {2017-07-31},
  eprint = {1704.07813},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1704.07813},
  url = {http://arxiv.org/abs/1704.07813},
  urldate = {2023-08-05},
  abstract = {We present an unsupervised learning framework for the task of monocular depth and camera motion estimation from unstructured video sequences. We achieve this by simultaneously training depth and camera pose estimation networks using the task of view synthesis as the supervisory signal. The networks are thus coupled via the view synthesis objective during training, but can be applied independently at test time. Empirical evaluation on the KITTI dataset demonstrates the effectiveness of our approach: 1) monocular depth performing comparably with supervised methods that use either ground-truth pose or depth for training, and 2) pose estimation performing favorably with established SLAM systems under comparable input settings.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\2.5d image understanding\\Zhou et al_2017_Unsupervised Learning of Depth and Ego-Motion from Video.pdf;C\:\\Users\\chsey\\Zotero\\storage\\PAX544KM\\1704.html}
}

@inproceedings{zhuDeformableDETRDeformable2021,
  title = {Deformable {{DETR}}: {{Deformable Transformers}} for {{End-to-End Object Detection}}},
  shorttitle = {Deformable {{DETR}}},
  author = {Zhu, Xizhou and Su, Weijie and Lu, Lewei and Li, Bin and Wang, Xiaogang and Dai, Jifeng},
  date = {2021-01-12},
  url = {https://openreview.net/forum?id=gZ9hCDWe6ke},
  urldate = {2023-05-28},
  abstract = {DETR has been recently proposed to eliminate the need for many hand-designed components in object detection while demonstrating good performance. However, it suffers from slow convergence and limited feature spatial resolution, due to the limitation of Transformer attention modules in processing image feature maps. To mitigate these issues, we proposed Deformable DETR, whose attention modules only attend to a small set of key sampling points around a reference. Deformable DETR can achieve better performance than DETR (especially on small objects) with 10\$\textbackslash times\$ less training epochs. Extensive experiments on the COCO benchmark demonstrate the effectiveness of our approach. Code is released at https://github.com/fundamentalvision/Deformable-DETR.},
  eventtitle = {International {{Conference}} on {{Learning Representations}}},
  langid = {english},
  file = {Y:\paper\2023_nips_dataset_track\related_works_references\visual to natural language\image captioning\Zhu et al_2021_Deformable DETR.pdf}
}

@inproceedings{zhuNotAllFeatures2023,
  title = {Not {{All Features Matter}}: {{Enhancing Few-shot CLIP}} with {{Adaptive Prior Refinement}}},
  shorttitle = {Not {{All Features Matter}}},
  author = {Zhu, Xiangyang and Zhang, Renrui and He, Bowei and Zhou, Aojun and Wang, Dong and Zhao, Bin and Gao, Peng},
  date = {2023},
  pages = {2605--2615},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Zhu_Not_All_Features_Matter_Enhancing_Few-shot_CLIP_with_Adaptive_Prior_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_few_shot\Zhu et al_2023_Not All Features Matter.pdf}
}

@inproceedings{zhuPromptalignedGradientPrompt2023,
  title = {Prompt-Aligned {{Gradient}} for {{Prompt Tuning}}},
  author = {Zhu, Beier and Niu, Yulei and Han, Yucheng and Wu, Yue and Zhang, Hanwang},
  date = {2023},
  pages = {15659--15669},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Zhu_Prompt-aligned_Gradient_for_Prompt_Tuning_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Zhu et al_2023_Prompt-aligned Gradient for Prompt Tuning.pdf}
}

@online{zhuSceneGraphGeneration2022,
  title = {Scene {{Graph Generation}}: {{A Comprehensive Survey}}},
  shorttitle = {Scene {{Graph Generation}}},
  author = {Zhu, Guangming and Zhang, Liang and Jiang, Youliang and Dang, Yixuan and Hou, Haoran and Shen, Peiyi and Feng, Mingtao and Zhao, Xia and Miao, Qiguang and Shah, Syed Afaq Ali and Bennamoun, Mohammed},
  date = {2022-06-22},
  eprint = {2201.00443},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.2201.00443},
  url = {http://arxiv.org/abs/2201.00443},
  urldate = {2023-04-24},
  abstract = {Deep learning techniques have led to remarkable breakthroughs in the field of generic object detection and have spawned a lot of scene-understanding tasks in recent years. Scene graph has been the focus of research because of its powerful semantic representation and applications to scene understanding. Scene Graph Generation (SGG) refers to the task of automatically mapping an image into a semantic structural scene graph, which requires the correct labeling of detected objects and their relationships. Although this is a challenging task, the community has proposed a lot of SGG approaches and achieved good results. In this paper, we provide a comprehensive survey of recent achievements in this field brought about by deep learning techniques. We review 138 representative works that cover different input modalities, and systematically summarize existing methods of image-based SGG from the perspective of feature extraction and fusion. We attempt to connect and systematize the existing visual relationship detection methods, to summarize, and interpret the mechanisms and the strategies of SGG in a comprehensive way. Finally, we finish this survey with deep discussions about current existing problems and future research directions. This survey will help readers to develop a better understanding of the current research status and ideas.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {Y\:\\paper\\2022 winter intern\\scene_graph_generation\\Zhu et al_2022_Scene Graph Generation.pdf;C\:\\Users\\chsey\\Zotero\\storage\\V9PDZUBQ\\2201.html}
}

@inproceedings{zhuSegPromptBoostingOpenWorld2023,
  title = {{{SegPrompt}}: {{Boosting Open-World Segmentation}} via {{Category-Level Prompt Learning}}},
  shorttitle = {{{SegPrompt}}},
  author = {Zhu, Muzhi and Li, Hengtao and Chen, Hao and Fan, Chengxiang and Mao, Weian and Jing, Chenchen and Liu, Yifan and Shen, Chunhua},
  date = {2023},
  pages = {999--1008},
  url = {https://openaccess.thecvf.com/content/ICCV2023/html/Zhu_SegPrompt_Boosting_Open-World_Segmentation_via_Category-Level_Prompt_Learning_ICCV_2023_paper.html},
  urldate = {2023-10-04},
  eventtitle = {Proceedings of the {{IEEE}}/{{CVF International Conference}} on {{Computer Vision}}},
  langid = {english},
  keywords = {notion,Segmentation},
  file = {Y:\paper\2023 graduation\visual language\iccv_2023_prompt\Zhu et al_2023_SegPrompt.pdf}
}

@article{zhuUnpairedImagetoImageTranslation2017,
  title = {Unpaired {{Image-to-Image Translation}} Using {{Cycle-Consistent Adversarial Networks}}},
  author = {Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A.},
  date = {2017-03-30},
  doi = {10.48550/arXiv.1703.10593},
  url = {https://arxiv.org/abs/1703.10593v7},
  urldate = {2022-12-09},
  abstract = {Image-to-image translation is a class of vision and graphics problems where the goal is to learn the mapping between an input image and an output image using a training set of aligned image pairs. However, for many tasks, paired training data will not be available. We present an approach for learning to translate an image from a source domain \$X\$ to a target domain \$Y\$ in the absence of paired examples. Our goal is to learn a mapping \$G: X \textbackslash rightarrow Y\$ such that the distribution of images from \$G(X)\$ is indistinguishable from the distribution \$Y\$ using an adversarial loss. Because this mapping is highly under-constrained, we couple it with an inverse mapping \$F: Y \textbackslash rightarrow X\$ and introduce a cycle consistency loss to push \$F(G(X)) \textbackslash approx X\$ (and vice versa). Qualitative results are presented on several tasks where paired training data does not exist, including collection style transfer, object transfiguration, season transfer, photo enhancement, etc. Quantitative comparisons against several prior methods demonstrate the superiority of our approach.},
  langid = {english},
  file = {Y:\paper\Computer Vision\traditional\PA3\Zhu et al_2017_Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks.pdf}
}

@online{zhuUnpairedImagetoImageTranslation2020,
  title = {Unpaired {{Image-to-Image Translation}} Using {{Cycle-Consistent Adversarial Networks}}},
  author = {Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A.},
  date = {2020-08-24},
  eprint = {1703.10593},
  eprinttype = {arXiv},
  eprintclass = {cs},
  doi = {10.48550/arXiv.1703.10593},
  url = {http://arxiv.org/abs/1703.10593},
  urldate = {2023-08-05},
  abstract = {Image-to-image translation is a class of vision and graphics problems where the goal is to learn the mapping between an input image and an output image using a training set of aligned image pairs. However, for many tasks, paired training data will not be available. We present an approach for learning to translate an image from a source domain \$X\$ to a target domain \$Y\$ in the absence of paired examples. Our goal is to learn a mapping \$G: X \textbackslash rightarrow Y\$ such that the distribution of images from \$G(X)\$ is indistinguishable from the distribution \$Y\$ using an adversarial loss. Because this mapping is highly under-constrained, we couple it with an inverse mapping \$F: Y \textbackslash rightarrow X\$ and introduce a cycle consistency loss to push \$F(G(X)) \textbackslash approx X\$ (and vice versa). Qualitative results are presented on several tasks where paired training data does not exist, including collection style transfer, object transfiguration, season transfer, photo enhancement, etc. Quantitative comparisons against several prior methods demonstrate the superiority of our approach.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,notion},
  file = {Y\:\\paper\\computer_vision_topics_18\\generative model\\Zhu et al_2020_Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks.pdf;C\:\\Users\\chsey\\Zotero\\storage\\5GPS4AB9\\1703.html}
}

@online{zophLearningTransferableArchitectures2018,
  title = {Learning {{Transferable Architectures}} for {{Scalable Image Recognition}}},
  author = {Zoph, Barret and Vasudevan, Vijay and Shlens, Jonathon and Le, Quoc V.},
  date = {2018-04-11},
  eprint = {1707.07012},
  eprinttype = {arXiv},
  eprintclass = {cs, stat},
  doi = {10.48550/arXiv.1707.07012},
  url = {http://arxiv.org/abs/1707.07012},
  urldate = {2023-08-05},
  abstract = {Developing neural network image classification models often requires significant architecture engineering. In this paper, we study a method to learn the model architectures directly on the dataset of interest. As this approach is expensive when the dataset is large, we propose to search for an architectural building block on a small dataset and then transfer the block to a larger dataset. The key contribution of this work is the design of a new search space (the "NASNet search space") which enables transferability. In our experiments, we search for the best convolutional layer (or "cell") on the CIFAR-10 dataset and then apply this cell to the ImageNet dataset by stacking together more copies of this cell, each with their own parameters to design a convolutional architecture, named "NASNet architecture". We also introduce a new regularization technique called ScheduledDropPath that significantly improves generalization in the NASNet models. On CIFAR-10 itself, NASNet achieves 2.4\% error rate, which is state-of-the-art. On ImageNet, NASNet achieves, among the published works, state-of-the-art accuracy of 82.7\% top-1 and 96.2\% top-5 on ImageNet. Our model is 1.2\% better in top-1 accuracy than the best human-invented architectures while having 9 billion fewer FLOPS - a reduction of 28\% in computational demand from the previous state-of-the-art model. When evaluated at different levels of computational cost, accuracies of NASNets exceed those of the state-of-the-art human-designed models. For instance, a small version of NASNet also achieves 74\% top-1 accuracy, which is 3.1\% better than equivalently-sized, state-of-the-art models for mobile platforms. Finally, the learned features by NASNet used with the Faster-RCNN framework surpass state-of-the-art by 4.0\% achieving 43.1\% mAP on the COCO dataset.},
  pubstate = {prepublished},
  keywords = {Computer Science - Computer Vision and Pattern Recognition,Computer Science - Machine Learning,notion,Statistics - Machine Learning},
  file = {Y\:\\paper\\computer_vision_topics_18\\neural architecture search\\Zoph et al_2018_Learning Transferable Architectures for Scalable Image Recognition.pdf;C\:\\Users\\chsey\\Zotero\\storage\\H78RX3UL\\1707.html}
}

@online{ZoteroYourPersonal,
  title = {Zotero | {{Your}} Personal Research Assistant},
  url = {https://www.zotero.org/},
  urldate = {2024-09-10},
  keywords = {notion}
}

@article{zouLecture02Basics,
  title = {Lecture 02- {{Basics}} of {{Image}} Processing},
  author = {Zou, Danping and Tong, Shanghai Jiao},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\Zou_Tong_Lecture 02- Basics of Image processing.pdf}
}

@article{zouLecture03Feature,
  title = {Lecture 03- {{Feature Points}} and {{Lines}}},
  author = {Zou, Danping and Tong, Shanghai Jiao},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\Zou_Tong_Lecture 03- Feature Points and Lines.pdf}
}

@article{zouLecture04Projective,
  title = {Lecture 04- {{Projective Geometry}}},
  author = {Zou, Danping and Tong, Shanghai Jiao},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\Zou_Tong_Lecture 04- Projective Geometry.pdf}
}

@article{zouLecture0607,
  title = {Lecture 06/07- {{Pose}} Estimation \& {{Absolute}} Orientation},
  author = {Zou, Danping and Tong, Shanghai Jiao},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\Zou_Tong_Lecture 06-07- Pose estimation & Absolute orientation.pdf}
}

@article{zouLecture08Nonlinear,
  title = {Lecture 08- {{Nonlinear}} Least Square \& {{RANSAC}}},
  author = {Zou, Danping},
  langid = {english},
  file = {Y:\paper\2022 winter intern\geommetric\SJU_vision_note\Zou_Lecture 08- Nonlinear least square & RANSAC.pdf}
}

@article{zuninoPredictingIntentionsMotion2020,
  title = {Predicting {{Intentions}} from {{Motion}}: {{The Subject-Adversarial Adaptation Approach}}},
  shorttitle = {Predicting {{Intentions}} from {{Motion}}},
  author = {Zunino, Andrea and Cavazza, Jacopo and Volpi, Riccardo and Morerio, Pietro and Cavallo, Andrea and Becchio, Cristina and Murino, Vittorio},
  date = {2020-01-01},
  journaltitle = {International Journal of Computer Vision},
  shortjournal = {Int J Comput Vis},
  volume = {128},
  number = {1},
  pages = {220--239},
  issn = {1573-1405},
  doi = {10.1007/s11263-019-01234-9},
  url = {https://doi.org/10.1007/s11263-019-01234-9},
  urldate = {2023-08-05},
  abstract = {This paper aims at investigating the action prediction problem from a pure kinematic perspective. Specifically, we address the problem of recognizing future actions, indeed human intentions, underlying a same initial (and apparently unrelated) motor act. This study is inspired by neuroscientific findings asserting that motor acts at the very onset are embedding information about the intention with which are performed, even when different intentions originate from a same class of movements. To demonstrate this claim in computational and empirical terms, we designed an ad hoc experiment and built a new 3D and 2D dataset where, in both training and testing, we analyze a same class of grasping movements underlying different intentions. We investigate how much the intention discriminants generalize across subjects, discovering that each subject tends to affect the prediction by his/her own bias. Inspired by the domain adaptation problem, we propose to interpret each subject as a domain, leading to a novel subject adversarial paradigm. The proposed approach favorably copes with our new problem, boosting the considered baseline features encoding 2D and 3D information and which do not exploit the subject information.},
  langid = {english},
  keywords = {Action recognition and prediction,Adversarial domain adaptation,Grasping,Human intentions,Kinematic analysis,notion},
  file = {Y:\paper\computer_vision_topics_18\memorability and intention interface\Zunino et al_2020_Predicting Intentions from Motion.pdf}
}


==> sec/backups/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/backups/2_method_1108.tex <==
% \section{Problem Definition and Previous Works}
% \begin{comment}
%     model merging은 이다.. 더욱 specifically, 같은 architecture의 model에 대하여 T개의 task에 대하여 각각이 $\{\theta_t \}_{t=1}^{T}$로 paramterized된 finentuend models $\{f(x; \theta_t)\}_i^{}$을 잘 조합하여 T개의 task를 잘 수행하는 weight $\theta$를 찾고자 한다.

% \end{comment}

\section{Preliminaries}
\paragraph{Model Merging}
Model merging aims to create a unified model that can perform multiple downstream tasks by combining individual models trained on each task. Given $T$ tasks, each task $t$ has a fine-tuned model $f(x; \theta_t)$ parameterized by $\theta_t$, where $x$ represents the input data, $\hat{y}$ the output label, and $ \theta $ the model parameters. The objective is to find a combination $\theta_{*}$ of these task-specific parameters $\theta_t$ such that the resulting model $f(x; \theta_{*})$ can perform well across all $T$ tasks. \citet{ilharcoEditingModelsTask2023} proposed the concept of a \textit{task vector}, defined as $\tau_t := \theta_t - \theta_{\text{pre}}$, where $\theta_{\text{pre}}$ represents pretrained parameters. Following this, a basic model merging approach can be represented as
\begin{equation} \label{eqn: simple merge}
    \theta_{*} = \theta_{\text{pre}} + \sum_{t=1}^{T} \lambda_{t} \tau_t.
\end{equation}

% \paragraph{Notations}
\begin{comment}
    이건 필요하다 싶을 때 살려서 notation들 넣어주도록 한다.
    생각을 해봤는데, $\{\tau_t\}$가 set of tsa vector라는 것을 나타낸다고 적어두는게 좋을 듯 하다. 
\end{comment}

\subsection{Parameter Interference}
% 이게 왜 발생하는 지 서술할 필요가 있다.
Even though Model Merging with Equation \ref{eqn: simple merge} is straightforward and effective, multi-task model (MTM) performance typically degrades as the number of merging tasks increases, a phenomenon commonly referred to as \textit{parameter interference}. Previous works address this issue using the following two approaches.

\begin{comment}
    While straightforward and effective, models merged with Equation \ref{eqn: simple merge} often suffers from task interference, which limits the merged model's performance. Previous work has attempted to mitigate this by either refining $\tau_t$ \cite{yadavTIESMergingResolvingInterference2023} or optimizing $\lambda_t$ \cite{yangAdaMergingAdaptiveModel2024a} through test-time adaptation. \cite{wangTentFullyTesttime2021}
    
    While Equation \ref{eqn: simple merge} is straightforward and effective, merging하는 task의 수가 늘어 남에 따라서 일반적으로 multi-task model (MTM) 성능이 급격하게 떨어지게 되고, 기존의 work들은 이를 \textit{parameter interference}라고 칭하고 broad하게 아래의 2개의 방식을 취하여 이를 해소한다.

    % task interfernce가 무엇인지 잘 짚고 넘어가자
    % 그리고 우리의 방법론은 저 랭크 objective와 negative similarity objective가 이를 잘 해결한다는 것을 보여야 하는데, 이를 어떠한 간단한 실험적 접근으로 보여야 할 지 고민이다.
\end{comment}

\paragraph{Task Vector Processing}
\citet{yadavTIESMergingResolvingInterference2023a} proposed a method called \textit{Trim}, where they set most of the parameters with small magnitude in the task vectors ${\tau_t}$ to zero, as these do not significantly affect the performance of the multi-task model. For parameters with large magnitude, they determined the values through majority voting among tasks called \textit {Elect and Disjoint Merge}. Additionally, \citet{yangAdaMergingAdaptiveModel2024} observed that the MTM performance varies significantly depending on the coefficients ${\lambda_t}$ in Equation \ref{eqn: simple merge}. To address this, they utilized the entropy of the model $f$'s posterior distribution $p(\hat{y}|x)$ over the test data distribution $\{\mathcal{D}_{t}^{\text{test}}\}$, where $p(\hat{y}|x)$ is the posterior distribution of the model $f$ given the input data $x$. This is defined as:

\begin{equation} \label{eqn: entropy}
     \mathcal{L}(x) = \mathbb{E}_{x \sim {\mathcal{D}_t^{\text{test}}}} \left[ -p(\hat{y}|x) \log p(\hat{y}|x) \right],
\end{equation}

and used it as a loss function at test time to tune $\{\lambda_t\}$. They experimentally demonstrated that tuning $\{\lambda_t\}$ using this loss function improves MTM performance robustly, even under drift in $\{\mathcal{D}_{t}^{\text{test}}\}$. However, both approaches have limitations in that they fix $\theta{\text{pre}}$, which can be considered the origin of $\{\tau_t\}$, and only process the task vectors $\{\tau_t\}$.
    
\begin{comment}
adamerging은 어떤 건지 좀더 생각을 해봐야겠다.
\citet{yadavTIESMergingResolvingInterference2023a}는 task vector들 $\{\tau_t\}$에서 magnitude가 작은 parameter 대부분을 MTM 성능에 영향을 주지 않기에 0으로 만드는 \textit{trimming}하고, magnitude가 큰 parameter들 중에서 tasks 간의 다수결로 value를 결정하게 된다. 또한, \citet{yangAdaMergingAdaptiveModel2024}는 Equation \ref{eqn: simple merge}의 $\{\lambda_t\}$에 따라서 MTM 성능이 크게 달라진다는 점에서 test time 에 다음으로 정의된 model f의 test data distribution $\{\mathcal{D}_{t}^{test}\}$에 대한 uncertainty인 entropy를
\begin{equation}
    \mathcal{L(x)} = \mathbb{E}_{x \sim \{\mathcal{D}_t^{test}\} }[-p(\hat{y}|x) log(\hat{y}|x)]
\end{equation}
loss로 사용하여, $\{\lambda_t\}$를 tuning하였을 때 $\{\mathcal{D}_{t}^{test}\}$ drift에도 robust하게 MTM 성능이 향상함을 실험적으로 보였다. 다만, 본질적으로 이들은 $\{\tau_t\}$들의 원점으로 볼 수 있는 $\theta_{\text{pre}}$을 고정하고 $\{\tau_t\}$만을 가공했다는 점에서 한계가 있다.
% 여기서 저자가 제시한 것처럼 이 redundant한 parameter가 task interference를 초래한다는 것으로부터, 우리도 SimMin으로부터 얻은 MTL model이 최대 rank보다 작은 rank로 자르는 것의 유의미 함으로 연결되어야 한다.
\end{comment}

\paragraph{Routing}
Under the relaxation that allows maintaining additional task-specific parameters per task, a router function $r: \mathbb{R}^d \rightarrow \mathbb{R}^T$ is employed, which dynamically determines $\{\lambda_t\}$ for each input using the feature embedding $h$ obtained just before the classification head of the model $f$. \citet{tangMergingMultiTaskModels2024} observed that task-specific knowledge is concentrated in the MLP modules of transformer architectures, leading to parameter interference. Based on this observation, they merged the attention modules using the method in Equation \ref{eqn: simple merge}, while retaining task-specific MLP modules. \citet{luTwinMergingDynamicIntegration2024} further proposed maintaining only 10\% of the original model parameters per task, based on the observation that pruning 90\% of the parameters in $\{\tau_t\}$ via Singular Value Decomposition (SVD) does not degrade performance. These methods achieve performance close to the average of single-task fine-tuned models. However, both approaches require storing additional $\mathcal{O}(T)$ parameters, necessitating the development of methods to reduce task-specific parameters more efficiently.
% 말을 끝 맺을 때, routing에서도 적절한 origin을 잡으면 효과적으로 task specific parameter를 pruning할 수 있음을 제시해야 하는데

\begin{comment}
    task별로 추가적인 specific parameter를 유지할 수 있다는 relaxation 하에서는 Router $r:\mathbb{R^d} \rightarrow \mathbb^{T}$, 일반적으로 input은 model f의 classification head 바로 전의 feature embedding $h$를 통해서 input에 대하여 dynamic하게 $\{\lambda_t\}$를 결정하게 된다. \citet{tangMergingMultiTaskModels2024}는 transformer architecture의 mlp module에 task specific knowledge가 집중되고 이것이 parameter interference를 초래한다는 관찰에서 attention module에 대해서는 Equation \ref{eqn: simple merge} 방식으로 mergeing을 하되 mlp module은 task별로 유지하는 방법을 취했다. \citet{luTwinMergingDynamicIntegration2024}는 더 나아가 $\{\tau_t\}$에 Sigular Value Decomposition을 통해서 90%의 parameter를 pruning하더라도 성능이 보존된다는 관찰로 부터 task별로 원래 model parameter의 10%만 유지하는 방법을 취했다.
    이러한 방법을 통해서 single task fintuned model들의 average 성능에 근접하게 되었으나, 두 방법 모두 $\mathcal{O}(T)$만큼의 parameter 추가적으로 보유해야만 한다는 점에서 task specific parameter를 매우 효율적으로 줄이는 방법을 고안해야만 한다.
    % 매 inference시마다,$\theta_{\text{pre}}$로 parameterized된 network $f()$를 통해서
\end{comment}

\section{Methodology}

\subsection{Motivations}
Unlike previous methods that handle $\{\tau_t\}$ from a fixed $\theta_{\text{pre}}$, we sought to process $\{\tau_t\}$ at a \textit{new point} to reduce parameter interference. \citet{tangParameterEfficientMultitask2024} observed that task vectors obtained via LoRA \cite{huLoRALowRankAdaptation2021} fine-tuning exhibit higher cosine similarity compared to those from full fine-tuning, which increases parameter interference. By fine-tuning task-specific LoRA parameters to be explicitly orthogonal—resulting in what they call L-LoRA—they achieved better model merging results. Inspired by this intuition, we explicitly optimized $\theta_{\text{shared}}$ to minimize the similarity among task-specific parameters $\tau'_t = \theta_t - \theta_{\text{shared}}$, ensuring that they become orthogonal to each other, by optimizing:

\begin{equation} \label{eqn: sim_min}
    \theta_{\text{shared}} = \underset{\theta_{shared}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i} \langle \tau'_{i}, \tau'_{j} \rangle_{F}
\end{equation}

where $\langle \tau'_{i}, \tau'_{j} \rangle_{F}$ denotes the Frobenius inner product between $\tau'_{i}$ and $\tau'_{j}$ (i.e., the sum of the element-wise products).

However, when we performed model merging using the obtained $\theta_{\text{shared}}$ and $\{\tau'_t\}$ via Equation \ref{eqn: simple merge} (e.g., green point), we still observed— as shown in Figure \ref{fig:rank_min}—that the model merging results using Equation \ref{eqn: simple merge} with $\theta_{\text{pre}}$ as the origin (e.g., red point) were better. We hypothesized that, as \citet{yadavTIESMergingResolvingInterference2023a} conjectured, abundant parameters cause interference. We pruned these parameters using SVD and examined the model merging results of Equation \ref{eqn: simple merge} at various rank preservation ratios, as shown in Figure \ref{fig:rank_min}. Even with this simple method, we achieved better results than the approach proposed by \citet{yadavTIESMergingResolvingInterference2023a}.

\begin{comment}
    % 여기 다시 쓰기
    $\{\tau_t\}$를 다루기 위해서 고정된 $\theta_{\text{pre}}$에서 하는 앞선 방법들과 다르게 우리는 parameter interference를 줄일 수 있는 새로운 지점에서 $\{\tau_t\}$를 가공하는 방법을 찾고자 하였다. \cite{tangParameterEfficientMultitask2024}는 LoRA \cite{huLoRALowRankAdaptation2021} finetune을 통해서 얻은 $\{\tau_t\}$가 full fine tune에서 얻은 $\{\tau_t\}$에 비해서 cosine similarity가 높고 이것이 paramter inteference를 늘린다는 점을 관찰하였고 task별 lora paramter들이 explicit하게 orthogonal해지도록 fintune을 하여 얻은 저자들이 칭하는 L-LoRA로 더 좋은 model merging 결과를 얻었다는 결과로부터 intuition을 받아서 우리는 explicit하게 $\{\tau_t\}$들이 orthogonality해지도록 task specific parameters $\tau^{'}_{t} = \theta_{t} -\theta_{shared}$간에 similiarity가 작아지도록 $\theta_{shared}$를 \begin{equation}\label{eqn: sim_min}
    \theta_{shared}^{l} = \underset{\theta^{l}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i}^{T} \langle \tau'_{i}, \tau'_{j} \rangle_{F}
    \end{equation}로 optimize하였다. where $\langle \tau'_{i}, \tau'_{j} \rangle_{F}$ denotes the Frobenius inner product between $\tau'_{i}$ and $\tau'_{j}$ (i.e., the sum of the element-wise products).  다만, 이렇게 찾아낸 $\theta_{\text{shared}}$와 $\{\tau'_t\}$을 Equation \ref{eqn: simple merge}로 model merging을 수행할 경우 (e.g., 초록색 점),  여전히 Figure \ref{fig:rank_min}에서 확인할 수 있듯이 $\theta_{\text{pre}}$를 origin으로하는 Equation \ref{eqn: simple merge}의 model merging 결과 (e.g., 빨간색 점)보다 떨어짐을 확인할 수 있었다. 우리는 이 것이 \citet{yadavTIESMergingResolvingInterference2023a}가 추측하듯이 abundant한 parameter가 interference를 초래한 것으로 추측하였고, 우리는 SVD를 통해서 abundant한 parameter를 pruning을 하였고 Figure \ref{fig:rank_min}에서 rank의 보존 비율 별로 \Equation \ref{eqn: simple merge}의 model merging 결과를 확인하였다. 이러한 단순한 방법만으로도, \citet{yadavTIESMergingResolvingInterference2023a}의 제시한 방법론에 비해서 좋은 결과를 얻을 수 있었다.
    
    % task별 lora paramter들이 explicit하게 orthogonal해지도록 fintune을 하여 얻은 저자들이 칭하는 L-LoRA로 더 좋은 model merging 결과를 얻었다는 결과로부터 intuition을 받아서

    우리는 이렇게 찾아진 weight 간에
    
    이렇게 단순하게 찾아진 MTM이 ViT-B-32의 경우에서 TiEs merging보다 좋다.

    다만 tirival solution이 존재하나 gradient step을 통해서 관찰하면 rank가 매우 줄어든다는 점이다.  매우 흥미로운 점은 
    
    In contrast,  we propose decomposing the parameters of $\{\theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T}\}$ into shared parameters, $\theta_{\text{shared}}$, and task-specific parameters, $\{\tau'_{1}, \dots, \tau'_{T}\}$. This approach effectively reduces task interference and enhances model merging performance.

    위의 관찰로부터 우리는 3가지 parameter를 recomposotion하는 방법을 제시한다.
    우리는 앞선 works들이 대체로 $\theta_{\text{pre}}$을 고정된 점으로 간주하는 것에서 벗어나, paramter interference를 줄일 수 있는 지점을 찾고자 하였다. 
    다만 최근의 연구에 있어서 실험적으로 orthogonality와 task interference의 상관 관계가 높음을 보였고 우리는
\end{comment}

\begin{comment}
    # revision -1
To address $\{\tau_t\}$, we sought to process them at a \textit{new point} that reduces parameter interference, differing from previous methods that operate from a fixed $\theta_{\text{pre}}$. \citet{tangParameterEfficientMultitask2024} observed that task vectors obtained via LoRA \cite{huLoRALowRankAdaptation2021} fine-tuning exhibit higher cosine similarity compared to those from full fine-tuning, which increases parameter interference. Therefore, we explicitly optimized $\theta_{\text{shared}}$ to minimize the similarity among task-specific parameters $\tau'_t = \theta_t - \theta_{\text{shared}}$, ensuring that they become orthogonal to each other, by optimizing:

\begin{equation} \label{eqn: sim_min}
    \theta_{\text{shared}}^{l} = \underset{\theta^{l}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i}^{T} \langle \tau'_{i}, \tau'_{j} \rangle_{F}
\end{equation}

where $\langle \tau'_{i}, \tau'_{j} \rangle_{F}$ denotes the Frobenius inner product between $\tau'_{i}$ and $\tau'_{j}$ (i.e., the sum of the element-wise products).
\end{comment}

\begin{figure}[h]
    % 일단은 너무 대충 만든 Figure 이므로 sim loss만 주었을 때 예쁘게 다시 뽑자.
    \centering
    \includegraphics[width=0.5\textwidth]{./fig/avg_is_all_you_need.png}
    \caption{Rank Minimization Example}
    \label{fig:rank_min}
\end{figure}

\begin{comment}
    # task-wise effective rank 측정 표 제시 필요
    # No, 정말 크더라
\end{comment}

% 아래 부분 부터는 우리 method를 적용하기 위한 방법론을 세세하게 작성하도록 한다.
% 여기 block이 너무 뜬금 없어서, 일단은 필요한 내용을 라면 레시피로 다 적고 레고처럼 싹싹 맞춰서 쓰도록 하자.
% \paragraph{Notations}
% % 이거 조금 뜬금 없기는 하다.
% 여기는 각 내용 설명하면서 녹여내도 될 듯하다.
% To facilitate the following discussion, we define several key notations. For layer-wise parameterization of each parameter set $\{ \theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T} \}$, we represent $\theta_i$ as $\theta_i := \{ \theta_{i}^{1}, \theta_{i}^{2}, \dots, \theta_{i}^{L} \}$. Additionally, for test-time adaptation, we assume an unlabeled test data distribution per task, denoted as $\{\mathcal{D}^{\text{test}}_{t}\}_{t=1}^{T}$, with input $x \in \mathcal{D}^{test}_t$.

\begin{comment}
    - 이후의 논의를 위해서 몇가지 notation을 정의하도록 한다.
    - 각 파라미터  $\{ \theta_{pre}, \theta_{1}, ..., \theta_{T}\}$의 layer wise한 parameterization을 하기 위해서, \theta_i := {\theta_{i}^{1}, \theta_{i}^{2}, ..., \theta_{i}^{L}}로서 정의한다.
    - test time adaptation을 위해서, unlabeled test data distribution $\{\mathcal{D}^{test}_{t} \}_{t=1}^{T}, x \in \mathcal{D}_t $을 per task를 상정한다.

\end{comment}


% 앞 문단과 너무 간극이 있는 연결 지점이다. 이 부분은 다시 한번 생각해보도록 하자.
% 내용을 갈아 엎기는 해야 되는데 일단 seed가 있어야 갈아 엎으니까 일단은 작성한다.
\subsection{ReOrigin} \label{sec: origin}
Building on the preceding observations, we propose decomposing the parameters $\{\theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T}\}$ into a new origin, $\theta_{\text{shared}}$, and task-specific parameters $\{\tau'_{1}, \dots, \tau'_{T}\}$, where each $\tau'_t := \theta_{t} - \theta_{\text{shared}}$.
\begin{comment}
    Building on the preceding observations, we propose decomposing the parameters $\{\theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T}\}$ into a new origin, $\theta_{\text{shared}}$, and task-specific parameters $\{\tau'_{1}, \dots, \tau'_{T}\}$, where each $\tau'_t := \theta_{t} - \theta_{\text{shared}}$.

    위의 관찰로부터 우리는 systemically 3개의 origin을 재구성하는 방법을 제시한다.
\end{comment}

%% 이거는 작성

\paragraph{Similiarity Minimization (SimMin)}
Equation \ref{eqn: sim_min} is convex with respect to $\theta_{\text{shared}}$ and possesses an analytic solution, with a detailed derivation provided in Section \ref{sec: sim_min_derivation}. The result is
\begin{align}
\theta_{\text{shared}} &= \frac{1}{T} \sum_{t=1}^{T} \theta_t \label{eqn:shared_solution} \\
\{\tau'_t\} &= \theta_t - \theta_{\text{shared}} \label{eqn:tau_prime}
\end{align}
In other words, $\theta_{\text{shared}}$ is simply the average of the fine-tuned weights. However, when optimizing $\theta_{\text{shared}}$ via gradient descent (GD) and observing the ranks of $\{\tau'_t\}$, as shown in Figure \ref{fig: low rank sol}, we confirmed that they converge to a low rank.
\begin{figure}[h]
    % 일단은 너무 대충 만든 Figure 이므로 sim loss만 주었을 때 예쁘게 다시 뽑자.
    \centering
    \includegraphics[width=0.5\textwidth]{./fig/avg_rank_equiv.png}
    \caption{GD steps vs Rank plot of $\{\tau'_t\}$}
    \label{fig: low rank sol}
\end{figure}
From this observation, we propose that the rank minimization loss
$$
\mathcal{L}(\theta) = \sum_{i=1}^{T} \| \theta_i - \theta \|_{*}
$$
where $\| \cdot \|_{*}$ denotes the nuclear norm (i.e., the sum of singular values), does not shift $\theta_{\text{shared}}$ to an ill-posed point. Thus, we additionally propose a method for determining the origin as follows.

\begin{comment}
Equation \ref{eqn: sim_min}은 $\theta_{shared}$에 대해서 convex하고 analytic solution이 존재하며 detailed derivation은 Section {sec: sim_min_derivation}에 있다. 결과는 \begin{align}
\theta_{\text{shared}} &= \frac{1}{n} \sum_{i=1}^{n} \theta_i \label{eqn:shared_solution} \\
\{\tau'_t\} &= \theta_t - \theta_{\text{shared}} \label{eqn:tau_prime}
\end{align}이다 즉, 매우 단순하게도 $\theta_{\text{shared}}$은 finetuned weight들의 평균이다. 다만, $\theta_{\text{shared}}$을 gradient descent (GD)를 통해서 optimize하면서 \{\tau'_t\}의 rank를 관찰할 때 Figure \ref{fig: low rank sol}와 같이 low rank로 수렴함을 확인할 수 있었고 이로부터, 우리는$\mathcal{\theta} = \sum_{i=1}^{T} \| \theta_i - \theta \|_{*}$ where $\| \cdot \|_{*}$ represent nuclear norm 로 정의된 rank minimization loss가 $\theta_{\text{shared}}$을 ill-posed point로 옮기지 않을 것이라 생각하여 origin을 지정하는 방법을 추가적으로 제시한다. 
---
Equation \ref{eqn: sim_min} is convex with respect to $\theta_{\text{shared}}$ and possesses an analytic solution, with a detailed derivation provided in Section \ref{sec: sim_min_derivation}. The solution is given by

\begin{align}
    \theta_{\text{shared}} &= \frac{1}{n} \sum_{i=1}^{n} \theta_i \label{eqn:shared_solution} \\
    \{\tau'_t\} &= \theta_t - \theta_{\text{shared}} \label{eqn:tau_prime}
\end{align}

Thus, $\theta_{\text{shared}}$ is simply the average of the fine-tuned weights. However, when optimizing $\theta_{\text{shared}}$ using gradient descent (GD), we observed that the ranks of $\{\tau'_t\}$ converge to low ranks, as illustrated in Figure \ref{fig: low rank sol}. Based on this observation, we propose that the rank minimization loss defined as

\begin{equation}
    \mathcal{L} = \sum_{i=1}^{T} \| \theta_i - \theta \|_{*}
\end{equation}

where $\| \cdot \|_{*}$ denotes the nuclear norm, prevents $\theta_{\text{shared}}$ from moving to an ill-posed point. Consequently, we additionally propose a method to specify the origin.


\end{comment}

\begin{comment}
    
\end{comment}

% gradient update trajectory가 유사하다는 점에
% 여기에서 위의 식이 implicit하게 task speicific parameter가 low-rank 구조로 감을 실험적으로 보인다. 따라서 rank minimization loss가 SimMin loss와 confilict를 유발하지 않을 것이고 우리는 이때, rank minimization loss를 또한 추가하여 explicit하게 low-rank 구조를 promote하고자 한다. 
% proposition을 Equation이 단순한기 때문에 결과적으로 analytic solution이 존재한다는 것을 제시하고 식의 전개는 appendix에 있다. 
\begin{comment}
    이 부분에서 proposition으로 실은 이 equation은 analytic solution이 존재한다는 것을 제시해야 하고 간단하게 appendix로 뺄 필요가 있다.
    Equation \ref{eqn: sim_min}은 $\theta_{shared}$에 대해서 convex하고 analytic solution이 존재한다. detailed derivation은 Section {sec: sim_min_derivation}를 참조하도록한다. 


    Building on the observation that task vectors across different tasks are nearly orthogonal, which suggests the possibility of task arithmetic \cite{ilharcoEditingModelsTask2023}, we optimize $\theta_{\text{shared}}$ according to Equation \ref{eqn: sim_min} to minimize the similarity between task-specific parameters, defined as $\tau'_{t} = \theta_{t} - \theta_{\text{shared}}$.
    다른 task간의 task vector가 거의 orthogonal하다는 사실과 이것에 의해서 task arithmetic이 가능할 수 도 있다는 추측으로부터 \cite{ilharcoEditingModelsTask2023}, task specific parameters $\tau^{'}_{t} = \theta_{t} -\theta_{shared}$간에 similiarity가 작아지도록  $\theta_{shared}$을 Equation \ref{eqn: sim_min}으로 optimize하였다. 
    To mitigate task interference, we aim to find a shared parameter $\theta_{shared}$ that reduces the similarity among task-specific parameters, defined as $\tau'_{t} = \theta_{t} - \theta_{shared}$ by optimizing the Equation \ref{eqn: sim_min}.
    % 뭔가 아전인수 격으로 orthogonal한게 좋다고 썼는데, trivial한 근거가 있어야 한다. 찾음
    % objective가 왜 이것이 되어야 하는가? 여기에 논리가 없다.
\end{comment}

\begin{comment}
    
\end{comment}

% \begin{equation} \label{eqn: sim_min}
%     \theta_{shared}^{l} = \underset{\theta^{l}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i}^{T} \langle \tau'_{i}, \tau'_{j} \rangle_{F}
% \end{equation}

% Frobenius inner product에 대해서 설명할 필요가 있다. 1줄 정도

% Equation \ref{eqn: sim_min} has an analytic solution, given by $\theta_{\text{shared}} = \frac{1}{T} \sum_{t=1}^{T} \theta_t$, which represents the average of the task weights. However, using this $\theta_{\text{shared}}$ and $\{\tau'_{t}\}$ to perform model merging as $\theta_{*} = \theta_{\text{shared}} + \sum_{t} \lambda_{t} \tau'_{t}$ results in significant task interference, leading to reduced performance. Empirical analysis revealed that the effective rank of matrix components within $\{\tau'_{t}\}$, such as the weights of MLP modules, is notably low. Based on the assumption that non-dominant eigenvectors contribute to task interference, we explicitly pruned the rank of these matrix components in $\{\tau'_{t}\}$. As demonstrated in Figure \ref{fig:rank_min}, ensuring that task-specific parameters maintain an appropriate rank effectively reduces task interference.
% \paragraph{Rank Minimization (RankMin)}
% 여기서 Nuclear Norm에 대해서 간략하게 설명한다.
% 여기는 corrlation이 높음이 실험적으로 많이 제시되었는데, 
% 여기서 similiarity minimization이 rank minimization과 high correlation이 있으며, 또한 explicit하게 task specific parameter에서 task interference를 줄이면서도 task speicific knowledge는 유지 하기에 이 objective를 기반으로 하면 매우매우 적은 task specific parameter로도 router를 구성하고 upper bound에 근접한 성능을 낼 수 있음을 서술하자
\paragraph{SimMin with Rank Minimization (SimRankMin)} \label{par: simrank}
\begin{align}
    \theta_{\text{shared}} &= \underset{\theta_{shared}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i} \langle \tau'_{i}, \tau'_{j} \rangle_{F} + k\sum_{i=1}^{T} \|\tau'_t \|_{*} \label{eqn:simrankmin} \\
    \{\tau'_t\} &= \theta_t - \theta_{\text{shared}} \label{eqn:tau_prime_new}
\end{align}
Although $\theta_{\text{shared}}$ cannot be determined solely through an analytic solution, the rank minimization loss term ensures that the principal components of $\{\tau'_t\}$ explicitly capture task-specific information, thereby allowing the pruning of most parameters.

\begin{comment}
    단순하게 analytic solution으로 $\theta_{\text{shared}}$을 구할 수는 없으나, rank minimization loss term에 의해서 $\{\tau'_t\}$의 prncipal components에 explicit하게 task speicifc 정보가 집중된다. (즉, 대부분의 parameter를 pruning할 수 있다.) 이렇게 구한 $\theta_{\text{shared}}$와 $\{\tau'_t\}$을 이용하여
\end{comment}

\subsection{Task Vector Processing} \label{sec: task_vector}
Through the previous discussion, we observed that changing the origin can help reduce task interference. However, since the optimal preserved rank for achieving peak performance may vary by task, as shown in Figure \ref{fig:rank_min_taskwise} in Appendix \ref{sec: TDO rank}, we propose an adaptive approach to determine this rank at test time, which we term \textit{AdaRank}.
\paragraph{Adaptive Rank Determination (AdaRank)} Using the method outlined in Section \ref{sec: origin}, we first determine $\theta_{\text{shared}}$ and $\{\tau'_t\}$. Then, we decompose $\{\tau'_t\}$ via SVD into $\{U_t, s_t, V_t\}$ and apply a learnable binary mask $M$ to $\{s_t\}$ using the Straight Through Estimator (STE) \cite{bengioEstimatingPropagatingGradients2013} (Torch-style \cite{paszkePyTorchImperativeStyle2019} implementation in Appendix Listing \ref{lst:STE}). This masking allows each task vector to be represented as $\tau'_t := U_t \cdot \text{diag}(M_t \circ s_t) \cdot V_t^T$, enabling the selection of an optimal rank per task, where $\circ$ denotes the element-wise product.

Additionally, as noted by \citet{yangAdaMergingAdaptiveModel2024}, the performance of MTM is highly sensitive to the coefficients $\{\lambda_t\}$ of $\{\tau'_t\}$, so we make these coefficients learnable. We update $\{M_t\}$ and $\{\lambda_t\}$ through test-time adaptation \cite{wangTentFullyTesttime2021} using Equation \ref{eqn: entropy} as the loss function. This approach allows us to obtain the optimal merged model parameters for the test data distribution $\{\mathcal{D}_{t}^{\text{test}}\}$ as $\theta_{*} := \theta_{\text{shared}} + \sum_t \lambda_t U_t \cdot \text{diag}(M_t \circ s_t) \cdot V_t^T$.
% adarank가 생각보다 말도 안되게 좋은 기술이다. paramter interference를 줄이는 데도 도움이 되고, 매우 trivial 한데 masking된 eigen vector를 pruning하면 task speicific parameter를 더 줄일 수 있다.
% explicit하게 rank를 자르고 시작한다는 진술을 더 적어줄 필요가 있다.
\begin{comment}
    Through the previous discussion, we observed that changing the origin can help reduce task interference. However, since the optimal preserved rank for achieving peak performance vary by task, Appendix \ref{sec: TDO rank}의 Figure \ref{fig:rank_min_taskwise}에서 확인할 수 있다.

    % ada rank를 강조해야 한다. 매우 중요한 기술이다.
    앞선 논의를 통해서 우리는 origin을 바꾸는 것이 task inteference를 줄일 수 있음을 관찰하였다. 그러나 $\{tau'_t\}$에 대하여 task별 최적의 성능이 나올 수 있는 최적의 preserverd rank가 다를 수 있다는 점 떄문에 우리는 test time에 이를 adaptive하게 결정할 수 있는 방법을 제시하며 이를 AdaRank라 칭하고자 한다. Section \ref{sec: origin}에 제시된 방법을 통해서 $\theta_{shared}$와 $\{tau'_t\}$을 결정하고 $\{tau'_t\}$ SVD로 $\{U_t, s_t, V_t\}$로 decompose하고 $\{s_t\}$에 Straight Through Estimator (STE) \cite{bengioEstimatingPropagatingGradients2013}을 이용한 learnable 한 binary mask M (torch style 구현은 Apeendix의 Code \ref{lst:STE} 참조)을 task vector $tau'_t := U_t \cdot diag(M_t \circ s_t) \cdot V^{T}_{t}$에 적용하여, task별로 최적의 rank를 고를 수 있도록 한다. 또한, \citet{yangAdaMergingAdaptiveModel2024}가 진술 했듯이 $\{tau'_t\}$의coefficient $\{\lambda_t\}$에 따라 MTM의 성능이 크게 변화하므로 learnable하도록 한다. 이후 Equation \ref{eqn: entropy}를 loss로 하여 test time adaptaion \cite{wangTentFullyTesttime2021}을 통해서 $\{M_t\}, \{lambda_t\}$를 update한다. 이렇게 test data distribution $\{\mathcal{D}_{t}^{\text{test}}\}$에 대한 최적의 merged model parameter $\theta_{*} := \theta_{shared} + \sum_t \lambda_t U_t \cdot diag(M \circ s_t) V_t^T $ 구할 수 있다. 여기서 $\circ$는 element-wise product를 의미한다.
\end{comment}


% 우리는 이 방법을 통해서 task


\begin{comment}
    이때, Equation \ref{eqn: sim_min}은 analytic solution이 존재하며 $\theta_{shared} = 1/T \sum_{t=1}^{T} \theta_t$이고 이는 task weight들의 평균이다. 하지만, 이렇게 얻은 $\theta_{shared}, \{\tau'_{t}\}$를 이용하여 $\theta_{*} = \theta_{shared} + \sum_{t} \lambda_{t} \{\tau'_{t}\}$로 model merging을 수행할 경우, 상당한 task interference로 낮은 성능을 낸다. 우리는 실험적으로 $\{tau'_{t} \}$중에서 matrix component들의 effective rank가 매우 낮다는 점을 확인하였고, 따라서 non-dominant eigenvectors가 task interference를 초래할 것이라는 가정하에, $\{\tau'_{t}\}$에서 matrix component들(예를 들어, mlp module의 weight 같은)의 rank를 explicit하게 pruning을 하였고 Figure \ref{fig:rank_min}로부터 task specific parmeter가 적절한 rank를 지니는 것이 task interference를 줄이는데 효과적임을 확인하였다. 
    $\theta_{*} = \theta_{shared} + \sum_i^{T} \lambda_{i}^{l} \tau_^{'}_{t} $
    % effective 낮다는 점은 table로 보여야 할지?
    % 아녀 effective rank가 낮은거랑, non-dominant eigenvectors가 task interference를 초래할 것이 어떻게 연결되는가?
    % 적절한 rank를 어떻게 결정해야 하는데...?
\end{comment}

\subsection{Routing}  % 적절한 용어 선정 필요함
% 여긴 0.5%p 1% 정도의 rank에서의 성능을 관찰해야만 서술할 수 있을 듯 하다.
As previously mentioned, efficient reduction of task-specific parameters through routing is crucial. First, we determine $\theta_{\text{shared}}$ and $\{\tau'_t\}$ following \textit{SimRankMin}. Next, we apply \textit{AdaRank} to $\{\tau'_t\}$, yielding $\tau'_t := U_t \cdot \text{diag}(M_t \circ s_t) \cdot V_t^T$. Although Section \ref{sec: task_vector} uses masking to mitigate parameter interference, it also naturally reduces task-specific parameters.

Following previous work \cite{tangMergingMultiTaskModels2024, luTwinMergingDynamicIntegration2024}, the merged model parameters are dynamically determined for input $x$ as $\theta_* = \theta_{\text{shared}} + \sum_{t} \lambda_{t} U_t \cdot \text{diag}(M_t \circ s_t) \cdot V_t^T$, where $\{\lambda_{t}\} = \text{softmax}(r(h(x)))$. Here, $h(x)$ is the feature embedding $\in \mathbb{R}^{d}$ from the layer immediately preceding the classifier head in $f(x; \theta_{\text{shared}})$, and $r$ is a shallow MLP module, $r: \mathbb{R}^{d} \rightarrow \mathbb{R}^{T}$. Finally, we update $\{M_t\}$ and the router $r$ at test time through test-time adaptation \cite{wangTentFullyTesttime2021}, using Equation \ref{eqn: entropy} as the loss.


\begin{comment}
    이전 work들과 근사한 성능을 내기 위한 test time adaptation을 수행한다.
    % TVP와 크게 다른 서술 방향을 제시할 필요는 없을 것이다. 20241108 05:30 현재 1%p rank만으로도 avg entropy loss가 16%p rank를 사용한 것들과 비슷한 값을 보이고 있다.
    % 4%p의 preserved rank ratio 만으로도 상당히 safe하다. previous sota인 twin merges는 10%p의 rank를 사용했음.
    % 여기 section에서 저랭크 구조로 지식을 압축하였음을 강조해서 서술해주자.
    앞서 언급하였듯이 routing은 task specific parameter 효율적으로 줄이는 것이 매우 중요하다. 먼저 \textit{SimRankMin}로 $\theta_{shared}$와 $\{tau'_t\}$를 결정한다. 이후 $\{tau'_t\}$에 AdaRank를 적용하여 $tau'_t := U_t \cdot diag(M_t \circ s_t) \cdot V^{T}_{t}$가 되도록한다. Section \ref{sec: task_vector}에서는 parameter interference를 경감하고자 사용하였으나, 자명하게도 masking은 task specific parameter를 줄일 수 있다. 이후 앞선 work들 \cite{tangMergingMultiTaskModels2024, luTwinMergingDynamicIntegration2024}을 따라 merged model parameter는 식 $\theta_* = \theta_{shared} + \sum_{t} \lambda_{t} U_t \cdot diag(M_t \circ s_t) \cdot V^{T}_{t}, \{\lambda_{t}\} = softmax(r(h(x)))$으로 입력 $x$에 따라 dynamic하게 결정된다. 여기서 h(x)는 $f(x;\theta_{shared})$의 classifier head 바로 앞의 feature embedding $\in \mathbb{R}^{d}$를 r은 shallow mlp module로 $r:\mathbb^{d} \rgihtarrow \mathbb^{T}\$이다.이후, Equation \ref{eqn: entropy}를 loss로 하여 test time adaptaion \cite{wangTentFullyTesttime2021}으로 $\{M_t\}$와 router $r$을 update한다.
     
\end{comment}

%%% Algorithms
% 넣으려고 생각해보니 분량이 너무 많아져서 일단은 보류

% \begin{algorithm}
%     \caption{Adaptive Merging with SimMin}
%     \label{alg:ada_sim}
%     \begin{algorithmic}[1]
%     \INPUT $\{ \theta_{pre}, \theta_{1}, ..., \theta_{T} \}$, $\{ \mathcal{D}^{test}_{t} \}_{t=1}^{T}$, condition
%     \IF{condition}
%         \OUTPUT $\theta_{*}$ using method 1
%     \ELSE
%         \OUTPUT $\theta_{*}$ using method 2
%     \ENDIF
%     \STATE Initialize $\theta_{shared}, \{ \{ \lambda_{t}^{l} \}_{l} \}_t$

%     \COMMENTTRIANGLE{ReParameterization}
%     \IF{condition}
%         \STATE Perform reparameterization method 1
%     \ELSE
%         \STATE Perform reparameterization method 2
%     \ENDIF

%     \COMMENTTRIANGLE{Test Time Adaptation}
%     \STATE Merge models: $\theta_{*} = \theta_{shared} + \sum_{i=1}^{T} \lambda_{i}^{l} \tau_{t}^{'}$
%     \STATE Perform test time adaptation using $\theta_{*}$ and $\mathcal{D}_{t}$
%     \RETURN $\theta_{*}$
%     \end{algorithmic}
% \end{algorithm}

\begin{comment}
    to sum up, ours method can be simply represmnt as algorith \ref{alg: ours_model_fusion}
\end{comment}

\begin{comment}
    약간의 task specific parameter와 2번의 inference가 가능하다는 relaxation에서 
\end{comment}


\begin{comment}
to sum up, 우리의 전반적인 알고리즘은 다음과 같이 구성될 수 있다.
\end{comment}



\begin{comment}
    글의 전체 전개 순서를 다음과 같이 가져가고 싶다.
    - 문제 정의와 기존의 work들의 방법론

    - rank minimization, similiarity minimization




\end{comment}


\section{Appendix}

\subsection{Derivation on Analytic Solution of Equation \ref{eqn: sim_min}} \label{sec: sim_min_derivation}
% 여기도 거의 GPT가 해준거니까 직접 유도해볼 필요 있다.
Let us define:
\[
\tau_i := \theta_i - \theta_{\text{shared}}
\]
where our objective is to minimize the following function:
\[
\min_{\theta_{\text{shared}}} \sum_i \sum_{j < i} \langle \tau_i^T, \tau_j \rangle_F
\]
where \(\langle A, B \rangle_F = \text{Tr}(A^T B)\) denotes the Frobenius inner product.

First, we expand the objective function in terms of \( \theta_i \) and \( \theta_{\text{shared}} \):
\begin{align*}
L(\theta_{\text{shared}}) &= \sum_i \sum_{j < i} \langle \tau_i^T, \tau_j \rangle_F \\
&= \sum_i \sum_{j < i} \text{Tr}\left( \tau_i^T \tau_j \right) \\
&= \sum_i \sum_{j < i} \text{Tr}\left( (\theta_i - \theta_{\text{shared}})^T (\theta_j - \theta_{\text{shared}}) \right).
\end{align*}

We differentiate \(L(\theta_{\text{shared}})\) with respect to \( \theta_{\text{shared}} \) and set it to zero:
\[
\frac{\partial L}{\partial \theta_{\text{shared}}} = \sum_i \sum_{j < i} \left( - \theta_i - \theta_j + 2 \theta_{\text{shared}} \right).
\]

Let \( n \) be the number of \(\theta_i\). Then we can simplify the gradient as follows:
\[
\frac{\partial L}{\partial \theta_{\text{shared}}} = -2 (n - 1) \sum_{i} \theta_i + n(n - 1) \theta_{\text{shared}}.
\]

Setting the gradient to zero:
\[
-2 (n - 1) \sum_{i} \theta_i + n(n - 1) \theta_{\text{shared}} = 0.
\]

Dividing by \(n - 1\) on both sides:
\[
-2 \sum_{i} \theta_i + n \theta_{\text{shared}} = 0.
\]

Rearranging gives:
\[
\theta_{\text{shared}} = \frac{1}{n} \sum_{i=1}^{n} \theta_i.
\]

The analytical solution to the objective function is:
\[
\theta_{\text{shared}} = \frac{1}{n} \sum_{i=1}^{n} \theta_i.
\]

\subsection{Task-wise Different Optimal Preserved Rank} \label{sec: TDO rank}
\begin{figure}[h]
    % 일단은 너무 대충 만든 Figure 이므로 sim loss만 주었을 때 예쁘게 다시 뽑자.
    \centering
    \includegraphics[width=0.5\textwidth]{./fig/avg_is_all_you_ned_taskwise.png}
    \caption{Rank Minimization Example}
    \label{fig:rank_min_taskwise}
\end{figure}

\subsection{Learnable Binary Mask M using STE}
% 나중에 예쁘게 고치자.
% 여기 표현 좀 더 정교하게 바꿔야 겠네 그냥 top k sigular value라고 하면 어디를 지칭하는지 모르잖아.
\begin{lstlisting}[language=Python, caption={binary mask M implemeted by STE}, label={lst:STE}, basicstyle=\footnotesize]
    A = torch.ones_like(s_t) * -1.0
    A[:k] = 1  # to select top k singular values
    A = torch.Parameter(A) 
    M = torch.sigmoid(A)
    masked_s = M * S + \
    ((M > 0.5) * S - M * S).detach()
\end{lstlisting}
    

==> sec/backups/2_method_1112.tex <==
\section{Method}

\subsection{Problem Setup}

\paragraph{Model Merging}
Model merging aims to create a general model for multiple tasks by combining the parameters of individually trained models without additional training.
We adopt the standard setting~\cite{matena2022merging} where all models to be merged share the same architecture $f(x; \theta)$ and are fine-tuned from a common initialization $\theta_{\text{pre}}$.
Let $\theta_t$ denote the parameters of the model trained for task $t$, and let $\mathcal{L}_t(\theta)$ represent the corresponding loss function.
Given parameters $\theta_1, \dots, \theta_T$ from $T$ task-specific models, our objective is to find $\theta_*$ such that $\mathcal{L}_t(\theta_*) \approx \mathcal{L}_t(\theta_t)$ for each task $t = 1, \dots, T$.
Importantly, we have access only to the trained parameters, not the data used for training the models.
A straightforward baseline is simple averaging: $\theta_* = \frac{1}{T}\sum_{i=1}^T \theta_t$.


\paragraph{Task Vectors}
We leverage the concept of \emph{task vectors} as proposed in the task arithmetic framework~\cite{ilharco2023editing}.
A task vector represents the direction in parameter space from a chosen origin $\theta_0$ to the fine-tuned parameters for each task: $\tau_t = \theta_t - \theta_0$.
We consider only the \emph{weight} parameters to construct task vectors, which are represented as real matrices.
We denote by $\theta^{(l)} \in \mathbb{R}^{m_l \times n_l}$ the weight matrix of the $l$-th layer of the model $f(x; \theta)$.
The parameters of the merged model are then computed by adding the task vectors:
\begin{equation}
    \theta_*^{(l)} = \theta_0^{(l)} + \lambda \sum_{t=1}^T (\theta_t^{(l)} - \theta_0^{(l)}),
    \label{eqn:task_arithmetic}
\end{equation}
where $\lambda$ is a hyper-parameter controlling the contribution of the task vectors.
The remaining parameters such as bias and layer normalization are merged by simple averaging.
Setting the pre-trained parameters as the origin ($\theta_0 = \theta_\text{pre}$) in Equation~\eqref{eqn:task_arithmetic} has proven effective for model merging~\cite{ilharco2023editing}.
However, fixing the origin at the pre-trained parameters can lead to suboptimal performance due to conflict between task vectors.
In the next section, we propose an alternative task vector formulation by \emph{re-originating} them to mitigate these conflicts.


\subsection{ReOrigin}
In this section, we propose a training-free model merging approach based on task arithmetic, called ReOrigin.
The overall pipeline is detailed in Algorithm~\ref{alg:reorigin}.
The key idea is to \emph{re-originate} the task vectors to alleviate conflicts (Section~\ref{sec:reorigin_operations}).
Using the adjusted task vectors, we perform task arithmetic to merge the models, with the option to incorporate complementary techniques like test-time adaptation (Section~\ref{sec:reorigin_pipeline}).


\subsubsection{Moving the Origin of Task Vectors}
\label{sec:reorigin_operations}
We observe that conflicts between task vectors arise due to fixing the \emph{origin} to the pre-trained parameters $\theta_{\text{pre}}$.
Since there is no guarantee that the vectors originating from $\theta_{\text{pre}}$ do not interfere with each other, we suggest moving the origin of the task vectors to reduce the conflicts.
We explore two objectives for re-originating the task vectors.


\paragraph{ReOrigin via Rank Minimization (RankMin)}
This objective aims to reduce the intrinsic rank of the task vectors.
Inspired by the success of low-rank adaptation (LoRA)\cite{hu2022lora} in fine-tuning, we propose to move the origin such that the task vectors become low-rank updates from the origin: \begin{equation}
    \theta_\text{RankMin}^{(l)} = \underset{\theta^{(l)}}{\text{argmin}} \sum_{t=1}^T \|\theta_t^{(l)} - \theta^{(l)}\|_*,
    \label{eqn:reorigin_rankmin}
\end{equation}
where $\| \cdot \|_*$ denotes the nuclear norm (\emph{i.e.,} the sum of the singular values).
By adjusting the origin, this objective compresses task vectors into lower-dimensional subspaces, which mitigates interference.
For example, by approximating task vectors as low-rank matrices, we reduce the overlap between their principal directions, which helps to minimize conflicts in the high-dimensional weight space.
We revisit this intuition later in this section with empirical results.

\paragraph{ReOrigin via Similarity Minimization (SimMin)}
We also propose an objective that explicitly reduces interference between task vectors.
Motivated by the observation from task arithmetic that task vectors are typically close to orthogonal~\cite{ilharco2023editing}, we find the origin $\theta_{\text{SimMin}}$ that minimizes the sum of pairwise similarities between task vectors: 
\begin{equation}
    \theta_\text{SimMin}^{(l)} = \underset{\theta^{(l)}}{\text{argmin}} \sum_{t=1}^T \sum_{t^\prime < t} \langle \theta_t^{(l)} - \theta^{(l)}, \theta_{t^\prime}^{(l)} - \theta^{(l)} \rangle_F,
    \label{eqn:reorigin_simmin}
\end{equation}
where $\langle \cdot, \cdot \rangle_F$ denotes the Frobenius inner product (\emph{i.e.}, the sum of the element-wise products).
This objective reduces conflicts by promoting orthogonality among task vectors.
Note that Equation~\eqref{eqn:reorigin_simmin} has an analytic solution: $\theta_\text{SimMin}^{(l)} = \frac{1}{T} \sum_{t=1}^T \theta_t^{(l)}$ (see Appendix for derivation).

To gain deeper insight into this objective, we expand it using singular value decomposition (SVD). 
Let $\theta_t^{(l)} - \theta^{(l)} = \sum_{i=1}^n \sigma_i \mathbf{u}_i \mathbf{v}_i^\top$ and $\theta_{t^\prime}^{(l)} - \theta^{(l)} = \sum_{j=1}^n \sigma_j^\prime \mathbf{u}_j^\prime {\mathbf{v}_j^\prime}^\top$ be the SVDs of the task vectors.
Using the bilinearity of the inner product, the objective can be expressed as:
\begin{equation}
    \langle \theta_t^{(l)} - \theta^{(l)}, \theta_{t^\prime}^{(l)} - \theta^{(l)} \rangle_F
    = \sum_{i=1}^n \sum_{j=1}^n \sigma_i \sigma_j
    \langle \mathbf{u}_i \mathbf{v}_i^\top, \mathbf{u}_j^\prime {\mathbf{v}_j^\prime}^\top \rangle_F.
    \label{eqn:simmin_svd}
\end{equation}
This expansion shows that the objective minimizes the sum of the similarities between the basis matrices of the task vectors, weighted by the corresponding singular values.
As a result, this objective mainly focuses on disentangling the principal directions of the task vectors that have large singular values, effectively reducing interference among them, while de-emphasizing directions associated with smaller singular values (\emph{i.e.,} noise).

\paragraph{Relationship between RankMin and SimMin}
Interestingly, minimizing the nuclear norm of the task vectors not only reduces their intrinsic ranks but also tends to decrease the Frobenius inner product between them, effectively making them more orthogonal (see Figure~\ref{fig:training_curve}).
Conversely, minimizing the pairwise similarities as in Equation~\eqref{eqn:reorigin_rankmin} inherently compresses the task vectors into lower-rank representations.

\begin{figure}[t]
    \centering
    % 첫 번째 서브 그림
    \begin{subfigure}[b]{0.49\linewidth} % 너비를 설정
        \centering
        \includegraphics[width=\linewidth]{fig/training_curve:NN.png}
        % \caption{First subfigure caption} % 첫 번째 그림 캡션
        % \label{fig:training_curve:NN}
    \end{subfigure}
    \hfill
    % 두 번째 서브 그림
    \begin{subfigure}[b]{0.49\linewidth} % 너비를 설정
        \centering
        \includegraphics[width=\linewidth]{fig/training_curve:FIP.png}
        % \caption{Second subfigure caption} % 두 번째 그림 캡션
        % \label{fig:training_curve:FIP}
    \end{subfigure}
    \caption{\textbf{The two objective terms update each other in a complementary manner.} The left plot illustrates the Nuclear Norm (NN), while the right plot depicts the Frobenius Inner Product (FIP) across gradient steps. Optimizing solely the FIP objective leads to a reduction in NN as well, as evidenced by the orange curve on the left, and vice versa.} % 전체 그림 캡션
    \label{fig:training_curve}
\end{figure}
\begin{comment}
\textbf{two objetive term이 서로를 complementary하게 update한다.} gradient step별로 왼쪽은 Nuclear Norm (NN)을 오른쪽은 Frobenius Inner Product (FIP)을 측정한 것으로, FIP objective만으로도 NN가 줄어듦을 왼쪽의 주황색 curve에서 확인할 수 있고 NN ojbective만으로도 FID가 줄어듦을 오른쪽의 파란색 curve에서 확인할 수 있다.   
\end{comment}

\subsubsection{Model Merging with ReOrigin}
\label{sec:reorigin_pipeline}

After finding the origin via the ReOrigin objectives defined in Section~\ref{sec:reorigin_operations}, we perform task arithmetic (Equation~\eqref{eqn:task_arithmetic}) using the re-originated task vectors to merge the models.

\paragraph{Rank Pruning of Task Vectors}
As discussed in Section~\ref{sec:reorigin_operations}, both methods reduce the intrinsic rank of the task vectors, compressing them into low-dimensional subspaces spanned by principal directions with large singular values.
This concentrates most of the task-specific knowledge in the principal directions, leaving others as noise.
Based on this property, we explicitly prune the rank of task vectors before performing task arithmetic using Equation~\eqref{eqn:task_arithmetic}.
In Figure~\ref{fig:perf_on_ranks}, 
we plot the model merging performance with varying pruned ranks.
We observe that SimMin performs worse at higher ranks and shows the best performance at lower ranks.
While RankMin is relatively less sensitive to rank pruning, it also achieves the best performance at lower ranks.
Therefore, we consider the rank pruning ratio as an additional hyperparameter, along with the coefficient $\lambda$ in Equation~\eqref{eqn:task_arithmetic}.
Notably, the optimal rank pruning ratio remains consistent across different experiments.
In our experiments, retaining approximately 8\% of the rank yields stable performance across different settings.

\paragraph{Test-Time Adaptation}
Our framework can be naturally combined with test-time adaptation techniques~\cite{yang2024adamerging,tang2024merging,lu2024twin} that exploit test data to improve model merging.
For example, AdaMerging~\cite{yang2024adamerging} replaces the global coefficient $\lambda$ for task vectors with task-wise and layer-wise coefficients as follows:
\begin{equation}
    \theta_*^{(l)} = \theta_0^{(l)} + \sum_{t=1}^T \lambda_t^{(l)} (\theta_t^{(l)} - \theta_0^{(l)}),
\end{equation}
 where the coefficients $\lambda_t^{(l)}$ are learned by minimizing the Shannon entropy on test data.
 When we allow maintaining a small number of task-specific parameters, we can dynamically compute the merging coefficients using a router network that is also trained by minimizing the entropy on test data~\cite{tang2024merging,lu2024twin}.
 Since these approaches are independent of $\theta_0$, we also explore whether ReOrigin remains beneficial when combined with test-time adaptation techniques.

\begin{algorithm}[t]
\caption{ReOrigin: Model Merging via Re-Originating Task Vectors}
\label{alg:reorigin}
\begin{algorithmic}[1]
\REQUIRE Fine-tuned model parameters $\{\theta_t\}_{t=1}^T$, rank pruning ratio $r$, merging coefficient $\lambda$, (if fixed), test data $\mathcal{D}_{\text{test}}$ (optional)
\ENSURE Merged model parameters $\theta_*$

\STATE \textbf{Choose} ReOrigin objective: RankMin or SimMin

\COMMENTTRIANGLE{Re-originate task vectors}
\IF{RankMin}
    \STATE Compute origin $\theta_0$ by solving:
    \begin{equation*}
        \theta_0^{(l)} = \arg\min_{\theta^{(l)}} \sum_{t=1}^T \| \theta_t^{(l)} - \theta^{(l)} \|_*
    \end{equation*}
\ELSIF{SimMin}
    \STATE Compute origin $\theta_0$ as the average of parameters:
    \begin{equation*}
        \theta_0^{(l)} = \frac{1}{T} \sum_{t=1}^T \theta_t^{(l)}
    \end{equation*}
\ENDIF

\STATE \textbf{Compute} task vectors for weight parameters:
\begin{equation*}
    \tau_t^{(l)} = \theta_t^{(l)} - \theta_0^{(l)} \quad \text{for } t = 1, \dots, T
\end{equation*}

\COMMENTTRIANGLE{Rank Pruning of task vectors}
\FOR{each layer $l$ and task $t$}
    \STATE Perform SVD: $\tau_t^{(l)} = U_t^{(l)} \Sigma_t^{(l)} {V_t^{(l)}}^\top$
    \STATE Compute the pruning rank $k = \lceil r \times \text{rank}(\tau_t^{(l)}) \rceil$
    \STATE Reconstruct pruned task vector:
    \begin{equation*}
        \tau_t^{(l)} \leftarrow U_t^{(l)}[:,1\!:\!k] \, \Sigma_t^{(l)}[1\!:\!k,1\!:\!k] \, {V_t^{(l)}[:,1\!:\!k]}^\top
    \end{equation*}
\ENDFOR

\COMMENTTRIANGLE{Task Arithmetic}
\IF{Test-Time Adaptation is enabled}
    \STATE Adjust merging coefficients $\lambda_t^{(l)}$ using test data $\mathcal{D}_{\text{test}}$
\ELSE
    \STATE Set $\lambda_t^{(l)} = \lambda$, \quad $\forall t, l$
\ENDIF

\STATE \textbf{Merge} models using task arithmetic:
\begin{equation*}
    \theta_*^{(l)} = \theta_0^{(l)} + \sum_{t=1}^T \lambda_t^{(l)} \tau_t^{(l)}
\end{equation*}

\STATE \RETURN Merged model parameters $\theta_*$
\end{algorithmic}
\end{algorithm}


==> sec/backups/2_method_1114.tex <==
\section{Revisiting Weight Averaging}
\label{sec:method}

In this section, we revisit the weight averaging in perspective of task vectors.
First, we empirically show that the weight average $\theta_\text{avg}$ serves as a good initialization for defining task vectors with low-rank approximations (Section~\ref{sec:intriguing_properties}).
Then we provide an in-depth analysis on the intriguing properties (Section~\ref{sec:analysis}).
Based on these, we propose a novel model merging approach by inducing task vectors from the weight average.


\subsection{Intriguing Properties of Weight Averaging}
\label{sec:intriguing_properties}
We begin by showing that the weight averaging in Eq.~\eqref{eqn:weight_averaging} can be rewritten in the form of task arithmetic in Eq.~\eqref{eqn:task_arithmetic} as follow:
% By redefining the task vectors in such a way that they point from the weight average $\theta_\text{avg}$ rather than the initialization $\theta_\text{pre}$, the corresponding task arithmetic becomes:
% By redefining the task vectors relative to the averaged weights rather than the pre-trained weights, it yields the following form:
\begin{equation}
    \theta_\text{TA-avg} = \theta_\text{avg} + \lambda \sum_{t=1}^T (\theta_t - \theta_\text{avg}),
    \label{eqn:weight_averaging_arithmetic}
\end{equation}
where $\theta_\text{TA-avg} = \theta_\text{avg}$ always holds regardless of $\lambda$.
% With this perspective, the weight average $\theta_\text{avg}$ is \emph{itself} the result of task arithmetic by posing $\theta_\text{avg}$ as an initial point for the vectors.
Eq.~\eqref{eqn:weight_averaging_arithmetic} provides a useful insight to understand weight averaging: the weight average $\theta_\text{avg}$ is \emph{itself} the result of task arithmetic by posing $\theta_\text{avg}$ as an initial point for the vectors.
Considering the inferior performance of weight averaging over task arithmetic, it may also seem to suggest that $\theta_\text{avg}$ is a bad initial point for defining task vectors than $\theta_\text{pre}$.

% However, the situation dramatically changes when we apply the low-rank approximation on the redefined task vectors $\theta_t - \theta_\text{avg}$.
However, we observe an intriguing trend when we apply the low-rank approximation on the redefined task vectors $\theta_t - \theta_\text{avg}$.
% Specifically, we consider \emph{matrix} parameters in intermediate layers of the model (\emph{e.g.,} weight matrices in MLPs, projection matrices in attention layers).
% Suppose the model consists of $L$ layers with matrix parameters and let $\theta^l \in \mathbb{R}^{m \times n}$ be the matrix within $\theta$ at $l$-th layer of rank $r$.
Suppose the model consists of $L$ layers and let $\theta^l \in \mathbb{R}^{m \times n}$ be the weight matrix at $l$-th layer of rank $r$.
Then we apply the arithmetic defined in Eq.~\eqref{eqn:weight_averaging_arithmetic} layer-wise, with low-rank approximation on the task vectors as follows: %\footnote{We consider matrix components of parameters such as weight matrices in MLP and project matrices in attention layers, while non-matrix components such as bias are set to weight averaging.}:
\begin{equation}
    \theta_*^l = \theta_\text{avg}^l + \lambda \sum_{t=1}^T \text{SVD}_k(\theta_t^l - \theta_\text{avg}^l), \quad \forall~ l \le L,
    \label{eqn:weight_averaging_arithmetic_with_lowrank}
\end{equation}
% where $\text{SVD}_k(\theta^l)$ denotes the $k$-rank approximation of $\theta^l$, \emph{i.e.,} $\text{SVD}_k(\theta^l) = \sum_{i=1}^k \sigma_i \mathbf{u}_i \mathbf{v}_i^\top$ where $\sum_{i=1}^r \sigma_i \mathbf{u}_i \mathbf{v}_i^\top$ is a singular value decomposition (SVD) of $\theta^l$.
where $\text{SVD}_k(\theta^l)$ denotes the low-rank approximation of $\theta^l$ with top-k singular vectors, \emph{i.e.,} $\text{SVD}_k(\theta^l) = \sum_{i=1}^k \sigma_i \mathbf{u}_i \mathbf{v}_i^\top$ where $\mathbf{u}_i$ and $\mathbf{v}_i$ denote i-th left and right singular vectors obtained by Singular Value Decomposition (SVD), respectively.
% For the non-matrix parameters such as bias or normalization parameters, we apply the vanilla weight averaging.

Figure~\ref{fig:perf_on_ranks} illustrates the average accuracy of the merged model obtained by Eq.~\eqref{eqn:weight_averaging_arithmetic_with_lowrank} with varying rank $k$ (orange solid line).
% We provide the plot of task-wise accuracies in Appendix.
% By increasing the rank from zero, the accuracy starts at the weight averaging accuracy to increase and shows a peak at certain rank, then decreases to returning back to the weight averaging accuracy at full rank (orange line in the figure).
% By increasing the rank from zero to full rank, we observe that the performance rapidly increases from the standard weight averaging, then decreases back to the weight averaging at the full rank. 
As the rank increases from zero to full, we observe a rapid performance improvement beyond standard weight averaging, followed by a decline back to the weight averaging level at full rank.
The accuracies at the endpoints coincide with Eq.~\eqref{eqn:weight_averaging_arithmetic_with_lowrank} since it reduces to weight averaging of Eq.~\eqref{eqn:weight_averaging_arithmetic} when $k=r$ and the summation of task vectors becomes zero when $k=0$.
% However, the "bell-curve" pattern at $0<k<r$ is intriguing since the peak is formed at surprisingly high accuracy, largely outperforming the task arithmetic and even surpasses its advanced variants, such as Ties-Merging~\cite{yadav2024ties} and AdaMerging~\cite{yang2024adamerging}.
However, the "bell-curve" pattern at $0<k<r$ is intriguing since the peak is formed at surprisingly high accuracy, significantly outperforming the task arithmetic~\cite{ilharco2023editing}, its advanced variants such as Ties-Merging~\cite{yadav2024ties} and even the one with test-time adaptation such as AdaMerging~\cite{yang2024adamerging}.
As we show in the experiment (Figure~\ref{fig:ViTB-rank}), the optimal performance is achieved consistently around the same rank ($\approx8\%$) across the tasks and model sizes.


Notably, such properties are only observed when we set the initial point of task vectors as the weight average $\theta_\text{avg}$.
When we replace $\theta_\text{avg}^l$ with the pre-trained parameters $\theta_\text{pre}^l$ in Eq.~\eqref{eqn:weight_averaging_arithmetic_with_lowrank}, the performance consistently decreases as rank reduces, collapsing to the pre-trained parameters at rank zero (blue solid line).
This motivates us to further investigate the spectral components of task vectors.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/average_preserved_rank_semibold.pdf}
    \caption{
    % Average performance of the task arithmetic induced from the weight average with low-rank approximation on task vectors by varying the reducing ranks.
    An average performance of model merging with low-rank approximations of task vectors. $\dagger$ denotes the method with test-time adaptation.
    }
    \label{fig:perf_on_ranks}
\end{figure}


\subsection{Spectral Analysis of Task Vectors}
\label{sec:analysis}

To understand the intriguing properties of weight averaging discussed in Section~\ref{sec:intriguing_properties}, we revisit the weight average $\theta_\text{avg}$ as an initial point of task vectors.
We remark that $\theta_\text{avg}$ is a closed-form solution that minimizes the sum of squared deviations of the induced task vectors.

\begin{remark}
    Let $\theta_1^l, \cdots, \theta_T^l \in \mathbb{R}^{m \times n}$ be real matrices.
    Then $\theta_\text{avg}^l = \frac{1}{T}\sum_{t=1}^T \theta_t^l$ is the solution of the following objective.
    \begin{equation}
        \underset{\theta^l \in \mathbb{R}^{m \times n}}{\textnormal{argmin}} \sum_{t=1}^T \| \theta_t^l - \theta^l \|_F^2,
        \label{eqn:total_variance}
    \end{equation}
    where $\| \cdot \|_F$ denotes the Frobenius norm.
    \begin{proof}
        We leave the proof in Appendix.
    \end{proof}
\end{remark}

This indicates that inducing task vectors from $\theta_\text{avg}$ makes the them as compact as possible, leaving most of the information into $\theta_\text{avg}$.
Therefore, each fine-tuned parameters $\theta_t^l$ are decomposed into the center $\theta_\text{avg}^l$ that encodes the shared knowledge across all tasks and the deviation $\theta_t^l - \theta_\text{avg}^l$ that encodes task-specific knowledge (see also Figure~\ref{fig:concept_figure}).
\begin{equation}
    \theta_t^l = \underbrace{\theta_\text{avg}^l}_{\text{shared center}} + \underbrace{(\theta_t^l - \theta_\text{avg}^l)}_{\text{per-task deviation}}
\end{equation}
However, performing the arithmetic (Eq.~\eqref{eqn:weight_averaging_arithmetic}) directly on the induced task vectors introduce severe interference between the parameters.
By summing the zero-centered deviations, task-specific knowledge is catastrophically forget, which makes Eq.~\eqref{eqn:weight_averaging_arithmetic} equal to Eq.~\eqref{eqn:weight_averaging}.
To avoid the catastrophic forgetting, we should filter out the noisy components from the task vectors.

Thanks to the compact decomposition, low-rank approximation of task vectors plays a crucial role.
From Eq.~\eqref{eqn:total_variance}, high-rank components that are commonly relevant to solving the tasks have been already separated to the center $\theta_\text{avg}$.
Then in the task vectors, most of the relevant knowledge can be efficiently contained in low-rank components, while remaining high-rank components mainly contains \emph{noisy} knowledge possibly comes from the randomness of fine-tuning.
This explains the intriguing "bell-curve" pattern of Figure~\ref{fig:perf_on_ranks}.
The accuracy increases at low-rank area because the task-relevant low-rank components are likely to be mutually orthogonal in the high-dimensional matrix space.
Also, the accuracy decreases at high-rank area since the noisy high-rank components are continuously added, which ends with catastrophic forgetting at full rank.
The peak accuracy around 8\% of the preserved rank comes from taking the best trade-off between including task-relevant components and filtering noisy components.


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/average_preserved_rank_semibold_reversed_nolegend.pdf}
        \caption{Task arithmetic with reversed rank reduction}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/average_preserved_rank_semibold_single_nolegend.pdf}
        \caption{Task vector with rank reduction}
        \label{fig:subfig2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/average_preserved_rank_semibold_reversed_single.pdf}
        \caption{Task vector with reversed rank reduction}
        \label{fig:subfig3}
    \end{subfigure}
    \caption{A figure with three subfigures aligned horizontally.}
    \label{fig:three_subfigures}
\end{figure*}



\subsection{Model Merging with \ours{}}
\label{sec:our_approach}

Based on the previous discussions, we propose a training-free model merging approach called \ours{}.
The method is simple; given $T$ parameters $\theta_1, \cdots, \theta_T$, we apply  Eq.~\eqref{eqn:weight_averaging_arithmetic_with_lowrank} for each layer $\theta^l$ that consists of matrix parameters, while applying simple averaging for the others.
While this introduces an additional hyper-parameter, the preserved rank $k$, retaining 8\% of the rank yields stable performance across different settings.

Since the re-definition of task vectors is general, \ours{} can be plugged in any merging method that leverages the task arithmetic framework.
For example, AdaMerging~\cite{yang2024adamerging} exploits test-time adaptation to improve the performance.
In this variant, rather than using a global merging coefficient $\lambda$, we use task-wise and layer-wise coefficients $\lambda_t^l$ and learn them by minimizing the Shannon entropy on test data.
Combined with this variant, Eq.~\eqref{eqn:weight_averaging_arithmetic_with_lowrank} can be transformed into
\begin{equation}
    \theta_{*-\text{Ada}}^l = \theta_\text{avg}^l + \sum_{t=1}^T \lambda_t^l \cdot  \text{SVD}_k(\theta_t^l - \theta_\text{avg}^l), \quad \forall~ l \le L,
    \label{eqn:weight_averaging_arithmetic_with_lowrank_adamerging}
\end{equation}
which we call \ours{}-Ada in our experiments.

==> sec/backups/2_method_old.tex <==
% \section{Problem Definition and Previous Works}
% \begin{comment}
%     model merging은 이다.. 더욱 specifically, 같은 architecture의 model에 대하여 T개의 task에 대하여 각각이 $\{\theta_t \}_{t=1}^{T}$로 paramterized된 finentuend models $\{f(x; \theta_t)\}_i^{}$을 잘 조합하여 T개의 task를 잘 수행하는 weight $\theta$를 찾고자 한다.

% \end{comment}

\section{Methodology}

\subsection{Problem Definition and Notation}
\paragraph{Model Merging}
Model merging aims to create a unified model that can perform multiple downstream tasks by combining individual models trained on each task. Given $T$ tasks, each task $t$ has a fine-tuned model $f(x; \theta_t)$ parameterized by $\theta_t$, where $x$ represents the input data, $y$ the output label, and $ \theta $ the model parameters. The objective is to find a combination $\theta_{*}$ of these task-specific weights $\theta_t$ such that the resulting model $f(x; \theta_{*})$ can perform well across all $T$ tasks.
\citet{ilharcoEditingModelsTask2023} proposed the concept of a \textit{task vector}, defined as $\tau_t := \theta_t - \theta_{\text{pre}}$, where $\theta_{\text{pre}}$ represents pretrained weights. Following this, a basic model merging approach can be represented as $\theta_{*} = \theta_{\text{pre}} + \sum_{t=1}^{T} \lambda_{t} \tau_t$. While straightforward and effective, this method often suffers from task interference, which limits performance. Previous work has attempted to mitigate this by either refining $\tau_t$ \cite{yadavTIESMergingResolvingInterference2023} or optimizing $\lambda_t$ \cite{yangAdaMergingAdaptiveModel2024a} through test-time adaptation. \cite{wangTentFullyTesttime2021}

In contrast, rather than addressing task interference by relying on fixed $\theta_{\text{pre}}$, we propose decomposing the parameters of $\{\theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T}\}$ into shared parameters, $\theta_{\text{shared}}$, and task-specific parameters, $\{\tau'_{1}, \dots, \tau'_{T}\}$. This approach effectively reduces task interference and enhances model merging performance.

\begin{comment}
    Model merging aims to create a unified model that can perform multiple downstream tasks by combining individual models trained on each task. Given $T$ tasks, each task $t$ has a fine-tuned model $f(x; \theta_t)$ parameterized by $\theta_t$, where $x$ represents the input data, $y$ the output label, and $ \theta $ the model parameters. The objective is to find a combination $\theta_{*}$ of these task-specific weights $\theta_t$ such that the resulting model $f(x; \theta_{*})$ can perform well across all $T$ tasks.
    \cite{ilharcoEditingModelsTask2023}가 제시한 task vector, $\tau_t := \theta_t \theta_{pre}\$, \theta_{pre}는 pretrained weight 개념을 따라서 가장 naive한 model merging은 $\theta_{*} = \theta_{pre} + \sum_{t}^{T} \lambda_{t} \tau_t$로서 될 수 있다. 매우 간단하고 효과적이나 task interference로 인하여 높은 성능으 아니기에, 이전의 work들은 \tau_t에 대한 가공을 하거나 \citet{yadavTIESMergingResolvingInterference2023} test time adaptation \cite{wangTentFullyTesttime2021}을 통해서 $\lambda_t$를 찾는 방법을 제시하였다. \cite{yangAdaMergingAdaptiveModel2024a}
    그러나, 우리는 고정된 $\theta_{pre}$에서 이를 다루는 것이 아닌, $\{ \theta_{pre}, \theta_{1}, ..., \theta_{T}\}$ shared parameter $\theta_{shared}$와 task specific parmeters $\{ \tau^{'}_{1}, ..., \tau^{'}_{T}\}$로 parameter를 다시 분해하여 결과적으로, task interference를 줄이고 model merging의 성능을 높힌다. 
\end{comment}

% 아래 부분 부터는 우리 method를 적용하기 위한 방법론을 세세하게 작성하도록 한다.
% 여기 block이 너무 뜬금 없어서, 일단은 필요한 내용을 라면 레시피로 다 적고 레고처럼 싹싹 맞춰서 쓰도록 하자.
% \paragraph{Notations}
% % 이거 조금 뜬금 없기는 하다.
% 여기는 각 내용 설명하면서 녹여내도 될 듯하다.
% To facilitate the following discussion, we define several key notations. For layer-wise parameterization of each parameter set $\{ \theta_{\text{pre}}, \theta_{1}, \dots, \theta_{T} \}$, we represent $\theta_i$ as $\theta_i := \{ \theta_{i}^{1}, \theta_{i}^{2}, \dots, \theta_{i}^{L} \}$. Additionally, for test-time adaptation, we assume an unlabeled test data distribution per task, denoted as $\{\mathcal{D}^{\text{test}}_{t}\}_{t=1}^{T}$, with input $x \in \mathcal{D}^{test}_t$.

\begin{comment}
    - 이후의 논의를 위해서 몇가지 notation을 정의하도록 한다.
    - 각 파라미터  $\{ \theta_{pre}, \theta_{1}, ..., \theta_{T}\}$의 layer wise한 parameterization을 하기 위해서, \theta_i := {\theta_{i}^{1}, \theta_{i}^{2}, ..., \theta_{i}^{L}}로서 정의한다.
    - test time adaptation을 위해서, unlabeled test data distribution $\{\mathcal{D}^{test}_{t} \}_{t=1}^{T}, x \in \mathcal{D}_t $을 per task를 상정한다.

\end{comment} 
% 앞 문단과 너무 간극이 있는 연결 지점이다. 이 부분은 다시 한번 생각해보도록 하자.
% 내용을 갈아 엎기는 해야 되는데 일단 seed가 있어야 갈아 엎으니까 일단은 작성한다.
\subsection{Model Merging with Similiarity Minimization (SimMin)}
\paragraph{Similiarity Minimization}
Building on the observation that task vectors across different tasks are nearly orthogonal, which suggests the possibility of task arithmetic \cite{ilharcoEditingModelsTask2023}, we optimize $\theta_{\text{shared}}$ according to Equation \ref{eqn: sim_min} to minimize the similarity between task-specific parameters, defined as $\tau'_{t} = \theta_{t} - \theta_{\text{shared}}$.
\begin{comment}
    다른 task간의 task vector가 거의 orthogonal하다는 사실과 이것에 의해서 task arithmetic이 가능할 수 도 있다는 추측으로부터 \cite{ilharcoEditingModelsTask2023}, task specific parameters $\tau^{'}_{t} = \theta_{t} -\theta_{shared}$간에 similiarity가 작아지도록  $\theta_{shared}$을 Equation \ref{eqn: sim_min}으로 optimize하였다. 
    To mitigate task interference, we aim to find a shared parameter $\theta_{shared}$ that reduces the similarity among task-specific parameters, defined as $\tau'_{t} = \theta_{t} - \theta_{shared}$ by optimizing the Equation \ref{eqn: sim_min}.
    % 뭔가 아전인수 격으로 orthogonal한게 좋다고 썼는데, trivial한 근거가 있어야 한다.
    % objective가 왜 이것이 되어야 하는가? 여기에 논리가 없다.
\end{comment}

\begin{equation}\label{eqn: sim_min}
    \theta_{shared}^{l} = \underset{\theta^{l}}{\arg\min} \sum_{i=1}^{T} \sum_{j<i}^{T} \langle (\tau'_{i}, \tau'_{j} \rangle_{F}
\end{equation}

Equation \ref{eqn: sim_min} has an analytic solution, given by $\theta_{\text{shared}} = \frac{1}{T} \sum_{t=1}^{T} \theta_t$, which represents the average of the task weights. However, using this $\theta_{\text{shared}}$ and $\{\tau'_{t}\}$ to perform model merging as $\theta_{*} = \theta_{\text{shared}} + \sum_{t} \lambda_{t} \tau'_{t}$ results in significant task interference, leading to reduced performance. Empirical analysis revealed that the effective rank of matrix components within $\{\tau'_{t}\}$, such as the weights of MLP modules, is notably low. Based on the assumption that non-dominant eigenvectors contribute to task interference, we explicitly pruned the rank of these matrix components in $\{\tau'_{t}\}$. As demonstrated in Figure \ref{fig:rank_min}, ensuring that task-specific parameters maintain an appropriate rank effectively reduces task interference.

\begin{comment}
    이때, Equation \ref{eqn: sim_min}은 analytic solution이 존재하며 $\theta_{shared} = 1/T \sum_{t=1}^{T} \theta_t$이고 이는 task weight들의 평균이다. 하지만, 이렇게 얻은 $\theta_{shared}, \{\tau'_{t}\}$를 이용하여 $\theta_{*} = \theta_{shared} + \sum_{t} \lambda_{t} \{\tau'_{t}\}$로 model merging을 수행할 경우, 상당한 task interference로 낮은 성능을 낸다. 우리는 실험적으로 $\{tau'_{t} \}$중에서 matrix component들의 effective rank가 매우 낮다는 점을 확인하였고, 따라서 non-dominant eigenvectors가 task interference를 초래할 것이라는 가정하에, $\{\tau'_{t}\}$에서 matrix component들(예를 들어, mlp module의 weight 같은)의 rank를 explicit하게 pruning을 하였고 Figure \ref{fig:rank_min}로부터 task specific parmeter가 적절한 rank를 지니는 것이 task interference를 줄이는데 효과적임을 확인하였다. 
    $\theta_{*} = \theta_{shared} + \sum_i^{T} \lambda_{i}^{l} \tau_^{'}_{t} $
    % effective 낮다는 점은 table로 보여야 할지?
    % 아녀 effective rank가 낮은거랑, non-dominant eigenvectors가 task interference를 초래할 것이 어떻게 연결되는가?
    % 적절한 rank를 어떻게 결정해야 하는데...?
\end{comment}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{./fig/avg_is_all_you_need.png}
    \caption{Rank Minimization Example}
    \label{fig:rank_min}
\end{figure}


\paragraph{Test Time Adaptation}
\begin{comment}
    이렇게 형성된 task specific parameter를 이용해서 test time adaptation을 수행할 경우, model merging에 있어서 SOTA를 보일 수 있다.
\end{comment}

\begin{algorithm}
    \caption{Adaptive Merging with SimMin}
    \label{alg:ada_sim}
    \begin{algorithmic}[1]
    \INPUT $\{ \theta_{pre}, \theta_{1}, ..., \theta_{T} \}$, $\{ \mathcal{D}^{test}_{t} \}_{t=1}^{T}$
    \OUTPUT $\theta_{*}$
    \STATE Initialize $\theta_{shared}, \{ \{ \lambda_{t}^{l} \}_{l} \}_t$

    \COMMENTTRIANGLE{Similiarity Minimization}

    % \STATE $\theta_{shared}$ \gets 

    \FOR{each task $t$}
        \STATE Compute task-specific parameter $\theta_{t}$
        \STATE Perform similarity minimization for $\theta_{t}$
    \ENDFOR

    \COMMENTTRIANGLE{Test Time Adaptation}
    % 
    \STATE Merge models: $\theta_{*} = \theta_{shared} + \sum_{i=1}^{T} \lambda_{i}^{l} \tau_{t}^{'}$
    \STATE Perform test time adaptation using $\theta_{*}$ and $\mathcal{D}_{t}$
    \RETURN $\theta_{*}$
    \end{algorithmic}
\end{algorithm}

\begin{comment}

\end{comment}

\begin{comment}
    to sum up, ours method can be simply represmnt as algorith \ref{alg: ours_model_fusion}
\end{comment}

\paragraph{Test Time Adaptation}
\begin{comment}
    약간의 task specific parameter와 2번의 inference가 가능하다는 relaxation에서 
\end{comment}


\subsection{Mixture of Expert (MoE) with Rank Minimization}

\begin{comment}
to sum up, 우리의 전반적인 알고리즘은 다음과 같이 구성될 수 있다.
\end{comment}



\begin{comment}
    글의 전체 전개 순서를 다음과 같이 가져가고 싶다.
    - 문제 정의와 기존의 work들의 방법론

    - rank minimization, similiarity minimization




\end{comment}

==> sec/backups/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/tables/main_table_1.tex <==
\begin{table*}[ht]
    % TODO 1: [ ] 빨리 수정 하셔요~
    % CARS 성능이 너무 떨어져서 어쩔 수 없음
    % is_perpect: True
      \small
      \centering
      \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}}         & \multicolumn{3}{c}{ViT-B-32}                     & \multicolumn{3}{c}{ViT-L-14}                    \\ 
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
                                                 & 8 tasks & 14 tasks          & 20 tasks           & 8 tasks & 14 tasks          & 20 tasks          \\ 
        \midrule
        \multicolumn{1}{c}{Pretrained}            & $48.0$ & $57.1$ & $56.0$ & $65.0$ & $68.4$ & $65.4$ \\
        \multicolumn{1}{c}{Individual}            & $90.5$ & $89.6$ & $90.5$ & $94.2$ & $93.3$ & $94.1$ \\
        \midrule
        \multicolumn{7}{c}{Without Test-Time-Adaptation} \\
        \midrule
        \multicolumn{1}{c}{Weight Averaging}      & $65.9$ & $64.3$ & $61.0$& $79.6$ & $76.8$ & $71.7$ \\
        \multicolumn{1}{c}{Task Arithmetic~\cite{ilharco2023editing}}       & $69.1$ & $65.4$& $60.5$ & $84.5$ & $79.6$ & $74.2$ \\
        \multicolumn{1}{c}{Ties-Merging~\cite{yadav2024ties}}          & $72.4$ & $65.2$& $62.9$ & $86.1$ & $79.5$& $75.8$\\
        \multicolumn{1}{c}{Consensus TA~\cite{wang2024localizing}}        & $75.2$ & $70.0$& $62.9$ & $86.6$& $81.9$& $78.8$\\
        \multicolumn{1}{c}{\textbf{\ours{} (Ours)}}                 & $\mathbf{84.7}$ & $\mathbf{79.5}$& $\mathbf{76.3}$& $\mathbf{92.6}$ & $\mathbf{88.7}$& $\mathbf{87.9}$\\
        \midrule
        \multicolumn{7}{c}{With Test-Time-Adaptation} \\
        \midrule
        \multicolumn{1}{c}{Adamerge+TA~\cite{yang2024adamerging}}            & $80.1$ & $76.7$ & $69.2$ & $90.8$& $88.0$ & $86.8$ \\
        \textbf{Adamerge+\ours{} (Ours)}               & $\mathbf{85.8}$ & $\mathbf{82.3}$ & $\mathbf{82.7}$ & $\mathbf{93.1}$ & $\mathbf{90.4}$ & $\mathbf{91.3}$ \\
        \bottomrule
      \end{tabular}
      \caption{Average absolute accuracy results on 8, 14 and 20 vision tasks model merging benchmark.}
      \label{tab:task_specific}
    \end{table*}

% TODO 2: [X] table을 분리해서 Model Merging, Model Merging with TTA, Model Selection with Indexing 으로 3개의 table로서 구성하되, 공간 절약을 위해서 쓸모없는 reference는 전부 배제해버리고 SOTA model에 대해서만 비교하도록 한다. 다한, table 형성 시에는 TA-32와 TA-14을 합치고 appendix 부분에 대하여, full table, NLP case에 대해서 진술토록 한다.
% TODO 2: [ ] 조졌다.. TSV가 너무 잘해서 8개를 최대한 강조하고 14, 20개는 평균을 내서 진술을 해야 한다...
% 다만 여전히 TTA 기법이 잘 먹힘을 진술하고, 저자들이 햇갈리지 않도록 only one merged model을 유지함을 꼭꼭 다시 discussion에서 진술하도록 한다.


==> sec/tables/main_table_2.tex <==
\begin{table*}[ht]
    \centering
    \caption{Multi-Task Performance on Eight Vision Tasks with Merged ViT-L-14 with CART.}
    \small
    \label{tab:method_comparison_large}
    \begin{tabular}{l| c c c c c c c c|c}
        \toprule
        \textbf{Method} & \textbf{SUN397} & \textbf{Cars} & \textbf{RESISC45} & \textbf{EuroSAT} & \textbf{SVHN} & \textbf{GTSRB} & \textbf{MNIST} & \textbf{DTD} & \textbf{Average} \\
        \midrule
        Pretrained & 66.8 & 77.7 & 71.0	& 59.0 & 58.4 & 50.5 & 76.3	& 55.3	& 64.5 \\
        Individual & 82.3 & 92.4 & 97.4	& 100.0	& 98.1	& 99.2	& 99.7	& 84.1	& 94.2 \\
        Traditional MTL & 80.8	& 90.6	& 96.3	& 96.3	& 97.6	& 99.1	& 99.6	& 84.4	& 93.5 \\
        \midrule
        \multicolumn{10}{c}{Without Test-Time-Adaptation}\\
        \midrule
        Weight Averaging & 72.1	& 81.6	& 82.6	& 91.9	& 78.2	& 70.7	& 97.1	& 62.8	& 79.6 \\
        Fisher Merging~\cite{matena2022merging} & 69.2	& 88.6	& 87.5	& 93.5	& 80.6	& 74.8 &	93.3	& 70.0	& 82.2 \\
        RegMean~\cite{jin2023regmean} & 73.3	& 81.8	& 86.1	& 97.0	& 88.0	& 84.2	& 98.5	& 60.8	& 83.7\\
        \midrule
        Task Arithmetic~\cite{ilharco2023editing} & 73.9	& 82.1	& 86.6	& 94.1	& 87.9	& 86.7 &	98.9	& 65.6 & 84.5\\
        Ties-Merging~\cite{yadav2024ties} & 76.5	& 85.0	& 89.3 & 95.7 & 90.3 & 83.3 & 99.0 & 68.6 & 86.0\\
        Consensus-Ties & 74.9 & 83.6 & 88.7 & 96.6 & 90.5 & 93.2 & 99.1 & 71.1 & 87.2 \\
        \textbf{\ours{} (Ours)} & \textbf{79.3} & \textbf{90.4} & \textbf{95.4} & \textbf{99.3} & \textbf{96.1} & \textbf{98.3} & \textbf{99.6} & \textbf{82.5} & \textbf{92.6} \\
        \midrule
        \multicolumn{10}{c}{With Test-Time-Adaptation}\\
        \midrule
        AdaMerging~\cite{yang2024adamerging} & 79.0	& 90.3	& 90.8	& 96.2	& 93.4	& 98.0	& 99.0	& 79.9	& 90.8 \\
        AdaMerging++~\cite{yang2024adamerging} & 79.4	& 90.3	& 91.6	& 97.4	& 93.4	& 97.5	& 99.0 &	79.2	& 91.0 \\
        \textbf{\ours{}++ (Ours)}  & \textbf{80.1} & \textbf{91.5} & \textbf{94.7} & \textbf{99.3} & \textbf{96.8} & \textbf{98.9} & \textbf{99.5} & \textbf{83.6} & \textbf{93.1} \\
        \bottomrule
    \end{tabular}
\end{table*}

\begin{comment}
    ㅋㅋㅋㅋ 다행이다. 8개에 대해서는 진짜 잘하네
\end{comment}

==> sec/tables/sub_table_roberta.tex <==
\begin{table*}[ht]
    \small
    \centering
    % is_perpect: True
    \caption{Multi-Task Performance on Eight NLP Tasks with Merged roBERTa-base with CART.}
    \begin{tabular}{l | c c c c c c c c | c}
        \toprule
        Method           & CoLA   & SST2   & MRPC   & STSB   & QQP    & MNLI   & QNLI   & RTE    & \textbf{Avg.} \\
        \midrule
        Individual       & 0.6018 & 0.9404 & 0.8922 & 0.9063 & 0.9141 & 0.8720 & 0.9271 & 0.7906 & 0.8556        \\
        \midrule
        Weight Averaging & 0.1396 & 0.6411 & 0.6936 & 0.3184 & 0.7536 & 0.4219 & 0.5870 & 0.5523 & 0.5134        \\
        Task Arithmetic  & 0.1878 & 0.8589 & 0.7990 & 0.7403 & 0.8378 & 0.5908 & 0.6967 & 0.6209 & 0.6665        \\
        Ties-Merging     & 0.2048 & 0.8440 & 0.8113 & 0.5819 & \textbf{0.8570} & \textbf{0.6465} & 0.7481 & 0.4296 & 0.6404        \\
        \textbf{\ours{} (Ours)} & \textbf{0.3294} & \textbf{0.9243} & \textbf{0.8284} & \textbf{0.7956} & 0.8225 & 0.5137 & \textbf{0.7985} & \textbf{0.6498} & \textbf{0.7078}        \\
        \bottomrule
    \end{tabular}
    \label{tab:roberta}
\end{table*}

% \begin{table}[ht]
%     \scriptsize
%     \caption{Multi-Task Performance on Eight NLP Tasks with Merged roBERTa-base with CART.}
%     \label{tab:roberta}
%     \begin{tabular}{l|ccccc}
%         \toprule
%         Task    & Individual & Weight Averaging & Task Arithmetic & Ties-Merging & \ours{} \\
%         \midrule
%         CoLA    & 0.6018     & 0.1396           & 0.1878          & 0.2048       & 0.3294  \\
%         SST2    & 0.9404     & 0.6411           & 0.8589          & 0.8440       & 0.9243  \\
%         MRPC    & 0.8922     & 0.6936           & 0.7990          & 0.8113       & 0.8284  \\
%         STSB    & 0.9063     & 0.3184           & 0.7403          & 0.5819       & 0.7956  \\
%         QQP     & 0.9141     & 0.7536           & 0.8378          & 0.8570       & 0.8225  \\
%         MNLI    & 0.8720     & 0.4219           & 0.5908          & 0.6465       & 0.5137  \\
%         QNLI    & 0.9271     & 0.5870           & 0.6967          & 0.7481       & 0.7985  \\
%         RTE     & 0.7906     & 0.5523           & 0.6209          & 0.4296       & 0.6498  \\
%         \midrule
%         Average & 0.8556     & 0.5134           & 0.6665          & 0.6404       & 0.7078  \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table*}[ht]
    \small
    \centering
    % is_perpect: True
    \caption{Additional result of eight NLP tasks with model compression benchmark. For \oursindexing{}, we retain 8% rank.}
    \begin{tabular}{l | c c c c c c c c | c}
        \toprule
        Method           & CoLA   & SST2   & MRPC   & STSB   & QQP    & MNLI   & QNLI   & RTE    & \textbf{Avg.} \\
        \midrule
        Individual       & 0.6018 & 0.9404 & 0.8922 & 0.9063 & 0.9141 & 0.8720 & 0.9271 & 0.7906 & 0.8556        \\
        \midrule
        \textbf{EMR-merge} & \textbf{0.3294} & \textbf{0.9243} & \textbf{0.8284} & \textbf{0.7956} & 0.8225 & 0.5137 & \textbf{0.7985} & \textbf{0.6498} & \textbf{0.7078}        \\
        \textbf{\ours{} (Ours)} & \textbf{0.3294} & \textbf{0.9243} & \textbf{0.8284} & \textbf{0.7956} & 0.8225 & 0.5137 & \textbf{0.7985} & \textbf{0.6498} & \textbf{0.7078}        \\
        \bottomrule
    \end{tabular}
    \label{tab:roberta}
\end{table*}
